Hilbert's epsilon as an Operator of Indefinite Committed Choice

Paul Bernays and David Hilbert carefully avoided overspecification of Hilbert's epsilon-operator and axiomatized only what was relevant for their proof-theoretic investigations. Semantically, this left the epsilon-operator underspecified. In the meanwhile, there have been several suggestions for semantics of the epsilon as a choice operator. After reviewing the literature on semantics of Hilbert's epsilon operator, we propose a new semantics with the following features: We avoid overspecification (such as right-uniqueness), but admit indefinite choice, committed choice, and classical logics. Moreover, our semantics for the epsilon supports proof search optimally and is natural in the sense that it does not only mirror some cases of referential interpretation of indefinite articles in natural language, but may also contribute to philosophy of language. Finally, we ask the question whether our epsilon within our free-variable framework can serve as a paradigm useful in the specification and computation of semantics of discourses in natural language.

==> header12pt.tex <==
%Math Notation
% \mathcommand\oast{\mathchoice
%              {{\oplus\hskip-9.15pt \otimes}}%     display-style
%              {{\oplus\hskip-9.15pt \otimes}}%     text-style
%              {{\oplus\hskip-6.60pt \otimes}}%     scriptstyle
%              {{\oplus\hskip-5.65pt \otimes}}%     scriptscriptstyle
% }
% \mathcommand\footnoteoast{{\footnotesize\mathchoice
%              {{\oplus\hskip-7.80pt \otimes}}%     display-style
%              {{\oplus\hskip-7.80pt \otimes}}%     text-style
%              {{\oplus\hskip-6.15pt \otimes}}%     scriptstyle
%              {{\oplus\hskip-5.50pt \otimes}}%     scriptscriptstyle
% }}
\mathcommand\notconflu{\mathchoice
             {{\hskip1.5pt\nmid\hskip-4.697545pt\downarrow}}%   display-style
             {{\hskip1.5pt\nmid\hskip-4.65pt\downarrow}}   %   text-style
             {{\hskip1pt\nmid\hskip-3.494pt\downarrow\hskip1pt}}  
                                                         %   scriptstyle
             {{\hskip1pt\nmid\hskip-3.01pt\downarrow\hskip0.5pt}}   
                                                         %   scriptscriptstyle
%             {{\nmid\hskip-6pt\downarrow}}     %     display-style
%             {{\nmid\hskip-6pt\downarrow}}     %     text-style
%             {{\nmid\hskip-4.25pt\downarrow}}  %     scriptstyle
%             {{\nmid\hskip-3.85pt\downarrow}}  %     scriptscriptstyle
}
% \mathcommand\footnotenotconflu{{\footnotesize\mathchoice
%              {{\nmid\hskip-5.54pt\downarrow}}%5.5-5.55   display-style
%              {{\nmid\hskip-5.54pt\downarrow}}%5.51-5.55    text-style
%              {{\nmid\hskip-4.0pt\downarrow}}%4.0-4.05   scriptstyle
%              {{\nmid\hskip-3.6pt\downarrow}}%3.5    scriptscriptstyle
% }}
\mathcommand\redpara{\mathchoice
           {{\redsimple\hskip-16pt  \shortparallel}\hskip8.5pt}%display-style
           {{\redsimple\hskip-16pt  \shortparallel}\hskip8.5pt}%text-style
           {{\redsimple\hskip-8.5pt \shortparallel}\hskip6pt}%scriptstyle
           {{\redsimple\hskip-7.5pt \shortparallel}\hskip5pt}%scriptscriptstyle
}
\mathcommand\antiredpara{\mathchoice
           {{\antired\hskip-14.6pt  \shortparallel}\hskip7pt}%display-style
           {{\antired\hskip-14.6pt  \shortparallel}\hskip7pt}%text-style
           {{\antired\hskip-8.pt \shortparallel}\hskip5pt}%scriptstyle
           {{\antired\hskip-7.pt \shortparallel}\hskip5pt}%scriptscriptstyle
}
\mathcommand\revpara{\mathchoice
           {{\redsimple\hskip-16pt  \infty}\hskip4.8pt}%display-style
           {{\redsimple\hskip-16pt  \infty}\hskip4.8pt}%text-style
           {{\redsimple\hskip-11.5pt\infty}\hskip4pt}%scriptstyle
           {{\redsimple\hskip-9.9pt \infty}\hskip3pt}%scriptscriptstyle
}
\mathcommand\antirevpara{\mathchoice
           {{\antired\hskip-15.4pt\infty}\hskip4pt}%display-style
           {{\antired\hskip-15.4pt\infty}\hskip4pt}%text-style
           {{\antired\hskip-10.8pt\infty}\hskip3pt}%scriptstyle
           {{\antired\hskip-9.5pt \infty}\hskip3pt}%scriptscriptstyle
}
\mathcommand\simpara{\mathchoice%this needs more fixing
           {{\redsimple\hskip-13pt  \circ}\hskip7pt}%display-style
           {{\redsimple\hskip-13pt  \circ}\hskip7pt}%text-style
           {{\redsimple\hskip-11.5pt\circ}\hskip4pt}%scriptstyle
           {{\redsimple\hskip-9.9pt \circ}\hskip3pt}%scriptscriptstyle
}


==> headerarticle.tex <==
\setcounter{tocdepth}{2}

\newlength{\sectionintocsep} %separation for section line in table of contents
\setlength{\sectionintocsep}{1.9\topsep}

\newlength{\contentsandreferencesheadroom} %room over line ``Contents''
\setlength{\contentsandreferencesheadroom}{0em}
%{2.0\topsep}

\newlength{\contentsandreferencesfootroom} %room under line ``Contents''
\setlength{\contentsandreferencesfootroom}{2.0\topsep}

\catcode`\@=11

% \tableofcontents <----------
\def\tableofcontents{\ignorespaces
%\vspace*\contentsandreferencesheadroom
\section*{\contentsname\@mkboth
{\uppercase{\contentsname}}{\uppercase{\contentsname}}}%
\vspace*\contentsandreferencesfootroom
\@starttoc{toc}}
\def\contentsname{Contents} % <----------
% \def\tableofcontents{\section*{Contents\@mkboth{CONTENTS}{CONTENTS}}
% \@starttoc{toc}}

\catcode`\@=12


==> headerhot.tex <==
\def\subsubsubsection{\paragraph}
\catcode`\@=11
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\font\sixsf  = cmss10 scaled 600
\font\fvesf  = cmss10 scaled 500
%\font\sevsf  = cmss10 scaled 700
\font\egtsf  = cmss10 scaled 800
%\font\twfvit  = cmti10   \@magscale5 % text italic

\def\xiipt{\textfont\z@\twlrm 
  \scriptfont\z@\egtrm \scriptscriptfont\z@\sixrm
\textfont\@ne\twlmi \scriptfont\@ne\egtmi \scriptscriptfont\@ne\sixmi
\textfont\tw@\twlsy \scriptfont\tw@\egtsy \scriptscriptfont\tw@\sixsy
\textfont\thr@@\tenex \scriptfont\thr@@\tenex \scriptscriptfont\thr@@\tenex
\def\unboldmath{\everymath{}\everydisplay{}\@nomath\unboldmath
          \textfont\@ne\twlmi 
          \textfont\tw@\twlsy \textfont\lyfam\twlly
          \@boldfalse}\@boldfalse
\def\boldmath{\@ifundefined{twlmib}{\global\font\twlmib\@mbi\@magscale1\global
        \font\twlsyb\@mbsy \@magscale1\global\font
         \twllyb\@lasyb\@magscale1\relax\@addfontinfo\@xiipt
              {\def\boldmath{\everymath
                {\mit}\everydisplay{\mit}\@prtct\@nomathbold
                \textfont\@ne\twlmib \textfont\tw@\twlsyb 
                \textfont\lyfam\twllyb\@prtct\@boldtrue}}}{}\@xiipt\boldmath}%
\def\prm{\fam\z@\twlrm}%
\def\pit{\fam\itfam\twlit}\textfont\itfam\twlit \scriptfont\itfam\egtit
   \scriptscriptfont\itfam\sevit
\def\psl{\fam\slfam\twlsl}\textfont\slfam\twlsl 
     \scriptfont\slfam\tensl \scriptscriptfont\slfam\tensl
\def\pbf{\fam\bffam\twlbf}\textfont\bffam\twlbf 
   \scriptfont\bffam\ninbf \scriptscriptfont\bffam\ninbf 
\def\ptt{\fam\ttfam\twltt}\textfont\ttfam\twltt
   \scriptfont\ttfam\nintt \scriptscriptfont\ttfam\nintt 
\def\psf{\fam\sffam\twlsf}\textfont\sffam\twlsf
    \scriptfont\sffam\egtsf \scriptscriptfont\sffam\sixsf
\def\psc{\@getfont\psc\scfam\@xiipt{\@mcsc\@magscale1}}%
\def\ly{\fam\lyfam\twlly}\textfont\lyfam\twlly 
   \scriptfont\lyfam\egtly \scriptscriptfont\lyfam\sixly
 \@setstrut \rm}

\def\xxvpt{\textfont\z@\twfvrm 
  \scriptfont\z@\twtyrm \scriptscriptfont\z@\svtnrm
\textfont\@ne\twtymi \scriptfont\@ne\twtymi \scriptscriptfont\@ne\svtnmi
\textfont\tw@\twtysy \scriptfont\tw@\twtysy \scriptscriptfont\tw@\svtnsy
\textfont\thr@@\tenex \scriptfont\thr@@\tenex \scriptscriptfont\thr@@\tenex
\def\unboldmath{\everymath{}\everydisplay{}\@nomath\unboldmath
        \textfont\@ne\twtymi \textfont\tw@\twtysy \textfont\lyfam\twtyly
        \@boldfalse}\@boldfalse
\def\boldmath{\@subfont\boldmath\unboldmath}%
\def\prm{\fam\z@\twfvrm}%
\def\pit{\fam\z@\twfvit}%
\def\psl{\@subfont\sl\rm}%
\def\pbf{\@getfont\pbf\bffam\@xxvpt{cmbx10\@magscale5}}%
\def\ptt{\@subfont\tt\rm}%
\def\psf{\@subfont\sf\rm}%
\def\psc{\@subfont\sc\rm}%
\def\ly{\fam\lyfam\twtyly}\textfont\lyfam\twtyly 
   \scriptfont\lyfam\twtyly \scriptscriptfont\lyfam\svtnly 
\@setstrut \rm}

\catcode`\@=12


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SUPERCOMMANDS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% The following redefines the latex macro \math not because 
% \math makes trouble but rather because I dont like it
\long\def\math#1{\relax\ifmmode{#1}\else$#1 $\fi}
%                                          ^ 
% This blank is necessary because otherwise \math{} may expand to $$
% which is different from $ $ insofar as it starts a displaymath environment 
\long\def\nomath#1{\relax\ifmmode\mbox{#1}\else{#1}\fi}
\newcommand\nlbmath[1]{\nolinebreak\math{#1}}
\newcommand\maths[2]{\math{#1#2}}
\newcommand\nlbmaths[2]{\nolinebreak\math{#1#2}}
%The fol. defines \mathcommand to work like \newcommand with the exception of 
%switching to math-mode iff the command is not called in math-mode.
%\remathcommand is like \renewcommand.

\catcode`\@=11

\long\def\@reargdefmath#1[#2]#3{\@reargdef#1[#2]{\math{#3}}}

\long\def\@argdefmath#1[#2]#3{\@ifdefinable #1{\@reargdefmath#1[#2]{#3}}}

\def\mathcommand#1{\@ifnextchar [{\@argdefmath#1}{\@argdefmath#1[0]}}

\def\remathcommand#1{\edef\@tempa{\expandafter\@cdr\string
  #1\@nil}\@ifundefined{\@tempa}{\@latexerr{\string#1\space undefined}\@ehc
    }{}\@ifnextchar [{\@reargdefmath#1}{\@reargdefmath#1[0]}}

\catcode`\@=12

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\mathapplycommand      
#1#2{\mathcommand{#1}[1]{{#2}({##1})}}
\def\mathdoubleapplycommand
#1#2{\mathcommand{#1}[2]{{#2}({##1},{##2})}}
\def\mathtripleapplycommand
#1#2{\mathcommand{#1}[3]{{#2}({##1},{##2},{##3})}}
%example: \mathapplycommand\foo{\rm rubbish}
%         \foo{x} 
%produces:
%         rubbish(x)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\mathoverline=\overline
\remathcommand\overline[1]{\mathoverline{#1}}
% This makes \overline more intelligent, namely switching into math-mode
% if use in text-mode

\newcommand\mycomment[1]{{\iffalse{#1}\fi}}
% The argument of \comment is completely ignored

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Typesetting basics (lengths, struts) %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \setlength{\parindent}{2.0em}
\newlength{\disp}
\setlength{\disp}{\textwidth}
\addtolength{\disp}{-2.0\parindent}

\newlength{\textwidthminustwomm}
\setlength{\textwidthminustwomm}{\textwidth}
\addtolength{\textwidthminustwomm}{-0.2cm}

\newlength{\textwidthminushalfcm}
\setlength{\textwidthminushalfcm}{\textwidth}
\addtolength{\textwidthminushalfcm}{-0.5cm}

\newlength{\textwidthminusonecm}
\setlength{\textwidthminusonecm}{\textwidth}
\addtolength{\textwidthminusonecm}{-1.0cm}

\newlength{\textwidthminustwocm}
\setlength{\textwidthminustwocm}{\textwidth}
\addtolength{\textwidthminustwocm}{-2.0cm}

\newlength{\textwidthminusfourcm}
\setlength{\textwidthminusfourcm}{\textwidthminustwocm}
\addtolength{\textwidthminusfourcm}{-2.0cm}

\newlength{\textwidthminussixcm}
\setlength{\textwidthminussixcm}{\textwidth}
\addtolength{\textwidthminussixcm}{-6.0cm}

\newcommand\notop   {\vspace{-1.0\topsep}}
\newcommand\yestop  {\vspace{\topsep}}
\newcommand\halftop {\vspace{0.5\topsep}}
\newcommand\eighthtop{\vspace{0.125\topsep}}
\newcommand\ohyestop{\vspace*{\topsep}}
\newcommand\noitem  {\vspace{-1.0\itemsep}}
\newcommand\yesitem {\vspace{\itemsep}}

\newcommand\schweinerei{
\topsep 4pt plus 1pt minus 2pt
\partopsep 2pt plus 1pt minus 1pt
\renewcommand{\baselinestretch}{0.96}
\hfuzz=4pt}



\newcommand\bigmath[1]{\ \math{#1}\ }
\newcommand\bigmaths[2]{\ \math{#1}#2\ }
\newcommand\bigmathnlb[2]{\ \mbox{\math{#1}#2}\ }
\newcommand\nlmath{$\hfill\mbox{}\\\mbox{}\hfill$}
\newcommand\nlnomath{\hfill\mbox{}\\\mbox{}\hfill}

%Dont include spaces for pretty print here
\newcommand\linemath[1]{\mbox{}\hfill$#1$\hfill\mbox{}\\}  
\newcommand\linemaths[2]{\mbox{}\hfill$#1$#2\hfill\mbox{}\\}  
\newcommand\linenomath[1]{\mbox{}\hfill{#1}\hfill\mbox{}\\}  
%Dont include spaces for pretty print here
\newcommand\LINEmath[1]{\mbox{}\hfill$#1$\hfill\mbox{}}
\newcommand\LINEmaths[2]{\mbox{}\hfill$#1$#2\hfill\mbox{}}
\newcommand\LINEnomath[1]{\mbox{}\hfill{#1}\hfill\mbox{}}
%Dont include spaces for pretty print here

\newcommand\mysection
[1]{\noindent{\Large\bf#1}\addcontentsline{toc}{section}{#1}}
\newcommand\mysubsection
[1]{\noindent{\Large\bf#1}\addcontentsline{toc}{subsection}{#1}}
\newcommand\mysubsubsection
[1]{\noindent{\bf#1}\addcontentsline{toc}{subsubsection}{#1}}

\newcommand\knuthquotation[2]
{{\footnotesize\begin{flushright}{\sl#1\par}{\noindent\sc--- #2}\end
{flushright}}}

% The fol. \par\noindent\initial{A} writes an initial letter A 
% Note that it was designed to have the bottom line exactly on
% the bottom line of the line it starts. So it works well with
%   \initial{\underline{\underline{\underline{\underline{First case:}}}}}
%   In the first case we have the following...
% The two texts "first case" share their bottom. The underline extends
% below it.
% If you do not want your intials to get the bottom line
% from the bottom line of the first but of the second line
% you must design another macro or use \initial{\raisebox{-3.5ex}{...}}

\newbox\yinibox
\def\initial#1{\par
\noindent
\setbox\yinibox\hbox{#1}%
\setbox\yinibox\vbox to \ht\yinibox{\offinterlineskip\hbox{{#1}~~}\vss}%
\leavevmode
\hangindent=\wd\yinibox
\hangafter=-2
\hbox to0pt{\hskip-\hangindent\box\yinibox\hfill}\ignorespaces}
   
%%% Parentheses: %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\mathcommand\inparentheses[1]{\left(\begin{array}[c]{l}#1\end{array}\right)}
\mathcommand\inparenthesestight
[1]{\left(\begin{array}{@{}l@{}}#1\end{array}\right)}
\mathcommand\inparenthesesinline[1]{(\ #1\ )}
\mathcommand\inpit[1]{(#1)}
\mathcommand\inparenthesesinlinetight[1]{\inpit{#1}}
\newcommand\mathinparenthesesinlinetight[1]{(#1)}%allows line breaking
\mathcommand\noparenthesesoplist[1]
{{\begin{array}{l l}\relax&#1\\\end{array}}}
\mathcommand\noparenthesesoplisttop[1]
{{\begin{array}[t]{l l}\relax&#1\\\end{array}}}
\mathcommand\inparenthesesoplist[1]
{{\left(\noparenthesesoplist{#1}\right)}}
\mathcommand\inparenthesesoplistbraces[1]
{{\left\{\noparenthesesoplist{#1}\right\}}}
\newcommand\oplistund        {\\\tightund        &}
\newcommand\oplistoder       {\\\tightoder       &}
\newcommand\oplistcup        {\\\tightcup        &}
\newcommand\oplistuplus      {\\\tightuplus      &}
\newcommand\oplistequivalent {\\\tightequivalent &}
\newcommand\oplistimplies    {\\\tightimplies    &}
\newcommand\oplistcirc       {\\\tightcirc       &}
\newcommand\oplistantiimplies{\\\tightantiimplies&}
\newcommand\oplistnl         {\\                 &}
\mathcommand\inparenthesesimplies[2]{{\left(\begin{array}{l l}
\multicolumn{2}{l}{#1}\\\tightimplies&#2\\\end{array}\right)}}
\newcommand\inparenthesesimpliestoplevel[3]
{\math{#1\left(\begin{array}{l}\majorheadroom\footroom#2
 \\\end{array}\right.}\\\getittotheright{\math{
 \left.\begin{array}{l l}\tightimplies&\majorheadroom\footroom#3
 \\\end{array}\right)}}} 

\newcommand\opta{{\rm[}}
\newcommand\opte{{\rm]}}
\newcommand\opt[1]{\opta#1\/\opte}
\mathcommand\displayopt
[1]{\left[\begin{array}[t]{@{\,}c@{\,}}#1\end{array}\right]}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MATH NOTATION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\stopq{\math{.}\penalty-1\relax\,\,} %\penalty-10 is too low
\mathcommand\hastype[2]{{#1}:{#2}}
\mathcommand\tighthastype[2]{{#1}\tight:{#2}}
\mathcommand\typed[3]{#1\hastype{#2}{#3}\stopq}
\mathcommand\comma{,\ \ }
\mathcommand\setwithstart{\{\ }
\newcommand\setwithmark{~\math|\penalty-9\relax\,\ } 
%\penalty-10 is too low, \penalty-1 is too high
\mathcommand\setwithmarkq[1] {\ |_{#1}\ }
\mathcommand\setwithstop     {\ \}}
\newcommand\setwith
[2]{\math{\setwithstart#1}\setwithmark\math{#2\setwithstop}}
%should not be mathcommand for enabling \penalty-1
\mathcommand\displaysetwith
[2]{{\left\{\begin{array}{@{\ \ }l@{\ \ }|@{\ \ }l@{\ \ }}#1&#2\\\end
{array}\right\}}}
\mathcommand\displayset
[1]{{\left\{\begin{array}{@{\ \ }l@{\ \ }}#1\\\end{array}\right\}}}

\newcommand\tight[1]{\math{#1}}
\newcommand\tightsubseteq   {\tight\subseteq  }
\newcommand\tightnotsubseteq{\tight\nsubseteq }
\newcommand\tightsuperseteq {\tight\superseteq}
\newcommand\tightsetminus   {\tight\setminus  }
\newcommand\tightplus       {\tight+          }
\newcommand\tighttimes      {\tight\times     }
\newcommand\tightcap        {\tight\cap       }
\newcommand\tightcup        {\tight\cup       }
\newcommand\tightuplus      {\tight\uplus     }
\newcommand\tightcirc       {\tight\circ      }
\newcommand\tightin         {\tight{\,\in\,}  }
\newcommand\tightnotin      {\tight{\,\not\in\,}  }
\newcommand\tightni         {\tight{\,\ni\,}  }
\newcommand\tightnotni      {\tight{\,\not\ni\,}  }
\newcommand\tightequal      {\tight{\,=\,}\penalty-1\relax}
\newcommand\tightnotequal   {\tight{\,\not=\,}}
\newcommand\tightpreceq     {\tight{\,\preceq\,}}
\newcommand\tightprec       {\tight{\,\prec\,}}
\newcommand\tightnotprec    {\tight{\,\nprec\,}}
\newcommand\tightsucceq     {\tight{\,\succeq\,}}
\newcommand\tightsucc       {\tight{\,\succ\,}}
\newcommand\tightgtr        {\tight{\,>\,}}
\newcommand\tightless       {\tight{\,<\,}}
\newcommand\tightleq        {\tight{\,\leq\,}}
\newcommand\tightgeq        {\tight{\,\geq\,}}

\newcommand\boldequal  {\tight=}
\newcommand\boldunequal{\tight{\not=}}
\newcommand\boldless   {\tight<}
\newcommand\boldnotless{\tight{\not<}}
\newcommand\boldimplies{\tight\Rightarrow}
\newcommand\Defnombox{{\rm Def}}
\newcommand\Def{\mbox{\Defnombox}}
\mathcommand\DEF{\Defnombox\:}

\mathcommand\tightimplies    {\Rightarrow}
\mathcommand\tightantiimplies{\Leftarrow}
\mathcommand\tightequivalent {\Leftrightarrow}
\mathcommand\tightund        {\wedge}
\mathcommand\tightoder       {\vee}
\mathcommand\tightshefferstroke{|}
\newcommand\implies      {\ \tightimplies      \penalty-2\relax\ }
\newcommand\und          {\ \tightund          \penalty-2\relax\ }
\newcommand\oder         {\ \tightoder         \penalty-2\relax\ }
\newcommand\antiimplies  {\ \tightantiimplies  \penalty-2\relax\ }
\newcommand\equivalent   {\ \tightequivalent   \penalty-2\relax\ }
\newcommand\shefferstroke{\ \tightshefferstroke\penalty-2\relax\ }

\newcommand \id          {{\rm id}}
\mathcommand\allall      {\mathcal{V}}
\mathcommand\allsets     {\POWER\allall}
\mathcommand\allfinitesets{\FINITE\allall}
\mathcommand\urelements  {\mathcal{U}}
\mathcommand\algebra     {\mathcal{A}}
\mathcommand\balgebra    {\mathcal{B}}
\mathcommand\calgebra    {\mathcal{C}}
\mathcommand\dalgebra    {\mathcal{D}}
\mathcommand\ialgebra    {\mathcal{I}}
\mathcommand\salgebra    {\mathcal{S}}
\mathcommand\walgebra    {\mathcal{W}}
\mathcommand\ralgebra    {\mathcal{R}}
\mathcommand\algebraprime{\mathcal{A}'}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mathapplycommand\FLD        {\rm field}
\mathapplycommand\DOM        {\rm dom}
\mathapplycommand\RAN        {\rm ran}
\mathapplycommand\kernel     {\rm ker}
% \mathapplycommand\FINITE     {\mbox{\fraknomath P}_\N}%for \frak from german
% \mathapplycommand\POWER      {\mbox{\fraknomath P}}
% \mathapplycommand\posfinPOWER{\mbox{\fraknomath P}_\posN\!}
\mathapplycommand\FINITE     {{\mathfrak P}_{\scriptscriptstyle\N}}%for \frak from amssymb
\mathcommand\POWERSYM        {{\mathfrak P}}
\mathapplycommand\POWER      {\POWERSYM}
\mathapplycommand\posfinPOWER{\POWERSYM_{\scriptscriptstyle\posN\!}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mathcommand\CARD[1]         {\,|{#1}|\,}
\mathcommand\FLOOR[1]        {\ \lfloor#1\rfloor\ }
\mathcommand\CEIL[1]         {\ \lceil#1\rceil\ }
\mathcommand\reverserelation[1]{{#1}^{-1}}
%\mathcommand\restrictedto[1]{|_{#1}}
\mathcommand\domres[2]{{_{#2}\tight\upharpoonleft#1}}
\mathcommand\ranres[2]{{#1\tight\upharpoonright_{#2}}}
\mathcommand\funarg[1]{(#1)}
\mathcommand\app[2]{#1(#2)}
\mathcommand\displayapp[2]{#1\inparentheses{#2}}
\mathcommand\apptotuple[2]{#1#2}
\mathcommand\relapp[2]{\langle#2\rangle#1}
\mathcommand\displayrelapp
[2]{\left\langle\begin{array}{@{}l@{}}#2\end{array}\right\rangle\!#1}
\mathcommand\relappsin[2]{\relapp{#1}{\!\{#2\}\!}}
\mathcommand\revrelapp[2]{#1\langle#2\rangle}
\mathcommand\displayrevrelapp
[2]{#1\!\left\langle\begin{array}{@{}l@{}}#2\end{array}\right\rangle}
\mathcommand\revrelappsin[2]{\revrelapp{#1}{\!\{#2\}\!}}
\mathcommand\pair[2]{(#1,#2)}
\mathcommand\displaypair[2]{\inparentheses{#1,\ \ #2}}
\mathcommand\trip[3]{(#1,#2,#3)}
\mathcommand\displaytrip[3]{\inparentheses{#1,\ \ #2,\ \ #3}}
\mathcommand\superdisplaytrip[3]{\left(\begin
{array}{l}#1,\\#2,\\#3,\\\end{array}\right)}
\mathcommand\quar[4]{(#1,#2,#3,#4)}
\mathcommand\displayquar[4]{\inparentheses{#1,\ \ #2,\ \ #3,\ \ #4}}
\mathcommand\superdisplayquar[4]{\left(\begin
{array}{l}#1,\\#2,\\#3,\\#4\\\end{array}\right)}
\mathcommand\quin[5]{(#1,#2,#3,#4,#5)}
\mathcommand\displayquin[5]{\inparentheses{#1,\ \ #2,\ \ #3,\ \ #4,\ \ #5}}
\mathcommand\sext[6]{(#1,#2,#3,#4,#5,#6)}
\mathcommand\sept[7]{(#1,#2,#3,#4,#5,#6,#7)}
\mathcommand\oct[8]{(#1,#2,#3,#4,#5,#6,#7,#8)}
\mathcommand\ninetuple[9]{(#1,#2,#3,#4,#5,#6,#7,#8,#9)}
\newcommand\tentuple[9]{(#1,#2,#3,#4,#5,#6,#7,#8,#9,\singletonrest}
\newcommand\singletonrest[1]{#1)}
\newcommand\elev[9]{(#1,#2,#3,#4,#5,#6,#7,#8,#9,\pairrest}
\newcommand\pairrest[2]{#1,#2)}
\mathcommand\setwithq[3]     {\setwithstart#2\setwithmarkq{#1}#3\setwithstop}
\mathcommand\setofwords[1]{#1^{\textstyle\ast}}
\mathcommand\setofwordsscriptstyle[1]{#1^{\ast}}
\mathcommand\setofnonemptywords[1]{#1^+}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mathcommand\FUNSET   [2]{{#1}\rightarrow{#2}}
\mathcommand\PARFUNSET[2]{{#1}\leadsto   {#2}}
\mathcommand\FUNDEF   [3]{\hastype{#1}{\FUNSET   {#2}{#3}}}
\mathcommand\PARFUNDEF[3]{\hastype{#1}{\PARFUNSET{#2}{#3}}}
%categories
\mathcommand\morphcolon{::}
\mathcommand\morpharrow{\rightarrow}
\mathcommand\morph  [3]{{#1}\morphcolon{#2}\morpharrow{#3}}
\newcommand\Idname{{\rm Id}}
\mathcommand\Id[1]{{\Idname_{#1}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mathcommand\equiclass[2]{{#1}{[\{{#2}\}]}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mathcommand\aritysugarsymbol{\rightarrow}
\mathcommand\aritysugar{\ \aritysugarsymbol\ }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\mathcommand\monus{\mathchoice
{\raisebox{-.4ex}{$\dot{\raisebox{.4ex}[0ex]{$-$}}$}}%     display-style
{\raisebox{-.4ex}{$\dot{\raisebox{.4ex}[0ex]{$-$}}$}}%     text-style
{\raisebox{-.3ex}{$\scriptstyle\dot{\raisebox{.3ex}[0ex]
{$\scriptstyle-$}}$}}                                %     scriptstyle
{\raisebox{-.2ex}{$\scriptscriptstyle\dot{\raisebox{.2ex}[0ex]
{$\scriptscriptstyle-$}}$}}                          %scriptscriptstyle
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\mathcommand\yields{\;\vdash\;}
\mathcommand\antiyields{\;\dashv\;}
\mathcommand\tightyields{\vdash}
\mathcommand\tightantiyields{\dashv}
\mathcommand\notyields{\;\nvdash\;}
\mathcommand\refltransyields{\hspace{0.5em}\raisebox{1.3ex}{\math{\scriptstyle
  \ast}}\hspace{-1.0em}\yields}
\mathcommand\transyields
{\hspace{0.5em}\raisebox{1.3ex}{$\scriptscriptstyle%\oplus
+$}\hspace
{-1.0em}\yields\hspace{0.3em}}
\mathcommand\notmodels{\:\not\!\models}

\newcommand\EVALSYM{{\rm eval}}
\mathapplycommand\EVAL{\EVALSYM}
\mathcommand\V{{\rm V}}
\mathcommand\X{{\rm X}}
\newcommand\nottight{\bigmath}
\mathcommand\refltransclosureinline[1]{{#1}^\ast}
\mathcommand\VARSYM {\mathcal{V}}
\mathapplycommand\VAR{\VARSYM}
\mathcommand\VARnoparentheses[1]{\VARSYM #1}
\mathcommand\VARsingleindex[1]{\VARSYM\!_{{#1}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ZAHLENMENGEN %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \N        Set of natural numbers
% \posN     Set of positive natural numbers
% \ordclass Proper class of ordinal numbers
% \ZZ       Set of integers
% \Q        Set of rationals
% \RE       Set of real numbers
% \posRE    Set of positive real numbers
% \nonnegRE Set of non-negative real numbers
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \mathcommand\N{{\rm
% %\rm must be out here because on rare occursions does not work
% %infront of the I\hskip....
% %\ifmmode%  Sind wir im Mathemodus ?
% \mathchoice{{I\hskip -2pt   N}}% display-style
%            {{I\hskip -2pt   N}}% text-style
%            {{I\hskip -1.5pt N}}% scriptstyle
%            {{I\hskip -1pt   N}}% scriptscriptstyle
% %\else\math{\rm I\hskip-2pt N}\fi
% }}
% \newcommand\ZZ{{\rm\ifmmode\mathchoice{{Z\hskip -4pt Z}}{{Z\hskip -4pt Z}}
% {{Z\hskip -3pt Z}}{{Z\hskip -3pt Z}}\else\mbox{\tenrm Z\hskip-4pt Z}\fi}}
\mathcommand\N{{\bf N}}
\mathcommand\posN{\N_{\:\!\!\mbox{\sixsf+}}}
\mathcommand\ZZ{{\bf Z}}
\mathcommand\Q{{\bf Q}}
\mathcommand\ordclass{\mathcal{O}}
%\newcommand\RE{{\rm\ifmmode\mathchoice{{I\hskip -2pt R}}{{I\hskip -2pt R}}
%{{I\hskip -1.5pt R}}{{I\hskip -1pt R}}\else{\tenrm I\hskip-2pt R}\fi}}
\mathcommand\RE{{\bf R}}
\mathcommand\posRE{\RE_{\scriptscriptstyle +}}
\mathcommand\nonnegRE{\RE_{\scriptscriptstyle\succeq0}}

\mathcommand\Qzero{{\cal Q}_0}
\newcommand\squaredot{\,\rule{0.4ex}{0.4ex}\,}

%Transitive closures
\mathcommand\transclosure[1]{\stackrel{\scriptscriptstyle+}{#1}}
\mathcommand\transclosureinline[1]{{#1}^{\scriptscriptstyle+}}

%_____________________________________________________________________________
%Signatures
\mathcommand\sigarity{\alpha}
\newcommand\sig{{\rm sig}}
\mathcommand\sigsorts  {{\mathbb S}}
\mathcommand\sigfunsym {{\mathbb F}}
\mathcommand\consfunsym{{\mathbb C}\,} 
% \, cures strange dvips bugg
\mathcommand\deffunsym {{\mathbb N}}
\mathcommand\Ax{\mathcal{AX}}

%from header.tex
%_____________________________________________________________________________
%Reduction relation

%\red...
%\notred
%\redpara
%\revpara
%\simpara
%\unired
\mathcommand\unired{\Longrightarrow}
\mathcommand\redsimple{\longrightarrow}
\mathcommand\redindex[1]{\redsimple_{_{\!#1}}}
\mathcommand\notredindex[1]{\,\,\,\not\!\!\!\!\redsimple_{_{\!#1}}}
\newcommand\redsub             {\redindex{\R ,\X        }}
\newcommand\redsubprime        {\redindex{\R',\X'       }}
\newcommand\redshortsub        {\redindex{\R ,\V        }}
\newcommand\redshortsubprime   {\redindex{\R',\V'       }}
\newcommand\redsubY            {\redindex{\R ,\Y        }}
\newcommand\redsubemptyset     {\redindex{\R ,\emptyset }}
\newcommand\redsubprimeemptyset{\redindex{\R',\emptyset }}
\newcommand\redsubVsig         {\smallfootroom\redindex{\R ,\Vsig     }}
\newcommand\redsubVsigprime    {\smallfootroom\redindex{\R',\Vsigprime}}
\mathcommand\redindexn[2]{\stackrel{#1}\redsimple_{_{\!#2}}}
\mathcommand\redparaindex[1]{\redpara_{\hskip-1.5pt\scriptscriptstyle#1}}
\mathcommand\revparaindex[1]{\revpara_{\hskip-1.5pt\scriptscriptstyle#1}}
\mathcommand\simparaindex[1]{\simpara_{\hskip-1.5pt\scriptscriptstyle#1}}
\mathcommand\uniredindex[1]{\unired_{\hskip-1.5pt\scriptscriptstyle#1}}

%\antired...
%\notantired..
%\antiredpara...
%\antirevpara...
%\antiunired...
\mathcommand\antiunired{\Longleftarrow}
\mathcommand\antired{\longleftarrow}
\mathcommand\antiuniredindex[1]{\antiunired_{_{\!#1}}}
\mathcommand\antiredindex[1]{\antired_{_{\!#1}}}
\mathcommand\notantiredindex[1]{\,\,\,\not\!\!\!\!\antired_{_{\!#1}}}
\newcommand\antiredsub          {\antiredindex{\R ,\X }}
\newcommand\antiredshortsub     {\antiredindex{\R ,\V }}
\newcommand\antiredshortsubprime{\antiredindex{\R',\V'}}
\newcommand\antiredsubVsig      {\smallfootroom\antiredindex{\R',\Vsig}}
\mathcommand\antiredindexn[2]{\stackrel{#1}\antired_{_{\!#2}}}
\mathcommand\antiredparaindex
[1]{\antiredpara_{\hskip-1.25pt\scriptscriptstyle#1}}
\mathcommand\antirevparaindex[1]
{\antirevpara_{\hskip-1.25pt\scriptscriptstyle#1}}

%\sym...
\mathcommand\sym{\longleftrightarrow}
\mathcommand\symindex[1]{\sym_{_{\!#1}}}
\mathcommand\symindexn[2]{\stackrel{#1}{\sym_{_{\!#2}}}}
\newcommand\symsub     {\symindex{\R,\X}}
\newcommand\symshortsub{\symindex{\R,\V}}
\newcommand\symsubVsig {\smallfootroom\symindex{\R,\Vsig}}

%Reflexive transitive closures
%Congruences
%\congru...
%\footnotecongru...
%\notcongru...
\mathcommand\refltransclosure[1]{\stackrel{\scriptstyle\ast}{#1}}
%{\mathop{#1}^{\scriptstyle\ast}}
\mathcommand\congru{\refltransclosure\sym}
\mathcommand\congruindex[1]{\congru_{_{\!#1}}}
\newcommand\congrusub             {\congruindex{\R ,\X            }}
\newcommand\congrushortsub        {\congruindex{\R ,\V            }}
\newcommand\congrusubVsig         {\smallfootroom\congruindex{\R ,\Vsig     }}
\newcommand\congrusubVsigprime    {\smallfootroom\congruindex{\R',\Vsigprime}}
\newcommand\congrusubemptyset     {\congruindex{\R ,\emptyset     }}
\newcommand\congrusubprimeemptyset{\congruindex{\R',\emptyset     }}
\mathcommand\footnotecongru%{\stackrel\footnoteoast\sym}
{\congru}
\mathcommand\footnotecongruindex[1]{\footnotecongru_{_{#1}}}
\mathcommand\notcongru{\hspace{0.6em}\not\hspace{-0.85em}\refltransclosure\sym}
\mathcommand\notcongruindex[1]{\notcongru_{_{\!#1}}}
\newcommand\notcongrusub        {\notcongruindex{\R,\X       }}
\newcommand\notcongrusubemptyset{\notcongruindex{\R,\emptyset}}

%Transitive closures
%\trans...
%\antitrans...
\mathcommand\trans{\transclosure\redsimple}
\mathcommand\transindex[1]{\trans_{_{\!#1}}}
\newcommand \transsub        {\transindex{\R,\X}}
\newcommand \transshortsub   {\transindex{\R,\V}}
\newcommand \transsubVsig    {\smallfootroom\transindex{\R,\Vsig}}
\newcommand \transsubemptyset{\transindex{\R,\emptyset}}
\mathcommand\antitrans{\transclosure\antired}
\mathcommand\antitransindex[1]{\antitrans_{_{\!#1}}}
\newcommand \antitranssub     {\antitransindex{\R,\X}}
\newcommand \antitransshortsub{\antitransindex{\R,\V}}
\newcommand \antitranssubVsig {\smallfootroom\antitransindex{\R,\Vsig}}

%Reflexive and transitive closures
%\refltrans...
%\footnoterefltrans...
%\notrefltrans...
%\antirefltrans...
%\footnoteantirefltrans...
\mathcommand\refltrans{\refltransclosure\redsimple}
\mathcommand\refltransindex[1]{\refltrans_{_{\!#1}}}
\newcommand \refltranssub          {\refltransindex{\R ,\X }}
\newcommand \refltranssubemptyset  {\refltransindex{\R ,\emptyset}}
\newcommand \refltranssubprime     {\refltransindex{\R',\X'}}
\newcommand \refltransshortsub     {\refltransindex{\R ,\V }}
\newcommand \refltransshortsubprime{\refltransindex{\R',\V'}}
\newcommand \refltranssubVsig      {\smallfootroom\refltransindex{\R ,\Vsig}}
\mathcommand\footnoterefltrans%{\stackrel\footnoteoast\redsimple}
{\refltrans}
\mathcommand\footnoterefltransindex[1]{\footnoterefltrans_{_{#1}}}
\newcommand \footnoterefltranssub     {\footnoterefltransindex{\R,\X}}
\newcommand \footnoterefltransshortsub{\footnoterefltransindex{\R,\V}}
\mathcommand\notrefltrans
            {\hspace{0.6em}\not\hspace{-0.85em}\refltransclosure\redsimple}
\mathcommand\antirefltrans{\refltransclosure\antired}
\mathcommand\antirefltransindex[1]{\antirefltrans_{_{\!#1}}}
\newcommand \antirefltranssub          {\antirefltransindex{\R ,\X }}
\newcommand \antirefltransshortsub     {\antirefltransindex{\R ,\V }} 
\newcommand \antirefltransshortsubprime{\antirefltransindex{\R',\V'}} 
\newcommand \antirefltranssubVsig      {\antirefltransindex{\R',\V'}} 
\mathcommand\footnoteantirefltrans%{\stackrel\footnoteoast\antired}
{\antirefltrans}
\mathcommand\footnoteantirefltransindex[1]{\footnoteantirefltrans_{_{#1}}}
\newcommand \footnoteantirefltranssub     {\footnoteantirefltransindex{\R,\X}}
\newcommand \footnoteantirefltransshortsub{\footnoteantirefltransindex{\R,\V}}

%joinability
\mathcommand\downarrowindex[1]{\downarrow_{_{#1}}}
\newcommand \downarrowsub        {\downarrowindex{\R ,\X       }}
\newcommand \downarrowsubemptyset{\downarrowindex{\R ,\emptyset}}
\newcommand \downarrowsubVsig    {\smallfootroom\downarrowindex{\R,\Vsig}}
\newcommand \downarrowsubprimeemptyset{\downarrowindex{\R',\emptyset}}
\mathcommand\notconfluindex[1]{\notconflu_{_{#1}}}
\newcommand \notconflusub        {\notconfluindex{\R,\X       }}
\newcommand \notconflusubemptyset{\notconfluindex{\R,\emptyset}}
\mathcommand\footnotenotconfluindex[1]{\footnotenotconflu_{_{#1}}}
\newcommand \footnotenotconflusub{\footnotenotconfluindex{\R,\X}}

%strong joinability
\mathcommand\downdownarrow        {\downdownarrows}
\mathcommand\downdownarrowindex[1]{\downdownarrow_{_{#1}}}
\newcommand \downdownarrowsub     {\downdownarrowindex{\R ,\X       }}

\mathcommand\reflclosure[1]{\stackrel
%{\raisebox{0.1em}{$\scriptscriptstyle\preceq$}{ 1}}
{\scriptscriptstyle=}
{#1}}
\mathcommand\reflclosureinline[1]{{#1}^{\scriptscriptstyle=}}
\mathcommand\onlyonce
%{{\displaystyle\mathop{\redsimple}^{{\leq}1}}}
{\reflclosure\redsimple}
\mathcommand\antionlyonce{\reflclosure\antired}
\mathcommand\onlyonceindex[1]{\onlyonce_{_{\!#1}}}
\mathcommand\antionlyonceindex[1]{\antionlyonce_{_{\!#1}}}

\mathapplycommand\nf{\rm NF}

\mathcommand\toconditiontermssub     {\twoheadrightarrow_{_{\R,\X}}}
\mathcommand\toconditiontermssubY    {\twoheadrightarrow_{_{\R,\Y}}}
\mathcommand\toconditiontermsshortsub{\twoheadrightarrow_{_{\R,\V}}}

%_____________________________________________________________________________
%Variables notation
\newcommand \U{{\rm U}}
\newcommand \Y{{\rm Y}}
\newcommand \Z{{\rm Z}}
\mathcommand\Xprime{{\rm X}'}
\mathcommand\Yprime{{\rm Y}'}
\mathcommand\Xprimeprime{{\rm X}''}
\newcommand \SIG     {{\rm SIG}}
\mathcommand\CONS    {\mathcal{C}}
\mathcommand\SIGsort     [1]{(\SIG     ,#1)}
\mathcommand\CONSsort    [1]{(\CONS    ,#1)}
\mathcommand\varsigmasort[1]{(\varsigma,#1)}
\mathcommand\SIGsortindex     [1]{_{\SIG ,#1}}
\mathcommand\CONSsortindex    [1]{_{\CONS,#1}}
\mathcommand\DUNNOsortindex   [1]{_{\DUNNO,#1}}
\mathcommand\varsigmasortindex[1]{_{\varsigma,#1}}
\mathcommand\Vsig      {\V \!_{\SIG }}
\mathcommand\Xsig      {\X   _{\SIG }}
\mathcommand\Vcons     {\V \!_{\CONS}}
\mathcommand\Sigmacons {\Sigmaoffont_{\CONS}}
\mathcommand\Xcons     {\X   _{\CONS}}
\mathcommand\Vconsprime{\V'\!_{\CONS}}
\mathcommand\Vsigprime {\V'\!_{\SIG }}
\mathcommand\sigV      {\Vsig\!\uplus\!\Vcons}
\mathcommand\sigVprime {\Vsigprime\!\uplus\!\Vconsprime}
\mathcommand\hiddenVindi     [2]{\V   \!_{{#1},{#2}}}
\mathcommand\hiddenXindi     [2]{\X     _{{#1},{#2}}}
\mathcommand\hiddenVprimeindi[2]{\V'\!\!_{{#1},{#2}}}
\newcommand \Vsigindex     [1]{\hiddenVindi\SIG     {#1}}
\newcommand \Xsigindex     [1]{\hiddenXindi\SIG     {#1}}
\newcommand \Vconsindex    [1]{\hiddenVindi\CONS    {#1}}
\newcommand \Xconsindex    [1]{\hiddenXindi\CONS    {#1}}
\newcommand \Vvarsigmaindex[1]{\hiddenVindi\varsigma{#1}}
\newcommand \Xvarsigmaindex[1]{\hiddenXindi\varsigma{#1}}
\mathapplycommand\VARCONS{\VARsingleindex\CONS}
\mathapplycommand\VARSIG {\VARsingleindex\SIG}
\mathapplycommand\VARord {\VARsingleindex\boldless}

%_____________________________________________________________________________
%Term notation
\mathcommand\vt{\mathcal{ T}}
\mathcommand\gt{\mathcal{GT}}
\mathcommand\hiddenvtindi[2]{\mathcal{ T}\!_{#1,#2}}
\mathcommand\hiddengtindi[2]{\mathcal{GT}\!_{#1,#2}}
\newcommand\vtsigindex     [1]{\hiddenvtindi{\SIG     }{#1}}
\newcommand\vtconsindex    [1]{\hiddenvtindi{\CONS    }{#1}}
\newcommand\vtvarsigmaindex[1]{\hiddenvtindi{\varsigma}{#1}}
\newcommand\gtsigindex     [1]{\hiddengtindi{\SIG     }{#1}}
\newcommand\gtconsindex    [1]{\hiddengtindi{\CONS    }{#1}}
\newcommand\gtvarsigmaindex[1]{\hiddengtindi{\varsigma}{#1}}
\mathapplycommand\hiddentv     {\mathcal{T}}
\mathapplycommand\hiddentg     {\mathcal{GT}}
\mathapplycommand\hiddentvprime{\mathcal{T}'}
%ground term sets
\newcommand\tgcons              {\hiddentg\cons }
\newcommand\tgsig               {\hiddentg\sig  }   
\newcommand\tgdunno             {\hiddentg\dunno}
\newcommand\tgconsprime         {\hiddentg{\cons'}}
\newcommand\tgsigprime          {\hiddentg{\sig' }}
\newcommand\tgunderlinecons     {\hiddentg{\underline{\underline{\cons }}}}
\newcommand\tgunderlineconsprime{\hiddentg{\underline{\underline{\cons'}}}}
%non-ground term sets
% variables from \Vsig or \Vsigprime
\newcommand\tsigV        {\hiddentv{\sig  ,\V}}
\newcommand\tsigVsig     {\hiddentv{\sig  ,\Vsig}}
\newcommand\tsigVsigprime{\hiddentv{\sig' ,\Vsigprime}}
% variables from \Vcons 
\newcommand\tcc{\hiddentv{\cons,\Vcons}}
% variables from \Vcons\cup\Vsig etc.
\newcommand\tss          {\hiddentv{\sig  ,\sigV     }}
\newcommand\tcs          {\hiddentv{\cons ,\sigV     }}
\newcommand\tcsprime     {\hiddentv{\cons',\sigVprime}}
% variables from \X or \X' etc.
\newcommand\tsigX        {\hiddentv{\sig ,\X }}
\newcommand\tconsX       {\hiddentv{\cons,\X }}
\newcommand\tsigXprime   {\hiddentv{\sig',\X'}}
\newcommand\tconsXprime  {\hiddentv{\cons',\X'}}
\newcommand\tconsVconsX  {\hiddentv{\cons,\Xcons}}
% variables from \Y
\newcommand\tsigY        {\hiddentv{\sig ,\Y }}
\newcommand\tconsY       {\hiddentv{\cons,\Y }}
%term algebras
\newcommand\tconsXalt {\app{{\mathcal T}_\CONS}\X}
\newcommand\tconsValt {\app{{\mathcal T}_\CONS}\V}
\newcommand\tX        {\hiddentv\X}
\newcommand\tXprime   {\hiddentv{\X'}}
\newcommand\tV        {\hiddentv\V}
\newcommand\tY        {\hiddentv\Y}
\newcommand\temptyset {\hiddentv\emptyset}
\newcommand\tVsig     {\hiddentv\Vsig}
\newcommand\tVsigprime{\hiddentvprime\Vsigprime}
% \newcommand{\gtc}{\hiddentg{\cons}}
%_____________________________________________________________________________
%substitutions
\mathcommand\SUBSYM{\mathcal{SU\hspace{-.08em}B}}
\mathdoubleapplycommand\SUBST{\SUBSYM}
\newcommand \Xsubst     {\SUBST\V\tX   }
\newcommand \Vsubst     {\SUBST\V\vt   }
\newcommand \Vsigsubst  {\SUBST\V\tVsig}
\newcommand \Gsubst     {\SUBST\V\gt   }
\mathcommand\Isubst     {{\rm CGSUB}(\V ,\cons )}
\mathcommand\Isubstprime{{\rm CGSUB}(\V',\cons')}
\mathcommand\GENSYM     {\mathcal{G\hspace{-.04em}E\hspace{-.09em}N}}
\mathcommand\GSSYM      {{\GENSYM\hspace{-.14em}}\SUBSYM}
\mathdoubleapplycommand\GS{\GSSYM}
\newcommand\VGS{\GS\V\vt}
\newcommand\XGS{\GS\V\tX}
\newcommand\VsigGS{\GS\V\tVsig}
%
\mathcommand\POSSYMBOL{\mathcal{P\hspace{-.08em}O\hspace{-.1em}S}}
\mathcommand\VPOSSYMBOL{\V\hspace{-.04em}\POSSYMBOL}
\mathcommand\FPOSSYMBOL{\sigfunsym\hspace{-.04em}\POSSYMBOL}
\mathapplycommand\TPOS{\POSSYMBOL}
%\mathapplycommand\POS{\POSSYMBOL} \POS is also used by xy. Use \TPOS instead!
\mathapplycommand\VPOS{\VPOSSYMBOL}
\mathapplycommand\FPOS{\FPOSSYMBOL}
%\mathcommand\OCCSYMBOL{\mathcal{O}}
%\mathapplycommand\OCC{\OCCSYMBOL}%obsolete but still in use
\mathcommand\neitherprefixsymbol{\parallel}
\mathcommand\neitherprefix[2]{{#1}\,\neitherprefixsymbol\,{#2}}
\mathcommand\replsuffix   [2]{[\,#1\leftarrow#2\,]}      %use \repl if possible
\mathcommand\replparsuffix[3]{\replsuffix{#1}{#2\ |\ #3}}%use \replpar
\mathcommand\repl         [3]{#1\penalty-1\replsuffix{#2}{#3}}
\mathcommand\replpar      [4]{#1\penalty-1\replparsuffix{#2}{#3}{#4}}
\mathcommand\eqvariablessig[1]{\mbox{\rm Eq}(\sig,{#1})}
\newcommand\eqvsig{\eqvariablessig{\sigV}}
\mathcommand\eqgsig{\mbox{\rm GEq}(\sig)}
\mathcommand\direqv[1]{\mbox{\rm DEq}(#1)}
\newcommand\direqvariablessig[1]{\direqv{\sig,{#1}}}
\newcommand\direqvsig{\direqv{\sig,\sigV}}
\mathapplycommand\MGU{\rm Mgu}
\mathdoubleapplycommand\minmgu{\rm mgu}
\mathdoubleapplycommand\sep{\rm Sep}
\mathdoubleapplycommand\minsep{\rm sep}
\mathapplycommand\depth{\rm depth}
\mathapplycommand\size{\rm size}
\newcommand\monotonic           {\tsigX-mono\-tonic}
\newcommand\Vmonotonic          {\vt-mono\-tonic}
%\newcommand\amonotonic          {an \X-mono\-tonic}
\newcommand\emptysetmonotonic   {\gt-mono\-tonic}
\newcommand\monotonicity        {\tsigX-mono\-toni\-city}
\newcommand\Vmonotonicity       {\vt-mono\-toni\-city}
%\newcommand\Monotonicity        {\X-mono\-toni\-city}
\newcommand\stable              {\X-stable}
\newcommand\Vstable             {\V-stable}
\newcommand\Ystable             {\Y-stable}
\newcommand\emptysetstable      {\mbox{$\emptyset$}-stable}
\newcommand\stability           {\X-stabi\-lity}
\newcommand\Stability           {\X-stabi\-lity}
\newcommand\Vstability          {\V-stabi\-lity}
\newcommand\VStability          {\V-stabi\-lity}
\newcommand\compatible          {\X-compa\-tible}
\newcommand\RXcompatible        {\RX-compa\-tible}
\newcommand\Vcompatible         {\V-compa\-tible}
\newcommand\Ycompatible         {\Y-compa\-tible}
\newcommand\leftrightcompatible {\X-left-right-compa\-tible}
\newcommand\Vleftrightcompatible{\V-left-right-compa\-tible}
\newcommand\dontcarecompatible  {\X-don't-care-compa\-tible}
\newcommand\aleftrightcompatible{an \X-left-right-compa\-tible}
\newcommand\adontcarecompatible {an \X-don't-care-compa\-tible}
\newcommand\compatibility       {\X-compa\-ti\-bility}
\newcommand\dontcarecompatibility{\X-don't-care-compa\-ti\-bility}
\newcommand\Vdontcarecompatible {\V-don't-care-compa\-tible}
\newcommand\Safety              {Safeness}
\newcommand\safety              {safeness}
\newcommand\safe                {safe}
\newcommand\Safe                {Safe}
\newcommand\unsafe              {unsafe}
\newcommand\safely              {safely}
\newcommand\constructorminimal{con\-struc\-tor-mini\-mal}
\newcommand\ConstructorMinimal{Con\-struc\-tor-Mini\-mal}
\newcommand\constructorminimality{con\-struc\-tor-mini\-mal\-ity}
\newcommand\constructorminimum{con\-struc\-tor-mini\-mum}
\newcommand\constructorpreserving{con\-struc\-tor-pre\-serving}
\newcommand\constructorpreservation{con\-struc\-tor-pre\-serva\-tion}
\newcommand\constructorbased{con\-struc\-tor-based}
\newcommand\Constructorbased{Con\-struc\-tor-based}
\newcommand\terminationpair{termi\-na\-tion-pair}
\newcommand\TerminationPair{Termi\-na\-tion-Pair}
\newcommand\inductivesubstitution{constructor ground substitution}
\newcommand\aninductivesubstitution{a constructor ground substitution}
\newcommand\Inductivesubstitution{Constructor ground substitution}
\newcommand\InductiveSubstitution{Constructor Ground Substitution}
\newcommand\inductiveinstance{constructor ground instance}

%Subterm
\newcommand\hiddensubST{_{_{\rm ST}}}
\mathcommand\superterm   {\rhd\hiddensubST}
\mathcommand\notsuperterm{\ntriangleright\hiddensubST}
\mathcommand\subterm     {\lhd\hiddensubST}
\mathcommand\notsubterm  {\ntriangleleft\hiddensubST}
\mathcommand\supertermeq {\trianglerighteq\hiddensubST}
\mathcommand\subtermeq   {\trianglelefteq\hiddensubST}

\mathcommand\sugarregel{l\boldequal r\rulesugar C}
\mathcommand\sugarregelindex[1]{l_{#1}\boldequal r_{#1}\rulesugar C_{#1}}
\mathcommand\sugaruncondregelindex[1]{l_{#1}\boldequal r_{#1}}
\mathcommand\ndrulewithassumption[3]{{{{\scriptstyle\lbrack}#1{\scriptstyle
\rbrack}}\atop\scriptstyle #2}\over #3}

%_____________________________________________________________________________
%Rules
\def\R{{\rm R}}
\mathcommand\RCONS{\R_\CONS}
\mathcommand\Rprime{{\rm R}'}
\mathcommand\RX{\R,\X}
\mathcommand\RCONSX{\RCONS,\X}
\mathcommand\DEFUNSYM{\mathcal{DEFUN}}
\mathapplycommand\DEFUN{\DEFUNSYM}
\newcommand\defsort{{\rm def}}
\mathcommand\ATSYM  {\mathcal{A\hspace{-.02em}T}}
\mathdoubleapplycommand\atomsof{\ATSYM}
\newcommand\atoms      {\atomsof\sig\V}
\newcommand\Xatoms     {\atomsof\sig\X}
\newcommand\Yatoms     {\atomsof\sig\Y}
\newcommand\scatoms    {\atomsof\sig\Vcons}
\mathcommand\GENATSYM  {\GENSYM\hspace{-.18em}\ATSYM}
\mathdoubleapplycommand\genatomsof{\GENATSYM}
\newcommand\genatoms      {\genatomsof\sig\V}
\newcommand\Xgenatoms     {\genatomsof\sig\X}
\newcommand\Ygenatoms     {\genatomsof\sig\Y}
\mathcommand\CONDSYM  {\mathcal{C\hspace{-.1em}O\hspace{-.12em}N\hspace{-.12em}D}}
\mathcommand\LITSYM   {\mathcal{LI\hspace{-.04em}T}}
\mathcommand\CONDLITSYM{\CONDSYM\hspace{-.04em}\LITSYM}
\mathapplycommand\condlitwitharg{\CONDLITSYM}
\newcommand\condlit {\condlitwitharg{\sig,\V}}
\newcommand\Xcondlit{\condlitwitharg{\sig,\X}}
\newcommand\Ycondlit{\condlitwitharg{\sig,\Y}}
\mathdoubleapplycommand\literals{\LITSYM}
\newcommand \lit        {\literals\sig\V}
\newcommand \Xlit       {\literals\sig\X}
\newcommand \Ylit       {\literals\sig\Y}
\mathcommand\GENLITSYM{\GENSYM\hspace{-.08em}\LITSYM}
\mathdoubleapplycommand\genliterals{\GENLITSYM}
\newcommand \genlit        {\genliterals\sig\V}
\newcommand \Xgenlit       {\genliterals\sig\X}
\newcommand \Ygenlit       {\genliterals\sig\Y}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% END %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> headernamesrest.tex <==
% FILE: headernamesrest.tex
% CONTENTS: CP's standard file for including world knowledge,
%           such as names, language, characters, life times.
%
% This file must be loadable as the first file of any latex file!
% So do not use any extensions which are not contained in it,
% such as \mathcommand
%
% Moreover, \emph must not be used here!

\usepackage{amssymb}

\input specialfonts

\newcommand\namefont{}
\newcommand\bibcrit[1]{\ {\sl{(#1)}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\hyphenation{
ab-ge-leitete
ab-ge-leitetem
ab-ge-leiteten
ab-ge-leiteter
ab-ge-leitetes
ab-weicht
accord-ing
Acker-mann
actual
actual-ly
aktiv
aktive
aktivem
aktiven
aktiver
aktives
although
analysis
an-ge-mie-te-ten
annota-tions
ante-cedent
ante-cedents
appli-ca-tion
appli-ca-tions
area
areas
argu-ment
aspect
asser-tion
asser-tions
assump-tion
assump-tions
Aus-wahl-funktion
Aus-spra-che
author
authors
auto-ma-ted
auto-ma-tion
auto-ma-tisch
auto-ma-ti-sche
auto-ma-ti-schem
auto-ma-ti-schen
auto-ma-ti-scher
auto-ma-ti-sches
Autoren
axio-ma-tics
axiom
Axiome
axioms
basic
basis
be-ein-flusst
be-endet
beharr-lich
being
be-kannte
be-kanntem
be-kannten
be-kannter
be-kanntes
be-rech-tig-te
Bereich
Be-rei-chen
be-zeich-net
Be-zeich-nung
bietet
bis-heri-gen
certain
che-mi-sche
che-mi-schem
che-mi-schen
che-mi-sches
che-mi-scher
com-pati-bi-lity
classi-fi-ca-tion
concept
con-struc-tor
co-rol-lary
counter-example
creati-vity
custom-ary
Dag-stuhl
define
defi-niert
defi-nierte
defi-niertem
defi-nierten
defi-nierter
defi-niertes
defi-nit
defi-nite
defi-nitem
defi-niten
defi-niter
defi-nites
defi-ni-tion
defi-ni-tions
de-monstra-tion
denen
der-arti-ge
der-arti-gen
der-arti-gem
der-arti-ger
der-arti-ges
De-signs
des-cente
descent
deter-mined
deutsche
deutschem
deutschen
deutscher
deutsches
develop-ing
deviate
diese
direc-tion
dis-equality
dis-equali-ties
dis-respected
durch-aus
Effi-zienz
easily
effec-tive
ehren-amt-licher
ehren-amt-liches
ehren-amt-liche
ehren-amt-lichen
ehren-amt-lichem
eigent-lichen
Ein-arbei-tung
eine
einem
einen
einer
eines
either
elek-tro-ni-scher
elek-tro-ni-sches
elek-tro-ni-sche
elek-tro-ni-schen
elek-tro-ni-schem
element
elements
elemen-tary
em-pfohlen
em-pfun-dener
em-pfun-denes
em-pfun-dene
em-pfun-denen
em-pfun-denem
enforce
enforced
enforces
eng-lisch
Engli-scher
Engli-sches
Engli-sche
Engli-schen
Engli-schem
englisch-sprachig
englisch-sprachi-ge
englisch-sprachi-gem
englisch-sprachi-gen
englisch-sprachi-ger
englisch-sprachi-ges
English
entitled
epsi-lon
equi-valent
equi-valence
especial-ly
essay
essays
estab-lish
evaluation
every
exist-ence
explain
explained
Ent-deckung
ent-schul-di-gen
Ent-wick-lung
Ent-wick-lun-gen
Ent-wurf
etab-lier-ter
etwas
every-where
exami-na-tion
exist
ex-peri-ence
Ex-peri-mente
existen-tial
extra-pola-tion
fach-wissen-schaft-liche
fach-wissen-schaft-lichen
Fach-be-reich
Fahr-zeu-gen
Falsi-fi-ka-tion
father
final
finally
finite
finitis-tic
focus
forma-tion
founda-tions
frequent
frequent-ly
further-more
general
ge-sicher-te
ge-sicher-tem
ge-sicher-ten
ge-sicher-ter
ge-sicher-tes
Ge-werk-schaft
glei-chen
Glei-chung
Glei-chun-gen
geo-metry
Geo-metrie
Gesamt-komplex
ge-sehen
Gestalt
grie-chi-sche
grie-chi-schem
grie-chi-schen
grie-chi-scher
grie-chi-sches
groun-ded-ness
glo-bal-ly 
Grund-lage
Grund-lagen
Grund-lagen-wissen-schaft 
Grund-lagen-wissen-schaf-ten 
guaran-tee-ing
Haltung
haupt-ver-ant-wort-lich
Haupt-ver-ant-wort-liche
Haupt-ver-ant-wort-lichem
Haupt-ver-ant-wort-lichen
Haupt-ver-ant-wort-licher
Haupt-ver-ant-wort-liches
have
Herbrand
hin-rei-chend
hin-rei-chen-de
hin-rei-chen-dem
hin-rei-chen-den
hin-rei-chen-der
hin-rei-chen-des
hyper-text
Hyper-texte
hypo-theses
hypo-thesis
hypo-the-size
hypo-the-sizing
idealis-ti-sche
idealis-ti-schem
idealis-ti-schen
idealis-ti-scher
idealis-ti-sches
ideali-za-tion
ihre
ihrem
ihren
ihrer
ihres
indeed
in-definite
index-ed
Induk-tions-be-wei-ser
Induk-tions-ord-nun-gen
Inferenz-systeme
in-finie
in-finite
in-formatics
inner-most
ins-ge-samt
interest
intro-duc-tion
irreflexive
Jahres-tref-fen
je-weils
Kai-sers-lau-tern
Kaplan
Kenn-zeichen
kenn-zeich-net
knowledge
knowledge-able
klassi-sche
klassi-schen
klassi-schem
klassi-scher
konnte
Kritik
kriti-sche
kriti-schen
kriti-schem
kriti-scher
kriti-sches
Kumu-la-tion
latter
leistet
lesen
little
logic
logics
logi-sche
logi-schen
logi-schem
logi-scher
logi-sches
magni-tude
mani-fold
mani-folds
mani-pu-la-tion
mathe-ma-tica
mathe-ma-tical
mathe-ma-tician
mathe-ma-ticians
mathe-ma-tics
Mathe-ma-tik
mathe-ma-ti-sche
mathe-ma-ti-schem
mathe-ma-ti-schen
mathe-ma-ti-scher
mathe-ma-ti-sches
method
methods
metho-di-cal
methodo-logi-sche
methodo-logi-schen
methodo-logi-schem
methodo-logi-scher
methodo-logi-sches
Mie-ter
Modell-klasse
modern
moder-ne
moder-nem
moder-nen
moder-ner
moder-nes
mono-toni-city
mora-lisch
mora-li-sche
mora-li-schen
mora-li-schem
mora-li-scher
mora-li-sches
Mieter-sache
Miet-vertrag
Miet-vertrages
mini-mum
mis-anthropic
mis-under-stood
mis-under-standing
mitt-lere
Musik
Nach-mieterin
natu-ral
Natur-wissen-schaft
Natur-wissen-schaf-ten
Neben-kosten
nega-tiv
nega-tive
neo-logism
never-the-less
Nomina-list
Nomina-listen
notable
nothing
notion
numeral
Ober-begriff
object
objects
Objekt
occur
occur-rence
occur-ren-ces
ohne
onto-logisch
onto-logi-sche
onto-logi-schem
onto-logi-schen
onto-logi-scher
onto-logi-sches
operationali-zation
order
Origi-nal
Origi-nals
Origi-nal-zitate
organi-sa-to-risch
organi-sa-to-ri-sche
organi-sa-to-ri-schem
organi-sa-to-ri-schen
organi-sa-to-ri-scher
organi-sa-to-ri-sches
other-wise
para-digm
Para-digma
Para-digmas
para-digms
Parallelen-axiom
para-meter
para-meters
parti-ci-pa-tion
philo-so-phisch
philo-so-phi-sche
philo-so-phi-schem
philo-so-phi-schen
philo-so-phi-scher
philo-so-phi-sches
parallel
poly-nomial
poly-nomials
posi-tiv
posi-tive
post-humously
product
pro-posi-tion
pro-posi-tions
pro-posi-tio-nal
ratio-nalis-mus
ratio-nalis-tisch 
ratio-nalis-tische 
ratio-nalis-tischem 
ratio-nalis-tischen 
ratio-nalis-tischer 
ratio-nalis-tisches 
really
Real-wissen-schaf-ten
recht-eckige
recht-eckigem
recht-eckigen
recht-eckiger
recht-eckiges
re-cog-nition
re-duci-bi-lity
Re-duk-tions-re-la-tion
regard-less
Regel
relation
relation-ship
relation-ships
re-organi-za-tion
repeti-tion
replace
represent
represents
represen-ted
represen-ting
repre-sen-ta-tion
require
requires
reso-lu-tion
result
Rhein-steig
Sammel-bezeich-nung 
schrift-lich
schwerere
Schwierig-keiten
second
seiten-gleich
seiten-gleiche
seiten-gleichem
seiten-gleichen
seiten-gleiches
seiten-gleicher
seman-tic
seman-tics
separa-tion
sequence
sequen-ces
several
sinn-voller
sitt-lich
sitt-liche
sitt-lichem
sitt-lichen
sitt-liches
sitt-licher
speaking
solu-tion
solu-tions
sophis-ti-ca-tion
Spezi-fi-ka-tio-nen
Spezi-fi-ka-tions-sprache
Sko-lem-i-za-tion
simpli-fi-cation
speci-fi-ca-tion
speci-fi-ca-tions
speci-fier
speci-fied
stable
sub-sequent
sym-metrical
sym-metrical-ly
tauto-logy
taking
tertium
theorem
theorems
Theorie
Theorien
theory
theo-re-ti-sche
theo-re-ti-schen
theo-re-ti-schem
theo-re-ti-sches
theo-re-ti-scher
thesis
topo-logy
total
trans-cend
typischer-weise
un-bestimmt
un-bestimmte
un-bestimm-tem
un-bestimm-ten
un-bestimm-ter
un-bestimm-tes
under
under-stand
under-stands
under-stood
unless
Un-par-tei-lich-keit
unter-bewusst
unter-schied
until
ur-element
ur-elements
Ur-sache
values
ver-an-lasst
Ver-an-stal-tung
Ver-bin-dung
ver-brei-ter-tem
Ver-mie-terin
ver-pflich-te-te
viel-leicht
Vor-annahme
Vor-annahmen
vor-kom-men-den
vor-para-dig-ma-ti-schen
vor-para-dig-ma-ti-scher
Vor-schrif-ten
wahr-ge-nom-men
weder
wei-te-ren
Weni-ger-ver-brauchs
wesent-liche
wesent-lichem
wesent-lichen
wesent-liches
wesent-licher
Win-kel
Wissen-schaft
Wissen-schaften
Wissen-schaft-ler
Wissen-schaft-lern
wissen-schaft-liche
wissen-schaft-lichen
wissen-schaft-licher
wissen-schaft-liches
Wissen-schafts-ent-wick-lung
wurde
zahl-reiche
zahl-reichen
zahl-reichem
zahl-reicher
zahl-reiches
zu-neh-men-den
zu-gleich
Zeich-nun-gen
zwei-sprachi-ge
zwei-sprachi-gem
zwei-sprachi-gen
zwei-sprachi-ger
zwei-sprachi-ges
Zweit-woh-nungs-steu-er
zwischen
}

\newcommand\majorfootroom{\raisebox{-1.9ex}{\rule{0ex}{.5ex}}}
\newcommand\mediumbigfootroom{\raisebox{-1.7ex}{\rule{0ex}{.5ex}}}
\newcommand\footroom{\raisebox{-1.5ex}{\rule{0ex}{.5ex}}}
\newcommand\mediumfootroom{\raisebox{-1.25ex}{\rule{0ex}{3ex}}}
\newcommand\smallfootroom{\raisebox{-1.0ex}{\rule{0ex}{3ex}}}

\newcommand\majorheadroom{\rule{0ex}{3.2ex}}
\newcommand\headroom{\rule{0ex}{2.8ex}}
\newcommand\mediumheadroom{\rule{0ex}{2.4ex}}
\newcommand\smallheadroom{\rule{0ex}{2.0ex}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% FIRST NAMES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\alan    {Alan}
\newcommand\albert  {Al\-bert}
\newcommand\alexander{Alex\-ander}
\newcommand\alfred  {Alfred}
\newcommand\andreas {An\-dre\-a\es}
\newcommand\andrew  {An\-drew}
\newcommand\bernd   {Bernd}
\newcommand\bernard {Bernard}
\newcommand\bernhard{Bern\-hard}
\newcommand\benjamin{Benjamin}
\newcommand\carl    {Carl}
\newcommand\carlos  {Car\-lo\es}
\newcommand\carsten {Car\esi ten}
\newcommand\catherine{{\namefont Catherine}}
\newcommand\charles {Charle\es}
\newcommand\charybdis{Charybdi\es}
\newcommand\christian{Christian}
\newcommand\christoph{Christoph}
\newcommand\claude  {Claude}
\newcommand\claus   {Clau\es}
\newcommand\david   {{\namefont David}}
\newcommand\donald  {Donald}
\newcommand\dieter  {Dieter}
\newcommand\dirk    {Dirk}
\newcommand\edmund  {\mbox{Edmund}}
\newcommand\edgar   {\mbox{Edgar}}
\newcommand\emil    {Emil}
\newcommand\ernst   {Ernst}
\newcommand\ferdinand{Ferdinand}
\newcommand\francois{Fran\-\c coi\es}
\newcommand\friedrich{Fried\-rich}
\newcommand\frank   {Frank}
\newcommand\gabriel {Gabri\ewithtrema l}
\newcommand\gerhard {Ger\-hard}
\newcommand\georg   {Georg}
\newcommand\george  {George}
\newcommand\gerd    {Gerd}
\newcommand\gottlob {Gott\-lob}
\newcommand\gustav  {Gustav}
\newcommand\hans    {Han\es}
\newcommand\helmut  {Hel\-mut}
\newcommand\heinrich{Hein\-rich}
\newcommand\henk    {Henk}
\newcommand\henry   {{\namefont Henry}}
\newcommand\herbert {Her\-bert}
\newcommand\hermann {Her\-mann}
\newcommand\horst   {Horst}
\newcommand\howard  {{\namefont Howard}}
\newcommand\hubert  {Hubert}
\newcommand\immanuel{Immanu\ewithtrema l}
\newcommand\immanuelwithouttrema{Immanuel}
\newcommand\irving  {Irving}
\newcommand\ismael  {Isma\ewithtrema l}
\newcommand\jacques {{\namefont Jacque\es}}
\newcommand\james   {Jame\es}
\newcommand\jan     {Jan}
\newcommand\joachim {Jo\-achim}
\newcommand\joerg   {J\oe rg}
\newcommand\johan   {Jo\-han}
\newcommand\jose    {Jos\'e}
\newcommand\joseph  {Joseph}
\newcommand\juergen {J\ue r\-gen}
\newcommand\jean    {Jean}
\newcommand\john    {John}
\newcommand\karl    {Karl}
\newcommand\klaus   {Klau\es}
\newcommand\konrad  {Kon\-rad}
\newcommand\kurt    {Kurt}
\newcommand\lawrence{Lawrence}
\newcommand\leon    {Leon}
\newcommand\leopold {Leo\-pold}
\newcommand\ludwig  {Lud\-wig}
\newcommand\magdalena{Magda\-lena}
\newcommand\manfred {Man\-fred}
\newcommand\maurice {{\namefont Maurice}}
\newcommand\maxchristiannamenonamefont{Max} %% \max is already a tex command
\newcommand\maxchristianname{{\namefont\maxchristiannamenonamefont}}
\newcommand\markus  {Mar\-ku\es}
\newcommand\martin  {Mar\-tin}
\newcommand\matthias{Matthia\es}
\newcommand\michael {Micha\-\ewithtrema l}%{Mi\-cha\-\ewithtrema l}
\newcommand\michaelwithouttrema{Micha\-el}%{Mi\-cha\-el}
\newcommand\nicolaus{Ni\-co\-lau\es}
\newcommand\ottonoconflict{Ot\-to}
\newcommand\paolo   {Paolo}
\newcommand\paul    {{\namefont Paul}}
\newcommand\peter   {Peter}
\newcommand\pierre  {Pierre}
\newcommand\raymond {Raymond}
\newcommand\rene    {Ren\'e}
\newcommand\redcap  {Red\-cap}
\newcommand\richard {Ri\-chard}
\newcommand\robert  {Ro\-bert}
\newcommand\roland  {Ro\-land}
\newcommand\rudolf  {Ru\-dolf}
\newcommand\ruediger{R\ue\-di\-ger}
\newcommand\scylla  {Scylla}
\newcommand\sergey  {Ser\-gey}
\newcommand\stanislaw{Stanis\l aw}
\newcommand\stanley {Stan\-ley}
\newcommand\stephan {Ste\-phan}
\newcommand\thomas  {Tho\-ma\es}
\newcommand\thoralf {{\namefont Thoralf}}
\newcommand\tobias  {{\namefont To\-bi\-a\es}}
\newcommand\wolfgang{Wolf\-gang}
\newcommand\ulrich  {Ul\-rich}
\newcommand\ulysses {Ulysse\es}
\newcommand\uwe     {Uwe}
\newcommand\vladimir{Vla\-di\-mir}
\newcommand\volker  {\mbox{Vol\-ker}}
\newcommand\werner  {Wer\-ner}
\newcommand\wilfried{Wil\-fried}
\newcommand\wilhelm {\mbox{Wilhelm}}
\newcommand\william {Will\-iam}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SCIENTISTS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\aanderaa        {{\namefont Aanderaa}}
\newcommand\aanderaaname    {{\namefont St\aa l \aanderaa}}
\newcommand\abel            {{\namefont Abel}}
\newcommand\abelname        {{\namefont Niel\es\ Henrik \abel}} % verified
\newcommand\abellifetime    {(1802--1829)} % verified
\newcommand\acerbi          {{\namefont Acerbi}}
\newcommand\acerbiname      {{\namefont Fabio \acerbi}}
\newcommand\ackermannindex  {\index{Ackermann!Wilhelm}}
\newcommand\ackermann       {{\namefont Acker\-mann}}
\newcommand\ackermannname   {\ackermannindex{\namefont \wilhelm\ \ackermann}}
\newcommand\ackermannlifetime{(1896--1962)}
\newcommand\aczel           {{\namefont Aczel}}
\newcommand\aczelname       {{\namefont \peter\ \aczel}}
\newcommand\adorno          {Adorno}
\newcommand\adornoname      {Theodor W. \adorno}
\newcommand\ahrendt         {{\namefont Ahrendt}}
\newcommand\ahrendtname     {{\namefont\wolfgang\ \ahrendt}}
\newcommand\ajdukiewicz     {Ajdukiewicz}
\newcommand\ajdukiewiczname {Kazimierz \ajdukiewicz}
\newcommand\ajdukiewiczlifetime{(1890--1963)}
\newcommand\anellis         {{\namefont Anelli\es}}
\newcommand\anellisname     {{\namefont\irving\ H. \anellis}}
\newcommand\anellislifetime {(*1946)}
\newcommand\albertus        {{\namefont Albertu\es}}
\newcommand\albertusname    {{\namefont\albertus\ Magnu\es}}
\newcommand\albertuslifetime{(\ca\,1200--1280)}
\newcommand\anselm          {{\namefont Anselmu\es}}
\newcommand\anselmname      {{\namefont\anselm\ Cantuariensi\es}}
\newcommand\anselmlifetime  {(1033--1109)}
\newcommand\artin           {{\namefont Artin}}
\newcommand\artinname       {{\namefont \emil\ \artin}}
\newcommand\artinlifetime   {(1898--1962)}
\newcommand\aristotle       {{\namefont Ari\esi totle}}
\newcommand\aristotlename   {{\namefont\aristotle\ of Stagira}}
\newcommand\aristotlelifetime{(384--322\,\BC)}
\newcommand\aristotelian    {{\namefont Ari\esi totelian}}
\newcommand\aristotelisch   {{\namefont Ari\esi totelisch}}
\newcommand\aristoteles     {{\namefont Ari\esi toteles}}
\newcommand\aristotelesname {{\namefont Ari\esi toteles von Stagira}}
\newcommand\aristoteleslifetime{(384--322\,v.\,Chr.)}
\newcommand\armando         {Armando}
\newcommand\armandoname     {Alessandro \armando}
\newcommand\asser           {{\namefont Asser}}
\newcommand\assername       {{\namefont G\ue nter \asser}}
\newcommand\asserlifetime   {(born\,1926)}
\newcommand\andrews         {\mbox{\namefont Andrew\es}}
\newcommand\andrewsname     {{\namefont\peter\ B. \andrews}}
\newcommand\andrewsnamewithoutmiddleinitial{{\namefont\peter\ \andrews}}
\newcommand\andrewslifetime {(*1937)}
\newcommand\augustinus      {{\namefont Augu\esi tinus}}
\newcommand\augustinusname  {{\namefont \augustinus\ Hipponensis}}
\newcommand\augustinuslifetime{(354--430)}
\newcommand\autexier        {\mbox{\namefont Autexier}}
\newcommand\autexiername    {{\namefont Serge \autexier}}
\newcommand\avenhaus        {{\namefont Aven\-hau\es}}
\newcommand\avenhausname    {{\namefont\juergen\ \avenhaus}}
\newcommand\avron           {{\namefont Avron}}
\newcommand\avronname       {{\namefont Arnon \avron}}
\newcommand\awodey          {{\namefont Awodey}}
\newcommand\awodeyname      {{\namefont Steve \awodey}}
\newcommand\baaz            {{\namefont Baaz}}
\newcommand\baazname        {{\namefont\matthias\ \baaz}}
\newcommand\babbage         {Babbage}
\newcommand\babbagename     {\charles\ \babbage}
\newcommand\babbagelifetime {(1792--1871)}
\newcommand\bach            {Bach}
\newcommand\bachname        {Emmon \bach}
\newcommand\bachet          {Bachet}
\newcommand\bachetname      {\claude\ Gaspard \bachet\ de M\'eziriac}
\newcommand\bachetlifetime  {(1581--1638)}
\newcommand\bachmair        {Bach\-mair}
\newcommand\bachmairname    {Leo \bachmair}
\newcommand\backhouse       {Backhouse}
\newcommand\backhousename   {\roland\ \backhouse}
\newcommand\bacon           {Bacon}
\newcommand\baconname       {Franci\es\ \bacon}
\newcommand\barendregt      {Barendregt}
\newcommand\barendregtname  {Hen(dri)k P. \barendregt}
\newcommand\barwise         {{\namefont Barwise}}
\newcommand\barwisename     {{\namefont Jon \barwise}}
\newcommand\basin           {{\namefont Basin}}
\newcommand\basinname       {{\namefont\david\ \basin}}
\newcommand\bauermengelberg {{\namefont Bauer-Mengelberg}}
\newcommand\bauermengelbergname{{\namefont Stefan \bauermengelberg}}
\newcommand\baumgartner     {Baum\-gart\-ner}
\newcommand\baumgartnername {\peter\ \baumgartner}
\newcommand\becker          {Becker}
\newcommand\beckername      {\klaus\ \becker}
\newcommand\beckert         {{\namefont Beckert}}
\newcommand\beckertname     {{\namefont\bernhard\ \beckert}}
\newcommand\bell            {Bell}
\newcommand\bellname        {\john\ Lane \bell}
\newcommand\beethoven       {Beethoven}
\newcommand\beethovenname   {\ludwig\ van \beethoven}
\newcommand\beethovenlifetime{(1770--1827)}
\newcommand\behmannindex    {\index{Behmann, Heinrich}}
\newcommand\behmann         {{\namefont Behmann}}
\newcommand\behmannname     {\behmannindex{\namefont\heinrich\ \behmann}}
\newcommand\bendix          {Bendix}
\newcommand\bendixname      {P. B. \bendix}
\newcommand\benzmueller     {{\namefont Benz\-m\ue ller}}
\newcommand\benzmuellername {{\namefont\christoph\ \benzmueller}}
\newcommand\berghammer      {Berg\-hammer}
\newcommand\berghammername  {\rudolf\ \berghammer}
\newcommand\bergstra        {{\namefont Bergstra}}
\newcommand\bergstraname    {{\namefont\jan\ A. \bergstra}}
\newcommand\berkeley        {{\namefont Berkeley}}
\newcommand\berkeleyname    {{\namefont \george\ \berkeley}}
\newcommand\berkeleylifetime{(1685--1753)}
\newcommand\bernaysindex    {\index{Bernays, Paul}}
\newcommand\bernays         {\mbox{\namefont Ber\-nay\es}}
\newcommand\bernaysname     {\bernaysindex{\namefont \paul\ \bernays}}
%                           {{\namefont \paul\ Isaak \bernays}}
\newcommand\bernaysschoenfinkel{\bernays--\schoenfinkel}
\newcommand\bernayslifetime {(1888--1977)}
\newcommand\bernstein       {{\namefont Bernstein}}
\newcommand\bernsteinname   {{\namefont Felix \bernstein}}
\newcommand\bernsteinlifetime{(1878--1956)}
\newcommand\bertling        {{\namefont Bertling}}
\newcommand\bertlingname    {{\namefont\hubert\ \bertling}}
\newcommand\bevers          {Bever\es}
\newcommand\beversname      {Eddy \bevers}
\newcommand\bibel           {{\namefont Bi\-bel}}
\newcommand\bibelname       {{\namefont\wolfgang\ \bibel}}
\newcommand\billy           {{\namefont Billy}}
\newcommand\billyname       {{\namefont\jacques\ de \billy}}
\newcommand\billylifetime   {(1602--1679)}
\newcommand\bledsoe         {{\namefont Bledsoe}}
\newcommand\bledsoename     {{\namefont Woody \bledsoe}}
\newcommand\bledsoelifetime {(1921--1995)}
\newcommand\bohr            {Bohr}
\newcommand\bohrname        {Nil\es\ \bohr}
\newcommand\bolzano         {{\namefont Bolzano}}
\newcommand\bolzanoname     {{\namefont\bernard\ \bolzano}}
\newcommand\bolzanolifetime {(1781--1848)}
\newcommand\bookhade        {Bookhade}
\newcommand\bookhadename    {\robert\ \bookhade}
\newcommand\boole           {{\namefont Boole}}
\newcommand\boolename       {{\namefont\george\ \boole}}
\newcommand\boolelifetime   {(1815--1864)}
\newcommand\myboolean       {Boolean}
\newcommand\boolos          {{\namefont Boolos}}
\newcommand\boolosname      {{\namefont\george\ \boolos}}
\newcommand\booloslifetime  {(1940--1996)}
\newcommand\born            {{\namefont Born}}
\newcommand\bornname        {{\namefont\maxchristianname\ \born}}
\newcommand\bouhoula        {Bou\-hou\-la}
\newcommand\bouhoulaname    {Adel \bouhoula}
\newcommand\bourbakiindex   {\index{Bourbaki, Nicolas}}
\newcommand\bourbaki        {{\namefont Bourbaki}}
\newcommand\bourbakiname    {\bourbakiindex{\namefont Nicola\es\ \bourbaki}}
\newcommand\boyer           {{\namefont Boyer}}
\newcommand\boyername       {{\namefont\robert\ S. \boyer}}
\newcommand\brahe           {Brahe}
\newcommand\brahename       {Tyge \brahe}%{Tyge B. \brahe}
\newcommand\brahelifetime   {(1546--1601)}
\newcommand\brentano        {{\namefont Brentano}}
\newcommand\brentanopoetname{{\namefont Clemens \brentano}}
\newcommand\brentanopoetlifetime{(1778--1842)}
\newcommand\brentanophilosophername{{\namefont Franz \brentano}}
\newcommand\brentanophilosopherlifetime{(1838--1917)}
\newcommand\bronsard        {{\namefont Bronsard}}
\newcommand\bronsardname    {{\namefont\francois\ \bronsard}}
\newcommand\brotherston     {{\namefont Brotherston}}
\newcommand\brotherstonname {{\namefont\james\ \brotherston}}
\newcommand\brouwersecondname{Brouwer} % Not: Brouwers (as often written)
\newcommand\brouwerfirstname{L. E. J.}
%{Luitzen}
%{Luitzen E. J.}
%Parsons: Also, Brouwer always referred to himself in print as L. E. J. Brouwer; that is the way most other writers have referred to him.  I don't know if anyone called him Luitzen; from van Dalen's biography, it is clear that he was known familiarly as Bertus (after Egbertus, his second Christian name).
\newcommand\brouwerindex    {\index{Brouwer, L. E. J.}}
\newcommand\brouwer         {{\namefont \brouwersecondname}}
\newcommand\brouwername     
                {\brouwerindex{\namefont \brouwerfirstname\ \brouwersecondname}}
\newcommand\brouwerlifetime {(1881--1966)}
\newcommand\brownchad       {{\namefont Brown}}
\newcommand\brownchadname   {{\namefont Chad E. \brownchad}}
\newcommand\broy            {Broy}
\newcommand\broyname        {\manfred\ \broy}
\newcommand\bruggaier       {Bruggaier}
\newcommand\bruggaiername   {Juliana \bruggaier}
\newcommand\bruijn          {Bruijn}
\newcommand\bruijnname      {Nicolaa\es\ Govert de \bruijn}
\newcommand\buchholz        {{\namefont Buch\-holz}}
\newcommand\buchholzname    {{\namefont\wilfried\ \buchholz}}
\newcommand\buechi          {{\namefont B\ue chi}}
\newcommand\buechiname      {{\namefont Julius \richard\ \buechi}}
\newcommand\buechilifetime  {(1924--1984)}
\newcommand\buerckert       {B\ue rckert}
\newcommand\buerckertname   {\hans-\juergen\ \buerckert}
\newcommand\buldtindex      {\index{Buldt, Bernd}}
\newcommand\buldt           {{\namefont Buldt}}
\newcommand\buldtname       {\buldtindex{\namefont \bernd\ \buldt}}
\newcommand\bundy           {{\namefont Bundy}}
\newcommand\bundyname       {{\namefont\alan\ \bundy}}
                          %{\alan\ R. \bundy}
\newcommand\burris          {Burri\es}
\newcommand\burrisname      {\stanley\ \burris}
\newcommand\bush            {Bush}
\newcommand\bushname        {Vannevar \bush}
\newcommand\bussotti        {{\namefont Bussotti}}
\newcommand\bussottiname    {{\namefont\paolo\ \bussotti}}
\newcommand\byrnes          {Byrne\es}
\newcommand\byrnesname      {\john\ \byrnes}
\newcommand\caferra         {{\namefont Caferra}}
\newcommand\caferraname     {{\namefont Ricardo \caferra}}
\newcommand\cantone         {{\namefont Cantone}}
\newcommand\cantonename     {{\namefont Domenico \cantone}}
\newcommand\cantorindex     {\index{Cantor!Georg}}
\newcommand\cantor          {{\namefont Cantor}}
\newcommand\cantorname      {\cantorindex{\namefont\georg\ \cantor}}
\newcommand\cantorlifetime  {(1845--1918)}
\newcommand\carcavi         {{\namefont Carcavi}}
\newcommand\carcaviname     {{\namefont\pierre\ de \carcavi}}
\newcommand\carnap          {{\namefont Carnap}}
\newcommand\carnapname      {{\namefont\rudolf\ \carnap}}
\newcommand\carnaplifetime  {(1891--1970)}
\newcommand\carroll         {Carroll}
\newcommand\carrollname     {Lewi\es\ \carroll}
\newcommand\carrolltrue     {Dodgson}
\newcommand\carrolltruename {\charles\ Lutwidge \carrolltrue}
\newcommand\carrolllifetime {(1832--1898)}
\newcommand\cassirer        {{\namefont Cassirer}}
\newcommand\cassirername    {{\namefont\ernst\ \cassirer}}
\newcommand\cate            {{\namefont Ten Cate}}
\newcommand\catename        {{\namefont Balder \cate}}
\newcommand\cauchyindex     {\index{Cauchy!Augustin Louis}}
\newcommand\cauchy          {{\namefont Cauchy}}
\newcommand\cauchyname      {\cauchyindex{\namefont Augustin Louis \cauchy}}
\newcommand\cauchylifetime  {(1789-1857)}
\newcommand\cavaillesname   {Jean Cavaill\`e\es}
\newcommand\cavailleslifetime{(1903--1944)}
\newcommand\cerrito         {Cerrito}
\newcommand\cerritoname     {Serenella \cerrito}
\newcommand\lassaadsecondname{{\namefont Cheikh\-rou\-hou}}
\newcommand\lassaadname     {{\namefont Las\-saad \lassaadsecondname}}
\newcommand\chrysippos      {Chrysippu\es}
\newcommand\chrysipposname  {\chrysippos\ of Soloi (Asia Minor)}
\newcommand\chrysipposlifetime{(\nth 3\,century\,\BC)}
\newcommand\chrysippossentence{\chrysippos\ sentence}
\newcommand\chevalley       {{\namefont Chevalley}}
\newcommand\chevalleyname   {{\namefont\claude\ \chevalley}}
\newcommand\chevalleylifetime{(1909--1984)}
\newcommand\churchindex     {\index{Church, Alonzo}}
\newcommand\church          {{\namefont Church}}
\newcommand\churchname      {\churchindex{\namefont Alonzo \church}}
\newcommand\churchlifetime  {(1903--1995)}
\newcommand\churchrosser    {\church--\rosser}
\newcommand\churchrossertheorem{\churchrosser\ Theorem}
\newcommand\cialdea         {Cialdea}
\newcommand\cialdeaname     {Marta \cialdea}
\newcommand\clausius        {{\namefont Clausius}}
\newcommand\clausiusname    {{\namefont\rudolf\ \clausius}}
\newcommand\cleanthes       {Cleanthe\es}
\newcommand\cleanthesname   {\cleanthes\ of Asso\es}
\newcommand\corcoran        {{\namefont Corcoran}}
\newcommand\corcoranname    {{\namefont\john\ \corcoran}}
\newcommand\comon           {{\namefont Comon}}
\newcommand\comonname       {{\namefont\hubert\ \comon}}
\newcommand\costa           {{\namefont Costa}}
\newcommand\costaname       {{\namefont Newton C. A. da \costa}}
\newcommand\courant         {{\namefont Courant}}
\newcommand\courantname     {{\namefont\richard\ \courant}}
\newcommand\courantlifetime {(1988--1972)}
\newcommand\craig           {Craig}
\newcommand\craigname       {\william\ \craig}
\newcommand\craigsinterpolationtheorem{\craig's Interpolation Theorem}
\newcommand\crelle          {{\namefont Crelle}}
\newcommand\crellename      {{\namefont August \leopold\ \crelle}}
\newcommand\crellelifetime  {(1780--1855)}
\newcommand\crossleyindex   {\index{Crossley, John N.}}
\newcommand\crossley        {{\namefont Crossley}}
\newcommand\crossleyname    {\crossleyindex{\namefont John N. \crossley}}
\newcommand\dalen           {{\namefont Dalen}}
\newcommand\dalenname       {{\namefont\dirk\ van \dalen}}
\newcommand\dalenlifetime   {(born\,1932)}
\newcommand\dalton          {Dalton}
\newcommand\daltonname      {\john\ \dalton}
\newcommand\daltonlifetime  {(1766--1844)}
\newcommand\davis           {{\namefont Davis}}
\newcommand\davisname       {{\namefont\martin\ \davis}}
\newcommand\davislifetime   {(born\,1928)}
\newcommand\dawson          {{\namefont Dawson}}
\newcommand\dawsonname      {{\namefont\john\ W. \dawson\ \jr}}
\newcommand\dieudonne       {{\namefont Dieudonn\'e}}
\newcommand\dieudonnename   {{\namefont\jean\ \dieudonne}}
\newcommand\dieudonnelifetime{(1906--1992)}
\newcommand\dillerindex     {\index{Diller, Justus}}
\newcommand\diller          {{\namefont Diller}}
\newcommand\dillername      {\dillerindex{\namefont Justu\es\ \diller}}
\newcommand\diophantus      {{\namefont Dio\-phan\-tu\es}}
\newcommand\diophantusname  {{\namefont\diophantus\ of Alexandria}}
\newcommand\diophantuslifetime{(\nth 3\,century?)}
\newcommand\dedekindindex   {\index{Dedekind!Richard}}
\newcommand\dedekind        {{\namefont Dedekind}}
\newcommand\dedekindname    {\dedekindindex{\namefont\richard\ \dedekind}}
                           %{J. W. \richard\ \dedekind}
\newcommand\dedekindlifetime{(1831--1916)}
\newcommand\degtyarev       {{\namefont Degtyarev}}
\newcommand\degtyarevname   {{\namefont Anatoli \degtyarev}}
\newcommand\demorgan        {De-Morgan}
\newcommand\demorganname    {Augustus \demorgan}
\newcommand\demorganlifetime{(1806--1871)}
\newcommand\denjoy          {{\namefont Denjoy}}
\newcommand\denjoyname      {{\namefont Arnaud Denjoy}}
\newcommand\denjoylifetime  {(1884--1974)} % verified
\newcommand\denton          {{\namefont Denton}}
\newcommand\dentonname      {{\namefont\john\ \denton}}
\newcommand\dershowitz      {{\namefont Dersho\-witz}}
\newcommand\dershowitzname  {{\namefont Nachum \dershowitz}}
\newcommand\descartes       {{\namefont De\esi carte\es}}
\newcommand\descartesname   {{\namefont\rene\ \descartes}}
\newcommand\descarteslifetime{(1596--1650)}
\newcommand\devidi          {DeVidi}
\newcommand\devidiname      {\david\ \devidi}
\newcommand\dietrich        {{\namefont Diet\-rich}}
\newcommand\dietrichname    {{\namefont Dominik \dietrich}}
\newcommand\dixnoconflict   {Dix}
\newcommand\dixname         {\juergen\ \dixnoconlflict}
\newcommand\dixon           {{\namefont Dixon}}
\newcommand\dixonname       {{\namefont Luca\es\ \dixon}}
\newcommand\doornbos        {Doornbo\es}
\newcommand\doornbosname    {\henk\ \doornbos}
\newcommand\drebenindex     {\index{Dreben, Burton}}
\newcommand\dreben          {{\namefont Dreben}}
\newcommand\drebenname      {\drebenindex{\namefont Burton \dreben}}
\newcommand\drebenlifetime  {(1927--1999)}
\newcommand\dunsscotus      {{\namefont Duns-Scotus}}
\newcommand\dunsscotusname  {{\namefont Johannes \dunsscotus}}
\newcommand\dunsscotuslifetime{(1265?--1308)}
\newcommand\ebertindex      {\index{Ebert, Philip}}
\newcommand\ebert           {{\namefont Ebert}}
\newcommand\ebertname       {\ebertindex{\namefont Philip \ebert}}
\newcommand\ebbinghaus      {{\namefont Ebbinghau\es}}
\newcommand\ebbinghauseinsname{{\namefont Heinz-Dieter \ebbinghaus}}
\newcommand\eckmann         {{\namefont Eckmann}}
\newcommand\eckmannname     {{\namefont Beno \eckmann}}
\newcommand\egli            {{\namefont Egli}}
\newcommand\egliname        {{\namefont Ur\es\ \egli}}
\newcommand\egly            {Egly}
\newcommand\eglyname        {\uwe\ \egly}
\newcommand\ehrenfels       {Ehrenfel\es}
\newcommand\ehrenfelsname   {\christian\ von \ehrenfels}
\newcommand\ehrenfelslifetime{(1859--1932)}
\newcommand\ehrig           {{\namefont Ehrig}}
\newcommand\ehrigname       {{\namefont Hartmut \ehrig}}
\newcommand\eijck           {{\namefont Eijck}}
\newcommand\eijckname       {{\namefont \jan\ van \eijck}}
\newcommand\elsenbroichindex{\index{Elsenbroich, Corinna}}
\newcommand\elsenbroich     {{\namefont Elsenbroich}}
\newcommand\elsenbroichname {\elsenbroichindex{\namefont Corinna \elsenbroich}}
\newcommand\einstein        {{\namefont Ein\-stein}}
\newcommand\einsteinname    {{\namefont\albert\ \einstein}}
\newcommand\einsteinlifetime{(1879--1955)}
\newcommand\eisenstein      {{\namefont Eisenstein}}
\newcommand\eisensteinname  {{\namefont Gotthold \eisenstein}}
%                           {\ferdinand\ Gotthold Max \eisenstein}
\newcommand\eisensteinlifetime{(1823--1852)}
\def       \enderton        {{\namefont Enderton}}
%newcommand has problems with \end..
\def       \endertonname    {{\namefont\herbert\ B. \enderton}}
\newcommand\engels          {\mbox{\namefont Engels}}
\newcommand\engelsname      {{\namefont\friedrich\ \engels}}
\newcommand\engesserindex   {\index{Engesser, Kurt}}
\newcommand\engesser        {{\namefont Engesser}}
\newcommand\engessername    {\engesserindex{\namefont\kurt\ \engesser}}
\newcommand\eschbach        {Esch\-bach}
\newcommand\eschbachname    {\robert\ \eschbach}
\newcommand\euclidindex     {\index{Euclid!of Alexandria}}
\newcommand\euclid          {{\namefont Euclid}}
\newcommand\euclidname      {\euclidindex{\namefont\euclid\ of Alexandria}}
\newcommand\euclidlifetime  {(\ca\ 300\,\BC)}
\newcommand\euler           {{\namefont Euler}}
\newcommand\euklid          {{\namefont Euklid}}
\newcommand\eulername       {{\namefont Leon\-hard \euler}}
\newcommand\eulerlifetime   {(1707--1783)}
\newcommand\ewald           {{\namefont Ewald}}
\newcommand\ewaldeinsname   {{\namefont \peter\ \paul\ \ewald}}
\newcommand\ewaldeinslifetime{(1888--1985)}
\newcommand\ewaldzweiname   {{\namefont \william\ \ewald}}
                           %{{\namefont \william\ Bragg \ewald}}
\newcommand\faltings        {{\namefont Faltings}}
\newcommand\faltingsname    {{\namefont \gerd\ \faltings}}
\newcommand\faraday         {Faraday}
\newcommand\feferman        {{\namefont Fefer\-man}}
\newcommand\fefermanname    {{\namefont Sol(omon) \feferman}}
\newcommand\fefermanlifetime{(*1928)}
\newcommand\fefermanshename {Anita Burdman \feferman}
\newcommand\fenstad         {{\namefont Fenstad}}
\newcommand\fenstadname     {{\namefont Jen\es\ E. \fenstad}}
\newcommand\fermat          {\mbox{\namefont Fermat}}
\newcommand\fermatname      {{\namefont \pierre\ \fermat}}
\newcommand\fermatnoblename {{\namefont\pierre\ {\em de} \fermat}}
\newcommand\fermatbirthyear {1607?}
\newcommand\fermatdeathyear {1665}
\newcommand\fermatlifetime  {(\fermatbirthyear--\fermatdeathyear)}
\newcommand\letterforhuygensyear{1659}
\newcommand\letterforhuygenstitle
              {Relation des nouvelles d\'ecouvertes en la science des
              nombres}
\newcommand\letterforhuygensproofcitation
                           {\cite[\Vol\,1, \p\,431\f]{fermat-oeuvres}}
\newcommand\fermatsprofession{conseilleur au parlement de Toulouse%
%et commissaire aux requ\^etes
% Das ist nur die Anfaengerposition!!!
}
\newcommand\fermatstitle    {\'eculier}
\newcommand\fermatslasttheorem{\fermat's Last Theorem}
\newcommand\fermueller      {{\namefont Fer\-m\ue ller}}
\newcommand\fermuellername  {{\namefont\christian\ G. \fermueller}}
\newcommand\fettig          {Fet\-tig-Vogt}
\newcommand\fettigname      {\roland\ \fettig}
\newcommand\feyerabend      {Feyer\-abend}
\newcommand\feyerabendname  {\paul\ \feyerabend}%{\paul\ K. \feyerabend}
\newcommand\feyerabendlifetime{(1924--1994)}
\newcommand\fiedler         {{\namefont Fiedler}}
\newcommand\fiedlername     {{\namefont Armin \fiedler}}
\newcommand\fitting         {{\namefont Fitting}}
\newcommand\fittingname     {{\namefont Melvin       \fitting}}
%                           {{\namefont Melvin C.    \fitting}}
%                           {{\namefont Melvin Ch.   \fitting}}
%                           {{\namefont Melvin Chris \fitting}}
\newcommand\fleuriot        {{\namefont Fleuriot}}
\newcommand\fleuriotname    {{\namefont\jacques\ \fleuriot}}
\newcommand\foellesdal      {{\namefont F\o llesdal}}
\newcommand\foellesdalname  {{\namefont Dagfinn \foellesdal}}
\newcommand\fourcolortheorem{Four-Color Theorem}
\newcommand\fraenkel        {{\namefont Fraenkel}}
\newcommand\fraenkelname    {{\namefont Adolf Abraham \fraenkel}}
\newcommand\fraenkellifetime{(1891--1965)}
\newcommand\franke          {{\namefont Franke}}
\newcommand\frankename      {{\namefont\andreas\ \franke}}
\newcommand\fraus           {Frau\es}
\newcommand\frausname       {\ulrich\ \fraus}
\newcommand\frechet         {{\namefont Fr\'echet}}
\newcommand\frechetname     {{\namefont Maurice Ren\'e Fr\'echet}}
\newcommand\frechetlifetime {(1878--1973)} % verified
\newcommand\fregeindex      {\index{Frege, Gottlob}}
\newcommand\frege           {{\namefont Frege}}
\newcommand\fregename       {\fregeindex{\namefont \gottlob\ \frege}}
                               %{F. L. \gottlob\ \frege}
\newcommand\fregelifetime   {(1848--1925)} 
\newcommand\Begriffsschrift {Begriff\esi schrift}
\newcommand\frenicle        {{\namefont Fr\'enicle}}
\newcommand\freniclename    {{\namefont\bernard\ \frenicle\ de Bessy}}
\newcommand\freniclelifetime{(1605?--1675)} 
\newcommand\freud           {{\namefont Freud}}
\newcommand\freudname       {{\namefont Sigmund \freud}}
\newcommand\freudlifetime   {(1856--1939)} 
\newcommand\fricke          {{\namefont Fricke}}
\newcommand\frickename      {{\namefont \robert\ \fricke}}
\newcommand\frickelifetime  {(1861--1930)}
\newcommand\furbach         {Furbach}
\newcommand\furbachname     {\ulrich\ \furbach}
\newcommand\furtwaengler    {Furt\-w\ae ngler}
\newcommand\furtwaenglername{\wilhelm\ \furtwaengler}
\newcommand\furtwaenglerlifetime{(1886--1954)}
\newcommand\galilei         {{\namefont Gali\-lei}}
\newcommand\galileiname     {{\namefont Gali\-leo \galilei}}
\newcommand\galileilifetime {(1564--1642)}
\newcommand\gaillard        {{\namefont Gaillard}}
\newcommand\gaillardname    {{\namefont \francois\ \gaillard}}
\newcommand\galois          {{\namefont Galoi\es}}
\newcommand\galoisname      {{\namefont Evariste \galois}}
\newcommand\galoislifetime  {(1811--1832)}
\newcommand\gabbaydovindex  {\index{Gabbay!Dov}}
\newcommand\gabbay          {{\namefont Gabbay}}
\newcommand\gabbayname      {\gabbaydovindex{\namefont Dov \gabbay}}
%                           {{\namefont Dov M. \gabbay}}
\newcommand\jamiegabbayindex{\index{Gabbay!Murdoch J.}}
\newcommand\jamiegabbayname {\jamiegabbayindex{\namefont Murdoch J. \gabbay}}
\newcommand\michaelgabbayindex{\index{Gabbay!Michael}}
\newcommand\michaelgabbayname{\michaelgabbayindex{\namefont\michaelwithouttrema\ \gabbay}}
\newcommand\gallier         {Gallier}
\newcommand\galliername     {\jean\ \gallier}
\newcommand\ganzinger       {Gan\-zin\-ger}
\newcommand\ganzingername   {Harald \ganzinger}
\newcommand\gauss           {{\namefont Gau\sz}}
\newcommand\gaussname       {{\namefont\carl\ \friedrich\ \gauss}}
\newcommand\gausslifetime   {(1777--1855)}
\newcommand\gentzenindex    {\index{Gentzen!Gerhard}}
\newcommand\gentzen         {{\namefont Gentzen}}
\newcommand\gentzenname     {\gentzenindex{\namefont\gerhard\ \gentzen}}
\newcommand\gentzenlifetime {(1909--1945)}
\newcommand\gentzensHauptsatz{{\namefont\gentzen}'\es\ {\germanfont \Hauptsatz}}
\newcommand\gentzensverschaerfterHauptsatz
{{\namefont\gentzen}'\es\ {\germanfont\verschaerfterHauptsatz}}
\newcommand\gentzensverschaerfterHauptsatzfootnote
{{\namefont\gentzen}'\es\ {\germanfontfootnote\verschaerfterHauptsatz}}
\newcommand\verschaerfterHauptsatz{Ver\-sch\ae rf\-ter \Hauptsatz}
\newcommand\Hauptsatz{Haupt\-satz}
\newcommand\gerson          {{\namefont Gerson}}
\newcommand\gersonname      {{\namefont Levi ben \gerson}}
\newcommand\gersonlifetime  {(1288--1344)}
\newcommand\geurts          {Geurt\es}
\newcommand\geurtsname      {Bart \geurts}
\newcommand\geser           {Geser}
\newcommand\gesername       {Alfons \geser}
\newcommand\giese           {{\namefont Giese}}
\newcommand\giesename       {{\namefont\martin\ \giese}}
\newcommand\giesl           {Giesl}
\newcommand\gieslname       {\juergen\ \giesl}
\newcommand\gilmore         {{\namefont Gilmore}}
\newcommand\gilmorename     {{\namefont\paul\ C. \gilmore}}
\newcommand\gilmorelifetime {(born\,1925)}
\newcommand\goedelindex     {\index{Goedel@G\"odel!Kurt}}
\newcommand\goedel          {{\namefont G\oe del}}
\newcommand\goedelname      {\goedelindex{\namefont \kurt\ \goedel}}
\newcommand\goedellifetime  {(1906--1978)}
\newcommand\goedelssecondincompletenesstheorem
{\goedel'\es\ \secondincompletenesstheorem}
\newcommand\goedelssecondIncompletenessTheorem
{\goedel'\es\ \secondIncompletenessTheorem}
\newcommand\secondincompletenesstheorem
% {\nth 2 \incompletenesstheorem}
{second \incompletenesstheorem}
\newcommand\secondIncompletenessTheorem
% {\nth 2 \IncompletenessTheorem}
{Second \IncompletenessTheorem}
\newcommand\incompletenesstheorem{incompleteness theorem}
\newcommand\IncompletenessTheorem{Incompleteness Theorem}
\newcommand\goethe          {{\namefont G\oe the}}
\newcommand\goethename      {{\namefont Johann \wolfgang\ von \goethe}}
\newcommand\gogolla         {Gogolla}
\newcommand\gogollaname     {\martin\ \gogolla}
\newcommand\goguen          {{\namefont Goguen}}
\newcommand\goguenname      {{\namefont\joseph\ \goguen}}
\newcommand\goldbachname    {{\namefont\christian\ \goldbach}}
\newcommand\goldbach        {{\namefont Gold\-bach}}
\newcommand\goldbachlifetime{(1690--1764)}
\newcommand\goldbachsconjecture{\goldbach's Conjecture}
\newcommand\goldfarb        {{\namefont Gold\-farb}}
\newcommand\goldfarbname    {{\namefont Warren %D.
                              \goldfarb}}
\newcommand\goldstein       {{\namefont Gold\-stein}}
\newcommand\goldsteinname   {{\namefont\catherine\ \goldstein}}
\newcommand\gonseth         {{\namefont Gonseth}}
\newcommand\gonsethname     {{\namefont \ferdinand\ \gonseth}}
\newcommand\gow             {{\namefont Gow}}
\newcommand\gowname         {{\namefont Jeremy \gow}}
\newcommand\gramlich        {{\namefont Gram\-lich}}
\newcommand\gramlichname    {{\namefont\bernhard\ \gramlich}}
\newcommand\greensurname    {{\namefont Green}}
\newcommand\greenname       {{\namefont Ian \greensurname}}
\newcommand\grimm           {Grimm}
\newcommand\grimmjacobname  {Jacob \grimm}
\newcommand\grimmwilhelmname{\wilhelm\ \grimm}
\newcommand\guillaume       {{\namefont Guillaume}}
\newcommand\guillaumename   {{\namefont Marcel \guillaume}}
\newcommand\gurevich        {{\namefont Gurevich}}
\newcommand\gurevichname    {{\namefont Yuri \gurevich}}
\newcommand\hadamard        {{\namefont Hadamard}}
\newcommand\hadamardname    {{\namefont\jacques\ Salomon \hadamard}}
\newcommand\hadamardlifetime{(1865--1963)}
\newcommand\haehnle         {{\namefont H\ae hnle}}
\newcommand\haehnlename     {{\namefont Reiner \haehnle}}
\newcommand\haerdername     {Theo H\ae r\-der}
\newcommand\hahn            {{\namefont Hahn}}
\newcommand\hahnname        {{\namefont\ottonoconflict\ \hahn}}
\newcommand\hahnlifetime    {(1879--1968)}
\newcommand\hailperin       {{\namefont Hailperin}}
\newcommand\hailperinname   {{\namefont Theodore \hailperin}}
\newcommand\hallett         {{\namefont Hallett}}
\newcommand\hallettname     {{\namefont\michaelwithouttrema\ \hallett}}
\newcommand\hallmann        {{\namefont Hall\-mann}}
\newcommand\hallmannname    {{\namefont\andreas\ \hallmann}}
\newcommand\hamilton        {{\namefont Hamilton}}
\newcommand\hamiltonname    {{\namefont Geoff \hamilton}}
\newcommand\hamoen          {Hamoen}
\newcommand\hamoenname      {Erik \hamoen}
\newcommand\hanus           {Hanu\es}
\newcommand\hanusname       {\michaelwithouttrema\ \hanus}
\newcommand\harmelen        {{\namefont Harmelen}}
\newcommand\harmelenname    {{\namefont\frank\ van \harmelen}}
\newcommand\hartogs         {{\namefont Hartogs}}
\newcommand\hartogsname     {{\namefont\friedrich\ \hartogs}}
\newcommand\hartogslifetime {(1874--1943)}
\newcommand\hartogswellorderingtheorem{\hartogs' Ordinal Theorem}
\newcommand\hasenjaegerindex{\index{Hasenjaeger, Gisbert}}
\newcommand\hasenjaeger     {{\namefont Hasenjaeger}}
\newcommand\hasenjaegername {\hasenjaegerindex{\namefont Gisbert \hasenjaeger}}
\newcommand\hasse           {{\namefont Hasse}}
\newcommand\hassename       {{\namefont\helmut\ \hasse}}
\newcommand\hasselifetime   {(1898--1979)}
\newcommand\haubrich        {{\namefont Haubrich}}
\newcommand\haubrichname    {{\namefont Ralf \haubrich}}
\newcommand\hauff           {{\namefont Hauff}}
\newcommand\hauffname       {{\namefont\wilhelm\ \hauff}}
\newcommand\haufflifetime   {(1802--1827)}
\newcommand\heath           {{\namefont Heath}}
\newcommand\heathname       {{\namefont \thomas\ L. \heath}}
\newcommand\heathlifetime   {(1861--1940)}
\newcommand\hecke           {{\namefont Hecke}}
\newcommand\heering         {Heering}
\newcommand\heeringname     {\jan\ \heering}
\newcommand\heidegger       {\mbox{\namefont Heidegger}}
\newcommand\heideggername   {{\namefont\martin\ \heidegger}}
\newcommand\heijenoortindex {\index{Heijenoort!Jean van}}
\newcommand\heijenoort      {{\namefont Heijen\-oort}}
\newcommand\vanheijenoort   {{\namefont van Heijen\-oort}}
\newcommand\heijenoortname  {\heijenoortindex{\namefont\jean\ %L. M. 
                             \vanheijenoort}}
\newcommand\heijenoortdeathyear{1986}
\newcommand\heijenoortlifetime{(1912--\heijenoortdeathyear)}
\newcommand\heijenoortonherbrandunpublishedtitle
{On the relation between the Falsifiability Tree Method and the 
\herbrand\ Method in Quantification Theory}
\newcommand\heisenberg      {{\namefont Heisen\-berg}}
\newcommand\heisenbergname  {{\namefont\werner\ \heisenberg}}
\newcommand\heisenberglifetime{(1901--1976)}
\newcommand\helmholtzindex  {\index{Helmholtz, Hermann von}}
\newcommand\helmholtz       {{\namefont Helm\-holtz}}
\newcommand\helmholtzname   {\helmholtzindex{\namefont \hermann\ von \helmholtz}}
\newcommand\helmholtzlifetime{(1821--1894)}
\newcommand\herbrandindex   {\index{Herbrand!Jacques}}
\newcommand\herbrand        {\mbox{\namefont Herbrand}}
\newcommand\herbrandname    {\herbrandindex{\namefont \jacques\ \herbrand}}
\newcommand\herbranddeathyear{1931}
\newcommand\herbrandlifetime{(1908--\herbranddeathyear)}
\newcommand\herbrandbirthday{\Feb\,12, 1908}
\newcommand\herbranddeathday{\Jul\,27, \herbranddeathyear}
\newcommand\herbrandPhDtitle
{Recherche\es\ sur la th\'eorie de la d\'e\-mon\-stra\-tion}
\newcommand\herbrandPhDdefensedate{\Jun\,11, 1930}
\newcommand\herbrandPhDapprovedforpublicationdate{\Jun\,20, 1929}
\newcommand\herbrandPhDdating{\Apr\,14, 1929}
\newcommand\herbrandtogoedeldate{\Apr\,7, 1931}
\newcommand\herbrandsfundamentaltheorem{\herbrand'\es\ \fundamentaltheorem}
\newcommand\fundamentaltheorem{Fundamental Theorem}
\newcommand\herbrandribet   {\herbrand--\ribet}
\newcommand\hermes          {{\namefont Herme\es}}
\newcommand\hermesname      {{\namefont\hans\ \hermes}}
\newcommand\hertz           {{\namefont Hertz}}
\newcommand\hertzeinsname   {{\namefont\heinrich\ \hertz}}
\newcommand\hertzzweiname   {{\namefont\gustav  \ \hertz}}
\newcommand\hertzdreiindex  {\index{Hertz!Paul}}
\newcommand\hertzdreiname   {\hertzdreiindex{\namefont\paul\ \hertz}}
\newcommand\hertzeinslifetime{(1857--1894)}
\newcommand\hertzzweilifetime{(1887--1975)}
\newcommand\hertzdreiphysicistlifetime {(1881--1940)}
\newcommand\hertzdreipoliticianlifetime{(1888--1961)}
\newcommand\heusinger       {Heusinger}
\newcommand\heusingername   {\klaus\ von \heusinger}
\newcommand\heytingindex    {\index{Heyting, Arend}}
\newcommand\heyting         {\mbox{\namefont Heyting}}
\newcommand\heytingname     {\heytingindex{\namefont Arend \heyting}}
\newcommand\heytinglifetime {(1898--1980)}
\newcommand\henkin          {{\namefont Henkin}}
\newcommand\henkinname      {{\namefont \leon\ \henkin}}
\newcommand\henkinlifetime  {(1921--2006)}
\newcommand\hessenberg      {{\namefont Hessenberg}}
\newcommand\hessenbergname  {{\namefont Gerhard \hessenberg}}
\newcommand\hessenberglifetime{(1847--1925)}
\newcommand\hilbertindex    {\index{Hilbert!David}}
\newcommand\hilbert         {\mbox{\namefont Hilbert}}
\newcommand\hilbertname     {\hilbertindex{\namefont \david\ \hilbert}}
\newcommand\hilbertlifetime {(1862--1943)}
\newcommand\hilbertsprogram {\hilbert'\es\ \programme}
\newcommand\hilbertsProgram {\hilbert'\es\ \Programme}
\newcommand\hilbertsepsilon {\hilbert'\es\ \nlbmath\varepsilon}
\newcommand\hilbertbernaysproject{{\namefont\hilbert\ \bernays\ Pro\-ject}}
\newcommand\hillenbrandindex{\index{Hillenbrand, Thomas}}
\newcommand\hillenbrand     {{\namefont Hillenbrand}}
\newcommand\hillenbrandname {\hillenbrandindex{\namefont\thomas\ \hillenbrand}}
\newcommand\hintermeier     {Hinter\-meier}
\newcommand\hintermeiername {\claus\ \hintermeier}
\newcommand\hintikka        {{\namefont Hintikka}}
\newcommand\hintikkaname    {{\namefont Jaakko \hintikka}}
%                           {K. Jaakko J. \hintikka}
\newcommand\hippasos        {{\namefont Hippasu\es}}
\newcommand\hippasosname    {{\namefont\hippasos\ of Metapontum}}
\newcommand\hippasoslifetime{(\ca\ 550\,\BC)}
\newcommand\hippasosgerman  {{\namefont Hippaso\es}}
\newcommand\hippasosnamegerman{{\namefont\hippasosgerman\ von Metapont}}
\newcommand\hoare           {Hoare}
\newcommand\hoarename       {C. A. R. \hoare}
\newcommand\hobbs           {Hobb\es}
\newcommand\hobbsname       {Jerry R. \hobbs}
\newcommand\hoeven          {Hoeven}
\newcommand\hoevenname      {Jori\es\ van der \hoeven}
\newcommand\hogger          {{\namefont Hogger}}
\newcommand\hoggername      {{\namefont Christopher \john\ \hogger}}
\newcommand\horacek         {{\namefont Horacek}}
\newcommand\horacekname     {{\namefont\helmut\ \horacek}}
\newcommand\howardname      {{\namefont\paul\ \howard}}
\newcommand\huebner         {H\ue bner}
\newcommand\huebnername     {Malte \huebner}
\newcommand\hudlak          {Hudlak}
\newcommand\hudlakname      {\paul\ \hudlak}
\newcommand\huet            {Huet}
\newcommand\huetname        {G\'erard \huet}
\newcommand\huff            {{\namefont Huff}}
\newcommand\huffname        {{\namefont\george\ \huff}}
\newcommand\hullot          {Hullot}
\newcommand\hullotname      {\jean-Marie \hullot}
\newcommand\humboldt        {{\namefont Hum\-boldt}}
\newcommand\humboldtname    {{\namefont Alexander von \humboldt}}
\newcommand\humboldtlifetime{(1769--1859)}
\newcommand\hume            {{\namefont Hume}}
\newcommand\humename        {{\namefont \david\ \hume}}
\newcommand\humelifetime    {(1711--1776)}
\newcommand\huntingtonindex {\index{Huntington, Edward V.}}
\newcommand\huntington      {{\namefont Huntington}}
\newcommand\huntingtonname  {\huntingtonindex{\namefont Edward V. \huntington}}
\newcommand\husserl         {{\namefont Husserl}}
\newcommand\husserlname     {{\namefont\edmund\ \husserl}}
\newcommand\husserllifetime {(1859--1938)}
\newcommand\hutter          {{\namefont Hutter}}
\newcommand\huttername      {{\namefont\dieter\ \hutter}}
\newcommand\huygens         {{\namefont Huygen\es}}
\newcommand\huygensname     {{\namefont Christiaan \huygens}}
\newcommand\huygenslifetime {(1629--1695)}
\newcommand\ireland         {{\namefont Ireland}}
\newcommand\irelandname     {{\namefont\andrew\ \ireland}}
\newcommand\jaskowskiindex  {\index{Jaskowski@Ja{\'s}kowski, \stanislaw}}
\newcommand\jaskowski       {\mbox{\namefont Ja{\'s}kowski}}
\newcommand\jaskowskiname   {\jaskowskiindex{\namefont \stanislaw\ \jaskowski}}
\newcommand\jaskowskilifetime{(1906--1965)}
\newcommand\jouannaud       {Jouannaud}
\newcommand\jouannaudname   {\jean-\pierre\ \jouannaud}
\newcommand\kahle           {{\namefont Kahle}}
\newcommand\kahlename       {{\namefont Rein\-hard \kahle}}
\newcommand\kalmarindex     {\index{Kalmar@Kalm\'ar, L\'aszl\'o}}
\newcommand\kalmar          {{\namefont Kalm\'ar}}
\newcommand\kalmarname      {\kalmarindex{\namefont L\'aszl\'o \kalmar}}
\newcommand\kalmarlifetime  {(1905--1976)}
\newcommand\kamp            {Kamp}
\newcommand\kampname        {\hans\ \kamp}
\newcommand\kanger          {Kan\-ger}
\newcommand\kangername      {Stig \kanger}
\newcommand\kant            {{\namefont Kant}}
\newcommand\kantname        {{\namefont\immanuelwithouttrema\ \kant}}
\newcommand\kantdeathyear   {1804}
\newcommand\kantlifetime    {(1724--\kantdeathyear)}
\newcommand\kaplan          {Kaplan}
\newcommand\kaplanname      {St\'ephane \kaplan}
\newcommand\kapur           {Kapur}
\newcommand\kapurname       {Deepak \kapur}
\newcommand\kaufmann        {{\namefont Kaufmann}}
\newcommand\kaufmannname    {{\namefont Matt \kaufmann}}
\newcommand\kelley          {{\namefont Kelley}}
\newcommand\kelleyname      {{\namefont \john\ L. \kelley}}
\newcommand\kelleylifetime  {(1916--1999)}
\newcommand\kepler          {{\namefont Kepler}}
\newcommand\keplername      {{\namefont Johanne\es\ \kepler}}
\newcommand\keplerlifetime  {(1571--1630)}
\newcommand\kerber          {Kerber}
\newcommand\kerbername      {\manfred\ \kerber}
\newcommand\kernighan       {Kernighan}
\newcommand\kernighanname   {Brian W. \kernighan}
\newcommand\kleeneindex     {\index{Kleene, Stephen C.}}
\newcommand\kleene          {{\namefont Kleene}}
\newcommand\kleenename      {\kleeneindex{\namefont Stephen C. \kleene}}
%                            {Stephen Cole \kleene}
\newcommand\klint           {Klint}
\newcommand\klintname       {\paul\ \klint}
\newcommand\klop            {Klop}
\newcommand\klopname        {\jan\ Willem \klop}
\newcommand\knuth           {Knuth}
\newcommand\knuthname       {\donald\ E. \knuth}
\newcommand\koenig          {K\oe nig}
\newcommand\koenigname      {\koenig}
\newcommand\koenigslemma    {\koenig's Lemma}
\newcommand\kohlhase        {{\namefont Kohl\-hase}}
\newcommand\kohlhasename    {{\namefont\michaelwithouttrema\ \kohlhase}}
\newcommand\koller          {Koller}
\newcommand\kollername      {\alexander\ \koller}
\newcommand\kolmogorov      {{\namefont Kolmogorov}}
\newcommand\kolmogorovname  {{\namefont Andrey \kolmogorov}}
\newcommand\kolmogorovlifetime{(1903--1987)}
\newcommand\kopernik        {Koper\-nik}% Das ist der einzige korrekte 
                                     % original polnische Name!
\newcommand\kopernikname    {Niko\-lau\es\ \kopernik}
\newcommand\koperniklifetime{(1473--1543)}
\newcommand\kopernikan      {\kopernik an}
\newcommand\kopernikanisch  {\kopernik a\-nisch}
\newcommand\kounalis        {Kounali\es}
\newcommand\kounalisname    {Emmanu\ewithtrema l \kounalis}
\newcommand\knaster         {{\namefont Knaster}}
\newcommand\knastername     {{\namefont Bronis\l aw \knaster}}
\newcommand\knasterlifetime {(1893--1990)}
\newcommand\knastertarski   {\knaster--\tarski}
\newcommand\kneser          {{\namefont Kneser}}
\newcommand\kneserzweiname  {{\namefont Hellmuth \kneser}}
\newcommand\kneserzweilifetime{(1898--1973)}
\newcommand\kreiselindex    {\index{Kreisel, Georg}}
\newcommand\kreisel         {{\namefont Kreisel}}
\newcommand\kreiselname     {\kreiselindex{\namefont\georg\ \kreisel}}
\newcommand\kreisellifetime {(born\,1923)}
\newcommand\kreowski        {{\namefont Kreow\-ski}}
\newcommand\kreowskiname    {{\namefont\hans-\joerg\ \kreowski}}
\newcommand\kroneckerindex  {\index{Kronecker, Leopold}}
\newcommand\kronecker       {\mbox{\namefont Kronecker}}
\newcommand\kroneckername   {\kroneckerindex{\namefont\leopold\ \kronecker}}
\newcommand\kroneckerlifetime{(1823--1891)}
\newcommand\kruskal         {Kruskal}
\newcommand\kruskalname     {\joseph\ B. \kruskal}
\newcommand\kuechlin        {K\ue ch\-lin}
\newcommand\kuechlinname    {\wolfgang\ \kuechlin}
\newcommand\kuehler         {{\namefont K\ue h\-ler}}
\newcommand\kuehlername     {{\namefont\ulrich\ \kuehler}}
\newcommand\kuhn            {{\namefont Kuhn}}
\newcommand\kuhnname        {{\namefont\thomas\ S. \kuhn}}
\newcommand\kuhnlifetime    {(1922--1996)}
\newcommand\kummer          {Kummer}
\newcommand\kummername      {\ernst\ Eduard \kummer}
\newcommand\kummerlifetime  {(1810--1893)}
\newcommand\kuratowski      {Kuratowski}
\newcommand\kuratowskiname  {Kazimierz \kuratowski}
\newcommand\kuratowskilifetime{(1896--1980)}
\newcommand\landau          {{\namefont\Landau}}
\newcommand\landauname      {{\namefont\edmund\ G. H. \landau}}
                           % G. H. = Georg Hermann
\newcommand\landaulifetime  {(1877--1938)}
\newcommand\lankford        {Lankford}
\newcommand\lankfordname    {Dalla\es\ S. \lankford}
\newcommand\laotse          {Lao\-zi}
\newcommand\laotsename      {\laotse}
\newcommand\taoteking       {Tao Te King}
\newcommand\lautman         {{\namefont Laut\-man}}
\newcommand\lautmanname     {{\namefont\albert\ \lautman}}
\newcommand\lautmanlifetime {(1908--1944)}
\newcommand\lavoisier       {La\-voi\-sier}
\newcommand\lavoisiername   {Antoine Laurent de \lavoisier}
\newcommand\lavoisierlifetime{(1743--1794)}
\newcommand\lee             {Lee}
\newcommand\leename         {\richard\ C.-T. \lee}
\newcommand\leeuwen         {Leeuwen}
\newcommand\leeuwenname     {\jan\ van \leeuwen}
\newcommand\lehmann         {{\namefont Lehmann}}
\newcommand\lehmannname     {{\namefont Daniel \lehmann}}
\newcommand\leibniz         {{\namefont Leibniz}}
\newcommand\leibnizname     {{\namefont Gottfried \wilhelm\ \leibniz}}
\newcommand\leibnizlifetime {(1646--1716)}
\newcommand\leisenring      {{\namefont Leisen\-ring}}
\newcommand\leisenringname  {{\namefont\leisenringfirstname\ \leisenring}}
\newcommand\leisenringfirstname
                            {\albert\ C.}
                            %{Al C.}
                            %{A. C.}
                            %{Al(bert) C.}
\newcommand\leisenringlifetime{(born\,1941?)}
\newcommand\leibowitz       {Leibowitz}
\newcommand\leibowitzname   {\rene\ \leibowitz}
\newcommand\leibowitzlifetime{(1913--1972)}
\newcommand\leitsch         {{\namefont Leitsch}}
\newcommand\leitschname     {{\namefont\alexander\ \leitsch}}
\newcommand\lenart          {{\namefont Lenart}}
\newcommand\lenartname      {{\namefont Mihaly \lenart}}
\newcommand\lesniewski      {{\namefont Le\'sniewski}}
\newcommand\lesniewskiname  {{\namefont\stanislaw\ \lesniewski}}
\newcommand\lesniewskilifetime{(1886--1939)}
\newcommand\letz            {{\namefont Letz}}
\newcommand\letzname        {{\namefont Rein\-hold \letz}}
\newcommand\levyname        {\jean-\jacques\ L\'evy}
\newcommand\lewi            {{\namefont Lewi}}
\newcommand\lewiname        {{\namefont\johan\ \lewi}}
\newcommand\lewis           {{\namefont Lewis}}
\newcommand\lewisname       {{\namefont Clarence \irving\ \lewis}}
\newcommand\lewislifetime   {(1883--1964)}
\newcommand\lewy            {{\namefont Lewy}}
\newcommand\lewyname        {{\namefont\hans\ \lewy}}
\newcommand\lewylifetime    {(1904--1980)}
\newcommand\lifschitz       {{\namefont Lifschitz}}
\newcommand\lifschitzname   {{\namefont\vladimir\ A. \lifschitz}}
\newcommand\lipschitz       {{\namefont Lipschitz}}
\newcommand\lipschitzname   {{\namefont\rudolf\ \lipschitz}}
\newcommand\lipschitzlifetime{1832--1903}
\newcommand\lindner         {{\namefont Lindner}}
\newcommand\lindnername     {{\namefont\wolfgang\ \lindner}}
\newcommand\linne           {{\namefont Linn\'e}}
\newcommand\linnename       {{\namefont\carl\ von \linne}}
\newcommand\linnelifetime   {(1707--1778)}
\newcommand\loechner        {{\namefont L\oe chner}}
\newcommand\loechnername    {{\namefont\bernd\ \loechner}}
\newcommand\loewenheimindex {\index{Loewenheim@L\oe wenheim!Leopold}}
\newcommand\loewenheimindexstart{\index{Loewenheim@L\oe wenheim!Leopold|(}}
\newcommand\loewenheimindexend{\index{Loewenheim@L\oe wenheim!Leopold|)}}
\newcommand\loewenheim      {{\namefont L\oe wen\-heim}}
\newcommand\loewenheimname  {\loewenheimindex{\namefont\leopold\ \loewenheim}}
\newcommand\loewenheimlifetime{(1878--1957)}
\newcommand\loewenheimskolem{\loewenheim--\skolem}
\newcommand\loewenheimskolemtheorem{\index
            {Loewenheim@L\oe wenheim!-Skolem Theorem}\loewenheimskolem\ Theorem}
\newcommand\loewenheimskolemtheoremindexstart{\index
                                    {Loewenheim@L\oe wenheim!-Skolem Theorem|(}}
\newcommand\loewenheimskolemtheoremindexend{\index
                                    {Loewenheim@L\oe wenheim!-Skolem Theorem|)}}
\newcommand\upwardloewenheimskolemtarskitheorem{\index
{Loewenheim@L\oe wenheim!-Skolem-Tarksi Theorem!Uward}%
                                     Upward \loewenheimskolem--\tarski\ Theorem}
\newcommand\loef            {{\namefont\martin-L\oe f}}
\newcommand\loefname        {{\namefont Per \loef}}
\newcommand\loria           {Lor\'\i a-S\'aenz}
\newcommand\lorianame       {\carlos\ A. \loria}
\newcommand\liouville       {Liouville}
\newcommand\liouvillename   {\joseph\ \liouville}
\newcommand\liouvillelifetime{(1809--1882)}
\newcommand\lukasiewiczindex{\index{Lukasiewicz@\L uka\-sie\-wicz, Jan}}
\newcommand\lukasiewicz     {{\namefont \L uka\-sie\-wicz}}
\newcommand\lukasiewiczname {\lukasiewiczindex{\namefont\jan\ \lukasiewicz}}
\newcommand\lukasiewiczlifetime{(1878--1956)}
\newcommand\titlelukasiewicztarski 
          {Unter\-suchungen \ue ber den Au\esi sagen\-kalk\ue l}
\newcommand\lunde           {Lunde}
\newcommand\lundename       {\ruediger\ \lunde}
\newcommand\luther          {{\namefont Luther}}
\newcommand\luthername      {{\namefont\martin\ \luther}}
\newcommand\lutherlifetime  {(1483--1546)}
\newcommand\maclane         {{\namefont MacLane}}
\newcommand\maclanename     {{\namefont Saunders \maclane}}
\newcommand\maclanelifetime {(1909--2005)}
\newcommand\macqueen        {MacQueen}
\newcommand\macqueenname    {\david\ B. \macqueen}
\newcommand\madlener        {Mad\-lener}
\newcommand\madlenername    {\klaus\ \madlener}
\newcommand\mahr            {{\namefont Mahr}}
\newcommand\mahrname        {{\namefont\bernd\ \mahr}}
\newcommand\majer           {{\namefont Majer}}
\newcommand\majername       {{\namefont\ulrich\ \majer}}
\newcommand\makinson        {{\namefont Makinson}}
\newcommand\makinsonname    {{\namefont\david\ \makinson}}
\newcommand\mancosu         {{\namefont Mancosu}}
\newcommand\mancosuname     {{\namefont\paolo\ \mancosu}}
\newcommand\mann            {{\namefont Mann}}
\newcommand\mannname        {{\namefont\thomas\ \mann}}
\newcommand\mannlifetime    {(1875--1955)}
\newcommand\manna           {Manna}
\newcommand\mannaname       {Zohar \manna}
\newcommand\manolios        {{\namefont Manolio\es}}
\newcommand\manoliosname    {{\namefont Panagioti\es\ ``Pete'' \manolios}}
\newcommand\marx            {{\namefont Marx}}
\newcommand\marxname        {{\namefont\karl\ \marx}}
\newcommand\maslov          {{\namefont Maslov}}
\newcommand\maslovname      {{\namefont\sergey\ Yu.\ \maslov}}
\newcommand\mattick         {Mattick}
\newcommand\mattickname     {\volker\ \mattick}
\newcommand\maurolycus      {{\namefont Maurolico}}
\newcommand\maurolycuslatin {{\namefont Maurolycu\es}}
\newcommand\maurolycusname  {{\namefont Francisco \maurolycus}}
\newcommand\maurolycuslifeplace{Messina}
\newcommand\maurolycuslifetime{(1494--1575)}
\newcommand\mccarthy        {{\namefont McCarthy}}
\newcommand\mccarthyname    {{\namefont John \mccarthy}}
\newcommand\mccarthylifetime{(1927--2011)}
\newcommand\meier           {{\namefont Meier}}
\newcommand\meiername       {{\namefont\andreas\ \meier}}
\newcommand\meinong         {{\namefont Meinong}}
\newcommand\meinongname     {{\namefont Alexiu\es\ \meinong}}
\newcommand\meinonglifetime {(1853--1920)}
\newcommand\Gegenstand      {Gegen\-stand}
\newcommand\Gegenstandstheorie{\Gegenstand\esi theo\-rie}
\newcommand\melisindex      {\index{Melis, Erica}}
\newcommand\melis           {{\namefont Meli\es}}
\newcommand\melisname       {\melisindex{\namefont Erica \melis}}
\newcommand\mendelssohn     {{\namefont Mendel\esi sohn}}
\newcommand\mendelssohnname {{\namefont Moses \mendelssohn}}
\newcommand\mendelssohnlifetime{(1729--1786)}
\newcommand\meseguer        {Meseguer}
\newcommand\meseguername    {\jose\ \meseguer}
\newcommand\meyerviol       {Meyer-Viol}
\newcommand\meyerviolname   {\wilfried\ P. M. \meyerviol}
\newcommand\middeldorp      {Middel\-dorp}
\newcommand\middeldorpname  {Aart \middeldorp}
\newcommand\miller          {{\namefont Mil\-ler}}
\newcommand\millername      {{\namefont Dale A. \miller}} 
% {Dale \miller} As his supervisor Peter Andrews
% cites him with middle initial, we had better do so, too
\newcommand\mints           {Mint\es}
\newcommand\mintsname       
{{\namefont Grigori    \mints}}
%{{\namefont Grigori E. \mints}}
\newcommand\mitchell        {Mitchell}
\newcommand\mitchellname    {Oscar \howard\ \mitchell} 
\newcommand\mitchelllifetime{(1851--1889)}
\newcommand\mitchelldeathdate{\Mar\,29, 1889}
\newcommand\mitchelldeathcourse{pneumonia}
% Lungenentzuendung, Quelle: Peirce, Chronological Edition, Vol. 6, p.lvi
\newcommand\montanari       {{\namefont Montanari}}
\newcommand\montanariname   {{\namefont Ugo \montanari}}
\newcommand\moore           {{\namefont Moore}}
\newcommand\moorename       {{\namefont J S.       \moore}}
%                           {{\namefont J Strother \moore}}
\newcommand\morse           {{\namefont Morse}}
\newcommand\morsename       {{\namefont Anthony P.    \morse}}
%                           {{\namefont Anthony Percy \morse}}
\newcommand\morselifetime   {(1911--1984)}
\newcommand\MKlong          {\morse--\kelley}
\newcommand\MKshort         {{\sc MK}}
\newcommand\moschnerindex   {\index{Moschner, Markus}}
\newcommand\moschner        {{\namefont Moschner}}
\newcommand\moschnername    {\moschnerindex{\namefont\markus\ \moschner}}
\newcommand\moser           {{\namefont Moser}}
\newcommand\mosername       {{\namefont\georg\ Ch.\ \moser}}
\newcommand\moss            {{\namefont Mo\ses}}
\newcommand\mossname        {{\namefont\lawrence\ \moss}}
\newcommand\mostowski       {{\namefont Mostowski}}
\newcommand\mostowskiname   {{\namefont Andrzej \mostowski}}
\newcommand\mostowskilifetime{(1913--1975)}
\newcommand\mozart          {\mbox{\namefont Mozart}}
\newcommand\mozartname      {{\namefont\wolfgang\ Amadeus \mozart}}
\newcommand\mozartlifetime  {(1756--1791)}
\newcommand\mueller         {{\namefont M\ue ller}}
\newcommand\muellername     {{\namefont Gert H. \mueller}}
\newcommand\musser          {{\namefont Musser}}
\newcommand\mussername      {{\namefont\david\ R. \musser}}
\newcommand\narendran       {Narendran}
\newcommand\narendranname   {Paliath \narendran}
\newcommand\nebel           {Nebel}
\newcommand\nebelname       {\bernhard\ \nebel}
\newcommand\nicolosi        {{\namefont Nicolosi-Asmundo}}
\newcommand\nicolosiname    {{\namefont Marianna \nicolosi}}
\newcommand\neumannindex    {\index{Neumann, John von}}
\newcommand\neumann         {{\namefont Neumann}}
\newcommand\neumannname     {\neumannindex{\namefont\john\ von \neumann}}
%                           {{\namefont\john\ L. von \neumann}}
\newcommand\neumannlifetime {(1903--1957)}
\newcommand\NBGlong         {\neumann--\bernays--\goedel}
\newcommand\NBGshort        {{\sc NBG}}
\newcommand\nelson          {{\namefont Nelson}}
\newcommand\nelsoneinsname  {{\namefont Leonard \nelson}}
\newcommand\nelsoneinslifetime{(1921--2006)}
\newcommand\newman          {Newman}
\newcommand\newmanname      {M. H. A. \newman}
\newcommand\newmanlemma     {\newman\ Lemma}
\newcommand\newton          {{\namefont Newton}}
\newcommand\newtonname      {{\namefont Isaac \newton}}
\newcommand\newtonlifetime  {(1643--1727)}
\newcommand\nieuwenhuis     {Nieuwenhui\es}
\newcommand\nieuwenhuisname {\robert\ \nieuwenhuis}
\newcommand\nipkow          {{\namefont Nipkow}}
\newcommand\nipkowname      {{\namefont\tobias\ \nipkow}}
\newcommand\nicod           {{\namefont Nicod}}
\newcommand\nicodname       {{\namefont\jean\ \nicod}}
\newcommand\nicodlifetime   {(1893--1924)}
\newcommand\nicolauscusanus {\nicolaus}
\newcommand\nicolauscusanusname{\nicolauscusanus\ of Cu\ewithtrema\es}
\newcommand\nicolauscusanuslifetime{(1401--1464)}
\newcommand\noether         {{\namefont Noether}}
%                           {{\namefont N\oe ther}}
% Though ``N\oe ther'' is also definitely correct as a ligature and is also
% the version of the birth certificate of Emmy,
% in the old age Max and in her adult age Emmy never used the 
% umlaut
\newcommand\noethername     {{\namefont Emmy \noether}}
%                           {{\namefont A. Emmy \noether}}
\newcommand\noetherfathername{\maxchristianname\ \noether}
\newcommand\noetherbirthyear{1882}
\newcommand\noetherdeathyear{1935}
\newcommand\noetherlifetime {(\noetherbirthyear--\noetherdeathyear)}
\newcommand\noetherfatherlifetime {(1844--1921)}
\newcommand\noetherian      {\noether ian}
\newcommand\theoremofnoetherianinduction{Theorem of\/ \noetherian\ Induction}
\newcommand\axiomofstructuralinductionfirsthalf{Axiom}
\newcommand\axiomofstructuralinductionsecondhalf{of Structural Induction}
\newcommand\axiomofstructuralinduction{\axiomofstructuralinductionfirsthalf\ 
\axiomofstructuralinductionsecondhalf}
\newcommand\axiomofchoice   {Axiom of Choice}
\newcommand\axiomofcollection{Axiom of Collection}
\newcommand\nonnengart      {{\namefont Nonnengart}}
\newcommand\nonnengartname  {{\namefont\andreas\ \nonnengart}}
\newcommand\nourani         {Nourani}
\newcommand\nouraniname     {Cyru\es\ F. \nourani}
\newcommand\okadaname       {Mitsuhiro Okada} 
\newcommand\ockham          {{\namefont Ockham}}
\newcommand\ockhamname      {{\namefont \william\ of \ockham}}
\newcommand\ockhamlifetime  {(1285--1347)}
\newcommand\oostrom         {{\namefont Oostrom}}
\newcommand\oostromname     {{\namefont Vincent van \oostrom}}
\newcommand\orevkov         {Orevkov}
\newcommand\orevkovname     {\vladimir\ P. \orevkov}
\newcommand\ottoname        {\friedrich\ \ottonoconflict}
\newcommand\padawitz        {{\namefont Pada\-witz}}
\newcommand\padawitzname    {{\namefont\peter\ \padawitz}}
\newcommand\paley           {{\namefont Paley}}
\newcommand\paleyname       {{\namefont\raymond\ \paley}}
\newcommand\paleylifetime   {(1907--1933)}
\newcommand\pandora         {Pandora}
\newcommand\parsonsindex    {\index{Parsons, Charles}}
\newcommand\parsons         {{\namefont Parsons}}
\newcommand\parsonsname     {\parsonsindex{\namefont\charles\ \parsons}}
\newcommand\pascal          {{\namefont Pascal}}
\newcommand\pascalname      {{\namefont Blaise \pascal}}
\newcommand\pascalbirthyear {1623}
\newcommand\pascaldeathyear {1662}
\newcommand\pascallifetime  {(\pascalbirthyear--\pascaldeathyear)}
\newcommand\pasztor         {Pasztor}
\newcommand\pasztorname     {Ana \pasztor}
\newcommand\paterson        {Paterson}
\newcommand\patersonname    {\michaelwithouttrema\ S. \paterson}
\newcommand\paulson         {{\namefont Paulson}}
\newcommand\paulsonname     {{\namefont\lawrence\ C. \paulson}}
%                           {Larry C. \paulson}
% Larry will das so!
\newcommand\peanoindex      {\index{Peano!Guiseppe}}
\newcommand\peano           {{\namefont Peano}}
\newcommand\peanoname       {\peanoindex{\namefont Guiseppe \peano}}
\newcommand\peanolifetime   {(1858--1932)}
\newcommand\peanoaxiom      {\dedekind--\peano\ axiom}
\newcommand\peckhausindex   {\index{Peckhaus, Volker}}
\newcommand\peckhaus        {{\namefont Peck\-haus}}
\newcommand\peckhausname    {\peckhausindex{\namefont \volker\ \peckhaus}}
\newcommand\peirceindex     {\index{Peirce!Charles S.}}
\newcommand\protectedpeirceindex{\protect\index{Peirce!Charles S.}}
\newcommand\peirce          {{\namefont Peirce}}
\newcommand\peircename      {\peirceindex{\namefont \charles\ S. \peirce}}
                           %{\charles\ Sanders \peirce}
\newcommand\peircelifetime  {(1839--1914)}
\newcommand\peircefathername{\benjamin\ \peirce}
\newcommand\peircefatherlifetime{(1809--1880)}
\newcommand\peters          {Peter\es}
\newcommand\petersname      {\stanley\ \peters}
\newcommand\bachpeterssentence{\bach--\peters\ sentence}
\newcommand\bachpetersSentence{\bach--\peters\ Sentence}
\newcommand\peterson        {Peterson}
\newcommand\petersonname    {\john\ \peterson}
\newcommand\pieri           {{\namefont Pieri}}
\newcommand\pieriname       {{\namefont Mario \pieri}}
\newcommand\pierilifetime   {(1860--1913)}
\newcommand\pinkal          {Pinkal}
\newcommand\pinkalname      {\manfred\ \pinkal}
\newcommand\plaisted        {Plaisted}
\newcommand\plaistedname    {\david\ A. \plaisted}
\newcommand\plancknonamefont{Planck}
\newcommand\planck          {{\namefont\plancknonamefont}}
\newcommand\plancknamenonamefont{\maxchristiannamenonamefont\ \plancknonamefont}
\newcommand\planckname      {{\namefont\plancknamenonamefont}}
\newcommand\plancklifetime  {(1858--1947)}
\newcommand\plato           {{\namefont Plato}}
\newcommand\platoname       {\plato} % Plato is a nickname ``the broad''.
\newcommand\platolifetime   {(427--347\,\BC)}
\newcommand\poincare        {{\namefont Poincar\'e}}
\newcommand\poincarename    {{\namefont Henri \poincare}}
\newcommand\poincarelifetime{(1854--1912)}
\newcommand\popper          {{\namefont\mbox{Popper}}}
\newcommand\poppername      {{\namefont\karl\ \popper}}
                           %{\karl\ R. \popper} 
\newcommand\popperlifetime  {(1902--1994)}
\newcommand\post            {{\namefont Post}}
\newcommand\postname        {{\namefont\emil\ \leon\ \post}}
\newcommand\postlifetime    {(1987--1954)}
\newcommand\pollet          {{\namefont Pollet}}
\newcommand\polletname      {{\namefont\martin\ \pollet}}
\newcommand\prause          {Prause}
\newcommand\prausename      {\gerhard\ \prause}
\newcommand\prawitz         {{\namefont Pra\-witz}}
\newcommand\prawitzname     {{\namefont Dag \prawitz}}
\newcommand\presburger      {{\namefont Pre\esi burger}} %actually: Prezburger
\newcommand\presburgername  {{\namefont\mbox{Moj\zwithdot es{}z} \presburger}}
\newcommand\presburgerlifetime{(1904--1943?)}
\newcommand\presburgerarithmetic{\presburger\ Arithmetic}
\newcommand\presburgertruename{Prez\-burger}
\newcommand\priestley       {Priestley}
\newcommand\priestleyname   {\joseph\ \priestley}
\newcommand\priestleylifetime{(1733--1804)}
\newcommand\prote           {Prote}
\newcommand\protename       {\horst\ \prote}
\newcommand\protzen         {{\namefont Protzen}}
\newcommand\protzenname     {{\namefont\martin\ \protzen}}
\newcommand\ptolemaios      {Ptole\-maio\es}
\newcommand\ptolemaiosname  {Klaudio\es\ \ptolemaios}
\newcommand\ptolemaioslifetime{(\ca\,100--\ca\,160)}
\newcommand\putnam          {{\namefont Putnam}}
\newcommand\putnamname      {{\namefont Hilary \putnam}}
\newcommand\putnamlifetime  {(born\,1926)}
\newcommand\pythagoras      {Pythagora\es}
\newcommand\pythagorasname  {\pythagoras}
%                           {\pythagoras\ of Samo\es}
% As the only other Pythagoras is also from Samos, what does ``of Samos'' help?
\newcommand\pythagoraslifetime{(\ca\,570--\ca\,500\BC)}
\newcommand\pythagorean     {{\namefont Pytha\-gorean}}
\newcommand\pythagoreans    {{\namefont\pythagorean s}}
\newcommand\quineindex      {\index{Quine, Willard Van O.}}
\newcommand\quine           {{\namefont Quine}}
\newcommand\quinename       {\quineindex{\namefont Willard Van O. \quine}}
%                           {{\namefont Willard Van %Orman \quine}}
\newcommand\quinelifetime   {(1908--2000)}
\newcommand\raamsdonk       {Raams\-donk}
\newcommand\raamsdonkname   {Femke van \raamsdonk}
\newcommand\readiname       {Rodrigo Readi-Nasser}
\newcommand\reddy           {Reddy}
\newcommand\reddyname       {Uday S. \reddy}
\newcommand\reichel         {Rei\-chel}
\newcommand\reichelname     {\horst\ \reichel}
\newcommand\reyle           {Reyle}
\newcommand\reylename       {\uwe\ \reyle}
\newcommand\rezaeiindex     {\index{Rezaei, Marianeh}}
\newcommand\rezaei          {{\namefont Rezaei}}
\newcommand\rezaeiname      {\rezaeiindex{\namefont Marianeh \rezaei}} 
\newcommand\ribet           {{\namefont Ribet}}
\newcommand\ribetname       {{\namefont Ken \ribet}} 
                           %{Kenneth A. \ribet}
\newcommand\riemann         {{\namefont Rie\-mann}}
\newcommand\riemannname     {{\namefont\bernhard\ \riemann}}
\newcommand\riemannlifetime {(1926--1966)}
\newcommand\ritchie         {Ritchie}
\newcommand\ritchiename     {Denni\es\ M. \ritchie}
\newcommand\robbins         {{\namefont Robbin\es}}
\newcommand\robbinsname     {{\namefont\herbert\ E. \robbins}}
\newcommand\robbinslifetime {(1922--2001)}
\newcommand\robbinsproblem  {\robbins\ Algebra problem}
\newcommand\robinson        {{\namefont Robinson}}
\newcommand\robinsonname    {{\namefont J. \alan\ \robinson}}
\newcommand\robinsonlifetime{(born\,1930)}
\newcommand\robinsontwoname {\peter\ J. \robinson}
\newcommand\roch            {{\namefont Roch}}
\newcommand\rochname        {{\namefont\gustav\ \roch}}
\newcommand\rochlifetime    {(1839--1866)}
\newcommand\roedding        {{\namefont R\oe dding}}
\newcommand\roeddingname    {{\namefont\dieter\ \roedding}}
\newcommand\rosu            {Ro\c su}
\newcommand\rosuname        {Grigore \rosu}
\newcommand\reinert         {Reinert}
\newcommand\reinertname     {Birgit \reinert}
\newcommand\roentgen        {R\oe ntgen}
\newcommand\roentgenname    {\wilhelm \ \roentgen}
\newcommand\roquette        {{\namefont Roquette}}
\newcommand\roquettename    {{\namefont\peter\ \roquette}}
\newcommand\rosser          {{\namefont Rosser}}
\newcommand\rossername      {{\namefont    Barkley \rosser}}
                           %{{\namefont J. Barkley \rosser}}
\newcommand\rosserlifetime  {(1907-1989)}
\newcommand\rubin           {Rubin}
\newcommand\rubinhename     {Herman \rubin}
\newcommand\rubinshename    {\jean\ E. \rubin}
\newcommand\rusinowitch     {Rusino\-witch}
\newcommand\rusinowitchname {\michael\ \rusinowitch}
\newcommand\russellindex    {\index{Russell!Bertrand}}
\newcommand\russell         {{\namefont Russell}}
\newcommand\russellname     {\russellindex{\namefont Bertrand \russell}}
% {Bertrand A.\,W. \russell} % no space after A.
\newcommand\russelllifetime {(1872--1970)}
\newcommand\russellsparadox {\russell'\es\ Paradox}
\newcommand\sankappanavar   {Sankappanavar}
\newcommand\sankappanavarname{H. P. \sankappanavar}
\newcommand\sannella        {Sannella}
\newcommand\sannellaname    {\donald\ T. \sannella}
\newcommand\salzer          {{\namefont Salzer}}
\newcommand\salzername      {{\namefont Gernot \salzer}}
\newcommand\sartre          {{\namefont Sartre}}
\newcommand\sartrename      {{\namefont\jean\ \paul\ \sartre}}
\newcommand\sattler         {{\namefont Sattler-Klein}}
\newcommand\sattlername     {{\namefont Andrea \sattler}}
\newcommand\samoa           {{\namefont Schmidt-Sa\-moa}}
\newcommand\samoaname       {{\namefont\tobias\ \samoa}}
\newcommand\scanlon         {Scanlon}
\newcommand\scanlonname     {\thomas\ M. \scanlon\ \jr}
\newcommand\scanlonlifetime {(born\,1940)}
\newcommand\schaperindex    {\index{Schaper, Hans von}}
\newcommand\schaper         {{\namefont Schaper}}
\newcommand\schapername     {\schaperindex{\namefont\hans\ von \schaper}}
\newcommand\schiller        {{\namefont Schiller}}
\newcommand\schillername    {{\namefont\friedrich\ von \schiller}}
\newcommand\schillermarvinindex{\index{Schiller, Marvin}}
\newcommand\schillermarvinname{\schillermarvinindex{\namefont Marvin \schiller}}
\newcommand\schlick         {{\namefont Schlick}}
\newcommand\schlickname     {{\namefont Moritz \schlick}}
\newcommand\schlicklifetime {(1882--1936)}
\newcommand\schmidt         {{\namefont Schmidt}}
\newcommand\fkschmidtname   {{\namefont\friedrich\ \karl\ \schmidt}}
\newcommand\arnoldschmidtname{{\namefont H. Arnold \schmidt}}
\newcommand\schmitt         {{\namefont Schmitt}}
\newcommand\schmittname     {{\namefont\peter\ H. \schmitt}}
\newcommand\schoenfinkelindex{\index{Schoenfinkel@Sch\oe n\-finkel, Moses}}
\newcommand\schoenfinkel    {{\namefont Sch\oe n\-finkel}}
\newcommand\schoenfinkelname
                          {\schoenfinkelindex{\namefont Mose\es\ \schoenfinkel}}
\newcommand\schoenfinkellifetime{(1889--1942)}
\newcommand\scholz          {{\namefont Scholz}}
\newcommand\scholzname      {{\namefont\heinrich\ \scholz}}
\newcommand\scholzlifetime  {(1884--1956)}
\newcommand\schroederindex  {\index{Schroeder@Schr\"oder, Ernst}}
\newcommand\schroeder       {{\namefont Schr\oe der}}
\newcommand\schroedername   {\schroederindex{\namefont\ernst\ \schroeder}}
\newcommand\schroederlifetime{(1841--1902)}
\newcommand\schroedinger    {Schr\oe\-din\-ger}
\newcommand\schuermann      {{\namefont Sch\ue r\-mann}}
\newcommand\schuermannname  {{\namefont\carsten\ \schuermann}}
\newcommand\schuetteindex   {\index{Schuette@Sch\ue tte, Kurt}}
\newcommand\schuette        {{\namefont Sch\ue tte}}
\newcommand\schuettename    {\schuetteindex{\namefont\kurt\ \schuette}}
\newcommand\schuettelifetime{(1909--1998)}
\newcommand\schulz          {Schulz}
\newcommand\schulzname      {\stephan\ \schulz}
\newcommand\schwaller       {{\namefont Schwaller de Lubicz}}
\newcommand\schwallername   {{\namefont \rene\ A. \schwaller}}
\newcommand\schwallerlifetime{(1887--1961)}
\newcommand\schweitzer      {{\namefont Schweitzer}}
\newcommand\schweitzername  {{\namefont\albert\ \schweitzer}}
\newcommand\schweitzerlifetime{(1875--1965)}
\newcommand\schweizer       {{\namefont Schweizer}}
\newcommand\schweizername   {{\namefont\stephan\ \schweizer}}
\newcommand\schwichtenberg  {{\namefont Schwichten\-berg}}
\newcommand\schwichtenbergname{{\namefont\helmut\ \schwichtenberg}}
\newcommand\scott           {{\namefont Scott}}
\newcommand\scottname       {{\namefont Dana S. \scott}}
\newcommand\sengler         {{\namefont Sengler}}
\newcommand\senglername     {{\namefont\claus\ \sengler}}
\newcommand\shakespeare     {Shakespeare}
\newcommand\shakespearename {\william\ \shakespeare}
\newcommand\shan            {{\namefont Shan}}
\newcommand\shanname        {{\namefont Chung-chieh \shan}}
\newcommand\sheffer         {{\namefont Sheffer}}
\newcommand\shefferindex    {\index{Sheffer!Henry Maurice}}
\newcommand\shefferstrokeindex{\index{Sheffer!stroke}}
\newcommand\sheffername     {\shefferindex{\namefont\henry\ \maurice\ \sheffer}}
\newcommand\shefferstrokename{\shefferstrokeindex\sheffer\ stroke}
\newcommand\siefkes         {{\namefont Siefkes}}
\newcommand\siefkesname     {{\namefont\dirk\ \siefkes}}
\newcommand\siegindex       {\index{Sieg, Wilfried}}
\newcommand\sieg            {{\namefont Sieg}}
\newcommand\siegname        {\siegindex{\namefont\wilfried\ \sieg}}
\newcommand\siekmannindex   {\index{Siekmann, \joerg}}
\newcommand\siekmann        {{\namefont Siek\-mann}}
\newcommand\siekmannname    {\siekmannindex{\namefont \joerg\ \siekmann}}
% The true name is actually \hans-\joerg\ \siekmann.
% Thus, the often found \joerg\ H. \siekmann\ is rubbish.
\newcommand\simpson         {{\namefont Simpson}}
\newcommand\simpsonname     {{\namefont Alex \simpson}}
\newcommand\sivakumarname   {G. Sivakumar}
\newcommand\skolemindex     {\index{Skolem!Thoralf}}
\newcommand\skolem          {{\namefont Skolem}}
\newcommand\skolemname      {\skolemindex\thoralf\ % A.
                             \skolem}
\newcommand\skolemlifetime  {(1887--1963)}
\newcommand\skolemizing     {\skolem\-izing}
\newcommand\skolemization   {\skolem\-ization}
\newcommand\skolemizedform  {\skolem\-ized form}   
\newcommand\skolemizedForm  {\skolem\-ized Form}   
% for validity, this is
% to denote the form that results by getting all general (universal) 
% quantifiers to the top on the price of incrementing their order,
% as used in Loewenheim (1915) and Skolem (1928).
\newcommand\skolemnormalform
{\index{Skolem!normal form}\skolem\ normal form}% for validity, this is 
% to denote the form that results by getting all restricted (existential)
% quantifiers to the top on the price of adding new relation symbols for the
% subformulas starting with general quantification
\newcommand\skolemsparadox  {\skolem's Paradox}
\newcommand\slind           {{\namefont Slind}}
\newcommand\slindname       {{\namefont\konrad\ \slind}}
\newcommand\smaill          {{\namefont Smaill}}
\newcommand\smaillname      {{\namefont\alan\ \smaill}}
\newcommand\smith           {{\namefont Smith}}
\newcommand\smithname       {{\namefont\james\ T. \smith}}
\newcommand\smolka          {{\namefont Smolka}}
\newcommand\smolkaname      {{\namefont Gert \smolka}}
\newcommand\smullyan        {{\namefont Smullyan}}
\newcommand\smullyanname    {{\namefont\raymond\ M. \smullyan}}
\newcommand\smullyanlifetime{(*1919)}
\newcommand\snyder          {Snyder}
\newcommand\snydername      {Wayne \snyder}
\newcommand\sobocinskiindex {\index{Sobociinski@Soboci\'nski, Boles\l aw}}
\newcommand\sobocinski      {{\namefont Soboci\'nski}}
\newcommand\sobocinskiname  {\sobocinskiindex{\namefont Boles\l aw \sobocinski}}
\newcommand\sobocinskilifetime{(1906--1990)}
\newcommand\sokrates        {{\namefont Sokrates}}
\newcommand\sokratesname    {{\namefont \sokrates\ the Older}}
\newcommand\sokrateslifetime{(469--399\BC)}
\newcommand\solon           {{\namefont Solon}}
\newcommand\solonname       {{\namefont \solon}}
\newcommand\solonlifetime   {(638?--after\,561\BC)}
\newcommand\sprenger        {Spren\-ger}
\newcommand\sprengername    {Christof \sprenger}
\newcommand\spurr           {{\namefont Spurr}}
\newcommand\spurrname       {{\namefont Jane \spurr}}
\newcommand\stanisfer       {{\namefont Stanisfer}}
\newcommand\stanisfername   {{\namefont Ryan \stanisfer}}
\newcommand\staples         {Staple\es}
\newcommand\staplesname     {\john\ \staples}
\newcommand\steele          {Steele}
\newcommand\steelename      {Guy L. \steele\ \jr}
\newcommand\steffenname     {\bernhard\ Steffen}
\newcommand\steinbach       {{\namefont Steinbach}}
\newcommand\steinbachname   {{\namefont\joachim\ \steinbach}}
\newcommand\stephansecondname{{\namefont Stephan}}
\newcommand\stephansecondnamename{{\namefont\werner\ \stephansecondname}}
\newcommand\stevens         {{\namefont Steven\es}}
\newcommand\stevensname     {{\namefont\andrew\ \stevens}}
\newcommand\stickel         {Stickel}
\newcommand\stickelname     {Mark E. \stickel}
\newcommand\stolzenburg     {Stol\-zen\-burg}
\newcommand\stolzenburgname {Frie\-der \stolzenburg}
\newcommand\stratulat       {Stratulat}
\newcommand\stratulatname   {Sorin \stratulat}
\newcommand\stuber          {Stu\-ber}
\newcommand\stubername      {\juergen\ \stuber}
\newcommand\sutcliffe       {Sutcliffe}
\newcommand\sutcliffename   {Geoff \sutcliffe}
\newcommand\suzuki          {Suzuki}
\newcommand\suzukiname      {Taro \suzuki}
\newcommand\szabo           {{\namefont Szabo}}
\newcommand\szaboname       {{\namefont \manfred\ E. \szabo}}
\newcommand\taitindex       {\index{Tait, William W.}}
\newcommand\tait            {{\namefont Tait}}
\newcommand\taitname        {\taitindex{\namefont William W. \tait}}
\newcommand\takagi          {{\namefont Takagi}}
\newcommand\takaginame      {{\namefont Teiji \takagi}}
\newcommand\takagilifetime  {(1875--1960)}
\newcommand\takeuti         {{\namefont Takeuti}}
\newcommand\takeutiname     {{\namefont Gaisi \takeuti}}
\newcommand\takeutilifetime {(*1926)}
\newcommand\tappindex       {\index{Tapp, Christian}}
\newcommand\tapp            {{\namefont Tapp}}
\newcommand\tappname        {\tappindex{\namefont\christian\ \tapp}}
\newcommand\tarski          {{\namefont Tar\-ski}}
\newcommand\tarskiname      {{\namefont\alfred\ \tarski}}
\newcommand\tarskilifetime  {(1901--1983)}
\newcommand\tarskigrothendieck{\tarski--Grothendieck}
\newcommand\thomasaquinas   {{\namefont\thomas}}
\newcommand\thomasaquinasname{{\namefont\thomasaquinas\ Aquina\es}}
\newcommand\thomasaquinaslifetime{(1225?--1274)}
\newcommand\thales          {{\namefont Thales}}
\newcommand\theiss          {{\namefont Theiss}}
\newcommand\theissname      {{\namefont\frank\ \theiss}}
\newcommand\thurber         {{\namefont Thurber}}
\newcommand\thurbername     {{\namefont\james\ \thurber}}
\newcommand\toepell         {{\namefont Toepell}}
\newcommand\toepellname     {{\namefont\michaelwithouttrema-\markus\ \toepell}}
\newcommand\toyama          {{\namefont Toyama}}
\newcommand\toyamaname      {{\namefont Yoshihito \toyama}}
\newcommand\troelstra       {{\namefont Troelstra}}
\newcommand\troelstraname   {{\namefont Anne Sjerp \troelstra}}
%                           {{\namefont Anne S. \troelstra}}
\newcommand\trotzki         {{\namefont Trotsky}}
\newcommand\trotzkiname     {{\namefont Leon \trotzki}}
\newcommand\trotzkilifetime {(1879--1940)}
\newcommand\turing          {{\namefont Turing}}
\newcommand\turingname      {{\namefont\alan\ \turing}}
\newcommand\turinglifetime  {(1912--1954)}
\newcommand\unguru          {{\namefont Unguru}}
\newcommand\unguruname      {{\namefont Sabetai \unguru}}
\newcommand\unruh           {{\namefont Unruh}}
\newcommand\unruhname       {{\namefont Fritz von \unruh}}
\newcommand\unruhlifetime   {(1885--1970)}
\newcommand\unverzagt       {{\namefont Unverzagt}}
\newcommand\stephanunverzagtname{{\namefont \stephan\ \unverzagt}}
\newcommand\urysohn         {{\namefont Urysohn}}
\newcommand\urysohnname     {{\namefont Pavel Samuilovich \urysohn}}
\newcommand\urysohnlifetime {(1898--1924)}
\newcommand\vandeveire      {Van de Veire}
\newcommand\vandeveirename  {Ann \vandeveire}
\newcommand\veblen          {{\namefont Veblen}}
\newcommand\veblenname      {{\namefont Oswald \veblen}}
\newcommand\venn            {Venn}
\newcommand\vennname        {\john\ \venn}
\newcommand\vennlifetime    {(1834--1923)}
\newcommand\vessiot         {{\namefont Vessiot}}
\newcommand\vessiotname     {{\namefont Ernest \vessiot}}
\newcommand\vessiotlifetime {(1865--1952)}
\newcommand\viete           {{\namefont Vi\`ete}}
\newcommand\vietename       {{\namefont\francois\ \viete}}
\newcommand\vietelifetime   {(1540--1603)}
\newcommand\villon          {Villon}
\newcommand\villonname      {\francois\ \villon}
\newcommand\voigt           {{\namefont Voigt}}
\newcommand\voigtname       {{\namefont\andreas\ \heinrich\ \voigt}}
\newcommand\voigtlifetime   {(1860--1940)}
\newcommand\voronkov        {{\namefont Voron\-kov}}
\newcommand\voronkovname    {{\namefont Andrei \voronkov}}
\newcommand\wagner          {{\namefont Wag\-ner}}
\newcommand\wagnername      {{\namefont Marc \wagner}}
\newcommand\waerden         {{\namefont Waerden}}
\newcommand\waerdenname     {{\namefont Bartel Leendert van der \waerden}}
\newcommand\waerdenlifetime {(1903--1996)}
\newcommand\wajsbergindex   {\index{Wajsberg@Waj\esi berg, Mordechai}}
\newcommand\wajsberg        {{\namefont Waj\esi berg}}
\newcommand\wajsbergname    {\wajsbergindex{\namefont Morde\-chai \wajsberg}}
\newcommand\wajsberglifetime{(1902--1940?)}
\newcommand\waldmann        {Wald\-mann}
\newcommand\waldmanneinsname{\bernard\ \waldmann}
\newcommand\waldmannzweiname{\uwe\ \waldmann}
\newcommand\wallen          {{\namefont Wallen}}
\newcommand\wallenname      {{\namefont Lincoln A. \wallen}}
\newcommand\walsh           {{\namefont Walsh}}
\newcommand\walshname       {{\namefont Toby \walsh}}
\newcommand\walshtwoname    {C. M. \walsh}
\newcommand\walters         {Walter\es}
\newcommand\waltersname     {Humphrey \robert\ ``Pum'' \walters}
\newcommand\walther         {{\namefont Walther}}
\newcommand\walthername     {{\namefont\christoph\ \walther}} 
\newcommand\wang            {Wang} 
\newcommand\wangname        {Hao \wang} 
\newcommand\wedderburn      {{\namefont Wedderburn}}
\newcommand\wedderburnname  {{\namefont\joseph\ H. M. \wedderburn}}
                          %{\joseph\ \henry\ Maclagen \wedderburn}
\newcommand\wedderburnlifetime{(1882--1948)}
\newcommand\weber           {{\namefont Weber}}
\newcommand\webername       {{\namefont \heinrich\ \weber}}
\newcommand\weberlifetime   {(1842--1913)}
\newcommand\wegener         {Wegener} 
\newcommand\wegenername     {Ingo \wegener} 
\newcommand\wegman          {Wegman} 
\newcommand\wegmanname      {Mark N. \wegman} 
\newcommand\weidenbach      {{\namefont Weidenbach}}
\newcommand\weidenbachname  {{\namefont\christoph\ \weidenbach}}
\newcommand\weierstrassindex{\index{Weierstrass@Weierstra\sz, Karl}}
\newcommand\weierstrass     {{\namefont Weierstra\sz}}
\newcommand\weierstrassname {\weierstrassindex{\namefont\karl\ \weierstrass}}
\newcommand\weierstrasslifetime{(1815--1897)}
\newcommand\weil            {{\namefont Weil}}
\newcommand\weilname        {{\namefont Andr\'e \weil}}
\newcommand\weillifetime    {(1906--1998)}
\newcommand\wertheimer      {Wertheimer}
\newcommand\wertheimername  {\maxchristianname\ \wertheimer}
\newcommand\wertheimerlifetime{(1880--1943)}
\newcommand\weylindex       {\index{Weyl, Hermann}}
\newcommand\weyl            {{\namefont Weyl}}
\newcommand\weylname        {\weylindex{\namefont\hermann\ \weyl}}
\newcommand\weyllifetime    {(1885--1955)}
\newcommand\whiteheadindex  {\index{Whitehead, Alfred North}}
\newcommand\whitehead       {{\namefont White\-head}}
\newcommand\whiteheadname   {\whiteheadindex{\namefont\alfred\ North \whitehead}}
\newcommand\whiteheadlifetime{(1861--1947)}
\newcommand\PM              {Principia Mathematica}
\newcommand\PMshort         {Principia}
\newcommand\principleofdependentchoice{Principle of Dependent Choice}
\newcommand\wiles           {{\namefont Wiles}}
\newcommand\wilesname       {{\namefont\andrew\ \wiles}}
\newcommand\wilhelmname     {{\namefont Rein\-hard \wilhelm}}
\newcommand\wirthindex      {\index{Wirth, Claus-Peter}}
\newcommand\wirth           {{\namefont Wirth}}
\newcommand\wirthname       {\wirthindex{\namefont\claus-\peter\ \wirth}}
\newcommand\wirtz           {{\namefont Wirtz}}
\newcommand\wirtzname       {{\namefont Daniela \wirtz}}
\newcommand\wittgenstein    {{\namefont Wittgenstein}} 
\newcommand\wittgensteinname{{\namefont\ludwig\ \wittgenstein}} 
\newcommand\wittgensteinlifetime{(1889--1951)}
\newcommand\wolff           {{\namefont Wolff}} 
\newcommand\wolffname       {{\namefont\christian\ \wolff}} 
%                           {{\namefont\christian\ Freiherr von \wolff}} 
\newcommand\wolfflifetime   {(1679--1754)}
\newcommand\wolska          {{\namefont Wol\-ska}}
\newcommand\wolskaname      {{\namefont\magdalena\ \wolska}}
%                           {{\namefont\magdalena\ A. M. \wolska}}
\newcommand\woods           {{\namefont Wood\es}}
\newcommand\woodsname       {{\namefont\john\ \woods}}
\newcommand\woudename       {Jaap van der Woude}
\newcommand\wrightson       {{\namefont Wright\-son}}
\newcommand\wrightsonname   {{\namefont Graham \wrightson}}
\newcommand\yamada          {Yamada}
\newcommand\yamadaname      {Toshiyuki \yamada}
\newcommand\zachindex       {\index{Zach, Richard}}
\newcommand\zach            {{\namefont Zach}}
\newcommand\zachname        {\zachindex{\namefont\richard\ \zach}}
\newcommand\zantema         {{\namefont Zantema}}
\newcommand\zantemaname     {{\namefont\hans\ \zantema}}
\newcommand\zaremba         {Zaremba}
\newcommand\zarembaname     {\stanislaw\ \zaremba}
\newcommand\zarembalifetime {(1863--1942)}
\newcommand\zeno            {{\namefont Zeno}} 
\newcommand\zenoeinsindex   {\index{Zeno!of Elea}}
\newcommand\zenoeinsname    {\zenoeinsindex{\namefont \zeno\ of Elea}}
                           % elatic school 
\newcommand\zenosparadoxindex{\index{Zeno!'s Paradox}}
\newcommand\zenosparadox    {\zenosparadoxindex{\zeno's Paradox}}
                           % the paradox stems from \zenoeinsname 
\newcommand\zenozweiname    {{\namefont \zeno\ of Citium}}
                           % founder of stoic school
\newcommand\zenodreiname    {{\namefont \zeno\ of Sidon}}
                           % Epicurean school, induction
\newcommand\zenoeinslifetime{(\nth 5\,century\,\BC)}
\newcommand\zenozweilifetime{(\ca\,333--262\,\BC)}
\newcommand\zenodreilifetime{(\ca\,150--70\,\BC)}
\newcommand\zermeloindex    {\index{Zermelo, Ernst}}
\newcommand\zermelo         {{\namefont Zermelo}}
\newcommand\zermeloname     {\zermeloindex{\namefont \ernst\ \zermelo}}
%                           {{\namefont \ernst\ F. E. \zermelo}}
\newcommand\zermelolifetime {(1871--1953)}
\newcommand\ZFlong          {\zermelo--\fraenkel}
\newcommand\ZFshort         {{\sc ZF}}
\newcommand\zhang           {{\namefont Zhang}}
\newcommand\zhangname       {{\namefont Han\-tao \zhang}}
\newcommand\zorn            {Zorn} 
\newcommand\zuse            {{\namefont Zuse}}
\newcommand\zusename        {{\namefont\konrad\ \zuse}}
%                           {{\namefont\konrad\ E. O. \zuse}}
\newcommand\zuselifetime    {(1910--1995)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ABBREVIATIONS and SPECIAL WORDS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%General:

\newcommand\am   {a.m.}
\newcommand\ASF  {ASF}
\newcommand\asfplus{\ASF\/\math{^+}}
\newcommand\afortiori{a fortiori}
\newcommand\Afortiori{A fortiori}
%\newcommand\Av   {\mbox{{A}\hspace{-.09em}{v}}}
\newcommand\appendixes{appendixes}
\newcommand\Apr  {April}
\newcommand\Aug  {Aug.}
\newcommand\ca   {ca.}
\newcommand\Ca   {Ca.}
\newcommand\ct   {c.t.}
\newcommand\fiance{fianc\'e}
\newcommand\FB   {FB}
\newcommand\FBinf{Fachbereich Informatik}
\newcommand\FBinfshort{\FB\ Informatik}
\newcommand\FR   {FR}
\newcommand\FRinf{Fachrichtung Informatik}
\newcommand\FRinfshort{\FR\ Informatik}
\newcommand\f    {\mbox{}{f.}}   %extra block blocks ligature to VI\f
\newcommand\ff   {\mbox{}{ff.}}  %extra block blocks ligature to VI\ff
\newcommand\Fa   {Fa.} % Modis
\newcommand\Feb  {Feb.}
\newcommand\FreeVariable{Free-\math\!Variable}
\newcommand\freevariable{free-variable}
\newcommand\freely{free}
\newcommand\defi {Definition} % note that this controls \litdefiref and \defiref
\newcommand\Dr   {Dr.}
\newcommand\Drrernat{Dr.\,\,rer.\,\,nat.}
\newcommand\EMAIL{E-mail}
\newcommand\eMAIL{e-mail}
\newcommand\ifandonlyif{if \nolinebreak and \onlyif}
\newcommand\Int  {Int.}
\newcommand\international{int.} % \int is the integral in math mode
\newcommand\Inc  {Inc.}
\newcommand\Inst {Inst.}
\newcommand\Jan  {Jan.}
\newcommand\jr   {Jr.}
\newcommand\Math {Math.}
\newcommand\mathe{math.}
\newcommand\MASlong{Mathematics Assistance System}
\newcommand\Maslong{Mathematics assistance system}
\newcommand\maslong{mathematics assistance system}
\newcommand\naiv {na\iwithtrema v}
\newcommand\naive{na\iwithtrema ve}
\newcommand\Naive{Na\iwithtrema ve}
\newcommand\Numero{No.}
\newcommand\Nov  {Nov.}
\newcommand\onlyif{only \nolinebreak if}
\newcommand\pmabbrev{p.m.} % \pm is already a command putting a +- in math
\newcommand\Prof {Prof.}
\newcommand\programme{program}
\newcommand\Programme{Program}
\newcommand\qedabbrev{q.e.d.}
\newcommand\qedhelp[1]{Q.e.d.~({#1})}
\newcommand\getittotheright[1]  
%puts argument flush right, if necessary on fol. line
{\hfill\mbox{}\penalty 100\mbox{\ \,}\nolinebreak
\hfill\hfill\hfill\nolinebreak\mbox{#1}\ignorespaces}
\newcommand\Qed      [1]{\underline{\qedhelp{#1}}}
\newcommand\Qeddouble[1]{\underline{\underline{\qedhelp{#1}}}}
\newcommand\Qedtriple[1]{\underline{\underline{\underline{\qedhelp{#1}}}}}
\newcommand\Qedbf    [1]{\mbox{\bf\qedhelp{#1}}}
\newcommand\QED      [1]{\getittotheright{\Qed      {#1}}}
\newcommand\QEDdouble[1]{\getittotheright{\Qeddouble{#1}}}
\newcommand\QEDtriple[1]{\getittotheright{\Qedtriple{#1}}}
\newcommand\QEDbf    [1]{\getittotheright{\Qedbf    {#1}}}
\newcommand\Role{R\^ole}
\newcommand\role{r\^ole}
\newcommand\Sep  {Sept.}
\newcommand\st   {s.t.}
% s.t. = sine tempore or such that
\newcommand\Tech {Tech.}
\newcommand\Tel  {Tel.}
\newcommand\theo {Theorem}
\newcommand\uni  {Uni\-ver\-si\-t\ae t}
\newcommand\Univ {Univ.}
\newcommand\Vol  {Vol.}
\newcommand\wintersemester{WS}%{Win\-ter-Semes\-ter}
\newcommand\WWW  {WWW}
\newcommand\www  {\url{http://www.ags.uni-sb.de/~cp}}
\newcommand\wwwhb{\url{http://www.dfki.de/hb}}
\newcommand\urlverbraucherpreise{\url{http://www.destatis.de/jetspeed/portal/cms/Sites/destatis/Internet/DE/Content/Statistiken/Zeitreihen/WirtschaftAktuell/Preise/Content100/kpre510bv4,templateId=renderPrint.psml}}

%Abbreviations: English or Latin:

\newcommand\AI   {Artificial Intelligence}
\newcommand\BC   {{\sc b.c.}} % Cf. Lyn Dupre, Bugs in Writing, Segment 21
\newcommand\Bull {Bull.}
\newcommand\Cf   {Cf.}
\newcommand\cf   {cf.}
\def\nlbcite{\nolinebreak\cite}
\newcommand\Cfnlb{\Cf\nolinebreak}
\newcommand\cfnlb{\cf\nolinebreak}
\newcommand\Co   {Co.}
\newcommand\Comm {Comm.}
\newcommand\Comp {Comp.}
\newcommand\Conf {Conf.}
\newcommand\contd{contd.}
\newcommand\ConstructorBased{Con\-struc\-tor-Based}
\newcommand\CS   {Computer \Sci}
\newcommand\CSlong{Computer Science}
\newcommand\Dec  {Dec.}
\newcommand\Dept {Dept.}
\newcommand\descenteinfinie{descente infinie}
\newcommand\Descenteinfinie{Descente infinie}
\newcommand\DescenteInfinie{Descente Infinie}
\newcommand\howdescenteinfiniegoes
{He starts with the conjecture and simplifies it by case analysis.
When he realizes that the current goal becomes 
similar to an instance of the conjecture, 
he applies the instantiated conjecture just like a lemma, 
but keeps in mind that he has actually applied an induction hypothesis. 
Finally, he searches for some \wellfounded\ ordering in which 
all the instances of the conjecture 
% he has
applied as induction hypotheses 
are smaller than the original conjecture.%
% itself.
}
\newcommand\howMethodofDescenteInfiniegoes{Show that for each 
assumed counterexample of \math\Gamma\
there is a smaller counter\-example of \math\Gamma\
\wrt\ a \wellfounded\ ordering \nlbmath<,
which does not depend on the counterexamples.}
\newcommand\theinnermostpartofW
{\math{\forall u\tight<v\stopq\app P  u}}
\newcommand\thelogicalpointofview
{At \fermat's time, natural language was still the predominant tool for 
expressing terms and equations in mathematical writing,
and it was too early for a formal axiomatization.
Moreover, note that an axiomatization captures only validity, but 
in \nolinebreak general neither induces a method of proof search
nor provides the data structures required to admit both
a formal treatment and a human-oriented proof search.
The formalizable logic part, however, of {\em\descenteinfinie}
can be expressed in what is called
the (\secondorder) {\em\theoremofnoetherianinduction} \nlbmath{(\ident{N})}, \ 
after \noethername\ \noetherlifetime. \ 
This is not to be confused with the {\em\axiomofstructuralinduction},
which is generically given for any inductively defined data structure, 
such as the {\em\axiomofstructuralinductionfirsthalf\ 
\nlbmath{(\ident{S})}
\axiomofstructuralinductionsecondhalf\ 
for the natural numbers inductively defined by the constructors
zero \nlbmath{\zeropp} and successor \nlbmath{\ssymbol}}. \
Moreover, we need the definition \nlbmath{(\Wellfpp{\tight<})}
of \wellfoundedness\ of a relation \nlbmath<\@.\smallfootroom
\par\noindent\math{\begin{array}{@{}l@{}r@{\ }l@{}}
 (\Wellfpp{\tight<}) 
&\forall Q\stopq
&\,\inparentheses{\headroom\footroom
     \exists x\stopq\app Q x
   {\nottight{\nottight{\nottight\implies}}}
     \exists m\stopq\inparentheses{\app Q m\und
     \neg\exists w\tight<m\stopq\app Q w}}
 \footroom\\\headroom
 \inpit{\ident{N}}
&\forall P\stopq
&\inparentheses{\headroom
     \forall x\stopq\app P  x
   {\nottight{\nottight{\nottight\antiimplies}}}
     \exists\tight<\stopq\inparenthesesoplist{
      \forall v\stopq\inparentheses{
           \app P  v
         \nottight{\nottight\antiimplies}
           \theinnermostpartofW}
    \oplistund
       \Wellfpp <}\!\!}
 \footroom\\\headroom
 \inpit{\ident{S}}
&\forall P\stopq
&\,\inparentheses{\headroom\forall x\stopq\app P  x
   {\nottight{\nottight{\nottight\antiimplies}}}
   \app P \zeropp\nottight\und
   \forall y\stopq\inparentheses{\app P {\spp y}\antiimplies\app P  y}}
 \footroom\\\headroom
 (\nat 1)
&\forall\boundvari x{}\stopq
&\inparentheses{
     \boundvari x{}\tightequal\zeropp
   \nottight\oder
     \exists
     \boundvari y{}\stopq
     \boundvari x{}\tightequal\spp{\boundvari y{}}}
 \footroom\\\headroom
 (\nat 2)
 &
 \forall
 \boundvari x{}\stopq
 &
 \spp x\tightnotequal\zeropp
 \footroom\\\headroom
 (\nat 3)
 &\forall x,y\stopq
 &\inparentheses{\spp x\tightequal\spp y\nottight\implies x\tightequal y}
\\\end{array}}
\par\halftop\noindent
Let \Wellfpp\ssymbol\ denote 
\Wellfpp{\lambda x,y.\,\inpit{\spp x\tightequal y}},
which implies the \wellfoundedness\ of the ordering of the natural numbers. 
The natural numbers can be specified up to isomorphism
either by \math{(\ident{S})}, \nlbmath{(\nat 2)}, 
and \nlbmath{(\nat 3)}, \hskip.15em 
or else by \Wellfpp\ssymbol\ and \nlbmath{(\nat 1)}\@.
The first alternative 
% is the traditional one, 
% following \dedekind\ and 
follows \dedekindname\ \dedekindlifetime\ and is 
named after \peanoname\ \peanolifetime. 
The second follows \pieriname\ \pierilifetime.  
As the instances for \math P and \nlbmath< in \nlbmath{\inpit{\ident{N}}}
are often still easy to find when the instances for \math P in 
\nlbmath{\inpit{\ident{S}}} are not, \hskip.15em 
the second alternative together with the theorem \nlbmath{\inpit{\ident{N}}}
is to be preferred in theorem proving for its usefulness and elegance. 
See \cite{wirthcardinal} for more on this.}
\newcommand\Diplomarbeit{Diplomarbeit (\Mastersthesis)}
\newcommand\Dissertation{Dissertation (\PhDthesis)}
\newcommand\EcoleNormaleSuperieure{\'Ecole Normale Sup\'erieure}
\newcommand\ed   {ed.}
\newcommand\Ed   {Ed.}
\newcommand\eds  {eds.}
\newcommand\edn  {edn.}
\newcommand\eg   {e.g.}
\newcommand\Eg   {E.g.}
\newcommand\Esp  {Esp.}
\newcommand\esp  {esp.}
%\newcommand\etal{\&al.}%name already use by jsc style.
\newcommand\etalabbrev{{\namefont\&al.}}
\newcommand\etc  {\&c.}
\newcommand\etclong{etc.}
\newcommand\exfalsoquodlibet{ex falso quodlibet}
\newcommand\extd {extd.}
\newcommand\Extd {Extd.}
\newcommand\sententialtautology{sentential tautology}
\newcommand\SententialTautology{Sentential Tautology}
\newcommand\sententialtautologies{sentential tautologies}
\newcommand\substitutionalsententialtautology
{substitutional sentential tautology}
\newcommand\substitutionalsententialtautologies
{substitutional sentential tautologies}
\newcommand\signatureenlarge     {enrich}
\newcommand\signatureenlarges    {enriches}
\newcommand\signatureenlarging   {enriching}
\newcommand\signatureenlarged    {enriched}
\newcommand\signatureenlargedby  {enriched with}
\newcommand\signatureenlargement {enrichment}
\newcommand\Signatureenlargement {Enrichment}
\newcommand\sr   {Sr.}
\newcommand\asignatureenlargement{an enrichment}
\newcommand\firstorder{first-order}
\newcommand\Firstorder{First-order}
\newcommand\FirstOrder{First-Order}
\newcommand\fol  {following}
\newcommand\ibid {ibid.} % ibidem, at the same place.
\newcommand\ie   {i.e.}
\newcommand\Ie   {I.e.}
\newcommand\incl {incl.}
\newcommand\uiff {\ iff\ }
\newcommand\udiff{\ if\ }
\newcommand\HumanOrientedInteractiveATP
{Human-Oriented Interactive Automated Theorem Proving}
\newcommand\ITP  {Inductive Theorem Proving}
\newcommand\Jun  {June}
\newcommand\Jul  {July}
% \newcommand\Log  {Log.}
\newcommand\LK   {{LK}}
\newcommand\LJ   {{LJ}}
\newcommand\Ltd  {Ltd.}
\newcommand\May  {May}
\newcommand\Mar  {March}
\newcommand\Mastersthesis{Master's thesis}
\newcommand\MSc  {M.Sc.}
\newcommand\MrUS {Mr.}
\newcommand\mutatismutandis{mutatis mutandis}
\newcommand\Mutatismutandis{Mutatis mutandis}
\newcommand\ND   {Natural Deduction}
% There is an alternative by \usepackage{proof} and 
% \infer*{#2}{[#1]} that does four nice dots in between.
\newcommand\nonpermutable{non-permu\-ta\-ble}
\newcommand\nonpermutability{non-permu\-ta\-bi\-lity}
\newcommand\NonPermutability{Non-Permu\-ta\-bi\-lity}
\newcommand\nonpermutabilities{non-permu\-ta\-bi\-li\-ties}
\newcommand\NonPermutabilities{Non-Permu\-ta\-bi\-li\-ties}
\newcommand\negbyfail{negation as failure}
\def\note{Note}
\newcommand\notes{Notes}
%note that \note determines \litnoteref and \noteref.
\newcommand\Oct  {Oct.}
\newcommand\p    {p.}
\newcommand\pp   {pp.}
\newcommand\PP[2]{\pp\,\ignorespaces#1--\ignorespaces#2}
% Like \pp but gets first and last page as arguments
\newcommand\PPcount[1]{#1\,\pp}
\newcommand\PhD  {PhD}%{Ph.D.}
\newcommand\PhDthesis{\PhD\ thesis}
\newcommand\PhDThesis{\PhD\ Thesis}
\newcommand\Proc {Proc.}
\newcommand\pnc  {posi\-tive/ne\-ga\-tive-condi\-tional}
\newcommand\Pnc  {Posi\-tive/ne\-ga\-tive-condi\-tional}
\newcommand\PNC  {Posi\-tive/Ne\-ga\-tive-Condi\-tional}
\newcommand\prep {prep.}
\newcommand\Publ {Publ.}
\newcommand\Quart{Quart.}
\newcommand\resp {resp.}
\newcommand\rev  {rev.}
\newcommand\Rev  {Rev.}
\newcommand\secondorder{second-order}
\newcommand\Secondorder{Second-Order}
\newcommand\sect {\myparagraphsymbol} 
%note that \sect determines \litsectref and \sectref.
\newcommand\sects{\myparagraphsymbol\myparagraphsymbol}
\newcommand\thissect{this \nolinebreak\sect}
\newcommand\Sci  {Sci.}
\newcommand\sic  {sic}
\newcommand\unary{singulary} % Following Quine's Mathematical Logic, p. 13:
% singulary, binary, ternary, quaternary, quinary
\newcommand\singulary{singulary}
\newcommand\Singulary{Singulary}
\newcommand\nullary  {nullary}
\newcommand\Soc  {Soc.}
\newcommand\substitutionlemma{{\sc Substitution \opt{Value} Lemma}}
\newcommand\explicitnesslemma{{\sc Explicitness Lemma}}
\newcommand\valuationlemma   {{\sc Valuation Lemma}}
\newcommand\foralllemma      {{\sc\math\forall-Lemma}}
\newcommand\existslemma      {{\sc\math\exists-Lemma}}
\newcommand\implieslemma     {{\sc\tightimplies-Lemma}}
%\newcommand\undlemma         {{\sc\tightund-Lemma}}
\newcommand\negationlemma    {{\sc\tight\neg-Lemma}}
\newcommand\vel  {vel}
\newcommand\vs   {vs.}
\newcommand\wellformed{well-formed}
\newcommand\wellformedness{well-formed\-ness}
\newcommand\wellfounded{well-founded}
\newcommand\WellFounded{Well-Founded}
\newcommand\nonwellfounded{non-well-founded}
\newcommand\wellfoundedness{well-founded\-ness}
\newcommand\Wellfoundedness{Well-founded\-ness}
\newcommand\wellordered{well-ordered}
\newcommand\wellorderedness{well-ordered\-ness}
\newcommand\wellordering{well-ordering}
\newcommand\Wellordering{Well-ordering}
\newcommand\WellOrdering{Well-Ordering}
\newcommand\WellOrderingTheorem{Well-Ordering Theorem}
\newcommand\wrog {w.l.o.g.} % My favorite misspelling. Moreover \wlog is
\newcommand\Wrog {W.l.o.g.} % already a latex command
\newcommand\wrt  {w.r.t.}
\newcommand\Wrt  {W.r.t.}
\newcommand\WWWhomepage{\WWW-home-page}
\newcommand\WYSIWYG{WYSIWYG}
\newcommand\zornslemma{\zorn's Lemma}

%Abbreviations: German
\newcommand\Abs{Abs.}
\newcommand\bzw{bzw\hskip-.08em.}
\newcommand\Dasheisst{D.\nolinebreak\,h.}
\newcommand\dasheisst{d.\nolinebreak\,h.}%\dh already defined
\newcommand\dasist{d.\nolinebreak\,i.}
\newcommand\Dez{Dez.}
\newcommand\exkl{exkl.}
\newcommand\ggf{ggf.}
\newcommand\geb{geb.}
\newcommand\Ges{Ges.}
\newcommand\Ing{Ing.}
\newcommand\inkl{inkl.}
\newcommand\Jh{Jh.}
\newcommand\lt{lt.}
\newcommand\Mae{M\ae rz}
\newcommand\Mai{Mai}
\newcommand\Juni{Juni}
\newcommand\MwSt{M\hskip-0.06emwSt.}
\newcommand\Nr{Nr.}
\newcommand\oa{o.\penalty100\,a.}
\newcommand\oViA{o.V.\penalty100\,i.\penalty100\,A.}
\newcommand\Okt{Okt.}
\newcommand\reell{re\unprotectedewithtrema ll}
\newcommand\so{s.o.}
\newcommand\St{St.}
\newcommand\Staatl{Staatl.}
\newcommand\Str{Str.}
\newcommand\ua{u.\penalty100\,a.} % und andere
\newcommand\usw{usw.}
\newcommand\vgl{vgl.}
\newcommand\Vgl{Vgl.}
\newcommand\vglnlb{\vgl\nolinebreak}
\newcommand\zB{z.\penalty100\,B.}
\newcommand\ZB{Z.\penalty100\,B.}
\newcommand\zT{z.\penalty100\,T.}
\newcommand\ZT{Z.\penalty100\,T.}
\newcommand\zHd{z.\penalty100\,H.}

\newcommand\pncgerman{posi\-tiv/ne\-ga\-tiv be\-dingt}
\newcommand\constructorbasedgerman{kon\-struk\-tor\-ba\-siert}
\newcommand\Inferenzsystem{In\-ferenz\-sy\esi tem}
\newcommand\Rahmeninferenzsystem{Rah\-men\-in\-ferenz\-sy\esi tem}
\newcommand\Inferenzregel{In\-ferenz\-re\-gel}
\newcommand\Termersetzungssystem{Term\-er\-setzung\esi sy\esi tem}
\newcommand\gegenueber{ge\-gen\-\ue ber}
\newcommand\Beweissteuerungskonzept{Be\-wei\esi steue\-rung\esi kon\-zept}

% references

\newcommand\Axioms{Axioms}
\newcommand\thewordand{and}
\newcommand\litspageref[1]{Page\,#1}
\newcommand\litspagerefs[2]{Pages #1 \nolinebreak \thewordand\ \nolinebreak #2}
\newcommand\litspagerefss[3]{Pages #1, #2 \thewordand\ \nolinebreak #3}
\newcommand\litconjref[1]{Conjecture\,#1}
\newcommand\litfootref[1]{Footnote\,#1}
\newcommand\litrequref[1]{Requirement\,#1}
\newcommand\litnoteref[1]{\note\,#1}
\newcommand\litremaref[1]{Remark\,#1}
\newcommand\lititemref[1]{Item\,#1}
\newcommand\litfiguref[1]{Figure\,#1}
\newcommand\litslidref[1]{Slide\,#1}
\newcommand\litprobref[1]{Problem\,#1}
\newcommand\littheoref[1]{\theo\,#1}
\newcommand\litsectref[1]{\sect\,#1} %previously called \sectimm
\newcommand\nlblitsectref[1]{\nolinebreak\litsectref{#1}}
\newcommand\litchapref[1]{Chapter\,#1} %{\sect\,#1}
\newcommand\litchapwithsectref[2]{Chapter\,#1, \sect\,#2}%{\sect\,#1.#2} 
\newcommand\litnotefromtoref[2]{\notes\,#1--#2}
\newcommand\litchapfromtoref[2]{Chapters\,#1--#2}
\newcommand\litsectfromtoref[2]{\sects\,#1--#2}%previously called \sectfromtoimm
\newcommand\lititemfromtoref[2]{Items #1 \nolinebreak to \nolinebreak #2}
\newcommand\litdefiref[1]{\defi\,#1}
\newcommand\Examplename{Ex\-am\-ple}
\newcommand\litexamref[1]{\Examplename\,#1}
\newcommand\litcoexref[1]{Counter\-ex\-am\-ple\,#1}
\newcommand\litlemmref[1]{Lem\-ma\,#1}
\newcommand\litaxioref[1]{Axiom\,#1}
\newcommand\litcororef[1]{Co\-rollary\,#1}
\newcommand\litpropref[1]{Pro\-po\-si\-tion\,#1}
\newcommand\litproprefs[2]
{Pro\-po\-si\-tions \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\litrequrefs
[2]{Require\-ments  \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\lititemrefs
[2]{Items           \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\litexamrefs[2]
{Examples        \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\litcoexrefs[2]
{Counterexamples \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\litlemmrefs[2]
{Lem\-mas        \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\litaxiorefs[2]
{\Axioms\        \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\litcororefs[2]
{Co\-rol\-laries \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\littheorefs[2]
{Theorems        \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\litnoterefs[2]
{\notes\         \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\litsectrefs[2]
{\sects\         \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\litfigurefs[2]
{Figures         \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\litchaprefs[2]
{Chapters        \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\litdefirefs[2]
{Definitions     \nolinebreak #1 \thewordand\ \nolinebreak #2}
\newcommand\lititemrefss
[3]{Items \nolinebreak #1, #2, \thewordand\ \nolinebreak #3}
\newcommand\litdefirefss
[3]{Definitions \nolinebreak #1, #2, \thewordand\ \nolinebreak #3}
\newcommand\litexamrefss
[3]{Examples \nolinebreak #1, #2, \thewordand\ \nolinebreak #3}
\newcommand\litlemmrefss
[3]{Lemmas \nolinebreak #1, #2, \thewordand\ \nolinebreak #3}
\newcommand\litaxiorefss
[3]{\Axioms\ \nolinebreak #1, #2, \thewordand\ \nolinebreak #3}
\newcommand\litcororefss
[3]{Co\-rol\-laries \nolinebreak #1, #2, \thewordand\ \nolinebreak #3}
\newcommand\litnoterefss
[3]{\notes\ \nolinebreak #1, #2, \thewordand\ \nolinebreak #3}
\newcommand\litsectrefss
[3]{\sects\ \nolinebreak #1, #2, \thewordand\ \nolinebreak #3}
\newcommand\litfigurefss
[3]{Figures \nolinebreak #1, #2, \thewordand\ \nolinebreak #3}
\newcommand\spageref[1]{\litspageref{\pageref{#1}}}
\newcommand\spagerefs[2]{\litspagerefs{\pageref{#1}}{\pageref{#2}}}
\newcommand\specref[1]{Spec.\,\ref{#1}}
\newcommand\requref[1]{\litrequref{\ref{#1}}}
\newcommand\conjref[1]{\litconjref{\ref{#1}}}
\newcommand\remaref[1]{\litremaref{\ref{#1}}}
\newcommand\slidref[1]{\litslidref{\ref{#1}}}
\newcommand\probref[1]{\litprobref{\ref{#1}}}
\newcommand\cororef[1]{\litcororef{\ref{#1}}}
\newcommand\lemmref[1]{\litlemmref{\ref{#1}}}
\newcommand\axioref[1]{\litaxioref{\ref{#1}}}
\newcommand\examref[1]{\litexamref{\ref{#1}}}
\newcommand\coexref[1]{\litcoexref{\ref{#1}}}
\newcommand\defiref[1]{\litdefiref{\ref{#1}}}
\newcommand\theoref[1]{\littheoref{\ref{#1}}}
\newcommand\itemref[1]{\lititemref{\ref{#1}}}
\newcommand\figuref[1]{\litfiguref{\ref{#1}}}
\newcommand\noteref[1]{\litnoteref{\ref{#1}}}
\newcommand\sectref[1]{\litsectref{\ref{#1}}}
\newcommand\nlbsectref[1]{\nolinebreak\sectref{#1}}
\newcommand\sectrefff[1]{\litsectref{\ref{#1}\,\ff\ \ignorespaces}}
\newcommand\Sectref[1]{\litsectref{\ref{#1}}}
\newcommand\itemrefs[2]{\lititemrefs{\ref{#1}}{\ref{#2}}}
\newcommand\requrefs[2]{\litrequrefs{\ref{#1}}{\ref{#2}}}
\newcommand\defirefs[2]{\litdefirefs{\ref{#1}}{\ref{#2}}}
\newcommand\lemmrefs[2]{\litlemmrefs{\ref{#1}}{\ref{#2}}}
\newcommand\axiorefs[2]{\litaxiorefs{\ref{#1}}{\ref{#2}}}
\newcommand\examrefs[2]{\litexamrefs{\ref{#1}}{\ref{#2}}}
\newcommand\coexrefs[2]{\litcoexrefs{\ref{#1}}{\ref{#2}}}
\newcommand\cororefs[2]{\litcororefs{\ref{#1}}{\ref{#2}}}
\newcommand\theorefs[2]{\littheorefs{\ref{#1}}{\ref{#2}}}
\newcommand\noterefs[2]{\litnoterefs{\ref{#1}}{\ref{#2}}}
\newcommand\sectrefs[2]{\litsectrefs{\ref{#1}}{\ref{#2}}}
\newcommand\figurefs[2]{\litfigurefs{\ref{#1}}{\ref{#2}}}
\newcommand\sectfromtoref[2]{\litsectfromtoref{\ref{#1}}{\ref{#2}}}
\newcommand\notefromtoref[2]{\litnotefromtoref{\ref{#1}}{\ref{#2}}}
\newcommand\globalrequirementref[1]{\globalrequirement\,\ref{#1}}
\newcommand\itemrefss[3]{\lititemrefss{\ref{#1}}{\ref{#2}}{\ref{#3}}}
\newcommand\defirefss[3]{\litdefirefss{\ref{#1}}{\ref{#2}}{\ref{#3}}}
\newcommand\examrefss[3]{\litexamrefss{\ref{#1}}{\ref{#2}}{\ref{#3}}}
\newcommand\noterefss[3]{\litnoterefss{\ref{#1}}{\ref{#2}}{\ref{#3}}}
\newcommand\lemmrefss[3]{\litlemmrefss{\ref{#1}}{\ref{#2}}{\ref{#3}}}
\newcommand\axiorefss[3]{\litaxiorefss{\ref{#1}}{\ref{#2}}{\ref{#3}}}
\newcommand\cororefss[3]{\litcororefss{\ref{#1}}{\ref{#2}}{\ref{#3}}}
\newcommand\sectrefss[3]{\litsectrefss{\ref{#1}}{\ref{#2}}{\ref{#3}}}
\newcommand\figurefss[3]{\litfigurefss{\ref{#1}}{\ref{#2}}{\ref{#3}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%% here starts the \nth macro %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% It gets an integer or a character as argument and prints e.g. 
%%% \nth{1}    --->   1st
%%% \nth{11}   --->  11th
%%% \nth{21}   --->  21st
%%% \nth{-31}  ---> -31th
%%% \nth n     ---> nth
%%% \nth q     ---> qth
%%% \nth{nn}   ---> NONSENSE
%%% some more computation features provided
%%% uses count 0-5
%%% \mth      is like \nth but sets base  number in math mode
%%% \nonumbermth is like \mth, but does not work for numbers,
%%%              but for whole mathematical expressions
%%% \nonumbermst is like \nonumbermth, but puts ``st''
%%% \smallnth is like \nth but sets power text tiny
% \newcommand\nth[1]{#1\/\math{^{\hbox{\scriptsize th}}}}
% this was raising too much! And too stupid!
%\newcommand\nth[1]{\nthpositioner{#1}{\nthstring{#1}}}
%This was too big.
\newcommand\nthpositioner[2]
% do not put something around the #1! It may remove relevant font information.
{#1\raisebox{0.52ex}{\scriptsize\hspace{0.07em}#2}}
\newcommand\nth[1]{\nthtinypositioner{#1}{\nthstring{#1}}}
\newcommand\nthtinypositioner[2]{#1\raisebox{0.52ex}{\tiny\hspace{0.07em}#2}}
\newcommand\mth[1]{\mthpositioner{#1}{\nthstring{#1}}}
\newcommand\mthpositioner[2]
% do not put something around the #1! It may remove relevant font information.
{\math{#1}\raisebox{0.52ex}{\scriptsize\hspace{0.07em}#2}}
\newcommand\modulointocountzero[2]
{\count1=#1
\count2=#2
\count0=\count1
\divide  \count0 by \count2
\multiply\count0 by-\count2
\advance \count0 by \count1}
\newcommand\absolutevalueintocountzero[1]
{\count0=#1
\ifnum\count0<0\multiply\count0 by -1\fi}
\newcommand\nthstring[1]
{\def\myargone{#1}\ifcat a\myargone th\else\nthstringnochar{#1}\fi}
\newcommand\nthstringnochar[1]
{\absolutevalueintocountzero{#1}%
\modulointocountzero{\count0}{100} %we need the blank here!
\ifnum\count0>9\ifnum\count0<20 th\else\stupidnthstring\fi
                                  \else\stupidnthstring\fi}
\newcommand\stupidnthstring
{\modulointocountzero{\count0}{10}
\ifnum\count0=1 \hskip-0.2em st\else
\ifnum\count0=2 nd\else
\ifnum\count0=3 rd\else 
                th\fi\fi\fi}
\newcommand\nonumbermth[1]{\mthpositioner{#1}{th}}
\newcommand\nonumbermst[1]{\mthpositioner{#1}{st}}

\newcommand\writeascents
%writes and integer abc as a.bc
% 0   --> 0.00
% 123 --> 1.23
[1]{\count4=#1
\ifnum\count4<0 
-\multiply\count4 by -1\fi
\modulointocountzero{\count4}{10}
\divide\count4 by 10
\count3=\the\count0
\modulointocountzero{\count4}{10}
\divide\count4 by 10
\the\count4
.\the\count0
\the\count3
}

\newcommand\frenchnth[1]{\nthtinypositioner{#1}{\frenchnthstring{#1}}}
% this work correctly only for 1 and 2 by now!
\newcommand\frenchnthstring[1]
{\def\myargone{#1}\ifcat a\myargone th\else\frenchnthstringnochar{#1}\fi}
\newcommand\frenchnthstringnochar[1]
{\absolutevalueintocountzero{#1}%
\modulointocountzero{\count0}{100} %we need the blank here!
\ifnum\count0>9\ifnum\count0<20 th\else\frenchstupidnthstring\fi
                                  \else\frenchstupidnthstring\fi}
\newcommand\frenchstupidnthstring
{\modulointocountzero{\count0}{10}
\ifnum\count0=1 \hskip-0.2em re\else
\ifnum\count0=2 me\else
\ifnum\count0=3 rd\else 
                th\fi\fi\fi}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%% here ends the \nth macro %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Systems %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\COQ       {{\sc Coq}}
\newcommand\ACLTWO    {{\sc Acl2}}
\newcommand\ASCII     {{\sc Ascii}}
\newcommand\INTWOMATH {In2Math}
\newcommand\DAMIT     {DaMiT}
\newcommand\MATHWEB   {{\sc MathWeb}}
\newcommand\ACTIVEMATH{\mbox{\sc ActiveMath}}
\newcommand\AUTOMATH  {\mbox{\sc AutoMath}}
\newcommand\OANTS     {\math\Omegaoffont{\sc Ants}}
\newcommand\OPENMATH  {{\sc OpenMath}}
\newcommand\TPS       {{\sc TPS}}
\newcommand\RRL       {{\sc Rrl}}
\newcommand\SPIKE     {{\sc Spike}}
\newcommand\INKA      {{\sc Inka}}
\newcommand\NQTHM     {{\sc Nqthm}}
\newcommand\PROLOG    {{\sc Prolog}}
\newcommand\PERL      {{\sc Perl}}
\newcommand\OMEGA     {\math\Omegaoffont{\sc mega}} 
\newcommand\OYSTER    {{\sc Oyster}}
\newcommand\OYSTERCLAM{\OYSTER-\CLAM}
\newcommand\CLAM      {{\rm CL\kern-.36em\raise.39ex\hbox{\sc a}\kern-.15emM}}
\newcommand\LEOII     {\mbox{\sc Leo-II}}
\newcommand\LAMBDACLAM{{\sc \math\lambda\CLAM}}
\newcommand\LATEXML   {{\sc \LaTeX ML}}
\newcommand\ISAPLANNER{{\sc Isa\-Plan\-ner}}
\newcommand\LOUI      {{\sc L}\math\Omegaoffont{\sc UI}} 
\newcommand\CORE      {{\sc CoRe}}
\newcommand\C         {{\sc C}} 
\newcommand\COMMONLISP{{\sc Common Lisp}} 
\newcommand\JAVA      {{\sc Java}} 
\newcommand\HASKELL   {{\sc Haskell}} 
\newcommand\CURRY     {{\sc Curry}}
\newcommand\FORTRAN   {{\sc Fortran}} 
\newcommand\QUODLIBET {{\sc Quod\-Libet}} 
\newcommand\QML       {{\sc Qml}} 
\newcommand\TECTON    {{\sc Tec\-ton}} 
\newcommand\TEXMACS   {{\sc T\kern-.1667em\lower.5ex\hbox{E}\kern-.125emX\kern-.1em\lower.5ex\hbox{\textsc{m\kern-.05ema\kern-.125emc\kern-.05ems}}}}
\newcommand\XQUODLIBET{{\sc XQuod\-Libet}} 
\newcommand\EXPANDER  {{\sc Expander}} 
\newcommand\XEXPANDER {{\sc eXpander}} 
\newcommand\UNICOM    {{\sc Unicom}} 
\newcommand\KNUTHBENDIX{\knuth--\bendix}
\newcommand\PREX{\mbox{\itshape P\hspace{-2pt}.\hspace{1pt}rex\/}}
\newcommand\MBASE{{\sc MBase}}
\newcommand\ml{{\sc ml}}
\newcommand\MLshort{{\sc ML}}
\newcommand\NFshort{{\sc NF}}
\newcommand\MLlong{\quine'\es\ \nolinebreak\MLshort}
\newcommand\NFlong{\quine'\es\ \nolinebreak\NFshort}
\newcommand\ISABELLE{{\sc Isabelle}}
\newcommand\ISABELLEHOL{{\sc Isa\-belle/HOL}}
\newcommand\PVS{{\sc PVS}}
\newcommand\SystemB{System\,(B)}
\newcommand\SystemZ{System\,(Z)}
\newcommand\VAMPIRE{{\sc Vampire}}
\newcommand\VERIFUN{{\normalsize\math{\checkmark\!\!}}{\footnotesize\sc eriFun}}
\newcommand\VSE{{\sc VSE}}
\newcommand\XML{{\sc XML}}
\newcommand\WALDMEISTER{\index{Waldmeister}{\sc Wald\-Meister}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Institutions %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\DFKI{\mbox{DFKI}}
\newcommand\ags{AG Siekmann}
\newcommand\CMU{Carnegie Mellon \Univ}
\newcommand\MPIIabbrev{MPI-INF}
\newcommand\MPII{\plancknamenonamefont\ \Inst\ f\ue r Informatik} 
\newcommand\MPIIenglish{\plancknamenonamefont\ \Inst\ for Informatics} 
\newcommand\MPIIenglishlong{\plancknamenonamefont\ Institute for Informatics} 
\newcommand\UCBerkeley{\Univ\ of \California, \Berkeley}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Geographic Places %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\Aberdeen       {Aber\-deen}
\newcommand\Amsterdam      {Amster\-dam}
\newcommand\Augsburg       {Aug\esi burg}
\newcommand\Avignon        {Avignon}
\newcommand\California     {California}
\newcommand\Cambridge      {Cam\-bridge}
\newcommand\Chicago        {Chicago}
\newcommand\Cologne        {Cologne}
\newcommand\Berkeley       {Berkeley}
\newcommand\Berlin         {Ber\-lin}    
\newcommand\Bologna        {Bologna}
\newcommand\Boston         {Boston}
\newcommand\Breslau        {Bre\esi lau}
\newcommand\Buffalo        {Buffalo (NY)}    
\newcommand\DO             {Dort\-mund}
\newcommand\Dagstuhl       {Dag\-stuhl}
\newcommand\Darmstadt      {Darm\-stadt}
\newcommand\Diez           {Diez}
\newcommand\EB             {Edin\-burgh}
\newcommand\FFM            {Frank\-furt am Main}
\newcommand\Freiburg       {Freiburg (Breisgau)}
\newcommand\Genf           {Gen\`eve}
\newcommand\Genua          {Genova}
\newcommand\Glasgow        {Glasgow}
\newcommand\Goettingen     {G\oe ttingen}
\newcommand\Halle          {Halle an der Saale}
\newcommand\Hamburg        {Ham\-burg}
\newcommand\Harvard        {Har\-vard}
\newcommand\Hildesheim     {Hilde\esi heim}
\newcommand\Heidelberg     {Heidel\-berg}
\newcommand\Helsinki       {Helsingfor\es}
\newcommand\Innsbruck      {Inn\esi bruck}
\newcommand\Jena           {Jena}
\newcommand\KA             {Karl\esi ruhe}
\newcommand\KL             {Kaiser\esi lau\-tern}
\newcommand\KO             {Ko\-blenz}
\newcommand\Koeln          {K\oe ln}
\newcommand\Koenigsberg    {K\oe nig\esi berg}
\newcommand\Kopenhagen     {K\o ben\-havn}
\newcommand\Landau         {Lan\-dau}
\newcommand\Marburg        {Mar\-burg}
\newcommand\NewBrunswick   {New Brun\esi wick (NJ)}
\newcommand\NewYork        {New York}
\newcommand\LA             {Lo\es\ Angele\es}
\newcommand\Leipzig        {Leip\-zig}
\newcommand\London         {Lon\-don}
\newcommand\Mannheim       {Mann\-heim}
\newcommand\Massachusetts  {Massachusett\es}
\newcommand\Muenchen       {M\ue n\-chen}
\newcommand\Muenster       {M\ue nster}
\newcommand\Nancy          {Nancy}
\newcommand\Napoli         {Napoli}
\newcommand\Nuernberg      {N\ue rn\-berg}
\newcommand\Oslo           {Oslo}
\newcommand\Oxford         {Oxford}
\newcommand\Pontamousson   {Pont-\`a-Mousson (France)}
\newcommand\Princetonnostate{Princeton}
\newcommand\Princeton      {\Princetonnostate\ (NJ)}
\newcommand\Prag           {Prague}
\newcommand\Paris          {Pari\es}
\newcommand\SB             {Saar\-br\ue cken}
\newcommand\StAndrews      {St\,Andrews}
\newcommand\StPetersburg   {\St\ Peter\-burg}
\newcommand\SaratogaSprings{Sara\-toga Springs (NY)}
\newcommand\Stuttgart      {Stutt\-gart}
\newcommand\Stanford       {Stan\-ford}
\newcommand\Torino         {Torino}
\newcommand\Turkey         {Turkey}
\newcommand\Warszawa       {Warszawa}
\newcommand\WarszawaEnglish{Warsaw}
\newcommand\Washington     {Washington (DC)}
\newcommand\Wien           {Wien}
\newcommand\WI             {Wie\esi ba\-den}
\newcommand\Worms          {Worms}
\newcommand\Zuerich        {\mbox{Z\ue rich}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ADDRESSES AND NAMES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\plzuniKL  {\mbox{D--67653}}
\newcommand\plzuniDO  {\mbox{D--44221}}
\newcommand\plzuniSB  {\mbox{D--66123}}
\newcommand\plzWIinnen{\mbox{D--65183}}
\newcommand\plzdiez   {\mbox{D--65582}}
\newcommand\plzdudweiler{\mbox{D--66125}}

\newcommand\kcl         {King's College, \London}
\newcommand\uniEB       {University of \EB}
\newcommand\uniAberdeen {University of \Aberdeen}
\newcommand\uniGlasgow  {University of \Glasgow}
\newcommand\uniStAndrews{University of \StAndrews}
\newcommand\HeriotWatt{Heriot--Watt}
\newcommand\uniheriotwatt{\HeriotWatt\ University}
\newcommand\uniDO{\uni\ \DO}
\newcommand\uniKO{\uni\ \KO-\Landau}
\newcommand\uniKA{\uni\ \KA}
\newcommand\uniKL{\uni\ \KL}
\newcommand\uniSB{\uni\ des Saar\-lan\-de\es}
\newcommand\uniKLenglish{University of \KL}
\newcommand\uniSBenglish{Saar\-land University}
\newcommand\uniSBenglishshort{Saar\-land \Univ}

\newcommand\uniDOshort{\Univ\ \DO}
\newcommand\uniKLshort{\Univ\ \KL}
\newcommand\uniSBshort{Saar\-land \Univ}
\newcommand\uniEBshort{\Univ\ \EB}
\newcommand\uniKOshort{\Univ\ \KO-\Landau}
\newcommand\uniKAshort{\Univ\ \KA}

\newcommand\addressuniKL{\FBinf, \uniKL}
\newcommand\addressuniKLshort{\FBinfshort, \uniKLshort}
\newcommand\addressuniDOshort{\FBinfshort, \uniDOshort}
\newcommand\addressuniSBshort{\FRinfshort, \uniSBshort}
\newcommand\addressuniKLcomplete
{\FBinf, \uniKL, Postfach\,3049, \plzuniKL\,\KL, Germany}
\newcommand\addressuniDOcomplete
{Informatik, \uniDO, \plzuniDO\,\DO, Germany} 
\newcommand\addressuniSBcomplete
{\FRinf, \uniSB, \plzuniSB\,\SB, Germany} 
\newcommand\addressuniKLlongwithnl
{\FBinf,\\\uniKL,\\\plzuniKL\,\KL}
\newcommand\addressuniDOlongwithnl
{Informatik,\\\uniDO,\\\plzuniDO\,\DO} 
\newcommand\addressuniKLlongwithnlwithoutcomma
{\FBinf\\\uniKL\\\plzuniKL\,\KL}
\newcommand\addressuniDOlongwithnlwithoutcomma
{Informatik\\\uniDO\\\plzuniDO\,\DO} 
\newcommand\addressuniSBlongwithnlwithoutcomma
{\FRinf\\\uniSB\\\plzuniSB\,\SB} 
\def       \emailcp      {{\tt wirth@logic.at}}
\newcommand\emailmhwithoutfontinfo{marianeh.rezaei@gmail.com}
\newcommand\emailmh      {{\tt \emailmhwithoutfontinfo}}
% {{\tt marianeh\_80@yahoo.com}}
\newcommand\Institutedept{\Dept\ of \CSlong}
\newcommand\Instituteinst{\mbox\uniSBenglish}
\newcommand\Instituteplac{\plzuniSB\,\SB}
\newcommand\Institutecoun{Germany}
\newcommand\Institute
{\Institutedept, \Instituteinst, \Instituteplac, \Institutecoun}
% {\planckname\ Institute for Informatics, \plzuniSB\,\SB, Germany}
% {Brandenburger Str.\,42, \plzdiez\ \Diez, Germany}
\newcommand\Institutewithnl
{\Institutedept\\\Instituteinst\\\Instituteplac\\\Institutecoun}


\newcommand\SFB        {Collaborative Research Center}
\newcommand\oursfbshort{SFB\,378}
\newcommand\oursfblong {\SFB\ \oursfbshort}
\newcommand\oursfbname {Resource-Adaptive Cognitive Processes}
\newcommand\oldsfbshort{SFB\,314}
\newcommand\oldsfblong {\SFB\ \oldsfbshort}
\newcommand\oldsfbname {AI~---~Knowledge-Based Systems}

\newcommand\Myfocusofinterest{P\myfocusofinterestrest}
\newcommand\myfocusofinterest{p\myfocusofinterestrest}
\newcommand\myfocusofinterestrest
{ractice-relevant human-oriented interactive (co-) inductive 
theorem proving in first- and higher-order logics
with strong automation support,
as exemplified by our \QUODLIBET\ and \OMEGA\ systems}
\newcommand\myareasofexpertise{%
Logic%
, 
Theoretical Computer 
% \Sci%
Science%
, 
Formal Methods%
, 
\AI%
}
\newcommand\mysubfields{%
(Co-) Inductive Theorem Proving (automated/interactive)%
, 
Conditional Term Rewriting, Confluence Theorems%
, 
\hilbert's epsilon%
, 
Free-Variable Calculi%
, 
Proof Planning%
, 
\MASlong s%
,
Efficient Algorithms%
, 
Algebraic Specification%
, 
Hypertext Web Models%
,
History of Philosophy and Logic%
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Citation commands %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% LECTURE NOTES

\newcommand\CSLILN[1]
{CSLI LN\,#1, CSLI Publications, \Stanford\ \Univ}

% SPRINGER LECTURE NOTES

% LNCS
\newcommand\LNCSvol[1]
{\mbox{LNCS}\,\ignorespaces#1}

% LNAI
\newcommand\LNAIvol[1]
{\mbox{LNAI}\,\ignorespaces#1}

% LNM
\newcommand\LNMvol[1]
{\mbox{LNM}\,\ignorespaces#1}


% Verlage---------------------------------------------------------------------
\newcommand\academicpress{Academic Press (\elsevier)}
\newcommand\ACM{ACM}
\newcommand\acmpress{\ACM\ Press}
\newcommand\addisonwesley{Addi\-son-Wes\-ley}
\newcommand\allenandunwin{\george\ Allen \& Unwin, \London}
\newcommand\birkhaeuser{Birkh\ae user (\springerverlag)}
\newcommand\cambridgeunipress{\Cambridge\ \Univ\ Press}
\newcommand\chicagounipress{\Univ\ \Chicago\ Press}
\newcommand\univcaliforinapress
{\Univ\ of \California\ Press, \Berkeley\ and \LA}
\newcommand\clarendonpress{Clarendon Press%, \Oxford
}
\newcommand\deGruyter{de\,Gruyter, \Berlin, \NewYork}
\newcommand\digitalpress{Digital Press (\elsevier)}
\newcommand\elsevier{Elsevier}
\newcommand\gauthiervillars{Gauthier-Villars, \Paris}
\newcommand\harvardunipress{\Harvard\ \Univ\ Press}
\newcommand\ieee{IEEE}
\newcommand\ieeepress{\ieee\ Press}
\newcommand\indianaunipress{Indiana \Univ\ Press}
\newcommand\infixverlag{Infix, 
Aka\-de\-mi\-sche Ver\-lags\-ge\-sell\-schaft Aka GmbH, 
Sankt Au\-gustin, \Berlin}
\newcommand\kluwer{Kluwer% Acad.\ \Publ
, now part of \SPRINGER}
\newcommand\mcgrawhill{McGraw-Hill}
\newcommand\morgankaufmann{Morgan Kaufman (\elsevier)}
\newcommand\mitpress{MIT Press}
\newcommand\northholland{North-Holland (\elsevier)}
\newcommand\oxfordunipress{\Oxford\ \Univ\ Press}
\newcommand\pitman{Pitman \Publ, \London%
% This has been taken over by Financial Times Press and is hard to find.
% Thus, the place should be given explicitly!
}
\newcommand\PrenticeHall{Prentice--Hall, \Inc}
\newcommand\princetonunipress{\Princetonnostate\ \Univ\ Press}
\newcommand\DReidelpublishing{D. Reidel \Publ, Dordrecht, now part of \SPRINGER}
\newcommand\sfischerverlagberlin{S. Fischer Ver\-lag, \Berlin}
\newcommand\sfischerverlagffm{S. Fischer Ver\-lag, \FFM}
\newcommand\springerverlag{Sprin\-ger}
\newcommand\SPRINGER{Springer Science+Business Media}
\newcommand\teubner{Teub\-ner}
\newcommand\teubnerverlag{B. G. \teubner\ Ver\-lags\-ge\-sell\-schaft}
\newcommand\teubnerarchivzurmathematik[1]
{\teubner-Archiv zur Mathe\-ma\-tik, \Vol\,#1, \teubnerverlag, \Leipzig}
\newcommand\vannostrand{D. Van Nostrand}
\newcommand\vieweg{Vieweg, Braunschweig} 
\newcommand\wiley{\john\ Wiley \& Sons}
\newcommand\wissenschaftlichebuchgesellschaftdarmstadt
 {Wissen\-schaft\-liche Buch\-gesell\-schaft, \Darmstadt}

%Reports----------------------------------------------------------------------
\newcommand\sekireportname{SEKI-Report}
\newcommand\sekireportissn{1437--4447}
\newcommand\sekireportnoaddress[2]{\sekireportname\ \mbox{SR--#1--#2}}
\newcommand\sekireport   [2]{\sekireportnoaddress{#1}{#2}, \addressuniKLshort}
\newcommand\sekireportSB [2]{\sekireportnoaddress{#1}{#2}, \addressuniSBshort}
\newcommand\sekireportnew[2]{\sekireportnoaddress{#1}{#2}, ISSN\,1437-4447}

\newcommand\sekiworkingpapername{SEKI-Working-Paper}
\newcommand\sekiworkingpaperissn{1860--5931}
\newcommand\sekiworkingpapernoaddress[2]
{\sekiworkingpapername\ \mbox{SWP--#1--#2}}
\newcommand\sekiworkingpaper[2]{\sekiworkingpapernoaddress
{#1}{#2}, \addressuniKLshort}
\newcommand\sekiworkingpapernew[2]{\sekiworkingpapernoaddress
{#1}{#2}, ISSN\,1860-5931}

\newcommand\gruenereihe[2]{Report #2/#1, \addressuniDOshort}

\newcommand\mpireportnoaddress[2]{MPI--I--#1--2--#2}
\newcommand\mpireport[2]{\mpireportnoaddress{#1}{#2}, \MPII, \SB}

\newcommand\daireport
[1]{DAI Research Paper \Numero\,#1, \Dept\ \AI, \uniEBshort}

%Conferencen------------------------------------------------------------------
\newcommand\lncsconf[6]{\nth{#2}\,#1\,#3, #4, \PP{#5}{#6}, \springerverlag}

%AAAI
\newcommand\AAAI[4]
{\nth{#1} AAAI 19#2, \PP{#3}{#4}, \mitpress}
\newcommand\eighthAAAIninety{\AAAI{8}{90}}

%ALP1
\newcommand\fourthAlgLogPninetyfour
{\lncsconf{Algebraic and Logic Programming}{4}{1994}{\LNCSvol{850}}}

%ALP2
\newcommand\fourteenthAutLanPeightyseven
{\lncsconf{Automata, Languages and Programming}{14}{1987}{\LNCSvol{267}}}


%CAAP
\newcommand\CAAPname{\Int\ Colloquium on Trees in Algebra and Programming}
\newcommand\CAAPshort{CAAP}
\newcommand\ninthCAAPeightyfourtitle
{\Proc\ \nth 9 \CAAPname\ (\CAAPshort\,1984), Bordeaux}
%% Please use a separate bib entry!
%% \newcommand\ninthCAAPeightyfour[2]
%% {In: Bruno Courcelle (\ed): \ninthCAAPeightyfourtitle,
%%% \PP{#1}{#2}, \cambridgeunipress}
\newcommand\twentyfirstCAAPninetysix
{\lncsconf\CAAPshort{21}{1996}{\LNCSvol{1059}}}

%CADE
\newcommand\CADEname{\Int\ \Conf\ on Automated Deduction}
\newcommand\CADEshort{CADE}
\newcommand\thelocalCADE[3]{\nth{#1} \CADEname, #3, #2}
\newcommand\fifthCADEeighty           
{\lncsconf\CADEshort {5}{1980}{\LNCSvol{  87}}}
\newcommand\eighthCADEeightysix                  
{\lncsconf\CADEshort {8}{1986}{\LNCSvol{ 230}}}
\newcommand\theninthCADEeightyeight                
{\thelocalCADE       {9}{1988}{Argonne National Laboratory (IL)}}
\newcommand\ninthCADEeightyeight                
{\lncsconf\CADEshort {9}{1988}{\LNAIvol{ 310}}}
\newcommand\thetenthCADEninety                      
{\thelocalCADE      {10}{1990}{\KL}}
\newcommand\tenthCADEninety                      
{\lncsconf\CADEshort{10}{1990}{\LNAIvol{ 449}}}
\newcommand\theeleventhCADEninetytwo             
{\thelocalCADE  {11}{1992}{\SaratogaSprings}}
\newcommand\eleventhCADEninetytwo                
{\lncsconf\CADEshort{11}{1992}{\LNAIvol{ 607}}}
\newcommand\thetwelvethCADEninetyfour            
{\thelocalCADE  {12}{1994}{Nancy}}
\newcommand\twelvethCADEninetyfour               
{\lncsconf\CADEshort{12}{1994}{\LNAIvol{ 814}}}
\newcommand\thethirteenthCADEninetysix           
{\thelocalCADE  {13}{1996}{\NewBrunswick}}
\newcommand\thirteenthCADEninetysix              
{\lncsconf\CADEshort{13}{1996}{\LNAIvol{1104}}}
\newcommand\thesixteenthCADEninetynine              
{\thelocalCADE  {16}{1999}{Trento, Italy}}
\newcommand\sixteenthCADEninetynine              
{\lncsconf\CADEshort{16}{1999}{\LNAIvol{1632}}}
\newcommand\eightteenthCADEtwo                   
{\lncsconf\CADEshort{18}{2002}{\LNAIvol{2392}}}
\newcommand\theeightteenthCADEtwo                   
{\thelocalCADE  {18}{2002}{\Kopenhagen}}
\newcommand\nineteenthCADEthree                   
{\lncsconf\CADEshort{19}{2003}{\LNAIvol{2741}}}
\newcommand\thenineteenthCADEthree                   
{\thelocalCADE  {19}{2003}{Miami Beach (FL)}}
\newcommand\thetwentiethCADEfive
{\thelocalCADE  {20}{2005}{Tallinn}}
\newcommand\twentiethCADEfive
{\lncsconf\CADEshort{20}{2005}{\LNAIvol{3632}}}

%CALCULEMUS

%CCL
\newcommand\firstCCL{\nth 1 Workshop on 
Construction of Computational Logics, Val d'Ajol (France), 1992}

%CLP
\newcommand\eighthCLPtitle
{\Proc\ \nth{8} \Int\ \Conf\ on Logic Programming}
\newcommand\twelvethCLPtitle
{\Proc\ \nth{12} \Int\ \Conf\ on Logic Programming}
%% Please use a new bib entry instead!
%% \newcommand\eighthCLP  [2]{\eighthCLPtitle,   1991, \PP{#1}{#2}, \mitpress}
%% \newcommand\twelvethCLP[2]{\twelvethCLPtitle, 1995, \PP{#1}{#2}, \mitpress}

%CSL
\newcommand\CSLname{\Conf\ of the European Association for \CS\ Logic}

%CTRS
\newcommand\CTRSname{\Int\ Workshop on Conditional Term Rewriting Systems}
\newcommand\CTRSshort{CTRS}
\newcommand\theCTRS[3]{\nth{#1} \CTRSname, #3, #2}
\newcommand\firstCTRSeightyseven   {\lncsconf\CTRSshort{1}{1987}{\LNCSvol{308}}}
\newcommand\thefirstCTRSninetytwo         {\theCTRS{1}{1987}
{Orsay (France)}}
\newcommand\secondCTRSninety       {\lncsconf\CTRSshort{2}{1990}{\LNCSvol{516}}}
\newcommand\thirdCTRSninetytwo     {\lncsconf\CTRSshort{3}{1992}{\LNCSvol{656}}}
\newcommand\thethirdCTRSninetytwo         {\theCTRS{3}{1992}{\Pontamousson}}
\newcommand\fourthCTRSninetyfour   {\lncsconf\CTRSshort{4}{1994}{\LNCSvol{968}}}
\newcommand\thefourthCTRSninetyfour       {\theCTRS{4}{1994}{Jerusalem}}

%ECAI
\newcommand\ECAIname{European \Conf\ on \AI}
\newcommand\ECAI[5]
{{\em\nth{#1} \ECAIname\ (ECAI\,#2)}, \PP{#4}{#5}, #3}
\newcommand\eighthECAIeightyeight
{{\namefont Y. Kodratoff} (\ed). \ECAI{8}{1988}{\pitman}}
% This is correct!
\newcommand\ninthECAIninety{\ECAI{9}{1990}{\pitman}}
\newcommand\eleventhECAIninetyfour
{{\namefont A. G. Cohn} (\ed). \ECAI{11}{1994}{\wiley}}

%FTP
\newcommand\FTPname{\Int\ Workshop on First-Order Theorem Proving}
\newcommand\FTPshort{FTP}

%ICALP
\newcommand\thirteenthICALPeightysix{\lncsconf{ICALP}{13}{1986}{\LNCSvol{226}}}

%IJCAI
\newcommand\IJCAIname{\Int\ Joint \Conf\ on \AI}
\newcommand\IJCAI    {IJCAI}
\newcommand\eleventhIJCAIeightnine
[2]{In: {\namefont N. S. Sridharan} (\ed). 
       {\em \Proc\ \nth{11} \IJCAIname\ (\IJCAI)}, \PP{#1}{#2},
       \morgankaufmann}
\newcommand\thirteenthIJCAIninetythree
[2]{In: {\namefont Ruzena Bajcsy} (\ed). 
       {\em \Proc\ \nth{13} \IJCAIname\ (\IJCAI)}, \PP{#1}{#2},
       \morgankaufmann}
\newcommand\seventeenthIJCAIone
[2]{In: \nebelname\ (\ed). 
       {\em \Proc\ \nth{17} \IJCAIname\ (\IJCAI)}, \PP{#1}{#2},
       \morgankaufmann}

%IJCAR
\newcommand\IJCARname{\Int\ Joint \Conf\ on Automated Reasoning}
\newcommand\thelocalIJCAR[3]{\nth{#1} \IJCARname, #3, #2}
\newcommand\firstIJCARone{\lncsconf{IJCAR}{1}{2001}{\LNAIvol{2083}}}
\newcommand\thefirstIJCARone{\thelocalIJCAR{1}{2001}{Siena, Italy}}

%LFCS
\newcommand\LFCSname{\Int\ Symposium on Logical Foundations of \CS}
\newcommand\LFCSshort{LFCS}
\newcommand\thirdLFCSninetyfour
{\lncsconf\LFCSshort{3}{1994}{\LNCSvol{813}}}

%LICS
\newcommand\LICSname{\ieee\ Symposium on Logic In \CS}
\newcommand\LICS[3]
{#1 \LICSname, \PP{#2}{#3}, \ieeepress}
\newcommand\firstLICSeightysix  {\LICS{\nth 1}}
\newcommand\thirdLICSeightyeight{\LICS{\nth 3}}

%LPAR
\newcommand\LPAR{LPAR}
\newcommand\LPARname{\Int\ \Conf\ on Logic for Programming, \AI, and Reasoning}
\newcommand\thirdLPARninetytwo  {\lncsconf{LPAR} {3}{1992}{\LNAIvol {624}}}
\newcommand\fifthLPARninetyfour {\lncsconf{LPAR} {5}{1994}{\LNAIvol {822}}}
\newcommand\eleventhLPARzerofour{\lncsconf{LPAR}{11}{2004}{\LNAIvol{3452}}}
\newcommand\twelfthLPARzerofive {\lncsconf{LPAR}{12}{2005}{\LNAIvol{3835}}}

%MKM
\newcommand\MKMshort{MKM}
\newcommand\MKMname{\Int\ \Conf\ on Mathematical Knowledge Management}
\newcommand\theforthMKMfive{\nth 4 \MKMname\ (\MKMshort), Bremen, 2005}
\newcommand\fourthMKMfive{\lncsconf{MKM}{4}{2005}{\LNAIvol{3863}}}

%RTA
\newcommand\RTAname
{\Int\ \Conf\ on Rewriting Techniques and Applications}
\newcommand\theRTA[3]
{\nth{#1} \RTAname, #3, #2}
\newcommand\thirdRTAeightynine       {\lncsconf{RTA}{ 3}{1989}{\LNCSvol{ 355}}}
\newcommand\fourthRTAninetyone       {\lncsconf{RTA}{ 4}{1991}{\LNCSvol{ 488}}}
\newcommand\thesixthRTAninetyfive           {\theRTA{ 6}{1995}{\KL}}
\newcommand\sixthRTAninetyfive       {\lncsconf{RTA}{ 6}{1995}{\LNCSvol{ 914}}}
\newcommand\theseventhRTAninetysix          {\theRTA{ 7}{1996}{\NewBrunswick}}
\newcommand\seventhRTAninetysix      {\lncsconf{RTA}{ 7}{1996}{\LNCSvol{1103}}}
\newcommand\eighthRTAninetyseven     {\lncsconf{RTA}{ 8}{1997}{\LNCSvol{1232}}}
\newcommand\tenthRTAninetynine       {\lncsconf{RTA}{10}{1999}{\LNCSvol{1631}}}

%STACS
\newcommand\STACSname{\Int\ Symposium on Theoretical Aspects of \CS}
\newcommand\STACSshort{STACS}
\newcommand\eleventhSTACSninetyfour{\lncsconf{STACS}{11}{1994}{\LNCSvol{775}}}

%TABLEAUX
\newcommand\TABLEAUname
{\Int\ \Conf\ on Tableaus and Related Methods}
\newcommand\TABLEAUshort{TAB\-LEAUX}
\newcommand\theTABLEAU[3]
{\nth{#1} \TABLEAUname, #3, #2}
\newcommand\thefourthTABLEAUninetyfive{\theTABLEAU{5}{1995}{\St\ Goar (Germany)}}
\newcommand\fourthTABLEAUninetyfive
{\lncsconf\TABLEAUshort{4} {1995}{\LNAIvol{ 918}}}
\newcommand\thesixthTABLEAUninetyseven{\theTABLEAU{6}{1997}{\Pontamousson}}
\newcommand\sixthTABLEAUninetyseven
{\lncsconf\TABLEAUshort{6} {1997}{\LNAIvol{1227}}}
\newcommand\eighthTABLEAUninetynine
{\lncsconf\TABLEAUshort{8} {1999}{\LNAIvol{1617}}}
\newcommand\theeighthTABLEAUninetynine    
{\theTABLEAU{8} {1999}{\SaratogaSprings}}
\newcommand\ninthTABLEAUzero       
{\lncsconf\TABLEAUshort{9} {2000}{\LNAIvol{1847}}}
\newcommand\theeleventhTABLEAUtwo  
{\theTABLEAU{11}{2002}{\Kopenhagen}}
\newcommand\eleventhTABLEAUtwo     
{\lncsconf\TABLEAUshort{11}{2002}{\LNAIvol{2381}}}
\newcommand\thefourteenthTABLEAUfive{\theTABLEAU{14}{2005}{\KO}}
\newcommand\fourteenthTABLEAUfive
{\lncsconf\TABLEAUshort{14}{2005}{\LNAIvol{3702}}}


%TAPSOFT
\newcommand\TAPSOFTninetythree[2]
{TAPSOFT 1993, \LNCSvol{668}, \PP{#1}{#2}, \springerverlag}

%TPHOLs
\newcommand\TPHOLshort{TPHOLs}
\newcommand\TPHOLname{\Int\ \Conf\ on Theorem Proving in Higher-Order Logics}
\newcommand\theninthTPHOLninetysix{\nth 9 \TPHOLname\ (\TPHOLshort), Turku (Finland), 1996}
\newcommand\TPHOLninetysix[2]
{\theninthTPHOLninetysix, \LNCSvol{1125}, \PP{#1}{#2}, \springerverlag}


%UNIF
\newcommand\UNIFname{\Int\ Workshop on Unificiation}
\newcommand\UNIFshort{UNIF}

%Newspapers-------------------------------------------------------------------

\newcommand\newspaperreference[5]
{\def\nameofjournalpress{#2}#1, #4 #5, #3\if?\nameofjournalpress
\else, #2\fi}

\newcommand\nytimes{\newspaperreference{The \NewYork\ Times}?}

%Journals---------------------------------------------------------------------

\newcommand\dateinjournal[1]{}

\newcommand\journalreference[6]
{\def\nameofjournalpress{#2}#1\nolinebreak\hskip.2em%
\dateinjournal{(#3) }{\mbox{\bf #4}}, \PP{#5}{#6}\if?\nameofjournalpress
\else, #2\fi}

\newcommand\journalreferenceprintyear[6]
{\def\nameofjournalpress{#2}#1 
{(#3) }{\bf #4}, \PP{#5}{#6}\if?\nameofjournalpress
\else, #2\fi}

\newcommand\journalreferenceprintyearaspartofnumber[6]
{\def\nameofjournalpress{#2}#1 
{#4/#3}, \PP{#5}{#6}\if?\nameofjournalpress
\else, #2\fi}

\newcommand\AARname{Association for Automated Reasoning}
\newcommand\AARshort{AAR}

\newcommand\AbhandlungenmathHamburgname
{Abhandlungen au\es\ dem mathematischen Seminar der \Univ\ Hamburg}
\newcommand\AbhandlungenmathHamburg
{\journalreference
{\AbhandlungenmathHamburgname}?}

\newcommand\actacybernetica
{\journalreference{Acta Cybernetica}{Szeged}}

\newcommand\actamathematicaprintyear
{\journalreference{Acta Mathematica}?}

\newcommand\americanmathematicalmonthlyname{American Mathematical Monthly}
\newcommand\americanmathematicalmonthly
{\journalreference{\americanmathematicalmonthlyname}?}

\newcommand\americanjmath
{\journalreference{American J. of \Math}?}

\newcommand\americanscientistname
{American Scientist}

\newcommand\americanscientistprintyear
{\journalreferenceprintyear{\americanscientistname}?}

\newcommand\annalesecolesuperieur
{\journalreference{Annales Scientifiques d l'\EcoleNormaleSuperieure}?}

\newcommand\annalesuniversiteparis
{\journalreference{Annales de l'Universit\'e de \Paris}?}

\newcommand\annalsofmathematicsname{Annals of Mathematics}
\newcommand\annalsofmathematics{\journalreference{\annalsofmathematicsname}?}

\newcommand\archivehistoryexactsciences
{\journalreference{Archive for History of Exact Sciences}\springerverlag}

\newcommand\artificialintelligence
{\journalreference{\AI}?}
\newcommand\artificialintelligenceprintyear
{\journalreferenceprintyear{\AI}?}

\newcommand\artificialintelligencetools
{\Int\ J. \AI\ Tools}

\newcommand\artificialintelligencetoolsprintyear
{\journalreferenceprintyear{\artificialintelligencetools}?}

\newcommand\AttiAccadTorinoname{Atti della Reale Accademia delle Scienze di \Torino\ ---  Classe di Scienze Morali, Storiche e Filologiche e Classe di Scienze Fisiche, Matematiche e Naturali}
\newcommand\AttiAccadTorino
{\journalreference{\AttiAccadTorinoname}?}

\newcommand\AttiAccadTorinoFisicheMatematicheNaturali
{\journalreference{Atti della Reale Accademia delle Scienze di \Torino\ ---
Classe di Scienze Fisiche, Matematiche e Naturali}?}

\newcommand\EATCSname{European Assoc.\ for Theoretical \CS}
\newcommand\EATCSshort{EATCS}
\newcommand\bulleatcs
{\journalreference{\Bull\ \EATCSshort}?}

\newcommand\AMSname{American \Math\ \Soc}
\newcommand\AMSshort{AMS}
\newcommand\bullamsname
{\Bull\ \AMSname}
\newcommand\bullams
{\journalreference{\bullamsname}?}

\newcommand\noticesamsname{Notices of the \AMSname}
\newcommand\transamsname{Transactions of the \AMSname}

\newcommand\cahierssemhistmath
{\journalreference{Cahiers du s\'eminaire d'histoire des math\'ematiques}?}

\newcommand\comptesrendusname
{Comptes rendus hebdomadaires des s\'eances de l'Acad\'emie des Sciences 
(\Paris)}

\newcommand\comptesrendus
{\journalreference{\comptesrendusname}?}

\newcommand\computationallinguisticsname{Computational Linguistic\es}
\newcommand\computationallinguistics
{\journalreference{\computationallinguisticsname}?}

\newcommand\commacm
{\journalreference{\Comm\ \ACM}\acmpress}

\newcommand\dmvjahresberichtname
{Jahre\esi bericht der Deutschen Mathe\-matiker-Ver\-eini\-gung}

\newcommand\dmvmitteilungenname{DMV-Mitteilungen}
\newcommand\dmvmitteilungen
{\journalreferenceprintyearaspartofnumber{\dmvmitteilungenname}?}

\newcommand\ENTCSname{Electronic Notes in Theoretical \CS}
\newcommand\ENTCS
{\journalreference\ENTCSname\elsevier}

\newcommand\erkenntisannalen{Erkenntnis (Annalen der Philosophie (und Philosophischen Kritik))}

\newcommand\forschungenname
{Forschungen zur Logik und zur Grundlegung der exakten Wissenschaften}

\newcommand\forschungen
{\journalreference
{\forschungenname}
\Leipzig}

\newcommand\fundamentainformaticaename
{Fundamenta Informaticae}

\newcommand\fundamentainformaticae
{\journalreference{\fundamentainformaticaename}?}

\newcommand\ieicetrans
{\journalreference{IEICE Transactions}?}

\newcommand\informationandcomputation
{\journalreference{Information and Computation}\academicpress}

\newcommand\informationandcontrol
{\journalreference{Information and Control}?}

\newcommand\historiamathematica
{\journalreference{Historia Mathematica}?}

\newcommand\historyandphilosophyoflogicname
{History and Philosophy of Logic}
\newcommand\historyandphilosophyoflogic
{\journalreference
{\historyandphilosophyoflogicname}{Taylor \& Francis, \London}}

\newcommand\aaeccname
{J. Applicable Algebra in Engineering, Communication and Computing (AAECC)}
\newcommand\aaecc
{\journalreference\aaeccname\springerverlag}
\newcommand\aaeccprintyear
{\journalreferenceprintyear\aaeccname\springerverlag}

\newcommand\ieeetransse
{\journalreference{\ieee\ Transactions on Software Engineering}\ieeepress}

\newcommand\jacm
{\journalreference{J. \ACM}\acmpress}

\newcommand\jalname{J. Applied Logic}
\newcommand\jal
{\journalreference\jalname\elsevier}
\newcommand\jalprintyear
{\journalreferenceprintyear\jalname\elsevier}

\newcommand\jarname
{J. Automated Reasoning}
\newcommand\jar
{\journalreference\jarname\kluwer}
\newcommand\jarprintyear
{\journalreferenceprintyear\jarname\kluwer}

\newcommand\janclname{J. Applied Non-Classical Logics}
\newcommand\jancl{\journalreference\janclname?}

\newcommand\jcssname{J. Computer and System \Sci}
\newcommand\jcss
{\journalreference{\jcssname}\academicpress}

\newcommand\jlc
{\journalreference{J. Logic Computat.}\oxfordunipress}


\newcommand\jmathpuresapplname
{J.  de \Math\ Pures et Appliqu\'ees (J. \liouville)}


\newcommand\jmathpuresappl
{\journalreference{\jmathpuresapplname}?}

\newcommand\jphillogicname{J. Philosophical Logic}
\newcommand\jphillogic
{\journalreference{\jphillogicname}\kluwer}


\newcommand\jreineundangewandtemathematikname
{J.\ f\ue r die reine und angewandte Mathematik (\crelle sches J.)}

\newcommand\jreineundangewandtemathematik
{\journalreference{\jreineundangewandtemathematikname}?}


\newcommand\jscname
{J. Symbolic Computation}
\newcommand\jsc
{\journalreference{\jscname}\academicpress}
\newcommand\jscshort
{\journalreference{\jscname}?}
\newcommand\jscprintyear
%{\journalreferenceprintyear{\jscname}?}
{\journalreferenceprintyear{\jscname}\academicpress}

\newcommand\jslname{J. Symbolic Logic}
\newcommand\jsl
{\journalreference{\jslname}?}

\newcommand\leinseignementmathematiquename
{L'Enseignement Math\'e\-matique}
\newcommand\leinseignementmathematique
{\journalreference{\leinseignementmathematiquename}?}

\newcommand\linguisticinquiryname{Linguistic Inquiry}
\newcommand\linguisticinquiry
{\journalreference{\linguisticinquiryname}\mitpress}

\newcommand\linguisticsandphilosophyname{Linguistics and Philosophy}
\newcommand\linguisticsandphilosophy
{\journalreference{\linguisticsandphilosophyname}?}

\newcommand\ljigplname{Logic J. of the IGPL}
\newcommand\ljigpl
{\journalreference\ljigplname\oxfordunipress}
\newcommand\ljigplprintyear
{\journalreferenceprintyear\ljigplname\oxfordunipress}

\newcommand\mathematicallogicquarterlyname{\Math\ Logic \Quart}
\newcommand\mathematicallogicquarterly
{\journalreference{\mathematicallogicquarterlyname}?}

\newcommand\mathematischezeitschrift
{\journalreference{Mathematische Zeitschrift}?}

\newcommand\mindname{Mind}

\newcommand\mind{\journalreference{\mindname}?}

\newcommand\MathematischeAnnalen{Mathe\-ma\-ti\-sche Annalen}
\newcommand\mathematischeannalen
{\journalreference{\MathematischeAnnalen}?}

\newcommand\mitteilungenmathgeshamburgprintyear
{\journalreferenceprintyear
{Mitteilungen der Mathematischen Gesellschaft in Hamburg}?}

\newcommand\modernlogic
{\journalreference{Modern Logic}?}

\newcommand\monatsheftempname
{Monat\esi hefte f\ue r Mathematik und Physik}

\newcommand\monatsheftemp
{\journalreference{\monatsheftempname}?}

\newcommand\NordiskMatematiskTidskrift
{\journalreference{Nordisk Matematisk Tidskrift}?}

\newcommand\notredamename{Notre Dame J. of Formal Logic}
\newcommand\notredame
{\journalreference{\notredamename}?}

\newcommand\philosphiamathname{Philosophia Mathematica (III)}
\newcommand\philosphiamath
{\journalreference{\philosphiamathname}?}

\newcommand\physisname{Physis}
\newcommand\physis{\journalreference{\physisname}?}

\newcommand\cambridgephilsoc
{\journalreference{\Proc\ \Cambridge\ Philosophical \Soc}?}

\newcommand\revuemetaphysiquemorale
{\journalreference{Revue de M\'etaphysique et de Morale}?}

\newcommand\sciencejournalname
{Science}

\newcommand\sciencejournalprintyear
{\journalreferenceprintyear{\sciencejournalname}?}

\newcommand\skriftername
{Skrifter, Norske Videnskaps-Akademi i Oslo 
(=  Videnskapsselskapet i Kristiania), 
Matema\-tisk-Natur\-viden\-skapelig Klasse}

\newcommand\skrifterpublisher
{J. Dybwad, \Oslo}

\newcommand\skrifter[4]
{\journalreference{\skriftername}
{\skrifterpublisher}{#1}{#1/#2}{#3}{#4}}

\newcommand\WarsawScientificSocietyIII
{Towarzystwa Naukowego Warszaw\-skiego, Wydzia\l\ III}

\newcommand\sprawozdaniazposiedzenname
{Sprawozdania z posiedze\'n \WarsawScientificSocietyIII\ (Comptes Rendus S\'eances Soci\'et\'e des Sciences et Lettres Varsovie, Cl.\,III)}

\newcommand\sprawozdaniazposiedzen
{\journalreference{\sprawozdaniazposiedzenname}?}

\newcommand\tcsname{Theoretical \CS}
\newcommand\tcsjournal
%{\journalreference\tcsname ?}
{\journalreference\tcsname\elsevier}
\newcommand\tcsjournalprintyear
%{\journalreference\tcsname ?}
{\journalreferenceprintyear\tcsname\elsevier}

\newcommand\themathematicsteachername{The Mathematics Teacher}
\newcommand\themathematicsteacher
{\journalreference{\themathematicsteachername}{ISSN\,0025-5769}}

\newcommand
\vierteljahresschriftfuerwissenschaftlichephilosophiename
{Vier\-tel\-jahr\esi schrift f\ue r wissenschaftliche Philosophie}

\newcommand\vierteljahresschriftfuerwissenschaftlichephilosophie
{\journalreference
{\vierteljahresschriftfuerwissenschaftlichephilosophiename}?}

\newcommand\ZLGname{Zeitschrift f\ue r \mathe\ Logik und Grundlagen der \Math}
\newcommand\ZLG
{\journalreference{\ZLGname}?}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ARCHIVES

\newcommand\handschrifenabteilungSUBGoettingen
{Nieders\ae chsische Staat\es- und Universit\ae t\esi bibliothek 
 % of the {\namefont Georg August} Universit\ae t 
 \Goettingen, Hand\-schriften\-ab\-teilung}

\newcommand\handschriftenabteilungMIGoettingen
{Georg August Universit\ae t \Goettingen, 
 Mathematisches \Inst, Lesesaal}
 

==> headertheorem.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\catcode`\@=11
%%%% added 3rd parameter being put to beginning of newtheorems text.
%       ****************************************
%       *         THEOREM ENVIRONMENTS         *
%       ****************************************
%
%  The user creates his own theorem-like environments with the command
%      \newtheorem{NAME}{TEXT}[COUNTER]  or
%      \newtheorem{NAME}[OLDNAME]{TEXT}
%  This defines the environment NAME to be just as one would expect a
%  theorem environment to be, except that it prints ``TEXT'' instead of
%  ``Theorem''.
%
%  If OLDNAME is given, then environments NAME and OLDNAME use the same
%  counter, so using a NAME environment advances the number of the next
%  NAME environment, and vice-versa.
%
%  If COUNTER is given, then environment NAME is numbered within COUNTER.
%  E.g., if COUNTER = subsection, then the first NAME in subsection 7.2
%  is numbered TEXT 7.2.1.
%
%  The way NAME environments are numbered can be changed by redefining
%  \theNAME.
%
%  DOCUMENT STYLE PARAMETERS
%
%  \@thmcounter{COUNTER} : A command such that
%               \edef\theCOUNTER{\@thmcounter{COUNTER}}
%         defines \theCOUNTER to produce a number for a theorem environment.
%         The default is:
%            BEGIN \noexpand\arabic{COUNTER} END
%
%  \@thmcountersep : A separator placed between a theorem number and
%         the number of the counter within which it is numbered.
%         E.g., to make the third theorem of section 7.2 be numbered
%         7.2-3, \@thmcountersep should be \def'ed to '-'.  Its
%         default is '.'.
%
%  \@begintheorem{NAME}{NUMBER} : A command that begins a theorem
%         environment for a 'theorem' named 'NAME NUMBER' --
%         e.g., \@begintheorem{Lemma}{3.7} starts Lemma 3.7.
%
%  \@opargbegintheorem{NAME}{NUMBER}{OPARG} : A command that begins a theorem
%         environment for a 'theorem' named 'NAME NUMBER' with optional
%         argument OPARG -- e.g., \@begintheorem{Lemma}{3.7}{Jones}
%         starts `Lemma 3.7 (Jones):'.
%
%  \@endtheorem : A command that ends a theorem environment.
%
% \newtheorem{NAME}{TEXT}[COUNTER] ==
%   BEGIN
%     if \NAME is definable
%       then \@definecounter{NAME}
%            if COUNTER present
%              then \@addtoreset{NAME}{COUNTER} fi
%                   \theNAME ==  BEGIN \theCOUNTER \@thmcountersep
%                                       eval\@thmcounter{NAME}      END
%              else \theNAME ==  BEGIN eval\@thmcounter{NAME} END
%            \NAME == \@thm{NAME}{TEXT}
%            \endNAME == \@endtheorem
%       else  error
%     fi
%   END
%
% \newtheorem{NAME}[OLDNAME]{TEXT}==
%   BEGIN
%     if \NAME is definable
%       then \theNAME == \theOLDNAME
%            \NAME == \@thm{OLDNAME}{TEXT}
%            \endNAME == \@endtheorem
%       else  error
%     fi
%   END
%
% \@thm{NAME}{TEXT} ==
%   BEGIN
%    \refstepcounter{NAME}
%    if next char = [
%       then \@ythm{NAME}{TEXT}
%       else \@xthm{NAME}{TEXT}
%    fi
%   END
%
% \@xthm{NAME}{TEXT} ==
%   BEGIN
%    \@begintheorem{TEXT}{\theNAME}
%    \ignorespaces
%   END
%
% \@ythm{NAME}{TEXT}[OPARG] ==
%   BEGIN
%    \@opargbegintheorem{TEXT}{\theNAME}{OPARG}
%    \ignorespaces
%   END
%
\def\newtheorem#1{\@ifnextchar[{\@othm{#1}}{\@nthm{#1}}}
 
\def\@nthm#1#2{%
%typical #1=definition, #2=Definition
\@ifnextchar[{\@xnthm{#1}{#2}}{\@ynthm{#1}{#2}}}
 
\def\@xnthm#1#2[#3]#4{%next line commented for brutal redefinition
%\expandafter\@ifdefinable\csname #1\endcsname
%typical #1=definition, #2=Definition, #3=section, #4=cpspecial
{\@definecounter{#1}\@addtoreset{#1}{#3}%
\expandafter\xdef\csname the#1\endcsname{\expandafter\noexpand
  \csname the#3\endcsname \@thmcountersep \@thmcounter{#1}}%
\global\@namedef{#1}{\@thm{#1}{#2}{#4}}\global\@namedef{end#1}{\@endtheorem}}}
 
\def\@ynthm#1#2#3{%next line commented for brutal redefinition
%\expandafter\@ifdefinable\csname #1\endcsname
%typical #1=definition, #2=Definition, #3=cpspecial
{\@definecounter{#1}%
\expandafter\xdef\csname the#1\endcsname{\@thmcounter{#1}}%
\global\@namedef{#1}{\@thm{#1}{#2}{#3}}\global\@namedef{end#1}{\@endtheorem}}}
 
\def\@othm#1[#2]#3#4{%next line commented for brutal redefinition
%\expandafter\@ifdefinable\csname #1\endcsname
%typical #1=definition, #2=theorem, #3=Definition, #4=cpspecial
  {\global\@namedef{the#1}{\@nameuse{the#2}}%
\global\@namedef{#1}{\@thm{#2}{#3}{#4}}%
\global\@namedef{end#1}{\@endtheorem}}}
 
\def\@thm#1#2#3{\refstepcounter
    {#1}\@ifnextchar[{\@ythm{#1}{#2}{#3}}{\@xthm{#1}{#2}{#3}}}
 
\def\@xthm#1#2#3{\@begintheorem{#2}{\csname the#1\endcsname}{#3}\ignorespaces}
\def\@ythm#1#2#3[#4]{\@opargbegintheorem{#2}{\csname
       the#1\endcsname}{#4}{#3}\ignorespaces}
 
%DEFAULT VALUES
\def\@thmcounter#1{\noexpand\arabic{#1}}
\def\@begintheorem#1#2#3{\trivlist \item[\hskip \labelsep{\bf #1\ #2}]#3}
\def\@opargbegintheorem#1#2#3#4{\trivlist
      \item[\hskip \labelsep{\bf #1\ #2\ (#3)}]#4}
\def\@endtheorem{\endtrivlist}
 
%\def\@thmcountersep{}
%\newtheorem{theorem}            {Theorem}[thmcounter]{\mbox{}\it}
\def\@thmcountersep{.}
\def\globalrequirement{Global Requirement}

\newcommand\romanhelper{\hskip0.5em\mbox{}\rm}
\newtheorem{theorem}{Theorem}[section]{\mbox{}\it}
\newtheorem{lemma}     
[theorem]{Lemma}{\mbox{}\it}
\newtheorem{sublemma}  
[theorem]{Sublemma}{\mbox{}\it}
\newtheorem{corollary} 
[theorem]{Corollary}{\mbox{}\it}
\newtheorem{example}   
[theorem]{\Examplename}{\romanhelper}
\newtheorem{counterexample}   
[theorem]{Counterexample}{\romanhelper}
\newtheorem{exercise}   
[theorem]{Exercise}{\romanhelper}
\newtheorem{remark}    
[theorem]{Remark}{\romanhelper}
\newtheorem{forderung} 
[theorem]{\globalrequirement}{\mbox{}\it}
\newtheorem{requirement} 
[theorem]{Requirement}{\romanhelper}
\newtheorem{definition}
[theorem]{Definition}{\romanhelper}
\newtheorem{aufgabe}   
[theorem]{Aufgabe}{\romanhelper}
\newtheorem{specification}
[theorem]{Specification}{\romanhelper}
\newtheorem{problem}
[theorem]{Problem}{\romanhelper}
\newtheorem{axiom}
[theorem]{Axiom}{\romanhelper}
\catcode`\@=12


==> pdf.tex <==
%&latex
\newcommand\SEKImasterusepackages{
%\usepackage{times}
\input headernamesrest
\newcommand\SEKIedition{}
%%% begin xy %%%
\input xy
\xyoption{all}
%%% end xy %%%%%
}
\input body


==> specialfonts.tex <==
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Characters and Punctuation signs %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\underscore{\underline~}
\let\aefranz\ae
\let\oefranz\oe
%\newcommand\aefranz{\char"1A}%This does not work any more 
%\newcommand\oefranz{\char"1B}%as latex 2e confuses font tables!
\newcommand\ttbackslash  {{\tt\char'134}}
\newcommand\ttdoublequote{{\tt\char'042}}

\newcommand\actualpagebreaknospace{{\rm\textbar}}
\newcommand\actualpagebreak{\actualpagebreaknospace\ }
\newcommand\actualsentencepagebreak{\actualpagebreaknospace\ \ }
\newcommand\actualparpagebreak
{\getittotheright{\actualpagebreaknospace\hskip-.09em}}
\newcommand\actualpagebreakindent
{\noindent\actualpagebreaknospace\hskip-.25em\indent}
\newcommand\actualpagebreaknoindent
{\noindent\actualpagebreak}

\mathchardef\Gammaoffont="7000
\mathchardef\Gamma="0100
\mathchardef\Deltaoffont="7001
\mathchardef\Delta="0101
\mathchardef\Thetaoffont="7002
\mathchardef\Theta="0102
\mathchardef\Lambdaoffont="7003
\mathchardef\Lambda="0103
\mathchardef\Xioffont="7004
\mathchardef\Xi="0104
\mathchardef\Pioffont="7005
\mathchardef\Pi="0105
\mathchardef\Sigmaoffont="7006
\mathchardef\Sigma="0106
\mathchardef\Upsilonoffont="7007
\mathchardef\Upsilon="0107
\mathchardef\Phioffont="7008
\mathchardef\Phi="0108
\mathchardef\Psioffont="7009
\mathchardef\Psi="0109
\mathchardef\Omegaoffont="700A
\mathchardef\Omega="010A
\mathchardef\itype="017B

\catcode`\@=11

\gdef\allowhyphens{\penalty\@M \hskip\z@skip}

\gdef\set@low@box#1{\setbox\tw@\hbox{,}\setbox\z@\hbox{#1}\dimen\z@\ht\z@
     \advance\dimen\z@ -\ht\tw@
     \setbox\z@\hbox{\lower\dimen\z@ \box\z@}\ht\z@\ht\tw@ \dp\z@\dp\tw@ }
%    (this lowers the german double left quotes to the same level as the comma.)
\gdef\set@low@boxsingle#1{\setbox\tw@\hbox{\rm,}\setbox\z@\hbox{#1}\dimen\z@\ht\z@
     \advance\dimen\z@ -\ht\tw@
     \setbox\z@\hbox{\lower\dimen\z@ \box\z@}\ht\z@\ht\tw@ \dp\z@\dp\tw@ }
%    (this lowers the german single left quotes to the same level as the comma.)

\gdef\@glqq{%
\ifhmode\edef\@SF{\spacefactor\the\spacefactor}%
\else\let\@SF\empty
\fi
\CheckFamily\font\fraknomath\ifSameFamily ``\relax
\else\CheckFamily\font\swab\ifSameFamily ``\relax
\else\leavevmode\set@low@box{''}\box\z@\kern-.04em\allowhyphens\@SF\relax
\fi\fi}
\gdef\glqq{\protect\@glqq\kern+.07em}
\gdef\@grqq{%
\ifhmode\edef\@SF{\spacefactor\the\spacefactor}%
\else\let\@SF\empty 
\fi 
\CheckFamily\font\fraknomath\ifSameFamily ''\relax
\else\CheckFamily\font\swab\ifSameFamily ''\relax
\else\kern+.07em``\kern.07em\@SF\relax
\fi\fi}
\gdef\grqq{\protect\@grqq}
\gdef\@glq{{\ifhmode \edef\@SF{\spacefactor\the\spacefactor}\else
     \let\@SF\empty \fi \leavevmode
     \set@low@boxsingle{'\/}\box\z@\kern-.04em\allowhyphens\@SF\relax}}
\gdef\glq{\protect\@glq\kern+.07em}
\gdef\@grq{\ifhmode \edef\@SF{\spacefactor\the\spacefactor}\else
     \let\@SF\empty \fi \kern-.0125em`\kern.07em\@SF\relax}
\gdef\grq{\protect\@grq}

\catcode`\@=12

% Use the following two signs like ``bla bla\closequotecomma
% Do not use them like             ``bla bla\closequotecomma\
% because this produces an extra space. This cannot be
% avoided because otherwise the end-of-sentence extra-space does 
% not work prperly.
\newcommand\closequotecommanospace{''\nolinebreak\hskip-0.23em,}
\newcommand\closequotecomma      {\closequotecommanospace\         \,}
\newcommand\closequotecommasmallextraspace{\closequotecommanospace\ \,\,}
\newcommand\closequotecommaextraspace{\closequotecommanospace\   \ \,}
\newcommand\closequotefullstop   {\closequotefullstopnospace\      \,}
\newcommand\closequotefullstopextraspace   
                                 {\closequotefullstopnospace\    \ \,}
\newcommand\closequotefullstopextraextraspace   
                                 {\closequotefullstopnospace\  \ \ \,}
\newcommand\closequotefullstopcloseparentheses   
                                 {\closequotefullstopnospace)        }
\newcommand\closequotefullstopcloseparenthesesextraspace
                                 {\closequotefullstopnospace)    \ \,}
\newcommand\closequotefullstopnospace
                                 {''\nolinebreak\hskip-0.20em\@.}
\newcommand\closequotecolonnospace{''\nolinebreak\hskip-0.10em:}
\newcommand\closequotecolon      {\closequotecolonnospace\ \,}
\newcommand\closequotecolonextraspace{\closequotecolonnospace\ \ \,}
\newcommand\closequotesemicolon  {''\nolinebreak\hskip-0.06em;     \,}
\newcommand\closequotesemicolonnospace{''\nolinebreak\hskip-0.06em;}
\newcommand\closequotesemicolonextraspace  {''\nolinebreak\hskip-0.10em; \ \,}
\newcommand\closequotesemicolonsmallextraspace{\closequotesemicolonnospace\ \,\,}
\newcommand\closesinglequotecomma{'\nolinebreak\hskip-0.20em,      \,}
\newcommand\closesinglequotecommaextraspace{'\nolinebreak\hskip-0.20em, \ \,}
\newcommand\closesinglequotefullstopnospace{'\nolinebreak\hskip-0.20em\@.}
\newcommand\closesinglequotefullstop{\closesinglequotefullstopnospace\ \,}
\newcommand\closesinglequotefullstopextraspace
{\closesinglequotefullstopnospace\ \ \,}
\newcommand\grqqcommanospace      {\grqq\nolinebreak\hskip-0.25em,}
\newcommand\grqqcomma             {\grqqcommanospace\ \,}
\newcommand\grqqcommaextraspace   {\grqqcomma\ \ }
\newcommand\grqqsemicolon         {\grqq\nolinebreak\hskip-0.15em;  \,}
\newcommand\grqcomma              {\grq\nolinebreak\hskip-0.25em,   \,}
\newcommand\grqfullstop           {\grq\nolinebreak\hskip-0.25em\@. \,}
\newcommand\grqsemicolon          {\grq\nolinebreak\hskip-0.15em; \,}
\newcommand\grqqfullstop          {\grqq\nolinebreak\hskip-0.25em\@. \,}
\newcommand\grqqfullstopextraspace{\grqq\nolinebreak\hskip-0.25em\@. \ \ \,}
\newcommand\grqqfullstopnospace   {\grqq\nolinebreak\hskip-0.25em\@.}
\newcommand\commanospace          {,\nolinebreak\hskip-0.23em}
\newcommand\fullstopnospace       {\@.\nolinebreak\hskip-0.23em}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% here starts oldgerman.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Alte deutsche Schrifttypen werden verfuegbar gemacht
% Dies sind die Schrifttypen
% (goth) gothisch
% (frak) Frankfurter Fraktur
% (swab) Schwabacher
% (init) Initialen
% font kann goth,frak,swab oder init sein.

% Jeden der Fonts gibt es in der normalen Textgroesse und den naechsten 4
% Vergroesserungen
% Aufruf mit 
% \font ... text ... 
% \Font ... text ...
% \FOnt ... text ... 
% \FONt ... text ... 
% \FONT ... text ...

% Zusaetzlich gibt es die fonts noch in Groessen fuer Indizes
% als \scriptfont \scriptscriptfont und \scriptscriptscriptfont
% Als Vergroesserungsstufen wurden mag 0.912, 0.833, 0.760 (entsprechend
% 1.2 ^ -0.5, -1, -1.5) gewaehlt.


% fuer Gebrauch im Mathemodus gibt es die Kommandos mfont, mFont, etc
% Diese erhalten ein Argument, dieses wird in einer mbox in diesem
% Font gesetzt.
% font kann goth,frak oder swab sein.
% entsprechen zu oben gibt es auch die Kommandos \mscriptscriptscriptfont,
% \mscriptscriptfont und \mscriptfont.

\makeatletter
\if \@ptsize 0
   \newfont{\scriptscriptscriptgoth}{ygoth scaled 760}
   \newfont{\scriptscriptgoth}{ygoth scaled 833}
   \newfont{\scriptgoth}{ygoth scaled 912}
   \newfont{\gothnomath}{ygoth}
   \newfont{\Goth}{ygoth scaled \magstephalf}
   \newfont{\GOth}{ygoth scaled \magstep1}
   \newfont{\GOTh}{ygoth scaled \magstep2}
   \newfont{\GOTH}{ygoth scaled \magstep3}

   \newfont{\scriptscriptscriptswab}{yswab scaled 760}
   \newfont{\scriptscriptswab}{yswab scaled 833}
   \newfont{\scriptswab}{yswab scaled 912}
   \newfont{\swab}{yswab}
   \newfont{\Swab}{yswab scaled \magstephalf}
   \newfont{\SWab}{yswab scaled \magstep1}
   \newfont{\SWAb}{yswab scaled \magstep2}
   \newfont{\SWAB}{yswab scaled \magstep3}

   \newfont{\scriptscriptscriptfrak}{yfrak scaled 760}
   \newfont{\scriptscriptfrak}{yfrak scaled 833}
   \newfont{\scriptfrak}{yfrak scaled 912}
   \newfont{\fraknomath}{yfrak}
   \newfont{\Frak}{yfrak scaled \magstephalf}
   \newfont{\FRak}{yfrak scaled \magstep1}
   \newfont{\FRAk}{yfrak scaled \magstep2}
   \newfont{\FRAK}{yfrak scaled \magstep3}

   \newfont{\init}{yinit}
   \newfont{\Init}{yinit scaled \magstephalf}
   \newfont{\INit}{yinit scaled \magstep1}
   \newfont{\INIt}{yinit scaled \magstep2}
   \newfont{\INIT}{yinit scaled \magstep3}
\fi
\if \@ptsize 1
   \newfont{\scriptscriptscriptgoth}{ygoth scaled 833}
   \newfont{\scriptscriptgoth}{ygoth scaled 912}
   \newfont{\scriptgoth}{ygoth}
   \newfont{\gothnomath}{ygoth scaled \magstephalf}
   \newfont{\Goth}{ygoth scaled \magstep1}
   \newfont{\GOth}{ygoth scaled \magstep2}
   \newfont{\GOTh}{ygoth scaled \magstep3}
   \newfont{\GOTH}{ygoth scaled \magstep4}

   \newfont{\scriptscriptscriptswab}{yswab scaled 833}
   \newfont{\scriptscriptswab}{yswab scaled 912}
   \newfont{\scriptswab}{yswab}
   \newfont{\swab}{yswab scaled \magstephalf}
   \newfont{\Swab}{yswab scaled \magstep1}
   \newfont{\SWab}{yswab scaled \magstep2}
   \newfont{\SWAb}{yswab scaled \magstep3}
   \newfont{\SWAB}{yswab scaled \magstep4}

   \newfont{\scriptscriptscriptfrak}{yfrak scaled 833}
   \newfont{\scriptscriptfrak}{yfrak scaled 912}
   \newfont{\scriptfrak}{yfrak}
   \newfont{\fraknomath}{yfrak scaled \magstephalf}
   \newfont{\Frak}{yfrak scaled \magstep1}
   \newfont{\FRak}{yfrak scaled \magstep2}
   \newfont{\FRAk}{yfrak scaled \magstep3}
   \newfont{\FRAK}{yfrak scaled \magstep4}

   \newfont{\init}{yinit scaled \magstephalf}
   \newfont{\Init}{yinit scaled \magstep1}
   \newfont{\INit}{yinit scaled \magstep2}
   \newfont{\INIt}{yinit scaled \magstep3}
   \newfont{\INIT}{yinit scaled \magstep4}
\fi
\if \@ptsize 2
   \newfont{\scriptscriptscriptgoth}{ygoth scaled 912}
   \newfont{\scriptscriptgoth}{ygoth}
   \newfont{\scriptgoth}{ygoth scaled \magstephalf}
   \newfont{\gothnomath}{ygoth scaled \magstep1}
   \newfont{\Goth}{ygoth scaled \magstep2}
   \newfont{\GOth}{ygoth scaled \magstep3}
   \newfont{\GOTh}{ygoth scaled \magstep4}
   \newfont{\GOTH}{ygoth scaled \magstep5}

   \newfont{\scriptscriptscriptswab}{yswab scaled 912}
   \newfont{\scriptscriptswab}{yswab}
   \newfont{\scriptswab}{yswab scaled \magstephalf}
   \newfont{\swab}{yswab scaled \magstep1}
   \newfont{\Swab}{yswab scaled \magstep2}
   \newfont{\SWab}{yswab scaled \magstep3}
   \newfont{\SWAb}{yswab scaled \magstep4}
   \newfont{\SWAB}{yswab scaled \magstep5}

   \newfont{\scriptscriptscriptfrak}{yfrak scaled 912}
   \newfont{\scriptscriptfrak}{yfrak}
   \newfont{\scriptfrak}{yfrak scaled \magstephalf}
   \newfont{\fraknomath}{yfrak scaled \magstep1}
   \newfont{\Frak}{yfrak scaled \magstep2}
   \newfont{\FRak}{yfrak scaled \magstep3}
   \newfont{\FRAk}{yfrak scaled \magstep4}
   \newfont{\FRAK}{yfrak scaled \magstep5}

   \newfont{\init}{yinit scaled \magstep1}
   \newfont{\Init}{yinit scaled \magstep2}
   \newfont{\INit}{yinit scaled \magstep3}
   \newfont{\INIt}{yinit scaled \magstep4}
   \newfont{\INIT}{yinit scaled \magstep5}
\fi
\newcommand{\mscriptscriptscriptgoth}[1]{\mbox{\scriptscriptscriptgoth#1}}
\newcommand{\mscriptscriptgoth}[1]{\mbox{\scriptscriptgoth#1}}
\newcommand{\mscriptgoth}[1]{\mbox{\scriptgoth#1}}
\newcommand{\mgoth}[1]{\mbox{\gothnomath#1}}
\newcommand{\mGoth}[1]{\mbox{\Goth#1}}
\newcommand{\mGOth}[1]{\mbox{\GOth#1}}
\newcommand{\mGOTh}[1]{\mbox{\GOTh#1}}
\newcommand{\mGOTH}[1]{\mbox{\GOTH#1}}

\newcommand{\mscriptscriptscriptswab}[1]{\mbox{\scriptscriptscriptswab#1}}
\newcommand{\mscriptscriptswab}[1]{\mbox{\scriptscriptswab#1}}
\newcommand{\mscriptswab}[1]{\mbox{\scriptswab#1}}
\newcommand{\mswab}[1]{\mbox{\swab#1}}
\newcommand{\mSwab}[1]{\mbox{\Swab#1}}
\newcommand{\mSWab}[1]{\mbox{\Swab#1}}
\newcommand{\mSWAb}[1]{\mbox{\Swab#1}}
\newcommand{\mSWAB}[1]{\mbox{\SWAB#1}}

\newcommand{\mscriptscriptscriptfrak}[1]{\mbox{\scriptscriptscriptfrak#1}}
\newcommand{\mscriptscriptfrak}[1]{\mbox{\scriptscriptfrak#1}}
\newcommand{\mscriptfrak}[1]{\mbox{\scriptfrak#1}}
\newcommand{\mfrak}[1]{\mbox{\fraknomath#1}}
\newcommand{\mFrak}[1]{\mbox{\Frak#1}}
\newcommand{\mFRak}[1]{\mbox{\Frak#1}}
\newcommand{\mFRAk}[1]{\mbox{\Frak#1}}
\newcommand{\mFRAK}[1]{\mbox{\FRAK#1}}
\makeatother
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% this is the end of oldgerman.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newif\ifSameFamily
\def\CheckFamily#1#2{\GetFamilyName{#1}\ArgOne
        \GetFamilyName{#2}\ArgTwo
        \ifx\ArgOne\ArgTwo\SameFamilytrue\else\SameFamilyfalse\fi}
\def\GetFamilyName#1{\edef\Tempa{#1}\def\Tempb{#1}\ifx\Tempa\Tempb
        \edef\Tempa{\fontname#1}\fi
        \edef\Tempa{\Tempa\space}%
        \expandafter\iGetFamilyName\Tempa\\}
\def\iGetFamilyName#1 #2\\#3{\def#3{#1}}
\def\DefFontName#1#2{{\escapechar-1\expandafter\expandafter\expandafter
        \iDefFontName\expandafter{\csname#2\endcsname}%
        \xdef#1{\expandafter\string\Tempa}}}
\def\iDefFontName{\def\Tempa}

%The usage is: \CheckFamily<font1><font2>\ifSameFamily ... \else ... \fi
%where <font1> and <font2> are either \font or font-id like
%\tenrm.  For example;
%
%        \CheckFamily\font\mymightyfont\ifSameFamily ... \else ... \fi
%
%will do what you want providing \mymightyfont has been
%loaded.  Otherwise, you must define font name beforehand by
%\DefFontName like;
%
%        \DefFontName\mymightyfont{mmf10}
%
%where "mmf10" is the family name of \mymightyfont.  This
%trick is required because \fontname produces a string of
%\catcode=12 (other) characters.
%
%Please note that;
%
%        \def\ifSame#1#2{\CheckFamily#1#2\ifSameFamily}
%                :
%        \ifSame\font\mymightyfont ... \else ... \fi
%
%will cause some trouble if "\ifSame ... \fi" is in the
%true/false part of another \ifXXX.  That is, when ourter
%\ifXXX causes "\ifSame" to be skipped, TeX won't think
%\ifSame is a kind of \if and will confuse \if-\fi
%construction.

\newcommand\unprotectedae
{\CheckFamily\font\fraknomath\ifSameFamily *a\else
 \CheckFamily\font\swab\ifSameFamily\char'212\else\"a\fi\fi}
\newcommand\unprotectedoe
{\CheckFamily\font\fraknomath\ifSameFamily 
*o\else\CheckFamily\font\swab\ifSameFamily\char'232\else\"o\fi\fi}
\newcommand\unprotectedue
{\CheckFamily\font\fraknomath\ifSameFamily 
*u\else\CheckFamily\font\swab\ifSameFamily\char'237\else\"u\fi\fi}
\newcommand\unprotectedAe
{\CheckFamily\font\fraknomath\ifSameFamily 
Ae\else\CheckFamily\font\swab\ifSameFamily Ae\else\"A\fi\fi}
\newcommand\unprotectedOe
{\CheckFamily\font\fraknomath\ifSameFamily 
Oe\else\CheckFamily\font\swab\ifSameFamily Oe\else\"O\fi\fi}
\newcommand\unprotectedUe
{\CheckFamily\font\fraknomath\ifSameFamily 
Ue\else\CheckFamily\font\swab\ifSameFamily Ue\else\"U\fi\fi}
\DefFontName\eccclarge{eccc1200}
\DefFontName\eccc{eccc1000}
\DefFontName\ecccsmall{eccc0900}
\DefFontName\ecccfootnotesize{eccc0800}
\newcommand\unprotectedsz
{\CheckFamily\font\fraknomath\ifSameFamily\char'032\else
 \CheckFamily\font\swab\ifSameFamily\char'032\else
 \CheckFamily\font\eccclarge\ifSameFamily sz\else
 \CheckFamily\font\eccc\ifSameFamily sz\else
 \CheckFamily\font\ecccsmall\ifSameFamily sz\else
 \CheckFamily\font\ecccfootnotesize\ifSameFamily sz\else
 \ss\fi\fi\fi\fi\fi\fi}
\newcommand\unprotectedes
{\CheckFamily\font\fraknomath\ifSameFamily\char'215\else
\CheckFamily\font\swab\ifSameFamily\char'215\else  
s\fi\fi}
% \newcommand\unprotectedses
% {\CheckFamily\font\fraknomath\ifSameFamily\char'032\else
% \CheckFamily\font\swab\ifSameFamily\char'032\else ss\fi\fi}
\newcommand\unprotectedses
{\CheckFamily\font\fraknomath\ifSameFamily 
s\nolinebreak\hskip-.055em\char'215\else
\CheckFamily\font\swab\ifSameFamily s\char'215\else ss\fi\fi}
\newcommand\unprotectedesi
{\CheckFamily\font\fraknomath\ifSameFamily\char'215\else
\CheckFamily\font\swab\ifSameFamily\char'215\else  
\mbox{s\hskip.04em}\fi\fi
\-\ignorespaces}
\newcommand\unprotectedesid
{\CheckFamily\font\fraknomath\ifSameFamily\char'215\-\hskip.055em d\else
\CheckFamily\font\swab\ifSameFamily\char'215\-d\else  
\mbox{s\hskip.055em}\-d\fi\fi
\ignorespaces}
\newcommand\unprotectedesis
{\CheckFamily\font\fraknomath\ifSameFamily\char'215\-\hskip.055em s\else
\CheckFamily\font\swab\ifSameFamily\char'215\-s\else  
\mbox{s\hskip.055em}\-s\fi\fi
\ignorespaces}
\newcommand\unprotectedefi
{\CheckFamily\font\fraknomath\ifSameFamily f\else
\CheckFamily\font\swab\ifSameFamily f\else  
\mbox{f\hskip.055em}\fi\fi
\-\ignorespaces}
\newcommand\unprotectedsesi
{\CheckFamily\font\fraknomath\ifSameFamily 
s\nolinebreak\hskip-.055em\char'215\else
\CheckFamily\font\swab\ifSameFamily s\char'215\else\mbox{ss\hskip.045em}\fi\fi
\-\ignorespaces}
\newcommand\unprotectedmyparagraphsymbol
{\CheckFamily\font\fraknomath\ifSameFamily 
\char'244\else\CheckFamily\font\swab\ifSameFamily
\char'244\else\S\fi\fi}
\newcommand\unprotectedzwithdot
{\CheckFamily\font\fraknomath\ifSameFamily 
\accent'137z\else\CheckFamily\font\swab\ifSameFamily z\else\.z\fi\fi}
\newcommand\unprotectedewithtrema
{\-\CheckFamily\font\fraknomath\ifSameFamily 
 "e\else\CheckFamily\font\swab\ifSameFamily "e\else\"e\fi\fi}
\newcommand\unprotectediwithtrema
{\-\CheckFamily\font\fraknomath\ifSameFamily 
 "\i\else\CheckFamily\font\swab\ifSameFamily "\i\else\"\i\fi\fi}

\renewcommand\ae{\protect\unprotectedae}
\renewcommand\oe{\protect\unprotectedoe}
\newcommand\ue  {\protect\unprotectedue}
\newcommand\Ae  {\protect\unprotectedAe}
\newcommand\Oe  {\protect\unprotectedOe}
\newcommand\Ue  {\protect\unprotectedUe}
\newcommand\sz  {\protect\unprotectedsz}
\newcommand\es  {\protect\unprotectedes}
\newcommand\ses {\protect\unprotectedses}
\newcommand\esi {\protect\unprotectedesi}  %wortinterne Version
\newcommand\esid{\protect\unprotectedesid}  %wortinterne Version
\newcommand\esis{\protect\unprotectedesis}  %wortinterne Version
\newcommand\efi {\protect\unprotectedefi}  %wortinterne Version
\newcommand\sesi{\protect\unprotectedsesi} %wortinterne Version
\newcommand\fbi {\discretionary{f-} {b}{f\mbox {\hskip.07em}b}} 
\newcommand\fdi {\discretionary{f-} {d}{f\mbox {\hskip.09em}d}} 
\newcommand\ffi {\discretionary{f-} {f}{f\mbox {\hskip.08em}f}} 
\newcommand\ffli{\discretionary{ff-}{l}{ff\mbox{\hskip.09em}l}} 
\newcommand\fgi {\discretionary{f-} {g}{f\mbox {\hskip.05em}g}} 
\newcommand\fki {\discretionary{f-} {k}{f\mbox {\hskip.11em}k}} 
\newcommand\fli {\discretionary{f-} {l}{f\mbox {\hskip.09em}l}} 
\newcommand\fni {\discretionary{f-} {n}{f\mbox {\hskip.07em}n}} 
\newcommand\fri {\discretionary{f-} {r}{f\mbox {\hskip.09em}r}} 
\newcommand\fsi {\discretionary{f-} {s}{f\mbox {\hskip.08em}s}} 
\newcommand\fti {\discretionary{f-} {t}{f\mbox {\hskip.09em}t}} 
\newcommand\fwi {\discretionary{f-} {w}{f\mbox {\hskip.09em}w}} 
\newcommand\gfi {\discretionary{g-} {f}{g\mbox {\hskip.09em}f}} 
\newcommand\lli {\discretionary{l-} {l}{l\mbox {\hskip.07em}l}} 
\newcommand\tzi {\discretionary{t-} {z}{t\mbox {\hskip.03em}z}} 
\newcommand\myparagraphsymbol{\protect\unprotectedmyparagraphsymbol}
\newcommand\zwithdot{\protect\unprotectedzwithdot}
\newcommand\ewithtrema{\protect\unprotectedewithtrema}
\newcommand\iwithtrema{\protect\unprotectediwithtrema}
% \ses\ stands for ss in the form of s ending-s (\es)
% In Fraktur and Schwabacher it prints as s\es, otherwise as ss.
% Duden recommends s\es in Fraktur and Biblia Germanica does it, too.
% \sz\ may be more convenient, however. 



==> xy.tex <==
%% xy.tex from $Id: xy.doc,v 3.7 1999/02/16 15:12:50 krisrose Exp $
%%
%% Basic Xy-pictures: Xy-pic bootstrap and kernel macros.
%% Copyright (c) 1991-1999 Kristoffer H. Rose <krisrose@ens-lyon.fr>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% Copyright (c) 1991-1999 Kristoffer H. Rose <krisrose@ens-lyon.fr>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined\else\message{not reloaded}\endinput\fi
\let\xyloaded=\relax
\message{Bootstrap\string'ing\string:}
{\catcode96 12\catcode`\#6\catcode`\.12\catcode`\:12\catcode`\'12\catcode`\@11
\ifx\xywarnifdefined\undefined\else \immediate\write16{}%
 \immediate\write16{Xy-pic Warning: \string\xywarnifdefined\space redefined.}%
 \immediate\write16{}\fi
\gdef\xywarnifdefined#1{\ifx#1\undefined\else \immediate\write16{}%
 \immediate\write16{Xy-pic Warning: `\string#1' redefined.}%
 \immediate\write16{}\fi}
\xywarnifdefined\xydef@ \gdef\xydef@#1{\xywarnifdefined#1\gdef#1}
\xywarnifdefined\xylet@ \gdef\xylet@#1{\xywarnifdefined#1\global\let#1}
\xywarnifdefined\xynew@
 \gdef\xynew@#1#2{\xywarnifdefined#2\csname new#1\endcsname#2}}
\message{catcodes\string,}
\xywarnifdefined\xyuncatcodes
\xywarnifdefined\xyreuncatcodes \def\xyreuncatcodes{\edef\xyuncatcodes{%
 \catcode92 0 \catcode123 1 \catcode125 2 \catcode37 14
 \catcode 9 \the\catcode 9 \catcode10 \the\catcode10 \catcode12 \the\catcode12
 \catcode35 \the\catcode35 \catcode36 \the\catcode36 \catcode38 \the\catcode38 
 \catcode43 \the\catcode43 \catcode45 \the\catcode45 \catcode46 \the\catcode46 
 \catcode47 \the\catcode47 
 \catcode60 \the\catcode60 \catcode61 \the\catcode61 \catcode62 \the\catcode62 
 \catcode64 \the\catcode64 \catcode96 \the\catcode96
 \newlinechar \the\newlinechar \endlinechar \the\endlinechar }}
\xyreuncatcodes
\xywarnifdefined\xycatcodes \def\xycatcodes{%
 \catcode 9 10
 \catcode 35 6 \catcode 36 3 \catcode 38 4
 \catcode 43 12 \catcode 45 12 \catcode 46 12 \catcode 47 12
 \catcode 60 12 \catcode 61 12 \catcode 62 12
 \catcode 64 11 \catcode 96 12 }
\xycatcodes
\message{docmode,}
{\catcode`\|0 \xywarnifdefined|DOCMODE
\gdef|DOCMODE#1{\ifx(#1\relax \xycatcodes \expandafter\ignorespaces
 \else \skipspecials@ \expandafter\docm@\fi}%
\xywarnifdefined\skipspecials@
\gdef\skipspecials@{%
 \catcode`\\12 \catcode`\{12 \catcode`\}12 \catcode`\#12 \catcode`\%12
 \catcode`\^^L12 \endlinechar`\^^J }%
\catcode`\/=12 \lccode`\/`\\%
\lccode`\D`\D \lccode`\O`\O \lccode`\C`\C \lccode`\M`\M \lccode`\E`\E
\lowercase{%
\xywarnifdefined\docm@ \gdef\docm@{\docm@i}%
\xywarnifdefined\docm@i \gdef\docm@i#1^^J{\docm@ii#1/DOCMODE\docm@iii}%
\xywarnifdefined\docm@ii
 \gdef\docm@ii#1/DOCMODE{\def\next@{#1}\futurelet\next\docm@iii}%
\xywarnifdefined\docm@iii \gdef\docm@iii#1\docm@iii{%
 \ifx\next\docm@iii \let\next\next@ \docecho@ \let\next@\docm@
 \else\ifx\next@\empty \let\next@\docfinish@
 \else \edef\next@{\noexpand\docm@iv\next@/DOCMODE#1\noexpand\docm@iv}%
 \fi\fi \next@}%
\xywarnifdefined\docm@iv
 \gdef\docm@iv#1/DOCMODE\docm@iv{\def\next{#1}\docecho@ \docm@}}%
\xywarnifdefined\docecho@ \global\let\docecho@\relax
\xywarnifdefined\docfinish@ \gdef\docfinish@{\xyuncatcodes|DOCMODE\next}}
\xydef@\xydefcsname@#1{\DN@{#1}\DNii@##1{%
 \ifx ##1\relax\else \xywarning@{\string`\string##1\string' redefined}\fi
 \def##1}%
 \expandafter\nextii@\csname\codeof\next@\endcsname}
\xydef@\xyletcsnamecsname@#1#2{\def\1{#1}\def\2{#2}\DN@##1##2{%
 \ifx ##1\relax\else \xywarning@{`\string##1\string' redefined}\fi
 \let##1=##2}%
 \expandafter\expandafter\expandafter\next@
 \expandafter\csname\expandafter\codeof\expandafter\1\expandafter\endcsname
 \csname\codeof\2\endcsname}
\xywarnifdefined\codeof
\xywarnifdefined\codeof@
{\catcode`\:=12
 \gdef\codeof#1{\expandafter\codeof@\meaning#1<-:}
 \gdef\codeof@#1:->#2<-:{#2}}
\xywarnifdefined\addAT@
\xywarnifdefined\addHASH@
\xywarnifdefined\addDOLL@
\xywarnifdefined\addAND@
\xywarnifdefined\addRQ@
\xywarnifdefined\addPLUS@
\xywarnifdefined\addDASH@
\xywarnifdefined\addDOT@
\xywarnifdefined\addLT@
\xywarnifdefined\addEQ@
\xywarnifdefined\addGT@
\xywarnifdefined\addLQ@
\xydef@\xymakeADD@#1#2 #3 {\ifnum\catcode#3=6 \def#1##1{##1#2#2}%
 \else \def#1##1{##1#2}\fi}
\xydef@\xyrecat@{\xymakeADD@\addAT@}
\xydef@\xyrecat{\xyrecat@}
\xydef@\xyresetcatcodes{\def\xyrecat{\xyrecat@}\xyreuncatcodes
 \input xyrecat \relax \xyuncatcodes}
\xyuncatcodes \xyresetcatcodes \xycatcodes
\xydef@\testAND@{{\aftergroup\ifx 
 \addAND@\ifx\next\addFalse@\else\addTrue@\fi}}
\xydef@\addFalse@{\aftergroup\iffalse}
\xydef@\addTrue@{\aftergroup\iftrue}
\input xyidioms
\xydef@\stripRCS$#1${\stripRCS@#1: @@ @@@}
\xydef@\stripRCS@#1: #2@ #3@@@{%
 \ifx @#2\string?\else\ifx :#2\else\stripRCS@@#2\fi\fi}
\xydef@\stripRCS@@#1 #2: @{#1}
\edef\next{\stripRCS$Revision: 3.7 $}
\xylet@\xyversion=\next
\edef\next{\stripRCS$Date: 1999/02/16 15:12:50 $}
\xylet@\xydate=\next
\xydef@\Xygreet@{%
 \W@{}%
 \W@{ Xy-pic version \xyversion\space<\xydate>}%
 \W@{ Copyright (c) 1991-1998 by Kristoffer H. Rose <krisrose@ens-lyon.fr>}%
 \W@{ Xy-pic is free software: see the User\string's Guide for details.}%
 \W@{}}
\Xygreet@
\expandafter\everyjob\expandafter{\the\everyjob\Xygreet@}
\message{Loading kernel:}
\xydef@\Xy{\leavevmode
 \hbox{\kern-.1em X\kern-.3em\lower.4ex\hbox{Y\kern-.15em}}}
\message{messages;}
\xywarnifdefined\thelineno@
\ifx\inputlineno\undefined \edef\thelineno@{\string?}
\else \def\thelineno@{\the\inputlineno}\fi
\xydef@\xytracelineno@{ \string[\jobname:\thelineno@\string]}
\xydef@\xywarning@#1{{\newlinechar=10
 \W@{}\W@{Xy-pic Warning: #1\xytracelineno@.}\W@{}}}
\xydef@\xyerror@#1#2{\if\inxy@\xy@{ERROR #1}{}\fi
 {\def\2{#2}\newlinechar=10
 \ifx\2\empty \errhelp{See the Xy-pic manual for further information.}%
 \else \errhelp{#2}\fi
 \errmessage{Xy-pic error: #1}}}
\xydef@\xybug@#1{{\newlinechar=10
 \errhelp{This is a bug in Xy-pic and should not happen!^^J%
If it did then please send a bug report with the offending Xy-pic code^^J%
to the author of Xy-pic, krisrose@ens-lyon.fr.}%
 \errmessage{Xy-pic BUG: #1 -- notify krisrose@ens-lyon.fr.}}}
\message{fonts;}
\xydef@\xyfont@#1{\ifx#1\undefined \DN@{\global\font#1}\expandafter\next@
 \else \xywarning@{Using previously loaded \string#1\space font}\fi}
\xyfont@\xydashfont=xydash10
\xydef@\xydashl@{\fontdimen6\xydashfont}
\xydef@\xydashh@{\fontdimen5\xydashfont}
\xydef@\xydashw@{\fontdimen8\xydashfont}
\xyfont@\xyatipfont=xyatip10
\xyfont@\xybtipfont=xybtip10
\xyfont@\xybsqlfont=xybsql10
\xydef@\xybsqll@{\fontdimen6\xybsqlfont}
\xydef@\xybsqlh@{\fontdimen5\xybsqlfont}
\xydef@\xybsqlw@{\fontdimen8\xybsqlfont}
\xyfont@\xycircfont=xycirc10
\message{allocations:}
\message{state,}
\xynew@{dimen}\X@c
\xynew@{dimen}\Y@c
\xynew@{dimen}\U@c
\xynew@{dimen}\D@c
\xynew@{dimen}\L@c
\xynew@{dimen}\R@c
\xynew@{toks}\Edge@c
\xynew@{dimen}\X@p
\xynew@{dimen}\Y@p
\xynew@{dimen}\U@p
\xynew@{dimen}\D@p
\xynew@{dimen}\L@p
\xynew@{dimen}\R@p
\xynew@{toks}\Edge@p
\xynew@{dimen}\X@origin \X@origin=\z@
\xynew@{dimen}\Y@origin \X@origin=\z@
\xynew@{dimen}\X@xbase \X@xbase=1mm
\xynew@{dimen}\Y@xbase \Y@xbase=\z@
\xynew@{dimen}\X@ybase \X@ybase=\z@
\xynew@{dimen}\Y@ybase \Y@ybase=1mm
\xynew@{dimen}\X@min
\xynew@{dimen}\Y@min
\xynew@{dimen}\X@max
\xynew@{dimen}\Y@max
\xynew@{box}\lastobjectbox@
\xynew@{box}\zerodotbox@
\setbox\zerodotbox@=\hbox{\dimen@=.5\xydashw@
 \kern-\dimen@ \vrule width\xydashw@ height\dimen@ depth\dimen@}
\wd\zerodotbox@=\z@ \ht\zerodotbox@=\z@ \dp\zerodotbox@=\z@
\xynew@{dimen}\almostz@ \almostz@=50sp
\xydef@\zz@#1{\ifdim#1<\z@-\fi#1<\almostz@\relax}
\xynew@{if}\iftmp@
\message{direction,}
\xynew@{dimen}\d@X
\xynew@{dimen}\d@Y
\xydef@\sd@X{}
\xydef@\sd@Y{}
\xynew@{count}\K@ \K@=1024
\xynew@{count}\KK@ \KK@=32
\xynew@{count}\Direction
\xynew@{dimen}\K@dXdY
\xynew@{dimen}\K@dYdX
\xydef@\cosDirection{}
\xydef@\sinDirection{}
\xywarnifdefined\DirectionChar
\xywarnifdefined\SemiDirectionChar
\xynew@{read}\xyread@
\xynew@{write}\xywrite@
\xynew@{count}\csp@
\xynew@{dimen}\quotPTK@
\message{utility macros;}
\xydef@\addtotoks@#1{\toks@=\expandafter{\the\toks@#1}}
\xydef@\xyinputorelse@#1#2{%
 \expandafter\let\expandafter\next@\csname#1loaded\endcsname
 \ifx\next@\empty \else
 \DN@{\xyinputorelse@@{#1}{\xyinputorelse@@{#1.doc}{#2}}}%
 \fi \next@}
\xydef@\xyinputorelse@@#1#2{\openin\xyread@=#1
 \ifeof\xyread@ \DN@{#2}\else \DN@{\closein\xyread@\input#1 }\fi \next@}
\global\csp@=\z@
\xydef@\enter@#1{\global\advance\csp@\@ne
 \expandafter\xdef\csname cs@\number\csp@\endcsname{#1}\ignorespaces}
\xydef@\nter@#1{\global\advance\csp@\@ne
 \expandafter\gdef\csname cs@\number\csp@\endcsname{#1}\ignorespaces}
\xydef@\dontleave@{\csname cs@\number\csp@\endcsname}
\xydef@\unenter@{\global\advance\csp@\m@ne}
\xydef@\leave@{\expandafter\unenter@\csname cs@\number\csp@\endcsname}
\quotPTK@=\p@ \divide\quotPTK@\K@
\xylet@\quotsign@@=\empty
\xywarnifdefined\removePT@
{\catcode`p=12 \catcode`t=12 \gdef\removePT@#1pt{#1}}
\xydef@\quotient@#1#2#3{\A@=#2\relax \B@=#3\relax
 \ifdim\A@<\z@\def\quotsign@@{-}\else\def\quotsign@@{+}\fi
 \ifdim\quotsign@@\A@<15pt \multiply\A@\K@
 \else\ifdim\quotsign@@\A@<511pt \multiply\A@\KK@
 \advance\B@\ifdim\B@<\z@-\fi 16sp \divide\B@\KK@
 \else
 \advance\B@\ifdim\B@<\z@-\fi 512sp \divide\B@\K@
 \fi\fi
 \ifdim\ifdim\B@<\z@-\fi\B@<\quotPTK@ \xywarning@{division overflow}%
 \else \advance\A@.5\B@ \divide\A@\B@ \fi
 \multiply\A@\quotPTK@ \edef#1{\expandafter\removePT@\the\A@}}
\xydef@\quotient@@#1#2#3{\A@=#2\relax \B@=#3\relax \multiply\A@\KK@
 \advance\B@\ifdim\B@<\z@-\fi 128sp \divide\B@\KK@ \divide\B@ 8
 \ifdim\B@=\z@\else \advance\A@.5\B@ \divide\A@\B@ \fi
 \B@=.125\quotPTK@ \multiply\A@\B@ \edef#1{\expandafter\removePT@\the\A@}}
\xydef@\loop@#1\repeat@{\def\body@{#1}\iterate@}\xylet@\repeat@=\fi
\xydef@\iterate@{\body@\expandafter\iterate@\else\fi}
\xydef@\xyinitial@#1#2{\DN@{#1}%
 \xyerror@{command used out of context: \codeof\next@}{}}
\xylet@\xy@=\xyinitial@
\xylet@\oxy@=\xy@
\xydef@\change@oxy@#1{\let\oxy@=#1\relax
}
\xydef@\inxy@{T\ifx\xy@\xyinitial@ F\else T\fi}
\xydef@\xyxy@@ix@{\begingroup
 \xyuncatcodes\afterassignment\endgroup\global\toks9=}
\xydef@\xy@@{\xy@{}}
\xydef@\plainxy@{\let\xy@=\xyxy@ \change@oxy@\xy@ \let\xy@@ix@=\xyxy@@ix@}
\message{pictures: \string\xy,}
\xydef@\xy{\ifmmode\expandafter\xymath@\else\expandafter\xynomath@\fi}
\xydef@\xymath@{\hbox\bgroup \dimen@=\the\fontdimen22\textfont\tw@ \xyinside@}
\xydef@\xynomath@{\hbox\bgroup \dimen@=\z@ \xyinside@}
\xydef@\xyinside@{%
 \saveXyStyle@ \aftergroup\xycheck@end
 \setboxz@h\bgroup
 \plainxy@
 \X@c=\z@ \Y@c=\z@ \czeroEdge@
 \X@p=\z@ \Y@p=\z@ \U@p=\z@ \D@p=\z@ \L@p=\z@ \R@p=\z@ \Edge@p={\zeroEdge}%
 \X@min=\hsize \X@max=-\hsize \Y@min=\hsize \Y@max=-\hsize
 \mathsurround=\z@
 \expandafter\POS\everyxy@@}
\xydef@\czeroEdge@{\U@c=\z@ \D@c=\U@c \L@c=\U@c \R@c=\U@c \Edge@c={\zeroEdge}}
\xydef@\xyxy@#1#2{#2}
\xywarnifdefined\everyxy
\expandafter\def\addEQ@\everyxy#1{\def\everyxy@@{#1}\ignorespaces}
\xylet@\everyxy@@=\empty
\xydef@\endxy{\if\inxy@\else\xyerror@{Unexpected \string\endxy}{}\fi
 \relax
 \dimen@=\Y@max \advance\dimen@-\Y@min
 \ifdim\dimen@<\z@ \dimen@=\z@ \Y@min=\z@ \Y@max=\z@ \fi
 \dimen@=\X@max \advance\dimen@-\X@min
 \ifdim\dimen@<\z@ \dimen@=\z@ \X@min=\z@ \X@max=\z@ \fi
 \edef\tmp@{\egroup
 \setboxz@h{\kern-\the\X@min\boxz@}%
 \ht\z@=\the\Y@max \dp\z@=-\the\Y@min \wdz@=\the\dimen@
 \noexpand\maybeunraise@ \raise\dimen@\boxz@
 \noexpand\recoverXyStyle@ \egroup \noexpand\xy@end
 \U@c=\the\Y@max \D@c=-\the\Y@min \L@c=-\the\X@min \R@c=\the\X@max}\tmp@}
\xydef@\maybeunraise@{\if\inxy@\else \dimen@ii=\dp\z@
 \ifdim\dimen@ii<\z@ \advance\dimen@\dimen@ii \fi\fi}
\xydef@\xycheck@end{\xyFN@\xycheck@end@}
\xydef@\xycheck@end@{\ifx\next\xy@end\DN@\xy@end{}\else\DN@{\xy@end}\fi\next@}
\xydef@\xy@end{%
 \xyerror@{An \string\xy\space environment is not closed correctly.}%
 {I expected \string\endxy. You probably have an umatched {} grouping.}}
\message{positions,}
\xydef@\POS{\afterPOS{}}
\xydef@\afterPOS#1{%
 \DN@##1{\def\afterPOS@{\def\afterPOS@{##1}#1}}%
 \expandafter\next@\expandafter{\afterPOS@}%
 \afterCOORD{\xyFN@\POS@}}
\xylet@\afterPOS@=\empty
\xydef@\afterCOORD#1{%
 \DN@##1{\def\afterCOORD@{\def\afterCOORD@{##1}#1}}%
 \expandafter\next@\expandafter{\afterCOORD@}%
 \afterVECTORorEMPTY{\xy@@\czeroEdge@ \afterCOORD@}{\xyFN@\COORD@}}
\xylet@\afterCOORD@=\empty
\xydef@\afterVECTORorEMPTY#1#2{%
 \DN@##1{\def\afterVECTOR@{\def\afterVECTOR@{##1}%
 \ifVECTORempty@\DN@{#2}\else\DN@{#1}\fi \next@}}%
 \expandafter\next@\expandafter{\afterVECTOR@}%
 \xyFN@\VECTOR@}
\xynew@{if}\ifVECTORempty@
\xylet@\afterVECTOR@=\empty
\xydef@\xyVECTOR@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\VECTOR@}%
 \else \ifcat A\noexpand\next \let\next@=\VECTOR@letter
 \else \let\next@=\VECTOR@other \fi\fi \next@}
\xylet@\VECTOR@=\xyVECTOR@
\def\notrelaxorelse@#1#2{\ifx#1\relax \expandafter#2\else\expandafter#1\fi}
\xydef@\VECTOR@letter{%
 \ifx a\next \expandafter\VECTOR@a \else \expandafter\CORNER@ \fi}
\xydef@\VECTOR@a a(#1){\xy@{a(#1)}{\vfromcartesianangle@{#1}}%
 \VECTORempty@false \afterVECTOR@}
\xydef@\CORNER@{%
 \xy@{}{\A@=-.5\L@c \advance\A@.5\R@c \B@=-.5\D@c \advance\B@.5\U@c
 \let\nextii@=\zeroit@}%
 \VECTORempty@true\CORNER@i}
\xydef@\zeroit@#1{#1=\z@}
\xydef@\CORNER@i{%
 \ifx D\next \DN@ D{\xy@{D}{\Y@c=-\D@c \nextii@\X@c \B@=\Y@c}\CORNER@ii}%
 \else\ifx U\next \DN@ U{\xy@{U}{\Y@c= \U@c \nextii@\X@c \B@=\Y@c}\CORNER@ii}%
 \else\ifx L\next \DN@ L{\xy@{L}{\X@c=-\L@c \nextii@\Y@c \A@=\X@c}\CORNER@ii}%
 \else\ifx R\next \DN@ R{\xy@{R}{\X@c= \R@c \nextii@\Y@c \A@=\X@c}\CORNER@ii}%
 \else\ifx C\next \DN@ C{\xy@{C}{\X@c= \A@ \Y@c= \B@}\CORNER@ii}%
 \else\ifx E\next \DN@ E{\xy@{E}{%
 \A@=\X@c \B@=\Y@c \the\Edge@c\z@ \advance\X@c-\A@ \advance\Y@c-\B@}%
 \CORNER@ii}%
 \else\ifx P\next \DN@ P{\xy@{P}{%
 \A@=\X@c \B@=\Y@c \the\Edge@c\thr@@ \advance\X@c-\A@ \advance\Y@c-\B@}%
 \CORNER@ii}%
 \else\ifx (\next
 \DN@(##1){\xy@{(##1)}{\X@c=##1\X@c \Y@c=##1\Y@c}\afterVECTOR@}%
 \else \let\next@=\afterVECTOR@
 \fi\fi\fi\fi\fi\fi\fi\fi \next@}
\xydef@\CORNER@ii{\xy@@{\let\nextii@=\eat@}%
 \VECTORempty@false \xyFN@\CORNER@i}
\xydef@\VECTOR@other{%
 \addLT@\ifx \next
 \addGT@{\addLT@\DN@##1}{\xy@{<##1>}{\vfromabsolute@{##1}}%
 \VECTORempty@false\afterVECTOR@}%
 \else\ifx (\next
 \DN@({\xyFN@\VECTOR@other@open}%
 \else\ifx /\next
 \DN@/##1/{\xy@@ix@{{##1}}%
 \xy@{/##1/}{\expandafter\vfromslide@\the\toks9 }%
 \VECTORempty@false\afterVECTOR@}%
 \else\ifx 0\next
 \DN@ 0{\xy@{0}{\X@c=\z@ \Y@c=\z@}\VECTORempty@false\afterVECTOR@}%
 \else
 \DN@{\VECTORempty@true\afterVECTOR@}%
 \fi\fi\fi\fi \next@}
\xydef@\VECTOR@other@open{%
 \ifx *\next \DN@{\VECTORempty@true \xyFN@\afterVECTOR@(}%
 \else
 \DN@##1){\xy@{(##1)}{\vfromcartesian@{##1}}\VECTORempty@false\afterVECTOR@}%
 \fi \next@}
\xydef@\xyCOORD@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\COORD@}%
 \else \ifcat A\noexpand\next \let\next@=\xyCOORD@letter
 \else \let\next@=\xyCOORD@other \fi\fi \next@}
\xylet@\COORD@=\xyCOORD@
\xydef@\xyCOORD@letter{%
 \ifx c\next
 \DN@ c{\xy@{c}{}\afterCOORD@}%
 \else\ifx p\next
 \DN@ p{\xy@{p}\cfromp@ \afterCOORD@}%
 \else\ifx x\next
 \DN@ x{\xy@{x}{\R@c=\X@xbase \U@c=\Y@xbase \intersect@}\afterCOORD@}%
 \else\ifx y\next
 \DN@ y{\xy@{y}{\R@c=\X@ybase \U@c=\Y@ybase \intersect@}\afterCOORD@}%
 \else\ifx s\next
 \DN@ s##1{\xy@{s{##1}}{\cfroms@{##1}}\afterCOORD@}%
 \else \let\next@=\afterCOORD@ \fi\fi\fi\fi\fi \next@}
\xydef@\xyCOORD@other{%
 \ifx "\next
 \DN@"##1"{\xy@{"##1"}{\cfromid@{##1}}\afterCOORD@}%
 \else\ifx \bgroup\next
 \DN@##1{\xy@{{##1}}{\enter@{\pfromthep@\basefromthebase@}}%
 \silencexy@ \POS##1\relax \unsilencexy@ \xy@@\leave@ \afterCOORD@}%
 \else\ifx (\next
 \DN@({\xyFN@\xyCOORD@other@open}%
 \else \let\next@=\afterCOORD@ \fi\fi\fi \next@}
\xynew@{if}\ifsilentxy@
\xydef@\silencexy@{%
 \ifsilentxy@ \nter@{}%
 \else \nter@{\silentxy@false \let\xy@=\unsilent@@xy@}
 \silentxy@true \let\unsilent@@xy@=\xy@ \def\xy@##1##2{\unsilent@@xy@{}{##2}}%
 \fi}
\xydef@\unsilencexy@{\leave@}
\xydef@\xyCOORD@other@open{%
 \ifx *\next
 \DN@*##1*){\xy@{(*}{\enter@{\pfromthep@\basefromthebase@}}%
 \POS##1\relax \xy@{*)}\leave@ \afterCOORD@}%
 \else \DN@{\xyFN@\afterCOORD@(}%
 \fi \next@}
\xydef@\xyPOS@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\POS@}%
 \else\addPLUS@\ifx \next
 \addPLUS@\DN@{\xy@+{\enter@\cplusthec@}%
 \afterCOORD{\xy@@\leave@ \xyFN@\POS@}}%
 \else\addDASH@\ifx \next
 \addDASH@\DN@{\xy@-{\enter@\cplusthec@}%
 \afterCOORD{\xy@@{\X@c=-\X@c \Y@c=-\Y@c\leave@}\xyFN@\POS@}}%
 \else\ifx !\next
 \DN@ !{\xy@!{\enter@\cskewthec@}\afterCOORD{\xy@@\leave@ \xyFN@\POS@}}%
 \else\addDOT@\ifx \next
 \addDOT@\DN@{\xy@.{\enter@\cmergethec@}%
 \afterCOORD{\xy@@\leave@ \xyFN@\POS@}}%
 \else\ifx ,\next
 \DN@ ,{\xy@,{\comma@@}\afterCOORD{\xyFN@\POS@}}%
 \else\ifx ;\next
 \DN@ ;{\xy@;{\swap@}\afterCOORD{\xyFN@\POS@}}%
 \else\ifx :\next
 \DN@ :{\xyFN@\POS@colon}%
 \else\addEQ@\ifx \next
 \addEQ@\DN@{\xyFN@\saveid@}%
 \else\ifx *\next
 \DN@ *{\xyFN@\POS@star}%
 \else \ifx ?\next
 \DN@?{\xy@?{}\afterPLACE{\xyFN@\POS@}}%
 \else \addAT@\ifx \next
 \addAT@\DN@{\xyFN@\STACK@}%
 \else
 \let\next@=\afterPOS@
 \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi \next@}
\xylet@\comma@@=\relax
\xylet@\POS@=\xyPOS@
\xydef@\POS@colon{\DNii@{\afterCOORD{\xyFN@\POS@}}%
 \ifx :\next \xy@{::}{\setbase@@\X@c\Y@c}\DN@:{\nextii@}%
 \else \xy@:{\setbase@\X@p\Y@p\X@c\Y@c}\let\next@=\nextii@ \fi
 \next@}
\xydef@\POS@star{%
 \ifx *\next
 \DN@*##1##{\nextii@{##1}}%
 \DNii@##1##2{\xy@@ix@{{##1}{##2}}%
 \xy@{**##1{##2}}{\expandafter\connect@\the\toks9 }\xyFN@\POS@}%
 \else
 \DN@##1##{\nextii@{##1}}%
 \DNii@##1##2{\xy@@ix@{{##1}{##2}}%
 \xy@{*##1{##2}}{\expandafter\drop@\the\toks9 }\xyFN@\POS@}%
 \fi
 \next@}
\xydef@\cfromp@{\X@c=\X@p \Y@c=\Y@p \U@c=\U@p \D@c=\D@p \L@c=\L@p \R@c=\R@p
 \Edge@c=\expandafter{\the\Edge@p}}
\xydef@\pfromc@{\X@p=\X@c \Y@p=\Y@c \U@p=\U@c \D@p=\D@c \L@p=\L@c \R@p=\R@c
 \Edge@p=\expandafter{\the\Edge@c}}
\xydef@\swapdimen@#1#2{\dimen@=#1\relax #1=#2\relax #2=\dimen@}
\xynew@{toks}\swaptoks@@
\xydef@\swap@{\swapdimen@\X@c\X@p \swapdimen@\Y@c\Y@p
 \swapdimen@\U@c\U@p\swapdimen@\D@c\D@p \swapdimen@\L@c\L@p\swapdimen@\R@c\R@p
 \swaptoks@@=\Edge@c \Edge@c=\Edge@p \Edge@p=\swaptoks@@}
\xydef@\vfromabsolute@#1{\vfromabsolute@@#1,@}
\xydef@\vfromabsolute@@#1,#2@{\X@c=#1\relax
 \DN@{#2}\ifx\next@\empty \Y@c=\X@c
 \else \DN@##1,{\Y@c=##1}\next@#2\relax \fi
}
\xydef@\cfromthec@{\X@c=\the\X@c \Y@c=\the\Y@c
 \U@c=\the\U@c \D@c=\the\D@c \L@c=\the\L@c \R@c=\the\R@c
 \Edge@c={\expandafter\noexpand\the\Edge@c}}
\xydef@\cfromthep@{\X@c=\the\X@p \Y@c=\the\Y@p
 \U@c=\the\U@p \D@c=\the\D@p \L@c=\the\L@p \R@c=\the\R@p
 \Edge@c={\expandafter\noexpand\the\Edge@p}}
\xydef@\pfromthep@{\X@p=\the\X@p \Y@p=\the\Y@p
 \U@p=\the\U@p \D@p=\the\D@p \L@p=\the\L@p \R@p=\the\R@p
 \Edge@p={\expandafter\noexpand\the\Edge@p}}
\xydef@\pfromthec@{\X@p=\the\X@c \Y@p=\the\Y@c
 \U@p=\the\U@c \D@p=\the\D@c \L@p=\the\L@c \R@p=\the\R@c
 \Edge@p={\expandafter\noexpand\the\Edge@c}}
\xydef@\cplusthec@{\advance\X@c\the\X@c \advance\Y@c\the\Y@c}
\xydef@\cskewthec@{%
 \noexpand\cskew@{\the\Y@c}{\the\X@c}{\the\D@c}{\the\U@c}{\the\L@c}{\the\R@c}}
\xydef@\cskew@#1#2#3#4#5#6{%
 \D@c=#3\advance\D@c \Y@c \ifdim\D@c<\z@ \D@c=\z@ \fi
 \U@c=#4\advance\U@c-\Y@c \ifdim\U@c<\z@ \U@c=\z@ \fi
 \advance\Y@c#1%
 \L@c=#5\advance\L@c \X@c \ifdim\L@c<\z@ \L@c=\z@ \fi
 \R@c=#6\advance\R@c-\X@c \ifdim\R@c<\z@ \R@c=\z@ \fi
 \advance\X@c#2%
 \Edge@c={\rectangleEdge}}
\xydef@\cmergethec@{%
 \noexpand\cmerge@{\the\Y@c}{\the\X@c}{\the\D@c}{\the\U@c}{\the\L@c}{\the\R@c}}
\xydef@\cmerge@#1#2#3#4#5#6{\the\Edge@c4%
 \A@=#2\advance\A@-\X@c \B@=#1\advance\B@-\Y@c
 \dimen@=#5\advance\L@c \A@ \ifdim\L@c<\dimen@ \L@c=\dimen@ \fi
 \dimen@=#6\advance\R@c-\A@ \ifdim\R@c<\dimen@ \R@c=\dimen@ \fi
 \dimen@=#3\advance\D@c \B@ \ifdim\D@c<\dimen@ \D@c=\dimen@ \fi
 \dimen@=#4\advance\U@c-\B@ \ifdim\U@c<\dimen@ \U@c=\dimen@ \fi
 \advance\X@c\A@ \advance\Y@c\B@}
\xydef@\halfroottwo{.70710678}
\xydef@\partroottwo{.29289322}
\xydef@\halfrootthree{.8660254}
\xydef@\vfromcartesian@#1{\vfromcartesian@@#1@}
\xydef@\vfromcartesian@@#1,#2@{%
 \X@c=\X@origin \advance\X@c#1\X@xbase \advance\X@c#2\X@ybase
 \Y@c=\Y@origin \advance\Y@c#1\Y@xbase \advance\Y@c#2\Y@ybase}
\xydef@\setbase@#1#2#3#4{%
 \X@origin=#1\relax \Y@origin=#2\relax
 \X@xbase=#3\relax \advance\X@xbase-\X@origin
 \Y@xbase=#4\relax \advance\Y@xbase-\Y@origin
 \X@ybase=-\Y@xbase \Y@ybase=\X@xbase}
\xydef@\setbase@@#1#2{%
 \X@ybase=#1\relax \advance\X@ybase-\X@origin
 \Y@ybase=#2\relax \advance\Y@ybase-\Y@origin}
\xydef@\basefromthebase@{\X@origin=\the\X@origin \Y@origin=\the\Y@origin
 \X@xbase=\the\X@xbase \Y@xbase=\the\Y@xbase
 \X@ybase=\the\X@ybase \Y@ybase=\the\Y@ybase}
\xydef@\vfromcartesianangle@#1{\enter@\basefromthebase@ \R@=#1\p@
 \B@=360\p@
 \loop@ \ifdim\R@<\z@ \advance\R@\B@ \repeat@
 \loop@ \ifdim\R@>\B@ \advance\R@-\B@ \repeat@
 \ifdim\R@<.5\B@\else \R@=-\R@ \advance\R@\B@
 \X@ybase=-\X@ybase \Y@ybase=-\Y@ybase \fi
 \B@=180\p@
 \ifdim\R@<.5\B@\else \R@=-\R@ \advance\R@\B@
 \X@xbase=-\X@xbase \Y@xbase=-\Y@xbase \fi
 \B@=90\p@
 \ifdim\R@<.5\B@ \let\nextiii@=\literal@
 \else \R@=-\R@ \advance\R@\B@ \def\nextiii@##1,##2@{##2,##1@}\fi
 \dimen@=\z@ \DN@{1,0@}%
 \dimen@ii=45\p@ \DNii@{.70710678,.70710678@}%
 \chooseangleinterval@
 {\chooseangleinterval@
 {\chooseangleinterval@
 {\chooseangleinterval@
 {\chooseangleinterval@
 {}%
 {4.090909}{.99677570,.08023846@}%
 {}}%
 {6}{.99452190,.10452846@}%
 {\chooseangleinterval@
 {}%
 {8.181818}{.98982144,.14231484@}%
 {}}}%
 {10}{.98480775,.17364818@}%
 {\chooseangleinterval@
 {}%
 {12.857143}{.97492791,.22252093@}%
 {}}}%
 {15}{.96592583,.25881905@}%
 {\chooseangleinterval@
 {\chooseangleinterval@
 {}%
 {16.363636}{.95949297,.28173256@}%
 {}}%
 {18}{.95105652,.30901699@}%
 {\chooseangleinterval@
 {}%
 {20}{.93969262,.34202014@}%
 {}}}}%
 {22.5}{.92387953,.38268343@}%
 {\chooseangleinterval@
 {\chooseangleinterval@
 {\chooseangleinterval@
 {}%
 {24.545455}{.90963200,.41541501@}%
 {}}%
 {25.714286}{.90096887,.43388374@}%
 {}}%
 {30}{.86602540,.5@}%
 {\chooseangleinterval@
 {\chooseangleinterval@
 {}%
 {32.727273}{.84125353,.54064082@}%
 {}}%
 {36}{.80901699,.58778525@}%
 {\chooseangleinterval@
 {\chooseangleinterval@
 {}%
 {38.571429}{.78183148,.62348980@}%
 {}}%
 {40.909091}{.75574957,.65486073@}%
 {\chooseangleinterval@
 {}%
 {40}{.76604444,.64278761@}%
 {}}}}}%
 \A@=\R@ \advance\A@-\dimen@
 \ifdim\ifdim\A@<\z@-\fi\A@<.01\p@ \edef\next@{\expandafter\nextiii@\next@}%
 \else \B@=\dimen@ii \advance\B@-\R@ 
 \ifdim\A@<\B@ \dimen@=\toradians@\A@
 \edef\next@{\next@ \expandafter\removePT@\the\dimen@ @}%
 \else \dimen@=-\toradians@\B@
 \edef\next@{\nextii@ \expandafter\removePT@\the\dimen@ @}%
 \fi
 \expandafter\interpolatepoint@\next@
 \edef\next@{\expandafter\nextiii@\next@}%
 \fi 
 \expandafter\vfromcartesian@@\next@
 \leave@}
\xydef@\chooseangleinterval@#1#2#3#4{%
 \B@=#2\p@ \def\next{#3}%
 \ifdim\R@<\B@ \dimen@ii=\B@ \let\nextii@=\next #1%
 \else \dimen@=\B@ \let\next@=\next \ifdim\B@<\R@ #4\fi\fi}
\xydef@\interpolateinterval@#1,#2@#3,#4@{%
 \A@=#1\p@ \dimen@=#3\p@ \advance\dimen@-\A@ \advance\A@\next\dimen@
 \B@=#2\p@ \dimen@=#4\p@ \advance\dimen@-\B@ \advance\B@\next\dimen@
 \edef\next@{\expandafter\removePT@\the\A@,\expandafter\removePT@\the\B@ @}}
\xydef@\toradians@{0.01745329}
\xydef@\interpolatepoint@#1,#2@#3@{%
 \A@=#1\p@ \dimen@ii=#3\A@ \dimen@ii=-.5\dimen@ii \advance\A@#3\dimen@ii
 \dimen@=-#2\p@ \advance\A@#3\dimen@
 \B@=#2\p@ \dimen@ii=#3\B@ \dimen@ii=-.5\dimen@ii \advance\B@#3\dimen@ii
 \dimen@=#1\p@ \advance\B@#3\dimen@
 \edef\next@{\expandafter\removePT@\the\A@,\expandafter\removePT@\the\B@ @}}
\xydef@\drop@#1#2{%
 \global\setbox\lastobjectbox@=\object#1{#2}%
 \ifHidden@ \dimen@=\X@c \advance\dimen@-\L@c \else
 \dimen@=\Y@c \advance\dimen@ \U@c \ifdim\Y@max<\dimen@ \Y@max=\dimen@ \fi
 \dimen@=\Y@c \advance\dimen@-\D@c \ifdim\dimen@<\Y@min \Y@min=\dimen@ \fi
 \dimen@=\X@c \advance\dimen@ \R@c \ifdim\X@max<\dimen@ \X@max=\dimen@ \fi
 \dimen@=\X@c \advance\dimen@-\L@c \ifdim\dimen@<\X@min \X@min=\dimen@ \fi
 \fi
 \ifInvisible@\else
 \setboxz@h{\kern\dimen@ \raise\Y@c\box\lastobjectbox@}%
 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ {\Drop@@}\fi}
\xydef@\connect@#1#2{\setupDirection@ \enter@{\cfromthec@}%
 \global\setbox\lastobjectbox@=\object#1{#2}\leave@
 \Connect@@}
\xydef@\preconnect@#1#2{\setupDirection@ \enter@{\cfromthec@}%
 \global\setbox\lastobjectbox@=\object#1{#2}\leave@ \connectStore@
 \ifInvisible@ \Connect@@ \else \Invisible@true\Connect@@\Invisible@false \fi}
\xynew@{box}\connectobjectbox@@
\xylet@\connectDrop@@=\empty
\xylet@\connectpreXY@style@=\empty
\xylet@\connectpostXY@style@=\empty
\xylet@\connectRest@@=\empty
\xydef@\connectStore@{%
 \global\setbox\connectobjectbox@@=\copy\lastobjectbox@
 \let\connectDrop@@=\Drop@@
 \let\connectpreXY@style@ =\preXY@style@ 
 \let\connectpostXY@style@=\postXY@style@
 \xdef\connectRest@@{%
 \def\noexpand\Upness@{\Upness@}%
 \def\noexpand\Leftness@{\Leftness@}%
 \ifInvisible@ \noexpand\Invisible@true \else \noexpand\Invisible@false \fi
 \ifHidden@ \noexpand\Hidden@true \else \noexpand\Hidden@false \fi}}
\xydef@\connectRestore@{%
 \ifvbox\connectobjectbox@@
 \setbox\lastobjectbox@=\copy\voidb@x
 \else
 \global\setbox\lastobjectbox@=\copy\connectobjectbox@@
 \fi
 \let\Drop@@=\connectDrop@@
 \global\let\preXY@style@ =\connectpreXY@style@ 
 \global\let\postXY@style@=\connectpostXY@style@
 \connectRest@@}
\xydef@\afterPLACE#1{%
 \DN@##1{\def\afterPLACE@{\xy@@\leave@ \def\afterPLACE@{##1}#1}}%
 \expandafter\next@\expandafter{\afterPLACE@}%
 \def\PLACEf@{{.5}}%
 \xy@@{\enter@{\pfromthep@}%
 \Creset@@ \def\PLACEf@{{.5}}%
 \let\PLACEedgep@@=\PLACEedgep@ \let\PLACEedgec@@=\PLACEedgec@}%
 \xyFN@\PLACE@}
\xydef@\PLACEf@{}
\xydef@\PLACEedgep@@{}
\xydef@\PLACEedgec@@{}
\xydef@\PLACEedgep@{\Cshavep@@ \def\PLACEedgep@@{\Cslidep@@\jot}}
\xydef@\PLACEedgec@{\Cshavec@@ \def\PLACEedgec@@{\Cslidec@@{-\jot}}}
\xylet@\afterPLACE@=\empty
\xydef@\PLACE@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\PLACE@}%
 \else\addLT@\ifx \next
 \addLT@\DN@{\addLT@\xy@{\def\PLACEf@{{0}}\PLACEedgep@@}\xyFN@\PLACE@}%
 \else\addGT@\ifx \next
 \addGT@\DN@{\addGT@\xy@{\def\PLACEf@{{1}}\PLACEedgec@@}\xyFN@\PLACE@}%
 \else\ifx (\next
 \DN@(##1){\def\PLACEf@{{##1}}\xy@{(##1)}{\def\PLACEf@{{##1}}}\xyFN@\PLACE@}%
 \else\ifx !\next
 \DN@!{\xyFN@\PLACE@intercept}%
 \else
 \DN@{\xy@@{\expandafter\Calong@@\PLACEf@ \czeroEdge@}\PLACE@@}%
 \fi\fi\fi\fi\fi \next@}
\xydef@\PLACE@intercept{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\PLACE@intercept}%
 \else\ifx \bgroup\next
 \DN@##1{\xy@{!{##1}}{}\PLACE@intercept@{##1}}%
 \else\ifx (\next
 \DN@(*##1*){\xy@{!(*##1*)}{}\PLACE@intercept@{##1}}%
 \else \DN@{\xyerror@{{<pos>} expected after ! in <place>}{}}%
 \fi\fi\fi \next@}
\xydef@\PLACE@intercept@#1{%
 \xy@@{\enter@{\pfromthep@\basefromthebase@}\begingroup}%
 \xy@@ix@{#1}\xy@@{\plainxy@ \expandafter\POS\the\toks9\relax
 \edef\next@{\endgroup
 \X@c =\the\X@c \Y@c=\the\Y@c \X@p=\the\X@p \Y@p=\the\Y@p}%
 \next@ \Cintercept@@ \leave@}%
 \PLACE@@}
\xydef@\PLACE@@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\PLACE@@}%
 \else\ifx /\next \DN@/##1/{\xy@{/##1/}{\Cslidec@@{##1}}\afterPLACE@}%
 \else \let\next@=\afterPLACE@
 \fi\fi \next@}
\xydef@\intersect@{%
 \d@X=\X@c \advance\d@X-\X@p \d@Y=\Y@c \advance\d@Y-\Y@p
 \A@=\X@c \advance\A@-\X@origin \B@=\Y@c \advance\B@-\Y@origin
 \edef\next@{\expandafter\removePT@\the\R@c}%
 \edef\nextii@{\expandafter\removePT@\the\U@c}%
 \D@c=\next@\d@Y \advance\D@c-\nextii@\d@X \divide\D@c\KK@
 \L@c=\next@\B@ \advance\L@c-\nextii@\A@ \divide\L@c\KK@
 \ifdim\D@c=\z@\zeroDivide@\else \quotient@\next@\L@c\D@c \fi
 \advance\X@c-\next@\d@X \advance\Y@c-\next@\d@Y
 \czeroEdge@}
\xydef@\zeroDivide@@{\zeroDivide@message{\intersect@}{treated as 0}\DN@{0}}
\xydef@\zeroDivide@message#1#2{\xywarning@{division by 0 in \string#1, #2}}
\xylet@\zeroDivide@=\zeroDivide@@
\xydef@\zeroDivideLimit@@{\ifdim\L@c=\z@ \DN@{0}%
 \else\ifdim\L@c<\z@\DN@{-\zeroDivide@Limit}%
 \else\DN@{\zeroDivide@Limit}\fi\fi
 \zeroDivide@message{\intersect@}{replaced by \zeroDivide@Limit}}
\xydef@\zeroDivideLimit@#1{\edef\zeroDivide@Limit{#1}%
 \let\zeroDivide@=\zeroDivideLimit@@}
\xylet@\zeroDivideLimit=\zeroDivideLimit@
\xydef@\vfromslide@#1{\enter@\DirectionfromtheDirection@ \begingroup
 \plainxy@\afterDIRECTIONorEMPTY\vfromslide@i\vfromslide@i#1@}
\xydef@\vfromslide@i#1@{\DN@{#1}%
 \edef\next{\endgroup
 \ifx\next@\empty \dimen@=.5pc \else \dimen@=#1\relax \fi
 \X@c=\cosDirection\dimen@ \Y@c=\sinDirection\dimen@}\next
 \leave@}
\xydef@\s@bot{-1}
\xydef@\s@top{-1}
\xydef@\cfroms@#1{\tests@{#1}\runs@\outofranges@}
\xydef@\tests@#1#2#3{\DN@{#3}%
 \count@=\s@top \advance\count@-#1\relax
 \ifnum\count@>\s@bot\relax \ifnum\count@>\s@top\else\DN@{#2}\fi\fi
 \next@}
\xydef@\runs@{\csname S@\the\count@\endcsname}
\xydef@\outofranges@{\count@=\s@top \advance\count@-\s@bot
 \xyerror@{stack index out of range (should be 0..\the\count@)}{}}
\xydef@\STACK@{%
 \addPLUS@\ifx\next
 \addPLUS@\DN@{\xy@{@+}{}\afterCOORD{\xy@@\spushc@ \xyFN@\POS@}}%
 \else\addDASH@\ifx\next
 \addDASH@\DN@{\xy@{@-}{}\afterCOORD{\xy@@\spop@ \xyFN@\POS@}}%
 \else \ifx i\next \DN@ i{\xy@{@i}\sinit@ \xyFN@\POS@}%
 \else \ifx (\next \DN@ ({\xy@{@(}\senter@ \xyFN@\POS@}%
 \else \ifx )\next \DN@ ){\xy@{@)}\sleave@ \xyFN@\POS@}%
 \else\addEQ@\ifx\next \addEQ@\DN@{\STACK@load}%
 \else\addAT@\ifx\next \addAT@\DN@{\xy@{@@}{}\smap@}%
 \else \DN@##1{\xyerror@{illegal stack command ##1}{}\afterCOORD{\xyFN@\POS@}}%
 \fi\fi\fi\fi\fi\fi\fi \next@}
\xydef@\STACK@load{\xy@{@=}{%
 \if\sempty@\else \xywarning@{loading on top of non-empty stack}\sinit@ \fi
 \let\comma@@=\spushc@}%
 \afterCOORD{\xy@@{\spushc@ \let\comma@@=\relax}\xyFN@\POS@}}
\xydef@\spushc@{%
 \count@=\s@top \advance\count@\@ne \edef\s@top{\the\count@}%
 \expandafter\edef\csname S@\s@top\endcsname{\cfromthec@}}
\xydef@\spushid@#1{\DNii@{#1}\edef\nextii@{\codeof\nextii@}%
 \expandafter\let\expandafter\next@\csname Q@\nextii@\endcsname
 \ifx\next@\relax \xyerror@{<pos> \string"\nextii@\string" not defined}{}%
 \else
 \count@=\s@top \advance\count@\@ne \edef\s@top{\the\count@}%
 \DNii@##1{\expandafter\def\csname S@\s@top\endcsname{##1}}%
 \expandafter\nextii@\expandafter{\next@}%
 \fi}
\xydef@\idfroms@#1#2{%
 \tests@{#2}{\DN@{\idfromxy@{#1}}%
 \expandafter\expandafter\expandafter\next@
 \expandafter\expandafter\expandafter{\csname S@\the\count@\endcsname}%
 }\outofranges@}
\xydef@\spop@{\count@=\s@top
 \ifnum\count@>\s@bot \advance\count@\m@ne \edef\s@top{\the\count@}%
 \else \xyerror@{nothing to pop from stack}{}\fi}
\xydef@\sinit@{\edef\s@top{\s@bot}}
\xydef@\senter@{%
 \count@=\s@top \advance\count@\@ne
 \expandafter\edef\csname S@\the\count@\endcsname{\s@bot}%
 \edef\s@bot{\the\count@}\edef\s@top{\the\count@}}
\xydef@\sleave@{%
 \ifnum\s@bot=\s@top\else \xywarning@{leaving non-empty stack}\sinit@ \fi
 \ifnum\s@bot>\m@ne \edef\s@bot{\csname S@\s@top\endcsname}%
 \count@=\s@top \advance\count@\m@ne \edef\s@top{\the\count@}%
 \edef\sbot{\the\count@}\fi}
\xydef@\sempty@{\ifnum\s@top=\s@bot TT\else TF\fi}
\xydef@\xytotoks@#1#2{\addtotoks@{#2}}
\xydef@\xytotoks@@toksix@#1{\addtotoks@{\toks9={#1}}}
\xydef@\smap@{%
 \begingroup \toks@={}\let\xy@=\xytotoks@ \change@oxy@\xy@
 \let\xy@@ix@=\xytotoks@@toksix@
 \afterCOORD{\expandafter\endgroup
 \expandafter\smapxy@@\expandafter{\the\toks@}\xyFN@\POS@}}
\xydef@\smapxy@@#1{\xy@@{\edef\smapp@@{\s@bot}\smapxy@i{#1}}}
\xylet@\smapp@@=\empty
\xydef@\smapxy@i#1{%
 \ifnum\smapp@@<\s@top
 \count@=\smapp@@ \advance\count@\@ne \edef\smapp@@{\the\count@}%
 \DN@{\csname S@\smapp@@\endcsname #1\relax \smapxy@i{#1}}%
 \else \let\next@=\relax
 \fi \next@}
\xydef@\saveid@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\saveid@}%
 \else \ifx "\next\DN@"##1"{\xy@{="##1"}{\idfromc@{##1}}\xyFN@\POS@}%
 \else \ifx :\next\DN@:##1"##2"{\xy@{=:"##2"}{\idfrombase@{##2}}\xyFN@\POS@}%
 \else\addAT@\ifx\next
 \addAT@\DN@"##1"{\xy@{=@"##1"}{\idfromstack@{##1}}\xyFN@\POS@}%
 \else \ifx s\next
 \DN@ s##1"##2"{\xy@{=s##1"##2"}{\idfroms@{##2}{##1}}\xyFN@\POS@}%
 \else\addEQ@\ifx\next \let\saveid@COORD@@=\saveid@COORDii
 \addEQ@\DN@{\xyFN@\saveid@COORD}%
 \else \let\saveid@COORD@@=\saveid@COORDi \let\next@=\saveid@COORD
 \fi\fi\fi\fi\fi\fi \next@}
\xylet@\saveid@COORD@@=\relax
\xydef@\idfromc@#1{\DN@{#1}%
 \expandafter\edef\csname Q@\codeof\next@\endcsname{\cfromthec@}}
\xydef@\idfrombase@#1{\DN@{#1}%
 \expandafter\edef\csname Q@\codeof\next@\endcsname{\basefromthebase@}}
\xydef@\idfromstack@#1{%
 \toks@={\if\sempty@\else
 \xywarning@{loading on top of non-empty stack}\sinit@ \fi}%
 \count@=\s@bot \advance\count@\@ne
 \ifnum\count@>\s@top\else
 \loop@
 \expandafter\let\expandafter\next@\csname S@\the\count@\endcsname
 \expandafter\addtotoks@\expandafter{\next@}%
 \ifnum\count@<\s@top \advance\count@\@ne \addtotoks@{\spushc@}\repeat@
 \fi
 \DN@{#1}\edef\next@##1{%
 \def\expandafter\noexpand\csname Q@\codeof\next@\endcsname{##1}}%
 \expandafter\next@\expandafter{\the\toks@}}
\xydef@\saveid@COORD{%
 \begingroup \toks@={}\let\xy@=\xytotoks@ \change@oxy@\xy@
 \let\xy@@ix@=\xytotoks@@toksix@
 \afterCOORD{\expandafter\saveid@COORDi\expandafter{\the\toks@}}}
\xydef@\saveid@COORDi#1#2"#3"{\endgroup \xy@@{\idfromxy@{#3}{#1}}\xyFN@\POS@}
\xydef@\saveid@COORDii#1#2"#3"{\endgroup \xy@@{\idfromcxy@{#3}{#1}}\xyFN@\POS@}
\xydef@\idfromxy@#1#2{\DN@{#1}%
 \expandafter\def\csname Q@\codeof\next@\endcsname{#2}}
\xydef@\idfromcxy@#1#2{\DN@{#1}%
 \expandafter\edef\csname Q@\codeof\next@\endcsname{\cfromthec@#2}}
\xydef@\cfromid@#1{\DNii@{#1}\edef\nextii@{\codeof\nextii@}%
 \expandafter\let\expandafter\next@\csname Q@\nextii@\endcsname
 \ifx\next@\relax \xyerror@{<pos> \string"\nextii@\string" not defined}{}%
 \else \expandafter\next@\fi}
\message{objects,}
\xydef@\OBJECT@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\OBJECT@}%
 \else\ifcat A\noexpand\next \let\next@=\OBJECT@letter
 \else \let\next@=\OBJECT@other \fi\fi \next@}
\xydef@\OBJECT@letter{%
 \ifx i\next \DN@ i{\addtotoks@\Invisible@true \xyFN@\OBJECT@}%
 \else\ifx h\next\DN@ h{\addtotoks@\Hidden@true \xyFN@\OBJECT@}%
 \else\ifx o\next\DN@ o{\xywarning@{Obsolete o modifier used}\OBJECT@shape{o}}%
 \else\ifx x\next\DN@ x{\xywarning@{Obsolete x modifier used}\OBJECT@shape{}}%
 \else\ifx @\next\DN@ @##1##{%
\xywarning@{Impossible @ (letter) should not be here!!}
 \OBJECT@@{\dir##1}}%
 \else \let\next@=\OBJECT@direction
 \fi\fi\fi\fi\fi \next@}
\xydef@\OBJECT@other{%
 \ifx !\next \DN@!{\OBJECT@shift}%
 \else\addPLUS@\ifx \next \DN@{\OBJECT@change}%
 \else\addDASH@\ifx \next \DN@{\OBJECT@change}%
 \else\addEQ@\ifx \next \DN@{\OBJECT@set}%
 \else\ifx [\next
 \DN@[##1]{\xy@{[##1]}{\OBJECT@shape{##1}}}%
 \else\ifx ^\next \let\next@=\OBJECT@direction
 \else\ifx _\next \let\next@=\OBJECT@direction
 \else\ifx :\next \let\next@=\OBJECT@direction
 \else\ifx ?\next
 \DN@ ?{\xywarning@{\string? modifier used}\xyFN@\OBJECT@direction}%
 \else\ifx (\next
 \let\next@=\OBJECT@direction
 \else\addAT@\ifx\next \addAT@\DN@##1##{\OBJECT@@{\dir##1}}%
 \else \DN@##1##{\OBJECT@@{##1}}%
 \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi \next@}
\xydef@\prevEdge@@{\zeroEdge}
\xydef@\OBJECT@@#1#2{%
 \expandafter\def\expandafter\prevEdge@@\expandafter{\the\Edge@c}%
 \expandafter\Edge@c\expandafter{\objectEdge}%
 \Invisible@false\Hidden@false
 \def\Leftness@{.5}\def\Upness@{.5}%
 \gdef\preXY@style@{}\gdef\postXY@style@{}%
 \def\Drop@@{\styledboxz@}\def\Connect@@{\straight@\relax}%
 \DN@{#1}\ifx\next@\empty \DNii@{#2}%
 \ifx\nextii@\empty \DN@{\hbox\bgroup\no@}\else \let\next@=\objectbox \fi\fi
 \setbox\z@=\next@{#2}\L@c=\Leftness@\wdz@ \R@c=\wdz@ \advance\R@c-\L@c
 \D@c=\dp\z@ \advance\D@c\ht\z@ \U@c=\Upness@\D@c \advance\D@c-\U@c
 \R@p=\z@ \L@p=\L@c \U@p=\U@c \advance\U@p-\ht\z@ \D@p=-\U@p
 \the\toks@\toks@={}\setboxz@h{\kern\R@p \raise\U@p\boxz@}%
 \checkZeroEdge@
 \dimen@=\L@c \advance\dimen@\R@c \wdz@=\dimen@ \ht\z@=\U@c \dp\z@=\D@c \boxz@
 \OBJECT@x}
\xydef@\adjustLR@{%
 \ifdim\zz@\wdz@ \L@c=\z@ \R@c=\z@ \dimen@=\Leftness@\p@
 \ifdim\dimen@<\z@ \L@c=\dimen@ \R@c=-\L@c
 \else\ifdim\dimen@>\p@ \L@c=\dimen@ \advance\L@c-\p@ \R@c=-\L@c \fi\fi
 \else \L@c=\Leftness@\wdz@ \R@c=\wdz@ \advance\R@c-\L@c \fi}
\xydef@\adjustUD@{\dimen@=\ht\z@ \advance\dimen@\dp\z@
 \ifdim\zz@\dimen@ \U@c=\z@ \D@c=\z@ \dimen@=\Upness@\p@
 \ifdim\dimen@<\z@ \U@c=\dimen@ \D@c=-\L@c
 \else\ifdim\dimen@>\p@ \U@c=\dimen@ \advance\U@c-\p@ \D@c=-\L@c \fi\fi
 \else \D@c=\dimen@ \U@c=\Upness@\dimen@ \advance\D@c-\U@c \fi}
\def\checkZeroEdge@{%
 \DN@{}%
 \ifdim\zz@\L@c \ifdim\zz@\R@c \ifdim\zz@\U@c \ifdim\zz@\D@c
 \DN@{\Edge@c={\zeroEdge}}\fi\fi\fi\fi
 \next@}
\xydef@\OBJECT@x{\toks@={\egroup\def\Drop@@}%
 \expandafter\addtotoks@\expandafter{\expandafter{\Drop@@}\def\Connect@@}%
 \expandafter\addtotoks@\expandafter{\expandafter{\Connect@@}}%
 \edef\tmp@{\D@c=\the\D@c \U@c=\the\U@c \L@c=\the\L@c \R@c=\the\R@c
 \Edge@c={\expandafter\noexpand\the\Edge@c}%
 \ifInvisible@\noexpand\Invisible@true\else\noexpand\Invisible@false\fi
 \ifHidden@\noexpand\Hidden@true\else\noexpand\Hidden@false\fi
 \def\noexpand\Leftness@{\Leftness@}\def\noexpand\Upness@{\Upness@}}%
 \expandafter\addtotoks@\expandafter{\tmp@}\the\toks@}
\xynew@{if}\ifInvisible@
\xynew@{if}\ifHidden@
\xydef@\Leftness@{}
\xydef@\Upness@{}
\xydef@\Drop@@{\styledboxz@}
\xydef@\Connect@@{}
\xydef@\objectbox#1{\hbox{$\m@th\objectstyle{#1}$}}
\xylet@\objectstyle=\textstyle
\xydef@\object{\hbox\bgroup\resetStyle@\object@}
\xydef@\object@{%
 \edef\next@{={\DirectionfromtheDirection@}}\expandafter\toks@\next@
 \plainxy@ \xyFN@\OBJECT@}
\xydef@\composite#1#{\hbox\bgroup\composite@{#1}}
\xydef@\composite@#1#2{%
 \DN@{#1}\ifx\next@\empty\else\xywarning@{no variants of
 \string\composite\space allowed}\fi
 \global\setbox9=\hbox\bgroup
 \D@p=-\maxdimen \U@p=-\maxdimen \L@p=-\maxdimen \R@p=-\maxdimen
 \xyFN@\composite@i#2@}
\xydef@\composite@i{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\composite@i}%
 \else\ifx *\next \DN@ *{\xyFN@\composite@i}%
 \else\ifx @\next \DN@ @{\composite@x}%
 \xyerror@{<composite> object expected}{}\czeroEdge@
 \else \DN@{\composite@ii}\fi\fi\fi \next@}
\xydef@\composite@ii#1#{\composite@iii{#1}}
\xydef@\composite@iii#1#2{%
 \setbox\z@=\object#1{#2}%
 \ifInvisible@ \setboxz@h{}\else
 \setboxz@h{\kern-\L@c \boxz@}\ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ {\Drop@@}\fi
 \ifHidden@\else
 \ifdim\U@p<\U@c \U@p=\U@c \fi \ifdim\D@p<\D@c \D@p=\D@c \fi
 \ifdim\R@p<\R@c \R@p=\R@c \fi \ifdim\L@p<\L@c \L@p=\L@c \fi
 \fi
 \xyFN@\composite@iv}
\xydef@\composite@iv{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\composite@iv}%
 \else \ifx @\next \DN@ @{\composite@x}%
 \else \let\next@=\composite@i \fi\fi \next@}
\xydef@\composite@x{%
 \edef\tmp@{\egroup
 \D@c=\the\D@p \U@c=\the\U@p \L@c=\the\L@p \R@c=\the\R@p}\tmp@
 \setboxz@h{\kern\L@c\box9}\ht\z@=\U@c \dp\z@=\D@c
 \dimen@=\L@c \advance\dimen@\R@c \wdz@=\dimen@
 \Edge@c={\rectangleEdge}\computeLeftUpness@ \boxz@
 \OBJECT@x}
\xydef@\computeLeftUpness@{%
 \dimen@=\L@c \advance\dimen@\R@c
 \ifdim\zz@\dimen@ \def\Connect@@{\straight@{\dottedSpread@\jot}}%
 \ifdim\zz@\L@c\else
 \DN@{\zeroEdge}\expandafter\DNii@\expandafter{\the\Edge@c}%
 \ifx\next@\nextii@\Edge@c={\rectangleEdge}\fi\fi
 \else \quotient@\Leftness@\L@c\dimen@ \fi
 \dimen@=\U@c \advance\dimen@\D@c 
 \ifdim\zz@\dimen@ \def\Connect@@{\straight@{\dottedSpread@\jot}}%
 \ifdim\zz@\U@c\else
 \DN@{\zeroEdge}\expandafter\DNii@\expandafter{\the\Edge@c}%
 \ifx\next@\nextii@\Edge@c={\rectangleEdge}\fi\fi
 \else \quotient@\Upness@\U@c\dimen@ \fi}
\xydef@\xybox#1{\xy#1\endxy \Edge@c={\rectangleEdge}\computeLeftUpness@}
\xydef@\OBJECT@shift{%
 \let\xy@=\xytotoks@ \afterVECTORorEMPTY
 {\OBJECT@shift@}%
 {\addtotoks@{\X@c=-\L@c \advance\X@c\R@p \advance\X@c\L@p \Y@c=\U@p}%
 \OBJECT@shift@}}
\xydef@\OBJECT@shift@{%
 \addtotoks@{\advance\U@p-\Y@c
 \advance\L@c\X@c \advance\R@c-\X@c \advance\D@c\Y@c \advance\U@c-\Y@c
 \computeLeftUpness@}%
 \let\xy@=\oxy@ \xyFN@\OBJECT@}
\xylet@\objectmargin@=\jot
\xylet@\objectwidth@=\z@
\xylet@\objectheight@=\z@
\xydef@\objectmargin{\afterADDOP{\Addop@@\objectmargin@}}
\xydef@\objectwidth{\afterADDOP{\Addop@@\objectwidth@}}
\xydef@\objectheight{\afterADDOP{\Addop@@\objectheight@}}
\xydef@\OBJECT@change{%
 \afterADDOP{%
 \addEQ@\ifx \next
 \addtotoks@{\X@c=\D@c \advance\X@c\U@c \Y@c=\L@c \advance\Y@c\R@c}%
 \else
 \addtotoks@{\X@c=\objectmargin@ \advance\X@c\X@c \Y@c=\X@c}%
 \fi
 \let\xy@=\xytotoks@ 
 \afterVECTORorEMPTY\OBJECT@change@\OBJECT@change@}}
\xydef@\OBJECT@set{%
 \afterADDOP{%
 \let\xy@=\xytotoks@ \afterVECTORorEMPTY\OBJECT@change@
 {\addtotoks@{\X@c=\objectwidth@ \Y@c=\objectheight@}\OBJECT@change@}}}
\xydef@\OBJECT@change@{%
 \addtotoks@{\advance\R@c\L@c \advance\R@p-\L@c \let\tmp@=\R@c}%
 \expandafter\addtotoks@\expandafter{\Addop@@\tmp@\X@c\R@c=\tmp@
 \L@c=\Leftness@\R@c \advance\R@p\L@c \advance\R@c-\L@c}%
 \addtotoks@{\advance\D@c\U@c \let\tmp@=\D@c}%
 \expandafter\addtotoks@\expandafter{\Addop@@\tmp@\Y@c\D@c=\tmp@
 \U@c=\Upness@\D@c \advance\D@c-\U@c}%
 \let\xy@=\oxy@ \xyFN@\OBJECT@}
\xydef@\afterADDOP#1{\def\afterADDOP@{#1}\xyFN@\ADDOP@}
\xylet@\afterADDOP@=\empty
\xydef@\ADDOP@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\ADDOP@}%
 \else\addPLUS@\ifx \next \addPLUS@\DN@{\xyFN@\ADDOP@plus}%
 \else\addDASH@\ifx \next \addDASH@\DN@{\xyFN@\ADDOP@minus}%
 \else\addEQ@\ifx \next
 \addEQ@\DN@{\def\Addop@@{\Addop@0+=}\afterADDOP@}%
 \else
 \DN@{\def\Addop@@{\Addop@0+=}\afterADDOP@}%
 \fi\fi\fi\fi \next@}
\xydef@\ADDOP@plus{%
 \addEQ@\ifx \next
 \addEQ@\DN@{\def\Addop@@{\Addop@0+<}\afterADDOP@}%
 \else
 \DN@{\def\Addop@@{\Addop@1+=}\afterADDOP@}%
 \fi \next@}
\xydef@\ADDOP@minus{%
 \addEQ@\ifx \next
 \addEQ@\DN@{\def\Addop@@{\Addop@0+>}\afterADDOP@}%
 \else
 \DN@{\def\Addop@@{\Addop@1-=}\afterADDOP@}%
 \fi \next@}
\xydef@\Addop@#1#2#3#4#5{%
 \dimen@=#4\relax \edef#4{\the\dimen@}%
 \dimen@=#1\dimen@ \advance\dimen@#2#5\relax
 \ifdim\dimen@#3#4\else \edef#4{\the\dimen@}\fi
 \ifx\xy@\xyinitial@\else \DN@##1{\xy@@{\edef#4{##1}\checkZeroEdge@}}%
 \expandafter\next@\expandafter{#4}\fi}
\xydef@\objectEdge{\rectangleEdge}
\xydefcsname@{shape [r]}{\advance\U@p\D@c \centerobject@
 \ifdim\L@c>\D@c
 \advance\R@c\L@c \L@c=.5\U@c \advance\L@c.5\D@c \advance\R@c-\L@c \fi
 \advance\U@p-\D@c}
\xydefcsname@{shape [l]}{\advance\U@p\D@c \centerobject@
 \ifdim\L@c>\D@c
 \advance\L@c\R@c \R@c=.5\U@c \advance\R@c.5\D@c \advance\L@c-\R@c \fi
 \advance\U@p-\D@c}
\xydefcsname@{shape [u]}{\advance\U@p\D@c \centerobject@
 \ifdim\D@c>\L@c
 \advance\U@c\D@c \D@c=.5\L@c \advance\D@c.5\R@c \advance\U@c-\D@c \fi
 \advance\U@p-\D@c}
\xydefcsname@{shape [d]}{\advance\U@p\D@c \centerobject@
 \ifdim\D@c>\L@c
 \advance\D@c\U@c \U@c=.5\L@c \advance\U@c.5\R@c \advance\D@c-\U@c \fi
 \advance\U@p-\D@c}
\xydefcsname@{shape [c]}{\advance\U@p\D@c \centerobject@ \advance\U@p-\D@c}
\xydef@\centerobject@{%
 \advance\D@c\U@c \D@c=.5\D@c \U@c=\D@c \advance\L@c\R@c \L@c=.5\L@c \R@c=\L@c}
\xydef@\OBJECT@shape#1{\DN@{shape [#1]}%
 \expandafter\let\expandafter\nextii@\csname\codeof\next@\endcsname
 \ifx\nextii@\relax\DN@{style [#1]}%
 \expandafter\let\expandafter\nextii@\csname\codeof\next@\endcsname
 \ifx\nextii@\relax \DN@{\OBJECT@shapei[#1]}%
 \else\DN@{\nextii@\xyFN@\OBJECT@}\fi
 \else \expandafter\addtotoks@\expandafter{\nextii@}%
 \DN@{\xyFN@\OBJECT@}%
 \fi \next@}
\xydefcsname@{shape []}{\the\Edge@c5\relax}%
\xydefcsname@{shape [Outer]}{\the\Edge@c5\relax}%
\xydefcsname@{shape [Inner]}{\the\Edge@c4\relax}%
\xydefcsname@{shape [o]}{\Edge@c={\circleEdge}\the\Edge@c5\relax 
 \Edge@c={\circleEdge}\def\prevEdge@@{\circleEdge}}
\xydefcsname@{shape [.]}{\czeroEdge@}
\def\OBJECT@shapei[#1#2]{\DN@{shape [#1...]}%
 \expandafter\let\expandafter\next\csname\codeof\next@\endcsname
 \ifx\next\relax\DN@{*stylechar@#1@}%
 \expandafter\let\expandafter\next\csname\codeof\next@\endcsname
 \ifx\next\relax\DNii@{shape [#1#2]}%
 \xywarning@{illegal [<shape>] ignored: \codeof\nextii@\space not defined}%
 \DN@{\xyFN@\OBJECT@}%
 \else% Delete this: \expandafter\addtotoks@\expandafter{\next{#2}}%
 \DN@{\next{#2}\xyFN@\OBJECT@}%
 \fi
 \else
\expandafter\addtotoks@\expandafter{\next{#2}}\DN@{\next{#2}\xyFN@\OBJECT@}%
 \fi \next@}
\xydef@\preXY@style@{}
\xydef@\postXY@style@{}
\xydef@\resetStyle@{\gdef\preXY@style@{}\gdef\postXY@style@{}}
\xynew@{toks}{\styletoks@}
\xydef@\addtostyletoks@#1{%
 \expandafter\styletoks@\expandafter{\the\styletoks@#1}}
\xydef@\styledboxz@{%
 \xypre@Style@@
 \boxz@
 \xypost@Style@@}
\xydef@\xypre@Style@{\styletoks@={}\saveXyStyle@\preXY@style@
 \expandafter\DN@\expandafter{\the\styletoks@}%
 \ifx\next@\empty \DN@{\let\xypre@Style@@=\relax 
 \let\xypost@Style@@=\relax \xypre@skipStyle@}%
 \else
 \let\xypre@Style@@=\relax \let\xypost@Style@@=\xypost@Style@
 \DN@{\expandafter\xydoprestyles@\expandafter{\the\styletoks@}}%
 \fi \next@ }
\xydef@\xypost@Style@{\styletoks@={}\postXY@style@
 \expandafter\xydopoststyles@\expandafter{\the\styletoks@}%
 \let\xypost@Style@@=\relax \let\xypre@Style@@=\xypre@Style@ }
\xydef@\xypre@skipStyle@#1\xypost@Style@@{#1\relax 
 \let\xypre@Style@@=\xypre@Style@ }
\xydef@\xydoprestyles@@{\literal@}
\xydef@\xydopoststyles@@{\literal@}
\xylet@\xydoprestyles@=\xydoprestyles@@
\xylet@\xydopoststyles@=\xydopoststyles@@
\xydef@\modXYstyle@{%
 \ifx\xy@style@\empty\resetStyle@\fi \checkXyStyle@
 \expandafter\expandafter\expandafter\DN@
 \expandafter\expandafter\expandafter{\preXYstyle@@}%
 \ifx\next@\empty\else\DN@{\modXYstyle@@}\fi \next@ }
\xydef@\modXYstyle@@{%
 \DN@##1{\expandafter\def\expandafter\tmp@\expandafter{##1}}%
 \expandafter\next@\expandafter{\preStyle@@}%
 \DN@##1{\expandafter\gdef\expandafter\preXY@style@\expandafter{%
 \preXY@style@ ##1}}\expandafter\next@\expandafter{\tmp@}%
 \DN@##1{\expandafter\def\expandafter\tmp@\expandafter{##1}}%
 \expandafter\next@\expandafter{\postStyle@@}%
 \DN@##1{\expandafter\gdef\expandafter\postXY@style@\expandafter{%
 \tmp@ ##1}}\expandafter\next@\expandafter{\postXY@style@}}
\xydef@\xy@style@{}
\xydef@\checkXyStyle@{\ifx\xy@style@\empty\resetStyle@\fi
 \let\xy@style@=\relax}
\xydef@\preStyle@@{}
\xydef@\postStyle@@{}
\xydef@\preXYstyle@@{\relax}
\xydef@\loadxystyle@{%
 \let\xypre@Style@@=\xypre@Style@ \def\preXYstyle@@{\preStyle@@}}
\loadxystyle@
\xydef@\Unloadstyle@{%
 \let\xypre@Style@@=\relax \let\xypost@Style@@=\relax
 \def\preXYstyle@@{\relax}}
\xydefcsname@{shape [=...]}#1{\checkXyStyle@ \addtotoks@{\xynamestyle@{#1}}}
\xydef@\xynamestyle@#1{\checkXyStyle@
 \expandafter\DNii@\expandafter{\csname shape [#1]\endcsname}%
 \expandafter\ifx\nextii@\relax
 \else\xywarning@{Redefining style [#1]}\fi
 \expandafter\xynamestyle@@\csname shape [#1]\endcsname }
\xydef@\xynamestyle@@#1{%
 \expandafter\def\expandafter\tmp@\expandafter{\preXY@style@}%
 \DN@##1{\def\tmp@{\checkXyStyle@\gdef\preXY@style@{##1}}}%
 \expandafter\next@\expandafter{\preXY@style@}%
 \DN@##1{\expandafter\gdef\expandafter#1\expandafter{\tmp@
 \gdef\postXY@style@{##1}}}%
 \expandafter\next@\expandafter{\postXY@style@}\DN@{}}
\xydef@\prevXypreStyle@@{}
\xydef@\prevXypostStyle@@{}
\xydef@\saveXyStyle@{\expandafter
 \def\expandafter\prevXypreStyle@@\expandafter{\preXY@style@}%
 \expandafter\def\expandafter\prevXypostStyle@@\expandafter{%
 \postXY@style@}}
\xydef@\recoverXyStyle@{\expandafter
 \gdef\expandafter\preXY@style@\expandafter{\prevXypreStyle@@}%
 \expandafter\gdef\expandafter\postXY@style@\expandafter{%
 \prevXypostStyle@@}}
\xydef@\newxystyle#1#2#3{%
 \DN@{#3}\ifx\next@\empty 
 \xydefcsname@{shape [#1]}{\csname xyshape@#1@\endcsname}%
 \else \expandafter\def\csname shape [#1]\endcsname{%
 \csname xyshape@#1@\endcsname}\fi
 \DN@{#2}\ifx\next@\empty
 \expandafter\def\csname xyshape@#1@\endcsname{%
 \xyundefinedStyle@{#1}{}@@}%
 \else \expandafter\def\csname xyshape@#1@\endcsname{#2}\fi}
\xydef@\xyundefinedStyle@#1#2@@{%
 \xywarning@{style #1 not defined, nothing to apply}}
\xydef@\applyFIFOstyle@#1#2#3#4{\bgroup
 \styletoks@={\egroup\gdef\preXY@style@}%
 \expandafter\toks@\expandafter{\preXY@style@}%
 \expandafter\addtotoks@\expandafter{\expandafter#1\expandafter{#2}}%
 \expandafter\addtostyletoks@\expandafter{\expandafter{\the\toks@}%
 \gdef\postXY@style@}%
 \expandafter\toks@\expandafter{\expandafter#3\expandafter{#4}}%
 \expandafter\addtotoks@\expandafter{\postXY@style@}%
 \expandafter\addtostyletoks@\expandafter{\expandafter{\the\toks@}}%
 \the\styletoks@ }
\xydef@\applyLIFOstyle@#1#2#3#4{\bgroup
 \styletoks@={\egroup\gdef\preXY@style@}%
 \expandafter\toks@\expandafter{\expandafter#1\expandafter{#2}}%
 \expandafter\addtotoks@\expandafter{\preXY@style@}%
 \expandafter\addtostyletoks@\expandafter{\expandafter{\the\toks@}%
 \gdef\postXY@style@}%
 \expandafter\toks@\expandafter{\postXY@style@}%
 \expandafter\addtotoks@\expandafter{\expandafter#3\expandafter{#4}}%
 \expandafter\addtostyletoks@\expandafter{\expandafter{\the\toks@}}%
 \the\styletoks@ }
\xydef@\OBJECT@direction{\afterDIRECTIONorEMPTY{%
 \edef\next@{{\DirectionfromtheDirection@}}\expandafter\addtotoks@\next@
 \xyFN@\OBJECT@}%
 {\xyFN@\OBJECT@}}
\xydef@\afterDIRECTIONorEMPTY#1#2{%
 \DN@##1{\def\afterDIRECTION@{\def\afterDIRECTION@{##1}%
 \ifDIRECTIONempty@\DN@{#2}\else\DN@{#1}\fi \next@}}%
 \expandafter\next@\expandafter{\afterDIRECTION@}%
 \xyFN@\DIRECTION@}
\xylet@\afterDIRECTION@=\empty
\xynew@{if}\ifDIRECTIONempty@
\xydef@\DIRECTION@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\DIRECTION@}%
 \else\ifx v\next \DN@ v{\DIRECTION@v}%
 \else\ifx \bgroup\next \let\next@=\DIRECTION@group
 \else\ifx (\next \DN@({\xyFN@\DIRECTION@open}%
 \else
 \DN@{\count@=8
 \afterDIAG{\ifnum\count@=8 \DN@{\DIRECTIONempty@true \xyFN@\DIRECTION@i}%
 \else \DN@{\xy@@{\dimen@=\xydashl@}\Directionfromdiag@}\fi \next@}}%
 \fi\fi\fi\fi \next@}
\xydef@\DIRECTION@open{%
 \ifx *\next \DN@*##1*){\DIRECTION@group{##1}}%
 \else \DN@{\xyerror@{(* <pos> *) expected}{} \xyFN@\DIRECTION@i}%
 \fi \next@}
\def\afterDIAG#1{\def\afterDIAG@{#1}\xyFN@\DIAG@}
\xydef@\DIAG@{%
 \ifx d\next \DN@ d{\count@=1 \xyFN@\DIAG@@}%
 \else\ifx r\next \DN@ r{\count@=3 \xyFN@\DIAG@@}%
 \else\ifx u\next \DN@ u{\count@=5 \xyFN@\DIAG@@}%
 \else\ifx l\next \DN@ l{\count@=7 \xyFN@\DIAG@@}%
 \else \let\next@=\afterDIAG@
 \fi\fi\fi\fi \next@}
\xydef@\DIAG@@{\ifcase\count@ \or
 \DIAG@@@ l0r2\or\or \DIAG@@@ d2u4\or\or \DIAG@@@ r4l6\or\or \DIAG@@@ u6d0%
 \else\xybug@{impossible <diag> number}\fi
 \next@}
\xydef@\DIAG@@@#1#2#3#4{%
 \ifx #1\next \count@=#2\DN@#1{\afterDIAG@}%
 \else \ifx #3\next \count@=#4\DN@#3{\afterDIAG@}%
 \else \let\next@=\afterDIAG@ \fi\fi}
\xydef@\Directionfromdiag@{\ifcase\count@
 \xy@@{\dlDirection@\dimen@}%
 \or \xy@@{\dDirection@\dimen@}%
 \or \xy@@{\drDirection@\dimen@}%
 \or \xy@@{\rDirection@\dimen@}%
 \or \xy@@{\urDirection@\dimen@}%
 \or \xy@@{\uDirection@\dimen@}%
 \or \xy@@{\ulDirection@\dimen@}%
 \or \xy@@{\lDirection@\dimen@}%
 \or
 \else\xybug@{impossible <diag>}\fi
 \DIRECTIONempty@false \xyFN@\DIRECTION@i}
\xydef@\DIRECTION@v{%
 \xy@{v}{\enter@{\cfromthec@ \X@origin=\the\X@origin \Y@origin=\the\Y@origin
 \X@p=\the\X@p \Y@p=\the\Y@p}%
 \X@origin=\z@ \Y@origin=\z@}%
 \afterVECTORorEMPTY
 {\xy@@{\X@p=\z@ \Y@p=\z@ \setupDirection@ \leave@}%
 \DIRECTIONempty@false \xyFN@\DIRECTION@i}%
 {\xy@@\leave@ \xyerror@{<vector> expected after v}{}%
 \DIRECTIONempty@false \xyFN@\DIRECTION@i}}
\xydef@\DIRECTION@group#1{%
 \xy@@{\begingroup}\xy@@ix@{#1}\xy@@{\plainxy@\expandafter\POS\the\toks9\relax
 \setupDirection@\edef\next@{\endgroup \DirectionfromtheDirection@}\next@}%
 \DIRECTIONempty@false \xyFN@\DIRECTION@i}
\xydef@\DIRECTION@i{%
 \ifx ^\next \DN@ ^{\xy@^{\aboveDirection@\xydashl@}%
 \DIRECTIONempty@false \xyFN@\DIRECTION@i}%
 \else\ifx _\next \DN@ _{\xy@_{\belowDirection@\xydashl@}%
 \DIRECTIONempty@false \xyFN@\DIRECTION@i}%
 \else\ifx :\next \DN@ :{%
 \xy@{:}{\enter@{\cfromthec@ \basefromthebase@ \X@p=\the\X@p \Y@p=\the\Y@p}%
 \X@origin=\z@ \Y@origin=\z@
 \X@xbase=\cosDirection\xydashl@ \Y@xbase=\sinDirection\xydashl@
 \X@ybase=-\Y@xbase \Y@ybase=\X@xbase}%
 \afterVECTORorEMPTY
 {\xy@@{\X@p=\z@ \Y@p=\z@ \setupDirection@ \leave@}%
 \DIRECTIONempty@false \xyFN@\DIRECTION@i}%
 {\xy@@\leave@ \xyerror@{<vector> expected after :}{}%
 \DIRECTIONempty@false \xyFN@\DIRECTION@i}}%
 \else
 \let\next@=\afterDIRECTION@
 \fi\fi\fi \next@}
\message{decorations;}
\xydef@\drop#1#{\DN@##1{\xy@@ix@{{#1}{##1}}%
 \xy@{\drop#1{##1}}{\expandafter\drop@\the\toks9 }\ignorespaces}\next@}
\xydef@\connect#1#{\DN@##1{\xy@@ix@{{#1}{##1}}%
 \xy@{\connect#1{##1}}{\expandafter\connect@\the\toks9 }\ignorespaces}\next@}
\xydef@\preconnect#1#{\DN@##1{\xy@@ix@{{#1}{##1}}%
 \xy@{\connect#1{##1}}{\expandafter\preconnect@\the\toks9 }\ignorespaces}\next@}
\xydef@\save{\relax\saveC}
\xydef@\saveC{\xy@\save\save@ \POS}
\xydef@\save@{\enter@{\cfromthec@ \pfromthep@ \basefromthebase@}}
\xydef@\restore{\xy@\restore\leave@ \ignorespaces}
\xydef@\xyecho{%
 \xy@\xyecho{\let\xy@=\xyecho@ \message{\string\xyecho}}\POS}
\xydef@\xyecho@#1#2{{\def\1{#1}\ifx\1\empty\else\message{\codeof\1}\fi}%
 \oxy@{#1}{#2}}
\xydef@\xyverbose{%
 \xy@\xyverbose{\let\xy@=\xyverbose@
 \W@{Xy: \string\xyverbose\xytracelineno@}}\POS}
\xydef@\xyverbose@#1#2{%
 {\def\1{#1}\ifx\1\empty\else\W@{Xy: \codeof\1\xytracelineno@}\fi}%
 \oxy@{#1}{#2}}
\xydef@\xytracing{%
 \xy@\xytracing{\let\xy@=\xytracing@
 \W@{Xy TRACE: \string\xytracing\xytracelineno@}\xystatus@:}\POS}
\xydef@\xytracing@#1#2{{\def\1{#1}\def\2{#2}%
 \W@{Xy TRACE: \codeof\1 {\codeof\2}\xytracelineno@}}\oxy@{#1}{#2}\xystatus@:}
\xydef@\xystatus@#1{\xystatus@cp{#1}%
 \W@{#1 d=<\the\d@X,\the\d@Y>
 Direction=\the\Direction=\string(\cosDirection,\sinDirection\string)}%
 \W@{#1 base=<\the\X@origin,\the\Y@origin>+%
 <\the\X@xbase,\the\Y@xbase>x+<\the\X@ybase,\the\Y@ybase>y}%
 \W@{#1 min/max=<\the\X@min,\the\Y@min>/<\the\X@max,\the\Y@max>
 S=\the\csp@}}
\xydef@\xystatus@cp#1{%
 \W@{#1 c=<\the\X@c,\the\Y@c> \expandafter\string\the\Edge@c
 \string[\the\L@c+\the\R@c,\the\D@c+\the\U@c\string]
 \ifInvisible@ I\fi\ifHidden@ H\fi}%
 \W@{#1 p=<\the\X@p,\the\Y@p> \expandafter\string\the\Edge@p
 \string[\the\L@p+\the\R@p,\the\D@p+\the\U@p\string]}}
\xydef@\xystatus@c#1{%
 \W@{#1<\the\X@c,\the\Y@c> \expandafter\string\the\Edge@c
 \string[\the\L@c+\the\R@c,\the\D@c+\the\U@c\string]}}
\xydef@\xyquiet{\xy@\xyquiet{\let\xy@=\oxy@}}
\xydef@\xyignore#1{\xy@\xyignore{\xyignore@{#1}}\ignorespaces}
\xydef@\xyignore@#1{{\let\xy@=\xyeat@ \change@oxy@\xy@ \POS#1\relax}}
\xydef@\xyeat@#1#2{}
\xydef@\xycompile@@{\jobname-}
\xydef@\xycompileno@@{0}
\xydef@\CompilePrefix#1{%
 \def\xycompile@@{#1}\xdef\xycompile@@{\codeof\xycompile@@}%
 \xdef\xycompileno@@{0}}
\xydef@\xycompile{%
 \count@=\xycompileno@@ \advance\count@\@ne
 \xdef\xycompileno@@{\ifnum10>\count@ 0\fi \the\count@}%
 \edef\next{\noexpand\xycompileto{\xycompile@@\xycompileno@@}}\next}
\xylet@\compilename@@=\empty
\xylet@\xyrecompile@@=\relax
\xydef@\xycompileto#1#2{%
 \if\inxy@ \DN@{\xy@@{\nter@{}}}%
 \else \DN@{\xy \xy@@{\nter@{\endxy}}}\fi \next@
 \ifxysaving@ \xyerror@{Compilations can not be nested}{}\fi
 \DN@{#1}\edef\compilename@@{\codeof\next@}\DNii@{#2}%
 \def\xyrecompile@@{recompiling TRUNCATED}%
 \expandafter\xyinputorelse@@\expandafter{\compilename@@.xyc}%
 {\def\xyrecompile@@{compiling to}}%
 \ifx\xyrecompile@@\relax \else \expandafter\xyrecompile@ \fi
 \xy@@\leave@ \ignorespaces}
\xydef@\xyrecompile@{%
 \message{(\xyrecompile@@\space\string`\compilename@@.xyc\string'}%
 \DN@{\immediate\openout\xywrite@=}\expandafter\next@\compilename@@.xyc
 \immediate\write\xywrite@{%
 \string\xycompiled{\compilename@@}%
 {\the\year/\the\month/\the\day\string:\the\time\xytracelineno@}%
 {Xy-pic \xyversion}\xycomment@}%
 \immediate\write\xywrite@{{\codeof\nextii@}\relax}%
 {\xysaving@ \expandafter\POS\nextii@ \relax}%
 \immediate\write\xywrite@{\string\xyendcompiled}%
 \immediate\closeout\xywrite@ \message{done)}%
 \expandafter\input\compilename@@.xyc
 \outlines@@\writeoutline@\writeoutline@}
\xydef@\xysaving@{\let\xy@=\xysave@ \change@oxy@\xy@
 \let\xy@@ix@=\xysave@@toksix@ \xysaving@true}
\xynew@{if}\ifxysaving@ \xysaving@false
\xydef@\xysave@#1#2{{\DN@{{#1}{#2}}%
 \immediate\write\xywrite@{\string\xy@\codeof\next@\xycomment@}}}
\xydef@\xysave@@toksix@#1{{\DN@{{#1}}%
 \immediate\write\xywrite@{\string\xy@@ix@\codeof\next@\relax}}}
\xywarnifdefined\xycomment@
{\catcode`\%=12 \catcode`\(=1 \catcode`\)=2 \gdef\xycomment@(%)}
\xydef@\xycompiled#1#2#3#4{\DN@{#1}\edef\next@{\codeof\next@}%
 \ifx\next@\compilename@@\else
 \xywarning@{This file does not contain the result of
 \string\xycompileto{\compilename@@}{...}^^J%
 but of \string\xycompileto{\next@}}\fi
 \edef\next{Xy-pic \xyversion}\DN@{#3}\ifx\next\next@
 \DN@{#4}\ifx\next@\nextii@ \xycatcodes \outlines@@\relax\readoutline@
 \else \def\xyrecompile@@{recompiling to}\endinput \fi
 \else \def\xyrecompile@@{Xy-pic version change - recompiling}\endinput \fi}
\xydef@\xyendcompiled{\let\xyrecompile@@=\relax \xyuncatcodes\endinput}
\xydef@\CompileFixPoint#1{%
 \expandafter\ifx\csname#1FIX@@\endcsname\relax
 \expandafter\xdef\csname#1FIX@@\endcsname{\xycompileno@@}%
 \else
 \xdef\xycompileno@@{\csname#1FIX@@\endcsname}\fi}
\xydef@\outlines@no#1#2{}
\xydef@\outlines@make#1#2{#1}
\xydef@\outlines@only#1#2{#2}
\xylet@\outlines@@=\outlines@no
\xylet@\writeoutline@@=\relax
\xylet@\readoutline@@=\relax
\xydef@\MakeOutlines{\let\outlines@@=\outlines@make}
\xydef@\OnlyOutlines{\xywarning@{Compiled pictures only shown as outlines}%
 \let\outlines@@=\outlines@only}
\xydef@\ShowOutlines{\let\readoutline@@=\typesetoutline@}
\xydef@\NoOutlines{\let\outlines@@=\outlines@no}
\xydef@\writeoutline@{%
 \DN@{\immediate\openout\xywrite@=}\expandafter\next@\compilename@@.xyd
 \immediate\write\xywrite@{\xycomment@\space\compilename@@.xyd}
 \immediate\write\xywrite@{%
 \string\X@min=\the\X@min \string\X@max=\the\X@max
 \string\Y@min=\the\Y@min \string\Y@max=\the\Y@max \string\relax}%
 \writeoutline@@
 \immediate\closeout\xywrite@}
\xynew@{if}\ifoutlineread@
\xydef@\readoutline@{\outlineread@true
 \expandafter\xyinputorelse@@\expandafter{\compilename@@.xyd}%
 {\def\xyrecompile@@{outline missing - recompiling to}\outlineread@false}%
 \ifoutlineread@ \readoutline@@
 \writeoutline@\expandafter\xyendcompiled\fi}
\xydef@\typesetoutline@{%
 \xy@@{\czeroEdge@ \U@p=\z@ \D@p=\z@ \L@p=\z@ \R@p=\z@ \Edge@p={\zeroEdge}%
 \X@p=\X@min \Y@p=\Y@min \X@c=\X@min \Y@c=\Y@max \connect@\dir{.}%
 \X@p=\X@c \Y@p=\Y@c \X@c=\X@max \Y@c=\Y@max \connect@\dir{.}%
 \X@p=\X@c \Y@p=\Y@c \X@c=\X@max \Y@c=\Y@min \connect@\dir{.}%
 \X@p=\X@c \Y@p=\Y@c \X@c=\X@min \Y@c=\Y@min \connect@\dir{.}}}
\message{kernel objects:}
\message{directionals,}
\xydef@\dir{\hbox\bgroup\xyFN@\dir@i}
\xydef@\dir@i{\ifx *\next \DN@*{\resetStyle@\object@}%
 \else \let\next@=\dir@ii \fi \next@}
\xydef@\dir@ii#1#{\dir@{#1}}
\xydef@\dir@#1#2{\DN@{dir#1{#2}}%
 \expandafter\let\expandafter\next\csname\codeof\next@\endcsname
 \ifx\next\relax \DN@{dir{#2}}%
 \expandafter\let\expandafter\next\csname\codeof\next@\endcsname
 \ifx\next\relax \DN@{\dir#1{#2}}%
 \xyerror@{illegal <dir>: \codeof\next@\space not defined}{}%
 \let\next=\no@ \fi\fi \next}
\xydefcsname@{dir{}}{\no@}
\xyletcsnamecsname@{dir0{}}{dir{}}
\xyletcsnamecsname@{dir1{}}{dir{}}
\xyletcsnamecsname@{dir^{}}{dir{}}
\xyletcsnamecsname@{dir_{}}{dir{}}
\xyletcsnamecsname@{dir2{}}{dir{}}
\xyletcsnamecsname@{dir3{}}{dir{}}
\xyletcsnamecsname@{dir{ }}{dir{}}
\xydef@\no@{\egroup \czeroEdge@
 \def\Leftness@{.5}\def\Upness@{.5}%
 \def\Drop@@{\setbox\z@=\copy\voidb@x}\def\Connect@@{\no@@}}
\xydefcsname@{dir1{-}}{\line@}
\xydefcsname@{dir2{-}}{\line@ \double@\xydashh@}
\xydefcsname@{dir3{-}}{\line@ \triple@\xydashh@}
\xyletcsnamecsname@{dir0{-}}{dir{}}
\xyletcsnamecsname@{dir{-}}{dir1{-}}
\xyletcsnamecsname@{dir{=}}{dir2{-}}
\xydef@\line@{\dimen@=\sd@Y\sinDirection\xydashl@
 \ifnum\SemiDirectionChar<31 \D@c=\z@ \U@c=\dimen@ \DN@{\d@Y<\z@}%
 \else\ifnum\SemiDirectionChar<64 \D@c=\dimen@ \U@c=\z@ \DN@{\z@<\d@Y}%
 \else\ifnum\SemiDirectionChar<96 \D@c=\dimen@ \U@c=\z@ \DN@{\d@X<\z@}%
 \else \D@c=\z@ \U@c=\dimen@ \DN@{\d@X<\z@}\fi\fi\fi
 \setboxz@h{\line@@}\ht\z@=\U@c \dp\z@=\D@c
 \L@c=\z@ \R@c=\wdz@
 \ifdim\next@ \dimen@=\R@c \R@c=\L@c \L@c=\dimen@
 \dimen@=\U@c \U@c=\D@c \D@c=\dimen@ \advance\dimen@-\U@c
 \lower\dimen@\boxz@
 \else \boxz@ \fi
 \edef\tmp@{\egroup \U@c=\the\U@c \D@c=\the\D@c \L@c=\the\L@c \R@c=\the\R@c}%
 \tmp@
 \Edge@c={\rectangleEdge}%
 \ifdim\z@<\U@c \def\Upness@{1}\else \def\Upness@{0}\fi
 \ifdim\z@<\L@c \def\Leftness@{1}\else \def\Leftness@{0}\fi
 \def\Drop@@{\styledboxz@}\def\Connect@@{\solid@}}
\xydef@\line@@{{\xydashfont\SemiDirectionChar\/}}
\xydef@\solid@{%
 \checkXy@rules@\solidhrule@\solidvrule@{\straight@\solidSpread@}}
\xydef@\checkXy@rules@#1#2#3{%
 \dimen@=\Y@c \advance\dimen@-\Y@p
 \ifjusthvtest@.05pt>\ifdim\dimen@<\z@-\fi\dimen@ \DN@{#1}%
 \else \dimen@=\X@c \advance\dimen@-\X@p
 \ifjusthvtest@.05pt>\ifdim\dimen@<\z@-\fi\dimen@ \DN@{#2}%
 \else \DN@{#3}\fi\fi \next@}
\xydef@\solidSpread@{\ifnum\z@<\count@@ \advance\count@@\@ne \fi}
\xylet@\ifjusthvtest@=\ifdim
\xydef@\NoRules{\let\ifjusthvtest@=\iffalse}
\xydef@\UseRules{\let\ifjusthvtest@=\ifdim}
\xydef@\solidvrule@{\no@@ \solidvrule@typeset \ifHidden@\else\noinsert@\fi
 \solidvrule@pre}
\xydef@\solidvrule@pre{%
 \def\Cbreak@@{%
 \connectRestore@ \swap@\lastbreak@@\swap@
 \solidvrule@typeset \edef\lastbreak@@{\cfromthec@}\Creset@@}%
 \def\Clast@@{%
 \connectRestore@ \Creset@@\swap@\lastbreak@@\swap@
 \solidvrule@typeset \Creset@@ \edef\lastbreak@@{\cfromthep@}}%
}
\xydef@\solidvrule@typeset{%
 \ifInvisible@ \let\next@=\relax \else \let\next@=\solidvrule@typeset@ \fi
 \checkoverlap@@ \next@}
\xydef@\solidvrule@typeset@{{%
 \advance\X@c\X@p \X@c=.5\X@c \X@p=\X@c
 \advance\X@c-.5\xydashw@ \advance\X@p.5\xydashw@
 \ifdim\Y@c<\Y@p \advance\Y@c\U@c \advance\Y@p-\D@p
 \else \swapdimen@\Y@c\Y@p \advance\Y@c\U@p \advance\Y@p-\D@c \fi
 \Droprule@}}
\xydef@\solidhrule@{\no@@ \solidhrule@typeset \ifHidden@\else\noinsert@\fi
 \solidhrule@pre}
\xydef@\solidhrule@pre{%
 \def\Cbreak@@{%
 \connectRestore@ \swap@\lastbreak@@\swap@
 \solidhrule@typeset \edef\lastbreak@@{\cfromthec@}\Creset@@}%
 \def\Clast@@{%
 \connectRestore@ \Creset@@\swap@\lastbreak@@\swap@
 \solidhrule@typeset \Creset@@ \edef\lastbreak@@{\cfromthep@}}%
}
\xydef@\solidhrule@typeset{%
 \ifInvisible@ \let\next@=\relax \else \let\next@=\solidhrule@typeset@ \fi
 \checkoverlap@@ \next@}
\xydef@\solidhrule@typeset@{{%
 \ifdim\X@c<\X@p \advance\X@c\R@c \advance\X@p-\L@p
 \else \swapdimen@\X@c\X@p \advance\X@c\R@p \advance\X@p-\L@c \fi
 \advance\Y@c\Y@p \Y@c=.5\Y@c \Y@p=\Y@c
 \advance\Y@c-.5\xydashw@ \advance\Y@p.5\xydashw@
 \Droprule@}}
\xydef@\Droprule@{\advance\X@p-\X@c
 \setboxz@h{\kern\X@c \vrule width\X@p depth-\Y@c height\Y@p}%
 \ht\z@=\z@ \wd\z@=\z@ \dp\z@=\z@ \Drop@@}
\xydef@\zerodot{\copy\zerodotbox@}
\xydefcsname@{dir1{.}}{\point@}
\xydefcsname@{dir2{.}}{\point@ \double@\xydashh@}
\xydefcsname@{dir3{.}}{\point@ \triple@\xydashh@}
\xyletcsnamecsname@{dir0{.}}{dir{}}
\xyletcsnamecsname@{dir{.}}{dir1{.}}
\xyletcsnamecsname@{dir{:}}{dir2{.}}
\xydef@\point@{\pointlike@\zerodot\p@}
\xydef@\pointlike@#1#2{%
 \setboxz@h{#1}\wdz@=\z@ \ht\z@=\z@ \dp\z@=\z@ \boxz@\egroup
 \def\Leftness@{.5}\def\Upness@{.5}\ctipEdge@
 \def\Drop@@{\styledboxz@}\def\Connect@@{\straight@{\dottedSpread@{#2}}}}
\xydef@\dottedSpread@#1{%
 \dimen@=#1\relax \DN@{\A@=2\A@ \B@=2\B@ \dottedSpread@i}%
 \A@=\sd@X\cosDirection\dimen@ \B@=\sd@Y\sinDirection\dimen@
 \dimen@=\A@ \advance\dimen@\B@
 \dimen@ii=\sd@X\d@X \advance\dimen@ii\sd@Y\d@Y
 \ifdim\dimen@>\dimen@ii \DN@{\count@@=\z@}\fi
 \next@}
\xydef@\dottedSpread@i{%
 \global\setbox8=\hbox to\A@{\hss
 \kern.5\A@\box\lastobjectbox@\kern.5\A@\hss}\dp8=.5\B@ \ht8=.5\B@
 \advance\d@X\sd@X\A@ \advance\d@Y\sd@Y\B@
 \advance\X@c\sd@X.5\A@ \advance\Y@c\sd@Y.5\B@
 \ifdim\sd@Y\d@Y<\sd@X\d@X \dimen@=\sd@X\d@X
 \ifdim\zz@\A@\else \divide\dimen@\A@ \fi \count@@=\dimen@
 \else \dimen@=\sd@Y\d@Y
 \ifdim\zz@\B@\else \divide\dimen@\B@ \fi \count@@=\dimen@
 \fi \advance\count@@\@ne}
\xydefcsname@{dir1{~}}{\squiggle@}
\xydefcsname@{dir2{~}}{\squiggle@ \double@\xybsqlh@}
\xydefcsname@{dir3{~}}{\squiggle@ \triple@\xybsqlh@}
\xyletcsnamecsname@{dir0{~}}{dir{}}
\xyletcsnamecsname@{dir{~}}{dir1{~}}
\xydef@\squiggle@{\xybsqlfont
 \dimen@=\sd@X\cosDirection\xybsqll@ \advance\dimen@.1\p@
 \dimen@ii=\sd@Y\sinDirection\xybsqll@
 \kern\dimen@\squiggle@@
 \edef\tmp@{\egroup \U@c=\the\dimen@ii \L@c=\the\dimen@}\tmp@
 \wdz@=2\L@c \R@c=\L@c \ht\z@=\U@c \D@c=\U@c \dp\z@=\U@c
 \Edge@c={\rectangleEdge}%
 \def\Leftness@{.5}\def\Upness@{.5}%
 \def\Drop@@{\styledboxz@}\def\Connect@@{\straight@\squiggledSpread@}}
\xydef@\squiggle@@{\DirectionChar \count@=\DirectionChar
 \advance\count@-64 \ifnum\count@<\z@ \advance\count@128 \fi \char\count@}
\xydef@\squiggledSpread@{%
 \dimen@=\d@X \advance\dimen@-\sd@X\count@@\A@ \advance\dimen@\sd@X.3\p@
 \advance\X@c-.5\dimen@ \advance\d@X-\dimen@
 \dimen@=\d@Y \advance\dimen@-\sd@Y\count@@\B@ \advance\dimen@\sd@Y.3\p@
 \advance\Y@c-.5\dimen@ \advance\d@Y-\dimen@}
\xydef@\double@#1{\edef\Drop@@{\dimen@=#1\relax
 \dimen@=.5\dimen@ \A@=-\sinDirection\dimen@ \B@=\cosDirection\dimen@
 \setboxz@h{\setbox2=\hbox{\kern\A@\raise\B@\copy\z@}%
 \dp2=\z@ \ht2=\z@ \wd2=\z@ \box2
 \setbox2=\hbox{\kern-\A@\raise-\B@ \noexpand\boxz@}%
 \dp2=\z@ \ht2=\z@ \wd2=\z@ \box2 }%
 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \noexpand\styledboxz@}}
\xydef@\triple@#1{\edef\Drop@@{\dimen@=#1\relax
 \A@=-\sinDirection\dimen@ \B@=\cosDirection\dimen@
 \setboxz@h{\setbox2=\hbox{\kern\A@\raise\B@\copy\z@}%
 \dp2=\z@ \ht2=\z@ \wd2=\z@ \box2
 \setbox2=\hbox{\kern-\A@\raise-\B@\copy\z@}%
 \dp2=\z@ \ht2=\z@ \wd2=\z@ \box2
 \dp\z@=\z@ \ht\z@=\z@ \wdz@=\z@ \noexpand\boxz@}%
 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \noexpand\styledboxz@}}
\xydefcsname@{dir1{--}}{\dash@}
\xydefcsname@{dir2{--}}{\dash@ \double@\xydashh@}
\xydefcsname@{dir3{--}}{\dash@ \triple@\xydashh@}
\xyletcsnamecsname@{dir0{--}}{dir{}}
\xyletcsnamecsname@{dir{--}}{dir1{--}}
\xyletcsnamecsname@{dir{==}}{dir2{--}}
\xydef@\dash@{\line@ \wdz@=2\wdz@ \ht\z@=2\ht\z@ \dp\z@=2\dp\z@
 \multiply\D@c\tw@ \multiply\U@c\tw@ \multiply\L@c\tw@ \multiply\R@c\tw@
 \def\Connect@@{\straight@\dashedSpread@}}
\xydef@\dashedSpread@{\ifnum\z@<\count@@ \advance\count@@\@ne \fi
 \advance\d@X\sd@X.5\A@ \advance\d@Y\sd@Y.5\B@
 \ifdim\z@<\d@X \advance\X@c.5\A@ \fi \advance\Y@c\sd@Y.5\B@}
\xydefcsname@{dir1{~~}}{\dashsquiggle@}
\xydefcsname@{dir2{~~}}{\dashsquiggle@ \double@\xybsqlh@}
\xydefcsname@{dir3{~~}}{\dashsquiggle@ \triple@\xybsqlh@}
\xyletcsnamecsname@{dir0{~~}}{dir{}}
\xyletcsnamecsname@{dir{~~}}{dir1{~~}}
\xydef@\dashsquiggle@{\squiggle@
 \multiply\D@c\tw@ \multiply\U@c\tw@ \multiply\L@c\tw@ \multiply\R@c\tw@
 \dimen@=\L@c \advance\dimen@\R@c \wdz@=\dimen@ \ht\z@=\U@c \dp\z@=\D@c
 \def\Connect@@{\straight@\dashsquiggledSpread@}}
\xydef@\dashsquiggledSpread@{\ifnum\z@<\count@@ \advance\count@@\@ne \fi
 \advance\X@c.5\A@ \advance\d@X.5\A@ \advance\Y@c.25\B@ \advance\d@Y.5\B@}
\xyletcsnamecsname@{dir1{..}}{dir{.}}
\xyletcsnamecsname@{dir2{..}}{dir2{.}}
\xyletcsnamecsname@{dir3{..}}{dir3{.}}
\xyletcsnamecsname@{dir{..}}{dir1{.}}
\xyletcsnamecsname@{dir{::}}{dir2{.}}
\xylet@\ctipEdge@=\czeroEdge@
\xydefcsname@{dir1{>}}{\tip@}
\xydefcsname@{dir^{>}}{\atip@}
\xydefcsname@{dir_{>}}{\btip@}
\xyletcsnamecsname@{dir0{>}}{dir{}}
\xyletcsnamecsname@{dir{>}}{dir1{>}}
\xydefcsname@{dir1{<}}{\reverseDirection@\tip@}
\xydefcsname@{dir^{<}}{\reverseDirection@\btip@}
\xydefcsname@{dir_{<}}{\reverseDirection@\atip@}
\xyletcsnamecsname@{dir0{<}}{dir{}}
\xyletcsnamecsname@{dir{<}}{dir1{<}}
\xydef@\tip@{\tip@x\tip@@}
\xydef@\atip@{\tip@x\atip@@}
\xydef@\btip@{\tip@x\btip@@}
\xydef@\tip@x#1{#1\egroup
 \ctipEdge@
 \def\Leftness@{.5}\def\Upness@{.5}%
 \def\Drop@@{\styledboxz@}\def\Connect@@{\straight@{\dottedSpread@\jot}}}
\xydef@\tip@@{\atip@@\btip@@}
\xydef@\atip@@{\xyatipfont\DirectionChar}
\xydef@\btip@@{\xybtipfont\DirectionChar}
\xydefcsname@{dir2{>}}{\Tip@}
\xydefcsname@{dir2{<}}{\reverseDirection@\Tip@}
\xydef@\Tip@{\kern2.5pt \vrule height2.5pt depth2.5pt width\z@
 \Tip@@ \kern2.5pt \egroup
 \U@c=2.5pt \D@c=2.5pt \L@c=2.5pt \R@c=2.5pt \Edge@c={\circleEdge}%
 \def\Leftness@{.5}\def\Upness@{.5}%
 \def\Drop@@{\styledboxz@}\def\Connect@@{\straight@{\dottedSpread@\jot}}}
\xydef@\Tip@@{\count@=\DirectionChar
 \advance\count@-4 \ifnum\count@<\z@ \advance\count@128 \fi
 \xyatipfont\char\count@
 \advance\count@ 8 \ifnum127<\count@ \advance\count@-128 \fi
 \xybtipfont\char\count@}
\xydefcsname@{dir3{>}}{\Ttip@}
\xydefcsname@{dir3{<}}{\composite@{}{:(-1,0)\dir3{>}}}
\xydef@\Ttip@{\kern3.2pt \vrule height3.2pt depth3.2pt width\z@
 \Ttip@@ \kern3.2pt \egroup
 \U@c=3.2pt \D@c=3.2pt \L@c=3.2pt \R@c=3.2pt \Edge@c={\circleEdge}%
 \def\Leftness@{.5}\def\Upness@{.5}%
 \def\Drop@@{\styledboxz@}\def\Connect@@{\straight@{\dottedSpread@\jot}}}
\xydef@\Ttip@@{%
 \setboxz@h\bgroup\reverseDirection@\line@ \wdz@=\z@ \ht\z@=\z@ \dp\z@=\z@
 \kern-\L@c \boxz@ \kern\L@c
 {\vDirection@(1,-.31)\xydashl@ \xyatipfont\char\DirectionChar}%
 {\vDirection@(1,+.31)\xydashl@ \xybtipfont\char\DirectionChar}}
\xydefcsname@{dir1{|}}{\stopper@}
\xydefcsname@{dir^{|}}{\aboveDirection@\xydashl@
 \shiftdir@\line@\z@ \pointlike@{}\xydashh@}
\xydefcsname@{dir_{|}}{\belowDirection@\xydashl@
 \shiftdir@\line@\z@ \pointlike@{}\xydashh@}
\xydefcsname@{dir2{|}}{\stopper@ \double@\xydashh@}
\xydefcsname@{dir3{|}}{\stopper@ \double@{2\xydashh@}}
\xyletcsnamecsname@{dir0{|}}{dir{}}
\xyletcsnamecsname@{dir{|}}{dir1{|}}
\xydef@\stopper@{\tip@x\stopper@@}
\xydef@\stopper@@{\setboxz@h{\count@=\SemiDirectionChar \advance\count@64
 \ifnum127<\count@ \advance\count@-128 \fi \xydashfont\char\count@\/}%
 \setboxz@h{\kern-.5\wdz@ \dimen@=\sd@Y\cosDirection\xydashl@ 
 \ifnum\SemiDirectionChar=95 \dimen@=\sd@X\sd@Y\dimen@ \fi
 \raise.5\dimen@\boxz@}%
 \wdz@=\z@ \ht\z@=\z@ \dp\z@=\z@ \boxz@}
\xydefcsname@{dir1{(}}{\hook@}
\xydefcsname@{dir^{(}}{\ahook@}
\xydefcsname@{dir_{(}}{\bhook@}
\xyletcsnamecsname@{dir0{(}}{dir{}}
\xyletcsnamecsname@{dir{(}}{dir1{(}}
\xydefcsname@{dir1{)}}{\reverseDirection@\hook@}
\xydefcsname@{dir^{)}}{\reverseDirection@\bhook@}
\xydefcsname@{dir_{)}}{\reverseDirection@\ahook@}
\xyletcsnamecsname@{dir0{)}}{dir{}}
\xyletcsnamecsname@{dir{)}}{dir1{)}}
\xydef@\hook@{\tip@x\hook@@}
\xydef@\hook@@{\setboxz@h{\xybsqlfont
 \vDirection@(1,-1){.707107\xybsqll@}%
 \hbox{\DirectionChar
 \kern-\d@Y\raise\d@X\hbox{\count@=\DirectionChar \advance\count@-32
 \ifnum\count@<\z@ \advance\count@128 \fi \char\count@}}}%
 \wdz@=\z@ \ht\z@=\z@ \dp\z@=\z@ \boxz@}
\xydef@\ahook@{\tip@x\ahook@@}
\xydef@\ahook@@{\setboxz@h{\xybsqlfont
 \vDirection@(1,-1){.707107\xybsqll@}\kern-\d@X
 \lower\d@Y\hbox{\DirectionChar
 \kern-\d@Y\raise\d@X\hbox{\count@=\DirectionChar \advance\count@-32
 \ifnum\count@<\z@ \advance\count@128 \fi \char\count@}}}%
 \wdz@=\z@ \ht\z@=\z@ \dp\z@=\z@ \boxz@}
\xydef@\bhook@{\tip@x\bhook@@}
\xydef@\bhook@@{\setboxz@h{\xybsqlfont
 \vDirection@(-1,-1){.707107\xybsqll@}\DirectionChar
 \kern\d@X\raise\d@Y\hbox{\count@=\DirectionChar \advance\count@-96
 \ifnum\count@<\z@ \advance\count@128 \fi \char\count@}}%
 \wdz@=\z@ \ht\z@=\z@ \dp\z@=\z@ \boxz@}
\xydefcsname@{dir^{'}}{\reverseDirection@\bturn@}
\xydefcsname@{dir_{'}}{\reverseDirection@\aturn@}
\xydefcsname@{dir^{`}}{\aturn@}
\xydefcsname@{dir_{`}}{\bturn@}
\xydef@\aturn@{\tip@x\aturn@@}
\xydef@\aturn@@{\setboxz@h{\xybsqlfont
 \vDirection@(1,-1){.707107\xybsqll@}\kern-\d@X
 \lower\d@Y\hbox{\DirectionChar}}%
 \wdz@=\z@ \ht\z@=\z@ \dp\z@=\z@ \boxz@}
\xydef@\bturn@{\tip@x\bturn@@}
\xydef@\bturn@@{\setboxz@h{\xybsqlfont
 \vDirection@(-1,-1){.707107\xybsqll@}\DirectionChar}%
 \wdz@=\z@ \ht\z@=\z@ \dp\z@=\z@ \boxz@}
\xydef@\newdir#1#{\newdir@{#1}}
\xydef@\newdir@#1#2#3{\xydefcsname@{dir#1{#2}}{\composite@{}{#3}}}
\xydef@\shiftdir@#1#2{%
 \setbox\z@=\hbox\bgroup#1\relax
 \setboxz@h{\dimen@ii=#2\relax
 \dimen@=-\cosDirection\dimen@ii \advance\dimen@-\L@c
 \kern\dimen@ \lower\sinDirection\dimen@ii\boxz@}%
 \wdz@\z@ \ht\z@=\z@ \dp\z@=\z@ \boxz@}
\xylet@\tipjot@=\jot
\xydefcsname@{dir1{>>}}{\shiftdir@\tip@\tipjot@ \tip@}
\xydefcsname@{dir^{>>}}{\shiftdir@\atip@\tipjot@ \atip@}
\xydefcsname@{dir_{>>}}{\shiftdir@\btip@\tipjot@ \btip@}
\xydefcsname@{dir2{>>}}{\composite@{}{h!/\tipjot@/\dir2{>}*\dir2{>}}}
\xydefcsname@{dir3{>>}}{\composite@{}{h!/\tipjot@/\dir3{>}*\dir3{>}}}
\xyletcsnamecsname@{dir0{>>}}{dir{}}
\xyletcsnamecsname@{dir{>>}}{dir1{>>}}
\xydefcsname@{dir1{<<}}{\reverseDirection@ \shiftdir@\tip@\tipjot@ \tip@}
\xydefcsname@{dir^{<<}}{\reverseDirection@ \shiftdir@\btip@\tipjot@ \btip@}
\xydefcsname@{dir_{<<}}{\reverseDirection@ \shiftdir@\atip@\tipjot@ \atip@}
\xydefcsname@{dir2{<<}}{\composite@{}{h!/-\tipjot@/\dir2{<}*\dir2{<}}}
\xydefcsname@{dir3{<<}}{\composite@{}{h!/-\tipjot@/\dir3{<}*\dir3{<}}}
\xyletcsnamecsname@{dir0{<<}}{dir{}}
\xyletcsnamecsname@{dir{<<}}{dir1{<<}}
\xydefcsname@{dir1{||}}{\shiftdir@\stopper@\xydashh@ \shiftdir@\stopper@\z@
 \pointlike@{}\jot}
\xydefcsname@{dir^{||}}{\shiftdir@{\aboveDirection@\xydashl@\line@}\xydashh@
 \shiftdir@{\aboveDirection@\xydashl@\line@}\z@ \pointlike@{}\jot}
\xydefcsname@{dir_{||}}{\shiftdir@{\belowDirection@\xydashl@\line@}\xydashh@
 \shiftdir@{\belowDirection@\xydashl@\line@}\z@ \pointlike@{}\jot}
\xydefcsname@{dir2{||}}{\shiftdir@\stopper@\xydashh@ \shiftdir@\stopper@\z@
 \pointlike@{}\jot \double@\xydashh@}
\xydefcsname@{dir3{||}}{\shiftdir@\stopper@\xydashh@ \shiftdir@\stopper@\z@
 \pointlike@{}\jot \double@{2\xydashh@}}
\xyletcsnamecsname@{dir0{||}}{dir{}}
\xyletcsnamecsname@{dir{||}}{dir1{||}}
\xydefcsname@{dir1{>|}}{\shiftdir@\stopper@\z@ \tip@}
\xydefcsname@{dir2{>|}}{\composite@{}{\dir2{>}*\dir2{|}}}
\xydefcsname@{dir3{>|}}{\composite@{}{\dir3{>}*\dir3{|}}}
\xyletcsnamecsname@{dir0{>|}}{dir{}}
\xyletcsnamecsname@{dir{>|}}{dir1{>|}}
\xydefcsname@{dir1{>>|}}{\shiftdir@\stopper@\z@ \shiftdir@\tip@\tipjot@ \tip@}
\xydefcsname@{dir2{>>|}}{\composite@{}{h!/\tipjot@/\dir2{>}*\dir2{>}*\dir2{|}}}
\xydefcsname@{dir3{>>|}}{\composite@{}{h!/\tipjot@/\dir3{>}*\dir3{>}*\dir3{|}}}
\xyletcsnamecsname@{dir0{>>|}}{dir{}}
\xyletcsnamecsname@{dir{>>|}}{dir1{>>|}}
\xydefcsname@{dir1{|<}}{\reverseDirection@ \shiftdir@\stopper@\z@ \tip@}
\xydefcsname@{dir2{|<}}{\reverseDirection@ \shiftdir@\stopper@\z@ \Tip@}
\xydefcsname@{dir3{|<}}{\reverseDirection@ \shiftdir@\stopper@\z@ \Ttip@}
\xyletcsnamecsname@{dir0{|<}}{dir{}}
\xyletcsnamecsname@{dir{|<}}{dir1{|<}}
\xydefcsname@{dir1{|<<}}{\reverseDirection@
 \shiftdir@\stopper@\z@ \shiftdir@\tip@\tipjot@ \tip@}
\xydefcsname@{dir2{|<<}}{%
 \composite@{}{h!/-\tipjot@/\dir2{<}*\dir2{<}*\dir2{|}}}
\xydefcsname@{dir3{|<<}}{%
 \composite@{}{h!/-\tipjot@/\dir3{<}*\dir3{<}*\dir3{|}}}
\xyletcsnamecsname@{dir0{|<<}}{dir{}}
\xyletcsnamecsname@{dir{|<<}}{dir1{|<<}}
\xydefcsname@{dir1{|-}}{\shiftdir@\stopper@\z@
 \shiftdir@\line@\z@ \pointlike@{}\jot}
\xydefcsname@{dir^{|-}}{\shiftdir@{\aboveDirection@\xydashl@ \line@}\z@
 \shiftdir@\line@\z@ \pointlike@{}\jot}
\xydefcsname@{dir_{|-}}{\shiftdir@{\belowDirection@\xydashl@ \line@}\z@
 \shiftdir@\line@\z@ \pointlike@{}\jot}
\xydefcsname@{dir2{|-}}{\shiftdir@\stopper@\z@
 \shiftdir@\line@\z@ \pointlike@{}\jot \double@\xydashh@}
\xydefcsname@{dir3{|-}}{\shiftdir@\stopper@\z@
 \shiftdir@\line@\z@ \pointlike@{}\jot \triple@\xydashh@}
\xyletcsnamecsname@{dir0{|-}}{dir{}}
\xyletcsnamecsname@{dir{|-}}{dir1{|-}}
\xyletcsnamecsname@{dir{|=}}{dir2{|-}}
\xydefcsname@{dir{+}}{%
 \DN@##1{\composite@{}{##10\dir{|}*!C##10\dir{-}}}\addEQ@\next@}
\xyletcsnamecsname@{dir0{+}}{dir{}}
\xydefcsname@{dir{x}}{\vDirection@(1,1)\jot
 \DN@##1{\composite@{}{##10\dir{|}*!C##10\dir{-}}}\addEQ@\next@}
\xyletcsnamecsname@{dir0{x}}{dir{}}
\xydefcsname@{dir{/}}{\vDirection@(1,-.3)\jot \stopper@}
\xyletcsnamecsname@{dir0{/}}{dir{}}
\xydefcsname@{dir{//}}{\vDirection@(1,-.3)\jot
 \shiftdir@\stopper@\xydashh@ \stopper@}
\xyletcsnamecsname@{dir0{//}}{dir{}}
\xydefcsname@{dir{*}}{\solidpoint@}
\xydef@\solidpoint@{%
 \pointlike@{\kern-1.8pt\lower1.8pt\hbox{$\scriptstyle\bullet$}}\jot}
\xyletcsnamecsname@{dir0{*}}{dir{}}
\xydefcsname@{dir{o}}{\hollowpoint@}
\xydef@\hollowpoint@{%
 \pointlike@{\kern-1.8pt\lower1.8pt\hbox{$\scriptstyle\circ$}}\jot}
\xyletcsnamecsname@{dir0{o}}{dir{}}
\message{circles,}
\xydef@\cir#1#{\hbox\bgroup
 \afterVECTORorEMPTY{\xy@@{\R@=\X@c}\cir@}{\xy@@{\R@=\R@c}\cir@}#1@}
\xydef@\cir@#1@#2{%
 \DN@{#1}\ifx\next@\empty\else \xyerror@{illegal circle <radius>: must be
 <vector> or <empty>}{}\fi
 \afterCIRorDIAG{\xyFN@\cir@cir}{\xyFN@\cir@diag}#2@}
\xydef@\cir@cir{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\cir@cir}%
 \else \ifx @\next \DN@ @{\cir@i}%
 \else \xyerror@{illegal <cir>: must have form <diag><orient><diag> or
 <empty>}{}%
 \fi\fi \next@}
\xydef@\cir@diag{%
 \DN@{\xyerror@{illegal <cir>: must have form <diag><orient><diag> or
 <empty>}{}}%
 \ifx @\next \ifnum\count@=8
 \DN@ @{\def\CIRin@@{0}\def\CIRorient@@{\CIRfull@}\def\CIRout@@{7}\cir@i}%
 \fi\fi \next@}
\xydef@\cir@i{%
 \ifnum\CIRin@@=8 \xyerror@{incomplete <cir> specification}{%
The <cir> you specified as <diag><orient><diag> is not sufficiently specific.}%
 \def\CIRin@@{0}\fi
 \ifdim\R@<.5\p@ \R@=\z@ \zerodot
 \else \CIRorient@@ \cirbuild@ \fi
 \L@c=\R@ \R@c=\R@ \D@c=\R@ \U@c=\R@ \def\Leftness@{.5}\def\Upness@{.5}%
 \def\Drop@@{\styledboxz@}\def\Connect@@{\straight@\relax}%
 \Edge@c={\circleEdge}\OBJECT@x}
\xydef@\CIRin@@{3}
\xydef@\CIRout@@{3}
\xylet@\CIRorient@@=\empty
\xydef@\afterCIRorDIAG#1#2{\def\afterCIR@{#1}\def\afterCIRDIAG@{#2}\xyFN@\CIR@}
\xylet@\afterCIR@=\empty
\xylet@\afterCIRDIAG@=\empty
\xydef@\CIR@{\count@=8 \afterDIAG{\edef\CIRin@@{\the\count@}\xyFN@\CIR@@}}
\xydef@\CIR@@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\CIR@@}%
 \else\ifx ^\next
 \DN@ ^{\def\CIRorient@@{\CIRacw@}%
 \afterDIAG{\edef\CIRout@@{\the\count@}\afterCIR@}}%
 \else\ifx _\next
 \DN@_{\def\CIRorient@@{\CIRcw@}%
 \afterDIAG{\edef\CIRout@@{\the\count@}\afterCIR@}}%
 \else
 \DN@{\def\CIRorient@@{\relax}\afterCIRDIAG@}%
 \fi\fi\fi \next@}
\xylet@\CIRtest@@=\relax
\xydef@\CIRlo@@{0}
\xydef@\CIRhi@@{0}
\xydef@\CIRfull@{\def\CIRtest@@##1##2{##2}}
\xydef@\cirbuild@{\cirrestrict@@ \multiply\count@8
 \circhar@0\circhar@7\kern\dimen@
 \circhar@1\circhar@6\kern\dimen@
 \circhar@2\circhar@5\kern\dimen@
 \circhar@3\circhar@4\kern\dimen@}
\xydef@\circhar@#1{%
 \setboxz@h{\circhar@@{#1}}\dimen@=\wdz@ \wdz@=\z@ \ht\z@=\R@ \dp\z@=\R@
 \CIRtest@@#1{\styledboxz@}\setbox\z@=\copy\voidb@x}
\xydef@\circhar@@#1{{\xycircfont \advance\count@#1\relax \char\count@}}
\xydef@\cirrestrict@@{\begingroup \dimen@=\R@
 \setboxz@h{\xycircfont\char\z@\char\@ne}\A@=\wdz@
 \ifdim\R@<8\A@ \count@=\dimen@ \divide\count@\A@ \advance\count@\m@ne
 \else\ifdim\R@<16\A@ \count@=\dimen@
 \dimen@=2\A@ \divide\count@\dimen@ \advance\count@3
 \else\ifdim\R@<32\A@ \count@=\dimen@
 \dimen@=4\A@ \divide\count@\dimen@ \advance\count@7
 \else \count@=15 \fi\fi\fi
 \R@=\A@
 \ifnum\count@<8 \multiply\R@\count@ \advance\R@\A@
 \else\ifnum\count@<12 \multiply\R@\count@ \multiply\R@\tw@ \advance\R@-6\A@
 \else\ifnum\count@<16 \multiply\R@\count@ \multiply\R@ 4 \advance\R@-28\A@
 \else \multiply\R@ 32 \fi\fi\fi
 \edef\@tmp{\endgroup \R@=\the\R@ \count@=\the\count@}\@tmp}
\xydef@\CIRacw@{\count@@=\CIRin@@ \count@=\CIRout@@
 \ifnum\count@=8 \count@=\count@@
 \ifnum\count@<6 \advance\count@\tw@ \else \advance\count@-6 \fi \fi
 \ifnum\count@@<\@ne \advance\count@@7 \else \advance\count@@\m@ne \fi
 \ifnum\count@<\@ne \advance\count@7 \else \advance\count@\m@ne \fi
 \ifnum\count@@>\count@ \let\CIRtest@@=\CIRtest@outside
 \edef\CIRlo@@{\the\count@}\edef\CIRhi@@{\the\count@@}%
 \else \let\CIRtest@@=\CIRtest@inside
 \edef\CIRlo@@{\the\count@@}\edef\CIRhi@@{\the\count@}%
 \fi}
\xydef@\CIRcw@{\count@@=\CIRin@@ \count@=\CIRout@@
 \ifnum\count@=8 \count@=\count@@
 \ifnum\count@>\@ne \advance\count@-\tw@ \else \advance\count@6 \fi \fi
 \ifnum\count@@<5 \advance\count@@\thr@@ \else \advance\count@@-5 \fi
 \ifnum\count@<5 \advance\count@\thr@@ \else \advance\count@-5 \fi
 \ifnum\count@@<\count@ \let\CIRtest@@=\CIRtest@outside
 \edef\CIRlo@@{\the\count@@}\edef\CIRhi@@{\the\count@}%
 \else \let\CIRtest@@=\CIRtest@inside
 \edef\CIRlo@@{\the\count@}\edef\CIRhi@@{\the\count@@}%
 \fi}
\xydef@\CIRtest@inside#1#2{\let\next@=\relax
 \ifnum\CIRlo@@>#1\else \ifnum#1<\CIRhi@@\DN@{#2}\fi\fi \next@}
\xydef@\CIRtest@outside#1#2{\let\next@=\relax
 \ifnum\CIRlo@@>#1\DN@{#2}\else \ifnum#1<\CIRhi@@\else\DN@{#2}\fi\fi \next@}
\message{text;}
\xydef@\txt{\hbox\bgroup \xyFN@\txt@}
\xydef@\txt@{%
 \addLT@\ifx\next \addGT@{\addLT@\DN@##1}{\A@=##1\txt@i}%
 \else \DN@{\A@=\maxdimen \txt@i}\fi \next@}
\xydef@\txt@i#1#{%
 \setboxz@h{#1\mathstrut}\dimen@=\ht\z@ \advance\dimen@\dp\z@
 \baselineskip=1.1\dimen@ \lineskip=.2\dimen@ \lineskiplimit=\lineskip
 \def\txtline@@##1{\txtline@{#1}{##1}}\object@\txt@ii}
\xylet@\txtline@@=\eat@
\xydef@\txtline@#1#2{\relax\setboxz@h{#1{\ignorespaces #2\unskip}}%
 \ifdim\A@<\wdz@ \setboxz@h{\hsize=\A@
 \leftskip=0pt plus4em \rightskip=\leftskip
 \parfillskip=0pt \parindent=0pt
 \spaceskip=.3333em \xspaceskip=.5em
 \pretolerance=9999 \tolerance=9999
 \hyphenpenalty=9999 \exhyphenpenalty=9999
 \vbox{#1\noindent\ignorespaces #2\unskip}}%
 \else\ifdim\A@<\maxdimen\setboxz@h to\A@{\hfil\boxz@\hfil}\fi\fi
 \boxz@}
\xydef@\txt@ii#1{\vbox{%
 \let\\=\cr
 \tabskip=\z@skip \halign{\relax\hfil\txtline@@{##}\hfil\cr\leavevmode#1\crcr}}}
\message{options;}
\xylet@\xyoption@@=\relax
\xydef@\xyoption#1{\DN@{#1}\edef\next@{\codeof\next@}%
 \csname xyeveryrequest@\next@ @\endcsname
 \xyinputorelse@{xy#1}{\xyoption@truncated#1@@@@@@@@@,#1@}%
 \def\xyoption@@{#1}\edef\xyoption@@{\codeof\xyoption@@}
 \expandafter\let\expandafter\next@\csname xy\xyoption@@ version\endcsname
 \expandafter\let\csname xy\xyoption@@ loaded\endcsname=\next@
 \runxywith@ \ignorespaces}
\xydef@\xyoption@truncated#1#2#3#4#5#6#7@#8,#9@{%
 \DN@{#7}\ifx\next@\empty \DN@##1##2{##2}\else\let\next@=\xyinputorelse@ \fi
 \next@{xy#1#2#3#4#5#6}%
 {\DN@{#1#2#3#4#5#6}\edef\next@{\codeof\next@}%
 \xyerror@{No `\next@' option}{%
Your \xyoption{#9} request could not be granted: the required^^J%
file `xy#9.tex' could not be located. Please make sure that it is^^J%
properly installed before continuing.}}}
\xydef@\xyrequire#1{\DN@{#1}\edef\next@{\codeof\next@}%
 \csname xyeveryrequest@\next@ @\endcsname
 \expandafter\let\expandafter\next@\csname xy\codeof\next@ loaded\endcsname
 \ifx \next@\relax \DN@{\xyoption{#1}}\else \DN@{\ignorespaces}\fi \next@}
\xylet@\xywith@@=\empty
\xydef@\runxywith@{\let\xywithdo@@=\xywithtest@ \xywith@@}
\xydef@\xywithoption#1#2{\DN@{#1}\edef\next@{\codeof\next@}%
 \expandafter\let\expandafter\nextii@\csname xy\next@ loaded\endcsname
 \ifx \nextii@\relax
 \expandafter\def\expandafter\xywith@@\expandafter{\xywith@@ 
 \xywithdo@@{#1}{#2}}%
 \else \expandafter\xywithrun@\expandafter{\next@}{#2}\fi}
\xydef@\xywithtest@#1#2{\DN@{#1}\edef\next@{\codeof\next@}%
 \ifx\next@\xyoption@@ \expandafter\xywithrun@\expandafter{\next@}{#2}\fi}
\xydef@\xywithrun@#1#2{\csname xyeverywithoption@#1@\endcsname #2}
\xydef@\xyevery@#1#2#3{\DN@{#2}\edef\next@{\codeof\next@}%
 \expandafter\ifx\csname xyevery#1@\next@ @\endcsname\relax
 \expandafter\let\csname xyevery#1@\next@ @\endcsname=\empty \fi
 \DNii@##1{\expandafter\def\expandafter##1\expandafter{##1#3}}%
 \expandafter\nextii@\csname xyevery#1@\next@ @\endcsname}
\xydef@\xyeveryrequest{\xyevery@{request}}
\xydef@\xyeverywithoption{\xyevery@{withoption}}
\xydef@\xyprovide#1#2#3#4#5#6{%
 \def\xyoption@@{#1}\edef\xyoption@@{\codeof\xyoption@@}\edef\next@{#3}%
 \message{ Xy-pic option: #2 v.\next@}%
 \expandafter\let\expandafter\nextii@\csname xy\xyoption@@ loaded\endcsname
 \ifx \next@\nextii@ \message{not reloaded}\endinput
 \else
 \ifx \nextii@\relax\else \xyerror@{Option `\xyoption@@' version mismatch}{%
You previously loaded, or the format has preloaded, a different version^^J%
of this option. Just continue to try to load this version instead (and^^J%
be prepared for a lot of warnings about redefinitions).}%
 \fi
 \expandafter\let\csname xy\xyoption@@ version\endcsname=\next@
 \expandafter\let\expandafter\xyenddocmode@\csname DOCMODE\endcsname
 \expandafter\let\csname DOCMODE\endcsname\xyprovidedocmode@
 \xycatcodes
 \fi \ignorespaces}
\xydef@\xyendinput{\expandafter\let\csname DOCMODE\endcsname=\xyenddocmode@
 \message{loaded}\xyuncatcodes\endinput}
\expandafter\xylet@\expandafter\xyprovidedocmode@\csname DOCMODE\endcsname
\xylet@\xyenddocmode@=\relax
\xydef@\xydriversloaded@@{\do{unload}}
\xylet@\xydriversselected@@=\empty
\xylet@\xydriver@unload@support@@=\empty
\xydef@\selectdriver@#1{\DN@{#1}\edef\next@{\codeof\next@}%
 \expandafter\selectdriver@@\expandafter{\next@}}
\xydef@\selectdriver@single#1{\xysetup@@{\def\xydriversselected@@{\do{#1}}%
 \xyLoadDrivers@}\let\selectdriver@@=\changedriver@single}
\xydef@\changedriver@single#1{\xysetup@@{\def\xydriversselected@@{\do{#1}}%
 \xyReloadDrivers@}}
\xydef@\selectdriver@multiple#1{\expandafter\xysetup@@\expandafter{%
 \expandafter\def\expandafter\xydriversselected@@\expandafter{%
 \xydriversselected@@ \do{#1}}%
 \let\do=\activatedriver@ \xydriversselected@@}}
\xydef@\UseSingleDriver{\let\selectdriver@@=\selectdriver@single}
\xydef@\MultipleDrivers{\let\selectdriver@@=\selectdriver@multiple}
\xydef@\xyLoadDrivers@{\let\do=\activatedriver@ \xydriversselected@@}
\xydef@\xyReloadDrivers@{\activatedriver@{unload}\xyLoadDrivers@}
\xylet@\xyReloadDrivers=\xyReloadDrivers@
\xydef@\activatedriver@#1{%
 \let\doii=\activatedriversupport@ \csname xydriver@#1@support@@\endcsname}
\xydef@\activatedriversupport@#1#2{%
 \expandafter\ifx\csname xy#1loaded\endcsname\relax\DN@{}%
 \else\DN@{#2}\fi \next@}
\UseSingleDriver
\xydef@\xyselectoptionsupport@{\let\do=\activatedriver@ \xydriversselected@@}
\xydef@\xyShowDrivers{{\W@{Loaded:}\let\do=\doShow \xydriversloaded@@
 \let\next@=\empty
 \def\do##1{\ifx\next@\empty \DN@{##1}%
 \else \expandafter\DN@\expandafter{\next@, ##1}\fi}%
 \xydriversselected@@\W@{Selected: \next@.}}}
\def\doShow#1{\let\next@=\empty
 \def\doii##1##2{\ifx\next@\empty \DN@{##1}%
 \else \expandafter\DN@\expandafter{\next@, ##1}\fi}%
 \csname xydriver@#1@support@@\endcsname
 \W@{ <driver> #1 supports \next@.}}
\xydef@\newdriver#1{%
 \def\nextiii@##1{%
 \expandafter\def\expandafter\xydriversloaded@@
 \expandafter{\xydriversloaded@@\do{##1}}%
 \expandafter\let\csname xydriver@\xyoption@@ @support@@\endcsname=\empty}%
 \def\do##1{\DNii@{##1}\ifx\xyoption@@\nextii@ \let\nextiii@=\eat@ \fi}%
 \xydriversloaded@@ \expandafter\nextiii@\expandafter{\xyoption@@}%
 #1\relax
 \DN@##1{\xywithoption{##1}{%
 \selectdriver@{##1}\xyeveryrequest{##1}{\selectdriver@{##1}}}}%
 \expandafter\next@\expandafter{\xyoption@@}\ignorespaces}
\xydef@\xyaddsupport{\expandafter\xyadddriversupport@\expandafter{\xyoption@@}}
\xydef@\xyaddunsupport{\xyadddriversupport@{unload}}
\xydef@\xyadddriversupport@#1#2#3{%
 \DNii@{#1}\edef\nextii@{\codeof\nextii@}%
 \def\nextiii@{#2}\edef\nextiii@{\codeof\nextiii@}%
\def\next{\xybug@{<driver> \nextii@\space not loaded}}%
\def\do##1{\DN@{##1}\edef\next@{\codeof\next@}%
 \ifx\next@\nextii@ \let\next=\relax \fi}\xydriversloaded@@ \next
\def\next{\xybug@{<driver> \nextii@\space already supports \nextiii@}}%
\def\doii##1##2{\DN@{##1}\edef\next@{\codeof\next@}%
 \ifx\next@\nextiii@ \let\next=\relax \fi}\xydriversloaded@@ \next
 \DN@##1##2{\ifx##1\relax \let##1=\empty \fi
 \expandafter\def\expandafter##1\expandafter{##1\doii{##2}{#3}}}%
 \expandafter\expandafter\expandafter\next@
 \expandafter\expandafter\csname xydriver@\nextii@ @support@@\endcsname
 \expandafter{\nextiii@}%
 \DN@##1{\expandafter\xyeverywithoption\expandafter{\nextiii@}{%
 \xytestforsupport@{##1}}}%
 \expandafter\next@\expandafter{\nextii@}\xydriversloaded@@
 \ignorespaces}
\xydef@\xytestforsupport@#1{\def\do##1{\DN@{##1}\DNii@{#1}%
 \ifx\next@\nextii@ \expandafter\xyselectoptionsupport@ \fi}}
\xynew@{if}\ifunsupportwarnings@
\xydef@\xyunsupportwarning@#1#2{{%
 \DN@{#1}\edef\next@{\codeof\next@}
 \expandafter\ifx\csname xywarn@unload@\next@ @\endcsname\relax
 \expandafter\gdef\csname xywarn@unload@\next@ @\endcsname{}%
 \ifunsupportwarnings@ \xyclosedown@@\xyunsupportwarnings@@ \fi
 \global\unsupportwarnings@true
 \expandafter\gdef\expandafter\xyunsupportwarnings@@\expandafter{%
 \xyunsupportwarnings@@ \W@{ #2.}}%
 \W@{}%
 \W@{Xy-pic Warning: `\next@' reproduction is NOT EXACT\xytracelineno@:}%
 \W@{ #2.}%
 \W@{}%
 \fi}}
\xydef@\xyunsupportwarnings@@{\W@{}%
 \W@{Xy-pic Warning: The produced DVI file is NOT EXACT:}}
\xynew@{if}\ifsupportwarnings@
\xydef@\xysupportwarning@#1#2{{%
 \DN@{#1}\edef\next@{\codeof\next@}\DNii@{#2}\edef\nextii@{\codeof\nextii@}%
 \expandafter\ifx\csname xywarn@\next@ @\nextii@ @\endcsname\relax
 \expandafter\gdef\csname xywarn@\next@ @\nextii@ @\endcsname{}%
 \ifsupportwarnings@ \xyclosedown@@\xysupportwarnings@@ \fi
 \global\supportwarnings@true
 \expandafter\gdef\expandafter\xysupportwarnings@@\expandafter{%
 \xysupportwarnings@@ \driverextensioncomplain@{#1}{#2}}%
 \W@{}%
 \W@{Xy-pic Warning: The produced DVI file is NOT PORTABLE\xytracelineno@:}%
 \driverextensioncomplain@{#1}{#2}%
 \W@{}%
 \fi}}
\xydef@\xysupportwarnings@@{%
 \W@{Xy-pic Warning: The produced DVI file is NOT PORTABLE:}}
\xydef@\driverextensioncomplain@#1#2{%
 \DN@{#1}\edef\next@{\codeof\next@}\DNii@{#2}\edef\nextii@{\codeof\nextii@}%
 \W@{ It contains <driver> `\next@' \string\special s for the `\nextii@'
 extension.}}
\xydef@\dvimessage@#1#2{\xysupportwarning@{#1}{#2}}
\xynew@{if}\ifxydrivernoloads@
\xydef@\xydrivernoload@#1{\xyerror@{Could not load xy#1.tex}{}%
 \xydrivernoloads@true}
\xydef@\xydriverfail@#1{\xyerror@{Sorry, #1 not supported.}{}}
\xydef@\xyunload@#1{\xywarning@{Unloading #1.}}
\message{algorithms: directions,}
\xydef@\DirectionfromtheDirection@{\noexpand\Direction=\the\Direction
 \noexpand\d@X=\the\d@X \noexpand\d@Y=\the\d@Y
 \def\noexpand\sd@X{\sd@X}\def\noexpand\sd@Y{\sd@Y}%
 \noexpand\K@dXdY=\the\K@dXdY \noexpand\K@dYdX=\the\K@dYdX
 \chardef\noexpand\DirectionChar=\the\DirectionChar
 \chardef\noexpand\SemiDirectionChar=\the\SemiDirectionChar
 \def\noexpand\cosDirection{\cosDirection}%
 \def\noexpand\sinDirection{\sinDirection}%
 \noexpand\resetupDirection@}
\xydef@\Directiontest@@#1#2{#2}
\xydef@\setupDirection@{%
 \d@X=\X@c\advance\d@X-\X@p \d@Y=\Y@c\advance\d@Y-\Y@p
 \Directiontest@@\relax\setupDirection@i}
\xydef@\setupDirection@i{\DN@{\setupDirection@ii}%
 \ifdim\d@X=\d@Y
 \ifdim\zz@\d@Y \DN@{}%
 \else\ifdim\d@X<\z@ \DN@{\dlDirection@{-1.4142\d@X}}%
 \else \DN@{\urDirection@{1.4142\d@X}}\fi\fi
 \else\ifdim\d@X<\d@Y
 \ifdim\zz@\d@X \DN@{\uDirection@\d@Y}%
 \else\ifdim\zz@\d@Y \DN@{\lDirection@{-\d@X}}%
 \else\ifdim-\d@X=\d@Y \DN@{\ulDirection@{-1.4142\d@X}}\fi\fi\fi
 \else
 \ifdim\zz@\d@X \DN@{\dDirection@{-\d@Y}}%
 \else\ifdim\zz@\d@Y \DN@{\rDirection@\d@X}%
 \else\ifdim\d@X=-\d@Y \DN@{\drDirection@{1.4142\d@X}}\fi\fi\fi
 \fi\fi \next@}
\xydef@\dlDirection@{\Direction=\z@
 \def\cosDirection{-.7071}\def\sinDirection{-.7071}\def\sd@X{-}\def\sd@Y{-}%
 \chardef\DirectionChar=127\relax\chardef\SemiDirectionChar=127\relax
 \K@dXdY=1\K@ \K@dYdX=1\K@ \fixedDirection@}
\xydef@\dDirection@{\Direction=\K@
 \def\cosDirection{0}\def\sinDirection{-1}\def\sd@Y{-}%
 \edef\sd@X{\ifdim\X@c<\X@p-\else+\fi}%
 \chardef\DirectionChar=15\relax\chardef\SemiDirectionChar=31\relax
 \K@dXdY=\z@ \K@dYdX=\KK@\K@ \fixedDirection@}
\xydef@\drDirection@{\dimen@ii=2\K@ \Direction=\dimen@ii
 \def\cosDirection{+.7071}\def\sinDirection{-.7071}\def\sd@X{+}\def\sd@Y{-}%
 \chardef\DirectionChar=31\relax\chardef\SemiDirectionChar=63\relax
 \K@dXdY=-1\K@ \K@dYdX=-1\K@ \fixedDirection@}
\xydef@\rDirection@{\dimen@ii=3\K@ \Direction=\dimen@ii
 \def\cosDirection{+1}\def\sinDirection{0}\def\sd@X{+}%
 \edef\sd@Y{\ifdim\Y@c<\Y@p-\else+\fi}%
 \chardef\DirectionChar=47\relax\chardef\SemiDirectionChar=95\relax
 \K@dXdY=\KK@\K@ \K@dYdX=\z@ \fixedDirection@}
\xydef@\urDirection@{\dimen@ii=4\K@ \Direction=\dimen@ii
 \def\cosDirection{+.7071}\def\sinDirection{+.7071}\def\sd@X{+}\def\sd@Y{+}%
 \chardef\DirectionChar=63\relax\chardef\SemiDirectionChar=127\relax
 \K@dXdY=1\K@ \K@dYdX=1\K@ \fixedDirection@}
\xydef@\uDirection@{\dimen@ii=-3\K@ \Direction=\dimen@ii
 \def\cosDirection{0}\def\sinDirection{+1}\def\sd@Y{+}%
 \edef\sd@X{\ifdim\X@c<\X@p-\else+\fi}%
 \chardef\DirectionChar=79\relax\chardef\SemiDirectionChar=31\relax
 \K@dXdY=\z@ \K@dYdX=\KK@\K@ \fixedDirection@}
\xydef@\ulDirection@{\dimen@ii=-2\K@ \Direction=\dimen@ii
 \def\cosDirection{-.7071}\def\sinDirection{+.7071}\def\sd@X{-}\def\sd@Y{+}%
 \chardef\DirectionChar=95\relax\chardef\SemiDirectionChar=63\relax
 \K@dXdY=-1\K@ \K@dYdX=-1\K@ \fixedDirection@}
\xydef@\lDirection@{\Direction=-\K@
 \def\cosDirection{-1}\def\sinDirection{0}\def\sd@X{-}%
 \edef\sd@Y{\ifdim\Y@c<\Y@p-\else+\fi}%
 \chardef\DirectionChar=111\relax\chardef\SemiDirectionChar=95\relax
 \K@dXdY=\KK@\K@ \K@dYdX=\z@ \fixedDirection@}
\xydef@\fixedDirection@#1{\dimen@ii=#1\relax
 \d@X=\cosDirection\dimen@ii \d@Y=\sinDirection\dimen@ii
 \resetupDirection@}
\xydef@\setupDirection@ii{%
 \ifdim\d@X<\z@ \def\sd@X{-}\else \def\sd@X{+}\fi
 \ifdim\d@Y<\z@ \def\sd@Y{-}\else \def\sd@Y{+}\fi
 \K@dXdY=\sd@X\d@X \ifdim\K@dXdY<500pt \multiply\K@dXdY\KK@ \fi
 \dimen@=\sd@Y\d@Y
 \advance\dimen@\ifdim\dimen@<\z@-\fi.5\KK@ \divide\dimen@\KK@
 \ifdim\dimen@=\z@\else
 \advance\K@dXdY by.5\dimen@\relax \divide\K@dXdY\dimen@
 \fi \K@dXdY=\sd@X\sd@Y\K@dXdY
 \K@dYdX=\sd@Y\d@Y \ifdim\K@dYdX<500pt \multiply\K@dYdX\KK@ \fi
 \dimen@=\sd@X\d@X
 \advance\dimen@\ifdim\dimen@<\z@-\fi.5\KK@ \divide\dimen@\KK@
 \ifdim\dimen@=\z@\else
 \advance\K@dYdX by.5\dimen@\relax \divide\K@dYdX\dimen@
 \fi \K@dYdX=\sd@X\sd@Y\K@dYdX
 \Direction=\maxdimen
 \ifnum\K@dXdY<-\K@ \else \ifnum\K@<\K@dXdY \else
 \ifdim \d@Y<\z@
 \Direction=\K@ \advance\Direction-\K@dXdY
 \else
 \Direction=\K@ \multiply\Direction-\thr@@ \advance\Direction-\K@dXdY
 \fi\fi\fi
 \ifnum-\K@<\K@dYdX \ifnum\K@dYdX<\K@
 \ifdim \d@X<\z@
 \Direction=-\K@ \advance\Direction\K@dYdX
 \else
 \Direction=\K@ \multiply\Direction\thr@@ \advance\Direction\K@dYdX
 \fi\fi\fi
 \ifnum\Direction=\maxdimen
 \Direction=\K@dYdX \advance\Direction-\K@dXdY 
 \advance\Direction\ifnum\Direction<\z@-\fi\@ne \divide\Direction\tw@ 
 \ifnum\K@dXdY<\z@ \advance\Direction\K@ \advance\Direction\K@
 \else \advance\Direction-\K@ \advance\Direction-\K@ \fi
 \fi
 \imposeDirection@i
 \resetupDirection@
 }
\xydef@\imposeDirection@{\count@@=\Direction 
 \loop@\ifnum\count@@>4096 \advance\count@@-8192 \repeat@
 \loop@\ifnum\count@@<-4096 \advance\count@@8192 \repeat@
 \def\sd@X{+}\ifnum\count@@<\K@ \relax
 \ifnum\count@@>-3072 \def\sd@X{-}\fi\fi
 \def\sd@Y{+}\ifnum\count@@<3072 \relax
 \ifnum\count@@>-\K@ \relax\def\sd@Y{-}\fi\fi
 \imposeDirection@i
 \d@X=\cosDirection\xydashl@ \d@Y=\sinDirection\xydashl@
 \resetupDirection@}
\xydef@\imposeDirection@i{%
 \count@@=\K@ \multiply\count@@ by8 \advance\count@@\Direction
 \count@=\count@@ \advance\count@\KK@ \divide\count@64 \advance\count@\m@ne
 \loop@\ifnum127<\count@ \advance\count@-128 \repeat@
 \chardef\DirectionChar\count@
 \advance\count@@16 \divide\count@@\KK@ \advance\count@@\m@ne
 \loop@\ifnum127<\count@@ \advance\count@@-128 \repeat@
 \chardef\SemiDirectionChar\count@@
 \setbox8=\hbox{\xydashfont\SemiDirectionChar\/}%
 \quotient@@\cosDirection{\sd@X\wd8}\xydashl@
 \setbox8=\hbox{\xydashfont\count@=\SemiDirectionChar\advance\count@-64
 \ifnum\count@<\z@ \advance\count@128 \fi \char\count@\/}%
 \quotient@@\sinDirection{\sd@Y\wd8}\xydashl@}
\xydef@\getxyDirection@#1{\xy@@\bgroup\xy@@ix@{#1}%
 \xy@@{\expandafter\POS\the\toks9\relax\setupDirection@
 \edef\next@{\egroup \Direction=\the\Direction}\next@ \imposeDirection@ }}
\xydef@\reverseDirection@{%
 \d@X=-\d@X \d@Y=-\d@Y
 \ifdim\d@X<\z@ \def\sd@X{-}\else \def\sd@X{+}\fi
 \ifdim\d@Y<\z@ \def\sd@Y{-}\else \def\sd@Y{+}\fi
 \dimen@=4\K@ \ifnum\Direction<\z@ \advance\Direction\dimen@
 \else \advance\Direction-\dimen@ \fi
 \count@=\DirectionChar \ifnum\count@<64 \advance\count@64
 \else \advance\count@-64 \fi \chardef\DirectionChar=\count@
 \edef\cosDirection{\if-\cosDirection\else-\cosDirection\fi}%
 \edef\sinDirection{\if-\sinDirection\else-\sinDirection\fi}%
 \resetupDirection@}
\xydef@\aboveDirection@#1{%
 \dimen@=\d@X \d@X=-\d@Y \d@Y=\dimen@
 \dimen@=\K@dXdY \K@dXdY=-\K@dYdX \K@dYdX=-\dimen@
 \ifdim\d@X<\z@ \def\sd@X{-}\else \def\sd@X{+}\fi
 \ifdim\d@Y<\z@ \def\sd@Y{-}\else \def\sd@Y{+}\fi
 \dimen@=2\K@ \ifdim 1\Direction<\dimen@\else \dimen@=-6\K@ \fi
 \advance\Direction\dimen@
 \count@=\DirectionChar \ifnum\count@<96 \advance\count@32
 \else \advance\count@-96 \fi \chardef\DirectionChar=\count@
 \count@=\SemiDirectionChar \ifnum\count@<64 \advance\count@64
 \else \advance\count@-64 \fi \chardef\SemiDirectionChar=\count@
 \let\tmp@=\cosDirection
 \edef\cosDirection{\if-\sinDirection\else-\sinDirection\fi}%
 \let\sinDirection=\tmp@
 \dimen@=#1\relax \d@X=\cosDirection\dimen@ \d@Y=\sinDirection\dimen@
 \resetupDirection@}
\xydef@\belowDirection@#1{%
 \dimen@=\d@X \d@X=\d@Y \d@Y=-\dimen@
 \dimen@=\K@dXdY \K@dXdY=-\K@dYdX \K@dYdX=-\dimen@
 \ifdim\d@X<\z@ \def\sd@X{-}\else \def\sd@X{+}\fi
 \ifdim\d@Y<\z@ \def\sd@Y{-}\else \def\sd@Y{+}\fi
 \dimen@=-2\K@\ifdim 1\Direction<\dimen@\dimen@=6\K@\fi
 \advance\Direction\dimen@
 \count@=\DirectionChar \ifnum\count@<32 \advance\count@96
 \else \advance\count@-32 \fi \chardef\DirectionChar=\count@
 \count@=\SemiDirectionChar \ifnum\count@<64 \advance\count@64
 \else \advance\count@-64 \fi \chardef\SemiDirectionChar=\count@
 \let\tmp@=\sinDirection
 \edef\sinDirection{\if-\cosDirection\else-\cosDirection\fi}%
 \let\cosDirection=\tmp@
 \dimen@=#1\relax \d@X=\cosDirection\dimen@ \d@Y=\sinDirection\dimen@
 \resetupDirection@}
\xydef@\vDirection@(#1,#2)#3{\dimen@ii=#3\relax
 \dimen@=#1\dimen@ii \dimen@ii=#2\dimen@ii
 \d@X=\cosDirection\dimen@ \advance\d@X-\sinDirection\dimen@ii
 \d@Y=\sinDirection\dimen@ \advance\d@Y \cosDirection\dimen@ii
 \X@p=\X@c \advance\X@p-\d@X \Y@p=\Y@c \advance\Y@p-\d@Y
 \setupDirection@\ignorespaces}
\xydef@\resetDirection@{%
 \d@X=\X@c\advance\d@X-\X@p \d@Y=\Y@c\advance\d@Y-\Y@p
 \let\next@=\resetupDirection@
 \ifdim\sd@X\d@X<\z@ \let\next@=\setupDirection@i \fi
 \ifdim\sd@Y\d@Y<\z@ \let\next@=\setupDirection@i \fi
 \next@}
\xydef@\resetupDirection@{%
 \edef\Directiontest@@##1##2{\noexpand\DN@{##2}%
 \noexpand\ifdim\noexpand\d@X=\the\d@X\relax
 \noexpand\ifdim\noexpand\d@Y=\the\d@Y\relax \noexpand\DN@{##1}%
 \noexpand\fi\noexpand\fi \noexpand\next@}}
\xydef@\unsetupDirection@{\def\Directiontest@@##1##2{##2}}
\uDirection@\xydashl@
\message{edges,}
\xynew@{if}\ifInside@
\xydef@\zeroEdge#1{%
 \ifcase#1\relax \or \Inside@false \or \dimen@=\z@
 \or \else \Edge@c={\rectangleEdge}\fi}
\xydef@\circleEdge#1{\ifcase#1\expandafter\circleEdge@
 \or \expandafter\circleUnder@ \or \dimen@=\R@c
 \or \expandafter\circleProp@ \or \expandafter\circleInner@
 \else \expandafter\circleOuter@ \fi}
\xydef@\circleEdge@{\DN@{\ellipseEdge@}%
 \ifdim\R@c=\L@c\relax \ifdim\U@c=\D@c\relax
 \ifdim\R@c=\U@c\DN@{\circlecentredEdge@}%
 \else\DN@{\ellipsecentredEdge@}\fi
 \fi\fi \next@}
\xydef@\circleProp@{\DN@{\reverseDirection@\ellipseEdge@}%
 \ifdim\R@c=\L@c\relax \ifdim\U@c=\D@c\relax
 \ifdim\R@c=\U@c\DN@{\reverseDirection@\circlecentredEdge@}%
 \else\DN@{\reverseDirection@\ellipsecentredEdge@}\fi
 \fi\fi \next@}
\xydef@\circleUnder@{\Inside@false
 \ifdim\X@p=\X@c \relax \ifdim\Y@p=\Y@c \Inside@true \fi \fi 
 \ifInside@ \else \expandafter \circleCentre@ \fi}
\xydef@\circleCentre@{{%
 \ifdim\L@c=\R@c \relax\else
 \dimen@=\R@c\advance\dimen@-\L@c \divide\dimen@\tw@
 \advance\X@c\dimen@ \advance\R@c-\dimen@ \fi
 \d@X=\X@c \advance\d@X-\X@p \d@X=\ifdim\d@X<\z@-\fi\d@X
 \ifdim\U@c=\D@c\relax \else
 \dimen@=\U@c\advance\dimen@-\D@c \divide\dimen@\tw@
 \advance\Y@c\dimen@ \advance\U@c-\dimen@ \fi
 \d@Y=\Y@c \advance\d@Y-\Y@p \d@Y=\ifdim\d@Y<\z@-\fi\d@Y
 \DN@{}\ifdim\d@X>\R@c \relax \else \ifdim\d@Y>\U@c \relax 
 \else \ifdim\U@c=\R@c \DN@{\circlecentredUnder@}%
 \else \DN@{\ellipsecentredUnder@}\fi
 \fi\fi \next@}}
\xydef@\circleInner@{\DN@{\ellipseInner@}%
 \ifdim\R@c=\L@c\relax \ifdim\U@c=\D@c\relax
 \ifdim\R@c=\U@c\DN@{\circlecentredInner@}%
 \else\DN@{\ellipsecentredInner@}\fi
 \fi\fi \next@}
\xydef@\circleOuter@{\DN@{\ellipseOuter@}%
 \ifdim\R@c=\L@c\relax \ifdim\U@c=\D@c\relax
 \ifdim\R@c=\U@c\DN@{\circlecentredOuter@}%
 \else\DN@{\ellipsecentredOuter@}\fi
 \fi\fi \next@}
\xydef@\circlecentredEdge@{%
 \dimen@=-\cosDirection\R@c \advance\X@c\dimen@
 \dimen@=-\sinDirection\R@c \advance\Y@c\dimen@}
\xydef@\circlecentredUnder@{%
 \loop\ifdim\R@c>100\p@ \circlescale@ \repeat
 \edef\tmp@{\expandafter\removePT@\the\R@c}\dimen@=\tmp@\R@c 
 \edef\tmp@{\expandafter\removePT@\the\d@X}\advance\dimen@-\tmp@\d@X
 \edef\tmp@{\expandafter\removePT@\the\d@Y}\advance\dimen@-\tmp@\d@Y
 \ifdim\dimen@>\z@ \aftergroup\Inside@true \fi}
%%\xydef@\circlescale@{\divide\R@c\KK@ \divide\d@X\KK@ \divide\d@Y\KK@ }
\xydef@\circlescale@{\divide\R@c\KK@ \divide\d@X\KK@ \divide\d@Y\KK@ }
\xydef@\circlecentredInner@{%
 \L@c=\sd@X\cosDirection\R@c \D@c=\sd@Y\sinDirection\R@c
 \R@c=\L@c \U@c=\D@c \Edge@c={\rectangleEdge}}
\xydef@\circlecentredOuter@{%
 \L@c=\R@c \D@c=\R@c \U@c=\D@c \Edge@c={\rectangleEdge}}
\xydef@\ellipsecentredEdge@{\bgroup \X@p=\X@c \Y@p=\Y@c 
 \ifdim\U@c>\R@c
 \X@c=\cosDirection\U@c \Y@c=\sinDirection\U@c
 \quotient@\tmp@\U@c\R@c \X@c=\tmp@\X@c \R@c=\U@c 
 \else
 \X@c=\cosDirection\R@c \Y@c=\sinDirection\R@c
 \quotient@\tmp@\R@c\U@c \Y@c=\tmp@\Y@c 
 \fi
 \advance\X@c\X@p \advance\Y@c\Y@p 
 \setupDirection@ \X@c=\X@p \Y@c=\Y@p \circlecentredEdge@
 \d@X=\X@c \advance\d@X-\X@p \d@Y=\Y@c \advance\d@Y-\Y@p 
 \ifdim\U@c>\L@c \quotient@\tmp@\L@c\U@c \d@X=\tmp@\d@X
 \else \quotient@\tmp@\U@c\R@c \d@Y =\tmp@\d@Y \fi
 \X@c=\X@p \advance\X@c\d@X \Y@c=\Y@p \advance\Y@c\d@Y 
 \edef\next@{\egroup \X@c=\the\X@c \Y@c=\the\Y@c}\next@ }%
\xydef@\ellipsecentredUnder@{%
 \ifdim\R@c>64\p@ \circlescale@ \divide\U@c\KK@ 
 \else \ifdim\U@c>64\p@ \circlescale@ \divide\U@c\KK@ \fi\fi
 \edef\tmp@{\expandafter\removePT@\the\R@c}\d@Y=\tmp@\d@Y 
 \edef\tmp@{\expandafter\removePT@\the\U@c}\d@X=\tmp@\d@X 
 \R@c=\tmp@\R@c \circlecentredUnder@ }
\xydef@\ellipsecentredOuter@{\Edge@c={\rectangleEdge}}
\xydef@\ellipsecentredInner@{%
 \bgroup \X@p=\X@c \Y@p=\Y@c \ellipsecentredEdge@
 \advance\X@c-\X@p \L@c=\ifdim\X@c<\z@-\fi\X@c
 \advance\Y@c-\Y@p \D@c=\ifdim\Y@c<\z@-\fi\Y@c
 \edef\next@{\egroup \L@c=\the\L@c \D@c=\the\D@c}\next@
 \R@c=\L@c \U@c=\D@c \Edge@c={\rectangleEdge}}
\xydef@\ellipseEdge@{\bgroup
 \A@=\R@c \B@=\U@c
 \ifdim\R@c=\L@c \d@X=\z@ 
 \else \d@X=.5\R@c \advance\d@X-.5\L@c 
 \advance\A@\L@c \divide\A@\tw@ \fi
 \ifdim\U@c=\D@c \d@Y=\z@ 
 \else \d@Y=.5\U@c \advance\d@Y-.5\D@c 
 \advance\B@\D@c \divide\B@\tw@ \fi
 \bgroup
 \L@c=\A@ \U@c=\B@
 \R@p=\U@c \advance\R@p\L@c \multiply\R@p\tw@
 \ifdim\B@<\A@ \quotient@\tmp@\U@c\L@c \R@c=\tmp@\p@ \D@c=\p@
 \quotient@\tmp@\R@p\L@c \R@p=\tmp@\p@
 \else
 \ifdim\A@<\B@ \quotient@\tmp@\L@c\U@c \D@c=\tmp@\p@ \R@c=\p@
 \quotient@\tmp@\R@p\U@c \R@p=\tmp@\p@
 \else
 \R@c=\p@ \D@c=\p@ \quotient@\tmp@\R@p\U@c \R@p=\tmp@\p@
 \fi\fi
 \quotient@\sd@X\d@X\L@c \d@X=\sd@X\p@
 \quotient@\sd@Y\d@Y\U@c \d@Y=\sd@Y\p@
 \loop
 \bgroup \U@p=-\p@ \D@p=\z@
 \ifdim\R@c<\p@
 \edef\tmp@{\expandafter\removePT@\the\R@c}\dimen@=\tmp@\R@p 
 \advance\d@X\cosDirection\dimen@
 \else \advance\d@X\cosDirection\R@p \fi
 \edef\sd@X{\expandafter\removePT@\the\d@X}%
 \advance\U@p\sd@X\d@X
 \ifdim\R@c<\p@
 \edef\tmp@{\expandafter\removePT@\the\R@c}\dimen@=\tmp@\d@X 
 \advance\D@p\cosDirection\dimen@
 \else \advance\D@p\cosDirection\d@X \fi
 \ifdim\D@c<\p@
 \edef\tmp@{\expandafter\removePT@\the\D@c}\dimen@=\tmp@\R@p 
 \advance\d@Y\sinDirection\dimen@
 \else \advance\d@Y\sinDirection\R@p \fi
 \edef\sd@Y{\expandafter\removePT@\the\d@Y}%
 \advance\U@p\sd@Y\d@Y
 \ifdim\D@c<\p@
 \edef\tmp@{\expandafter\removePT@\the\D@c}\dimen@=\tmp@\d@Y 
 \advance\D@p\sinDirection\dimen@
 \else \advance\D@p\sinDirection\d@Y \fi
 \multiply\D@p\tw@ 
 \dimen@=\ifdim\U@p<\z@-\fi\U@p 
 \ifdim\dimen@<.01\p@ \U@p=\z@ 
 \else
 \quotient@\tmp@\U@p\D@p \U@p=\tmp@\p@
 \ifdim\U@p<\z@\xywarning@{poor convergence}\U@p=\z@
 \else \advance\R@p-\U@p \U@p=\ifdim\U@p<\z@-\fi\U@p 
 \fi \fi
 \edef\next@{\egroup \R@p=\the\R@p \U@p=\the\U@p \D@p=\the\D@p}\next@
 \ifdim\U@p>\z@ \repeat
 \edef\next@{\egroup \dimen@=\the\R@p}\next@
 \edef\tmp@{\expandafter\removePT@\the\dimen@}%
 \ifdim\B@<\A@ \dimen@=\tmp@\B@ \else \dimen@=\tmp@\A@ \fi
 \dimen@=-\dimen@
 \advance\X@c\cosDirection\dimen@
 \advance\Y@c\sinDirection\dimen@
 \edef\next@{\egroup \X@c=\the\X@c \Y@c=\the\Y@c}\next@ }%
\xydef@\ellipseOuter@{\Edge@c={\rectangleEdge}}
\xydef@\ellipseInner@{%
 \bgroup \X@p=\X@c \Y@p=\Y@c \ellipseEdge@
 \d@X=\X@c\advance\d@X-\X@p
 \ifdim\d@X>\z@ \R@p=\d@X \L@p=\R@p
 \ifdim\L@c=\R@c\else\advance\L@p\L@c \advance\L@p-\R@c \fi
 \else \L@p=-\d@X \R@p=\L@p
 \ifdim\L@c=\R@c \else\advance\R@p\R@c \advance\R@p-\L@c \fi
 \fi
 \d@Y=\Y@c\advance\d@Y-\Y@p
 \ifdim\d@Y>\z@ \U@p=\d@Y \D@p=\U@p
 \ifdim\D@c=\U@c\else\advance\D@p\D@c \advance\D@p-\U@c \fi
 \else \D@p=-\d@Y \U@p=\D@p
 \ifdim\D@c=\U@c\else\advance\U@p\U@c \advance\U@p-\D@c \fi
 \fi
 \edef\next@{\egroup
 \L@c=\the\L@p \D@c=\the\D@p \R@c=\the\R@p \U@c=\the\U@p}%
 \next@ \Edge@c={\rectangleEdge}}
\xydef@\rectangleEdge#1{\ifcase#1\expandafter\rectangleEdge@
 \or \expandafter\rectangleUnder@ \or \expandafter\rectangleDist@
 \or \expandafter\rectangleProp@
 \else \relax \fi}
\xydef@\rectangleEdge@{%
 \ifdim\d@Y<-.05\p@ \rectangleEdge@i
 \else\ifdim\d@Y<.05\p@ \rectangleEdge@ii
 \else \rectangleEdge@iii\fi\fi
 \resetupDirection@}
\xydef@\rectangleEdge@i{%
 \ifdim\d@X<-.05\p@
 \settomin@\X@c+\R@c\U@c\d@X\d@Y \settomin@\Y@c+\U@c\R@c\d@Y\d@X%1a
 \else\ifdim\d@X<.05\p@ \advance\Y@c\U@c
 \else \settomin@\X@c-\L@c\U@c\d@X\d@Y \settomin@\Y@c+\U@c\L@c\d@Y\d@X
 \fi\fi}
\xydef@\rectangleEdge@ii{%
 \ifdim\d@X<-.05\p@ \advance\X@c\R@c
 \else\ifdim\d@X<.05\p@
 \else \advance\X@c-\L@c
 \fi\fi}
\xydef@\rectangleEdge@iii{%
 \ifdim\d@X<-.05\p@
 \settomin@\X@c+\R@c\D@c\d@X\d@Y \settomin@\Y@c-\D@c\R@c\d@Y\d@X%3a
 \else\ifdim\d@X<.05\p@ \advance\Y@c-\D@c
 \else \settomin@\X@c-\L@c\D@c\d@X\d@Y \settomin@\Y@c-\D@c\L@c\d@Y\d@X
 \fi\fi}
\xydef@\settomin@#1#2#3#4#5#6{%
 \edef\nextii@{\A@=\the\A@ \B@=\the\B@}\quotient@\next@{#5}{#6}\nextii@
 \dimen@=\sd@X\sd@Y\next@#4\relax
 \ifdim#3<\dimen@ \dimen@=#3\fi \advance#1#2\dimen@}
\xydef@\rectangleUnder@{\Inside@false
 \ifdim\X@p=\X@c \ifdim\Y@p=\Y@c \Inside@true \fi\fi 
 \ifInside@ \else
 \dimen@=\X@p \advance\dimen@-\X@c 
 \ifdim \dimen@>-\L@c \relax \ifdim\dimen@<\R@c 
 \dimen@=\Y@p \advance\dimen@-\Y@c 
 \ifdim \dimen@>-\D@c \relax \ifdim\dimen@<\U@c 
 \Inside@true 
 \fi\fi\fi\fi\fi }
\xydef@\rectangleDist@{\let\next@=\rectangleDist@i
 \ifdim\d@X<-.05\p@ \dimen@=\R@c
 \else\ifdim\d@X<.05\p@ \dimen@=\z@ \DN@{\dimen@=\dimen@ii}%
 \else \dimen@=\L@c \fi\fi
 \ifdim\d@Y<-.05\p@ \dimen@ii=\U@c
 \else\ifdim\d@Y<.05\p@ \DN@{}%
 \else \dimen@ii=\D@c \fi\fi
 \next@}
\xydef@\rectangleDist@i{%
 \begingroup \quotient@\next\p@{\sd@X\cosDirection\p@}%
 \edef\next{\endgroup \dimen@=\next\dimen@}\next
 \begingroup \quotient@\next\p@{\sd@Y\sinDirection\p@}%
 \edef\next{\endgroup \dimen@ii=\the\dimen@ii}\next
 \ifdim\dimen@ii<\dimen@ \dimen@=\dimen@ii \fi}
\xydef@\rectangleProp@{%
 \enter@{\A@=\the\A@ \B@=\the\B@ \DirectionfromtheDirection@}%
 \reverseDirection@
 \dimen@=1\Direction \count@=\K@ \multiply\count@\tw@
 \ifnum \Direction>\count@
 \DN@{0}%
 \advance\dimen@-2\K@ \quotient@\nextii@{\dimen@}{2\K@}%
 \else\ifnum \Direction>\z@
 \dimen@=-\dimen@ \advance\dimen@2\K@ \quotient@\next@{\dimen@}{2\K@}%
 \DNii@{0}%
 \else\ifnum \Direction>-\count@
 \DN@{1}%
 \quotient@\nextii@{-\dimen@}{2\K@}%
 \else
 \advance\dimen@4\K@ \quotient@\next@{\dimen@}{2\K@}%
 \DNii@{1}%
 \fi\fi\fi
 \advance\X@c-\L@c \dimen@=\L@c \advance\dimen@\R@c 
 \ifdim\dimen@=\z@ \advance\X@c 2\L@c \else \advance\X@c\next@\dimen@ \fi
 \advance\Y@c+\U@c \dimen@=\D@c \advance\dimen@\U@c 
 \ifdim\dimen@=\z@ \advance\Y@c-2\U@c \advance\Y@c\Upness@\U@c
 \else \advance\Y@c-\nextii@\dimen@ \fi
 \leave@}
\message{connections;}
\xydef@\Creset@@{}
\xydef@\Cshavep@@{\noCshavep@@}
\xydef@\Cshavec@@{\noCshavec@@}
\xydef@\Cslidep@@{\noCslidep@@}
\xydef@\Cslidec@@{\noCslidec@@}
\xydef@\Calong@@{\noCalong@@}
\xydef@\Cintercept@@{\noCintercept@@}
\xydef@\Cbreak@@{\noCbreak@@}
\xydef@\Clast@@{\noClast@@}
\xylet@\lastbreak@@=\empty
\xydef@\noCshavep@@{\setupDirection@
 \enter@{\cfromthec@ \DirectionfromtheDirection@}%
 \reverseDirection@ \cfromp@ \the\Edge@c\z@
 \pfromc@ \leave@ \resetDirection@}
\xydef@\noCshavec@@{\setupDirection@ \the\Edge@c\z@ \resetDirection@}
\xydef@\noCslidep@@#1{\dimen@=#1\relax
 \advance\X@p\cosDirection\dimen@ \advance\Y@p\sinDirection\dimen@
 \resetDirection@}
\xydef@\noCslidec@@#1{\dimen@=#1\relax
 \advance\X@c\cosDirection\dimen@ \advance\Y@c\sinDirection\dimen@
 \resetDirection@}
\xydef@\noCalong@@#1{%
 \d@X=#1\d@X \d@Y=#1\d@Y \X@c=\X@p \Y@c=\Y@p \advance\X@c\d@X \advance\Y@c\d@Y
 \resetupDirection@}
\xydef@\noCintercept@@{\enter@{\pfromthep@}%
 \begingroup\Creset@@ \edef\tmp@{\endgroup
 \X@origin=\the\X@p \Y@origin=\the\Y@p \R@c=\the\d@X \U@c=\the\d@Y}\tmp@
 \loop@\dimen@=\ifdim\R@c<\z@-\fi\R@c \advance\dimen@\ifdim\U@c<\z@-\fi\U@c
 \ifdim\dimen@>10\p@ \advance\R@c \ifdim\R@c<\z@-\fi 16sp \divide\R@c\KK@ 
 \advance\U@c \ifdim\U@c<\z@-\fi 16sp \divide\U@c\KK@ \repeat@
 \intersect@ \leave@}
\xydef@\noCbreak@@{\edef\lastbreak@@{\cfromthec@}}
\xydef@\noClast@@{\Creset@@ \edef\lastbreak@@{\cfromthep@}}
\xydef@\no@@{\setupDirection@ \edef\lastbreak@@{\cfromthep@}%
 \enter@{\cfromthec@\pfromthep@\DirectionfromtheDirection@}%
 \edef\Creset@@{\cfromthec@ \pfromthep@ \DirectionfromtheDirection@}%
 \edef\next@{{\sd@X}{\sd@Y}}\expandafter\straightcheckoverlap@\next@
 \setupDirection@ \the\Edge@c\z@
 \swap@\reverseDirection@\the\Edge@c\z@\swap@\reverseDirection@
 \resetDirection@
 \edef\Cshavep@@{\DirectionfromtheDirection@
 \pfromthep@\noexpand\resetDirection@}%
 \edef\Cshavec@@{\DirectionfromtheDirection@
 \cfromthec@\noexpand\resetDirection@}%
 \leave@
 \def\Cslidep@@{\noCslidep@@}\def\Cslidec@@{\noCslidec@@}%
 \def\Calong@@{\noCalong@@}\def\Cintercept@@{\noCintercept@@}%
 \def\Cbreak@@{\noCbreak@@}\def\Clast@@{\noClast@@}\noinsert@}
\xydef@\noinsert@{\ifHidden@\else
 \ifdim\Y@c>\Y@max \Y@max=\Y@c \fi \ifdim\Y@p>\Y@max \Y@max=\Y@p \fi
 \ifdim\Y@c<\Y@min \Y@min=\Y@c \fi \ifdim\Y@p<\Y@min \Y@min=\Y@p \fi
 \ifdim\X@c>\X@max \X@max=\X@c \fi \ifdim\X@p>\X@max \X@max=\X@p \fi
 \ifdim\X@c<\X@min \X@min=\X@c \fi \ifdim\X@p<\X@min \X@min=\X@p \fi
 \fi}
\xydef@\Spread@@{}
\xydef@\checkoverlap@@{}
\xydef@\straight@#1{\setupDirection@ \def\Spread@@{#1}%
 \edef\Creset@@{\cfromthec@ \pfromthep@ \DirectionfromtheDirection@}%
 \edef\lastbreak@@{\cfromthep@}%
 \edef\next@{{\sd@X}{\sd@Y}}\expandafter\straightcheckoverlap@\next@
 \setupDirection@ \the\Edge@c\z@
 \swap@\reverseDirection@\the\Edge@c\z@\swap@\reverseDirection@
 \resetDirection@
 \edef\Cshavep@@{\DirectionfromtheDirection@
 \pfromthep@\noexpand\resetDirection@}%
 \edef\Cshavec@@{\DirectionfromtheDirection@
 \cfromthec@\noexpand\resetDirection@}%
 \noinsert@
 \straight@typeset
 \def\Cbreak@@{\straightCbreak@}\def\Clast@@{\straightClast@}%
 \def\Cslidep@@{\noCslidep@@}\def\Cslidec@@{\noCslidec@@}%
 \def\Calong@@{\noCalong@@}\def\Cintercept@@{\noCintercept@@}%
 \Creset@@}
\xydef@\straightcheckoverlap@#1#2{\def\checkoverlap@@{%
 \ifdim#1\X@p>#1\X@c \let\next@=\relax \fi
 \ifdim#2\Y@p>#2\Y@c \let\next@=\relax \fi}}
\xydef@\straight@typeset{%
 \ifInvisible@ \let\next@=\relax
 \else\ifdim 1\Direction<-2\K@ \DN@{\straightv@}%
 \else\ifdim 1\Direction<\z@ \DN@{\straighth@}%
 \else\ifdim 1\Direction<2\K@ \DN@{\straightv@}%
 \else \DN@{\straighth@}%
 \fi\fi\fi\fi \checkoverlap@@ \next@}
\xylet@\nextbreak@@=\empty
\xydef@\straightCbreak@{\connectRestore@
 \edef\nextbreak@@{\cfromthec@}%
 \Creset@@ \swap@ \the\Edge@c4\enter@{\cmergethec@}\lastbreak@@ \leave@
 \swap@ \the\Edge@c4\enter@{\cmergethec@}\nextbreak@@ \leave@
 \setupDirection@
 \the\Edge@c\z@
 \swap@ \reverseDirection@ \the\Edge@c\z@ \swap@ \reverseDirection@
 \resetDirection@ \noinsert@ \straight@typeset
 \Creset@@ \let\lastbreak@@=\nextbreak@@}
\xydef@\straightClast@{\connectRestore@
 \Creset@@ \swap@ \the\Edge@c4\enter@{\cmergethec@}\lastbreak@@ \leave@
 \swap@
 \setupDirection@
 \the\Edge@c\z@
 \swap@\reverseDirection@ \the\Edge@c\z@ \swap@\reverseDirection@
 \resetDirection@ \noinsert@ \straight@typeset
 \Creset@@ \edef\lastbreak@@{\cfromthep@}}
\xydef@\straighth@{\setbox\z@=\hbox{%
 \setbox8=\copy\lastobjectbox@
 \A@=\wd8\relax \B@=\dp8\relax \advance\B@\ht8\relax
 \ifdim \A@=\z@ \count@@=\m@ne
 \else \dimen@=\sd@X\d@X \divide\dimen@\A@ \count@@=\dimen@ \fi
 \Spread@@
 \ifdim\d@X>\z@ \advance\X@c-\wd8\relax\fi
 \dimen@=-\sd@X\wd8\relax
 \multiply\dimen@\K@dYdX \divide\dimen@\K@
 \ifdim\d@X>\z@ \advance\Y@c\dimen@ \advance\Y@c-\Leftness@\dimen@
 \else \advance\Y@c\Leftness@\dimen@ \fi
 \dimen@=\wd8\relax \A@=\sd@X\d@X \advance\A@-\dimen@
 \B@=\sd@X\dimen@ \multiply\B@\K@dYdX \divide\B@\K@
 \advance\B@-\d@Y \B@=\sd@Y\B@
 \count@=\count@@ \advance\count@\m@ne
 \ifnum\z@<\count@ \divide\A@\count@ \divide\B@\count@ \fi
 \A@=-\sd@X\A@ \B@=\sd@Y\B@ \wd8=\A@
 \kern\X@c \count@=\z@
 \loop@\ifnum\count@<\count@@ \advance\count@\@ne
 \raise\Y@c\copy8\relax \advance\Y@c\B@ \repeat@}%
 \ht\z@=\z@ \wd\z@=\z@ \dp\z@=\z@ {\Drop@@}}
\xydef@\straightv@{\setbox\z@=\vtop{%
 \setbox8=\copy\lastobjectbox@
 \A@=\wd8\relax \B@=\dp8\relax \advance\B@\ht8\relax
 \ifdim \B@=\z@ \count@@=\m@ne
 \else \dimen@=\sd@Y\d@Y \divide\dimen@\B@ \count@@=\dimen@ \fi
 \Spread@@
 \dimen@=\dp8\relax \advance\dimen@\ht8\relax
 \B@=\sd@Y\d@Y \advance\B@-\dimen@
 \A@=\sd@Y\dimen@ \multiply\A@\K@dXdY \divide\A@\K@ \advance\A@-\d@X
 \A@=\sd@X\A@ \count@=\count@@ \advance\count@\m@ne
 \ifnum\z@<\count@ \divide\B@\count@ \divide\A@\count@ \fi
 \B@=\sd@Y\B@ \A@=\sd@X\A@ \ht8=\B@ \dp8=\z@
 \ifdim\d@Y<\z@ 
 \advance\Y@c\dimen@ \advance\Y@c\Upness@\B@
 \else
 \advance\dimen@\Upness@\B@ \advance\Y@c-\dimen@ \advance\Y@c\B@
 \fi
 \advance\Y@c\B@ 
 \ifdim\d@X<\z@ \else \advance\X@c-\wd8\relax \fi
 \null \kern-\Y@c \count@=\z@
 \loop@\ifnum\count@<\count@@ \advance\count@\@ne
 \nointerlineskip \moveright\X@c\copy8\relax \advance\X@c\A@
 \repeat@}%
 \ht\z@=\z@ \wd\z@=\z@ \dp\z@=\z@ {\Drop@@}}
\message{ Xy-pic loaded}\xyuncatcodes \endinput


==> xy16textures.tex <==
%% xy16textures.tex from $Id: xy16textures.doc,v 3.3 1996/12/18 14:21:23 ross Exp $
%%
%% Xy-pic ``Textures v1.6'' driver interface option.
%% Copyright (c) 1995-1996 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1996 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{16textures}{Textures v1.6 driver}{\stripRCS$Revision: 3.3 $}%
 {Ross Moore}{ross@mpce.mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xydef@\oldTextures@@#1{\dvimessage@{Textures v1.6}{#1}}
\newdriver{%
 \xyaddsupport{color}\oldtexturesColor@@
 \xyaddsupport{crayon}\oldtexturesCrayon@@
 \xyaddsupport{ps}\oldtexturesPS@@
 \xyaddsupport{rotate}\oldtexturesRotate@@
 \xyaddsupport{line}\oldtexturesLine@@
 \xyaddsupport{frame}\oldtexturesFrames@@
 \xyaddsupport{tile}\oldtexturesTiles@@
 \xyaddsupport{cmtip}\relax
}
\xydef@\oldTexturesColours@{\oldtexturesPStypes@
 \let\xylocalColor@=\xyNoColor@@ \def\xycolor@{\xycolor@@}%
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-c}{\xydrivernoload@{ps-c}}%
 \installPScolor@ }\else\DN@{}\fi \next@
 \ifx\xycolor@@\xyNoColor@ \let\xycolor@@=\xycolor@raw@@\fi
 \ifx\xycrayolaloaded\empty \DN@{\xystandardcolors@\oldtexturesCrayon@@{}}%
 \else\let\next@=\xystandardcolors@ \fi \next@ 
 \let\xycolorwarning@=\relax
 \let\oldtexturesColor@@=\relax
 \let\UnloadColor@@=\NooldTexturesColor@
 }
\xydef@\oldtexturesColor@@{\oldTexturesColours@}
\xydef@\NooldTexturesColor@{%
 \let\xylocalColor@=\xyNoColor@@
 \let\xycolor@=\xyNoColor@
 \let\xycolorwarning@=\xycolorwarning@@
 \let\oldtexturesColor@@=\oldTexturesColours@
 \let\UnloadColor@@=\UnloadColor@
 }
\xydef@\oldtexturesCrayon@@{\oldtexturesColor@@\oldtexturesCrayon@}
\xydef@\oldtexturesCrayon@{\installCrayolaColors@}%
\xydef@\oldtexturesPS@@{\oldtexturesPS@}
\xydef@\oldtexturesPSunload@{\UnloadPS@
 \ifx\xyrealshipout@\undefined\else
 \ifx\shipout\xyrealshipout@
 \else \let\shipout=\xyrealshipout@\fi\fi
 \let\installxyps@@=\relax
 \let\UnloadPS@@=\UnloadPS@
 \let\oldtexturesPS@@=\oldtexturesPS@ }
\xydef@\oldTexturesSpecial@#1{\firstPS@@\special{postscript #1}}
\xydef@\oldTexturesMacro@#1{\special{postscript {#1}xy}}
\xydef@\oldTexturesInclude@#1{\firstPS@@\special{rawpostscriptfile #1}}
\xydef@\oldTexturesRaw@#1{\firstPS@@\special{rawpostscript #1}}
\xydef@\oldtexturesPStypes@{%
 \xyinputorelse@{xyps-ps}{\xydrivernoload@{ps-ps}}%
 \ifx\PSspecial@@\oldTexturesSpecial@\else
 \let\PSspecial@@=\oldTexturesSpecial@
 \let\PSmacro@@=\oldTexturesMacro@
 \let\PSdict@@=\oldTexturesRaw@
 \let\PSraw@@=\oldTexturesRaw@
 \let\PSinclude@@=\oldTexturesInclude@
 \let\PSspecialdict@@=\oldTexturesRaw@
 \let\xyPSobeylines@@=\obeyoldTextureslines@
 \oldTextures@@{PostScript}%
 \fi 
 \oldtexturesCurrpt@ \@PSshipout }
{\catcode`\^^M=\active
 \gdef\next{\catcode`\^^M=\active \let^^M=\par \obeyspaces}}
\xylet@\obeyoldTextureslines@=\next
\xydef@\oldtexturesCurrpt@{\let\xyPScurrpt@@=\oldtexturesCurrpt@@}%
\xydef@\oldtexturesCurrpt@@{\PSspecial@@{xyi}\PSraw@@{userdict begin xyx end}}
\xydef@\oldtexturesPS@{\oldtexturesPStypes@ 
 \let\oldtexturesPS@@=\relax
 \let\UnloadPS@@=\oldtexturesPSunload@ 
 \let\installxyps@@=\@PSshipout \installxyps@ }
\xydef@\oldtexturesRotate@@{\oldtexturesRotate@}
\xydef@\oldtexturesRotate@{\oldtexturesPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-r}{\xydrivernoload@{ps-r}}%
 \xyRotScale@@ \installPSrotscale@ }%
 \else\DN@{\xydriverfail@{rotations are}\UnloadRotate@\relax}\fi
 \next@ }
\xydef@\oldtexturesLine@@{\oldtexturesLine@}
\xydef@\oldtexturesLine@{\oldtexturesPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-l}{\xydrivernoload@{ps-l}}%
 \installPSline@ }%
 \else\DN@{\xydriverfail@{line-styles are}\UnloadLine@\relax}\fi
 \next@ }
\xydef@\oldtexturesFrames@@{\oldtexturesFrames@}
\xydef@\oldtexturesFrames@{\oldtexturesPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-f}{\xydrivernoload@{ps-f}}%
 \installPSframes@ }%
 \else\DN@{\xydriverfail@{frames are}\UnloadPSFrames@\relax}\fi
 \next@ }
\xydef@\oldtexturesTiles@@{\oldtexturesTiles@}
\xydef@\oldtexturesTiles@{\oldtexturesPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-t}{\xydrivernoload@{ps-t}}%
 \installPSpatterns@ \xystandardpatterns@}%
 \else\DN@{\xydriverfail@{Patterns are}\UnloadPSpatterns@\relax}\fi
 \next@ }
\xyendinput


==> xy17oztex.tex <==
%% xy17oztex.tex from $Id: xy17oztex.doc,v 3.3 1996/12/18 14:21:23 ross Exp $
%%
%% Xy-pic ``OzTeX v1.7'' driver interface option.
%% Copyright (c) 1995-1996 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1996 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{17oztex}{OzTeX v1.7 driver}{\stripRCS$Revision: 3.3 $}%
 {Ross Moore}{ross@mpce.mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xydef@\OzTeX@@#1{\dvimessage@{OzTeX v1.7}{#1}}
\newdriver{%
 \xyaddsupport{color}\oldoztexColor@@
 \xyaddsupport{crayon}\oldoztexCrayon@@
 \xyaddsupport{ps}\oldoztexPS@@
 \xyaddsupport{rotate}\oldoztexRotate@@
 \xyaddsupport{line}\oldoztexLine@@
 \xyaddsupport{frame}\oldoztexFrames@@
 \xyaddsupport{tile}\oldoztexTiles@@
 \xyaddsupport{cmtip}\relax
}
\xydef@\oldoztexColor@@{\oldOzTeXColours@}
\xydef@\oldOzTeXColours@{\oldOzTeXPStypes@
 \let\xylocalColor@=\xyNoColor@@ \def\xycolor@{\xycolor@@}%
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-c}{\xydrivernoload@{ps-c}}%
 \installPScolor@ }\else\DN@{}\fi \next@
 \ifx\xycrayolaloaded\empty \DN@{\xystandardcolors@\oldOzTeXCrayon@@{}}%
 \else\let\next@=\xystandardcolors@\fi \next@
 \let\xycolorwarning@=\relax
 \let\oldoztexColor@@=\relax
 \let\UnloadColor@@=\NooldOzTeXColor@
 }
\xydef@\NooldOzTeXColor@{%
 \let\xylocalColor@=\xyNoColor@@
 \let\xycolor@=\xyNoColor@
 \let\xycolorwarning@=\xycolorwarning@@
 \let\oldoztexColor@@=\oldOzTeXColours@
 \let\UnloadColor@@=\UnloadColor@
 }
\xydef@\oldOzTeXCrayon@@{\installCrayolaColors@}
\xydef@\oldoztexPS@@{\oldoztexPS@}
\xydef@\oldoztexPSunload@{\UnloadPS@
 \def\xyPSdictname{}\UsePSdict@@false
 \let\installxyps@@=\relax
 \let\UnloadPS@@=\UnloadPS@
 \xyPSshapes@true 
 \let\oldoztexPS@@=\oldoztexPS@ }
\xydef@\oldOzTeXSpecial@#1{\special{empty.ps {#1}xy}}
\xydef@\oldOzTeXMacro@#1{\special{empty.ps {#1}xy}}
\xydef@\oldOzTeXDict@#1{\special{empty.ps @obxy{#1}stopped pop @eoxy}}
\xydef@\oldOzTeXinclude@#1{\special{#1}}
\xydef@\oldOzTeXraw@#1{\special{empty.ps @boxy #1 @eoxy}}%
\xydef@\oldOzTeXPStypes@{%
 \xyinputorelse@{xyps-ps}{\xydrivernoload@{ps-ps}}%
 \ifx\PSspecial@@\oldOzTeXSpecial@\else
 \let\PSspecial@@=\oldOzTeXSpecial@
 \let\PSmacro@@=\oldOzTeXMacro@
 \let\PSdict@@=\oldOzTeXDict@
 \let\PSraw@@=\oldOzTeXraw@
 \let\PSinclude@@=\oldOzTeXinclude@
 \let\xyPSobeylines@@=\obeyoldOzTeXlines@
 \let\PSspecialdict@@=\oldOzTeXDict@
 \oldOzTeX@@{PostScript}%
 \fi
 \oldOzTeXCurrpt@ }
{\catcode`\^^M=\active
 \gdef\next{\catcode`\^^M=\active \let^^M=\space \obeyspaces}}
\xylet@\obeyoldOzTeXlines@=\next
\xydef@\oldOzTeXCurrpt@{\let\xyPScurrpt@@=\OzTeXCurrpt@@}%
\xydef@\oldOzTeXCurrpt@@{}
\xydef@\oldoztexPS@@{\oldOzTeXPStypes@ 
 \let\installxyps@@=\old@OzTeX@PS@
 \installxyps@ }
\xydef@\old@OzTeX@PS@{\UsePSdict@@true
 \let\includePSmessage@=\xyoldOzTeXheader 
 \ifx\undefined\xyPSdictname\def\xyPSdictname{global.ps}\fi}
\xydef@\xyoldOzTeXheader#1#2#3{\UsePSdict@@true}
\xydef@\oldoztexLine@@{\oldoztexLine@}
\xydef@\oldoztexLine@{\oldOzTeXPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-l}{\xydrivernoload@{ps-l}}\installPSline@ }%
 \else\DN@{\xydriverfail@{line-styles are}\UnloadLine@\relax}\fi
 \next@ }
\xydef@\oldoztexFrames@@{\oldOzTeXFrames@}
\xydef@\oldOzTeXFrames@{\oldOzTeXPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-f}{\xydrivernoload@{ps-f}}\installPSframes@ }%
 \else\DN@{\xydriverfail@{frames are}\UnloadPSFrames@\relax}\fi
 \next@ }
\xydef@\oldoztexTiles@@{\oldOzTeXTiles@}
\xydef@\oldOzTeXTiles@{\oldOzTeXPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-t}{\xydrivernoload@{ps-t}}\installPSpatterns@
 \xystandardpatterns@ }%
 \else\DN@{\xydriverfail@{Patterns are}\UnloadPSpatterns@\relax}\fi
 \next@ }
\xydef@\oldoztexRotate@@{\oldOzTeXRotate@}
\xydef@\oldOzTeXRotate@{\oldOzTeXPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-r}{\xydrivernoload@{ps-r}}%
 \xyRotScale@@ \installPSrotscale@ \xyPSshapes@false }%
 \else\DN@{\xydriverfail@{rotations are}\UnloadRotate@\relax}\fi
 \next@ }
\xyendinput


==> xy2cell.tex <==
%% xy2cell.tex from $Id: xy2cell.doc,v 3.3 1996/12/18 14:21:23 ross Exp $
%%
%% Xy-pic ``2-cell'' feature.
%% Copyright (c) 1993-1996 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1996 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this macro package; if not, write to the Free Software Foundation,
%% Inc., 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{2cell}{Two-cell feature}{\stripRCS$Revision: 3.3 $}%
 {Ross Moore}{ross@mpce.mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xyrequire{curve}\xycatcodes
\message{two-cells,}
\xydef@\UseTwocells{\definesupermorphism{twocell}{%
 \xy@{start of 2-cell}{\begingroup}%
 \twocell@}}
\xydef@\UseHalfTwocells{%
 \definesupermorphism{uppertwocell}{%
 \xy@{start of 2-cell}{\begingroup}%
 \uppertwocell@}%
 \definesupermorphism{lowertwocell}{%
 \xy@{start of 2-cell}{\begingroup}%
 \lowertwocell@}}
\xydef@\UseCompositeMaps{\definesupermorphism{compositemap}{%
 \xy@{start composite-map}{\begingroup}%
 \compositemap@}}
\xydef@\UseAllTwocells{%
 \UseTwocells \UseHalfTwocells \UseCompositeMaps }
\xydef@\supermorphism#1[#2]#3{\def\afterMORPHISM{[#2]#3}#1}
\xydef@\afterMORPHISM{}
\xydef@\definesupermorphism#1#2{%
 \expandafter\def\csname x#1\endcsname{\supermorphism{#2}}%
 \expandafter\def\csname u#1\endcsname{\supermorphism{#2}[-1,0]{}}%
 \expandafter\def\csname d#1\endcsname{\supermorphism{#2}[1,0]{}}%
 \expandafter\def\csname l#1\endcsname{\supermorphism{#2}[0,-1]{}}%
 \expandafter\def\csname r#1\endcsname{\supermorphism{#2}[0,1]{}}%
 \expandafter\def\csname uu#1\endcsname{\supermorphism{#2}[-2,0]{}}%
 \expandafter\def\csname dd#1\endcsname{\supermorphism{#2}[2,0]{}}%
 \expandafter\def\csname ll#1\endcsname{\supermorphism{#2}[0,-2]{}}%
 \expandafter\def\csname rr#1\endcsname{\supermorphism{#2}[0,2]{}}%
 \expandafter\def\csname ur#1\endcsname{\supermorphism{#2}[-1,1]{}}%
 \expandafter\def\csname ul#1\endcsname{\supermorphism{#2}[-1,-1]{}}%
 \expandafter\def\csname dr#1\endcsname{\supermorphism{#2}[1,1]{}}%
 \expandafter\def\csname dl#1\endcsname{\supermorphism{#2}[1,-1]{}}%
 \expandafter\def\csname uul#1\endcsname{\supermorphism{#2}[-2,-1]{}}%
 \expandafter\def\csname uur#1\endcsname{\supermorphism{#2}[-2,1]{}}%
 \expandafter\def\csname ull#1\endcsname{\supermorphism{#2}[-1,-2]{}}%
 \expandafter\def\csname urr#1\endcsname{\supermorphism{#2}[-1,2]{}}%
 \expandafter\def\csname ddl#1\endcsname{\supermorphism{#2}[2,-1]{}}%
 \expandafter\def\csname ddr#1\endcsname{\supermorphism{#2}[2,1]{}}%
 \expandafter\def\csname dll#1\endcsname{\supermorphism{#2}[1,-2]{}}%
 \expandafter\def\csname drr#1\endcsname{\supermorphism{#2}[1,2]{}}%
 \expandafter\def\csname uull#1\endcsname{\supermorphism{#2}[-2,-2]{}}%
 \expandafter\def\csname uurr#1\endcsname{\supermorphism{#2}[-2,2]{}}%
 \expandafter\def\csname ddll#1\endcsname{\supermorphism{#2}[2,-2]{}}%
 \expandafter\def\csname ddrr#1\endcsname{\supermorphism{#2}[2,2]{}}}
\newdir{=>}{!/5pt/\dir{=}!/2.5pt/\dir{=}*!/-5pt/\dir2{>}}
\xydef@\arrowobject#1{\def\Arrowobject@{#1}}
\xydef@\Arrowobject@{\dir{=>}}
\xydef@\twocell@{\toks6={3.5}\toks5={@}\toks7={@}\toks8={@}\toks3={f}%
 \tw@cell@ }
\xydef@\uppertwocell@{\toks6={7}\toks5={@}\toks7={@}\toks8={@}\toks3={o}%
 \tw@cell@ }
\xydef@\lowertwocell@{\toks6={-7}\toks5={@}\toks7={@}\toks8={@}\toks3={o}%
 \tw@cell@ }
\xydef@\compositemap@{\toks6={3.5}\toks5={@}\toks7={@}\toks8={@}\toks3={t}%
 \tw@cell@ }
\xydef@\tw@cell@@@{%
 \expandafter\ifx\the\toks6\omit\relax\toks6={}\else
 \expandafter\ifx\expandafter @\the\toks7\relax\expandafter\dimen@\the\toks6\p@
 \expandafter\if\the\toks3t\relax\dimen@=\p@
 \else\expandafter\if\the\toks3o\divide\dimen@\tw@
 \ifdim\dimen@<\z@ \dimen@ii-\p@ \advance\dimen@ii\dimen@
 \dimen@=\dimen@ii \else \dimen@\p@ \fi
 \else\dimen@\p@
 \fi\fi
 \edef\tmp@{\expandafter\removePT@\the\dimen@}%
 \expandafter\toks\expandafter7\expandafter{\tmp@}\fi
 \expandafter\ifx\expandafter @\the\toks8\relax
 \expandafter\dimen@\the\toks6\p@
 \expandafter\if\the\toks3t\relax\dimen@\p@
 \else\expandafter\if\the\toks3o\divide\dimen@\tw@
 \ifdim\dimen@<\z@ \dimen@ii-\p@ \advance\dimen@ii\dimen@
 \dimen@=\dimen@ii \else \dimen@\p@ \fi
 \else\dimen@\p@
 \fi\fi
 \edef\tmp@{\expandafter\removePT@\the\dimen@}%
 \expandafter\toks\expandafter8\expandafter{\tmp@}\fi
 \expandafter\ifx\expandafter @\the\toks5\relax
 \expandafter\dimen@\the\toks6\p@
 \expandafter\if\the\toks3o\divide\dimen@ by-4\relax
 \else\dimen@\z@\fi
 \edef\tmp@{\expandafter\removePT@\the\dimen@}%
 \expandafter\toks\expandafter5\expandafter{\tmp@}\fi
 \fi
 \twocellmod@ 
 \expandafter\if\the\toks3t\relax
 \edef\tmp@{.[\noexpand\twocell@@@@{\the\toks6}{\the\toks5}%
 {\the\toks7}{\the\toks8}{\the\toks3}%
 {\the\toks2}{\the\toks1}{\the\toks@}{\the\toks4}!!!].\afterMORPHISM}%
 \else
 \edef\tmp@{.[\noexpand\twocell@@@@{\the\toks6}{\the\toks5}%
 {\the\toks7}{\the\toks8}{\the\toks3}%
 {\the\toks1}{\the\toks2}{\the\toks@}{\the\toks4}!!!].\afterMORPHISM}%
 \fi 
 \toks@={\endgroup}%
 \expandafter\def\expandafter\next@\expandafter{%
 \expandafter\def\expandafter\twocellhead@\expandafter{\twocellhead@}}%
 \expandafter\addtotoks@\expandafter{\next@}%
 \expandafter\def\expandafter\next@\expandafter{%
 \expandafter\def\expandafter\twocelltail@\expandafter{\twocelltail@}}%
 \expandafter\addtotoks@\expandafter{\next@}%
 \expandafter\addtotoks@\expandafter{\expandafter\twocellPATH\tmp@}%
 \the\toks@ }%
\xydef@\twocellstyle{\scriptstyle}
\xydef@\droptwocelllabel@#1{\xyFN@\droptwocelllabel@@#1@!}
\xydef@\droptwocelllabel@@{%
 \ifx*\next\DN@*{\droptwocelldrop@}%
 \else\DN@##1@!{\droptwocelltext@{##1}}%
 \fi \next@ }
{\xyuncatcodes \gdef\next#1{\drop+!C{\twocellstyle #1}}}
\xylet@\droptwocelltext@=\next
\xydef@\droptwocelldrop@#1@!{\bgroup \let\xy@=\oxy@ 
 \let\objectstyle=\twocellstyle \drop#1{}%
 \edef\tmp@{\egroup \X@min=\the\X@min \X@max=\the\X@max
 \Y@min=\the\Y@min \Y@max=\the\Y@max}\tmp@ }
\xydef@\twocellhead#1{\def\twocellhead@{#1}}
\xydef@\twocelltail#1{\def\twocelltail@{#1}}
\xydef@\twocellhead@{\dir{>}}
\xydef@\twocelltail@{}
\xywarnifdefined\twocellmod@
\xydef@\tw@cell@{\begingroup
 \toks@={{}}\toks1={{}}\toks2={{}}\toks4={{}}%
 \def\twocellmod@{}\xyFN@\tw@@cell@}%
\xydef@\tw@@cell@{%
 \ifx\space@\next\expandafter\DN@\space{\xyFN@\tw@@cell@}%
 \else\ifx\bgroup\next \let\next@=\toks@\afterassignment\tw@@cell@@
 \else\ifx ^\next \DN@^##1{\toks@={##1}\nudgepos@71\tw@@cell@}%
 \else\ifx _\next \DN@_##1{\toks@={##1}\nudgepos@82\tw@@cell@}%
 \else\addLT@\ifx \next \addGT@{\addLT@\DN@##1}{%
 \toks6={##1}\ifx\omit##1\relax\toks3={t}\toks5={0}\fi\xyFN@\tw@@cell@}%
 \else\ifx\omit\next \DN@\omit{\omitarrows@\xyFN@\tw@@cell@}%
 \else\ifx~\next \DN@~{\xyFN@\whichCurveObject@}%
 \else \DN@{\xyFN@\tw@cell@@\empty @}%
 \fi\fi\fi\fi\fi\fi\fi%
 \next@ }
\xydef@\whichCurveObject@{%
 \ifx\space@\next\expandafter\DN@\space{\xyFN@\whichCurveObject@}%
 \else\ifx\next^\DN@^##1{\xy@{~^{##1}}{\uppercurveobject{##1}}\xyFN@\tw@@cell@}%
 \else\ifx\next_\DN@_##1{\xy@{~_{##1}}{\lowercurveobject{##1}}\xyFN@\tw@@cell@}%
 \else\addRQ@\ifx\next \addRQ@\DN@##1{%
 \xy@{~'{##1}}{\def\twocellhead@{##1}}\xyFN@\tw@@cell@}%
 \else\addLQ@\ifx\next \addLQ@\DN@##1{%
 \xy@{~`{##1}}{\def\twocelltail@{##1}}\xyFN@\tw@@cell@}%
 \else\ifx!\next \DN@!{\xyFN@\checkmodmap@}%
 \else\ifx\next\bgroup\DN@##1{\xy@{~{##1}}{\curveobject{##1}}\xyFN@\tw@@cell@}%
 \else\DN@##1{\xy@{~##1}{\curveobject{##1}}\xyFN@\tw@@cell@}%
 \fi\fi\fi\fi \fi\fi\fi 
 \next@ }
\xydef@\checkmodmap@{%
 \ifx\space@\next\expandafter\DN@\space{\xyFN@\checkmodmap@}%
 \else \def\twocellmod@{\modmap@}%
 \ifx\next!\DN@!##1{%
 \xy@{~!!{##1}}{\def\modmapobject@{##1}}\xyFN@\tw@@cell@}%
 \else \DN@{\xyFN@\tw@@cell@}\fi
 \fi \next@ }
\xydef@\omitarrows@{\toks5={0}\toks6={}\toks7={0}\toks8={0}}
\xydef@\tw@@cell@@{\expandafter\xyFN@\expandafter\tw@cell@@\the\toks@ @}
\xydef@\tw@cell@@{\ifx \space@\next\expandafter\DN@\space{\xyFN@\tw@cell@@}%
 \else\ifx ^\next 
 \DN@^##1@{\toks@={##1}\toks4={^}\nudgepos@50\tw@cell@@@}%
 \else\addEQ@\ifx\next 
 \addEQ@\DN@##1@{\toks@={##1}\toks4={=}\nudgepos@50\tw@cell@@@}%
 \else\ifx _\next 
 \DN@_##1@{\toks@={##1}\toks4={_}\nudgepos@50\tw@cell@@@}%
 \else\addLT@\ifx \next 
 \DN@##1@{\toks@={##1}\toks4={_}\nudgepos@50\tw@cell@@@}%
 \else\ifx\omit\next \DN@\omit##1@{\toks4={@}\toks@={##1}\tw@cell@@@}%
 \else\addRQ@\ifx\next \addRQ@\DN@##1@{\toks4={@}\toks3={/}\toks@={##1}%
 \nudgepos@50\tw@cell@@@}%
 \else\addLQ@\ifx\next \addLQ@\DN@##1@{\toks4={@}\toks3={b}\toks@={##1}%
 \nudgepos@50\tw@cell@@@}%
 \else\ifx"\next \DN@"##1@{\toks4={@}\toks3={B}\toks@={##1}%
 \nudgepos@50\tw@cell@@@}%
 \else\ifx!\next \DN@!##1@{\toks4={@}\toks3={@}\toks@={##1}%
 \nudgepos@50\tw@cell@@@}%
 \else\ifx\next\empty\DN@##1@{\toks@={{}}\toks4={_}\tw@cell@@@}%
 \else\DN@##1@{\toks@={##1}\toks4={_}\tw@cell@@@}%
 \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi \next@ }
\xywarnifdefined\whichnudge
\xywarnifdefined\whichinfo
\xywarnifdefined\afternudge
\xydef@\nudgepos@#1#2#3{\def\whichnudge{\toks#1}\def\whichinfo{\toks#2}%
 \def\afternudge{#3}\expandafter\xyFN@\expandafter\nudgepos@@\the\toks@ @}
\xydef@\nudgepos@@{\ifx \space@\next\expandafter\DN@\space{\xyFN@\nudgepos@}%
 \else\addLT@\ifx \next
 \addGT@{\addLT@\DN@##1}##2@{%
 \ifx\omit##1\relax\whichnudge={0}\whichinfo={}%
 \else\whichnudge={##1}\whichinfo={##2}\fi\xyFN@\afternudge}%
 \else \DN@##1@{\whichinfo={##1}\xyFN@\afternudge}%
 \fi\fi \next@ }
\xydef@\modmap@{%
 \expandafter\ifx\the\toks4@\toks4={!}%
 \else\expandafter\ifx\the\toks4=\toks4={H}%
 \else\expandafter\ifx\the\toks4^\toks4={A}%
 \else\expandafter\ifx\the\toks4_\toks4={V}\fi\fi\fi\fi 
 \expandafter\DN@\expandafter{\the\toks6}%
 \ifx\next@\empty\relax\else\expandafter\moddefs@\fi}
\xydef@\moddefs@{%
 \expandafter\dimen@\the\toks6\p@
 \ifdim\dimen@=\z@\relax
 \expandafter\dimen@\the\toks7\p@
 \ifdim\dimen@<\z@\advance\dimen@.5\p@\else\advance\dimen@-.5\p@\fi
 \edef\tmp@{\noexpand\toks7={\expandafter\removePT@\the\dimen@}}\tmp@
 \expandafter\dimen@\the\toks8\p@
 \ifdim\dimen@<\z@\advance\dimen@-.5\p@\else\advance\dimen@.5\p@\fi
 \expandafter\ifx\the\toks3t\advance\dimen@-1\p@\fi
 \edef\tmp@{\noexpand\toks8={\expandafter\removePT@\the\dimen@}}\tmp@
 \else
 \ifdim\dimen@<\z@\advance\dimen@-.5\p@\else\advance\dimen@.5\p@\fi
 \edef\tmp@{\noexpand\toks6={\expandafter\removePT@\the\dimen@}}\tmp@
 \expandafter\dimen@\the\toks7\p@
 \ifdim\dimen@<\z@\advance\dimen@-.5\p@\else\advance\dimen@.5\p@\fi
 \expandafter\ifx\the\toks3t\advance\dimen@-2\p@\fi
 \edef\tmp@{\noexpand\toks7={\expandafter\removePT@\the\dimen@}}\tmp@
 \expandafter\dimen@\the\toks8\p@
 \ifdim\dimen@<\z@\advance\dimen@-.5\p@\else\advance\dimen@.5\p@\fi
 \expandafter\ifx\the\toks3t\advance\dimen@-2\p@\fi
 \edef\tmp@{\noexpand\toks8={\expandafter\removePT@\the\dimen@}}\tmp@
 \fi }%
\xydef@\modmapobject#1{\def\modmapobject@{#1}}
\xydef@\modmapobject@{\dir{|}}
\xydef@\@modmapobject@{{\if\@mod@\relax\expandafter\empty
 \else\expandafter\modmapobject@\fi}} 
\xydef@\curveobject#1{\def\ucurveObject@{~*#1}\def\dcurveObject@{~*#1}}
\xydef@\uppercurveobject#1{\def\ucurveObject@{~*#1}}
\xydef@\lowercurveobject#1{\def\dcurveObject@{~*#1}}
\xydef@\ucurveObject@{}
\xydef@\dcurveObject@{}
\xydef@\savetwocellobjects{%
 \xy@{twocell objects}{%
 \expandafter\uppercurveobject\expandafter{\ucurveObject@}%
 \expandafter\lowercurveobject\expandafter{\dcurveObject@}%
 \expandafter\modmapobject\expandafter{\modmapobject@}%
 \expandafter\twocellhead\expandafter{\twocellhead@}%
 \expandafter\twocelltail\expandafter{\twocelltail@}%
 \expandafter\arrowobject\expandafter{Arrowobject@}%
 }}
\xydef@\twocell@path.[#1].{%
 \expandafter\ifx\csname Q@@c\endcsname\relax
 \DN@{\enter@{\cfromthec@ \pfromthep@ \basefromthebase@}%
 \xy@{}{\expandafter\edef\csname Q@@\endcsname{\cfromthec@}}%
 \afterPOS{\xy@{}%
 {\expandafter\edef\csname Q@@c\endcsname{\cfromthec@}}%
 \xy@{}%
 {\cfromid@{@}\expandafter\edef\csname Q@@p\endcsname{\cfromthec@}}%
 \xy@{twocell #1}{#1}\leave@\aftertwoCELL};p,}%
 \else 
 \DN@{\enter@{\cfromthec@ \pfromthep@ \basefromthebase@}%
 \xy@{twocell #1}{#1}\leave@\aftertwoCELL}%
 \fi \next@ }
\xydef@\twocellpath.[#1].{%
 \expandafter\edef\csname Q@@p\endcsname{\cfromthec@}%
 \xy@{}{\enter@{\pfromthep@}}%
 \xy@{}{\enter@{\cfromthec@ \pfromthep@ \basefromthebase@}%
 \enter@{\pfromthec@}}%
 \afterPOS{\xy@{}{\leave@\setupDirection@}#1\restore\restore
 \xy@{end of 2-cell}\xysaveMinMax@ }}%
\xydef@\xysaveMinMax@{\edef\tmp@{\endgroup
 \noexpand\ifdim\X@max<\the\X@max \X@max=\the\X@max\noexpand\fi 
 \noexpand\ifdim\X@min>\the\X@min \X@min=\the\X@min\noexpand\fi 
 \noexpand\ifdim\Y@max<\the\Y@max \Y@max=\the\Y@max\noexpand\fi 
 \noexpand\ifdim\Y@min>\the\Y@min \Y@min=\the\Y@min\noexpand\fi 
 }\tmp@ }
\xylet@\twocellPATH=\twocellpath
\xydef@\aftertwo@CELL{\let\twocellPATH=\twocellpath \def\aftertwoCELL{}}
\xydef@\aftertwoCELL{}
\xydef@\twocell@@@@#1!!!{\xy@{twocell #1}{\twocell@@#1!!!}}
\let\xystatus=\xystatus@
\xydef@\twocell{\hbox\bgroup\@twocell}
\xydef@\uppertwocell{\hbox\bgroup\@uppertwocell}
\xydef@\lowertwocell{\hbox\bgroup\@lowertwocell}
\xydef@\compositemap{\hbox\bgroup\@compositemap}
\xydef@\twocelll#1#{\hbox\bgroup\xy@\save\save@\@twocelll{#1}}
\xydef@\@twocelll#1#2{%
 \afterPOS{\@twocelll@\xyFN@\twocell@#1{#2}}}
\xydef@\uppertwocelll#1#{\hbox\bgroup\xy@\save\save@\@uppertwocelll{#1}}
\xydef@\@uppertwocelll#1#2{%
 \afterPOS{\@twocelll@\xyFN@\uppertwocell@#1{#2}}}
\xydef@\lowertwocelll#1#{\hbox\bgroup\xy@\save\save@\@lowertwocelll{#1}}
\xydef@\@lowertwocelll#1#2{%
 \afterPOS{\@twocelll@\xyFN@\lowertwocell@#1{#2}}}
\xydef@\compositemapp#1#{\hbox\bgroup\xy@\save\save@\@compositemapp{#1}}
\xydef@\@compositemapp#1#2{%
 \afterPOS{\@twocelll@\xyFN@\compositemap@#1{#2}}}
\xydef@\@twocelll@{%
 \expandafter\edef\csname Q@@c\endcsname{\cfromthec@}\swap@
 \expandafter\edef\csname Q@@p\endcsname{\cfromthec@}\swap@
 \let\twocellPATH=\twocell@path
 \def\aftertwoCELL{\twocell@DONE \xy@\restore \leave@ 
 }}
\xydef@\@twocell#1{\DN@{\@twocell@\twocell@}\xyFN@\next@[#1]}
\xydef@\@uppertwocell#1{\DN@{\@twocell@\uppertwocell@}\xyFN@\next@[#1]}
\xydef@\@lowertwocell#1{\DN@{\@twocell@\lowertwocell@}\xyFN@\next@[#1]}
\xydef@\@compositemap#1{\DN@{\@twocell@\compositemap@}\xyFN@\next@[#1]}
\xydef@\@twocell@#1{\ifx\next[\DN@[{\toks@={#1}\xyFN@\@@twocell@}%
 \else\DN@{#1{}}\fi
%% 
 \expandafter\edef\csname Q@@c\endcsname{\cfromthec@}\swap@
 \expandafter\edef\csname Q@@p\endcsname{\cfromthec@}\swap@
 \let\twocellPATH=\twocell@path
 \def\aftertwoCELL{\twocell@DONE}\next@}
\xydef@\@@twocell@{\ifx\next\bgroup\DN@##1]{\the\toks@{##1}}%
 \else\DN@##1]{\the\toks@##1}\fi\next@}
%% \DN@{\twocell}%
%% \expandafter\def\csname*dir@@\codeof\next@ @\endcsname{\@twocell}
%% \DN@{\uppertwocell}%
%% \expandafter\def\csname*dir@@\codeof\next@ @\endcsname{\@uppertwocell}
%% \DN@{\lowertwocell}%
%% \expandafter\def\csname*dir@@\codeof\next@ @\endcsname{\@lowertwocell}
%% \DN@{\compositemap}%
%% \expandafter\def\csname*dir@@\codeof\next@ @\endcsname{\@compositemap}
\xydef@\twocell@DONE{%
 \edef\tmp@{\egroup \X@min=\the\X@min \X@max=\the\X@max
 \Y@min=\the\Y@min \Y@max=\the\Y@max}\tmp@
 \L@c=\X@c \advance\L@c-\X@min \R@c=\X@max \advance\R@c-\X@c
 \D@c=\Y@c \advance\D@c-\Y@min \U@c=\Y@max \advance\U@c-\Y@c
 \ht\z@=\U@c \dp\z@=\D@c \dimen@=\L@c \advance\dimen@\R@c \wdz@=\dimen@
 \computeLeftUpness@
\setboxz@h{\kern-\X@p \raise-\Y@c\boxz@ }%
\dimen@=\L@c \advance\dimen@\R@c \wdz@=\dimen@ \ht\z@=\U@c \dp\z@=\D@c 
 \Edge@c={\rectangleEdge}\Invisible@false \Hidden@false
 \edef\Drop@@{\noexpand\drop@Twocell
 \noexpand\def\noexpand\Leftness@{\Leftness@}%
 \noexpand\def\noexpand\Upness@{\Upness@}}%
 \edef\Connect@@{\noexpand\connect@Twocell
 \noexpand\ifdim\X@max<\the\X@max \X@max=\the\X@max\noexpand\fi 
 \noexpand\ifdim\X@min>\the\X@min \X@min=\the\X@min\noexpand\fi 
 \noexpand\ifdim\Y@max<\the\Y@max \Y@max=\the\Y@max\noexpand\fi 
 \noexpand\ifdim\Y@min>\the\Y@min \Y@min=\the\Y@min\noexpand\fi }}%
\xydef@\drop@Twocell{\boxz@ }
\xydef@\connect@Twocell{%
 \setboxz@h{\kern\X@p \raise\Y@c\box\lastobjectbox@ }%
 \wdz@=\z@ \ht\z@=\z@ \dp\z@=\z@ \Drop@@ }
\xywarnifdefined\@mod@
\xywarnifdefined\Arrowtok@
\xydef@\twocell@@#1#2#3#4#5#6#7#8#9!!!{%
 \def\@mod@{@}\DN@{#9}%
 \ifx #9!\def\Arrowtok@{@}\else\ifx #9A\def\Arrowtok@{^}%
 \else\ifx #9V\def\Arrowtok@{_}\else\ifx #9H\def\Arrowtok@{=}%
 \else\def\@mod@{\relax}%
 \ifx #5/\def\Arrowtok@{@}\else\ifx #5b\def\Arrowtok@{@}%
 \else\ifx #5B\def\Arrowtok@{@}\else\ifx #5@\def\Arrowtok@{@}%
 \else\def\Arrowtok@{#9}%
 \fi\fi\fi\fi\fi\fi\fi\fi
 \addEQ@\ifx #9\def\Arrowtok@{=}\fi
 \DN@{\omit}\ifx\next@\Arrowtok@\def\Arrowtok@{}\else
 \edef\Arrowtok@{\codeof\Arrowtok@}\fi
 \save@ \idfromc@{@c}\swap@\idfromc@{@p}\swap@
 \cfromid@{@c}\no@@
 \ifdim \X@c<\X@p \X@min=\X@c \X@max=\X@p \else \X@min=\X@p \X@max=\X@c \fi
 \ifdim \Y@c<\Y@p \Y@min=\Y@c \Y@max=\Y@p \else \Y@min=\Y@p \Y@max=\Y@c \fi
 \Calong@@{.5}\idfromc@{@m}\idfromc@{@m1}\idfromc@{@m2}%
 \ifx #5t\relax 
 \enter@{\cplusthec@\pfromthep@}%
 \enter@\DirectionfromtheDirection@ \begingroup\aboveDirection@ \xydashl@
 \DN@{#1}\ifx\next@\empty\dimen@=\z@\else\dimen@=#1\p@\fi
 \ifdim\dimen@=\z@ \DN@{\vfromslide@i{\xydashl@}@}\relax
 \else\DN@{\vfromslide@i{#1\xydashl@}@}\fi \next@
 \czeroEdge@ \leave@ \no@@ \drop@{+}{}\idfromc@{@m1}%
 \DN@{#1}\ifx\next@\empty\DN@{\no@@}\else\DN@{\connect@{\dir}{-}}\fi
 \else 
 \DN@{#1}\ifx\next@\empty\dimen@=\z@\else\dimen@=#1\p@\fi
 \ifdim\dimen@=\z@ \enter@{\cplusthec@\pfromthep@}%
 \enter@\DirectionfromtheDirection@ \begingroup\aboveDirection@\xydashl@
 \vfromslide@i{\xydashl@}@\czeroEdge@ \leave@ \idfromc@{@m1}%
 \cfromid@{@p}\swap@\cfromid@{@c}%
 \DN@{#1}\ifx\next@\empty\DN@{\no@@}\else\DN@{\connect@{\dir}{-}}\fi
 \else \DN@{\enter@\cplusthec@ 
 \enter@\DirectionfromtheDirection@ \begingroup\aboveDirection@ \xydashl@
 \vfromslide@i{#1\xydashl@}@\czeroEdge@ \leave@
 \idfromc@{@m1}\cfromid@{@p}\swap@\cfromid@{@c}%
 \edef\next@{\codeof\ucurveObject@}%
 \ifx\next@\empty\DN@{\connect@\crv{"@m1"}}%
 \else 
 \DNii@####1{\connect@\crv{####1}}\expandafter\DN@\expandafter{%
 \expandafter\nextii@\expandafter{\ucurveObject@"@m1"}}%
 \fi \next@ }%
%% \ifx\next@\empty\def\ucurveObject@{.}\fi
%% \enter@\cfromthec@\sinit@\cfromid@{@m1}\senter@\leave@
%% \expandafter\connect@\expandafter\crvs\expandafter{\ucurveObject@}%
%% \sinit@\sleave@ }%
 \fi
 \fi \next@ 
 \DN@{#1}\ifx\next@\empty\relax\else
 \if\@mod@ @\relax 
 \enter@\pfromthep@ \Creset@@
 \ifx #5t\relax
 \PLACEedgec@ \PLACEedgep@ \def\PLACEf@{{.5}}%
 \else \def\next@{\crvreset@}%
 \ifx\next@\Creset@@
 \gettwocelledges@ \edef\PLACEf@{{\expandafter\removePT@\the\dimen@}}%
 \else \PLACEedgec@ \PLACEedgep@ \def\PLACEf@{{.5}}\fi 
 \fi
 \expandafter\Calong@@\PLACEf@ \czeroEdge@ \leave@
 \edef\tmp@{\codeof\modmapobject@}%
 \ifx\tmp@\empty \DN@{\drop@{\dir}{|}}%
 \else \DNii@##1##{\drop@{##1}}%
 \DN@{\expandafter\nextii@\modmapobject@{}}%
 \fi \next@ 
 \fi\fi
 \DN@{#6}\ifx\next@\empty\DN@{\relax}\else
 \DNii@{{}}\ifx\next@\nextii@\DN@{\relax}\else
 \ifx @#3\relax\DN@{\relax}\else
 \DN@{\enter@\pfromthep@ \Creset@@
 \Calong@@{.5}\czeroEdge@ \leave@
 \enter@\cplusthec@ 
 \enter@\DirectionfromtheDirection@\begingroup
 \DN@{#1}\ifx\next@\empty\dimen@\z@\else\dimen@=#1\p@\fi
 \ifdim\dimen@<\z@ \belowDirection@ \xydashl@ 
 \else \aboveDirection@ \xydashl@ \fi
 \dimen@=#3\p@ \if\@mod@ @\relax 
 \advance\dimen@\ifdim\dimen@<\z@-\fi.5\p@\fi
 \edef\next@{\expandafter\removePT@\the\dimen@}%
 \expandafter\vfromslide@i\expandafter{\next@\xydashl@}@\leave@
 \droptwocelllabel@{#6}}%
 \fi\fi\fi \next@ 
 \DN@{#1}\ifx\next@\empty\relax\else
 \ifx #5b\relax
 \enter@ {\pfromthep@ }\Creset@@ \PLACEedgep@
 \Calong@@{0}\czeroEdge@ \leave@
 \edef\next@{\codeof\twocelltail@}%
 \ifx\next@\empty \DN@{\dir{>}}%
 \ifx\next@\twocellhead@\drop@{\dir}{<}%
 \else 
 \reverseDirection@ \DNii@##1##{\drop@{##1}}%
 \expandafter\nextii@\twocellhead@{}\reverseDirection@
 \fi
 \else 
 \DNii@##1##{\drop@{##1}}\expandafter\nextii@\twocelltail@{}%
 \fi
 \else\ifx #5@\relax
 \else
 \enter@\pfromthep@ \Creset@@ \PLACEedgec@
 \Calong@@{1}\czeroEdge@ \leave@
 \edef\next@{\codeof\twocellhead@}%
 \ifx\next@\empty\drop@{\dir}{>}%
 \else 
 \DNii@##1##{\drop@{##1}}\expandafter\nextii@\twocellhead@{}%
 \fi
 \ifx #5B\relax
 \enter@ {\pfromthep@ }\Creset@@ \PLACEedgep@
 \Calong@@{0}\czeroEdge@ \leave@
 \edef\next@{\codeof\twocelltail@}%
 \ifx\next@\empty \DN@{\dir{>}}%
 \ifx\next@\twocellhead@\drop@{\dir}{<}%
 \else 
 \reverseDirection@\DNii@##1##{\drop@{##1}}%
 \expandafter\nextii@\twocellhead@{}\reverseDirection@
 \fi
 \else 
 \DNii@##1##{\drop@{##1}}\expandafter\drop\twocelltail@{}%
 \fi
 \else\ifx #5/\relax
 \else \edef\next@{\codeof\twocelltail@}%
 \ifx\next@\empty\relax\else 
 \enter@\pfromthep@ \Creset@@ \PLACEedgep@
 \Calong@@{0}\czeroEdge@ \leave@
 \DNii@##1##{\drop@{##1}}\expandafter\nextii@\twocelltail@{}%
 \fi\fi\fi
 \fi\fi\fi 
 \cfromid@{@p}\swap@\cfromid@{@c}\no@@ \cfromid@{@m}%
 \ifx #5t\relax 
 \idfromc@{@m2}\cfromid@{@m1}\swap@ \cfromid@{@c}\no@@
 \DN@{#1}\ifx\next@\empty\DN@{\no@@}\else\DN@{\connect@{\dir}{-}}\fi
 \else\ifx #5o\relax
 \idfromc@{@m2}\DN@{}%
 \else
 \DN@{#1}\ifx\next@\empty\dimen@=\z@\else\dimen@=#1\p@\fi
 \ifdim\dimen@=\z@
 \enter@{\cplusthec@\pfromthep@}%
 \enter@\DirectionfromtheDirection@ \begingroup \belowDirection@\xydashl@
 \vfromslide@i{\xydashl@}@\czeroEdge@ \leave@ \idfromc@{@m2}%
 \DN@{\cfromid@{@p}\swap@\cfromid@{@c}\no@@}%
 \else \DN@{\enter@\cplusthec@
 \enter@\DirectionfromtheDirection@ \begingroup \belowDirection@ \xydashl@
 \vfromslide@i{#1\xydashl@}@\czeroEdge@ \leave@
 \idfromc@{@m2}\cfromid@{@p}\swap@\cfromid@{@c}%
 \edef\next@{\codeof\dcurveObject@}%
 \ifx\next@\empty\DN@{\connect@\crv{"@m2"}}%
 \else 
 \DNii@####1{\connect@\crv{####1}}\expandafter\DN@\expandafter{%
 \expandafter\nextii@\expandafter{\dcurveObject@"@m2"}}%
 \fi \next@ }\fi
%% \enter@\cfromthec@\sinit@\cfromid@{@m2}\senter@\leave@
%% \expandafter\connect@\expandafter\crvs\expandafter{\dcurveObject@}%
%% \sinit@\sleave@ 
%% }\fi
 \fi\fi \next@ 
 \DN@{#1}\ifx\next@\empty\relax\else \ifx #5o\relax\else
 \if\@mod@ @\DN@{\enter@\pfromthep@ \Creset@@ 
 \ifx #5t\relax
 \PLACEedgec@ \PLACEedgep@ \def\PLACEf@{{.5}}%
 \else \def\next@{\crvreset@}%
 \ifx\next@\Creset@@
 \gettwocelledges@ \edef\PLACEf@{{\expandafter\removePT@\the\dimen@}}%
 \else \PLACEedgec@ \PLACEedgep@ \def\PLACEf@{{.5}}\fi 
 \fi
 \expandafter\Calong@@\PLACEf@ \czeroEdge@ \leave@
 \edef\tmp@{\codeof\modmapobject@}\ifx\tmp@\empty\DN@{\drop@{\dir}{|}}%
 \else \DNii@####1####{\drop@{####1}}%
 \DN@{\expandafter\nextii@\modmapobject@{}}\fi
 \next@ }\else\DN@{\relax}\fi
 \next@ \fi\fi
 \DN@{#7}\ifx\next@\empty\DN@{\relax}\else
 \DNii@{{}}\ifx\next@\nextii@\DN@{\relax}\else
 \ifx @#4\relax\DN@{\relax}\else
 \DN@{\enter@\pfromthep@ \Creset@@
 \Calong@@{.5}\czeroEdge@ \leave@
 \enter@\cplusthec@ 
 \enter@\DirectionfromtheDirection@ \begingroup
 \DN@{#1}\ifx\next@\empty\dimen@\z@ \else\dimen@=#1\p@\fi
 \ifx #5t\relax \ifdim\dimen@<\z@ \belowDirection@ \xydashl@
 \else \aboveDirection@ \xydashl@ \fi
 \else \ifdim\dimen@<\z@ \aboveDirection@ \xydashl@ 
 \else \belowDirection@ \xydashl@ \fi
 \fi \dimen@=#4\p@ \if\@mod@ @\relax 
 \advance\dimen@\ifdim\dimen@<\z@-\fi.5\p@\fi
 \edef\next@{\expandafter\removePT@\the\dimen@}%
 \expandafter\vfromslide@i\expandafter{\next@\xydashl@}@\leave@
 \droptwocelllabel@{#7}}%
 \fi\fi\fi \next@
 \DN@{#1}\ifx\next@\empty\relax\else
 \ifx #5o\relax
 \else\ifx #5b\relax
 \enter@ {\pfromthep@ }\Creset@@ \PLACEedgec@ 
 \Calong@@{1}\czeroEdge@ \leave@ 
 \edef\next@{\codeof\twocelltail@}%
 \ifx\next@\empty \DN@{\dir{>}}%
 \ifx\next@\twocellhead@\drop@{\dir}{>}%
 \else 
 \DNii@##1##{\drop@{##1}}\expandafter\nextii@\twocellhead@{}%
 \fi
 \else
 \DNii@##1##{\drop@{##1}}\expandafter\drop\twocelltail@{}%
 \fi
 \else\ifx #5/\relax
 \enter@{\pfromthep@}\Creset@@ \PLACEedgep@
 \Calong@@{0}\czeroEdge@ \leave@
 \edef\next@{\codeof\twocelltail@}%
 \ifx\next@\empty \DN@{\dir{>}}%
 \ifx\next@\twocellhead@\drop@{\dir}{<}%
 \else 
 \reverseDirection@\DNii@##1##{\drop@{##1}}%
 \expandafter\nextii@\twocellhead@{}\reverseDirection@
 \fi
 \else
 \DNii@##1##{\drop@{##1}}\expandafter\nextii@\twocelltail@{}%
 \fi
 \else\ifx #5@\relax
 \else
 \enter@\pfromthep@ \Creset@@ \PLACEedgec@
 \Calong@@{1}\czeroEdge@ \leave@
 \edef\next@{\codeof\twocellhead@}%
 \ifx\next@\empty\drop@{\dir}{>}%
 \else
 \DNii@##1##{\drop@{##1}}\expandafter\nextii@\twocellhead@{}%
 \fi
 \ifx #5B\relax
 \enter@ {\pfromthep@ }\Creset@@ \PLACEedgep@
 \Calong@@{0}\czeroEdge@ \leave@
 \edef\next@{\codeof\twocelltail@}%
 \ifx\next@\empty\DN@{\dir{>}}%
 \ifx\next@\twocellhead@\drop@{\dir}{<}%
 \else 
 \reverseDirection@\DNii@##1##{\drop@{##1}}%
 \expandafter\nextii@\twocellhead@{}\reverseDirection@
 \fi
 \else
 \DNii@##1##{\drop@{##1}}\expandafter\nextii@\twocelltail@{}%
 \fi
 \else
 \edef\next@{\codeof\twocelltail@}%
 \ifx\next@\empty\relax\else
 \enter@ {\pfromthep@ }\Creset@@ \PLACEedgep@
 \Calong@@{0}\czeroEdge@ \leave@
 \DNii@##1##{\drop@{##1}}\expandafter\nextii@\twocelltail@{}%
 \fi\fi
 \fi\fi\fi
 \fi\fi
 \DN@{#1}\ifx\next@\empty\dimen@=\z@\else\dimen@=#1\p@\fi
 \ifdim\dimen@<\z@ \cfromid@{@m2}\swap@\cfromid@{@m1}%
 \else \cfromid@{@m1}\swap@\cfromid@{@m2}%
 \fi \no@@ \cfromid@{@m}%
 \ifx\Arrowtok@\empty
 \else\DN@{_}\edef\next@{\codeof\next@}\ifx\next@\Arrowtok@
 \enter@{\pfromthep@ \cplusthec@}\dimen@=#2\xydashl@ 
 \enter@\DirectionfromtheDirection@ \begingroup
 \expandafter\vfromslide@i\expandafter{\the\dimen@}@\czeroEdge@
 \leave@ \idfromc@{@m}%
 \DNii@##1##{\drop@{##1}}\expandafter\nextii@\Arrowobject@{}%
 \else\DN@{^}\edef\next@{\codeof\next@}\ifx\next@\Arrowtok@
 \DN@{_}\edef\Arrowtok@{\codeof\next@}%
 \enter@{\pfromthep@ \cplusthec@}\dimen@=#2\xydashl@ 
 \enter@\DirectionfromtheDirection@ \begingroup
 \expandafter\vfromslide@i\expandafter{\the\dimen@}@\czeroEdge@
 \leave@ \idfromc@{@m}\reverseDirection@
 \DNii@##1##{\drop@{##1}}\expandafter\nextii@\Arrowobject@{}%
 \else \DN@{=}\edef\next@{\codeof\next@}\ifx\next@\Arrowtok@
 \enter@{\pfromthep@ \cplusthec@}%
 \dimen@=#2\xydashl@ \advance\dimen@\xydashl@ 
 \enter@\DirectionfromtheDirection@ \begingroup
 \expandafter\vfromslide@i\expandafter{\the\dimen@}@\czeroEdge@
 \leave@ \idfromc@{@m2}%
 \cfromid@{@m}%
 \enter@{\pfromthep@ \cplusthec@}%
 \dimen@=#2\xydashl@ \advance\dimen@-\xydashl@ 
 \enter@\DirectionfromtheDirection@ \begingroup
 \expandafter\vfromslide@i\expandafter{\the\dimen@}@\czeroEdge@
 \leave@ \idfromc@{@m1}%
 \cfromid@{@m2}\swap@\cfromid@{@m1}\connect@{\dir 2}{-}%
 \fi\fi\fi\fi
 \DN@{#8}\ifx\next@\empty\DN@{}\else\DN@{%
 \ifx\Arrowtok@\empty
 \Calong@@{.5}%
 \else\DN@{=}\edef\next@{\codeof\next@}\ifx\next@\Arrowtok@
 \Calong@@{.5}%
 \else\DN@{_}\edef\next@{\codeof\next@}\ifx\next@\Arrowtok@
 \cfromid@{@m}%
 \fi\fi\fi
 \enter@\cplusthec@
 \enter@\DirectionfromtheDirection@ \begingroup \aboveDirection@\xydashl@
 \ifx\Arrowtok@\empty
 \def\tmp@{0pt}%
 \else\DN@{=}\edef\next@{\codeof\next@}\ifx\next@\Arrowtok@
 \def\tmp@{\xydashl@}%
 \else\DN@{_}\edef\next@{\codeof\next@}\ifx\next@\Arrowtok@
 \def\tmp@{1.2\xydashl@}%
 \else\def\tmp@{0pt}%
 \fi\fi\fi
 \expandafter\vfromslide@i\expandafter{\tmp@}@\czeroEdge@ \leave@
 \droptwocelllabel@{#8}%
 }\fi \next@ 
 \leave@ }%
\xydef@\gettwocelledges@{%
 \bgroup \the\crvpts@ 
 \edef\next@{\edges@}%
 \expandafter\gettwocelledges@@\next@ }
\xydef@\gettwocelledges@@#1;#2,#3;#4,{%
 \dimen@=#2\advance\dimen@-#4\relax
 \advance\dimen@ 2\p@ \divide\dimen@ by4 \relax
 \edef\next@{\egroup\dimen@=\the\dimen@ }\next@}%
\xyendinput


==> xyall.tex <==
%% xyall.tex from $Id: xyall.doc,v 3.3 1996/12/19 03:31:56 krisrose Exp $
%%
%% Xy-pic ``All features'' option.
%% Copyright (c) 1993-1996 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1996 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{all}{All features}{\stripRCS$Revision: 3.3 $}%
 {Kristoffer H.~Rose}{krisrose@brics.dk}%
 {BRICS/Computer Science, University of Aarhus, Ny Munkegade, building 540,
 DK--8000 Aarhus~C}
\xyrequire{curve}
\xyrequire{frame}
\xyrequire{cmtip}
\xyrequire{line}
\xyrequire{rotate}
\xyrequire{color}
\xyrequire{matrix}
\xyrequire{arrow}
\xyrequire{graph}
\xyendinput


==> xyarc.tex <==
%% xyarc.tex from $Id: xyarc.doc,v 3.4 1997/05/18 01:13:24 ross Exp $
%%
%% Xy-pic ``Circles, Ellipses and Arcs'' feature.
%% Copyright (c) 1995-1997 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1997 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The XY-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The XY-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{arc}{Circle, Ellipse, Arc feature}{\stripRCS$Revision: 3.4 $}%
 {Ross Moore}{ross@mpce.mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xyrequire{curve}
\xycatcodes
\xydef@\ellipse#1#{\xy@{ELLIPSE}{\hbox\bgroup\save@}%
 \let\endarc@=\endellipse@@ \xyFN@\preARC@ #1@}
\xydef@\endellipse@@{\xy@{endELLIPSE}{\leave@\origDirection@
 \edef\next@{\egroup \X@min=\the\X@min \X@max=\the\X@max
 \Y@min=\the\Y@min \Y@max=\the\Y@max }\next@}\let\bstartPLACE@=\relax}
\xydef@\preARC@{%
 \ifx\next\space@ \expandafter\DN@\space{\xyFN@\preARC@}%
 \else\ifx\next @\DN@{\xy@{ellipseARC}\ellipticARC@ \arc@}%
 \else\ifx\next ~\DN@~##1{\tildeARC@{##1}}%
 \else\DN@{\xy@{ellipticARC}\ellipticARC@ \arc@}%
 \fi\fi\fi \next@ }
\xydef@\arc@#1@#2{\DN@{#2}%
 \ifx\next@\empty \xy@{arcSTYLE}{\def\arcSTYLE{-}}%
 \else \xy@{arcSTYLE}{\def\arcSTYLE{#2}}\fi \arc@i
 \DNii@{#1}%
 \ifx\nextii@\empty \DN@{\fullCircle@}%
 \else \DN@{_}%
 \ifx\next@\nextii@ \xy@{_}{\def\arcOrient@@{_}}%
 \let\arcOrient@@=\next@ \DN@{\fullCircle@}%
 \else \DN@{^}%
 \ifx\next@\nextii@ \xy@{^}{\def\arcOrient@@{^}}%
 \let\arcOrient@@=\next@ \DN@{\fullCircle@}%
 \else \DN@{\def\afterARCextents@@{%
 \xy@{aftARCext}{\let\doCircleArc@=\doCircleArc@@}%
 \ellipseArc@ \xy@{doCircARCs}{\doCircleArcs@}\endarc@ }%
 \xyFN@\getarcparams@#1@}\fi\fi\fi
 \next@ }
\xydef@\arc@i{\xy@{ARCi}{%
 \save@\idfromc@{0@c}\cfromp@\idfromc@{0@p}%
 \enter@\cplusthec@ \enter@\relax\begingroup\vfromslide@i{}@\czeroEdge@ 
 \leave@\idfromc@{0@m}\leave@ \zeroDivideLimit@{50}%
 \edef\origDirection@{\Direction=\the\Direction
 \relax\noexpand\imposeDirection@}%
 \let\startDirection@=\origDirection@ \def\startDirection@@{}%
 \def\endDirection@{}\def\endDirection@@{}\def\arcOrient@@{^}}%
 \def\arcOrient@@{^}\let\processDirections@=\checkstartDirection@ 
 \def\arcRadius@{}\def\ellipseRatio@{}\def\arcScale@{\arcScale@@}}
\message{circles,}
\xydef@\fullCircle@{\xy@{fullCIRC}{\let\endDirection@=\relax
 \let\doCircleArc@=\doMergeEndArc@@}\circleArc@ }%
\xydef@\getarcparams@{%
 \ifx\space@\next \expandafter\DN@\space{\xyFN@\getarcparams@}%
 \else\addLT@\ifx \next \xy@{<}{}%
 \addGT@{\addLT@\DN@##1}{\splitRadius@dim##1,,@}%
 \else\ifx\next (\DN@({\xyFN@\checkRadOpen@}%
 \else\ifx\next @\xy@{@}{}\DN@ @{\fullEllipse@}%
 \else \addLQ@\ifx \next \addLQ@\DN@{\xy@`{}\ARCturn@}%
 \else \DN@{\getarcExtents@}%
 \fi\fi\fi\fi\fi \next@ }
\xydef@\checkRadOpen@{%
 \ifx\next *\DN@{\xyFN@\getarcExtents@ (}%
 \else \xy@{(}{}\DN@##1){\splitRadius@##1,,@}%
 \fi \next@ }
\xydef@\fixedRadiusArc@{%
 \xy@{fixRadArc}{\save@ \idfromc@{0@0}\cfromp@\idfromc@{0@c}\leave@}%
 \xyFN@\fixedRadiusArc@i }
\xydef@\fixedRadiusArc@i{%
 \ifx\next\space@ \expandafter\DN@\space{\xyFN@\fixedRadiusArc@i}%
 \else\ifx\next @\xy@{@}{}\DN@ @{\fullEllipse@}%
 \else\DN@{\let\processDirections@=\processArcDirections@
 \def\afterARCextents@@{\xy@{aftARCext}{\let\doCircleArc@=\doCircleArc@@ 
 \ellipseSector@}}\xyFN@\getarcExtents@}%
 \fi\fi \next@ }
\xydef@\arcScale@@{\xy@{arcSCALE@@}{\save@
 \cfromid@{0@0}\pfromc@\cfromid@{0@p}\setbase@\X@p\Y@p\X@c\Y@c}}
\xydef@\arcScale@dim#1{\xy@{arcSCALEdim}{\save@
 \cfromid@{0@0}\pfromc@ \cfromid@{0@p}\setupDirection@\cfromp@
 \enter@\cplusthec@ \begingroup\vfromslide@i#1@%
 \setbase@\X@p\Y@p\X@c\Y@c \idfromc@{0@p}}}
\xydef@\ellipseScale@dim#1{\xy@{ellSCALEdim}{\setupDirection@\cfromp@ 
 \enter@\cplusthec@ \aboveDirection@\xydashl@ \vfromslide@{#1}\leave@
 \setbase@@\X@c\Y@c}}
\xydef@\ellipseScale@#1{\xy@{ellSCALE@}%
 {\vfromcartesian@@0,#1@\setbase@@\X@c\Y@c}}
\xydef@\splitRadius@dim#1,#2,#3@{%
 \DN@{#1}\ifx\next@\empty\dimen@=\z@\else\dimen@=#1\relax%\splinetracing 
 \expandafter\def\expandafter\arcRadius@
 \expandafter{\arcScale@dim{#1}}\fi
 \DN@{#2}\ifx\next@\empty\dimen@ii=\z@\def\ellipseRatio@{}%
 \else\dimen@ii=#2\relax \expandafter
 \def\expandafter\ellipseRatio@\expandafter{\ellipseScale@dim{#2}}%
 \fi \fixedRadiusArc@ }
\xydef@\splitRadius@#1,#2,#3@{%
 \DN@{#1}\ifx\next@\empty\dimen@=\z@\else\dimen@=#1\p@\relax\fi
 \DN@{#2}\ifx\next@\empty\dimen@ii=\z@\else\dimen@ii=#2\p@\relax\fi 
 \ifdim\dimen@=\z@ \ifdim\dimen@ii=\z@\else \expandafter
 \def\expandafter\ellipseRatio@\expandafter{\ellipseScale@{#2}}\fi
 \else
 \ifdim\dimen@ii=\z@
 \def\arcScale@{\xy@{arcSCALE@}{\save@\cfromid@{0@0}%
 \X@origin=\X@c \Y@origin=\Y@c
 \X@xbase=#1\X@xbase \Y@xbase=#1\Y@xbase
 \X@ybase=#1\X@ybase \Y@ybase=#1\Y@ybase 
 \advance\X@c\X@xbase \advance\Y@c\Y@xbase \czeroEdge@
 \idfromc@{0@p}\idfromc@{0@c}}}%
 \else
 \def\arcScale@{\xy@{arcSCALE@}{\save@\cfromid@{0@0}%
 \X@origin=\X@c \Y@origin=\Y@c
 \X@xbase=#1\X@xbase \Y@xbase=#1\Y@xbase
 \X@ybase=#2\X@ybase \Y@ybase=#2\Y@ybase 
 \advance\X@c\X@xbase \advance\Y@c\Y@xbase \czeroEdge@
 \idfromc@{0@p}\idfromc@{0@c}}}%
 \fi
 \fi \fixedRadiusArc@ }
\xydef@\baseOrient@{\DN@{_}\ifx\next@\arcOrient@@
 \X@ybase=-\X@ybase \Y@ybase=-\Y@ybase \fi }
\message{ellipses,}
\xydef@\fullEllipse@{\xy@{fullELLIPSE}%
 {\def\startDirection@{}\let\doCircleArc@=\doMergeEndArc@@}%
 \ellipseArc@
 \xy@{doCIRCarcs}{\leave@ \doCircleArcs@}\endarc@ }
\xydef@\ellipseArc@{%
 \arcScale@ \arcRadius@ \ellipseRatio@
 \xy@{arcCONTROLS}{\baseOrient@ \arcControls@ \let\bstartPLACE@=\relax }}
\xydef@\cubicARCcontrols@@{\czeroEdge@
 \vfromcartesian@@0,1@\idfromc@{1@c}%
 \vfromcartesian@@-1,0@\idfromc@{2@c}%
 \vfromcartesian@@0,-1@\idfromc@{3@c}%
 \vfromcartesian@@1,\arcparam@ @\idfromc@{1@m}%
 \vfromcartesian@@\arcparam@,1@\idfromc@{2@m}%
 \vfromcartesian@@-\arcparam@,1@\idfromc@{3@m}%
 \vfromcartesian@@-1,\arcparam@ @\idfromc@{4@m}%
 \vfromcartesian@@-1,-\arcparam@ @\idfromc@{5@m}%
 \vfromcartesian@@-\arcparam@,-1@\idfromc@{6@m}%
 \vfromcartesian@@\arcparam@,-1@\idfromc@{7@m}%
 \vfromcartesian@@1,-\arcparam@ @\idfromc@{8@m}%
 }
\xydef@\doCircleArc@@#1#2{\save@ \ifcase#2\relax
 \doCircleArc@@@{0@p}{1@m}{2@m}{1@c}{#1}\or
 \doCircleArc@@@{1@c}{3@m}{4@m}{2@c}{#1}\or
 \doCircleArc@@@{2@c}{5@m}{6@m}{3@c}{#1}\or
 \doCircleArc@@@{3@c}{7@m}{8@m}{0@p}{#1}\or
 \doCircleArc@@@{0@p}{1@m}{2@m}{1@c}{#1}\or
 \doCircleArc@@@{1@c}{3@m}{4@m}{2@c}{#1}\or
 \doCircleArc@@@{2@c}{5@m}{6@m}{3@c}{#1}\or
 \doCircleArc@@@{3@c}{7@m}{8@m}{0@p}{#1}\fi \leave@ }
\xydef@\doCircleArc@@@#1#2#3#4#5{%
 \cfromid@{#1}\pfromc@\senter@
 \cfromid@{#2}\spushc@\cfromid@{#3}\spushc@\cfromid@{#4}%
 \connect@\crvs{#5}\relax\sinit@\sleave@}
\xydef@\doMergeEndArc@@#1#2{\save@\ifcase#2\relax
 \doMergeEnd@@@{0@p}{1@m}{2@m}{1@c}{#1}\relax\or
 \doMergeEnd@@@{1@c}{3@m}{4@m}{2@c}{#1}\relax\or
 \doMergeEnd@@@{2@c}{5@m}{6@m}{3@c}{#1}\relax\or
 \doMergeEnd@@@{3@c}{7@m}{8@m}{0@p}{#1}@\fi \leave@ }
\xydef@\doMergeEnd@@@#1#2#3#4#5#6{%
 \cfromid@{#1}\pfromc@\senter@
 \cfromid@{#2}\spushc@\cfromid@{#3}\spushc@\cfromid@{#4}%
 \ifx#6\relax
 \L@c=.1\p@ \R@c=\L@c \U@c=\L@c \D@c=\L@c \Edge@c={\rectangleEdge}\fi
 \enter@\cmergethec@\cfromid@{0@c}\leave@
 \enter@\cmergethec@\cfromcontrols@{#1}{#2}{#3}{#4}\leave@
 \connect@\crvs{#5}\relax
 \sinit@\sleave@}
\xydef@\doMergeStartArc@#1#2{\save@\ifcase#2\relax
 \doMergeStart@@{0@p}{1@m}{2@m}{1@c}{#1}@\or
 \doMergeStart@@{1@c}{3@m}{4@m}{2@c}{#1}\relax\or
 \doMergeStart@@{2@c}{5@m}{6@m}{3@c}{#1}\relax\or
 \doMergeStart@@{3@c}{7@m}{8@m}{0@p}{#1}\relax\fi \leave@ }
\xydef@\doMergeStart@@#1#2#3#4#5#6{%
 \cfromid@{#1}\ifx#6\relax
 \L@c=.1\p@ \R@c=\L@c \U@c=\L@c \D@c=\L@c \Edge@c={\rectangleEdge}\fi
 \enter@\cmergethec@\cfromid@{0@x}\leave@
 \enter@\cmergethec@\cfromcontrols@{#4}{#3}{#2}{#1}\leave@
 \pfromc@
 \senter@ \cfromid@{#2}\spushc@\cfromid@{#3}\spushc@\cfromid@{#4}%
 \connect@\crvs{#5}\relax\sinit@\sleave@}
\xydef@\doMergeBothArc@#1#2{\save@\ifcase#2\relax
 \doMergeBoth@@{0@p}{1@m}{2@m}{1@c}{#1}@\or
 \doMergeBoth@@{1@c}{3@m}{4@m}{2@c}{#1}\relax\or
 \doMergeBoth@@{2@c}{5@m}{6@m}{3@c}{#1}\relax\or
 \doMergeBoth@@{3@c}{7@m}{8@m}{0@p}{#1}\relax\fi \leave@ }
\xydef@\doMergeBoth@@#1#2#3#4#5#6{%
 \cfromid@{#1}\ifx#6\relax
 \L@c=.1\p@ \R@c=\L@c \U@c=\L@c \D@c=\L@c \Edge@c={\rectangleEdge}\fi
 \enter@\cmergethec@\cfromid@{0@x}\leave@
 \enter@\cmergethec@\cfromcontrols@{#4}{#3}{#2}{#1}\leave@
 \pfromc@
 \senter@ \cfromid@{#2}\spushc@\cfromid@{#3}\spushc@\cfromid@{#4}%
 \enter@\cmergethec@\cfromid@{0@c}\leave@ 
 \enter@\cmergethec@\cfromcontrols@{#1}{#2}{#3}{#4}\leave@
 \connect@\crvs{#5}\relax\sinit@\sleave@}
\xydef@\doMergeEndArc@#1#2{\count@@=#2\relax
 \ifnum\count@@>\thr@@ \advance\count@@-4\fi\relax
 \doMergeEndArc@@{#1}\count@@ }
\xydef@\doStraightArc@@#1{\xy@{STRAITarc}{\save@
 \cfromid@{0@p}\pfromc@\cfromid@{0@c}%
 \senter@\connect@\crvs{#1}\sinit@\sleave@\leave@}}
\xydef@\cfromcontrols@#1#2#3#4{\bgroup
 \cfromid@{#1}\L@p=\X@c \U@p=\Y@c
 \cfromid@{#4}\R@p=\X@c \D@p=\Y@c
 \cfromid@{#3}\A@=\X@c \B@=\Y@c \cfromid@{#2}%
 \ifdim\R@p>\L@p \ifdim\A@>\R@p \R@p=\A@
 \ifdim\X@c>\R@p \R@p=\X@c\fi\fi
 \else \ifdim\A@<\R@p \R@p=\A@
 \ifdim\X@c<\R@p \R@p=\X@c\fi\fi
 \fi
 \ifdim\D@p>\U@p \ifdim\B@>\D@p \D@p=\B@
 \ifdim\Y@p>\D@p \D@p=\Y@p\fi\fi
 \else \ifdim\B@<\D@p \D@p=\B@
 \ifdim\Y@p<\D@p \D@p=\Y@p\fi\fi
 \fi 
 \edef\next@{\egroup \X@c=\the\R@p \Y@c=\the\D@p}\next@ }
\xydef@\doCircleArcs@{\save@
 \cfromid@{0@0}\pfromc@\cfromid@{0@p}\setupDirection@
 \startDirection@ \edef\startDirection@@{\the\Direction}%
 \cfromid@{1@c}\setupDirection@ \edef\quadDirection@{\the\Direction}\relax 
 \count@=\quadDirection@ \relax\def\nextii@{^}%
 \let\preDirection@@=\startDirection@@ 
 \ifx\nextii@\arcOrient@@
 \ifnum\quadDirection@>\startDirection@@ \relax
 \else \advance\count@ by8192 \relax\edef\quadDirection@{\the\count@}\fi
 \ifx\endDirection@@\empty
 \ifx\endDirection@\relax
 \bgroup\cfromid@{0@c}\setupDirection@
 \edef\next@{\egroup \count@@=\the\Direction}\next@ \relax
 \ifnum\count@@<\startDirection@@ \advance\count@@ 8192 \fi
 \edef\endDirection@@{\the\count@@}%
 \else
 \count@@=\startDirection@@
 \advance\count@@ by8192 \edef\endDirection@@{\the\count@@}%
 \fi
 \else 
 \count@@=\endDirection@@ \relax\ifnum\count@@<\startDirection@@ \relax
 \advance\count@@ by8192 \edef\endDirection@@{\the\count@@}\fi
 \fi
 \ifnum\endDirection@@>\quadDirection@
 \DN@{\expandafter\doCircleArc@@\expandafter{\arcSTYLE}{0}}%
 \else
 \DN@{\expandafter\doCircleArc@\expandafter{\arcSTYLE}{0}}%
 \fi
 \else
 \ifnum\count@<\startDirection@@\relax\else\advance\count@ by-8192 \relax
 \edef\quadDirection@{\the\count@}\fi
 \ifx\endDirection@@\empty
 \ifx\endDirection@\relax
 \bgroup\cfromid@{0@c}\setupDirection@
 \edef\next@{\egroup \count@@=\the\Direction}\next@ \relax
 \ifnum\count@@>\startDirection@@ \advance\count@@-8192 \fi
 \edef\endDirection@@{\the\count@@}%
 \else
 \count@@=\startDirection@@
 \advance\count@@ by-8192 \edef\endDirection@@{\the\count@@}%
 \fi
 \else 
 \count@@=\endDirection@@ \relax \ifnum\count@@>\startDirection@@
 \advance\count@@ by-8192 \edef\endDirection@@{\the\count@@}\fi
 \fi
 \ifnum\endDirection@@<\quadDirection@
 \DN@{\expandafter\doCircleArc@@\expandafter{\arcSTYLE}{0}}%
 \else \DN@{\expandafter\doCircleArc@\expandafter{\arcSTYLE}{0}}\fi
 \fi
 \next@ \relax
 \count@=\quadDirection@ \relax\def\nextii@{^}\DN@{}%
 \ifx\nextii@\arcOrient@@
 \count@@=\startDirection@@ \advance\count@@ by4096 \relax
 \ifnum \count@<\endDirection@@ \relax
 \ifnum\endDirection@@>\count@@
 \DN@{\expandafter\doCircleArc@@\expandafter{\arcSTYLE}{1}}%
 \else \DN@{\expandafter\doCircleArc@\expandafter{\arcSTYLE}{1}}\fi
 \fi
 \else 
 \count@@=\startDirection@@ \advance\count@@ by-4096 \relax
 \ifnum \count@>\endDirection@@ \relax 
 \ifnum\endDirection@@<\count@@
 \DN@{\expandafter\doCircleArc@@\expandafter{\arcSTYLE}{1}}%
 \else \DN@{\expandafter\doCircleArc@\expandafter{\arcSTYLE}{1}}\fi
 \fi\fi 
 \next@ \relax
 \ifx\next@\empty \else \relax
 \count@=\startDirection@@ \relax\def\nextii@{^}\DN@{}%
 \ifx\nextii@\arcOrient@@ \advance\count@ by4096 \relax
 \count@@=\quadDirection@ \advance\count@@ by4096 \relax
 \ifnum \count@<\endDirection@@ 
 \ifnum\endDirection@@>\count@@
 \DN@{\expandafter\doCircleArc@@\expandafter{\arcSTYLE}{2}}%
 \else \DN@{\expandafter\doCircleArc@\expandafter{\arcSTYLE}{2}}\fi
 \fi
 \else \advance\count@ by-4096 \relax
 \count@@=\quadDirection@ \advance\count@@ by-4096 \relax
 \ifnum \count@>\endDirection@@ \relax
 \ifnum\endDirection@@<\count@@
 \DN@{\expandafter\doCircleArc@@\expandafter{\arcSTYLE}{2}}%
 \else \DN@{\expandafter\doCircleArc@\expandafter{\arcSTYLE}{2}}\fi
 \fi\fi 
 \next@ \relax
 \fi
 \ifx\next@\empty \else \relax
 \count@=\quadDirection@ \def\nextii@{^}\DN@{}%
 \ifx\nextii@\arcOrient@@ \advance\count@ by4096 \relax
 \ifnum \count@<\endDirection@@
 \DN@{\expandafter\doCircleArc@\expandafter{\arcSTYLE}{3}}\fi
 \else \advance\count@ by-4096 \relax
 \ifnum \count@>\endDirection@@ 
 \DN@{\expandafter\doCircleArc@\expandafter{\arcSTYLE}{3}}\fi
 \fi \next@ \relax
 \fi
 \leave@ }
\message{elliptical arcs,}
\xydef@\arcmagic@@{0.5517847}
\xylet@\arcmagic=\arcmagic@@
\xydef@\tildeARC@#1{%
 \if q#1\DN@{\xy@{quadARC}\quadARC@ \arc@}%
 \else\if c#1\DN@{\xyFN@\cubicARC@i}%
 \else\if e#1\DN@{\xy@{ellipticARC}\ellipticARC@ \arc@}%
 \else\if i#1\DN@{\xy@{interpARC}\interpARC@ \arc@}%
 \else\if p#1\DN@{\xy@{cuspidalARC}\cuspidalARC@ \arc@}%
 \else\xywarning@{unknown arc type: #1 }%
 \DN@{\xy@{ellipticARC}\ellipticARC@ \arc@}%
 \fi\fi\fi\fi\fi \next@ }
\xydef@\cubicARC@i{%
 \ifx\next\space@ \expandafter\DN@\space{\xyFN@\cubicARC@i}%
 \else\ifx\next (\DN@(##1){\xy@{cubicARC(##1)}{\cubicARC@{##1}}\arc@}%
 \else \DN@{\xy@{cubicARC(1)}{\cubicARC@{1}}\arc@}%
 \fi\fi \next@ }
\xydef@\ellipticARC@{\let\arcControls@=\cubicARCcontrols@@
 \edef\arcparam@{\arcmagic@@}}
\xydef@\cubicARC@#1{\let\arcControls@=\cubicARCcontrols@@
 \dimen@=#1\p@ \edef\arcparam@{\expandafter\removePT@\the\dimen@}}
\xydef@\quadARC@{\let\arcControls@=\cubicARCcontrols@@
 \def\arcparam@{.66667}}
\xydef@\cuspidalARC@{\let\arcControls@=\cubicARCcontrols@@
 \def\arcparam@{2}}
\xydef@\interpARC@{\let\arcControls@=\cubicARCcontrols@@
 \def\arcparam@{1.33333}}
\xydef@\ARCturn@{\xy@@\bgroup\afterCOORD{%
 \xy@@{\edef\next@{\egroup \A@=\the\X@c \B@=\the\Y@c}\next@}\ARCturn@@}}
\xydef@\ARCturn@@#1@{\DN@{#1}\DNii@{^}%
 \ifx\next@\nextii@ \xy@{^}{\def\arcOrient@@{^}}%
 \else\DNii@{_}\ifx\next@\nextii@ \xy@{_}{\def\arcOrient@@{_}}%
 \else\xy@{}{\def\arcOrient@@{}}\fi\fi
 \xy@@\ARCturn@@@ \processDirections@@ }
\xydef@\ARCturn@@@{%
 \bgroup\cfromid@{0@p}\X@p=\X@c \Y@p=\Y@c \X@c=\A@ \Y@c=\B@
 \setupDirection@ \edef\next@{\egroup\count@=\the\Direction}\next@\relax
 \edef\startDirection@@{\the\count@ }%
 \bgroup\cfromid@{0@c}\X@p=\A@ \Y@p=\B@
 \setupDirection@ \edef\next@{\egroup\count@=\the\Direction}\next@\relax
 \edef\endDirection@@{\the\count@}%
 \ifx\arcOrient@@\empty
 \bgroup\cfromid@{0@p}\X@p=\X@c \Y@p=\Y@c \cfromid@{0@c}%
 \setupDirection@ \edef\next@{\egroup\count@@=\the\Direction}\next@\relax
 \count@=-\count@@ \advance\count@\startDirection@@ \relax \count@=-\count@
 \ifnum\count@>4096 \def\arcOrient@@{_}%
 \else\ifnum\count@<-4096 \def\arcOrient@@{^}%
 \else\ifnum\count@>\z@ \def\arcOrient@@{^}%
 \else\def\arcOrient@@{_}\fi\fi\fi
 \fi }
\xydef@\circleArc@{%
 \xy@{circARC@}{\cfromid@{0@p}\pfromc@\cfromp@\startDirection@ 
 \arcCenter@\idfromc@{0@0}%
 \def\startDirection@{\bgroup
 \cfromid@{0@0}\pfromc@\cfromid@{0@p}\setupDirection@ 
 \edef\next@{\egroup \Direction=\the\Direction}\next@
 \relax\imposeDirection@}}%
 \ifx\endDirection@@\empty
 \ifx\arcRadius@\empty \ifx\ellipseRatio@\empty\else
 \DN@{\arcScale@@}\ifx\arcScale@\next@\else
 \xy@@{\bgroup\cfromid@{0@0}\pfromc@\cfromid@{0@c}\setupDirection@
 \edef\next@{\egroup \Direction=\the\Direction}\next@ 
 \edef\endDirection@@{\the\Direction}}\fi\fi\fi\fi
 \ellipseArc@ \xy@@{\leave@ \doCircleArcs@}\endarc@ }
\xydef@\arcbisector{%
 \cfromid@{0@p}\pfromc@\cfromid@{0@c}\setupDirection@
 \advance\X@c\X@p\divide\X@c\tw@ 
 \advance\Y@c\Y@p\divide\Y@c\tw@ \czeroEdge@ \pfromc@
 \enter@\cplusthec@ \enter@\relax\begingroup
 \aboveDirection@\xydashl@ \vfromslide@i{}@\leave@ }
\xydef@\arcCenter@{%
 \cfromid@{0@p}\pfromc@\cfromid@{0@m}\setupDirection@
 \cfromp@\enter@\cplusthec@ \enter@\relax\begingroup
 \aboveDirection@\xydashl@ \vfromslide@i{}@\leave@\no@@
 \arcCenter@i }
\xydef@\arcCenter@i{%
 \enter@{\pfromthep@}\setupDirection@ \Creset@@
 \let\PLACEedgep@@=\PLACEedgep@ \let\PLACEedgec@@=\PLACEedgec@
 \enter@{\pfromthep@\basefromthebase@}\bgroup 
 \arcbisector \edef\next@{\egroup 
 \X@c =\the\X@c \Y@c=\the\Y@c \X@p=\the\X@p \Y@p=\the\Y@p }%
 \next@ \Cintercept@@ \leave@\leave@ }
\xydef@\getarcExtents@{%
 \ifx\space@\next\expandafter\DN@\space{\xyFN@\getarcExtents@}%
 \else\ifx\next @\xy@{@}{}\DN@ @{\fullEllipse@}%
 \else\DN@{\xy@{arcEXTENTs}{\save@ 
 \def\startDirection@{\Direction=\startDirection@@ \imposeDirection@}}%
 \xyFN@\getarcExtents@ii}\fi\fi \next@ }
\xydef@\getarcExtents@ii{%
 \ifx\next!\xy@{![[}{}\DN@![[##1]]{\getxyDirection@{##1}\getarcExtents@iv}%
 \else\DN@{\getarcExtents@iv}\fi \next@ }
\xydef@\getarcExtents@iv{\afterDIRECTIONorEMPTY
 {\xy@{startDIR}{\edef\startDirection@@{\the\Direction}\leave@}%
 \xyFN@\getarcOrientation@}%
 {\xy@{startDIR}{\edef\startDirection@@{\the\Direction}\leave@}%
 \xyFN@\getarcOrientation@}}
\xydef@\getarcOrientation@{%
 \ifx\space@\next\expandafter\DN@\space{\xyFN@\getarcOrientation@}%
 \else\ifx\next @\xy@{@}{}\DN@{\getEndDirection@x}%
 \else\ifx\next,\xy@{,}{}\DN@,{\xyFN@\getarcOrientation@i}%
 \else\DN@{\getarcOrientation@i}\fi\fi\fi \next@ }%
\xydef@\getarcOrientation@i{%
 \ifx\space@\next\expandafter\DN@\space{\xyFN@\getarcOrientation@i}%
 \else\ifx\next @\xy@{@}{}\DN@{\getEndDirection@x}%
 \else\ifx\next^{}\DN@##1{\xy@{^}{\def\arcOrient@@{^}}%
 \def\arcOrient@@{^}\xyFN@\getEndDirection@}%
 \else\ifx\next_\DN@##1{\xy@{_}{\def\arcOrient@@{_}}%
 \def\arcOrient@@{_}\xyFN@\getEndDirection@}%
 \else\DN@{\xyFN@\getEndDirection@}%
 \fi\fi\fi\fi \next@ }
\xydef@\getEndDirection@{%
 \ifx\space@\next\expandafter\DN@\space{\xyFN@\getEndDirection@}%
 \else\ifx\next,\DN@,{\xy@{,}{}\xyFN@\getEndDirection@}%
 \else\addEQ@\ifx\next\addEQ@\DN@{\xy@{=}{\save@\startDirection@}%
 \xyFN@\getEqDirection@}%
 \else \ifx\next!\DN@![[##1]]{\xy@{![[}{\save@}\getxyDirection@{##1}%
 \xy@{endDIR}{\edef\endDirection@@{\the\Direction}}%
 \xyFN@\getEndDirection@i}%
 \else \DN@{\xy@{origDIR}{\save@\origDirection@}\getEndDirection@i}%
 \fi\fi\fi\fi \next@ }
\xydef@\getEqDirection@{%
 \ifx\space@\next\expandafter\DN@\space{\xyFN@\getEqDirection@}%
 \else\ifx\next @\xy@{@}{}\DN@ @{%
 \xy@{sameDIR}{\edef\endDirection@@{\startDirection@@}\leave@}%
 \parEllipse@{1}{}}%
 \else\ifx\next (\DN@({\xyFN@\checkEqOpen@}%
 \else \DN@{\getEndDirection@i}\fi\fi\fi \next@ }
\xydef@\checkEqOpen@{%
 \ifx\next *\DN@{\getEndDirection@i (}%
 \else \DN@##1)##2@{\xy@{()}\leave@ \parEllipse@{##1}{##2}}%
 \fi \next@ }
\xydef@\getEndDirection@i{\afterDIRECTIONorEMPTY
 {\xy@{endDIR}{\edef\endDirection@@{\the\Direction}\leave@}%
 \getEndDirection@x }%
 {\xy@{endDIR}\leave@ \getEndDirection@x }}
\xydef@\getEndDirection@x#1@{%
 \DN@{#1}\ifx\next@\empty\relax \else\xywarning@{\omittingTokens@}\fi
 \processDirections@ }
\xydef@\omittingTokens@{omitting unused tokens: \codeof\next@ }
\xydef@\processDirections@@{%
 \ifx\endDirection@@\empty \skewCircle@
 \else \skewEllipse@ \expandafter \afterARCextents@@ \fi }
\xydef@\processArcDirections@{%
 \xy@{ARCdirs}{\ifx\endDirection@@\empty
 \origDirection@ \edef\endDirection@@{\the\Direction}\fi}%
 \ellipseArc@ 
 \xy@{procARCdirs}\processArcDirections@@
 \let\arcScale@\ellsave@ \let\arcRadius@\ellsave@ \def\ellipseRatio@{}%
 \xy@{circSECTORS}{\doCircleSectors@}\endarc@ }
\xydef@\ellsave@{\xy@@{\save@}}
\xydef@\processArcDirections@@{\save@
 \bgroup \cfromid@{0@0}\pfromc@ \Direction=\startDirection@@ 
 \DN@{_}\ifx\next@\arcOrient@@
 \advance\Direction \ifnum\Direction<\z@-\fi 4096 \relax\fi 
 \imposeDirection@
 \d@X=\cosDirection\Y@ybase \advance\d@X-\sinDirection\X@ybase
 \d@Y=-\cosDirection\Y@xbase \advance\d@Y\sinDirection\X@xbase
 \setupDirection@i
 \d@X=-\cosDirection\X@ybase \advance\d@X\sinDirection\X@xbase
 \d@Y=-\cosDirection\Y@ybase \advance\d@Y\sinDirection\Y@xbase
 \enter@\cplusthec@\X@c=\d@X \Y@c=\d@Y \leave@ \czeroEdge@
 \setupDirection@i 
 \czeroEdge@
 \edef\next@{\egroup \cfromthec@ \count@=\the\Direction}\next@
 \edef\startDirection@@{\the\count@}\idfromc@{0@x}%
 \bgroup \cfromid@{0@0}\pfromc@ \Direction=\endDirection@@
 \DN@{_}\ifx\next@\arcOrient@@
 \advance\Direction \ifnum\Direction<\z@-\fi 4096 \relax\fi 
 \imposeDirection@ 
 \d@X=\cosDirection\Y@ybase \advance\d@X-\sinDirection\X@ybase
 \d@Y=-\cosDirection\Y@xbase \advance\d@Y\sinDirection\X@xbase
 \setupDirection@i
 \d@X=-\cosDirection\X@ybase \advance\d@X\sinDirection\X@xbase
 \d@Y=-\cosDirection\Y@ybase \advance\d@Y\sinDirection\Y@xbase
 \enter@\cplusthec@\X@c=\d@X \Y@c=\d@Y \leave@
 \czeroEdge@ 
 \setupDirection@i 
 \edef\next@{\egroup \cfromthec@ \count@=\the\Direction}\next@
 \edef\endDirection@@{\the\count@}\idfromc@{0@c}%
 \count@=\startDirection@@ \relax \count@@=\endDirection@@ \relax
 \DN@{^}\ifx\arcOrient@@\next@
 \ifnum\count@@>\count@ \else\advance\count@@ 8192 \relax\fi
 \else
 \ifnum\count@@<\count@ \else\advance\count@@-8192 \relax\fi\fi
 \edef\startDirection@@{\the\count@}%
 \edef\endDirection@@{\the\count@@}}%
\xydef@\doCircleSectors@{%
 \let\doCircleArc@=\doMergeEndArc@@ \leave@ \leave@
 \cfromid@{0@0}\pfromc@\cfromid@{0@p}\setupDirection@ 
 \count@=\Direction \DN@{^}\ifx\arcOrient@@\next@
 \ifnum\count@>\startDirection@@ \advance\count@-8192 \fi\relax
 \count@@=\count@ \advance\count@@ 8192 \relax
 \ifnum\count@@<\endDirection@@ \advance\count@@ 8192 \fi\relax
 \else 
 \ifnum\count@<\startDirection@@ \advance\count@ 8192 \fi\relax
 \count@@=\count@ \advance\count@@-8192 \relax
 \ifnum\count@@>\endDirection@@ \advance\count@@-8192 \fi\relax
 \fi \relax
 \edef\preDirection@@{\the\count@}\edef\postDirection@@{\the\count@@}%
 \cfromid@{1@c}\setupDirection@ \count@=\Direction 
 \def\nextii@{^}\ifx\nextii@\arcOrient@@
 \DN@{\forwardSectors@\doEllipseSectors@}%
 \ifnum\count@<\preDirection@@ \advance\count@ 8192 \relax
 \else \count@@=\count@\advance\count@-8192 \relax
 \ifnum\count@@<\preDirection@@ \else\count@=\count@@ \fi\fi
 \else
 \DN@{\backwardSectors@\doEllipseSectors@}%
 \ifnum\count@>\preDirection@@ \advance\count@-8192 \relax
 \else \count@@=\count@\advance\count@ 8192 \relax
 \ifnum\count@@>\preDirection@@ \else\count@=\count@@ \fi\fi
 \fi \edef\quadDirection@{\the\count@}%
 \next@ }
\xydef@\forwardSectors@{%
 \ifnum \startDirection@@<\quadDirection@ \def\startSector@@{0}%
 \else\count@=\preDirection@@ \advance\count@ 4096 \relax
 \ifnum \startDirection@@<\count@ \def\startSector@@{1}%
 \else\count@=\quadDirection@ \advance\count@ 4096 \relax
 \ifnum\startDirection@@<\count@ \def\startSector@@{2}%
 \else \def\startSector@@{3}\fi\fi\fi 
 \ifnum\quadDirection@ <\endDirection@@ \relax
 \count@=\preDirection@@ \advance\count@ 4096 \relax
 \ifnum\count@<\endDirection@@ \relax
 \count@=\quadDirection@ \advance\count@ 4096 \relax
 \ifnum\count@<\endDirection@@ \relax
 \count@=\preDirection@@ \advance\count@ 8192 \relax
 \ifnum\count@<\endDirection@@ \relax
 \count@=\quadDirection@ \advance\count@ 8192 \relax
 \ifnum\count@<\endDirection@@ \relax
 \count@=\preDirection@@ \advance\count@ 12288 \relax
 \ifnum\count@<\endDirection@@ \relax
 \count@=\quadDirection@ \advance\count@ 12288 \relax
 \ifnum\count@<\endDirection@@ \def\endSector@@{7}%
 \else \def\endSector@@{6}\fi
 \else \def\endSector@@{5}\fi
 \else \def\endSector@@{4}\fi
 \else \def\endSector@@{3}\fi
 \else \def\endSector@@{2}\fi
 \else \def\endSector@@{1}\fi
 \else \def\endSector@@{0}\fi }
\xydef@\backwardSectors@{%
 \ifnum \startDirection@@>\quadDirection@ \def\startSector@@{0}%
 \else\count@=\preDirection@@ \advance\count@-4096 \relax
 \ifnum \startDirection@@>\count@ \def\startSector@@{1}%
 \else\count@=\quadDirection@ \advance\count@-4096 \relax
 \ifnum\startDirection@@>\count@ \def\startSector@@{2}%
 \else \def\startSector@@{3}\fi\fi\fi 
 \ifnum\quadDirection@>\endDirection@@ \relax
 \count@=\preDirection@@ \advance\count@-4096 \relax
 \ifnum\count@>\endDirection@@ \relax
 \count@=\quadDirection@ \advance\count@-4096 \relax
 \ifnum\count@>\endDirection@@ \relax
 \count@=\preDirection@@ \advance\count@-8192 \relax
 \ifnum\count@>\endDirection@@ \relax
 \count@=\quadDirection@ \advance\count@-8192 \relax
 \ifnum\count@>\endDirection@@ \relax
 \count@=\preDirection@@ \advance\count@-12288 \relax
 \ifnum\count@>\endDirection@@ \relax
 \count@=\quadDirection@ \advance\count@-12288 \relax
 \ifnum\count@>\endDirection@@ \def\endSector@@{7}%
 \else \def\endSector@@{6}\fi
 \else \def\endSector@@{5}\fi
 \else \def\endSector@@{4}\fi
 \else \def\endSector@@{3}\fi
 \else \def\endSector@@{2}\fi
 \else \def\endSector@@{1}\fi
 \else \def\endSector@@{0}\fi }
\xydef@\doEllipseSectors@{%
 \ifx\startSector@@\endSector@@
 \DN@{\expandafter\doMergeBothArc@\expandafter{\arcSTYLE}{\endSector@@}}%
 \else
 \expandafter\doMergeStartArc@\expandafter{\arcSTYLE}{\startSector@@}%
 \edef\countArcs@@{\startSector@@}%
 \loop@ \count@=\countArcs@@ \relax \advance\count@\@ne
 \ifnum \count@ < \endSector@@ \edef\countArcs@@{\the\count@}%
 \bgroup\expandafter\doCircleArc@@\expandafter{\arcSTYLE}{\countArcs@@}%
 \egroup 
 \repeat@
 \DN@{\expandafter\doMergeEndArc@\expandafter{\arcSTYLE}{\endSector@@}}%
 \fi \next@ }
\xydef@\checkstartDirection@{%
 \bgroup\no@@ \edef\next@{\egroup\count@@=\the\Direction}\next@\relax
 \ifnum\count@@=\startDirection@@ \relax \DN@{\straightArc@}%
 \else \advance\count@@-\startDirection@@ \relax
 \ifnum\count@@=\ifnum\count@@<\z@-\fi 4096 \relax \DN@{\straightArc@}%
 \else \DN@{\processDirections@@}\fi\fi \next@ }
\xydef@\straightArc@{\xywarning@{straight arc encountered}%
 \xy@@{\let\bstartPLACE@=\relax 
 \expandafter\doStraightArc@@\expandafter{\arcSTYLE}}\endarc@ }%
\xydef@\skewEllipse@{\xy@@{\doskewEllipse@}%
 \def\afterARCextents@@{\xy@{aftARCext}{\let\doCircleArc@=\doMergeEndArc@@}%
 \ellipseArc@ \xy@{doCircARCs}{\doCircleArcs@}\endarc@ }%
 \let\arcScale@=\relax \def\arcRadius@{}\def\ellipseRatio@{}}
\xydef@\skewCircle@{\xy@@{\setupDirection@}%
 \ifnum\Direction=\startDirection@@\relax\DN@{\halfEllipse@{1}}%
 \else
 \xy@@{\def\startDirection@{\Direction=\startDirection@@\imposeDirection@}%
 \cfromid@{0@p}\enter@\cplusthec@ \startDirection@
 \enter@\relax\begingroup\vfromslide@i{}@\czeroEdge@\leave@\idfromc@{0@m}%
 \let\endDirection@=\relax \let\doCircleArc@=\doMergeEndArc@@}%
 \DN@{\circleArc@}%
 \fi \next@ }
\xydef@\doskewEllipse@{%
 \def\startDirection@{\Direction=\startDirection@@ \relax
 \imposeDirection@}\startDirection@ \cfromid@{0@p}%
 \enter@\cplusthec@ \enter@\relax\begingroup\vfromslide@i{}@\leave@ 
 \idfromc@{0@x}%
 \ifx\endDirection@@\empty \parallelDirection@
 \else
 \def\endDirection@{\Direction=\endDirection@@ \relax
 \imposeDirection@ }\endDirection@ \skewEllB@ 
 \bgroup\setupDirection@\edef\next@{\egroup\count@@=\the\Direction}\next@
 \edef\endDirection@@{\the\count@@}%
 \fi
 \cfromid@{0@p}\bgroup \setupDirection@
 \edef\next@{\egroup \count@@=\the\Direction}\next@
 \edef\startDirection@@{\the\count@@}}
\xydef@\halfEllipse@#1{\xy@@{%
 \cfromid@{0@p}\pfromc@\cfromid@{0@c}\no@@
 \edef\endDirection@@{\the\Direction}%
 \advance\X@c\X@p \divide\X@c\tw@ \advance\Y@c\Y@p \divide\Y@c\tw@
 \idfromc@{0@0}\pfromc@ \cfromid@{0@p}\setbase@\X@p\Y@p\X@c\Y@c 
 \dimen@=\X@origin \advance\dimen@-\X@c \dimen@ii=\cosDirection\dimen@
 \dimen@=\Y@origin \advance\dimen@-\Y@c \advance\dimen@ii \sinDirection\dimen@
 \X@c=\X@origin \Y@c=\Y@origin \enter@\cplusthec@ 
 \dimen@=#1\p@ \ifdim\dimen@<\z@ \DN@{^}\dimen@ii=-#1\dimen@ii
 \ifx\next@\arcOrient@@\def\arcOrient@@{_}\else\def\arcOrient@@{^}\fi
 \else \dimen@ii=#1\dimen@ii\fi 
 \startDirection@ \enter@\relax\begingroup\expandafter
 \vfromslide@i\expandafter{\the\dimen@ii}@\leave@
 \idfromc@{1@c}\setbase@@ \X@c \Y@c \adjustBaseOrient@
 \count@@=\endDirection@@ \relax
 \DN@{^}\advance\count@@\ifx\arcOrient@@\next@\else-\fi 4096 \relax
 \edef\startDirection@@{\the\count@@}%
 \def\startDirection@{\Direction=\startDirection@@ \imposeDirection@ }%
 \let\doCircleArc@=\doMergeEndArc@@ }%
 \let\arcScale@=\relax \ellipseArc@
 \xy@@{\doCircleArcs@}\endarc@ }
\xydef@\parallelDirection@{\show\parallelDirection@}%
\xydef@\parEllipse@#1#2{\DN@{#2}\ifx\next@\empty 
 \else\xywarning@{\omittingTokens@ }\fi \halfEllipse@{#1}}
\xydef@\skewEllB@{\cfromid@{0@c}\pfromc@\enter@\cplusthec@
 \enter@\relax\begingroup\vfromslide@i{}@\leave@
 \enter@{\pfromthep@\basefromthebase@}\no@@
 \bgroup \cfromid@{0@p}\pfromc@\cfromid@{0@x}\edef\next@{\egroup 
 \X@c =\the\X@c \Y@c=\the\Y@c \X@p=\the\X@p \Y@p=\the\Y@p }\next@
 \Cintercept@@\leave@ \idfromc@{0@x}\cfromid@{0@p}\enter@\cplusthec@
 \cfromid@{0@c}\leave@ \enter@\cplusthec@ \cfromid@{0@x}%
 \X@c=-\X@c \Y@c=-\Y@c \leave@ \idfromc@{0@0}\pfromc@\cfromid@{0@p}%
 \setbase@\X@p\Y@p\X@c\Y@c \cfromid@{0@c}\setbase@@\X@c\Y@c
 \adjustBaseOrient@ }
\xydef@\adjustBaseOrient@{%
 \edef\tmp@{\expandafter\removePT@\the\X@xbase}\dimen@=\Y@ybase
 \divide\dimen@ 64 \relax \dimen@ii=\tmp@\dimen@
 \edef\tmp@{\expandafter\removePT@\the\X@ybase}\dimen@=\Y@xbase
 \divide\dimen@ 64 \relax \dimen@=\tmp@\dimen@
 \ifdim\dimen@>\dimen@ii \X@ybase=-\X@ybase \Y@ybase=-\Y@ybase \fi }
\xyendinput


==> xyarrow.tex <==
%% xyarrow.tex from $Id: xyarrow.doc,v 3.5 1997/05/28 13:05:01 krisrose Exp $
%%
%% Xy-pic ``Arrows and Paths'' feature.
%% Copyright (c) 1991-1997 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1997 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{arrow}{Arrow and Path feature}{\stripRCS$Revision: 3.5 $}%
 {Kristoffer H.~Rose}{krisrose@brics.dk}%
 {BRICS/Computer Science, University of Aarhus, Ny Munkegade, building 540,
 DK--8000 Aarhus~C}
\message{path,}
\xydef@\PATH{\afterPATH{}}
\xylet@\afterPATH@=\empty
\xydef@\afterPATH#1{\save
 \DN@##1{\def\afterPATH@{\restore \def\afterPATH@{##1}#1}}%
 \expandafter\next@\expandafter{\afterPATH@}%
 \let\PATHfail@@=\empty
 \let\PATHbefore@@=\empty
 \let\PATHafter@@=\empty
 \let\PATHlabelsevery@@=\empty
 \let\PATHlabelsnext@@=\empty
 \let\PATHlabelslast@@=\empty
 \xy@{\afterPATH{#1}}{\def\PATHslide@@{\z@}}%
 \def\PATHcontinue@@{\xyFN@\PATH@}%
 \xyFN@\PATH@}
\xynew@{if}\ifPATHsingle@
\xydef@\PATH@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\PATH@}%
 \else\ifPATHsingle@ \let\next@=\PATH@single
 \else \let\next@=\PATH@normal \fi\fi \next@}
\xydef@\PATH@normal{%
 \ifx ~\next \DN@ ~{\xyFN@\PATHsetting@}%
 \else \addRQ@\ifx \next \addRQ@\DN@{\xy@'{}\xyFN@\PATHstraight@}%
 \else \addLQ@\ifx \next \addLQ@\DN@{\xy@`{}\xyFN@\PATHturn@}%
 \else\ifx \PATHfail@@\PATH@x \DN@{\xyFN@\PATHfinal@}%
 \else
 \DNii@{\let\PATHfail@@=\PATH@x \xyFN@\PATH@}%
 \DN@{\expandafter\nextii@\PATHfail@@}%
 \fi\fi\fi\fi \next@}
\xylet@\PATHfail@@=\empty
\xylet@\PATHbefore@@=\empty
\xylet@\PATHafter@@=\empty
\xylet@\PATHlabelsevery@@=\empty
\xylet@\PATHlabelsnext@@=\empty
\xylet@\PATHlabelslast@@=\empty
\xydef@\PATHsetting@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\PATHsetting@}%
 \else\ifx \bgroup\next
 \DN@##1{\xy@{~{##1}}{}\def\PATHfail@@{##1}\xyFN@\PATH@}%
 \else \addEQ@\ifx \next
 \addEQ@\DN@##1{\xy@{~={##1}}{}\def\PATHbefore@@{##1}\xyFN@\PATH@}%
 \else \addLT@\ifx \next
 \addLT@\DN@##1{\xy@{~<{##1}}{}\def\PATHlabelsnext@@{##1}\xyFN@\PATH@}%
 \else \addGT@\ifx \next
 \addGT@\DN@##1{\xy@{~>{##1}}{}\def\PATHlabelslast@@{##1}\xyFN@\PATH@}%
 \else \addPLUS@\ifx \next
 \addPLUS@\DN@##1{\xy@{~+{##1}}{}\def\PATHlabelsevery@@{##1}\xyFN@\PATH@}%
 \else \ifx /\next
 \DN@/##1{\xy@{~/{##1}}{}\def\PATHafter@@{##1}\xyFN@\PATH@}%
 \else \addDASH@\ifx \next
 \xywarning@{Obsolete `-' PATH <action> translated to `='.}%
 \addDASH@\DN@##1{\xy@{~-{##1}}{}\def\PATHbefore@@{##1}\xyFN@\PATH@}%
 \else
 \xyerror@{Unknown \string~ setting: \meaning\next}%
 {See the Xy-pic arrow feature documentation for help.}%
 \fi\fi\fi\fi\fi\fi\fi\fi \next@}
\xylet@\PATHinit@@=\empty
\xylet@\PATHextra@@=\empty
\xylet@\PATHpost@@=\empty
\xylet@\PATHcontinue@@=\empty
\xydef@\PATHstraight@{%
 \def\PATHinit@@{\PATHinitstraight@}%
 \let\PATHextra@@=\empty
 \let\PATHpost@@=\empty
 \let\PATHlabelsextra@@=\relax
 \xy@@\pfromc@ \PATHafterPOS{\xyFN@\PATHsegment@}}
\xydef@\PATHfinal@{%
 \def\PATHinit@@{\PATHinitstraight@}%
 \def\PATHextra@@{\let\PATHcontinue@@=\afterPATH@}%
 \let\PATHpost@@=\empty
 \let\PATHlabelsextra@@=\PATHlabelsextralast@
 \xy@@\pfromc@ \PATHafterPOS{\xyFN@\PATHsegment@}}
\xydef@\PATHlabelsextralast@{\let\PATHlabelsextra@@=\relax
 \expandafter\xyFN@\expandafter\PATHlabels@\PATHlabelslast@@}
\xydef@\PATHinitstraight@{\xy@@{\setupDirection@ \dimen@=\PATHslide@@
 \dimen@ii=-\sinDirection\dimen@
 \ifPATHomitslide@@\else\advance\X@p\dimen@ii\fi \advance\X@c\dimen@ii
 \dimen@ii= \cosDirection\dimen@
 \ifPATHomitslide@@\else\advance\Y@p\dimen@ii\fi \advance\Y@c\dimen@ii
 \PATHomitslide@@false \resetupDirection@}}
\xydef@\PATHslide@@{\z@}
\xynew@{if}\ifPATHomitslide@@
\xydef@\PATHsegment@{%
 \addLT@\ifx\next
 \addGT@{\addLT@\DN@##1}{%
 \xy@{<##1>}{\dimen@=##1\relax \edef\PATHslide@@{\the\dimen@}}%
 \xyFN@\PATHsegment@@}%
 \else \let\next@=\PATHsegment@@
 \fi \next@}
\xydef@\PATHsegment@@{\PATHinit@@ \addEQ@\PATHaction@\PATHbefore@@ \PATHextra@@
 \expandafter\toks@\expandafter{\PATHlabelsnext@@}\let\PATHlabelsnext@@=\empty
 \expandafter\addtotoks@\expandafter{\PATHlabelsevery@@}%
 \expandafter\def\expandafter\PATHlabels@@\expandafter{\the\toks@}%
 \toks@={}\expandafter\xyFN@\expandafter\PATHlabels@\PATHlabels@@}
\xylet@\PATHlabelit@@=\empty
\xydef@\PATHlabels@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\PATHlabels@}%
 \else \ifx ^\next 
 \DN@##1{\xy@^{}\let\PATHlabelit@@=\PATHlabelabove@@
 \DNii@{}\xyFN@\PATHanchor@}%
 \else \ifx _\next
 \DN@##1{\xy@_{}\let\PATHlabelit@@=\PATHlabelbelow@@
 \DNii@{}\xyFN@\PATHanchor@}%
 \else \ifx |\next
 \DN@##1{\xy@|{}\let\PATHlabelit@@=\PATHlabelbreak@
 \DNii@{}\xyFN@\PATHanchor@}%
 \else \let\next@=\PATHfinishsegments@ \fi\fi\fi\fi \next@}
\xydef@\PATHanchor@{\begingroup \toks@={}\PATHanchor@i}
\xydef@\PATHanchor@i{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\PATHanchor@i}%
 \else\addDASH@\ifx \next
 \addDASH@\DN@{\expandafter\addtotoks@\expandafter{\PATHanchor@toks}%
 \xyFN@\PATHanchor@i}%
 \else
 \DNii@##1{\endgroup\afterPLACE{\xyFN@\PATHit@}##1}%
 \DN@{\expandafter\nextii@\expandafter{\the\toks@}}%
 \fi\fi \next@}
{\xyuncatcodes \gdef\next{<>(.5)}}
\xylet@\PATHanchor@toks=\next
\xylet@\PATHitshapes@@=\empty
\xydef@\PATHit@{\let\PATHitshape@@=\empty \xyFN@\PATHit@i}
\xydef@\PATHit@i{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\PATHit@i}%
 \else \ifx *\next \DN@*##1##{\PATHlabelit@@{!C##1}}%
 \else \addAT@\ifx\next \addAT@\DN@##1##{\PATHlabelit@@{\dir##1}}%
 \else \ifx [\next \DN@[##1]{%
 \expandafter\def\expandafter\PATHitshape@@\expandafter{\PATHitshape@@[##1]}%
 \xyFN@\PATHit@i}%
 \else \DN@{\PATHlabelit@@{}}%
 \fi\fi\fi\fi \next@}
\xydef@\PATHfinishsegments@{%
 \ifx\PATHlabelsextra@@\relax \expandafter\PATHfinishsegments@i
 \else
 \expandafter\PATHlabelsextra@@ \fi}
\xydef@\PATHfinishsegments@i{%
 \xy@@{\Clast@@}\the\toks@ \toks@={}%
 \xy@@\setupDirection@
 \PATHpost@@ \PATHaction@/\PATHafter@@
 \PATHcontinue@@}
\xydef@\PATHaction@default#1#2{\xy@{PATHaction#1{#2}}{}\POS#2\relax}
\xylet@\PATHaction=\PATHaction@default
\xydef@\PATHaction@#1#2{\expandafter\PATHaction\expandafter#1\expandafter{#2}}
\xylet@\PATHafterPOS@default=\afterPOS
\xylet@\PATHafterPOS=\PATHafterPOS@default
\xydef@\PATHlastout@@{3}
\xydef@\PATHturn@{\afterCIRorDIAG\PATHturn@cir\PATHturn@diag}
\xydef@\PATHturn@cir{\toks@={\xy@@{%
 \count@=\CIRin@@ \ifnum\count@<4\else\advance\count@-4\fi
 \count@@=\CIRout@@ \ifnum\count@@<4\else\advance\count@@-4\fi
 \ifnum\count@=\count@@ \xyerror@{<turn> cannot be half or full}{%
You asked for a <turn>ed segment with parallel in- and out-direction.^^J%
This is not allowed because it is not possible to position it uniquely.}\fi}}%
 \edef\next@{{\CIRin@@}{\expandafter\noexpand\CIRorient@@}{\CIRout@@}}%
 \expandafter\PATHturn@i\next@}
\xydef@\PATHturn@diag{\toks@={\xy@@{%
 \setupDirection@ \count@=\CIRin@@ \dimen@=\xydashl@ \ABfromdiag@
 \ifdim \sinDirection\A@>\cosDirection\B@ \def\CIRorient@@{\CIRacw@}%
 \advance\count@\ifnum\count@<6 \tw@ \else -6\fi
 \else \def\CIRorient@@{\CIRcw@}%
 \advance\count@\ifnum\count@>\@ne -\tw@ \else 6\fi
 \fi
 \edef\CIRout@@{\the\count@}}}%
 \edef\next@{{\CIRin@@}{}{}}%
 \expandafter\PATHturn@i\next@}
\xylet@\PATHpostpos@@=\empty
\xydef@\PATHturn@i#1#2#3{%
 \DN@##1{\def\PATHinit@@{\xy@@{%
 \def\CIRin@@{#1}\def\CIRorient@@{#2}\def\CIRout@@{#3}%
 \ifnum\CIRin@@=8 \let\CIRin@@=\PATHlastout@@ \fi
 \R@=\turnradius@
 ##1\relax}%
 \xy@@{\count@=\CIRin@@
 \ifPATHomitslide@@ \dimen@=-\PATHslide@@
 \ABfromdiag@ \advance\X@p-\B@ \advance\Y@p\A@ \fi
 \enter@{\pfromthep@ \basefromthebase@}}%
 \xy@@{\dimen@=\expandafter\ifx\CIRorient@@\CIRcw@-\fi\R@
 \ABfromdiag@ \advance\X@p-\B@ \advance\Y@p\A@
 \X@origin=\X@p \Y@origin=\Y@p}%
 \xy@@{\dimen@=\xydashl@ \ABfromdiag@ \R@c=\A@ \U@c=\B@
 \count@=\CIRout@@
 \dimen@=\expandafter\ifx\CIRorient@@\CIRcw@-\fi\R@
 \ABfromdiag@ \advance\X@c-\B@ \advance\Y@c\A@
 \dimen@=\xydashl@ \X@p=\X@c \Y@p=\Y@c
 \ABfromdiag@ \advance\X@p-\A@ \advance\Y@p-\B@
 \intersect@
 \count@=\CIRin@@ \dimen@=\p@ \ABfromdiag@}%
 \xy@@{\edef\next@{\expandafter\removePT@\the\A@}%
 \edef\nextii@{\expandafter\removePT@\the\B@}%
 \A@=\X@c \advance\A@-\X@origin \B@=\Y@c \advance\B@-\Y@origin
 \ifdim \next@\A@<-\nextii@\B@
 \dontleave@ \cfromp@
 \count@=\CIRin@@ \advance\count@\ifnum\count@<4 +4\else -4\fi
 \dimen@=\xydashl@ \Directionfromdiag@
 \the\Edge@c\z@
 \count@=\CIRin@@ \dimen@=\expandafter\ifx\CIRorient@@\CIRcw@-\fi\R@
 \ABfromdiag@ \advance\X@c-\B@ \advance\Y@c\A@
 \dimen@=5sp \ABfromdiag@ \advance\X@c\A@ \advance\Y@c\B@
 \fi
 \dimen@ii=\expandafter\ifx\CIRorient@@\CIRacw@-\fi\PATHslide@@
 \advance\R@\dimen@ii
 \drop@\literal@{\hbox\bgroup\cir@i}}%
 \xy@@{\X@p=\X@c \Y@p=\Y@c
 \count@=\CIRout@@
 \dimen@=\expandafter\ifx\CIRorient@@\CIRacw@-\fi\R@c
 \ABfromdiag@ \advance\X@p-\B@ \advance\Y@p\A@
 \edef\PATHpostpos@@{\X@c=\the\X@p \Y@c=\the\Y@p \noexpand\czeroEdge@
 \noexpand\PATHomitslide@@true}}%
 \xy@@{\count@=\CIRin@@
 \dimen@=\expandafter\ifx\CIRorient@@\CIRacw@-\fi\R@c
 \ABfromdiag@ \advance\X@c-\B@ \advance\Y@c\A@ \czeroEdge@}%
 \xy@@{\leave@
 \count@=\CIRin@@ \dimen@=\PATHslide@@
 \ABfromdiag@ \advance\X@p-\B@ \advance\Y@p\A@
 \edef\PATHlastout@@{\CIRout@@}%
 \count@=\CIRout@@ \dimen@=\xydashl@ \Directionfromdiag@}}}%
 \expandafter\next@\expandafter{\the\toks@}\toks@={}%
 \let\PATHextra@@=\empty
 \def\PATHpost@@{\xy@@\PATHpostpos@@}%
 \let\PATHlabelsextra@@=\relax
 \xyFN@\PATHturn@ii}
\xydef@\PATHturn@ii{%
 \ifx /\next
 \DN@ /{\afterassignment\nextii@\dimen@=}%
 \DNii@{%
 \edef\next@{\noexpand\xy@@{\edef\noexpand\turnradius@{\the\dimen@}}}\next@
 \xy@@\pfromc@ \PATHafterPOS{\xyFN@\PATHsegment@}}%
 \else \DN@{\xy@@\pfromc@ \PATHafterPOS{\xyFN@\PATHsegment@}}\fi
 \next@}
\xydef@\ABfromdiag@{\ifcase\count@\relax
 \A@=-.7071\dimen@ \B@=-.7071\dimen@ \or \A@=\z@ \B@=-\dimen@
 \or \A@=+.7071\dimen@ \B@=-.7071\dimen@ \or \A@=\dimen@ \B@=\z@
 \or \A@=+.7071\dimen@ \B@=+.7071\dimen@ \or \A@=\z@ \B@=+\dimen@
 \or \A@=-.7071\dimen@ \B@=+.7071\dimen@ \or \A@=-\dimen@ \B@=\z@
 \else\xybug@{impossible <diag>?}\fi}
\xydef@\turnradius@{10pt}
\xydef@\turnradius{\afterADDOP{\Addop@@\turnradius@}}
\xydef@\PATHlabelabove@#1#2{\droplabel@\belowDirection@{#1}{#2}%
 \let\afteraliases@@=\empty \xyFN@\PATHlabelalias@}
\xydef@\PATHlabelbelow@#1#2{\droplabel@\aboveDirection@{#1}{#2}%
 \let\afteraliases@@=\empty \xyFN@\PATHlabelalias@}
\xylet@\PATHlabelabove@@=\PATHlabelabove@
\xylet@\PATHlabelbelow@@=\PATHlabelbelow@
\xydef@\droplabel@#1#2#3{\xy@@{\enter@\DirectionfromtheDirection@}%
 \DN@{#2}\ifx\next@\empty
 \expandafter\xy@@ix@\expandafter{\PATHitshape@@\labelbox{#3}}%
 \else \expandafter\xy@@ix@\expandafter{\PATHitshape@@#2{#3}}\fi
 \xy@@{\setbox\z@=\expandafter\object\the\toks9
 \advance\L@c\labelmargin@ \advance\R@c\labelmargin@
 \advance\D@c\labelmargin@ \advance\U@c\labelmargin@ 
 \setboxz@h{\kern\labelmargin@\boxz@\kern\labelmargin@}%
 \A@=\X@c \B@=\Y@c #1\xydashl@ \the\Edge@c\thr@@ 
 \advance\A@-\X@c \advance\B@-\Y@c \advance\X@c 2\A@ \advance\Y@c 2\B@
 \ht\z@=\U@c \dp\z@=\D@c \dimen@=\L@c \advance\dimen@\R@c \wd\z@=\dimen@ 
 \setbox\lastobjectbox@=\hbox{\X@c=\L@c \Y@c=\z@ \Drop@@}%
 \drop@{\box\lastobjectbox@}{}%
 \leave@}}
\xydef@\PATHlabelbreak@#1#2{%
 \DN@{#1}\ifx\next@\empty \drop\labelbox{#2}\else \drop#1{#2}\fi
 \def\afteraliases@@{\xy@@\Cbreak@@}\xyFN@\PATHlabelalias@}
\xylet@\labelmargin@=\objectmargin@
\xydef@\labelmargin{\afterADDOP{\Addop@@\labelmargin@}}
\xydef@\hole{\hbox{\dimen@=\objectmargin@ \kern2\dimen@
 \vrule height\dimen@ depth\dimen@ width\z@}}
\xylet@\labelstyle=\scriptstyle
\xydef@\labelbox#1{\hbox{$\m@th\labelstyle{#1}$}}
\xydef@\PATHlabelalias@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\PATHlabelalias@}%
 \else \addEQ@\ifx \next
 \addEQ@\DN@"##1"{\savealias@{##1}\xyFN@\PATHlabelalias@}%
 \else \DN@{\afteraliases@@\PATHlabels@}\fi\fi \next@}
\xylet@\afteraliases@@=\empty
\xydef@\savealias@#1{\xy@@{\enter@\cfromthec@
 \advance\X@c-\L@c \advance\L@c\R@c \L@c=.5\L@c \R@c=\L@c \advance\X@c\L@c 
 \advance\Y@c-\D@c \advance\D@c\U@c \D@c=.5\D@c \U@c=\D@c \advance\Y@c\D@c 
 \idfromc@{#1}\leave@}}
\message{\string\ar,}
\xylet@\arvariant@@=\empty
\xylet@\arstemprefix@@=\empty
\xylet@\artail@@=\empty
\xylet@\arstem@@=\empty
\xylet@\arhead@@=\empty
\xylet@\armodifiers@@=\empty
\xylet@\arlabels@@=\empty
\xylet@\arafterPOS@@=\empty
\xylet@\arinit@@=\empty
\xylet@\arexit@@=\empty
\xylet@\arcomponent@@=\relax
\xylet@\arcomponenttype@@=\relax
\xylet@\afterar@@=\relax
\xydef@\ar{\relax\arSAFE}
\xydef@\arSAFE{%
 \let\arvariant@@=\empty
 \def\arstemprefix@@{\dir}%
 \edef\artail@@{\arvariant@@{}}%
 \edef\arstem@@{\arvariant@@{-}}%
 \edef\arhead@@{\arvariant@@{>}}%
 \def\armodifiers@@{}%
 \def\arafterPOS@@{}%
 \def\arlabels@@{}%
 \def\arinit@@{}%
 \def\arexit@@{}%
 \let\PATHlabelabove@@=\PATHlabelabove@
 \let\PATHlabelbelow@@=\PATHlabelbelow@
 \xyFN@\ar@}
\xydef@\ar@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\ar@}%
 \else \addAT@\ifx\next \addAT@\DN@{\xyFN@\ar@form}%
 \else\ifx |\next
 \DN@ |{\ar@anchor|}%
 \else\ifx ^\next
 \DN@ ^{\ar@anchor^}%
 \else\ifx _\next
 \DN@ _{\ar@anchor_}%
 \else \let\next@=\ar@x \fi\fi\fi\fi\fi \next@}
\xydef@\addtoarinit@#1{%
 \expandafter\def\expandafter\arinit@@\expandafter{\arinit@@ #1}}
\xydef@\addtoarlabels@#1{%
 \expandafter\def\expandafter\arlabels@@\expandafter{\arlabels@@ #1}}
\xydef@\ar@anchor#1{\begingroup
 \def\PATHlabelit@@##1##2{%
 \DN@{##1}\ifx\next@\empty
 \DN@####1{\expandafter\endgroup\expandafter\addtoarlabels@
 \expandafter{\the\toks@####1{##2}}\xyFN@\ar@}%
 \else
 \DN@####1{\expandafter\endgroup\expandafter\addtoarlabels@
 \expandafter{\the\toks@*!C####1##1{##2}}\xyFN@\ar@}\fi
 \expandafter\next@\expandafter{\PATHitshape@@}}%
 \toks@={#1}%
 \def\xy@##1##2{\addtotoks@{##1}}\change@oxy@\xy@ \let\xy@@ix@=\eat@
 \DNii@{}\xyFN@\PATHanchor@}
\xydef@\ar@form{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\ar@form}%
 \else\ifx ^\next \DN@ ^{\xyFN@\ar@style}\edef\arvariant@@{\string^}%
 \else\ifx _\next \DN@ _{\xyFN@\ar@style}\edef\arvariant@@{\string_}%
 \else\ifx 0\next \DN@ 0{\xyFN@\ar@style}\def\arvariant@@{0}%
 \else\ifx 1\next \DN@ 1{\xyFN@\ar@style}\def\arvariant@@{1}%
 \else\ifx 2\next \DN@ 2{\xyFN@\ar@style}\def\arvariant@@{2}%
 \else\ifx 3\next \DN@ 3{\xyFN@\ar@style}\def\arvariant@@{3}%
 \else\ifx \bgroup\next \let\next@=\ar@style
 \else\ifx [\next \DN@[##1]{\ar@modifiers{[##1]}}%
 \else\ifx *\next \DN@ *{\ar@modifiers}%
 \else\addLT@\ifx\next \let\next@=\ar@slide
 \else\ifx /\next \let\next@=\ar@curveslash
 \else\ifx (\next \let\next@=\ar@curveinout
 \else\addRQ@\ifx\next \addRQ@\DN@{\ar@curve@}%
 \else\addLQ@\ifx\next \addLQ@\DN@{\xyFN@\ar@curve}%
 \else\addDASH@\ifx\next \addDASH@\DN@{\defarstem@-\xyFN@\ar@}%
 \else\addEQ@\ifx\next \addEQ@\DN@{\def\arvariant@@{2}\defarstem@-\xyFN@\ar@}%
 \else\addDOT@\ifx\next \addDOT@\DN@{\defarstem@.\xyFN@\ar@}%
 \else\ifx :\next \DN@:{\def\arvariant@@{2}\defarstem@.\xyFN@\ar@}%
 \else\ifx ~\next \DN@~{\defarstem@~\xyFN@\ar@}%
 \else\ifx !\next \DN@!{\dasharstem@\xyFN@\ar@}%
 \else\ifx ?\next \DN@?{\ar@upsidedown\xyFN@\ar@}%
 \else \let\next@=\ar@error
 \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi \next@}
\xydef@\defarstem@#1{\edef\arstem@@{\arvariant@@{\string#1}}%
 \DNii@##1##{\next@}%
 \edef\next@##1{\def\noexpand\artail@@{\arvariant@@{##1}}}%
 \expandafter\nextii@\artail@@
 \edef\next@##1{\def\noexpand\arhead@@{\arvariant@@{##1}}}%
 \expandafter\nextii@\arhead@@}
\xydef@\dasharstem@{%
 \DN@##1##{\nextii@{##1}}\DNii@##1##2{\def\arstem@@{##1{##2##2}}}%
 \expandafter\next@\arstem@@}
\xydef@\ar@error#1{\xyerror@{Illegal <form>ation (\meaning\next)}{}%
 \xyFN@\ar@}
\xydef@\ar@style{%
 \ifx \bgroup\next \def\artail@@{{}}%
 \edef\arstem@@{\arvariant@@{-}}\edef\arhead@@{\arvariant@@{>}}%
 \expandafter\ar@i
 \else \resetvariant@\artail@@ \resetvariant@\arstem@@ \resetvariant@\arhead@@
 \expandafter\xyFN@\expandafter\ar@ \fi}
\xydef@\resetvariant@#1{%
 \DN@##1##{\DN@{##1}\ifx\next@\empty
 \DN@{\expandafter\nextii@\expandafter{\arvariant@@}}%
 \else \DN@{\nextii@{##1}}\fi \next@}%
 \DNii@##1##2{\def#1{##1{##2}}}%
 \expandafter\next@#1}
\xydef@\ar@i#1{\DN@{#1}%
 \ifx\next@\empty \edef\arstem@@{\arvariant@@{}}\edef\arhead@@{\arvariant@@{}}%
 \DN@{\xyFN@\ar@}%
 \else
 \let\arcomponent@@=\ar@ii \let\arcomponenttype@@=\artip@
 \DN@{\xyFN@\arcomponent@#1$}%
 \fi \next@}
\xydef@\ar@ii{\ifx $\next \let\next@=\ar@iv
 \else \expandafter\def\expandafter\artail@@\expandafter{\the\toks@}%
 \let\arcomponent@@=\ar@iii \let\arcomponenttype@@=\arconn@
 \DN@{\xyFN@\arcomponent@}\fi \next@}
\xydef@\ar@iii{%
 \expandafter\def\expandafter\arstem@@\expandafter{\the\toks@}%
 \resetvariant@\artail@@
 \let\arcomponent@@=\ar@iv \let\arcomponenttype@@=\artip@
 \xyFN@\arcomponent@}
\xydef@\ar@iv{%
 \expandafter\def\expandafter\arhead@@\expandafter{\the\toks@}%
 \ifx $\next \DN@ ${\xyFN@\ar@}%
 \else \xyerror@{illegal <arrow>: \meaning\next\space not valid}{}\fi \next@}
\xydef@\ar@x{%
 \let\arsavedPATHafterPOS@@=\PATHafterPOS \let\PATHafterPOS=\arafterPOS@
 \toks@={\ar@PATH}%
 \expandafter\addtotoks@\expandafter{\expandafter{\artail@@}}%
 \expandafter\addtotoks@\expandafter{\expandafter{\arstem@@}}%
 \expandafter\addtotoks@\expandafter{\expandafter{\arstemprefix@@}}%
 \expandafter\addtotoks@\expandafter{\expandafter{\arhead@@}}%
 \expandafter\addtotoks@\expandafter{\expandafter{\armodifiers@@}}%
 \expandafter\addtotoks@\expandafter{\expandafter{\arinit@@}}%
 \expandafter\addtotoks@\expandafter{\expandafter{\arexit@@}}%
 \expandafter\addtotoks@\expandafter{\expandafter{\arlabels@@}}%
 \addtotoks@{\afterar@@}%
 \expandafter\DNii@\expandafter{\the\toks@}\toks@={}%
 \nextii@}
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8#9{%
 \def\next{%
 \afterPATH{#9}%
 ~={#6\preconnect#5#3#2}%
 ~/{#7}%
 ~<{|<*h#5\dir#1}%
 ~>{|>*h#5\dir#4}%
 ~+{#8}%
 }%
 \next}}
\xylet@\ar@PATH=\next
\xydef@\arafterPOS@#1{%
 \arsavedPATHafterPOS@@{\let\PATHafterPOS=\arsavedPATHafterPOS@@
 \DN@{#1}\expandafter\next@\arafterPOS@@}}%
\xylet@\arsavedPATHafterPOS@@=\relax
\xydef@\arcomponent@{%
 \ifx ^\next \toks@ii={^}\DN@ ^{\xyFN@\arcomponent@i}%
 \else\ifx _\next \toks@ii={_}\DN@ _{\xyFN@\arcomponent@i}%
 \else\ifx 1\next \toks@ii={1}\DN@ 1{\xyFN@\arcomponent@i}%
 \else\ifx 2\next \toks@ii={2}\DN@ 2{\xyFN@\arcomponent@i}%
 \else\ifx 3\next \toks@ii={3}\DN@ 3{\xyFN@\arcomponent@i}%
 \else\ifx \bgroup\next \expandafter\toks@ii\expandafter{\arvariant@@}%
 \let\next@=\arcomponent@i
 \else\ifx *\next \DN@*##1##{\arcomponent@ii{##1}}%
 \else \expandafter\toks@ii\expandafter{\arvariant@@}\toks@={}%
 \let\next@=\arcomponenttype@@
 \fi\fi\fi\fi\fi\fi\fi
 \next@}
\xydef@\arcomponent@i#1{\toks@={#1}\arcomponent@x}
\xydef@\arcomponent@ii#1#2{\toks@={*#1{#2}}\xyFN@\arcomponent@@}
\xydef@\artip@{%
 \addGT@\ifx\next \addGT@\addtotoks@ \addGT@\DN@{\xyFN@\artip@}%
 \else\addLT@\ifx\next \addLT@\addtotoks@ \addLT@\DN@{\xyFN@\artip@}%
 \else\ifx (\next \addtotoks@(\DN@({\xyFN@\artip@}%
 \else\ifx )\next \addtotoks@)\DN@){\xyFN@\artip@}%
 \else\ifx |\next \addtotoks@|\DN@|{\xyFN@\artip@}%
 \else\addLQ@\ifx\next \addLQ@\addtotoks@ \addLQ@\DN@{\xyFN@\artip@}%
 \else\addRQ@\ifx\next \addRQ@\addtotoks@ \addRQ@\DN@{\xyFN@\artip@}%
 \else\addPLUS@\ifx \next \addPLUS@\addtotoks@ \addPLUS@\DN@{\xyFN@\artip@}%
 \else\ifx /\next \addtotoks@/\DN@/{\xyFN@\artip@}%
 \else\ifcat A\noexpand\next \DN@##1{\addtotoks@{##1}\xyFN@\artip@}%
 \else\ifx\space@\next \addtotoks@{ }\expandafter\DN@\space{\xyFN@\artip@}%
 \else \let\next@=\arcomponent@x
 \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi \next@}
\xydef@\arconn@{%
 \addDASH@\ifx\next \addDASH@\addtotoks@ \addDASH@\DN@{\xyFN@\arconn@}%
 \else\addEQ@\ifx\next \addEQ@\addtotoks@ \addEQ@\DN@{\xyFN@\arconn@}%
 \ifx\arvariant@@\empty \def\arvariant@@{2}\fi
 \else\addDOT@\ifx\next \addDOT@\addtotoks@ \addDOT@\DN@{\xyFN@\arconn@}%
 \else\ifx :\next \addtotoks@:\DN@:{\xyFN@\arconn@}%
 \ifx\arvariant@@\empty \def\arvariant@@{2}\fi
 \else\ifx ~\next \addtotoks@~\DN@~{\xyFN@\arconn@}%
 \else \let\next@=\arcomponent@x
 \fi\fi\fi\fi\fi \next@}
\xydef@\arcomponent@x{%
 \DN@##1{\toks@=\expandafter{\the\toks@ii{##1}}}%
 \expandafter\next@\expandafter{\the\toks@}%
 \xyFN@\arcomponent@@}
\xydef@\ar@curveslash/#1/{\expandafter\ar@curve@\ar@slashing{#1}}
\xydef@\ar@slashing#1{{\xy@{**{} ?+/#1/+/#1/ @+c}{\setupDirection@
 \vfromslide@{#1}%
 \X@c=2\X@c \advance\X@c\X@p \advance\X@c.5\d@X
 \Y@c=2\Y@c \advance\Y@c\Y@p \advance\Y@c.5\d@Y
 \czeroEdge@
 \spushc@}}}
{\xyuncatcodes \catcode`\#=6
 \gdef\next(#1,#2){{+/#1 3pc/,p+/#2 3pc/}}}
\xylet@\ar@curveinout@=\next
\xydef@\ar@curveinout{\expandafter\ar@curve@load\ar@curveinout@}
\xydef@\ar@curve{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\ar@curve}%
 \else\ifx \bgroup\next \let\next@=\ar@curve@load
 \else\ifx "\next \DN@"##1"{\ar@curve@{"##1"}}%
 \else \xyerror@{@= <form> must be followed by \string"<id>\string" or
 {<control point list>}}{}%
 \fi\fi\fi \next@}
{\xyuncatcodes \gdef\next#1#2{\def#1##1{#2{;@={##1}}}}}
\next\ar@curve@load\ar@curve@
\xydef@\ar@curve@#1{\curve@check
 \setcurvearinit@{#1}\setcurvearexit@\arexit@@
 \def\arstemprefix@@{\crvi}\xyFN@\ar@}
{\xyuncatcodes \gdef\next#1{\save @(,#1\restore}}
\xylet@\setcurvearinit@i=\next
\xydef@\setcurvearinit@#1{%
 \expandafter\addtoarinit@\expandafter{\setcurvearinit@i{#1}}}
{\xyuncatcodes \gdef\next#1{\def#1{\POS @i @) }}}
\xylet@\setcurvearexit@=\next
\xydef@\curve@check{%
 \xyerror@{Forms @/.../, @(...), and @`{...}, only available when curve
 extension loaded}{}}
\xywithoption{curve}{\let\curve@check=\relax}
\xydef@\ar@modifiers#1{%
 \expandafter\def\expandafter\armodifiers@@\expandafter{\armodifiers@@#1}%
 \xyFN@\ar@}
{\xyuncatcodes \catcode`\#=6 \catcode`\@=11
 \gdef\next<#1>{\def\arafterPOS@@{<#1>}\xyFN@\ar@}}
\xylet@\ar@slide=\next
\xydef@\ar@upsidedown{\let\next=\PATHlabelabove@@
 \let\PATHlabelabove@@=\PATHlabelbelow@@ \let\PATHlabelbelow@@=\next}
\xyendinput


==> xycmactex.tex <==
%% xycmactex.tex from $Id: xycmactex.doc,v 3.3 1996/12/18 08:54:25 ross Exp $
%%
%% Xy-pic ``CMacTeX'' driver interface option.
%% Copyright (c) 1995-1996 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1996 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{cmactex}{CMacTeX driver}{\stripRCS$Revision: 3.3 $}%
 {Ross Moore}{ross@mpce.mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xyrequire{dvips}
\xyendinput


==> xycmtip.tex <==
%% xycmtip.tex from $Id: xycmtip.doc,v 3.3 1996/12/19 03:31:56 krisrose Exp $
%%
%% Xy-pic ``Computer Modern tips'' extension.
%% Copyright (c) 1992-1996 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% Copyright (c) 1991-1996 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{cmtip}{Computer Modern tip extension}{\stripRCS$Revision: 3.3 $}%
 {Kristoffer H.~Rose}{krisrose@brics.dk}%
 {BRICS/Computer Science, University of Aarhus, Ny Munkegade, building 540,
 DK--8000 Aarhus~C}
\xyrequire{tips}\xycatcodes
\xydef@\UseComputerModernTips{\SelectTips{cm}{10}\UseTips}
\xydef@\NoComputerModernTips{\NoTips}
\xyendinput


==> xycolor.tex <==
%% xycolor.tex from $Id: xycolor.doc,v 3.3 1996/12/19 03:50:08 ross Exp $
%%
%% Xy-pic ``Colour extension'' option.
%% Copyright (c) 1993-1996 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1996 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{color}{Colour extension}{\stripRCS$Revision: 3.3 $}%
 {Ross Moore}{ross@mpce.mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xydef@\xycolorwarning@@{\xycolormessage@
 \gdef\xycolorwarning@{\xycolormessage@
 \xywarning@{...no further colour warnings will be given.}%
 \global\let\xycolorwarning@=\relax }}
\xylet@\xycolorwarning@=\xycolorwarning@@
\xydef@\xycolormessage@{%
 \xywarning@{Current driver does not support colour.}}%
\xydef@\xyNoColor@#1{}
\xylet@\xycolor@@=\xyNoColor@
\xydef@\xyNoColor@@#1#2{\xycolorwarning@}
\xydef@\xycolor@{\xycolor@@}
\xylet@\xylocalColor@=\xyNoColor@@
\xydef@\UnloadColor@{%
 \let\xylocalColor@=\xyNoColor@@
 \let\xycolor@@=\xyNoColor@
 \let\xycolorwarning@=\xycolorwarning@@ }
\xylet@\UnloadColor@@=\UnloadColor@
\xyaddunsupport{color}{\UnloadColor@@\relax}
\ifx\current@color\undefined \xydef@\xybasecolor@{}%
\else \def\xybasecolor@{\current@color}\fi
\xydef@\xystackcolor@{\bgroup \DN@##1##2{\egroup}%
 \ifInvisible@\else\ifHidden@\else\DNii@{\no@@}\ifx\nextii@\Connect@@ 
 \else\DN@{\xystackcolor@i}\fi\fi\fi \next@ } 
\xydef@\xystackcolor@i#1#2{\checkXyStyle@ 
 \DN@{#2}\ifx\next@\empty
 \def\tmp@##1{\DN@{\xycolor@push{#1}##1\xycolor@pop}}%
 \else\def\tmp@##1{\DN@{\xycolor@push{#2 #1}##1\xycolor@pop}}\fi
 \toks@={\egroup \let\xy@style@=\relax \def\Drop@@}%
 \expandafter\tmp@\expandafter{\Drop@@}%
 \expandafter\addtotoks@\expandafter{\expandafter{\next@}\def\Connect@@}%
 \expandafter\tmp@\expandafter{\Connect@@}%
 \expandafter\addtotoks@\expandafter{\expandafter{\next@}}%
 \the\toks@ }%
\xydef@\xycolor@push@@#1{\special{color push #1}}
\xydef@\xycolor@pop{\special{color pop}}
\xylet@\xycolor@push=\xycolor@push@@
\xydef@\newxycolor#1#2{\newxyColor{#1}{}{}{#2}{}}
\xydef@\newxyColor#1#2#3#4{\newxycolor@{#1}{#2}{#3}{#4}{}}
\xydef@\newxycolor@#1#2#3#4#5{%
 \expandafter\let\expandafter\next@\csname shape [#1]\endcsname
 \ifx\next@\relax
 \DN@{#4}\ifx\next@\empty
 \DN@{#2}\ifx\next@\empty
 \DN@{\newxystyle{#1}{\xylocalColor@{}{#3}\xycolor@{#3}}}%
 \else
 \DN@{\newxystyle{#1}{\xylocalColor@{#2}{#3}\xycolor@{#2 #3}}}%
 \fi
 \else\DN@{#2#3}\ifx\next@\empty
 \DN@{\newxystyle{#1}{\xylocalColor@{#4}{}\xycolor@{#4}}}%
 \else
 \DN@{\newxystyle{#1}{\xylocalColor@{#2}{#3}\xycolor@{#4}}}%
 \fi \fi 
 \else \def\tmp@{\relax}\DNii@{#5}%
 \ifx\nextii@\tmp@
 \DN@{#4}\ifx\next@\empty
 \DN@{#2}\ifx\next@\empty
 \DN@{\newxystyle{#1}{\xylocalColor@{}{#3}\xycolor@{#3}}}%
 \else
 \DN@{\newxystyle{#1}{\xylocalColor@{#2}{#3}\xycolor@{#2 #3}}}%
 \fi
 \else
 \DN@{#2#3}\ifx\next@\empty
 \DN@{\newxystyle{#1}{\xylocalColor@{#4}{}\xycolor@{#4}}}%
 \else
 \DN@{\newxystyle{#1}{\xylocalColor@{#2}{#3}\xycolor@{#4}}}%
 \fi \fi 
 \else\DN@{}\fi\fi \next@\relax}
\xydef@\xystandardcolors@{%
 \newxycolor@{black}{0. 0. 0.}{rgb}{}\relax
 \newxycolor@{white}{1. 1. 1.}{rgb}{}\relax
 \newxycolor@{gray}{.5}{gray}{}\relax
 \newxycolor@{grey}{.5}{gray}{}\relax
 \newxycolor@{red}{1. 0. 0.}{rgb}{}\relax
 \newxycolor@{green}{0. 1. 0.}{rgb}{}\relax
 \newxycolor@{blue}{0. 0. 1.}{rgb}{}\relax
 \newxycolor@{cyan}{0. 1. 1.}{rgb}{}\relax
 \newxycolor@{magenta}{1. 0. 1.}{rgb}{}\relax
 \newxycolor@{yellow}{1. 1. 0.}{rgb}{}\relax
 \xyuncatcodes }
\xydef@\UseCrayolaColors{\xyrequire{crayon}\xyuncatcodes}%
\xydef@\xyBEcolorcheck@{\ifx\xycolor@@\xyNoColor@\else
 \xywarning@{PostScript colour support should be OK.}\fi }%
\xywithoption{ps}{%
 \xyinputorelse@{xyps-c}{\xyerror@{Could not load xyps-c}{}}}%
 \xycatcodes
\xyendinput


==> xycrayon.tex <==
%% xycrayon.tex from $Id: xycrayon.doc,v 3.3 1996/12/18 08:58:16 ross Exp $
%%
%% Xy-pic ``Crayola colours'' PostScript backend support.
%% Copyright (c) 1995-1996 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1996 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{crayon}{Crayola Colours}{\stripRCS$Revision: 3.3 $}%
 {Ross Moore}{ross@mpce.mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xydef@\installCrayolaColors@{%
 \xyinputorelse@{xyps-col}{\xyerror@{Could not load Crayola colours}{}}%
 \let\installCrayolaColors@=\relax
 \xyuncatcodes }
\xyendinput
#


==> xycurve.tex <==
%% xycurve.tex from $Id: xycurve.doc,v 3.7 1999/02/16 15:12:50 krisrose Exp $
%%
%% Xy-pic ``Curves and Splines'' extension.
%% Copyright (c) 1993-1997 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1997 Kristoffer H. Rose <krisrose@ens-lyon.fr>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{curve}{Curve and Spline extension}{\stripRCS$Revision: 3.7 $}%
 {Ross Moore}{ross@mpce.mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\message{curve,}
\xynew@{count}\crv@cnt@
\xydef@\xynumctrlpts@{\the\crv@cnt@}
\xynew@{toks}\crvpts@
\xydef@\setcurve@{%
 \edef\xysplineparams@{%
 \expandafter\noexpand\csname params@\endcsname}%
 \edef\xysplineedges@{%
 \expandafter\noexpand\csname edges@\endcsname}%
 \edef\xycrvcnt@{%
 \expandafter\noexpand\csname crvcnt@\endcsname}%
 \expandafter\edef\xycrvcnt@{\number\crv@cnt@}%
 \ifcase\crv@cnt@
 \expandafter\xycvxhull@\or
 \expandafter\xyquadbezier@\or
 \expandafter\xycubicbezier@\or
 \expandafter\xybspline@iii\or
 \expandafter\xybspline@iv\else
 \expandafter\xybspline@
 \fi}
\xydef@\curve{\connect\crv}
\xydef@\crv#1#{\hbox \bgroup \crvresetbreaks@ \initshape@
 \def\pure@crv{\crv@saveStyles@}\crv@{#1}}
\xydef@\crv@#1#2{%
 \DN@{#1}\ifx\empty\next@
 \DN@{\def\afterCURVEaction@{}\parsecurve@\xycurve@@}%
 \else\DN@{\parseCURVE@#1\parsecurve@\curveSTYLE@}\fi
 \next@ #2\@endcurve\endcrv@ }
\xydef@\curveSTYLE@{\xycurve@@}%
\xydef@\afterCURVEaction@{}%
\xydef@\@endcurve{}%
\xydef@\endcrv@@{\endcrv@\POS}%
\xydef@\pure@crv{\relax}
\xywarnifdefined\crv@normaltemplate
\xywarnifdefined\crv@othertemplate
\xywarnifdefined\crv@specialtemplate@@
{\xyuncatcodes \catcode`\@=11 \catcode`\#=6
 \gdef\crv@normaltemplate#1{{}{~**#1\xy@@crvaddstack@}}
 \gdef\crv@othertemplate#1{{}{~*=<2\jot>{}~**#1\xy@@crvaddstack@}}
 \gdef\crv@specialtemplate@@#1{{}{~**\dir{#1}\xy@@crvaddstack@}}
}
\xydef@\crvs#1#{\hbox \bgroup \def\pure@crv{\relax}\crvs@{#1}}%
\xydef@\crvi#1#{\hbox \bgroup \def\pure@crv{\relax}\invisbreaks@ \crvs@{#1}}%
\xydef@\crvs@#1{\DN@{\initshape@ \@crv@{#1}}%
 \def\crv@defaultshape{-}%
 \ifx\bstartPLACE@\relax \else
 \ifx\bstartPLACE@\empty \Invisible@true \else
\splinetrace@{bstartPLACE@=\bstartPLACE@, bendPLACE@=\bendPLACE@}%
 \DN@{\let\xy@@crvaddstack@=\xy@@samecurve@
 \let\saveshape@=\savesame@ 
 \let\savectrlptsnum@=\relax
 \let\startxycurve@=\recovercurve@ 
 \crv@cnt@=\xycrvptsnum@\relax \@crv@{#1}}%
 \fi \fi \next@ }
\xydef@\xy@@samecurve@{\xyFN@\checkendcurve@}
\xydef@\savesame@{\egroup }
\xydef@\recovercurve@{%
 \crv@cnt@=\xycrvptsnum@ \splinereset@ \recovercv@end
 \ifx\bendPLACE@\relax \def\bendPLACE@{1}\fi
 \ifdim\zz@\R@c \ifdim\zz@\L@c \ifdim\zz@\D@c \ifdim\zz@\U@c
 \Edge@c={\zeroEdge}\fi\fi\fi\fi
 \edef\cv@end{\cfromthec@}\edef\cv@start{\cfromthep@}}
\xydef@\recovercv@end{\count@=\ptsnum@\relax\advance\count@\@ne
 \edef\tmp@{\the\count@}\csname cv@\tmp@\endcsname}%
\xydef@\crvSTYLE@@{}
\expandafter\xydef@\expandafter\crv@defaultshape\expandafter{\addDASH@{}}
\xydef@\crv@noobject{\Invisible@true}
\xydef@\@crv@#1#2{\DN@{#1#2}%
 \ifx\next@\empty \edef\next@{\crv@defaultshape}%
 \ifx\bstartPLACE@\empty \xdef\crvSTYLE@@{{\crv@defaultshape}}\fi
 \else 
 \ifx\bstartPLACE@\empty \gdef\crvSTYLE@@{#1{#2}}\fi
 \fi
 \ifx\next@\empty \crv@noobject \DN@{\crv@{}{\xy@@crvaddstack@}}%
 \else\def\tmp@{-}\ifx\next@\tmp@ \DN@{\crv@{}{\xy@@crvaddstack@}}%
 \else\def\tmp@{=}\ifx\next@\tmp@ 
 \DN@{\expandafter\crv@\crv@normaltemplate{\dir{=}}}%
 \else\def\tmp@{2-}\ifx\next@\tmp@ 
 \DN@{\expandafter\crv@\crv@normaltemplate{\dir{2.}}}%
 \else\def\tmp@{3-}\ifx\next@\tmp@ 
 \DN@{\expandafter\crv@\crv@normaltemplate{\dir{3.}}}%
 \else\def\tmp@{--}\ifx\next@\tmp@
 \DN@{\expandafter\crv@\crv@specialtemplate@{--}}%
 \else\def\tmp@{==}\ifx\next@\tmp@ 
 \DN@{\expandafter\crv@\crv@normaltemplate{\dir2{--}}}%
 \else\def\tmp@{2--}\ifx\next@\tmp@ 
 \DN@{\expandafter\crv@\crv@normaltemplate{\dir2{--}}}%
 \else\def\tmp@{3--}\ifx\next@\tmp@ 
 \DN@{\expandafter\crv@\crv@normaltemplate{\dir3{--}}}%
 \else\def\tmp@{.}\ifx\next@\tmp@
 \DN@{\expandafter\crv@\crv@specialtemplate@{.}}%
 \else\def\tmp@{:}\ifx\next@\tmp@
 \DN@{\expandafter\crv@\crv@normaltemplate{\dir{:}}}%
 \else\def\tmp@{2.}\ifx\next@\tmp@
 \DN@{\expandafter\crv@\crv@normaltemplate{\dir{:}}}%
 \else\def\tmp@{..}\ifx\next@\tmp@
 \DN@{\expandafter\crv@\crv@specialtemplate@{.}}%
 \else
 \DN@{\expandafter\crv@\crv@othertemplate{\dir#1{#2}}}%
 \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi \next@}
\xylet@\crv@specialtemplate@=\crv@specialtemplate@@
\xydef@\crv@special#1{}
\xydef@\parseCURVE@{\def\curveSTYLE@{\xycurve@@}\def\afterCURVEaction@{}%
 \xyFN@\parseCURVE@@}
\xydef@\parseCURVE@@{%
 \ifx\space@\next\expandafter\DN@\space{\xyFN@\parseCURVE@@}%
 \else\ifx ~\next \DN@ ~{\xy@~{}\xyFN@\setcurveSTYLE@@}%
 \else\ifx\parsecurve@\next\DN@{}%
 \else\ifcat\active\noexpand\next\DN@{\xyactive@Warning}%
 \else\ifcat a\noexpand\next\DN@##1{\xytilde@Warning\setcurveSTYLE@{##1}%
 \xyFN@\parseCURVE@@}%
 \else\DN@{}\fi\fi\fi\fi\fi \next@ }%
\xydef@\xyactive@Warning{\xywarning@{expandable control sequences should 
 not be here, results are unpredictable in diagrams.}}%
\xydef@\xytilde@Warning{Please use ~ to set curve style.}%
\xydef@\setcurveSTYLE@#1{\xyFN@\setcurveSTYLE@@#1}
\xydef@\setcurveSTYLE@@{%
 \ifx\next p\def\curveSTYLE@{\xyc@trlpts@@}%
 \DN@ p{\xyFN@\setafterCURVEaction@}%
 \else\ifx\next P\def\curveSTYLE@{\xyc@trlpts@}%
 \DN@ P{\xyFN@\setafterCURVEaction@}%
 \else\ifx\next l\def\curveSTYLE@{\xyc@vxhull@@}%
 \DN@ l{\xyFN@\setafterCURVEaction@}%
 \else\ifx\next L\def\curveSTYLE@{\xyc@vxhull@}%
 \DN@ L{\xyFN@\setafterCURVEaction@}%
 \else\ifx\next c\def\curveSTYLE@{\xycurve@@}%
 \DN@ c{\xyFN@\setafterCURVEaction@}%
 \else\ifx\next C\def\curveSTYLE@{\xycurve@@}%
 \DN@ C{\xyFN@\setafterCURVEaction@}%
 \else \DN@##1{\xywarning@{unknown curve style ##1}\xyFN@\parseCURVE@@}%
 \fi\fi\fi\fi\fi\fi \next@ }
\xydef@\setafterCURVEaction@{%
 \ifx\next~\DN@~{\xyFN@\setcurveSTYLE@@}%
 \else\ifcat a\noexpand\next\DN@{\setafterCURVEaction@@}%
 \else\DN@{\xyFN@\parseCURVE@@}%
 \fi\fi \next@}
\xydef@\setafterCURVEaction@@{%
 \ifx\next c\DN@ c{%
 \def\afterCURVEaction@{\noexpand\endcurve\noexpand\xy@curve@}%
 \xyFN@\parseCURVE@@ }%
 \else\ifx\next C\DN@ C{%
 \def\afterCURVEaction@{\noexpand\endcurve\noexpand\xy@curve@@}%
 \xyFN@\parseCURVE@@ }%
 \else \DN@##1{\xywarning@{unknown after-curve action ##1}%
 \xyFN@\parseCURVE@@ }%
 \fi\fi \next@ }
\xydef@\parsecurve@{\xyFN@\parsecurve@@}
\xydef@\parsecurve@@{%
 \ifx\space@\next\expandafter\DN@\space{\xyFN@\parsecurve@@}%
 \else\ifx\next\@endcurve\DN@\@endcurve{\checkafterCURVE@}%
 \else\ifcat\active\noexpand\next\DN@{\relax}%
 \else\DN@{\xycurve@@}\fi\fi\fi\next@}%
\xydef@\xycurve@{\begingroup\afterCURVE{\setcurve@\endgroup}\crvobjects@
 \startxycurve@\xycrvmods@}
\xydef@\xycurve@@{\afterCURVE{\setcurve@}\crvobjects@\startxycurve@
 \xycrvmods@}
\xydef@\xy@curve@{\xy@curve@@@{\splinedefaulttol@\crvobjects@}}
\xydef@\xy@curve@@{\xy@curve@@@{\resetcrvobjects@}}
\xydef@\xy@curve@@@#1{\ifx\cv@start\relax
 \DN@{\xywarning@{There is no curve to plot}}.
 \else\DN@{\begingroup\afterCURVE{\setcurve@\endgroup}#1\cv@end}%
 \fi \next@ }
\xydef@\crvobjects@{\def\xycrvdrop@{}\def\xycrvconn@{}}
\xydef@\resetcrvobjects@{\crvobjects@}
\xylet@\savecurve=\xycurve@@
\xylet@\samecurve=\xy@curve@
\xydef@\xycrvmods@{\xyFN@\xy@crvmods@}%
\xydef@\xy@crvmods@{%
 \ifx\space@\next\expandafter\DN@\space{\xyFN@\xy@crvmods@}%
 \else\ifx\next ~\DN@ ~{\xyFN@\xy@crvmods@@}%
 \else\DN@{\xy@crvmods@@@@}\fi\fi \next@}%
\xydef@\xy@crvmods@@@@{\xyFN@\checkendcurve@}%
\xydef@\xy@crvmods@@{%
 \ifx\space@\next\expandafter\DN@\space{\xyFN@\xy@crvmods@@}%
 \else\ifx\next *\DN@ *{\xyFN@\xy@@crvmods@}%
 \else\addAT@\ifx\next\addAT@\DN@{\xyFN@\xy@@crvaddstack}%
 \else\DN@{\xywarning@{badly-formed curve option}\xyFN@\xy@crvmods@}%
 \fi\fi\fi \next@}%
\xydef@\xy@@crvmods@{%
 \ifx\space@\next\expandafter\DN@\space{\xyFN@\xy@@crvmods@}%
 \else\ifx\next *\DN@ *{\xyFN@\xy@@crvmods@@}%
 \else\DN@{\xy@crv@mods@@}\fi\fi \next@}%
\xydef@\xy@crv@mods@@#1#{\DN@##1{\xy@crvmods@@@{#1}{##1}}\next@}%
\xydef@\xy@crvmods@@@#1#2{%
 \DN@{#1#2}\ifx\next@\empty \def\xycrvdrop@{ #1{\zerodot}}%
 \else \def\xycrvdrop@{ #1{#2}}\fi
 \xyFN@\xy@crvmods@ }%
\xydef@\xy@@crvmods@@#1#{\DN@##1{\xy@@crvmods@@@{#1}{##1}}\next@}%
\xydef@\xy@@crvmods@@@#1#2{\def\xycrvconn@{ #1{#2}}\xyFN@\xy@crvmods@ }%
\xydef@\checkendcurve@{%
 \ifx\space@\next\expandafter\DN@\space{\xyFN@\checkendcurve@}%
 \else\ifx\next\endcurve\DN@\endcurve{\clearsearchflag@\endxycurve@}%
 \else\ifx\next\@endcurve\DN@\@endcurve{\checkafterCURVE@}%
 \else\ifx\next\xy@@crvaddstack@\DN@{}%
 \else\ifx\next\endxy\DN@{\clearsearchflag@\sloppyendcrv@}%
 \else\testAND@\iffalse \DN@##1{\clearsearchflag@\searchnextpt@}%
 \else\ifx ~\next\DN@ ~{\xyFN@\checkcrvtilde@}%
 \else\ifx\next\relax\DN@\relax{\clearsearchflag@\searchnextpt@}%
 \else\ifx\next\\\DN@\\{\clearsearchflag@\searchnextpt@}%
 \else\ifx\searchflag@\relax
 \DN@{\setsearchflag@\searchnextpt@}%
 \else\DN@##1{\flagwarn@{##1}}\fi
 \fi\fi\fi\fi\fi\fi\fi\fi\fi \next@ }
\xydef@\searchnextpt@{\afterPOS{\xy@@\addtocrv@ \xyFN@\checkendcurve@}}
\xydef@\checkafterCURVE@{%
 \edef\tmp@{\noexpand\xyFN@\noexpand\checkendcurve@
 \afterCURVEaction@\noexpand\endcurve}\tmp@ }
\xylet@\searchflag@=\relax
\xydef@\setsearchflag@{\let\searchflag@=@}
\xydef@\clearsearchflag@{\let\searchflag@=\relax}
\xydef@\flagwarn@#1{%
 \ifx\next\@endcurve\DN@{\xyFN@\checkendcurve@\endcurve}%
 \else\setsearchflag@\DN@{\xyFN@\checkendcurve@}%
 \xywarning@{skipping invalid token \string#1\space in curve}%
 \fi \next@ }
\xydef@\sloppyendcrv@{%
\xywarning@{Please use \string\endcurve\space to end the curve.}\endxycurve@}
\xydef@\endcrv@{\saveshape@
 \Edge@c={\splineEdge}\Invisible@false\Hidden@false
 \edef\Drop@@{\noexpand\ifInvisible@ \setbox\z@=\copy\voidb@x
 \noexpand\else
 \noexpand\wdz@=\z@
 \noexpand\ht\z@=\z@ \noexpand\dp\z@=\z@
 \noexpand\splineDrop@
 \noexpand\fi }%
 \edef\Connect@@{%
 \noexpand\setbox\z@=\noexpand\box\lastobjectbox@
 \noexpand\wdz@=\z@
 \noexpand\ht\z@=\z@ \noexpand\dp\z@=\z@
 \expandafter\noexpand\pure@crv
 \noexpand\ifInvisible@ \noexpand\crv@saveStyles@ \noexpand\else 
 \noexpand\crv@getStyles@\noexpand\styledboxz@ \noexpand\fi
 \noexpand\ifHidden@\noexpand\else 
 \noexpand\ifx\noexpand\COORD@\noexpand\xymatrixCOORD@ \noexpand\else
 \noexpand\X@min=\the\X@min \noexpand\X@max=\the\X@max 
 \noexpand\Y@min=\the\Y@min \noexpand\Y@max=\the\Y@max
 \noexpand\fi \noexpand\fi
 \savecrvparams@ \noexpand\crvconnect@
 }%
 \wdz@=\z@
 \ht\z@=\z@ \dp\z@=\z@ }
\xydef@\crvXY@pre@{}
\xydef@\crvXY@post@{}
\xydef@\crv@saveStyles@{\def\xy@style@{}%
 \expandafter\def\expandafter\crvXY@pre@\expandafter{\preXY@style@}%
 \expandafter\def\expandafter\crvXY@post@\expandafter{\postXY@style@}}
\xydef@\crv@getStyles@{\def\xy@style@{}%
 \gdef\preXY@style@{\crvXY@pre@}\gdef\postXY@style@{\crvXY@post@}}
\xydef@\initshape@{\savescope@ 
 \ifdim\X@c>\X@p \X@min=\X@p \X@max=\X@c \else \X@max=\X@p \X@min=\X@c \fi
 \ifdim\Y@c>\Y@p \Y@min=\Y@p \Y@max=\Y@c \else \Y@max=\Y@p \Y@min=\Y@c \fi }
\xydef@\saveshape@{\savectrlptsnum@ 
 \R@c=\X@max \advance\R@c-\X@c \L@c=\X@c \advance\L@c-\X@min
 \U@c=\Y@max \advance\U@c-\Y@c \D@c=\Y@c \advance\D@c-\Y@min
 \edef\tmp@{\egroup \U@c=\the\U@c \D@c=\the\D@c \L@c=\the\L@c \R@c=\the\R@c
 \noexpand\ifdim\noexpand\X@min>\the\X@min\noexpand\X@min=\the\X@min\noexpand\fi
 \noexpand\ifdim\noexpand\Y@min>\the\Y@min\noexpand\Y@min=\the\Y@min\noexpand\fi
 \noexpand\ifdim\noexpand\X@max<\the\X@max\noexpand\X@max=\the\X@max\noexpand\fi
 \noexpand\ifdim\noexpand\Y@max<\the\Y@max\noexpand\Y@max=\the\Y@max\noexpand\fi
 \savecrvparams@ \def\noexpand\pure@crv{\expandafter\noexpand\pure@crv}}%
 \tmp@ }
\xydef@\savecrvparams@{\crvpts@={\the\crvpts@}%
 \noexpand\def\noexpand\crvconnect@{\expandafter\noexpand\crvconnect@}}%
\xydef@\splineEdge{\rectangleEdge}
\xydef@\xy@@crvaddstack{%
 \ifx\next ~\xywarning@{there should be a poslist here, \string~@ ignored}%
 \DN@{\xy@crvmods@}%
 \else\DN@{\xy@@crvaddstack@}\fi \next@}
\xydef@\xy@@crvaddstack@{\smapxy@@\addtocrv@ \xyFN@\checkendcurve@}
\xydef@\checkcrvtilde@{%
 \addAT@\ifx\next\addAT@\DN@{\xy@@crvaddstack@}%
 \else\xywarning@{invalid token after ~, ignored}%
 \DN@##1{\xyFN@\checkendcurve@}%
 \fi \next@ }
\xydef@\crvconnect@@{%
 \def\Creset@@{\crvreset@}%
 \def\Cshavep@@{\crvshavep@}%
 \def\Cshavec@@{\crvshavec@}%
 \def\Cslidep@@{\crvslidep@}%
 \def\Cslidec@@{\crvslidec@}%
 \def\Calong@@{\crvalong@}%
 \def\Cintercept@@{\crvintercept@}%
 \def\Cbreak@@{\crvbreak@}%
 \def\Clast@@{\crvlast@}%
}
\xydef@\straitconnect@{\crvconnect@@ 
 \let\crvreset@=\straitreset@
 \let\crvshavep@=\straitshavep@
 \let\crvshavec@=\straitshavec@
 \let\crvslidep@=\straitslidep@
 \let\crvslidec@=\straitslidec@
 \let\crvalong@=\straitalong@
 \let\crvintercept@=\straitintercept@
 \let\crvbreak@=\straitbreak@
 \let\crvlast@=\straitlast@
}
\xydef@\straitreset@{\the\crvpts@ 
 \edef\xycrvptsnum@{\csname ptsnum@\endcsname}%
 \def\segmentnum@{0}}
\xydef@\straitslidep@{\setupDirection@ii \noCslidep@@ }
\xydef@\straitslidec@{\setupDirection@ii \noCslidec@@ }
\xydef@\straitshavep@{%
 \expandafter\ifnum\xycrvptsnum@>\z@
 \def\segmentnum@{0}%
 \csname cv@1\endcsname 
 \resetDirection@ \setupDirection@ii 
 \fi \noCshavep@@ }
\xydef@\straitshavec@{%
 \expandafter\ifnum\xycrvptsnum@>\z@
 \expandafter\count@@\xycrvptsnum@\relax 
 \bgroup \csname cv@\number\count@@\endcsname 
 \edef\tmp@{\egroup \X@p=\the\X@c \Y@p=\the\Y@c}\tmp@ 
 \edef\segmentnum@{\xycrvptsnum@}%
 \resetDirection@ \setupDirection@ii 
 \fi \noCshavec@@ }
\xydef@\straitalong@#1{%
 \ifdim#1\p@<\z@ 
 \xywarning@{parameter value #1 is negative, using 0}%
 \cfromp@ \def\PLACEf@{{0}}%
 \else 
 \dimen@=#1\p@ \count@=\dimen@ \divide\count@\p@ 
 \expandafter\count@@\xycrvptsnum@\relax \advance\count@@\@ne
 \advance\dimen@\segmentnum@\p@ 
 \advance\count@\segmentnum@\relax 
 \def\segmentnum@{0}%
 \ifnum\count@@<\count@
 \xywarning@{parameter value #1 too large, using \the\count@@}%
 \count@=\count@@ \advance\count@\m@ne \edef\PLACEf@{{1}}%
 \else
 \advance\dimen@-\count@\p@ 
 \ifdim\zz@\dimen@\ifnum\count@>\z@
 \advance\count@\m@ne \advance\dimen@\p@ \fi\fi
 \edef\PLACEf@{{\expandafter\removePT@\the\dimen@}}%
 \fi
 \ifnum\count@=\z@\else \bgroup
 \csname cv@\number\count@\endcsname 
 \edef\tmp@{\egroup \X@p=\the\X@c \Y@p=\the\Y@c}\tmp@
 \fi
 \advance\count@\@ne
 \ifnum\count@<\count@@
\splinetrace@{find place \the\dimen@\space along straight segment 
 \the\count@}%
 \csname cv@\number\count@\endcsname
 \fi
 \d@X=\X@c \advance\d@X-\X@p \d@Y=\Y@c \advance\d@Y-\Y@p 
 \fi \expandafter\noCalong@@\PLACEf@ \czeroEdge@ }
\xydef@\straitintercept@{\noCintercept@@}
\xydef@\straitbreak@{\straightCbreak@@}
\xydef@\straitlast@{\straightClast@@}
\xydef@\splineconnect@{%
 \let\crvreset@=\splinereset@
 \let\crvshavep@=\splineshavep@
 \let\crvshavec@=\splineshavec@
 \let\crvslidep@=\splineslidep@
 \let\crvslidec@=\splineslidec@
 \let\crvalong@=\splinealong@
 \let\crvintercept@=\splineintercept@
 \let\crvbreak@=\splinebreak@
 \let\crvlast@=\splinelast@
}
\xydef@\splinereset@{\the\crvpts@ 
 \edef\xycrvptsnum@{\csname ptsnum@\endcsname}%
 \edef\xysplineparams@{%
 \expandafter\noexpand\csname params@\endcsname}%
 \edef\xysplineedges@{%
 \expandafter\noexpand\csname edges@\endcsname}%
 \def\segmentnum@{1}\def\splinecorrect@p{0}\def\splinecorrect@c{0}%
 \splinelength@=\z@ \def\splineplace@f{.5}%
}
\xydef@\splineshavep@{\begingroup 
 \edef\xysplineedges@{%
 \expandafter\noexpand\csname edges@\endcsname}%
 \expandafter\expandafter\expandafter\getsplineedges@safe\xysplineedges@ @@%
 \edef\tmp@{\noexpand\removePT@\the\dimen5}%
 \edef\tmp@{\endgroup 
 \noexpand\def\noexpand\splinecorrect@p{\tmp@}}\tmp@ 
 \setupDirection@ii }
\xydef@\splineshavec@{\begingroup 
 \edef\xysplineedges@{%
 \expandafter\noexpand\csname edges@\endcsname}%
 \expandafter\expandafter\expandafter\getsplineedges@safe\xysplineedges@ @@%
 \dimen@=-\dimen7\relax \advance\dimen@\p@
%% \getcrvsegsnum@ \advance\dimen@\count@\p@
 \edef\tmp@{\noexpand\removePT@\the\dimen@}%
 \edef\tmp@{\endgroup 
 \noexpand\def\noexpand\splinecorrect@c{\tmp@}}\tmp@ 
 \setupDirection@ii }
\xydef@\splineslidep@#1{\enter@{\pfromthep@}%
 \begingroup \splinealong@@{0}{#1}+\splineslidep@@@
 \setupDirection@ii \leave@ }%
\xydef@\splineslidep@@@{%
 \d@X=\dimen5 \d@Y=\dimen7 \edef\tmp@{\postfind@}\tmp@ \dimen@=\splineval@
 \expandafter\count@\xycrvptsnum@\relax
 \ifnum\count@>\tw@ \advance\count@\m@ne 
 \advance\dimen@\segmentnum@\p@ \advance\dimen@-\p@ 
 \fi 
 \edef\tmp@{\endgroup \endgroup
 \noexpand\def\noexpand\xysplineval@{\the\splineval@}%
 \noexpand\def\noexpand\splinecorrect@p{\expandafter\removePT@\the\dimen@}%
\splinetrace@{slide = \the\splinelength@}%
 \X@c=\dimen@i \Y@c=\dimen3
 \d@X=\the\d@X \d@Y=\the\d@Y
 \noexpand\def\noexpand\segmentnum@{\segmentnum@}}\tmp@ }
\xydef@\splineslidec@#1{\enter@{\pfromthep@}%
 \begingroup
 \expandafter\splinealong@@\PLACEf@{#1}+\splineslidec@@@
 \setupDirection@ii \leave@ }
\xydef@\splineslidec@@@{%
 \d@X=\dimen5 \d@Y=\dimen7 \edef\tmp@{\postfind@}\tmp@ \dimen@=\splineval@
 \expandafter\count@\xycrvptsnum@\relax
 \ifnum\count@>\tw@ \advance\count@\m@ne 
 \advance\dimen@\segmentnum@\p@ \advance\dimen@-\p@ 
 \dimen@=-\dimen@ \advance\dimen@\count@\p@
 \else \dimen@=-\dimen@ \advance\dimen@\p@ \fi
%% splinecorrect@c is probably wrong here!!
 \edef\tmp@{\endgroup \endgroup
 \noexpand\def\noexpand\xysplineval@{\the\splineval@}%
 \noexpand\def\noexpand\splinecorrect@c{\expandafter\removePT@\the\dimen@}%
\splinetrace@{slide = \the\splinelength@; correct@c=\noexpand\splinecorrect@c}%
 \X@c=\dimen@i \Y@c=\dimen3
 \d@X=\the\d@X \d@Y=\the\d@Y
 \noexpand\def\noexpand\segmentnum@{\segmentnum@}}\tmp@ }
\xydef@\checkslidemore@#1{%
 \dimen@ii=-#1\relax\ifdim\dimen@ii<\z@\multiply\dimen@ii\m@ne\fi
 \dimen@=-\splinelength@ \advance\dimen@\dimen@ii\relax 
 \ifdim\dimen@<\z@\dimen@ii=-\dimen@\else\dimen@ii=\dimen@\fi
 \ifdim\dimen@ii<.2\p@\DN@{\splineslidec@@ \leave@}%
 \else \splinetrace@{not found yet, \the\dimen@ii\space still to go}%
 \dimen@ii=#1\relax\ifdim\dimen@ii<\z@\multiply\dimen@\m@ne\fi
 \DN@{\expandafter\splineslidemore@\expandafter{\the\dimen@}}\fi 
 \next@}%
\xydef@\splineslidemore@#1{%
 \expandafter\count@\segmentnum@\relax
 \ifdim#1<\z@\advance\count@\m@ne\dimen@=\p@
 \else\advance\count@\@ne\dimen@=\z@\fi
 \ifnum\count@<\@ne
 \expandafter\splinesegment@\expandafter{\segmentnum@}%
 \DN@{\xywarning@{cannot slide beyond start of curve}%
 \spline@find{\z@}{\z@}{}\splineslidec@@ \leave@ }%
 \else \expandafter\count@@\xycrvptsnum@\relax\advance\count@@\m@ne
 \expandafter\ifnum\count@@<\count@\relax
 \expandafter\splinesegment@\expandafter{\segmentnum@}%
 \DN@{\xywarning@{cannot slide beyond end of curve}%
 \spline@find{\p@}{\z@}{}\splineslidec@@ \leave@ }%
 \else
 \edef\segmentnum@{\the\count@}%
 \expandafter\splinesegment@\expandafter{\segmentnum@}%
\splinetrace@{sliding onto segment \segmentnum@}%
 \expandafter\spline@find\expandafter{\the\dimen@}{#1}{}%
 \DN@{\checkslidemore@{#1}}%
 \fi\fi \next@ }
\xydef@\splineslidec@@{%
 \dimen@=\splineval@ \advance\dimen@\segmentnum@\p@\advance\dimen@-\p@ 
 \edef\tmp@{\endgroup 
 \noexpand\def\noexpand\xysplineval@{\the\dimen@}%
\splinetrace@{slide = \the\splinelength@}%
 \X@c=\the\dimen@i \Y@c=\the\dimen3 \d@X=\the\dimen5 \d@Y=\the\dimen7 \postfind@ 
 \noexpand\def\noexpand\segmentnum@{\segmentnum@}}\tmp@
 \setupDirection@ii}
\xydef@\splinealong@#1{\def\postfind@{}\splinealong@@{#1}\z@+%
 \splineslidec@@ 
 \dimen@=\xysplineval@\relax 
 \count@=\xycrvptsnum@\relax \ifnum\count@>\@ne \advance\count@\m@ne\fi
 \ifnum\count@>\@ne \dimen@nth\count@\dimen@
 \fi \edef\bthisPLACE@{\expandafter\removePT@\the\dimen@}%
\splinetrace@{bthisPLACE@=\bthisPLACE@}}%
\xydef@\splinealong@@#1#2#3{%
 \edef\tmp@{#1}\relax \dimen@ii\tmp@\p@ 
%% \getcrvsegsnum@
%% \dimen@=-\count@\p@ 
 \dimen@=-\p@
 \expandafter\advance\expandafter\dimen@\splinecorrect@p\p@
 \expandafter\advance\expandafter\dimen@\splinecorrect@c\p@
 \edef\tmp@{#1}\relax \dimen@=-\tmp@\dimen@ \relax
 \expandafter\advance\expandafter\dimen@\splinecorrect@p\p@
 \getcrvsegsnum@ \multiply \dimen@ by\count@\relax
\splinetrace@{actual:\the\dimen@; f:\the\dimen@ii; p:\splinecorrect@p, c:\splinecorrect@c}%
 \count@=\dimen@ \divide\count@\p@ \DN@{\relax}%
 \def\tmp@{\relax}\ifx\next@\tmp@
 \expandafter\ifnum\xycrvptsnum@<\count@
 \xywarning@{parameter value #1 too large}%
 \DNii@{\relax}\DN@{\begingroup}%
 \else
 \edef\xysplineval@{\the\dimen@}%
 \advance\dimen@-\count@\p@ 
 \ifdim\dimen@=\z@ 
\splinetrace@{find knot point \the\count@}%
 \ifnum\count@=\z@ \count@=\@ne \else \dimen@=\p@ \fi
 \else \advance\count@\@ne
\splinetrace@{find point \the\dimen@\space on spline segment \the\count@}%
 \fi 
 \edef\segmentnum@{\the\count@}%
 \edef\next@{\begingroup\noexpand\splinesegment@{\the\count@}}%
 \edef\nextii@{%
 \noexpand\spline@find{\the\dimen@}{#2}{}\noexpand\checksplinefind@{#2}}%
 \ifx>#3\relax 
 \edef\nextii@{%
 \noexpand\spline@find{\the\dimen@}{#2}#3\noexpand\checksplinefind@{#2}}%
 \else\ifx-#3\relax \ifdim\dimen@>\z@\relax \ifdim\dimen@<\p@
 \dimen@=-\dimen@ \advance\dimen@\p@
 \edef\nextii@{\noexpand\splinereverse@ 
 \noexpand\spline@find{\the\dimen@}{#2}{}\noexpand\checksplinefind@{#2}}%
 \fi\fi
 \else\ifx<#3\relax \ifdim\dimen@>\z@\relax \ifdim\dimen@<\p@
 \dimen@=-\dimen@ \advance\dimen@\p@
 \edef\nextii@{\noexpand\splinereverse@ 
 \noexpand\spline@find{\the\dimen@}{#2}#3\noexpand\checksplinefind@{#2}}%
 \fi\fi
 \fi\fi\fi
 \fi\fi \expandafter\next@\nextii@ }
\xydef@\checksplinefind@#1{%
 \dimen@ii=#1\relax \dimen@=\splinelength@
 \ifdim\dimen@ii=\z@\DN@{}%
 \else
 \ifdim\dimen@ii<\z@\advance\dimen@\dimen@ii
 \else\advance\dimen@-\dimen@ii\fi
 \ifdim\dimen@<\z@\multiply\dimen@\m@ne\fi
 \ifdim\dimen@<.2\p@\DN@{}%
 \else
 \count@=\segmentnum@\relax 
 \ifdim\dimen@ii<\z@\advance\dimen@ii\splinelength@
 \ifnum\count@>\@ne\advance\count@\m@ne
 \edef\next@{\noexpand\splinesegment@{\the\count@}%
 \noexpand\spline@find\p@{\the\dimen@ii}{}%
 \noexpand\checksplinefind@{\the\dimen@ii}}%
 \else
 \xywarning@{cannot slide \the\dimen@ii\space before start}%
 \DN@{\splinesegment@\@ne \spline@find\z@\z@{}}\fi
 \else\advance\dimen@ii-\splinelength@
 \count@@=\numcontrolpts 
 \ifnum\count@<\count@@ \advance\count@\@ne
 \edef\next@{\noexpand\splinesegment@{\the\count@}%
 \noexpand\spline@find\z@{\the\dimen@ii}{}%
 \noexpand\checksplinefind@{\the\dimen@ii}}%
 \else
 \xywarning@{cannot slide \the\dimen@ii\space beyond end}%
 \DN@{\splinesegment@{\the\count@@}\spline@find\p@\z@{}}\fi
 \fi
 \fi\fi \next@ }
\xydef@\resetbreaks@{%
 \let\bstartPLACE@=\relax \let\bthisPLACE@=\empty
 \let\bendPLACE@=\relax \let\bprevPLACE@=\relax}
\xydef@\invisbreaks@{\resetbreaks@ \let\bstartPLACE@=\empty}
\xydef@\crvresetbreaks@{\resetbreaks@ \let\bstartPLACE@=\relax }
\xydef@\initbreaks@{\xy@@{\ifx\bstartPLACE@\relax
 \def\bstartPLACE@{0}\def\bendPLACE@{1}\else
 \ifx\bstartPLACE@\empty\def\bstartPLACE@{0}\def\bendPLACE@{1}%
 \fi\fi}}
\xydef@\lastbreaks@{\ifx\bprevPLACE@\relax \def\bstartPLACE@{0}%
 \else \expandafter \bprevPLACE@ \fi 
 \let\bprevPLACE@\relax \let\bendPLACE@\relax}
\xylet@\bstartPLACE@\relax
\xylet@\bendPLACE@\relax
\xylet@\bprevPLACE@\relax
\xydef@\bthisPLACE@{1}
\xydef@\splinebreak@{%
\splinetrace@{***new break*** this:\bthisPLACE@ }%
 \ifx\bthisPLACE@\empty\def\bendPLACE@{1}%
 \else\edef\bendPLACE@{\bthisPLACE@}\let\bthisPLACE@\empty\fi
 \ifx\bprevPLACE@\relax\def\bstartPLACE@{0}\else\expandafter\bprevPLACE@\fi
 \edef\bprevPLACE@{\def\noexpand\bstartPLACE@{\bendPLACE@}\pfromthec@}%
\splinetrace@{splineBREAK: \bstartPLACE@ <> \bendPLACE@}%
 \edef\cv@brend{\cfromthec@}%
 \edef\cv@brstart{\cfromthep@}%
 \expandafter\connect\expandafter\crvs\crvSTYLE@@{}%
 \let\cv@brend=\relax
 \let\cv@brstart=\relax
\splinetrace@{**break done**}%
} 
\xydef@\splinelast@{\splinereset@ \lastbreaks@
\splinetrace@{splineLAST}%
 \edef\cv@brend{\cfromthec@}%
 \edef\cv@brstart{\cfromthep@}%
 \expandafter\connect\expandafter\crvs\crvSTYLE@@{}%
 \let\cv@brend=\relax
 \let\cv@brstart=\relax
\splinetrace@{**last done**}%
 \resetbreaks@}
\xydef@\splineNointercept@{\enter@{\pfromthep@}%
 \begingroup \splinereset@ \csname cv@0\endcsname \swap@ 
 \count@=\ptsnum@ \advance\count@\@ne \csname cv@\the\count@\endcsname 
 \edef\tmp@{\endgroup \X@origin=\the\X@p \Y@origin=\the\Y@p
 \R@c=\the\d@X \U@c=\the\d@Y}\tmp@
 \loop@
 \dimen@=\ifdim\R@c<\z@-\fi\R@c
 \advance\dimen@ \ifdim\U@c<\z@-\fi\U@c
 \ifdim\dimen@>10\p@
 \advance\R@c \ifdim\R@c<\z@-\fi 16sp \divide\R@c\KK@ 
 \advance\U@c \ifdim\U@c<\z@-\fi 16sp \divide\U@c\KK@
 \repeat@
 \intersect@ \leave@}
\xydef@\splineintercept@{\Hidden@true\Invisible@true\splineintercept@i}
\xydef@\splineintercept@i{\enter@{\pfromthep@}\begingroup 
 \R@p=\X@c \L@p=\X@p \d@X=\R@p \advance\d@X-\L@p
 \D@p=\Y@c \U@p=\Y@p \d@Y=\D@p \advance\d@Y-\U@p
 \dimen@nth\KK@\d@X \edef\sd@X{\expandafter\removePT@\the\d@X}%
 \dimen@nth\KK@\d@Y \edef\sd@Y{\expandafter\removePT@\the\d@Y}%
 \dimen@=\sd@Y\L@p \advance\dimen@-\sd@X\U@p 
 \edef\sideOffset@{\the\dimen@}\def\closestseg@{1}%
 \let\crvconnect@@=\relax \crvconnect@
 \let\spline@end=\splinef@end
 \def\spline@start{\bgroup \def\prevnext@{+-}%
 \def\splinerec@{\let\splinerec@=\splineIrec@ \splineinterceptTest@}%
 \def\splinedecast@{\let\splinedecast@=\splinedecast@@
 \def\splineadvance@{\splineIadvance@@}\splinedecast@@}%
 \def\splineadvance@{\intercepthull@}%
 \global\let\splinepoint=\splineIpt@@
 \global\let\splinegoal@=\splinef@pt
 \global\let\splinefinish@=\splinefinish@@}%
 \begingroup \splineIsegment@ 
 \splinesetparams@ \splined@@ \def\postfind@{}\splineIplace@
 \setupDirection@ii \leave@ }
\xydef@\splineIplace@{%
 \d@X=\dimen5 \d@Y=\dimen7 \dimen@=\splineval@
 \expandafter\count@\xycrvptsnum@\relax
 \ifnum\count@>\tw@ \advance\count@\m@ne
 \advance\dimen@\segmentnum@\p@ \advance\dimen@-\p@ 
 \dimen@nth\count@\dimen@
 \fi \edef\tmp@{\endgroup \endgroup
 \def\noexpand\PLACEf@{{\expandafter\removePT@\the\dimen@}}%
 \X@c=\dimen@i \Y@c=\dimen3
 \d@X=\the\d@X \d@Y=\the\d@Y }\tmp@
\splinetrace@{PLACE = \PLACEf@:(\the\X@c, \the\Y@c)}%
 \expandafter\edef\expandafter\bthisPLACE@\PLACEf@
 }
\xydef@\splineIrec@{\splineinterceptTest@ }
\xydef@\squineIpt@{\edef\tmp@{\endgroup
 \def\noexpand\prevnext@{\next}\begingroup}\tmp@ }
\xydef@\squineIadvance@{\edef\tmp@{\endgroup
 \def\noexpand\prevnext@{\next}\def\noexpand\howclose@{\howclose@}}%
 \tmp@ \splineadvance@@\begingroup}
\xydef@\cubicIpt@{\edef\tmp@{\endgroup
 \def\noexpand\prevnext@{\next}\begingroup}\tmp@ }
\xydef@\cubicIadvance@{\edef\tmp@{\egroup
 \def\noexpand\prevnext@{\next}\def\noexpand\howclose@{\howclose@}}%
 \tmp@ \splineadvance@@\bgroup}
\xydef@\splineIsegment@{\DN@{\splinesegment@\@ne}%
 \ifx\splinesegment@\squinesegment@\else
 \ifx\splinesegment@\cubicsegment@\else\DN@{\findIsegment@}%
 \fi\fi\next@}
\xydef@\findIsegment@{\expandafter\count@\xycrvptsnum@ \count@@\z@ 
 \loop@ \advance\count@@\@ne \bgroup 
 \expandafter\splinesegment@\expandafter{\the\count@@}%
 \xysidesofinterval@
 \findIsegment@i \repeat@ 
 \expandafter\dimen@\prevhowclose@ \relax
 \ifdim\dimen@=\z@ \edef\closestseg@{\the\count@@}\fi
 \expandafter\splinesegment@\expandafter{\closestseg@}}
\xydef@\findIsegment@i{%
 \expandafter\ifx\next \expandafter\findIsegment@ii
 \else\expandafter\findIsegment@x\fi \next@ }
\xydef@\findIsegment@ii{\expandafter\count@\xycrvptsnum@ \relax
 \advance\count@\m@ne \ifnum\count@>\segmentnum@\relax
 \expandafter\findIsegment@y\else\expandafter\findIsegment@x\fi}
\xydef@\findIsegment@x{%
 \edef\next@{\egroup\def\noexpand\next{\next}%
 \def\noexpand\prevhowclose@{\prevhowclose@}%
 \def\noexpand\closestseg@{\closestseg@}\noexpand\iffalse}}
\xydef@\findIsegment@y{%
 \edef\next@{\egroup\def\noexpand\next{\next}%
 \def\noexpand\prevhowclose@{\prevhowclose@}%
 \def\noexpand\closestseg@{\closestseg@}\noexpand\iftrue}}
\xydef@\xysidesofinterval@{\bgroup 
 \L@p=\sd@X\Y@p \advance\L@p-\sd@Y\X@p \advance\L@p\sideOffset@
 \U@p=\sd@X\Y@c \advance\U@p-\sd@Y\X@c \advance\U@p\sideOffset@
 \def\this@{}\ifdim\L@p>\almostz@ \ifdim\U@p>\almostz@ \def\next{++}\else
 \ifdim\U@p<-\almostz@ \def\next{+-}\else\def\next{+0}\def\this@{-}\fi\fi
 \else\ifdim\L@p<-\almostz@ \ifdim\U@p>\almostz@ \def\next{-+}\else
 \ifdim\U@p<-\almostz@ \def\next{--}\else\def\next{-0}\def\this@{+}\fi\fi
 \else \ifdim\U@p>\almostz@ \def\next{0+}\else
 \ifdim\U@p<-\almostz@ \def\next{0-}\else\def\next{00}\def\this@{+}\fi\fi
 \fi\fi
 \ifx\this@\empty
 \L@p=\ifdim\L@p<\z@-\fi\L@p \U@p=\ifdim\U@p<\z@-\fi\U@p 
 \ifdim\L@p<\U@p \edef\howclose@{\the\L@p}\def\this@{-}%
 \else \edef\howclose@{\the\U@p}\def\this@{+}\fi
 \else\def\howclose@{0.0pt}\fi 
\splinetrace@{\next:\this@:\howclose@;\the\splineval@:%
 (\the\X@p,\the\Y@p);(\the\X@c,\the\Y@c)}%
 \ifdim\howclose@<\prevhowclose@\relax 
 \edef\tmp@{\egroup\def\noexpand\this@{\this@}\def\noexpand\next{\next}%
 \def\noexpand\howclose@{\howclose@}\def\noexpand\prevhowclose@{\howclose@}%
 \def\noexpand\closestseg@{\segmentnum@}}%
\splinetrace@{closest yet: \howclose@, in segment \segmentnum@}%
 \else
 \edef\tmp@{\egroup\def\noexpand\this@{\this@}\def\noexpand\next{\next}%
 \def\noexpand\howclose@{\howclose@}}%
 \fi \tmp@ }
\xydef@\splineinterceptTest@{%
 \xysidesofinterval@ \DN@{\splineadvance@}%
 \DNii@{0.0pt}\ifx\howclose@\nextii@ \DN@{\splineclosest@}%
 \else\expandafter\ifx\next \expandafter\ifx\prevnext@
 \ifx\next\prevnext@\else\DN@{\X@c=\X@p \Y@c=\Y@p 
 \splinefinishf@}\fi\fi
 \else \DN@{\splinedecast@}\fi\fi 
 {\splinefar@false \splinenear@\X@p\X@c\Y@p\Y@c 
 \ifsplinefar@ \aftergroup\next@
 \else\aftergroup\splineclosest@
\splinetrace@{too close: (\the\X@p,\the\Y@p)::(\the\X@c,\the\Y@c)}%
 \fi}}
\xydef@\splineclosest@{%
 \expandafter\ifx\this@-\relax
 \X@c=\X@p \Y@c=\Y@p \global\advance\splineval@-\splinedepth@
 \fi \splinefinishf@ }%
\xydef@\squinetestcvxhull@{\begingroup
\splinetrace@{hull: closest in segment \closestseg@}%
 \expandafter\splinesegment@\ifx\undefined\closestseg@\@ne\else\closestseg@\fi
 \X@c=\L@c \Y@c=\U@c \xysidesofinterval@ 
 \expandafter\ifx\next \expandafter\splineoutsidehull@@
 \else \expandafter\splineinsidehull@\fi}
\xydef@\cubictestcvxhull@{\begingroup
 \expandafter\splinesegment@\ifx\undefined\closestseg@\@ne\else\closestseg@\fi
 \X@c=\L@c \Y@c=\U@c \xysidesofinterval@ 
 \expandafter\ifx\next \expandafter\cubictestcvxhull@i
 \else \expandafter\splineinsidehull@\fi}
\xydef@\cubictestcvxhull@i{%
 \X@c=\R@c \Y@c=\D@c \xysidesofinterval@ 
 \expandafter\ifx\next \expandafter\splineoutsidehull@@
 \else \expandafter\splineinsidehull@\fi}
\xydef@\xysidesofhull@{\bgroup 
 \L@p=\sd@X\Y@p \advance\L@p-\sd@Y\X@p \advance\L@p\sideOffset@
 \U@p=\sd@X\Y@c \advance\U@p-\sd@Y\X@c \advance\U@p\sideOffset@
 \L@p=\ifdim\L@p<\z@-\fi\L@p \U@p=\ifdim\U@p<\z@-\fi\U@p 
 \ifdim\L@p<\U@p \edef\howclose@{\the\L@p}\def\this@{-}%
 \else \edef\howclose@{\the\U@p}\def\this@{+}\fi
 \ifx\splinedecast@\squinedecast@ \D@c=\U@c \R@c=\L@c \fi
 \L@p=\sd@X\U@c \advance\L@p-\sd@Y\L@c \advance\L@p\sideOffset@
 \L@p=\ifdim\L@p<\z@-\fi\L@p 
 \expandafter\if\this@-%
 \ifdim\L@p<\prevhowclose@ \def\next{-+}\else \def\next{--}\fi
 \else
 \ifdim\L@p<\howclose@ \def\next{-+}\else 
 \U@p=\sd@X\D@c \advance\U@p-\sd@Y\R@c \advance\U@p\sideOffset@
 \U@p=\ifdim\U@p<\z@-\fi\U@p
 \ifdim\U@p<\howclose@ \def\next{+-}\else \def\next{++}\fi
 \fi\fi
 \edef\tmp@{\egroup\def\noexpand\this@{\this@}\def\noexpand\next{\next}%
 \def\noexpand\howclose@{\howclose@}}\tmp@ }
\def\PLACE@intercept@#1{%
 \xy@@{\enter@{\pfromthep@\basefromthebase@}\begingroup}%
 \xy@@ix@{#1}\xy@@{\plainxy@ \def\Creset@@{}%
 \expandafter\POS\the\toks9\relax
 \DNii@{\crvreset@}\ifx\nextii@\Creset@@ \edef\next@{\endgroup
 \def\noexpand\xyinterceptpts@{\the\crvpts@}%
 \X@c =\the\X@c \Y@c=\the\Y@c \X@p=\the\X@p \Y@p=\the\Y@p
 \noexpand\CCintercept@@ }%
 \else \edef\next@{\endgroup
 \X@c =\the\X@c \Y@c=\the\Y@c \X@p=\the\X@p \Y@p=\the\Y@p
 \noexpand\Cintercept@@ }%
 \fi \next@ \leave@}%
 \PLACE@@}
\xydef@\CCintercept@@{\splineSintercept@}
\xydef@\splineSintercept@{\enter@{\pfromthep@}\begingroup 
 \Creset@@ \edef\connect@pts{\cfromthec@ \pfromthep@}%
 \xyinterceptpts@ \splinereset@ \connect@pts \splineintercept@
 \edef\next@{\endgroup \cfromthec@ \DirectionfromtheDirection@ }%
 \next@ \let\xyinterceptpts@=\empty \leave@}
\xydef@\nointerceptwarning@{\let\nointerceptwarning@=\relax
 \xywarning@{perhaps no curve intersection, or many. }}
\xydef@\intercepthull@{\nointerceptwarning@ 
 \expandafter\def\expandafter\prevnext@\expandafter{\next}%
 \splinetestcvxhull@}
\xydef@\splinetestcvxhull@{\begingroup 
 \X@c=\L@c \Y@c=\U@c \splinetrace@{hull:}\xysidesofinterval@ 
 \expandafter\ifx\next \expandafter\splineoutsidehull@@
 \else \expandafter\splineinsidehull@\fi}
\xydef@\splineinsidehull@{\edef\tmp@{\endgroup 
 \def\noexpand\howcvxclose@{\howclose@}%
 \noexpand\interceptinsidehull@}\tmp@ }
\xydef@\interceptinsidehull@{\edef\prevhowclose@{\howclose@}%
 \splinedecast@@ }
{\xdef\next{\the\maxdimen}}
\xylet@\prevhowclose@=\next
\xydef@\splineoutsidehull@{\edef\tmp@{\endgroup
 \def\noexpand\howcvxclose@{\howclose@}%
 \noexpand\interceptoutsidehull@}\tmp@}
\xylet@\splineoutsidehull@@=\splineoutsidehull@
\xydef@\interceptoutsidehull@{\dimen@=\howcvxclose@ \relax
\splinetrace@{OUTSIDE HULL: \the\dimen@ : (\howclose@)(\prevhowclose@)}%
 \let\splinedecast@=\splinedecast@@
 \let\splinerec@\splineHnear@test
 \let\splineadvance@\splineIadvance@@
 \splinedecast@@ }
\xydef@\splineHnear@test{%
 \xysidesofhull@ \DN@{\splinedecast@}%
 \ifdim\howclose@<\prevhowclose@\edef\howclose@{\prevhowclose@}\fi
 \expandafter\if\this@-%
 \expandafter\ifx\next\DN@{\splineclosest@}\fi
 \else
 \expandafter\ifx\next\DN@{\splineadvance@}\fi
 \fi
 {\splinefar@false \splinenear@\X@p\X@c\Y@p\Y@c 
 \ifsplinefar@ \aftergroup\next@
 \else\aftergroup\splineclosest@
\splinetrace@{too close: (\the\X@p,\the\Y@p)::(\the\X@c,\the\Y@c)}%
 \fi}}
\xydef@\cubicoutsidehull@{\edef\tmp@{\endgroup
 \def\noexpand\howcvxclose@{\howclose@}}\tmp@
 \edef\prevhowcvxclose@{\howcvxclose@}\begingroup 
 \X@p=\R@c \Y@p=\D@c \splinetrace@{hullii:}\xysidesofinterval@ 
 \expandafter\ifx\next \expandafter\cubicoutsidehull@i
 \else \expandafter\cubicinsidehull@\fi} 
\xydef@\cubicinsidehull@{\edef\tmp@{\endgroup
 \def\noexpand\howclose@{\howclose@}}\tmp@
 \cubicoutsidehull@ii }
\xydef@\cubicoutsidehull@i{\edef\tmp@{\endgroup
 \def\noexpand\howcvxclose@{\howclose@}}\tmp@
 \dimen@=\prevhowcvxclose@\relax 
 \ifdim\dimen@<\howcvxclose@ \relax
 \edef\howcvxclose@{\the\dimen@}\expandafter\interceptoutsidehull@
 \else \expandafter\cubicoutsidehull@ii\fi }
\xydef@\cubicoutsidehull@ii{%
 \def\splineadvance@{\splineadvance@@}%
 \def\splinepoint\endgroup{\endgroup
 \global\let\splinepoint=\relax
 \def\splineadvance@{\intercepthull@}}%
 \splinedecast@@ }%
\xydef@\splineHadvance@{\futurelet\next@\splineHadvance@i}
\xydef@\splineHadvance@i{\ifx\next@\endgroup
 \expandafter\splineHadvance@x\else\expandafter\splineclosest@\fi}
\xydef@\splineHadvance@x{\edef\tmp@{\endgroup
 \def\noexpand\prevhowclose@{\prevhowclose@}%
 \def\noexpand\prevnext@{\next}\def\noexpand\howcvxclose@{\howclose@}}%
 \tmp@ \dimen@=\prevhowclose@ \relax
 \ifdim\dimen@<\howclose@ \relax \DN@{\splineclosest@\begingroup}%
 \else\ifdim\howcvxclose@=\dimen@\DN@{\splineclosest@\begingroup}%
 \else\DN@{\splineadvance@@\begingroup}\fi\fi \next@ }
\xydef@\xyclearcrv@{\cv@end\cv@restore\loop@
 \expandafter\let\csname cv@\number\crv@cnt@\endcsname\relax
 \ifnum\crv@cnt@>0\advance\crv@cnt@\m@ne\repeat@
 \let\cv@start=\relax \let\cv@end=\relax \let\cv@restore=\relax \POS}
\xylet@\clearcurve=\xyclearcrv@
\xylet@\numcontrolpts=\xynumctrlpts@
\xydef@\xycontrolpt@#1{{%
 \ifnum#1<\z@\aftergroup\cv@restore\aftergroup\cv@start
 \else
 \expandafter\count@\xycrvptsnum@\relax \advance\count@\@ne
 \ifnum#1>\count@ \ifx\cv@end\relax 
 \expandafter\aftergroup\csname cv@\number#1\endcsname
 \else\aftergroup\cv@end\fi
 \else 
 \expandafter\ifx\csname cv@\number#1\endcsname\relax
 \ifnum#1=\z@\aftergroup\cv@start\else\aftergroup\cv@end\fi
 \else\expandafter\aftergroup\csname cv@\number#1\endcsname
 \fi\fi\fi}}%
\xylet@\xycontrolpt=\xycontrolpt@
\xydef@\startxycurve@@{\crv@cnt@=\z@
 \edef\cv@start{\cfromthep@}%
 \ifdim\zz@\R@c \ifdim\zz@\L@c \ifdim\zz@\D@c \ifdim\zz@\U@c
 \Edge@c={\zeroEdge}\fi\fi\fi\fi
 \edef\cv@end{\cfromthec@}%
 \edef\cv@restore{\pfromthep@\basefromthebase@}}
\xylet@\startxycurve@=\startxycurve@@
\xylet@\cv@start=\relax
\xylet@\cv@end=\relax
\xylet@\cv@restore=\relax
\xydef@\readxycurve@{\startxycurve@\xycrvmods@}
\xylet@\readxycurve=\readxycurve@
\xydef@\addtocrv@{\advance\crv@cnt@\@ne 
 \edef\tmp@{%
 \expandafter\noexpand\csname cv@\number\crv@cnt@\endcsname}%
 \expandafter\edef\tmp@{\cfromthec@}%
 \edef\tmp@{\noexpand\addtocrvpts@{\noexpand\def
 \expandafter\noexpand\tmp@{\X@c=\the\X@c \Y@c=\the\Y@c }}}\tmp@
 \edef\xycrvptsnum@{\the\crv@cnt@}%
}
\xydef@\xycrvdrop@{ {\zerodot}}
\xydef@\xycrvconn@{}
\xydef@\xyc@trlpts@{\def\xycrvdrop@{ \dir{x}}\def\xycrvconn@{}%
 \afterCURVE{\savecrvobjects@\xyctrlpts@}\readxycurve@}
\xydef@\xyc@trlpts@@{%
 \afterCURVE{\savecrvobjects@\def\xycrvdrop@{ \dir{x}}%
 \def\xycrvconn@{}\xyctrlpts@}\readxycurve@}
\xydef@\xyc@vxhull@{\def\xycrvdrop@{ {}}%
 \edef\xycrvconn@{ \noexpand\dir{\addDASH@{}}}%
 \afterCURVE{\savecrvobjects@\xycvxhull@}\readxycurve@}
\xydef@\xyc@vxhull@@{%
 \afterCURVE{\savecrvobjects@\def\xycrvdrop@{ {}}%
 \edef\xycrvconn@{ \noexpand\dir{\addDASH@{}}}\xycvxhull@}\readxycurve@}
\xylet@\controlpts=\xyc@trlpts@
\xylet@\convexhull=\xyc@vxhull@
\xydef@\savecrvobjects@{\bgroup 
 \expandafter\toks@\expandafter{\xycrvdrop@}%
 \expandafter\toks@ii\expandafter{\xycrvconn@}%
 \edef\tmp@{\egroup\noexpand\def\noexpand\resetcrvobjects@{%
 \noexpand\def\noexpand\xycrvdrop@{\the\toks@}%
 \noexpand\def\noexpand\xycrvconn@{\the\toks@ii}%
 }}\tmp@}
\xydef@\afterCURVE#1{\def\afterCURVE@{#1}}
\xydef@\endxycurve@{\cv@end\savectrlptsnum@
 \expandafter\def\csname params@\endcsname{\the\crvpts@}%
 \cv@restore\afterCURVE@\POS}
\xylet@\endcurve=\endxycurve@
\xydef@\xyctrlpts@{\cv@end \cv@restore
 \def\crvconnect@{\straitconnect@}%
 \ifnum\crv@cnt@>\z@ 
 \count@@@=\@ne \DN@{\loop@\xycontrolpt@{\count@@@}\relax
 \expandafter\xycvxhulldrop@\xycrvdrop@
 \ifnum\crv@cnt@>\count@@@\advance\count@@@\@ne\repeat@ 
 \cv@end \cv@restore }%
 \else\DN@{\relax}\fi \next@ }
\xylet@\xyctrlpts=\xyctrlpts@
\xydef@\addtocrvpts@#1{\crvpts@=\expandafter{\the\crvpts@#1}}
\xydef@\savescope@{\crvpts@={}%
 \edef\tmp@{\expandafter\noexpand\csname cv@0\endcsname}%
 \edef\tmp@{\noexpand\addtocrvpts@{\noexpand\def
 \expandafter\noexpand\tmp@{\X@c=\the\X@p \Y@c=\the\Y@p}}}%
 \tmp@ }
\xydef@\savectrlptsnum@{%
 \advance\crv@cnt@\@ne \edef\tmp@{%
 \expandafter\noexpand\csname cv@\number\crv@cnt@\endcsname}%
 \edef\tmp@{\noexpand\addtocrvpts@{\noexpand\def
 \expandafter\noexpand\tmp@{\X@c=\the\X@c \Y@c=\the\Y@c}}}\tmp@
 \advance\crv@cnt@\m@ne 
 \edef\tmp@{\expandafter\noexpand\csname ptsnum@\endcsname}%
 \edef\tmp@{\noexpand\addtocrvpts@{%
 \noexpand\def\expandafter\noexpand\tmp@{\number\crv@cnt@}}}%
 \tmp@ }
\xydef@\xycvxhull@{\cv@end \cv@restore 
 \addtocrvpts@{\def\crvconnect@{\straitconnect@}}%
 \def\crvconnect@{\straitconnect@}%
 \ifnum\crv@cnt@>\z@ 
 \count@@@=\@ne\relax \DN@{\loop@\xycontrolpt@{\count@@@}\relax
 \expandafter\xycvxhulldrop@\xycrvdrop@
 {\expandafter\connect\xycrvconn@{}}\pfromc@
 \ifnum\crv@cnt@>\count@@@\relax \advance\count@@@\@ne\repeat@ 
 \cv@end }%
 \else
 \ifx\empty\xycrvconn@
 \edef\xycrvconn@{\noexpand!C\noexpand\dir{\addDASH@{}}}\fi
 \DN@{\relax}\fi \next@ 
 {{\expandafter\connect\xycrvconn@{}}}%
 \cv@end \cv@restore }
\xylet@\xycvxhull=\xycvxhull@
\xydef@\xycvxhulldrop@#1#{\drop@{#1}}
\xydef@\savespline@{%
\splinetrace@{savespline@:}%
 \edef\endspline@{\endgroup 
 \savesplineparams@ \savesplinerefs@
 \X@min=\the\X@min\relax \X@max=\the\X@max\relax
 \Y@min=\the\Y@min\relax \Y@max=\the\Y@max\relax
 \ifInvisible@\noexpand\Invisible@true
 \else\noexpand\Invisible@false\fi
 }\endspline@ 
 \edef\tmp@{\noexpand\addtocrvpts@{\savesplineparams@}}\tmp@
 \xycontrolpt@\z@ \cv@end }
\xydef@\savesplineparams@{%
 \noexpand\def\expandafter\noexpand\xysplineedges@{\xysplineedges@}}
\xydef@\savesplinerefs@{%
 \noexpand\def\noexpand\xysplineparams@{%
 \expandafter\noexpand\xysplineparams@}%
 \noexpand\def\noexpand\xysplineedges@{%
 \expandafter\noexpand\xysplineedges@}%
}
\xynew@{box}\splinebox@ 
\xynew@{dimen}\splineval@ 
\xynew@{dimen}\splinedepth@ 
\xynew@{dimen}\splinetol@ 
\xynew@{dimen}\splinelength@ 
\xynew@{if}\ifsplinefar@
\xynew@{if}\ifsplineplot@
\xydef@\splinetracing{\let\splinetrace@=\W@}
\xydef@\splineignore@#1{}
\xylet@\splinetrace@=\splineignore@
\xydef@\readsplineparams@{%
 \expandafter\expandafter\expandafter\getsplineparams@\xysplineparams@
 \expandafter\expandafter\expandafter\getsplineedges@safe\xysplineedges@ @@}
\xydef@\getsplineedges@safe#1@@{\DN@{#1}%
 \ifx\next@\empty \DN@{\getsplineedges@.0pt;0.0pt,0.0pt;0.0pt,}%
 \else \DN@{\getsplineedges@safe@#1@@}\fi \next@}
\xydef@\getsplineedges@safe@#1;#2,#3@@{\DN@{#3}%
\splinetrace@{getsplineedges@safe}%
 \ifx\next@\empty \DN@{\getsplineedges@#1;#2,0.0pt;0.0pt,}%
 \else \DN@{\getsplineedges@#1;#2,#3}\fi \next@}
\xydef@\getsplineedges@#1;#2,#3;#4,{%
 \global\dimen@i=#1\global\dimen5=#2\relax
 \dimen@=#3\multiply\dimen@\m@ne \advance\dimen@\splinelength@
 \global\dimen3=\dimen@
 \dimen@=#4\relax 
 \ifdim\dimen@>\p@ \xywarning@{edge out-of-range: \the\dimen@}%
 \count@=\dimen@ \divide\count@\p@
 \advance\dimen@-\count@\p@ \multiply\dimen@\m@ne
 \advance\dimen@ \count@\p@ \advance\dimen@\p@
\splinetrace@{\the\dimen@}%
 \else
 \multiply\dimen@\m@ne \advance\dimen@\p@
 \fi
 \global\dimen7=\dimen@ }
\xydef@\dimen@half{%
 \advance\dimen@ \ifdim\dimen@<\z@-\fi 1sp \divide\dimen@\tw@}
\xydef@\halve@dimen#1{\dimen@=#1\relax \dimen@half #1=\dimen@}
\xydef@\dimen@nth#1#2{\dimen@=#2\relax \dimen@ii=#1sp
 \advance\dimen@ \ifdim\dimen@<\z@-\fi.5\dimen@ii 
 \divide\dimen@ by#1\relax #2=\dimen@}
\xydef@\splinetolerance@#1{\dimen@=#1\relax
 \ifdim\dimen@>\z@ \splinetol@=\dimen@
 \else\splinetol@=.4\p@\fi}
\xylet@\splinedefaulttol@=\relax
\xydef@\splinetolerance#1{\splinetolerance@{#1}%
 \edef\splinedefaulttol@{\splinetol@=\the\splinetol@}}
\splinetolerance\z@
\xydef@\SloppyCurves{\splinetolerance{.8\p@}}
\xydef@\xylowtolerance@{\splinedefaulttol@
 \ifdim\splinetol@<\p@ \divide\splinetol@\tw@ \fi}
\xywarnifdefined\splinedrop@
\xydef@\setstdsplinedrop@{%
 \setbox\splinebox@=\hbox\bgroup
 \setboxz@h{\expandafter\object\xycrvdrop@{}}%
 \splinedefaulttol@ \dimen@=\wd\z@ \dimen@ii=\ht\z@ \advance\dimen@ii\dp\z@
 \ifdim\dimen@ii>\dimen@ \dimen@=\dimen@ii \fi \dimen@=1.4142\dimen@
 \ifdim\dimen@>\splinetol@ \splinetol@=\dimen@\else\dimen@=\splinetol@\fi
 \dimen@=.5\wd\z@ 
 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \kern-\dimen@ \Drop@@ \kern\dimen@
 \edef\tmp@{\egroup \splinetol@=\the\splinetol@
 \ifInvisible@\noexpand\Invisible@true
 \else\noexpand\Invisible@false\fi}\tmp@
 \edef\splinedefaulttol@{\splinetol@=\the\splinetol@}%
 \def\splinedrop@{\copy\splinebox@\splineextra@@}}
\xywarnifdefined\splineconn@
\xydef@\stdsplineconn@{{\setsplinedir@
 \setboxz@h\bgroup\expandafter\object\xycrvconn@{}%
 \edef\tmp@{\egroup\L@c=\the\L@c \R@c=\the\R@c \D@c=\the\D@c \U@c=\the\U@c
 \noexpand\def\noexpand\Drop@@}\expandafter\tmp@\expandafter{\Drop@@}%
 \setboxz@h{\kern-\L@c \boxz@}%
 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \Drop@@}}
\xydef@\setcrvobjects@{\setstdsplinedrop@ \def\splineconn@{\stdsplineconn@}}
\xylet@\splineextra@@=\relax
\xydef@\splinenear@#1#2#3#4{{\d@X=#1\advance\d@X-#2%
 \ifdim\d@X<\z@ \d@X=-\d@X\fi
 \ifdim\splinetol@<\d@X \aftergroup\splinefar@true
 \else \d@Y=#3\advance\d@Y-#4\ifdim\d@Y<\z@ \d@Y=-\d@Y\fi
 \ifdim\splinetol@<\d@Y\aftergroup\splinefar@true
 \else \xydist@\d@X\d@Y
 \ifdim\splinetol@<\dimen@ \aftergroup\splinefar@true
 \else 
 \ifdim\dimen@<.1\splinetol@\aftergroup\splinetooclose@\fi
 \fi\fi\fi}}
\xydef@\splineadvance@@{\global\advance\splineval@\splinedepth@}
\xydef@\splinetooclose@{\aftergroup\aftergroup\aftergroup\splinetooclose@@}
\xydef@\splinetooclose@@{\def\splineplotpt@{\relax}}
\xydef@\splinepoint@@{%
\splinetrace@{P@:(\the\X@c,\the\Y@c)::\the\splineval@;\the\splinedepth@}%
 {\splinetest@\ifsplineplot@\relax\else\aftergroup\splinecontinue\fi}}
\xydef@\splinepoint@{%
 {\splinetest@\ifsplineplot@\aftergroup\splinecontinue\fi}}
\xylet@\splinepoint=\splinepoint@
\xydef@\splinecontinue@{%
 \global\let\splinepoint=\splinepoint@@
 \global\let\splinecontinue=\splinecontinue@@}
\xydef@\splinecontinue@@{%
 \global\let\splinepoint=\splinepoint@
 \global\let\splinecontinue=\relax}
\xylet@\splinecontinue=\splinecontinue@
\xydef@\splineknotpoint@{{\X@p=\X@c \Y@p=\Y@c \cv@start 
 \the\Edge@c\@ne \ifInside@\else\aftergroup\splineknotpoint@@\fi}}%
\xydef@\splineknotpoint@@{{\X@p=\X@c \Y@p=\Y@c \cv@end 
 \the\Edge@c\@ne \ifInside@\else \aftergroup\splinepoint\fi}}%
\xylet@\firstsplinepoint@=\splineknotpoint@
\xylet@\lastsplinepoint@= \splineknotpoint@
\xydef@\splined@@@{%
\splinetrace@{finding end types}%
\splinetrace@{bstartPLACE@:\bstartPLACE@; bendPLACE@:\bendPLACE@}%
 \DN@{\splinescan@}\ifx\bstartPLACE@\empty
 \ifx\bendPLACE@\relax\def\bendPLACE@{1}\fi
 \else\ifx\bstartPLACE@\relax
 \else\ifx\bstartPLACE@\undefined
 \else 
 \DN@{\splinescanbreak@}\ifx\bendPLACE@\relax\def\bendPLACE@{1}\fi
 \DNii@{0}\ifx\bstartPLACE@\nextii@
 \DNii@{1}\ifx\bendPLACE@\nextii@\DN@{}%
 \fi\fi
 \fi\fi\fi \next@ }%
\xydef@\splineStarttest@{{\X@p=\X@c \Y@p=\Y@c \cv@start \the\Edge@c\@ne 
 \ifInside@\aftergroup\splineplot@false\else\aftergroup\splineplot@true\fi}}%
\xydef@\splineEndtest@{{\X@p=\X@c \Y@p=\Y@c \cv@end \the\Edge@c\@ne 
 \ifInside@\aftergroup\splineplot@false\else\aftergroup\splineplot@true\fi}}%
\xydef@\splineBreakStarttest@{{\X@p=\X@c \Y@p=\Y@c \cv@brstart \the\Edge@c\@ne 
 \ifInside@\aftergroup\splineplot@false\else\aftergroup\splineplot@true\fi}}%
\xydef@\splineBreakEndtest@{{\X@p=\X@c \Y@p=\Y@c \cv@brend \the\Edge@c\@ne 
 \ifInside@\aftergroup\splineplot@false\else\aftergroup\splineplot@true\fi}}%
\xylet@\splineStarttest=\splineStarttest@
\xylet@\splineEndtest=\splineEndtest@
\xydef@\splineSlowStarttest{{\X@p=\X@c \Y@p=\Y@c \cv@start \the\Edge@c\@ne 
 \ifInside@\aftergroup\splineplot@maybe@@\else\aftergroup\splineplot@true\fi}}%
\xydef@\splineSlowEndtest{{\X@p=\X@c \Y@p=\Y@c \cv@end \the\Edge@c\@ne 
 \ifInside@\aftergroup\splineplot@maybe@@\else\aftergroup\splineplot@true\fi}}%
\xydef@\splineplot@maybe{\splineplot@false}%
\xylet@\splineplot@maybe@@=\splineplot@maybe
\xydef@\splinescan@{\bgroup%
 \expandafter\def\xysplineedges@{\z@;\z@,\z@;\z@,}%
 \bgroup \cv@start 
 \expandafter\DN@\expandafter{\the\Edge@c}\DNii@{\zeroEdge}%
 \ifx\next@\nextii@ \gdef\splineedges@{\z@;\z@,}%
 \else\aftergroup\splinestartScan@\fi
 \egroup \relax
 \bgroup \cv@end 
 \expandafter\DN@\expandafter{\the\Edge@c}\DNii@{\zeroEdge}%
 \ifx\next@\nextii@ 
 \getcrvsegsnum@ \edef\segmentnum@{\the\count@}%
 \splineval@=\z@ \splineRecordEndValue@
 \else\aftergroup\splineendScan@\fi
 \egroup \egroup
 \expandafter\testsplineedges@\splineedges@;,@@%
 \expandafter\edef\xysplineedges@{\splineedges@}%
 \global\let\splineedges@=\relax
\splinetrace@{edge params: \xysplineedges@}}%
\xydef@\testsplineedges@#1;#2,#3;#4,#5@@{%
 \DN@{#5}\ifx\next@\empty
 \DNii@{#4}\ifx\nextii@\empty
 \xynoedgespline@{end}\def\splineedges@{#1;#2,\z@;\z@,}\fi
 \DNii@{#2}\ifx\nextii@\empty
 \xynoedgespline@{start}\def\splineedges@{\z@;\z@,\z@;\z@,}\fi
 \fi }
\xydef@\xynoedgespline@#1{\xywarning@{#1 edge of spline not found}}%
\xydef@\splinestartScan@{\bgroup
\splinetrace@{scan for start}%
 \global\let\splineadvance@=\splineadvance@@
 \let\spline@start=\splinefindStart@
 \let\spline@end=\spline@end@@
 \let\splinefinish@=\splinefinish@@
 \let\splinewhich=\relax
 \global\splinelength@=\z@
 \def\splinerec@{\let\splinerec@=\splineSrec@ \splinedecast@@}%
 \edef\splineedges@{}%
 \expandafter\let\xysplineedges@\relax
 \xylowtolerance@ \splined@@ 
 \ifx\splineedges@\empty\expandafter\splineslowScan@\fi
 \ifx\splineedges@\relax\expandafter\splinenostart@\fi
 \egroup }%
\xydef@\splineslowScan@{%
 \let\splineStarttest=\splineSlowStarttest 
 \let\splinescanStarttest=\relax 
 \def\splinerec@{\let\splinerec@=\splineSrec@ \splinedecast@@}%
 \splined@@ }
\xydef@\splineslowEnd@{%
 \global\let\splineEndtest=\splineSlowEndtest 
 \let\splinescanEndtest=\relax 
 \def\splinerec@{\let\splinerec@=\splineErec@ \splinedecast@@}%
 \splined@@ }
\xydef@\splinenostart@{%
 \def\segmentnum@{1}\splinelength@=\z@ \splineval@=\z@
 \xynoedgespline@{start}\splineRecordValue@ }
\xydef@\splineendScan@{\bgroup
 \bgroup
\splinetrace@{scan for end}%
 \global\let\splineadvance@=\splineadvance@@
 \let\spline@start=\splinefindEnd@
 \let\spline@end=\spline@end@@ 
 \let\splinefinish@=\splinefinish@@
 \let\splinewhich=\relax
 \global\splinelength@=\z@ 
 \global\let\splineEndtest=\splineEndtest@ 
 \def\splinerec@{\let\splinerec@=\splineErec@ \splinedecast@@}%
 \expandafter\def\expandafter\prevedges@\expandafter{\splineedges@}%
 \xylowtolerance@ \splined@@ 
 \ifx\splineedges@\prevedges@\expandafter\splineslowScan@\fi
 \egroup \egroup}
\xydef@\splinescanbreak@{%
\splinetrace@{SCANBREAK}%
 \gdef\breakedges@{}%
 \DN@{0}\ifx\next@\bstartPLACE@
 \DN@{\bgroup \def\tmp@####1;####2,####3;####4,{%
 \global\splineval@=####2\relax}%
 \expandafter\expandafter\expandafter\tmp@\xysplineedges@
 \def\segmentnum@{1}\splineRecordBreakValue@ \egroup}%
 \else
 \bgroup \cv@start 
 \expandafter\DN@\expandafter{\the\Edge@c}\DNii@{\zeroEdge}%
 \ifx\next@\nextii@ \aftergroup\splinezerostart
 \else\aftergroup\splinewidestart\fi
 \egroup 
 \fi \next@ 
 \DN@{1}\ifx\next@\bendPLACE@ 
 \DN@{\bgroup \def\tmp@####1;####2,####3;####4,{%
 \global\splineval@=####4\relax}%
 \expandafter\expandafter\expandafter\tmp@\xysplineedges@
%% \multiply\splineval@\m@ne \advance\splineval@\p@
%% \def\segmentnum@{1}
 \getcrvsegsnum@ \edef\segmentnum@{\the\count@}%
 \global\multiply\splineval@\count@ 
 \splineRecordEndBreakValue@ \egroup}%
 \else
 \bgroup \cv@end 
 \expandafter\DN@\expandafter{\the\Edge@c}\DNii@{\zeroEdge}%
 \ifx\next@\nextii@ \aftergroup\splinezeroend
 \else\aftergroup\splinewideend\fi
 \egroup 
 \fi \next@ 
 \expandafter\def\expandafter
 \xybreakedges@\expandafter{\breakedges@}%
 \global\let\breakedges@=\relax
\splinetrace@{break params: \xybreakedges@::\bstartPLACE@--\bendPLACE@}%
 \expandafter\let\xysplineedges@\xybreakedges@ }
\xydef@\getcrvsegsnum@{%
 \count@=\ptsnum@\relax \ifnum\count@>\@ne\advance\count@\m@ne\fi}
\xydef@\splinezerostart{\DN@{\bgroup 
\splinetrace@{splinezerostart:}%
 \dimen@=\bstartPLACE@\p@ 
 \global\splineval@=\dimen@ 
 \splineRecordBreakValue@ \egroup }}
\xydef@\splinezeroend{\DN@{\bgroup 
\splinetrace@{splinezeroend:}%
 \dimen@=\bendPLACE@\p@
 \multiply\dimen@\m@ne \advance\dimen@\p@
 \def\segmentnum@{0}\global\splineval@=\dimen@ 
 \splineRecordEndBreakValue@ \egroup }}
\xydef@\splinewidestart{\DN@{\bgroup 
 \splinetrace@{scan for start}%
 \let\splinefbcontinue@=\breakstartcontinue@
 \let\splinef@pt=\splinef@breakpt
 \let\splinef@end=\break@start
 \edef\tmp@{{\bstartPLACE@}}%
 \expandafter\splinealong@@\tmp@\z@>\endgroup\egroup }}
\xydef@\splinewideend{\DN@{\bgroup 
 \splinetrace@{scan for wide end}%
 \let\splinefbcontinue@=\breakendcontinue@
 \let\splinef@pt=\splinef@breakpt
 \let\splinef@end=\break@end
 \edef\tmp@{{\bendPLACE@}}%
 \expandafter\splinealong@@\tmp@\z@<\endgroup\egroup }}
\xydef@\splineSrec@{{%
\splinetrace@{v=\the\splineval@ + d=\the\splinedepth@ :
 (\the\X@p,\the\Y@p);(\the\X@c,\the\Y@c):Srec }%
 \splineStarttest
 \ifsplineplot@ 
 \ifdim\splinedepth@<.0001\p@ \aftergroup\splinefinish@
 \global\advance\splineval@ .5\splinedepth@
 \else\aftergroup\splinedecast@@ \fi
 \else \aftergroup\splineadvance@ \fi}}
\xydef@\splinefindStart@@{\bgroup \bgroup 
 \expandafter\expandafter\expandafter\getsplineparams@\xysplineparams@
 \global\let\splineadvance@=\splineadvance@@
 \global\let\splinepoint=\relax
 \let\splinegoal@=\splineRecordValue@ \global\dimen5=\z@ 
 {\X@c=\X@p \Y@c=\Y@p \splinescanStarttest }%
} 
\xydef@\splinefindStart@{%
 \expandafter\crv@cnt@\xycrvptsnum@\relax
 \ifnum\crv@cnt@>\tw@
 \crv@cnt@=\@ne \splineplot@false \splinesegment@{\crv@cnt@}%
 {\splineStarttest
 \ifsplineplot@\aftergroup\splineplot@true\fi}%
 \ifsplineplot@ \else \searchforStartsegment@ \fi 
 \splinesegment@{\crv@cnt@}%
\splinetrace@{start is in segment \segmentnum@}%
 \else \splinesegment@\@ne \fi
 \splineplot@false \splinefindStart@@
}
\xydef@\searchforStartsegment@{\splineplot@true\loop@ 
 \advance\crv@cnt@\@ne 
 \expandafter\count@\xycrvptsnum@\relax
 \ifnum\count@=\crv@cnt@\expandafter\splineplot@false
 \else 
 \splinesegment@{\crv@cnt@}{\splineStarttest
 \ifsplineplot@\aftergroup\splineplot@false
 \else\aftergroup\splineplot@true\fi }%
 \fi \ifsplineplot@\repeat@ 
}
\xydef@\splinefindEnd@@{\bgroup \bgroup
 \expandafter\expandafter\expandafter\getsplineparams@\xysplineparams@
\splinetrace@{params:\xysplineparams@}%
 \splinereverse@@
\splinetrace@{params:\xysplineparams@}%
 \global\let\splineadvance@=\splineadvance@@
 \global\let\splinepoint=\splinescanEndtest 
 \let\splinegoal@=\splineRecordEndValue@ \global\dimen5=\z@ 
 {\X@c=\X@p \Y@c=\Y@p \splinescanEndtest }%
}
\xydef@\splinereverse@@{\splinereverse@@@}
\xydef@\splinereverse@@@{%
 \def\postspline@{\d@X=-\d@X \d@Y=-\d@Y}%
 \dimen@ii=\X@c \X@c=\X@p \X@p=\dimen@ii 
 \dimen@ii=\Y@c \Y@c=\Y@p \Y@p=\dimen@ii 
 \global\dimen5=-\dimen5\relax 
 \global\advance\dimen5\splinelength@ }
\xydef@\postspline@{}
\xydef@\splineErec@{{%
 \dimen@=\splineval@ \advance\dimen@\splinedepth@
\splinetrace@{ER (\the\X@p,\the\Y@p);(\the\X@c,\the\Y@c);;;
\the\dimen@,\the\splinedepth@}%
 \splineEndtest
 \ifsplineplot@ 
 \ifdim\splinedepth@<.0001\p@ \aftergroup\splinefinish@
 \else\aftergroup\splinedecast@@ \fi
 \else \aftergroup\splineadvance@ \fi}}
\xydef@\splinefindEnd@{%
 \expandafter\crv@cnt@\xycrvptsnum@\relax 
 \ifnum\crv@cnt@>\tw@
 \advance\crv@cnt@\m@ne 
 \splineplot@false \splinesegment@{\crv@cnt@}%
 {\X@c=\X@p \Y@c=\Y@p \splineEndtest
 \ifsplineplot@\aftergroup\splineplot@true\fi }%
 \ifsplineplot@ 
 \else \searchforEndsegment@ \fi 
 \splinesegment@{\crv@cnt@}%
\splinetrace@{end is in segment: \segmentnum@ }%
 \else \splinesegment@\@ne \fi
 \splineplot@false\splinefindEnd@@
}
\xydef@\searchforEndsegment@{\splineplot@true\loop@ 
 \advance\crv@cnt@\m@ne 
 \ifnum\crv@cnt@=\z@\expandafter\splineplot@false
 \else 
 \splinesegment@{\crv@cnt@}{\X@c=\X@p \Y@c=\Y@p \splineEndtest
 \ifsplineplot@\aftergroup\splineplot@false
 \else\aftergroup\splineplot@true\fi}%
 \fi \ifsplineplot@\repeat@ 
}
\xydef@\splinescanStarttest{%
\splinetrace@{SST (\the\X@c,\the\Y@c); \the\splinelength@, \the\splineval@}%
 {\splineplot@false\splineStarttest
 \ifsplineplot@\expandafter\splinefinish@\fi}}
\xydef@\splinescanEndtest{%
\splinetrace@{SET (\the\X@c,\the\Y@c); \the\splinelength@, \the\splineval@}%
 {\splineplot@false\splineEndtest 
 \ifsplineplot@\expandafter\splinefinish@\fi}}
\xydef@\splineBrec@{{%
 \dimen@=\splineval@ \advance\dimen@\splinedepth@
\splinetrace@{BR (\the\X@p,\the\Y@p);(\the\X@c,\the\Y@c);;;
\the\dimen@,\the\splinedepth@}%
 \splineEndtest
 \ifsplineplot@ \aftergroup\splineadvance@ \else
 \ifdim\splinedepth@<.0001\p@ \aftergroup\splinefinish@
 \else\aftergroup\splinedecast@@ \fi \fi}}
\xydef@\splineBSrec@{{%
\splinetrace@{SR (\the\X@p,\the\Y@p);(\the\X@c,\the\Y@c);;;
\the\dimen@,\the\splinedepth@:SR}%
 \splineStarttest
 \ifsplineplot@ 
 \ifdim\splinedepth@<.0001\p@ \aftergroup\splinefinish@
 \global\advance\splineval@ .5\splinedepth@
 \else \advance\splineval@\splinedepth@
 \splinetest@ \advance\splineval@-\splinedepth@
 \ifsplineplot@\aftergroup\splineadvance@
 \else\aftergroup\splinedecast@@\fi
 \fi
 \else
 \global\advance\splineval@\splinedepth@
 \aftergroup\splinefinish@ \fi }}
\xydef@\splineBErec@{{%
 \dimen@=\splineval@ \advance\dimen@\splinedepth@
\splinetrace@{BE (\the\X@p,\the\Y@p);(\the\X@c,\the\Y@c);;;
 \the\dimen@,\the\splinedepth@}%
 \splineEndtest
 \ifsplineplot@ 
 \ifdim\splinedepth@<.0001\p@ \aftergroup\splinefinish@
 \global\advance\splineval@ .5\splinedepth@
 \else \advance\splineval@\splinedepth@
 \splinetest@ \advance\splineval@-\splinedepth@
 \ifsplineplot@\aftergroup\splineadvance@
 \else\aftergroup\splinedecast@@\fi
 \fi
 \else
 \ifdim\splinedepth@<\p@ \global\advance\splineval@\splinedepth@ \fi
 \aftergroup\splinefinish@ \fi }}
\xydef@\splinef@breakpt#1{%
 \ifdim\splineval@>\z@
\splinetrace@{found: val=\the\splineval@;(\the\X@c,\the\Y@c)}%
 \else
\splinetrace@{found: val=\the\splineval@;(\the\X@p,\the\Y@p)}%
 \fi \splinefbcontinue@ }
\xydef@\splinef@pt@@{%
 \ifdim\splineval@>\z@ 
\splinetrace@{found: val=\the\splineval@;c:(\the\X@c,\the\Y@c)}%
 \global\dimen@i=\X@c \global\dimen3=\Y@c 
 \else
\splinetrace@{found: val=\the\splineval@;p:(\the\X@p,\the\Y@p)}%
 \fi
 \setsplinedir@ \global\dimen5=\d@X \global\dimen7=\d@Y 
 \global\splineval@=\splineval@
 \aftergroup\splinefocus@ }
\xydef@\findbreakwarning@#1{%
 \xywarning@{#1 of break not found: bSTART=\bstartPLACE@, bEND=\bendPLACE@}%
 \DN@{#1}\def\DNii@{start}\ifx\next@\nextii@\splineRecordBreakValue@
 \else\splineRecordEndBreakValue@\fi\egroup}%
\xydef@\breakstartcontinue@{\bgroup \cv@start
 \expandafter\DN@\expandafter{\the\Edge@c}\DNii@{\zeroEdge}%
 \ifx\next@\nextii@ \aftergroup\breakstartfound@
 \else \aftergroup\breakstartcontinue@i\fi \egroup }%
\xydef@\breakstartcontinue@i{%
\splinetrace@{move to start edge, from (\the\X@c,\the\Y@c): val=\the\splineval@ }%
 \global\let\splineEndtest=\splineBreakStarttest@
 \global\let\splinetest@=\splineBreakStarttest@
 \gdef\splinerec@{\global\let\splinerec@=\splineSrec@ \splinedecast@@}%
 \global\let\splinepoint=\relax
 \global\let\spline@end=\checkfoundSbreak@ 
 \global\let\splinegoal@=\splineRecordSBreakValue@ 
 \global\let\splinefinish@=\splinefinish@@ }
\xydef@\breakstartfound@{%
\splinetrace@{found start edge, at (\the\X@c,\the\Y@c): val=\the\splineval@ }%
 \global\let\splinetest@=\splineStarttest
 \gdef\splinerec@{\splinegoal@ \global\let\splinerec@=\splinefinish@ }%
 \global\let\splinepoint=\relax
 \global\let\spline@end=\relax
 \global\let\splinegoal@=\splineRecordBreakValue@ 
 \global\let\splinefinish@=\splinefinish@@
 }
\xydef@\checkfoundSbreak@{%
 \ifnum\xycrvptsnum@<\thr@@\DN@{\findbreakwarning@{start}}%
 \else\DN@{\searchBreakSsegment@}\fi \next@ }%
\xydef@\searchBreakSsegment@{%
 \crv@cnt@=\segmentnum@ \DN@{}\count@=\crv@cnt@
 \DNii@{}\ifnum\splineval@=\z@ \ifnum\crv@cnt@=\@ne
 \ifnum\xycrvptsnum@=\@ne\count@=\z@\DNii@{\egroup}\fi
 \else \DN@{\egroup}\fi 
 \else \ifnum\splineval@=\m@ne 
 \else \advance\crv@cnt@\@ne \fi \fi
 \ifnum\crv@cnt@=\xycrvptsnum@\relax
 \ifnum\xycrvptsnum@>\tw@ \DNii@{\egroup}\fi
 \DN@{\expandafter\splineRecordBreakValue@\nextii@}%
 \else
 \DN@{\splinesegment@{\crv@cnt@}\splinesetparams@
 \splined@@ \egroup}%
 \fi \next@ }
\xydef@\checkfoundEbreak@{%
 \ifnum\xycrvptsnum@<\thr@@\DN@{\findbreakwarning@{end}}%
 \else\DN@{\searchBreakEsegment@}\fi \next@ }%
\xydef@\searchBreakEsegment@{%
 \crv@cnt@=\segmentnum@ \DN@{}\count@=\crv@cnt@
 \DNii@{}\ifnum\splineval@=\z@ \ifnum\crv@cnt@=\@ne
 \ifnum\xycrvptsnum@=\@ne\count@=\z@\DNii@{\egroup}\fi
 \else\DN@{\egroup}\fi
 \else \advance\crv@cnt@\m@ne \fi 
 \ifnum\count@=\z@
 \ifnum\xycrvptsnum@>\tw@ \splineval@=\m@ne\p@
 \DNii@{\egroup}\fi
 \DN@{\expandafter\splineRecordEndBreakValue@\nextii@}\else
 \DN@{\splinesegment@{\crv@cnt@}\splinereverse@
 \readsplineparams@ \splined@@ \egroup}%
 \fi \next@ }
\xydef@\break@start{\egroup \egroup 
\splinetrace@{scan for start}%
 \global\let\splineadvance@=\splineadvance@@
 \let\spline@start=\splinefindBStart@
 \let\spline@end=\egroup
 \let\splinefinish@=\splinefinish@@
 \let\splinewhich=\relax
 \global\let\splineadvance@=\splineadvance@@
 \global\let\splinepoint=\relax
 \let\splinegoal@=\splineRecordBreakValue@
 \global\dimen5=\z@ \global\splinelength@=\z@
 \let\splinerec@=\splineSrec@ 
 \def\breakedges@{}%
 \bgroup \bgroup \splined@@ }
\xydef@\splinefindBStart@{\bgroup
 \global\splineval@=\z@ \splinedepth@=.5\p@}
\xydef@\breakendcontinue@{\bgroup
 \edef\tmp@{\X@p = \the\X@c \Y@p=\the\Y@c}\cv@end\tmp@
 \expandafter\DN@\expandafter{\the\Edge@c}\DNii@{\zeroEdge}%
 \ifx\next@\nextii@ \aftergroup\breakendfound@
 \else\aftergroup\breakendcontinue@i\fi \egroup }%
\xydef@\breakendcontinue@i{%
\splinetrace@{move to end edge, from (\the\X@c,\the\Y@c): val=\the\splineval@ }%
 \global\let\splineEndtest=\splineBreakEndtest@
 \global\let\splinetest@=\splineBreakEndtest@
 \gdef\splinerec@{\global\let\splinerec@=\splineErec@\splinedecast@@}%
 \global\let\splinepoint=\relax
 \global\let\spline@end=\checkfoundEbreak@ 
 \global\let\splinegoal@=\splineRecordEBreakValue@ 
 \global\let\splinefinish@=\splinefinish@@ 
 \splinerec@ }
\xydef@\splineRecordEBreakValue@{%
\splinetrace@{\the\count@\space segments, \the\splineval@}%
 \splineRecordEndBreakValue@ }
\xydef@\splineRecordSBreakValue@{\getcrvsegsnum@
 \dimen@=\splineval@ 
 \advance\dimen@\segmentnum@\p@ \advance\dimen@-\p@
 \dimen@nth\count@\dimen@
 \global\splineval@=\dimen@ \def\segmentnum@{1}%
 \splineRecordBreakValue@ }
\xydef@\breakendfound@{%
\splinetrace@{found end edge, at (\the\X@c,\the\Y@c): val=\the\splineval@ }%
 \global\let\splinetest@=\splineEndtest
 \gdef\splinerec@{\splinegoal@ \global\let\splinerec@=\splinefinish@}%
 \global\let\splinepoint=\relax
 \global\let\spline@end=\relax
 \global\let\splinegoal@=\splineRecordEndBreakValue@ 
 \global\let\splinefinish@=\splinefinish@@ }
\xydef@\break@end{\egroup \egroup
 \global\let\splineadvance@=\splineadvance@@
 \let\spline@start=\splinefindBEnd@
 \let\spline@end=\egroup 
 \let\splinefinish@=\splinefinish@@
 \let\splinewhich=\relax
 \global\let\splineadvance@=\splineadvance@@
 \global\let\splinegoal@=\splineRecordEndBreakValue@
 \global\splinelength@=\z@ 
 \let\splinerec@=\splineErec@ 
 \global\let\splineEndtest=\splineEndtest@ 
 \bgroup \splined@@ }
\xydef@\splinefindBEnd@{\bgroup\bgroup 
 \splinereverse@ \readsplineparams@ 
 \global\splineval@=\z@ }
\xydef@\splineRecordValue@{%
 \ifx\unknown\segmentnum@\relax
 \else
 \getcrvsegsnum@ 
 \dimen@=\splineval@ \advance\dimen@ \segmentnum@\p@
 \advance\dimen@-\p@ \dimen@nth\count@\dimen@
 \global\splineval@=\dimen@
 \fi
 \xdef\splineedges@{\splineedges@\the\splinelength@;\the\splineval@,}%
\splinetrace@{found edge: \splineedges@}}
\xydef@\splineRecordEndValue@{%
 \ifx\unknown\segmentnum@\relax
 \else
 \getcrvsegsnum@
 \dimen@=\splineval@ \advance\dimen@ \count@\p@
 \advance\dimen@-\segmentnum@\p@ \dimen@nth\count@\dimen@
 \global\splineval@=\dimen@
 \fi
 \xdef\splineedges@{\splineedges@\the\splinelength@;\the\splineval@,}%
\splinetrace@{found edge: \splineedges@}}
\xydef@\splineRecordBreakValue@{%
 \ifx\unknown\segmentnum@\relax
 \else\expandafter\advance\expandafter\splineval@\segmentnum@\p@
 \count@=\segmentnum@\relax 
 \ifnum\count@>0 \advance\splineval@-\p@ \fi\fi
 \xdef\breakedges@{\breakedges@\the\splinelength@;\the\splineval@,}%
 \global\let\spline@end=\egroup
\splinetrace@{found break edge: \breakedges@}}
\xydef@\splineRecordEndBreakValue@{%
 \ifx\unknown\segmentnum@\relax 
 \else\count@=\segmentnum@\relax \ifnum\count@=\z@
 \else \getcrvsegsnum@ 
 \count@@=\count@ \advance\count@@-\segmentnum@\relax
 \dimen@=\splineval@ \advance\dimen@ \count@@\p@
 \dimen@nth\count@\dimen@
 \global\splineval@=\dimen@
 \fi\fi
 \ifdim\splineval@<\z@ \relax\splineval@=\z@ \fi
 \ifx\breakedges@\relax\relax\else\ifx\breakedges@\empty\else
 \ifdim\splineval@<\p@\relax \ifdim\splineval@>\z@ 
 \expandafter\testbreakedges@\breakedges@ @%
 \fi\fi\fi\fi
 \xdef\breakedges@{\breakedges@\the\splinelength@;\the\splineval@,}%
 \global\let\spline@end=\egroup
\splinetrace@{found break edge: \breakedges@}}
\xydef@\testbreakedges@#1;#2,#3@{\bgroup \dimen@=#2\relax
 \advance\dimen@\splineval@ \advance\dimen@-\p@
\splinetrace@{testbreak: #1;#2,#3@ \the\splineval@::\the\dimen@}%
 \DN@{\egroup}\ifdim\dimen@>\z@
 \edef\next@{\egroup\def\noexpand\breakedges@{#1;1pt,#3}}%
 \else\ifdim\zz@\dimen@ 
 \edef\next@{\egroup\def\noexpand\breakedges@{#1;1pt,#3}}%
 \fi \fi \next@ }
\xydef@\splineRecordBreakEValue{%
 \ifdim\splineval@>\z@
 \splineval@=-\splineval@ \advance\splineval@\p@ \fi
 \splineRecordBreakValue@ }%
\xydef@\xydist@#1#2{\ifdim#1>#2\relax
 \quotient@@\tmp@#2#1\expandafter\dimen@ii\tmp@#2\relax
 \ifdim\dimen@ii>.41422#1\relax
 \dimen@=1.060665#1\advance\dimen@ .353555\dimen@ii\relax
 \else \dimen@=#1\advance\dimen@.5\dimen@ii\fi
 \else 
 \quotient@@\tmp@#1#2\expandafter\dimen@ii\tmp@#1\relax
 \ifdim\dimen@ii>.41422#2\relax
 \dimen@=1.060665#2\advance\dimen@ .353555\dimen@ii\relax
 \else \dimen@=#2\advance\dimen@.5\dimen@ii\fi
 \fi}
\xydef@\splineDadvance@{\splineadvance@@
 \expandafter\splineDadvance@@\splineDadvance@@@}
\xydef@\splineDadvance@@#1#2#3#4{%
 {\d@X=#1\advance\d@X-#2\ifdim\d@X<\z@ \d@X=-\d@X\fi 
 \d@Y=#3\advance\d@Y-#4\ifdim\d@Y<\z@ \d@Y=-\d@Y\fi
 \xydist@\d@X\d@Y 
 \global\advance\splinelength@\dimen@ 
\splinetrace@{d=(\the\d@X,\the\d@Y): v=\the\splineval@: l=\the\splinelength@}%
}}
\xydef@\spline@end@{\lastsplinepoint@ \egroup \egroup
 \ht\z@=\z@ \dp\z@=\z@ \wdz@=\z@ \boxz@}%
\gdef\splinetest@{\splineplot@true}
\xydef@\spline@end@@{\egroup \egroup}
\xydef@\splinefrec@{{%
 \advance\splineval@\splinedepth@
\splinetrace@{F:(\the\X@p,\the\Y@p);(\the\X@c,\the\Y@c);;
\the\splineval@;\the\splinedepth@}%
 \ifdim\dimen5=\splineval@ \aftergroup\splinefinishf@ 
 \else \dimen@=\dimen5\advance\dimen@-\splineval@
 \ifdim\dimen@<\z@ \dimen@=-\dimen@ \fi
 \ifdim\dimen@<.0001\p@ \aftergroup\splinefinishf@
 \else
 \ifdim\dimen5<\splineval@\aftergroup\splinedecast@@
 \else \aftergroup\splineadvance@ 
 \fi\fi\fi}}
\xydef@\splinefinishf@{\global\advance\splineval@\splinedepth@
 \splinefinish@}%
\xydef@\spline@find#1#2#3{%
\splinetrace@{spline@find #1 #2 #3}%
 \readsplineparams@
 \global\let\splinefinish@=\splinefinish@@
 \global\let\splinegoal@=\splinef@pt 
 \global\let\splinepoint=\relax
 \dimen@=#1\relax\dimen@ii=#2\relax
 \ifdim\dimen@ii=\z@ \def\postfind@{}%
 \else\def\postfind@{}%
 \ifdim\dimen@ii<\z@ \splinereverse@ 
 \readsplineparams@ 
\splinetrace@{reverse orientation: (\the\X@p,\the\Y@p),(\the\X@c,\the\Y@c)}%
 \dimen@=#1\relax\dimen@ii=#2\relax
 \multiply\dimen@\m@ne \advance\dimen@\p@ \multiply\dimen@ii\m@ne
 \def\postfind@{\d@X=-\the\d@X \d@Y=-\the\d@Y \noexpand\reversesplineval@}%
 \fi\fi
 \expandafter\splinetrace@\expandafter{\xysplineparams@}%
 \edef\next@{\noexpand\spline@@find{\the\dimen@}{\the\dimen@ii}{#3}}%
 \next@ }
\xydef@\reversesplineval@{\splineval@=-\splineval@ \advance\splineval@\p@ }
\xydef@\spline@@find#1#2#3{%
\splinetrace@{spline@@find #1 #2 #3}%
 \let\splinerec@=\splinefrec@ 
 \global\let\splineadvance@=\splineadvance@@
 \dimen5=#1\relax
 \ifdim #2=\z@\relax
 \ifdim #1=\z@\relax \bgroup 
 \let\splined@@=\spline@@knot
 \global\splineval@=\m@ne\p@ 
 \else\ifdim #1=\p@\relax \bgroup
 \let\splined@@=\spline@@knot 
 \global\splineval@=\z@ 
 \else 
 \global\splineval@=\z@ 
 \global\let\splineadvance@=\splineadvance@@
 \DN@{#3}\ifx\next@\empty \setsplinetest@\splineval@>{#1}{}%
 {{\ifdim\splineval@=\dimen5\aftergroup\splineplot@false\fi}}%
 \else\DNii@{>}\ifx\next@\nextii@
 \setsplineundertest@\splineval@>{#1}{}{}%
 \let\splinerec@=\splineBSrec@ 
 \else\DNii@{<}\ifx\next@\nextii@
 \setsplineundertest@\splineval@>{#1}{}{}%
 \let\splinerec@=\splineBErec@ 
 \else\xywarning@{unknown find-mode: #3}\fi\fi\fi
 \fi\fi
 \else 
 \global\splineval@=\z@ 
 \def\splineslidetest@@{%
 \setsplinetest@\splinelength@<{#2}{}{}}%
 \let\splinefinish@=\splinefcontinue@
 \fi
 \let\spline@end=\splinef@end
 \let\splinepoint@=\relax
 \splinelength@=\z@ 
 \def\spline@start{\bgroup\xylowtolerance@}%
 \splined@@ }
\xydef@\spline@@knot{%
 \let\setsplinedir@=\setsplineknotdir@
 \splinesetparams@\spline@start
 \splinedepth@=\p@
 \global\dimen@i=\X@p \global\dimen3=\Y@p 
 \splinefinishf@ \spline@end \egroup }
\xydef@\splinefcontinue@{%
\splinetrace@{sliding... from (\the\X@c,\the\Y@c): val=\the\splineval@ }%
 \global\let\splinerec@=\splinerec@@
 \global\splinelength@=\z@
 \global\splineval@=\splineval@
 \global\let\splinepoint=\splinefindtest@
 \global\let\splinegoal@=\splinef@pt 
 \global\let\splineadvance@=\splineDadvance@
 \global\let\splinefinish@=\splinefinish@@ 
 \splineslidetest@@ 
 }
\xydef@\splinefindtest@{%
\splinetrace@{SFT (\the\X@c,\the\Y@c); \the\splinelength@, \the\splineval@}%
 {\splineplot@false\splinetest@ 
 \ifsplineplot@\expandafter\splinefinishf@\fi}}
\def\setsplineundertest@#1#2#3#4#5{%
\splinetrace@{setsplineundertest@: #1,#2,#3,#4,#5,}%
 \DNii@{\gdef\splinetest@}%
 \DN@##1\next{\def\tmp@{{\splineplot@false 
 \ifdim#1#2##1\relax #4\else\splineplot@true#5\fi }}}%
 \next@#3\relax\next
 \expandafter\nextii@\tmp@ }
\xydef@\splinef@end{\edef\tmp@{\egroup\splinelength@=\the\splinelength@}\tmp@}
\xydef@\splinef@pt{%
 \ifdim\splineval@>\z@ 
\splinetrace@{found: val=\the\splineval@;c:(\the\X@c,\the\Y@c)}%
 \global\dimen@i=\X@c \global\dimen3=\Y@c 
 \else
\splinetrace@{found: val=\the\splineval@;p:(\the\X@p,\the\Y@p)}%
 \fi
 \setsplinedir@ \global\dimen5=\d@X \global\dimen7=\d@Y 
 \global\splineval@=\splineval@
 \aftergroup\splinefocus@ }
\def\setsplinetest@#1#2#3#4#5{%
 \DNii@{\gdef\splinetest@}%
 \DN@##1\next{\def\tmp@{{\splineplot@false \ifdim#1#2##1\relax
 #4\else\splineplot@true#5\fi}}}%
 \next@#3\relax\next
 \expandafter\nextii@\tmp@ }%
\xydef@\splinefocus@{%
 \d@X=\dimen5\relax \d@Y=\dimen7\relax \setsplinedir@ }
\xydef@\splinesegment@#1{}
\xydef@\xyprecurve@{}
\xydef@\xypostcurve@{}
\xydef@\splineset@{%
\splinetrace@{splineset@:}%
 \ifx\bstartPLACE@\empty
 \DN@{\xyprecurve@ 
 \edef\tmp@{\egroup \X@max=\the\X@max \X@min=\the\X@min
 \Y@max=\the\Y@max \Y@min=\the\Y@min}\tmp@ \xypostcurve@ }%
 \else
 \DN@{\xyprecurve@ \xysplinespecialcases@
 \edef\tmp@{\egroup \X@max=\the\X@max \X@min=\the\X@min
 \Y@max=\the\Y@max \Y@min=\the\Y@min}\tmp@ \xypostcurve@ }%
 \fi
 \next@ }
\xydef@\xysplinespecialcases@{%
 \ifx\empty\xycrvdrop@ 
 \ifx\empty\xycrvconn@ \DN@{\splinesolid@}%
 \else \DN@{ \dir{-}}\ifx\next@\xycrvconn@ \DN@{\splinesolid@}%
 \else \DN@{ \dir 2{-}}\ifx\next@\xycrvconn@ \DN@{\splinedoubled@}%
 \else \DN@{ \dir{=}}\ifx\next@\xycrvconn@ \DN@{\splineribboned@}%
 \else \DN@{ \dir {2.}}\ifx\next@\xycrvconn@ \DN@{\splinedoubled@}%
 \else \DN@{ \dir 3{-}}\ifx\next@\xycrvconn@ \DN@{\splinetrebled@}%
 \else \DN@{ \dir {3.}}\ifx\next@\xycrvconn@ \DN@{\splinetrebled@}%
 \else \DN@{ \dir{--}}\ifx\next@\xycrvconn@ \DN@{\splinedashed@}%
 \else \DN@{ \dir{.}}\ifx\next@\xycrvconn@ \DN@{\splinedotted@}%
 \else \DN@{ \dir{:}}\ifx\next@\xycrvconn@ \DN@{\splinedbldotted@}%
 \else \ifdim\splinetol@>\z@ \else \splinedefaulttol@ \fi
 \DN@{\splineset@@}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi
 \else
 \DN@{\splineset@@}%
 \fi \ifInvisible@\DN@{}\fi \next@ }
\xydef@\splinesolid@{\setbox\splinebox@=\zerodot \def\xycrvdrop@{ }%
 \def\xycrvconn@{}\splineset@@}
\xydef@\splinedoubled@{\splinedefaulttol@\def\xycrvdrop@{ }\def\splinedrop@{}%
 \def\xycrvconn@{!C\dir2{.}}\splineset@@}
\xydef@\splineribboned@{\splinedefaulttol@\def\xycrvdrop@{ }\def\splinedrop@{}%
 \def\xycrvconn@{!C\dir{:}}\splineset@@}
\xydef@\splinetrebled@{\splinedefaulttol@\def\xycrvdrop@{ }\def\splinedrop@{}%
 \def\xycrvconn@{!C\dir3{.}}\splineset@@}
\xydef@\splinedashed@{\splinetol@=1.5pc \def\xycrvdrop@{ }%
 \def\splinedrop@{}\edef\xycrvconn@{\noexpand!C\noexpand\dir{\addDASH@{}}}%
 \splineset@@}
\xydef@\splinedotted@{\setbox\splinebox@=\zerodot \def\xycrvdrop@{ }%
 \splinetol@=1.5\jot \def\xycrvconn@{}\splineset@@}
\xydef@\splinedbldotted@{\def\xycrvdrop@{ }\def\splinedrop@{}%
 \splinetol@=1.5\jot \def\xycrvconn@{!C\dir{:}}\splineset@@}
\xydef@\splineset@@{%
 \readsplineparams@
 \ifx\xycrvdrop@\empty \splinetol@=7.5\p@
 \def\splinedefaulttol@{\splinetol@=7.5\p@}\def\splinedrop@{}%
 \else\edef\splinedefaulttol@{\splinetol@=\the\splinetol@}\fi
 \ifx\xycrvconn@\empty \def\splineconn@{}\fi
\splinetrace@{set the curve: >\the\dimen5, <\the\dimen7}%
 \global\let\splineadvance@=\splineadvance@@
 \let\splinerec@=\splineTrec@
 \def\splineStarttest{\splinetest@}%
 \global\let\splinepoint=\relax
 \let\spline@start=\spline@start@
 \let\spline@end=\spline@end@
 \ifdim\dimen7=\p@ 
 \gdef\splinecontinue{\splinesetting@
 \global\let\splinetest@=\splineplot@true}%
 \else
 \ifdim\dimen7=\tw@\p@
%% \ifdim\bendPLACE@\p@=\z@ \emptyspline@ \else
 \ifdim\bendPLACE@\p@=\p@
 \fi
 \else
 \xdef\splinecontinue{\noexpand\setsplinetest@
 \splineval@>{\the\dimen7}{\noexpand\splinebreakcancel@}{}%
 \noexpand\splinesetting@ }%
 \fi\fi
 \ifdim\dimen7>\z@ \DN@{\splinesetting@\splinecontinue}%
 \ifdim\zz@{\dimen5}%
 \else 
 \edef\next@{\noexpand\setsplinetest@
 \splineval@<{\the\dimen5}{}%
 {\noexpand\expandafter\noexpand\splinecontinue}%
 \noexpand\splinesetting@ }%
 \fi
 \else\DN@{\dimen5=\p@}\fi
 \next@
 \ifdim\dimen5=\p@\DN@{}\else\DN@{\splined@@}\fi \next@ 
 }
\xydef@\emptyspline@{\xywarning@{empty curve subsegment}%
\splinetrace@{bstartPLACE@=\bstartPLACE@, bendPLACE@=\bendPLACE@, 
 empty segment}%
 \gdef\splinecontinue{\splinesetting@
 \global\let\splinetest@=\splineplot@false
 \global\dimen5=\z@ }}
\xydef@\splineTrec@{{%
 \advance\splineval@\splinedepth@
 \ifdim\dimen5=\splineval@
 \aftergroup\splinecontinue
 \else \dimen@=\dimen5\advance\dimen@-\splineval@
 \ifdim\dimen@<\z@ \dimen@=-\dimen@ \fi
 \ifdim\dimen@<.001\p@
 \aftergroup\splinecontinue
 \else
 \ifdim\dimen5<\splineval@\aftergroup\splinedecast@@
 \else \aftergroup\splineadvance@
 \fi\fi\fi}}
\xydef@\splinesetting@{\splinesetting@@}
\xydef@\splinesetting@@{%
\splinetrace@{splinesetting@@:}%
 \ifdim\splinedepth@=\z@ \splinedepth@=\p@ \fi
 \ifdim\splinedepth@=\p@
 \def\splinerec@{\global\let\splinerec@=\splinerec@@\splinedecast@@}%
 \else \global\let\splinerec@=\splinerec@@ \fi
 \gdef\splinepoint{\splineplotpt@}}
\xydef@\splineplotpt@{{\global\advance\dimen@i-\X@c 
 \splinetest@ \DN@{\splineglue@}\ifsplineplot@ 
 \DN@{\dosplineplotpt@}%
 \fi \next@ \global\dimen@i=\X@c \global\dimen3=\Y@c }}
\xydef@\splineglue@{\hglue-\dimen@i
\splinetrace@{N:(\the\X@c,\the\Y@c);;\the\dimen@i;\the\dimen3%
 ,\the\splinelength@,\the\splineval@,\the\splinedepth@}}
\xydef@\dosplineplotpt@{\ifdim\dimen@i<\z@
 \raise\Y@c\hbox to-\dimen@i{\hfill\splinedrop@}%
 \else \kern-\dimen@i\raise\Y@c\hbox{\splinedrop@}\fi
 \ifx\splineconn@\relax\else\raise\Y@c\hbox{%
 \setboxz@h{\splineconn@}\Drop@@}\fi
\splinetrace@{P:(\the\X@c,\the\Y@c);;\the\dimen@i;\the\dimen3
 ,\the\splinelength@,\the\splineval@,\the\splinedepth@}}
\xydef@\splinefinish@@{\postspline@ \splinegoal@ \splinecancel@ }
\xydef@\splinecancel@{%
 \global\let\splinerec@=\relax
 \global\let\splinepoint=\relax 
 \global\let\splinecontinue=\relax
 \global\let\splinedecast@=\relax
 }
\xydef@\splinebreakcancel@{\bsplinecancel@ \splinecancel@}
\xydef@\bsplinecancel@{\gdef\lastbspline@{\leave@\leave@}%
 \global\let\middlebspline@=\lastbspline@ }
\xydef@\splinegoal@{\ifdim\splineval@>\z@
 \global\dimen@i=\X@c \global\dimen3=\Y@c \fi
 \global\splineval@=\splineval@ \global\splinelength@=\splinelength@
 \splinesetdir@ }
\xylet@\splinefinish@\splinefinish@@
\xylet@\splinewhich\splineDwhich@
\xydef@\squinewhich@{%
 \ifdim\dimen5>\squinelength
 \d@X=\X@c \d@Y=\Y@c \advance\d@X-\L@c \advance\d@Y-\U@c 
 \advance\squineval-\squinedepth 
 \else \X@c=\X@p \Y@c=\Y@p \advance\squineval-\squinedepth
 \d@X=\L@c \d@Y=\U@c \advance\d@X-\X@p \advance\d@Y-\Y@p \fi
 \d@X=-\d@X \d@Y=-\d@Y
 \squinefinish}
\xydef@\squineDwhich@{%
 \ifdim\dimen5>\squinelength
 \d@X=\X@c \d@Y=\Y@c \advance\d@X-\L@c \advance\d@Y-\U@c 
 \else \X@c=\X@p \Y@c=\Y@p \advance\squineval-\squinedepth
 \d@X=\L@c \d@Y=\U@c \advance\d@X-\X@p \advance\d@Y-\Y@p \fi
 \d@X=-\d@X \d@Y=-\d@Y
 \squinefinish}
\xydef@\xyquadbezier@{%
 \global\let\splinerec@=\relax
 \addtocrvpts@{\def\crvconnect@{\squineconnect@}}%
 \xyquadmethods@ \let\splinesegment@=\squinesegment@
 \begingroup\setcrvobjects@ \xysplineparams@ \splined@@@
 \bgroup \setupsquine@ \squined@ \splineset@ \savespline@ }
\xydef@\xyquadmethods@{%
 \def\crvconnect@{\squineconnect@}%
 \def\splinereverse@@{\splinereverse@@@}%
 \let\getsplineparams@=\getsquineparams@
 \let\spline@start@=\squine@start@
 \let\splinedecast@@=\squinedecast@
 \let\splinerec@@=\squinerec@
 \let\splined@@=\squined@@
 \let\splineIpt@@=\squineIpt@
 \let\splineIadvance@@=\squineIadvance@
 \let\splineinfo@=\squineinfo@
 \let\setsplinedir@=\setsquinedir@
 \let\splinetestcvxhull@=\squinetestcvxhull@
 \let\setsplineknotdir@=\setsquineknotdir@
 \let\splinereverse@=\squinereverse@
 \let\splineDadvance@@@=\squineDadvance@@@
 \let\splinesetparams@=\squinesetparams@
 \let\splineplot@maybe@@=\squineplot@maybe
}
\xydef@\squineconnect@{\splineconnect@ \crvconnect@@ 
 \let\splinesegment@=\squinesegment@ }%
\xydef@\squinesegment@#1{\xyquadmethods@ \def\segmentnum@{1}%
 \setupsquine@ \squined@ }
\xydef@\setupsquine@{%
 \xycontrolpt@\z@ \X@p=\X@c \Y@p=\Y@c
 \xycontrolpt@\@ne \A@=\X@c \B@=\Y@c 
 \xycontrolpt@\tw@ 
 \ifdim \A@>\X@max
 \dimen@=\X@p\advance\dimen@\A@ \dimen@half
 \ifdim \dimen@>\X@max \X@max=\dimen@ \fi
 \dimen@=\X@c\advance\dimen@\A@ \dimen@half
 \ifdim \dimen@>\X@max \X@max=\dimen@ \fi
 \else \ifdim \A@<\X@min 
 \dimen@=\X@p\advance\dimen@\A@ \dimen@half
 \ifdim \dimen@<\X@min \X@min=\dimen@ \fi
 \dimen@=\X@c\advance\dimen@\A@ \dimen@half
 \ifdim \dimen@>\X@min \X@min=\dimen@ \fi
 \fi\fi
 \ifdim \B@>\Y@max 
 \dimen@=\Y@p\advance\dimen@\B@ \dimen@half
 \ifdim \dimen@>\Y@max \Y@max=\dimen@ \fi
 \dimen@=\Y@c\advance\dimen@\B@ \dimen@half
 \ifdim \dimen@>\Y@max \Y@max=\dimen@ \fi
 \else \ifdim \B@<\Y@min
 \dimen@=\Y@p\advance\dimen@\B@ \dimen@half
 \ifdim \dimen@<\Y@min \Y@min=\dimen@ \fi
 \dimen@=\Y@c\advance\dimen@\B@ \dimen@half
 \ifdim \dimen@>\Y@min \Y@min=\dimen@ \fi
 \fi\fi }
\xydef@\squinedecast@{\halve@dimen\splinedepth@
 \R@c=\L@c \advance\L@c\X@p \halve@dimen\L@c
 \advance\R@c\X@c \halve@dimen\R@c
 \A@=\L@c \advance\A@\R@c \halve@dimen\A@
 \D@c=\U@c \advance\U@c\Y@p \halve@dimen\U@c
 \advance\D@c\Y@c \halve@dimen\D@c
 \B@=\U@c \advance\B@\D@c \halve@dimen\B@
 \begingroup \X@c=\A@ \Y@c=\B@ \splinerec@ \endgroup
 \begingroup \X@c=\A@ \Y@c=\B@ \splinepoint \endgroup
 \X@p=\A@ \L@c=\R@c \Y@p=\B@ \U@c=\D@c \splinerec@}
\xydef@\squinerec@{{\splinefar@false \splinenear@\X@p\X@c\Y@p\Y@c 
 \ifsplinefar@ \aftergroup\squinedecast@ 
 \else \aftergroup\splineadvance@ \fi}}
\xydef@\squineDadvance@@@{\X@p\L@c\Y@p\D@c}
\xydef@\squineplot@maybe{{\X@p=\L@c \Y@p=\U@c \cv@start \the\Edge@c\@ne 
 \ifInside@\aftergroup\splineplot@false\else\aftergroup\splineplot@true\fi}}
\xydef@\setsquinedir@{%
 \d@X=\X@c \advance\d@X-\L@c \d@Y=\Y@c \advance\d@Y-\U@c 
 \dimen@=\ifdim\d@X<\z@-\fi\d@X \ifdim\dimen@<.02\p@
 \dimen@=\ifdim\d@Y<\z@-\fi\d@Y \ifdim\dimen@<.02\p@ 
 \d@X=\X@c \advance\d@X-\X@p \d@Y=\Y@c \advance\d@Y-\Y@p \fi\fi
 \ifdim\X@c=\X@p \ifdim\Y@c=\Y@p 
 \d@X=\L@c \advance\d@X-\X@p \d@Y=\U@c \advance\d@Y-\Y@p \fi\fi
 \setupDirection@ii } 
\xydef@\setsquineknotdir@{%
 \ifdim\zz@\splineval@ \expandafter \setsquinezerodir@
 \else\expandafter \setsquinedir@ \fi } 
\xydef@\setsquinezerodir@{%
 \d@X=\L@c \advance\d@X-\X@p \d@Y=\U@c \advance\d@Y-\Y@p 
 \ifdim\zz@\d@X \ifdim\zz@\d@Y 
 \d@X=\X@c \advance\d@X-\X@p \d@Y=\Y@c \advance\d@Y-\Y@p 
 \fi\fi \setupDirection@ii }
\xydef@\getsquineparams@#1,#2,#3,#4,#5,#6,#7,{%
 \splinelength@=#1\relax\X@p=#2\relax\Y@p=#3\relax
 \A@=#4\relax\B@=#5\relax\X@c=#6\relax\Y@c=#7\relax
}
\xydef@\squineinfo@{%
\expandafter\removePT@\the\X@c\space
\expandafter\removePT@\the\Y@c\space
\expandafter\removePT@\the\A@\space
\expandafter\removePT@\the\B@\space
\expandafter\removePT@\the\X@p\space
\expandafter\removePT@\the\Y@p\space
\expandafter\removePT@\the\dimen5\space\space
\expandafter\removePT@\the\dimen7\space
 }%
\xydef@\squinereverse@{\readsplineparams@
 \expandafter\edef\xysplineparams@{\the\splinelength@,%
 \the\X@c,\the\Y@c,\the\A@,\the\B@,\the\X@p,\the\Y@p,}}%
\xydef@\squine@start@{\setboxz@h\bgroup
 \global\splinelength@=\z@ \global\dimen@i=\z@ \global\dimen3=\z@
 \kern\X@p
 {\squinesetparams@ \X@c=\X@p \Y@c=\Y@p \firstsplinepoint@
 }\bgroup }
\xydef@\squinesetparams@{%
 \global\dimen@i=\X@p \global\dimen3=\Y@p 
 \L@c=\A@ \U@c=\B@ \R@c=\L@c \D@c=\U@c }%
\xydef@\squined@{%
 \expandafter\edef\xysplineparams@{%
 \the\z@,\the\X@p,\the\Y@p,\the\A@,\the\B@,\the\X@c,\the\Y@c,}}
\xydef@\squined@@{%
 \splinedepth@=\p@ 
 \global\splineval@=\z@ 
 \global\dimen@i=\X@p \global\dimen3=\Y@p
 \spline@start 
 \ifx\splinerec@\relax \let\splinerec@=\squinerec@\fi
 \L@c=\A@ \U@c=\B@ \R@c=\L@c \D@c=\U@c 
 \splinerec@ \spline@end }
\xydef@\xycubicbezier@{%
 \addtocrvpts@{\def\crvconnect@{\cubicconnect@}}%
 \xycubicmethods@ \let\splinesegment@=\cubicsegment@
 \begingroup \setcrvobjects@ \xysplineparams@ \splined@@@ 
 \bgroup \setupcubic@ \cubiced@ \splineset@ \savespline@ }
\xydef@\xycubicmethods@{%
 \def\crvconnect@{\cubicconnect@}%
 \def\splinereverse@@{\cubicreverse@@}%
 \let\getsplineparams@=\getcubicparams@
 \let\spline@start@=\cubic@start@
 \let\splinedecast@@=\cubicdecast@
 \let\splinerec@@=\cubicrec@
 \let\splined@@=\cubiced@@
 \let\splineIpt@@=\cubicIpt@
 \let\splineIadvance@@=\cubicIadvance@
 \let\splineoutsidehull@@=\cubicoutsidehull@
 \let\splinetestcvxhull@=\cubictestcvxhull@
 \let\splineinfo@=\cubicinfo@
 \let\setsplinedir@=\setcubicdir@
 \let\setsplineknotdir@=\setcubicknotdir@
 \let\splinereverse@=\cubicreverse@ 
 \let\splineDadvance@@@=\cubicDadvance@@@
 \let\splinesetparams@=\cubicsetparams@
 \let\splineplot@maybe@@=\cubicplot@maybe
 }
\xydef@\cubicconnect@{\splineconnect@ \crvconnect@@
 \let\splinesegment@=\cubicsegment@ }%
\xydef@\cubicsegment@#1{\xycubicmethods@ \def\segmentnum@{1}%
 \setupcubic@ \cubiced@ }
\xydef@\setupcubic@{%
 \xycontrolpt@\z@ \X@p=\X@c \Y@p=\Y@c
 \xycontrolpt@\@ne \A@=\X@c \B@=\Y@c 
 \xycontrolpt@\tw@ \global\dimen3=\X@c \global\dimen5=\Y@c
 \xycontrolpt@\thr@@ 
 \adjustmaxmin@ }
\xydef@\adjustmaxmin@{%
 \ifdim \A@>\X@max \dimen@=\A@ \advance\dimen@\X@p \dimen@half 
 \ifdim\dimen@>\X@max \X@max=\dimen@ \fi \else
 \ifdim \A@<\X@min \dimen@=\A@ \advance\dimen@\X@p \dimen@half 
 \ifdim\dimen@<\X@min \X@min=\dimen@ \fi \fi\fi
 \ifdim \B@>\Y@max \dimen@=\B@ \advance\dimen@\Y@p \dimen@half 
 \ifdim\dimen@>\Y@max \Y@max=\dimen@ \fi \else
 \ifdim \B@<\Y@min \dimen@=\B@ \advance\dimen@\Y@p \dimen@half 
 \ifdim\dimen@<\Y@min \Y@min=\dimen@ \fi \fi\fi
 \ifdim \dimen3>\X@max \dimen@=\dimen3\advance\dimen@\X@c \dimen@half 
 \ifdim\dimen@>\X@max \X@max=\dimen@ \fi \else
 \ifdim \dimen3<\X@min \dimen@=\dimen3\advance\dimen@\X@c \dimen@half 
 \ifdim\dimen@<\X@min \X@min=\dimen@ \fi \fi\fi
 \ifdim \dimen5>\Y@max \dimen@=\dimen5\advance\dimen@\Y@c \dimen@half 
 \ifdim\dimen@>\Y@max \Y@max=\dimen@ \fi \else
 \ifdim \dimen5<\Y@min \dimen@=\dimen5\advance\dimen@\Y@c \dimen@half 
 \ifdim\dimen@<\Y@min \Y@min=\dimen@ \fi \fi\fi
 \dimen@=\A@ \advance\dimen@\dimen3 \dimen@half
 \ifdim\dimen@>\X@max \X@max=\dimen@
 \else \ifdim\dimen@<\X@min \X@min=\dimen@ \fi\fi
 \dimen@=\B@ \advance\dimen@\dimen5 \dimen@half
 \ifdim\dimen@>\Y@max \Y@max=\dimen@
 \else \ifdim\dimen@<\Y@min \Y@min=\dimen@ \fi\fi
}
\xydef@\cubicdecast@{\halve@dimen\splinedepth@
 \A@=\L@c \advance\A@\R@c \halve@dimen\A@
 \advance\R@c\X@c \halve@dimen\R@c
 \B@=\U@c \advance\B@\D@c \halve@dimen\B@
 \advance\D@c\Y@c \halve@dimen\D@c
 \advance\L@c\X@p \halve@dimen\L@c
 \advance\U@c\Y@p \halve@dimen\U@c
 \begingroup 
 \X@c=\R@c \advance\X@c\L@c \halve@dimen\X@c
 \advance\X@c\A@ \halve@dimen\X@c
 \Y@c=\D@c \advance\Y@c\U@c \halve@dimen\Y@c
 \advance\Y@c\B@ \halve@dimen\Y@c
 \R@c=\L@c \advance\R@c\A@ \halve@dimen\R@c
 \D@c=\U@c \advance\D@c\B@ \halve@dimen\D@c
 \bgroup \splinerec@ 
 \egroup \splinepoint \endgroup 
 \X@p=\L@c \advance\X@p\R@c \halve@dimen\X@p
 \advance\X@p\A@ \halve@dimen\X@p
 \L@c=\R@c \advance\L@c\A@ \halve@dimen\L@c
 \Y@p=\U@c \advance\Y@p\D@c \halve@dimen\Y@p
 \advance\Y@p\B@ \halve@dimen\Y@p
 \U@c=\D@c \advance\U@c\B@ \halve@dimen\U@c
 \splinerec@ }
\xydef@\cubicrec@{{\splinefar@false \splinenear@\X@p\X@c\Y@p\Y@c 
 \ifsplinefar@ \aftergroup\cubicdecast@
 \else \aftergroup\splineadvance@ \fi}}
\xydef@\cubicDadvance@@@{\X@p\X@c\Y@p\Y@c}
\xydef@\cubicplot@maybe{{\X@p=\L@c \Y@p=\U@c \cv@start \the\Edge@c\@ne 
 \ifInside@\aftergroup\cubicplot@maybeii\else\aftergroup\splineplot@true\fi}}
\xydef@\cubicplot@maybeii{{\X@p=\R@c \Y@p=\D@c \cv@start \the\Edge@c\@ne 
 \ifInside@\aftergroup\splineplot@false\else\aftergroup\splineplot@true\fi}}
\xydef@\cubiced@@{%
 \splinedepth@=\p@ 
 \global\splineval@=\z@ 
 \spline@start 
 \global\dimen@i=\X@p \global\dimen3=\Y@p
 \splinerec@ \spline@end }
\xydef@\setcubicdir@{%
 \ifdim\splinedepth@<.001\p@\DN@{\cubiccoarsedir@}%
 \else\DN@{\cubicfinedir@}\fi \next@ }
\xydef@\cubicfinedir@{%
 \d@X=\X@c \advance\d@X-\R@c \d@Y=\Y@c \advance\d@Y-\D@c 
 \ifdim\zz@\d@X \ifdim\zz@\d@Y 
 \d@X=\X@c \advance\d@X-\L@c \d@Y=\Y@c \advance\d@Y-\U@c 
 \ifdim\zz@\d@X \ifdim\zz@\d@Y 
 \d@X=\X@c \advance\d@X-\X@p \d@Y=\Y@c \advance\d@Y-\Y@p 
 \fi\fi \fi\fi
 \setupDirection@ii 
\splinetrace@{dir:(\the\d@X,\the\d@Y),\the\Direction; depth:\the\splinedepth@}%
} 
\xydef@\cubiccoarsedir@{%
 \d@X=\X@c \advance\d@X-\X@p \d@Y=\Y@c \advance\d@Y-\Y@p \setupDirection@ii
 \global\dimen5=\d@X \global\dimen7=\d@Y
\splinetrace@{dir:(\the\d@X,\the\d@Y),\the\Direction; depth:\the\splinedepth@}%
}
\xydef@\setcubicknotdir@{%
 \ifdim\zz@\splineval@ \DN@{\setcubiczerodir@}%
 \else \DN@{\cubicfinedir@}\fi \next@ } 
\xydef@\setcubiczerodir@{%
 \d@X=\L@c \advance\d@X-\X@p \d@Y=\U@c \advance\d@Y-\Y@p 
 \ifdim\zz@\d@X \ifdim\zz@\d@Y 
 \d@X=\R@c \advance\d@X-\X@p \d@Y=\D@c \advance\d@Y-\Y@p 
 \ifdim\zz@\d@X \ifdim\zz@\d@Y 
 \d@X=\X@c \advance\d@X-\X@p \d@Y=\Y@c \advance\d@Y-\Y@p 
 \fi\fi \fi\fi \setupDirection@ii }
\xydef@\getcubicparams@#1,#2,#3,#4,#5,#6,#7,#8,#9,{%
 \splinelength@=#1\relax\X@p=#2\relax\Y@p=#3\relax\L@c=#4\relax
 \U@c=#5\relax\R@c=#6\relax\D@c=#7\relax\X@c=#8\relax\Y@c=#9\relax
}%
\xydef@\cubicinfo@{%
\expandafter\removePT@\the\X@p\space
\expandafter\removePT@\the\Y@p\space
\expandafter\removePT@\the\L@c\space
\expandafter\removePT@\the\U@c\space
\expandafter\removePT@\the\R@c\space
\expandafter\removePT@\the\D@c\space
\expandafter\removePT@\the\X@c\space
\expandafter\removePT@\the\Y@c\space
\expandafter\removePT@\the\dimen5\space\space
\expandafter\removePT@\the\dimen7\space
 }%
\xydef@\cubicreverse@{\readsplineparams@
 \expandafter\edef\xysplineparams@{\the\splinelength@,%
 \the\X@c,\the\Y@c,\the\R@c,\the\D@c,\the\L@c,\the\U@c,\the\X@p,\the\Y@p,}}%
\xydef@\cubicreverse@@{%
 \splinereverse@@@ 
 \dimen@ii=\L@c \L@c=\R@c \R@c=\dimen@ii 
 \dimen@ii=\U@c \U@c=\D@c \D@c=\dimen@ii }
\xydef@\cubic@start@{\setboxz@h\bgroup
 \global\splinelength@=\z@ \global\dimen@i=\z@ \global\dimen3=\z@
 \kern\X@p
 {\cubicsetparams@ \X@c=\X@p \Y@c=\Y@p \R@c=\X@c \D@c=\Y@c
 \firstsplinepoint@ }\bgroup 
}
\xydef@\cubicsetparams@{%
 \expandafter\expandafter\expandafter\getsplineparams@\xysplineparams@
 \global\dimen@i=\X@p \global\dimen3=\Y@p }
\xydef@\cubiced@{%
 \expandafter\edef\xysplineparams@{\the\z@,\the\X@p,\the\Y@p
 ,\the\A@,\the\B@,\the\dimen3,\the\dimen5,\the\X@c,\the\Y@c,}%
 }%
\xydef@\xybspline@iii{%
 \addtocrvpts@{\def\crvconnect@{\bsplineiiiconnect@}}%
 \def\crvconnect@{\bsplineiiiconnect@}\xybsplinemethods@ 
 \let\splinesegment@=\bsplinesegment@iii
 \begingroup\setcrvobjects@ \dobspline@ \savespline@ }
\xydef@\bsplineiiiconnect@{\splineconnect@ \crvconnect@@
 \let\splinesegment@=\bsplinesegment@iii }%
\xydef@\xybspline@iv{%
 \addtocrvpts@{\def\crvconnect@{\bsplineivconnect@}}%
 \def\crvconnect@{\bsplineivconnect@}\xybsplinemethods@
 \let\splinesegment@=\bsplinesegment@iv
 \begingroup\setcrvobjects@ \dobspline@ \savespline@ }
\xydef@\bsplineivconnect@{\splineconnect@ \crvconnect@@
 \let\splinesegment@=\bsplinesegment@iv }%
\xydef@\xybspline@{%
\splinetrace@{B-spline with \numcontrolpts\space control points.}%
 \addtocrvpts@{\def\crvconnect@{\bsplineconnect@}}%
 \def\crvconnect@{\bsplineconnect@}\xybsplinemethods@ 
 \let\splinesegment@=\bsplinesegment@ 
 \begingroup\setcrvobjects@
 \dobspline@ \savespline@ }
\xydef@\xybsplinemethods@{%
 \def\splinereverse@@{\cubicreverse@@}%
 \let\getsplineparams@=\getbsplineparams@
 \let\spline@start@=\cubic@start@
 \let\splinedecast@@=\cubicdecast@
 \let\splinerec@@=\cubicrec@
 \let\splineIpt@@=\cubicIpt@
 \let\splineIadvance@@=\cubicIadvance@
 \let\splined@@=\bsplined@@
 \let\splineinfo@=\cubicinfo@
 \let\setsplinedir@=\setcubicdir@
 \let\setsplineknotdir@=\setcubicknotdir@
 \let\splinereverse@=\cubicreverse@ 
 \let\splineDadvance@@@=\cubicDadvance@@@
 \let\splinesetparams@=\cubicsetparams@
 \global\let\lastbspline@=\lastbspline@@
 \global\let\middlebspline@=\middlebspline@@
}
\xydef@\bsplined@@{%
 \splinedepth@=\p@ 
 \global\splineval@=\z@ 
 \spline@start 
 \global\dimen@i=\X@p \global\dimen3=\Y@p
 \splinerec@ \spline@end }
\xydef@\bsplineconnect@{\splineconnect@ \crvconnect@@
 \let\splinesegment@=\bsplinesegment@ }%
\xydef@\getbsplineparams@{\getcubicparams@}
\xydef@\dobspline@{\xysplineparams@ \scanbspline@ \firstbspline@ }%
\xydef@\firstbspline@{%
 \enter@{\pfromthep@ \cfromthec@}\enter@{\cfromthec@}\bgroup
 \def\segmentnum@{1}\xycontrolpt@\z@ \X@p=\X@c \Y@p=\Y@c
\splinetrace@{0: \the\X@p, \the\Y@p}%
 \xycontrolpt@\@ne \A@=\X@c \B@=\Y@c 
\splinetrace@{1: \the\X@c, \the\Y@c}%
 \xycontrolpt@\tw@ 
\splinetrace@{2: \the\X@c, \the\Y@c}%
 \dimen@=\X@c \advance\dimen@\A@ \dimen@half
 \global\dimen3=\dimen@
 \dimen@=\Y@c \advance\dimen@\B@ \dimen@half
 \global\dimen5=\dimen@
 \xycontrolpt@{3}%
\splinetrace@{3: \the\X@c, \the\Y@c}%
 \expandafter\count@\xycrvcnt@\relax
 \ifnum\count@=3\relax 
 \advance\X@c-\A@ \dimen@nth4\X@c
 \advance\X@c\dimen3\relax
 \advance\Y@c-\B@ \dimen@nth4\Y@c
 \advance\Y@c\dimen5\relax
 \enter@{\X@p=\the\X@c \Y@p=\the\Y@c \crv@cnt@=\@ne\relax
 \noexpand\lastbspline@ }%
 \else 
 \advance\X@c 7\dimen3 \advance\X@c-2\A@ 
 \dimen@nth6\X@c
 \advance\Y@c 7\dimen5 \advance\Y@c-2\B@ 
 \dimen@nth6\Y@c
 \enter@{\X@p=\the\X@c \Y@p=\the\Y@c \crv@cnt@=\@ne\relax
 \noexpand\middlebspline@ }%
 \fi \adjustmaxmin@ \czeroEdge@
 \bsplined@ \splineset@ \leave@ }
\xydef@\lastbspline@@{\bgroup 
 \advance\crv@cnt@\@ne \edef\segmentnum@{\the\crv@cnt@}%
\splinetrace@{<: \the\X@p, \the\Y@p}%
 \advance\crv@cnt@\@ne \xycontrolpt@{\crv@cnt@}%
 \global\dimen3=\X@c \global\dimen5=\Y@c
\splinetrace@{\the\crv@cnt@: \the\X@c, \the\Y@c}%
 \advance\crv@cnt@\m@ne \xycontrolpt@{\crv@cnt@}%
\splinetrace@{\the\crv@cnt@: \the\X@c, \the\Y@c}%
 \A@=\X@c \advance\A@\dimen3 \halve@dimen\A@
 \B@=\Y@c \advance\B@\dimen5 \halve@dimen\B@
 \adjustmaxmin@ \leave@ \relax \cv@end
\splinetrace@{>: \the\X@c, \the\Y@c}%
 \bsplined@ \splineset@ \leave@ }%
\xylet@\lastbspline@=\lastbspline@@
\xydef@\middlebspline@@{%
 \advance\crv@cnt@\@ne \edef\segmentnum@{\the\crv@cnt@}%
\splinetrace@{<: \the\X@p, \the\Y@p}%
 \bgroup 
 \xycontrolpt@{\crv@cnt@}\A@=2\X@c \B@=2\Y@c
\splinetrace@{\the\crv@cnt@: \the\X@c, \the\Y@c}%
 \advance\crv@cnt@\@ne \xycontrolpt@{\crv@cnt@}%
\splinetrace@{\the\crv@cnt@: \the\X@c, \the\Y@c}%
 \advance\A@\X@c \dimen@nth3\A@
 \advance\B@\Y@c \dimen@nth3\B@
 \advance\X@c\A@ \halve@dimen\X@c
 \advance\Y@c\B@ \halve@dimen\Y@c
 \global\dimen3=\X@c \global\dimen5=\Y@c 
 \advance\crv@cnt@\@ne \xycontrolpt@{\crv@cnt@}%
\splinetrace@{\the\crv@cnt@: \the\X@c, \the\Y@c}%
 \expandafter\count@\xycrvcnt@\relax 
 \ifnum\crv@cnt@<\count@\relax 
 \advance\X@c 7\dimen3\advance\X@c-2\A@
 \dimen@nth6\X@c
 \advance\Y@c 7\dimen5\advance\Y@c-2\B@
 \dimen@nth6\Y@c
 \enter@{\X@p=\the\X@c \Y@p=\the\Y@c \crv@cnt@=\segmentnum@\relax
 \noexpand\middlebspline@}%
 \else 
 \advance\X@c-\A@ \dimen@nth4\X@c
 \advance\X@c \dimen3\relax
 \advance\Y@c-\B@ \dimen@nth4\Y@c
 \advance\Y@c \dimen5\relax
 \enter@{\X@p=\the\X@c \Y@p=\the\Y@c \noexpand\lastbspline@}%
 \fi \adjustmaxmin@ 
 \bsplined@ \splineset@ \leave@ } 
\xylet@\middlebspline@=\middlebspline@@
\xydef@\scanbspline@{\splined@@@}
\xydef@\bsplined@{\cubiced@ 
 \expandafter\ifx\xysplineedges@\relax\relax\DN@{}%
 \else\DN@{\adjustbsplineedges@}\fi \next@ }
\xydef@\adjust@forsegments@{\getcrvsegsnum@ 
 \ifnum\count@>\@ne
\splinetrace@{adjust for \the\count@\space segments:
 \the\dimen5, \the\dimen7}%
 \multiply\dimen5 by \count@\relax \dimen@=\segmentnum@\p@
 \ifnum\dimen5>\dimen@ \relax\dimen5=\p@
 \else \advance\dimen5-\segmentnum@\p@ \advance\dimen5 by\p@ \fi
 \ifnum\dimen5<\z@ \relax\dimen5=\z@\relax\fi
 \multiply\dimen7 by \count@\relax
 \dimen@=\segmentnum@\p@
 \ifnum\dimen7<\dimen@ \advance\dimen@-\p@
 \ifnum\dimen7>\dimen@ \advance\dimen7-\dimen@
 \else \dimen7=\z@ \fi
 \else \dimen7=\p@ \fi
\splinetrace@{adjusted for \the\count@\space segments:
 \the\dimen5, \the\dimen7}%
 \fi}
\xydef@\adjustbsplineedges@{\bgroup
\splinetrace@{** adjusting edges **}%
 \readsplineparams@ \adjust@forsegments@
\splinetrace@{params:\xysplineparams@}%
\splinetrace@{segment \segmentnum@:<\the\dimen5,\the\dimen7>:\xysplineedges@}%
 \multiply\dimen7by\m@ne \advance\dimen7by\p@
 \expandafter\edef\xysplineedges@{%
 \noexpand\z@;\the\dimen5,\noexpand\z@;\the\dimen7,}%
 \edef\tmp@{\egroup 
 \noexpand\def\expandafter\noexpand\xysplineedges@{\xysplineedges@}}%
 \tmp@ }
\xydef@\bsegment@@ii@iii{%
 \xycontrolpt@{\count@@}\global\dimen3=\X@c \global\dimen5=\Y@c
\splinetrace@{\the\count@@: \the\X@c, \the\Y@c}%
 \advance\count@@\@ne \xycontrolpt@{\count@@}\A@=\X@c \B@=\Y@c
 \advance\A@ by2\dimen3 \dimen@nth3\A@
 \advance\B@ by2\dimen5 \dimen@nth3\B@
 \dimen@=\dimen3 \advance\dimen@ by2\X@c
 \dimen@nth3\dimen@
 \global\dimen3=\dimen@
 \dimen@=\dimen5 \advance\dimen@ by2\Y@c
 \dimen@nth3\dimen@
 \global\dimen5=\dimen@
\splinetrace@{<: \the\dimen3, \the\dimen5}%
\splinetrace@{>: \the\A@, \the\B@}%
 \advance\count@@\m@ne }
\xydef@\bsegment@@i{\bgroup
 \advance\count@@\m@ne \xycontrolpt@{\count@@}%
\splinetrace@{\the\count@@: \the\X@c, \the\Y@c}%
 \edef\tmp@{\egroup \X@p=\the\X@c \Y@p=\the\Y@c}\tmp@
 \advance\X@p-2\dimen3\advance\X@p by7\A@
 \dimen@nth6\X@p
 \advance\Y@p-2\dimen5\advance\Y@p by7\B@ 
 \dimen@nth6\Y@p
}
\xydef@\bsegment@@iv{%
 \advance\count@@\tw@ \xycontrolpt@{\count@@}%
\splinetrace@{\the\count@@: \the\X@c, \the\Y@c}%
 \advance\X@c by7\dimen3\advance\X@c-2\A@ 
 \dimen@nth6\X@c
 \advance\Y@c by7\dimen5\advance\Y@c-2\B@ 
 \dimen@nth6\Y@c
\splinetrace@{>>: \the\X@c, \the\Y@c }%
}
\xydef@\bsegment@@ii@i{\bgroup
 \advance\count@@\m@ne \xycontrolpt@{\count@@}%
\splinetrace@{\the\count@@: \the\X@c, \the\Y@c}%
 \edef\tmp@{\egroup \X@p=\the\X@c \Y@p=\the\Y@c}\tmp@
 \advance\X@p-\dimen3\advance\X@p by4\A@ 
 \dimen@nth4\X@p
 \advance\Y@p-\dimen5\advance\Y@p by4\B@ 
 \dimen@nth4\Y@p
\splinetrace@{<<: \the\X@p, \the\Y@p}%
}
\xydef@\bsegment@@y@iv{%
 \advance\count@@\tw@ \xycontrolpt@{\count@@}%
\splinetrace@{\the\count@@: \the\X@c, \the\Y@c}%
 \advance\X@c by4\dimen3\advance\X@c-\A@ 
 \dimen@nth4\X@c
 \advance\Y@c by4\dimen5\advance\Y@c-\B@ 
 \dimen@nth4\Y@c
}
\xydef@\bsegment@i{%
 \xycontrolpt@\z@ \X@p=\the\X@c \Y@p=\the\Y@c
\splinetrace@{0: \the\X@p \the\Y@p}%
 \xycontrolpt@\@ne
\splinetrace@{1: \the\X@c, \the\Y@c}\A@=\X@c \B@=\Y@c 
 \xycontrolpt@\tw@
 \dimen@=\X@c \advance\dimen@\A@ \dimen@half
 \global\dimen3=\dimen@
\splinetrace@{2: \the\X@c, \the\Y@c}%
 \dimen@=\Y@c \advance\dimen@\B@ \dimen@half
 \global\dimen5=\dimen@ }
\xydef@\bsegment@i@iv{%
 \xycontrolpt@{3}%
\splinetrace@{3: \the\X@c, \the\Y@c}%
 \advance\X@c by7\dimen3\advance\X@c-2\A@ 
 \dimen@nth6\X@c
 \advance\Y@c by7\dimen5\advance\Y@c-2\B@ 
 \dimen@nth6\Y@c
 }
\xydef@\bsegment@z{%
 \expandafter\count@@\xycrvptsnum@ \advance\count@@\@ne 
 \xycontrolpt@{\the\count@@}\relax
\splinetrace@{\the\count@@: \the\X@c, \the\Y@c}%
 \advance\count@@\m@ne
 \bgroup
 \xycontrolpt@{\the\count@@}%
\splinetrace@{\the\count@@: \the\X@c, \the\Y@c}%
 \global\dimen3=\X@c \global\dimen5=\Y@c
 \advance\count@@\m@ne \xycontrolpt@{\the\count@@}%
\splinetrace@{\the\count@@: \the\X@c, \the\Y@c}%
 \A@=\X@c \advance\A@\dimen3 \halve@dimen\A@
 \B@=\Y@c \advance\B@\dimen5 \halve@dimen\B@
 \edef\tmp@{\egroup \A@=\the\A@ \B@=\the\B@ \count@@=\the\count@@}%
 \tmp@ }
\xydef@\bsegment@z@i{%
 \expandafter\count@@\xycrvptsnum@\relax\advance\count@@-\tw@ 
 \bgroup
 \xycontrolpt@{\count@@}\X@p=\the\X@c \Y@p=\the\Y@c
\splinetrace@{\the\count@@: \the\X@c, \the\Y@c}%
 \advance\X@p by7\A@ \advance\X@p-2\dimen3 \dimen@nth6\X@p
 \advance\Y@p by7\B@ \advance\Y@p-2\dimen5 \dimen@nth6\Y@p
 \edef\tmp@{\egroup \X@p=\the\X@p \Y@p=\the\Y@p}%
 \tmp@ }
\xydef@\bsplinesegment@#1{\xybsplinemethods@ 
 \count@@=#1\relax 
 \ifnum\count@@=\@ne
 \bsegment@i \bsegment@i@iv
 \else\ifnum\count@@=\tw@
 \bsegment@@ii@iii \bsegment@@ii@i \bsegment@@iv
 \else\expandafter\count@\xycrvptsnum@\advance\count@\m@ne
 \ifnum\count@@=\count@
 \bsegment@z \bsegment@z@i 
 \else\advance\count@\m@ne
 \ifnum\count@@=\count@
 \bsegment@@ii@iii \bsegment@@i \bsegment@@y@iv
 \else
 \bsegment@@ii@iii \bsegment@@i \bsegment@@iv
 \fi\fi\fi\fi 
 \expandafter\def\expandafter\segmentnum@\expandafter{\number#1}%
 \bsplined@ }
\xydef@\bsplinesegment@iii#1{\xybsplinemethods@ 
\splinetrace@{2 segments; \number#1}%
 \count@@=#1\relax 
 \ifnum\count@@=\@ne \bsegment@i 
 \xycontrolpt@{3}%
\splinetrace@{3: \the\X@c, \the\Y@c}%
 \advance\X@c 4\dimen3\advance\X@c-\A@ 
 \dimen@nth4\X@c
 \advance\Y@c 4\dimen5\advance\Y@c-\B@ 
 \dimen@nth4\Y@c
 \else\ifnum\count@@=\tw@ \bsegment@z 
 \bgroup\xycontrolpt@{\@ne}%
\splinetrace@{1: \the\X@c, \the\Y@c}%
 \edef\tmp@{\egroup \X@p=\the\X@c \Y@p=\the\Y@c}\tmp@
 \advance\X@p 4\A@ \advance\X@p-\dimen3
 \dimen@nth4\X@p
 \advance\Y@p 4\B@ \advance\Y@p-\dimen5
 \dimen@nth4\Y@p
 \fi\fi
 \expandafter\def\expandafter\segmentnum@\expandafter{\number#1}%
 \bsplined@ }
\xydef@\bsplinesegment@iv#1{\xybsplinemethods@ 
\splinetrace@{3 segments; \number#1}%
 \count@@=#1\relax
 \ifnum\count@@=\@ne \bsegment@i \bsegment@i@iv
 \else\ifnum\count@@=\tw@
 \bsegment@@ii@iii \bsegment@@ii@i \bsegment@@y@iv
 \else\ifnum\count@@=3\relax
 \bsegment@z \bsegment@z@i
 \fi\fi\fi 
 \expandafter\def\expandafter\segmentnum@\expandafter{\number#1}%
 \bsplined@ }
\message{circles,}
\xydef@\Circmagic@@{0.5517847}
\xylet@\Circmagic=\Circmagic@@
\xydef@\twoPi@{6.2831852}
\xydef@\fullPi@{3.1415926}
\xydef@\halfPi@{1.5707963}
\xynew@{dimen}\L@
\xydef@\xycircle#1#{\hbox\bgroup\afterVECTORorEMPTY{%
 \xy@@{\R@=\X@c \L@=\Y@c}\xycircle@}{\xy@@{\R@=\R@c \L@=\L@c}\xycircle@}#1@}
\xydef@\xycircle@#1@#2{%
 \DN@{#1}\ifx\next@\empty\def\onlyQuad@{}\else \count@=#1\relax 
 \ifnum\count@<5 \advance\count@-3\relax 
 \ifnum\count@<\z@ \advance\count@ 4\relax\fi \edef\onlyQuad@{\the\count@}%
 \else\xyerror@{illegal circle <radius>: must be <vector> or <empty>}{}\fi
 \fi \xy@@{\def\circleSTYLE@{#2}}\def\circleSTYLE@{#2}\xycircle@i}
\xydef@\xycircle@i{\hbox{\vbox{\vskip\L@
 \hbox to2\R@{\hfill \buildcircle@ \hfill}\vskip\L@ }}%
 \L@c=\R@ \R@c=\R@ \D@c=\L@ \U@c=\L@ \def\Leftness@{.5}\def\Upness@{.5}%
 \def\Drop@@{\styledboxz@}\def\Connect@@{\straight@\relax}\Edge@c={\circleEdge}%
 \OBJECT@x}
\xydef@\adjustMinMaxcirc@#1#2{%
 \dimen@=\X@c \advance\dimen@#1\relax\ifdim\dimen@>\X@max \X@max=\dimen@\fi
 \dimen@=\X@c \advance\dimen@-#1\relax\ifdim\dimen@<\X@min \X@min=\dimen@\fi
 \dimen@=\Y@c \advance\dimen@#2\relax\ifdim\dimen@>\Y@max \Y@max=\dimen@\fi
 \dimen@=\Y@c \advance\dimen@-#2\relax\ifdim\dimen@<\Y@min \Y@min=\dimen@\fi
}
%% \cubicCircleControls@@ 
\xydef@\cubicCircleControls@@{\X@origin=\z@ \Y@origin=\z@
 \X@xbase=\R@ \Y@xbase=\z@ \X@ybase=\z@ \Y@ybase=\L@
 \vfromcartesian@@1,0@\czeroEdge@\idfromc@{0@c}%
 \vfromcartesian@@0,1@\czeroEdge@\idfromc@{1@c}%
 \vfromcartesian@@-1,0@\czeroEdge@\idfromc@{2@c}%
 \vfromcartesian@@0,-1@\czeroEdge@\idfromc@{3@c}%
 \vfromcartesian@@1,\Circmagic@@ @\czeroEdge@\idfromc@{1@m}%
 \vfromcartesian@@\Circmagic@@,1@\czeroEdge@\idfromc@{2@m}%
 \vfromcartesian@@-\Circmagic@@,1@\czeroEdge@\idfromc@{3@m}%
 \vfromcartesian@@-1,\Circmagic@@ @\czeroEdge@\idfromc@{4@m}%
 \vfromcartesian@@-1,-\Circmagic@@ @\czeroEdge@\idfromc@{5@m}%
 \vfromcartesian@@-\Circmagic@@,-1@\czeroEdge@\idfromc@{6@m}%
 \vfromcartesian@@\Circmagic@@,-1@\czeroEdge@\idfromc@{7@m}%
 \vfromcartesian@@1,-\Circmagic@@ @\czeroEdge@\idfromc@{8@m}%
 }
\xydef@\doCircleQuadrant@@#1#2{\save@ \ifcase#2\relax
 \doCircleQuadrant@@@{0@c}{1@m}{2@m}{1@c}{#1}\or
 \doCircleQuadrant@@@{1@c}{3@m}{4@m}{2@c}{#1}\or
 \doCircleQuadrant@@@{2@c}{5@m}{6@m}{3@c}{#1}\or
 \doCircleQuadrant@@@{3@c}{7@m}{8@m}{0@c}{#1}\or
 \doCircleQuadrant@@@{0@c}{1@m}{2@m}{1@c}{#1}\or
 \doCircleQuadrant@@@{1@c}{3@m}{4@m}{2@c}{#1}\or
 \doCircleQuadrant@@@{2@c}{5@m}{6@m}{3@c}{#1}\or
 \doCircleQuadrant@@@{3@c}{7@m}{8@m}{0@c}{#1}\fi \leave@ }
\xydef@\doCircleQuadrant@@@#1#2#3#4#5{%
 \cfromid@{#1}\pfromc@\senter@
 \cfromid@{#2}\spushc@\cfromid@{#3}\spushc@\cfromid@{#4}%
 \let\bstartPLACE@=\empty \connect@\crvs{#5}\relax\sinit@\sleave@
 \resetbreaks@}
\xydef@\dosolidcircle@#1{%
 \cubicCircleControls@@ 
 \doCircleQuadrant@@{#1}1 \relax\Clast@@
 \doCircleQuadrant@@{#1}2 \relax\Clast@@
 \doCircleQuadrant@@{#1}3 \relax\Clast@@
 \doCircleQuadrant@@{#1}4 \relax\Clast@@}%
\xydef@\solidcircle@{\dosolidcircle@@}
\xylet@\dosolidcircle@@=\dosolidcircle@
\xydef@\circledobjects@{\cubicCircleControls@@ 
 \setboxz@h{\expandafter\object\circleSTYLE@{}}%
 \ifdim\L@>\R@ \dimen@ii=\ht\z@ \advance\dimen@ii \dp\z@
 \ifdim\zz@\dimen@ii \dimen@ii=\wdz@\fi
 \else \dimen@ii=\wdz@ 
 \ifdim\zz@\dimen@ii \dimen@ii=\ht\z@ \advance\dimen@ii \dp\z@\fi
 \fi \ifdim\zz@\dimen@ii \dimen@ii=2\jot\fi
 \expandafter\dimen@\ifdim\L@>\R@ \twoPi@\L@\else \twoPi@\R@\fi
 \advance\dimen@.5\dimen@ii
 \count@@=\dimen@ \count@=\dimen@ii \divide\count@@\count@
 \edef\numobjects{\the\count@@}\dimen@=4\p@
 \dimen@nth\numobjects\dimen@
 \edef\circleseparation@{\expandafter\removePT@\the\dimen@}%
 \edef\circleplace@{-\circleseparation@}\placeQuadrants@}%
\xydef@\placeQuadrants@{\DN@{\placeAllQuadrants@}%
 \ifx\onlyQuad@\undefined\else\ifx\onlyQuad@\empty\else
 \DN@{\expandafter\placeCircQuadrant@\expandafter{\onlyQuad@}}%
 \fi\fi \next@ }%
\xydef@\placeAllQuadrants@{%
 \placeCircQuadrant@{1}%
 \advance\dimen@-\p@\advance\dimen@-\circleseparation@\p@
 \edef\circleplace@{\expandafter\removePT@\the\dimen@}%
 \placeCircQuadrant@{2}%
 \advance\dimen@-\p@\advance\dimen@-\circleseparation@\p@
 \edef\circleplace@{\expandafter\removePT@\the\dimen@}%
 \placeCircQuadrant@{3}%
 \advance\dimen@-\p@\advance\dimen@-\circleseparation@\p@
 \edef\circleplace@{\expandafter\removePT@\the\dimen@}%
 \placeCircQuadrant@{4}}
\xydef@\placeCircQuadrant@#1{%
 \let\bstartPLACE@=\relax \doCircleQuadrant@@{}#1%
 \loop@
 \expandafter\dimen@\circleplace@\p@
 \advance\dimen@\circleseparation@\p@
 \edef\circleplace@{\expandafter\removePT@\the\dimen@}%
 \ifdim\dimen@<\p@ \placeCircObject@
 \repeat@ }
\xydef@\placeCircObject@{\begingroup
 \crvconnect@@ \Creset@@ \Invisible@false
 \expandafter\splinealong@\expandafter{\circleplace@}%
 \expandafter\drop\circleSTYLE@{}\endgroup }
\xydef@\buildcircle@{\save@
 \DNii@{\circledobjects@}%
 \ifx\circleSTYLE@\empty\DNii@{\solidcircle@{}}%
 \else \expandafter\DN@\expandafter{\addDASH@{}}\relax
 \ifx\next@\circleSTYLE@ \DNii@{\solidcircle@{}}%
 \else \expandafter\DN@\expandafter{\addEQ@{}}%
 \ifx\next@\circleSTYLE@ 
 \expandafter\circletemplate@\expandafter{\addEQ@{}}{}%
 \else \expandafter\DN@\expandafter{\addDASH@ 2}%
 \ifx\next@\circleSTYLE@ \DNii@{\doublecircle@{}}%
 \else \expandafter\DN@\expandafter{\addDASH@ 3}%
 \ifx\next@\circleSTYLE@ \DNii@{\triplecircle@{}}%
 \else \expandafter\expandafter\expandafter\DN@\expandafter\expandafter
 \expandafter{\expandafter\addDASH@\addDASH@{}}%
 \ifx\next@\circleSTYLE@ \DNii@{\dashedcircle@{}}%
 \else \expandafter\expandafter\expandafter\DN@\expandafter\expandafter
 \expandafter{\expandafter\addEQ@\addEQ@{}}%
 \ifx\next@\circleSTYLE@ \expandafter\expandafter\expandafter
 \circletemplate@\expandafter\expandafter\expandafter{%
 \expandafter\addEQ@\addEQ@{}}2%
 \else \expandafter\expandafter\expandafter\DN@\expandafter\expandafter
 \expandafter{\expandafter\addEQ@\addEQ@2}%
 \ifx\next@\circleSTYLE@ \expandafter\expandafter\expandafter
 \circletemplate@\expandafter\expandafter\expandafter{%
 \expandafter\addEQ@\addEQ@{}}2%
 \else \expandafter\expandafter\expandafter\DN@\expandafter\expandafter
 \expandafter{\expandafter\addEQ@\addEQ@3}%
 \ifx\next@\circleSTYLE@ \expandafter\expandafter\expandafter
 \circletemplate@\expandafter\expandafter\expandafter{%
 \expandafter\addEQ@\addEQ@{}}3%
 \else \expandafter\DN@\expandafter{\addDOT@{}}\relax
 \ifx\next@\circleSTYLE@ \DNii@{\dottedcircle@{}}%
 \else \expandafter\DN@\expandafter{\addDOT@2}\relax
 \ifx\next@\circleSTYLE@ \DNii@{\dbldottedcircle@{}}%
 \else \expandafter\DN@\expandafter{\addDOT@3}\relax
 \ifx\next@\circleSTYLE@ \DNii@{\trpldottedcircle@{}}%
 \else \DN@{:}\relax
 \ifx\next@\circleSTYLE@ \DNii@{\dbldottedcircle@{}}%
 \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi \nextii@ \leave@}
\xydef@\circletemplate@#1#2{\def\circleSTYLE@{\dir#2{#1}}}
\xydef@\doublecircle@#1{%
 \advance\R@-\p@ \advance\L@-\p@ \solidcircle@{}%
 \advance\R@ 2\p@ \advance\L@ 2\p@ \solidcircle@{}}
\xydef@\triplecircle@#1{%
 \advance\R@-2\p@ \advance\L@-2\p@ \solidcircle@{}%
 \advance\R@ 2\p@ \advance\L@ 2\p@ \solidcircle@{}%
 \advance\R@ 2\p@ \advance\L@ 2\p@ \solidcircle@{}}
\xydef@\dottedcircle@#1{%
 \expandafter\def\expandafter\circleSTYLE@\expandafter{%
 \zerodot@i}%
 \circledobjects@}
\xydef@\dashedcircle@#1{%
 \expandafter\def\expandafter\circleSTYLE@\expandafter{\zerodash@i}%
 \circledobjects@}
\xydef@\dbldottedcircle@#1{%
 \advance\R@-\p@ \advance\L@-\p@ \dottedcircle@{}%
 \advance\R@ 2\p@ \advance\L@ 2\p@ \dottedcircle@{}}
\xydef@\trpldottedcircle@{%
 \advance\R@-2\p@ \advance\L@-2\p@ \dottedcircle@{}%
 \advance\R@ 2\p@ \advance\L@ 2\p@ \dottedcircle@{}%
 \advance\R@ 2\p@ \advance\L@ 2\p@ \dottedcircle@{}}
{\xyuncatcodes \gdef\next{=<.75\jot>{\zerodot}}}
\xylet@\zerodot@i=\next
{\dimen0=2\xydashl@ \xyuncatcodes 
\expandafter\gdef\expandafter\next\expandafter{\expandafter
 =\expandafter<\the\dimen0 >_\dir{|}}}
\xylet@\zerodash@i=\next
{\xyuncatcodes\gdef\next{--}}
\xylet@\dashcorntemp@@=\next
{\xyuncatcodes\gdef\next{.}}
\xylet@\dotcorntemp@@=\next
\xydef@\dotcorner@#1{%
 \expandafter\circleCorner@\expandafter{\dotcorntemp@@}{#1}}%
\xydef@\dashcorner@#1{%
 \expandafter\circleCorner@\expandafter{\dashcorntemp@@}{#1}}
\xydef@\circleCorner@#1#2{\setboxz@h\bgroup 
 \edef\next{#2\relax\R@=\the\R@\relax\L@=\R@ }%
 \expandafter\xycircle@\next @{#1}%
 \ifcase#2\or \setboxz@h{\lower\R@\boxz@\kern\X@c}%
 \or \setboxz@h{\kern-\R@\lower\R@\boxz@\kern\R@\kern\X@c}%
 \or \setboxz@h{\kern-\R@\lower\R@\boxz@\kern\R@\kern\X@c}%
 \or \setboxz@h{\lower\R@\boxz@\kern\X@c}\fi
 \wdz@=\R@ \ht\z@=\R@ \dp\z@=\R@ \boxz@
 }
\xydef@\qspline{\hbox\bgroup\crvresetbreaks@ \xy@spline@}
\xydef@\xy@spline@#1#{\if\sempty@ \DN@{\crvs@{}\resetbreaks@}%
 \else\DN@{\xy@spline@i{#1}}\fi \next@ }%
\xydef@\xy@spline@i#1#2{\def\splineSTYLE@{#2}%
 \DN@{\xy@spline@ii}\DNii@{#1}%
 \ifx\nextii@\empty\DN@{\xy@spline@ii@@}\fi \next@ }
\xydef@\xy@spline@ii{\save@ \cfromp@\idfromc@{@p}%
 \enter@\cplusthec@ \count@@=\s@top\advance\count@@\m@ne
 \cfroms@{\count@@}\leave@
 \halve@dimen\X@c
 \halve@dimen\Y@c
 \czeroEdge@ \idfromc@{@c}%
 \expandafter\doSplineStraight@\expandafter{\splineSTYLE@}%
 \count@=\@ne \edef\next@{\the\count@}%
 \ifx\next@\s@top\DN@{\xy@spline@iv}\else\DN@{\xy@spline@iii}\fi 
 \next@ }
\xylet@\xy@spline@ii@@=\xy@spline@ii
\xydef@\xy@spline@iii{\crv@cnt@=\s@top 
 \loop \advance\crv@cnt@\m@ne \xy@spline@g \ifnum\crv@cnt@>\@ne\repeat
 \xy@spline@iv}
\xydef@\xy@spline@g{\cfromid@{@c}\idfromc@{@p}%
 \count@@=\crv@cnt@\cfroms@{\count@@}\idfromc@{@m}%
 \enter@\cplusthec@ \count@@=\crv@cnt@ \advance\count@@\m@ne
 \cfroms@{\count@@}\leave@
 \halve@dimen\X@c
 \halve@dimen\Y@c
 \czeroEdge@\idfromc@{@c}%
 \expandafter\doSplineSegment@\expandafter{\splineSTYLE@}}
\xydef@\xy@spline@iv{\cfromid@{@c}\idfromc@{@p}%
 \cfroms@{\z@}\idfromc@{@m}\leave@ \save@
 \enter@\cplusthec@ \cfromid@{@m}\leave@
 \halve@dimen\X@c
 \halve@dimen\Y@c
 \czeroEdge@\idfromc@{@c}%
 \expandafter\doSplineSegment@\expandafter{\splineSTYLE@}%
 \xy@spline@v }
\xydef@\xy@spline@v{\cfromid@{@c}\idfromc@{@p}%
 \leave@ \save@ \idfromc@{@c}%
 \expandafter\doSplineStraight@\expandafter{\splineSTYLE@}%
 \xy@spline@x }
\xydef@\xy@spline@x{\leave@ 
 \def\Drop@@{\splineDrop@ \resetbreaks@}%
 \def\Connect@@{\straight@\relax\splineConnect@ \resetbreaks@}%
 \OBJECT@x}
\xydef@\splineDrop@{\ifInvisible@\setboxz@h{}%
 \else\setboxz@h{\kern-\the\X@c\raise-\the\Y@c\hbox{\styledboxz@}}\fi
 \wdz@=\z@ \ht\z@=\z@ \dp\z@=\z@ \boxz@ }
\xydef@\splineConnect@{%
 \ifInvisible@\else\box\lastobjectbox@\fi }%
\xydef@\doSplineStraight@#1{\begingroup \sinit@
 \cfromid@{@p}\pfromc@\cfromid@{@c}%
 \connect@\crvs{#1}\relax\sleave@\endgroup }
\xydef@\doSplineSegment@#1{\begingroup \sinit@
 \cfromid@{@p}\pfromc@\senter@\cfromid@{@m}\spushc@\cfromid@{@c}%
 \connect@\crvs{#1}\relax\sinit@\sleave@\endgroup }
\xyendinput


==> xydummy.tex <==
%% xydummy.tex from $Id: xydummy.doc,v 3.3 1996/12/19 03:31:56 krisrose Exp $
%%
%% Xy-pic ``Dummy'' option.
%% Copyright (c) 1993-1996 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1996 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{dummy}{Dummy option}{\stripRCS$Revision: 3.3 $}%
 {Kristoffer H.~Rose}{krisrose@brics.dk}%
 {BRICS/Computer Science, University of Aarhus, Ny Munkegade, building 540,
 DK--8000 Aarhus~C}
\xynew@{count}\xydummyrequires@@
\xyeveryrequest{dummy}{\global\advance\xydummyrequires@@\@ne
 \W@{The `dummy' option was used \the\xydummyrequires@@\space times!}}
\xyendinput


==> xydvidrv.tex <==
%% xydvidrv.tex from $Id: xydvidrv.doc,v 3.3 1996/12/18 09:12:40 ross Exp $
%%
%% Xy-pic ``dvidrv-driver'' option.
%% Copyright (c) 1995-1996 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1996 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{dvidrv}{dvidrv driver}{\stripRCS$Revision: 3.3 $}%
 {Ross Moore}{ross@mpce.mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xydef@\dvidrv@@#1{\dvimessage@{dvidrv}{#1}}
\newdriver{%
 \xyaddsupport{emtex}\dvidrvEmTeX@@
 \xyaddsupport{line}\dvidrvLine@@
}
\xydef@\dvidrvEmTeX@@{\dvidrvEmTeX@}%
\xydef@\dvidrvEmTeX@{\setupxyEMTeX@}%
\xydef@\dvidrvLine@@{\dvidrvLine@}%
\xydef@\dvidrvLine@{\xywithoption{emtex}{\installEMline@}}%
\xyendinput


==> xydvips.tex <==
%% xydvips.tex from $Id: xydvips.doc,v 3.3 1996/12/18 09:13:14 ross Exp $
%%
%% Xy-pic ``dvips-driver'' option.
%% Copyright (c) 1995-1996 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1996 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{dvips}{DVIPS driver}{\stripRCS$Revision: 3.3 $}%
 {Ross Moore}{ross@mpce.mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xydef@\dvips@@#1{\dvimessage@{dvips}{#1}}
\newdriver{%
 \xyaddsupport{color}\dvipsColor@@
 \xyaddsupport{crayon}\dvipsCrayola@@
 \xyaddsupport{ps}\dvipsPS@@
 \xyaddsupport{rotate}\dvipsRotate@@
 \xyaddsupport{line}\dvipsLine@@
 \xyaddsupport{frame}\dvipsFrames@@
 \xyaddsupport{tile}\dvipsTiles@@
 \xyaddsupport{tpic}\dvipsTPIC@ 
 \xyaddsupport{emtex}\dvipsEM@
 \xyaddsupport{cmtip}\relax
}
\xydef@\dvips@Color@{\dvipsPStypes@ 
 \let\xylocalColor@=\xystackcolor@ 
 \let\xycolor@push\xycolor@push@@
 \def\xycolor@{\xycolor@@}\let\xycolorwarning@=\relax
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-c}{\xydrivernoload@{ps-c}}\installPScolor@ }%
 \else\DN@{}\fi \next@ 
 \ifx\xycolor@@\xyNoColor@ \let\xycolor@@=\xycolor@raw@@\fi
 \ifx\xycrayolaloaded\empty \DN@{\xystandardcolors@\dvipsCrayola@{}}%
 \else \DN@{\xystandardcolors@}\fi \next@
 \let\dvipsColor@@=\relax
 \let\UnloadColor@@=\NoDVIPScolor@
 }%
\xydef@\dvipsColor@@{\dvips@Color@}
\xydef@\NoDVIPScolor@{%
 \def\xycolor@{\xycolor@@}%
 \let\xycolor@@=\xyNoColor@
 \let\xylocalColor@=\xyNoColor@@
 \let\xycolorwarning@=\xycolorwarning@@
 \let\dvipsColor@@=\dvips@Color@
 \let\UnloadColor@@=\UnloadColor@
 }
\xydef@\NoDVIPScolordvi@{\xywarning@{%
 Neither colordvi.tex nor colordvi.sty could be found.}%
 \xyBEcolorcheck@}%
\xydef@\dvipsCrayola@@{\dvipsColor@@\dvipsCrayola@}
\xydef@\dvipsCrayola@{%
 \let\prevxycolor@=\newxycolor@
 \def\newxyDVIPScolor@##1##2##3{\prevxycolor@{##1}{}{##1}}%
 \let\newxycolor@=\newxyDVIPScolor@ \dvipsInclude@{color.pro}%
 \installCrayolaColors@
 \let\newxycolor@=\prevxycolor@ }%
\xydef@\dvipsPS@@{\dvipsPS@}
\xydef@\dvipsPS@unload{\UnloadPS@
 \let\UnloadPS@@=\UnloadPS@
 \let\dvipsPS@@=\dvipsPS@ }
\xydef@\dvipsPStypes@{%
 \xyinputorelse@{xyps-ps}{\xydrivernoload@{ps-ps}}%
 \ifx\PSspecial@@\dvipsSpecial@\else
 \let\PSspecial@@=\dvipsSpecial@
 \let\PSmacro@@=\dvipsMacro@
 \let\PSdict@@=\dvipsDict@
 \let\PSspecialdict@@=\dvipsDict@
 \let\PSraw@@=\dvipsRaw@
 \let\PSinclude@@=\dvipsInclude@
 \let\xyPSobeylines@@=\obeyDVIPSlines@
 \let\xyPScurrpt@@=\dvipsCurrpt@@
 \dvips@@{PostScript}%
 \fi
 \XYpredict@ }
\xywarnifdefined\dvipsSpecial@
\xywarnifdefined\dvipsMacro@
\xywarnifdefined\dvipsDict@
\xywarnifdefined\dvipsInclude@
\xywarnifdefined\dvipsRaw@
{\catcode`\"=11 \catcode`\!=11 \catcode`\:=11
 \gdef\dvipsSpecial@#1{\special{ps:: SDict begin #1 end}}
 \gdef\dvipsMacro@#1{\firstPS@@\special{" {#1}xy}}
 \gdef\dvipsDict@#1{\special{! #1}}
 \gdef\dvipsInclude@#1{\special{header=#1}}
 \gdef\dvipsRaw@#1{\special{ps: SDict begin #1 end}}
\catcode`\^^M=\active
 \gdef\next{\catcode`\^^M=\active \let^^M=\space }}%
\xylet@\obeyDVIPSlines@=\next
\xydef@\dvipsCurrpt@{\let\xyPScurrpt@@=\dvipsCurrpt@@}%
\xydef@\dvipsCurrpt@@{\PSraw@@{xyp}}
\xydef@\dvipsPS@{\dvipsPStypes@ 
 \let\dvipsPS@@=\PSspecials@true
 \let\UnloadPS@@=\dvipsPS@unload 
 \let\installxyps@@=\relax \installxyps@ }
\xydef@\dvipsRotate@@{\dvipsRotate@}
\xydef@\dvipsRotate@{\dvipsPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-r}{\xydrivernoload@{ps-r}}%
 \dvipsCurrpt@ \dvipsRotScale@ \installPSrotscale@ }%
 \else\DN@{\xydriverfail@{rotations are}UnloadRotate@\relax}\fi
 \next@ }
\xydef@\dvipsRotScale@{%
 \def\xyrot@start(##1){{xyct ##1\space xyrs }}%
 \def\xyrot@end{}%
 \def\xyscale@start(##1,##2){{xyct ##1\space##2\space xyss }}%
 \def\xyscale@end{}}
\xydef@\dvipsLine@@{\dvipsLine@}
\xydef@\dvipsLine@{\dvipsPStypes@ 
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-l}{\xydrivernoload@{ps-l}}\installPSline@ }%
 \else\DN@{\xydriverfail@{line-widths are}\UnloadLine@\relax}\fi
 \next@ }
\xydef@\dvipsFrames@@{\dvipsFrames@}
\xydef@\dvipsFrames@{\dvipsPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-f}{\xydrivernoload@{ps-f}}\installPSframes@ }%
 \else\DN@{\xydriverfail@{frames are}\UnloadFrames@\relax}\fi
 \next@ }
\xydef@\dvipsTiles@@{\dvipsTiles@}
\xydef@\dvipsTiles@{\dvipsPStypes@ 
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-t}{\xydrivernoload@{ps-t}}\installPSpatterns@ }%
 \else\DN@{\xydriverfail@{Patterns are}\UnloadPSpatterns@\relax}\fi
 \next@ }
\xydef@\dvipsTPIC@@{\dvipsTPIC@}
\xydef@\dvipsTPIC@{\setupxyTPIC@}
\xydef@\dvipsEM@@{\dvipsEM@}
\xydef@\dvipsEM@{\setupxyEMTeX@}
\xyendinput


==> xydvitops.tex <==
%% xydvitops.tex from $Id: xydvitops.doc,v 3.3 1996/12/18 09:14:36 ross Exp $
%%
%% Xy-pic ``DVITOPS-driver'' option.
%% Copyright (c) 1995-1996 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1996 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{dvitops}{DVITOPS driver}{\stripRCS$Revision: 3.3 $}%
 {Ross Moore}{ross@mpce.mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xydef@\dvitops@@#1{\dvimessage@{DVITOPS}{#1}}
\newdriver{%
 \xyaddsupport{color}\dvitopsColor@@
 \xyaddsupport{crayon}\dvitopsCrayon@@
 \xyaddsupport{ps}\dvitopsPS@@
 \xyaddsupport{rotate}\dvitopsRotate@@
 \xyaddsupport{line}\dvitopsLine@@
 \xyaddsupport{frame}\dvitopsFrames@@
 \xyaddsupport{tile}\dvitopsTiles@@
 \xyaddsupport{cmtip}\relax
}
\xydef@\dvitopsColor@@{\dvitops@Color@}
\xydef@\dvitops@Color@{\dvitopsPStypes@ 
 \let\xylocalColor@=\xyDVITOPScolor@ 
 \let\xycolor@push\xycolor@push@@
 \def\xycolor@{\xycolor@@}\let\xycolorwarning@=\relax
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-c}{\xydrivernoload@{ps-c}}\xycatcodes
 \installPScolor@ }\else\DN@{}\fi \next@
 \ifx\xycolor@@\xyNoColor@ \let\xycolor@@=\xycolor@raw@@\fi
 \ifx\xycrayolaloaded\empty \DN@{\xystandardcolors@\dvitopsCrayon@{}}%
 \else\let\next@=\xystandardcolors@
 \fi \next@
 \let\dvitops@Color@@=\relax
 \let\UnloadColor@@=\NoDVITOPScolor@
 }%
\xydef@\NoDVITOPScolor@{%
 \def\xycolor@{\xycolor@@}%
 \let\xycolor@@=\xyNoColor@
 \let\xylocalColor@=\xyNoColor@@
 \let\xycolorwarning@=\xycolorwarning@@
 \let\dvitops@Color@@=\dvitops@Color@
 }
\xydef@\xyDVITOPScolor@{\bgroup \DN@##1##2{\egroup}%
 \ifInvisible@\else\ifHidden@\else\DNii@{\no@@}\ifx\nextii@\Connect@@ 
 \else\DN@{\xyDVITOPScolor@i}\fi\fi\fi \next@ }
\xydef@\xyDVITOPScolor@i#1#2{\checkXyStyle@ 
 \DN@{#2}\ifx\next@\empty
 \def\tmp@##1{\DN@{\xycolor@begin##1\xycolor@end{#1}}}%
 \else\DNii@{gray}\ifx\next@\nextii@
 \def\tmp@##1{\DN@{\xycolor@begin##1\xycolor@end{gray}{#1}}}%
 \else\DNii@{rgb}\ifx\next@\nextii@
 \def\tmp@##1{\DN@{\xycolor@begin##1\xycolor@end{rgbcolor}{#1}}}%
 \else\DNii@{hsb}\ifx\next@\nextii@
 \def\tmp@##1{\DN@{\xycolor@begin##1\xycolor@end{hsbcolor}{#1}}}%
 \else \DN@{\xywarning@{DVITOPS cannot support color: #2 #1}}%
 \fi\fi\fi\fi
 \toks@={\egroup \let\xy@style@=\relax \def\Drop@@}%
 \expandafter\tmp@\expandafter{\Drop@@}%
 \expandafter\addtotoks@\expandafter{\expandafter{\next@}\def\Connect@@}%
 \expandafter\tmp@\expandafter{\Connect@@}%
 \expandafter\addtotoks@\expandafter{\expandafter{\next@}}%
 \the\toks@ }%
\xydef@\xycolor@begin{\dvitopsBegin@{color}}
\xydef@\xycolor@end{\dvitopsEnd@{color}\dvitopsColor@x}
\xydef@\dvitopsCrayon@@{\dvitopsColor@@\dvitopsCrayon@}
\xydef@\dvitopsCrayon@{\installCrayolaColors@}%
\xydef@\dvitopsPS@@{\dvipsPS@}
\xydef@\dvitopsPS@unload{\UnloadPS@
 \let\UnloadPS@@=\UnloadPS@
 \let\dvitopsPS@@=\dvitopsPS@ }
\xydef@\dvitopsPStypes@{%
 \xyinputorelse@{xyps-ps}{\xydrivernoload@{ps-ps}}%
 \ifx\PSspecial@@\dvitopsSpecial@\else
 \let\PSspecial@@=\dvitopsSpecial@
 \let\PSmacro@@=\dvitopsMacro@
 \let\PSdict@@=\dvitopsDict@
 \let\PSspecialdict@@=\dvitopsDict@
 \let\PSraw@@=\dvitopsRaw@
 \let\PSinclude@@=\dvitopsInclude@
 \let\xyPSobeylines@@=\obeyDVIPSlines@
 \let\xyPScurrpt@@=\dvitopsCurrpt@@
 \dvitops@@{PostScript}%
 \fi
 \XYpredict@ }
\xywarnifdefined\dvitopsSpecial@
\xywarnifdefined\dvitopsMacro@
\xywarnifdefined\dvitopsDict@
\xywarnifdefined\dvitopsInclude@
\xywarnifdefined\dvitopsRaw@
\xywarnifdefined\dvitopsOrigin@
\xywarnifdefined\dvitopsBegin@
\xywarnifdefined\dvitopsEnd@
\xywarnifdefined\dvitopsRotate@x
\xywarnifdefined\dvitopsTransform@x
\xywarnifdefined\dvitopsColor@x
{\catcode`\:=11
 \gdef\dvitopsSpecial@#1{\special{dvitops: inline #1}}
 \gdef\dvitopsMacro@#1{\special{dvitops: inline {#1}xy}}
 \gdef\dvitopsDict@#1{\special{dvitops: inline #1}}
 \gdef\dvitopsInclude@#1{\special{dvitops: prolog #1}}
 \gdef\dvitopsRaw@#1{\special{dvitops: inline #1}}
 \gdef\dvitopsOrigin@#1{\special{dvitops: origin #1}}
 \gdef\dvitopsBegin@#1{\special{dvitops: begin #1}}
 \gdef\dvitopsEnd@#1{\special{dvitops: end #1}}
 \gdef\dvitopsRotate@x#1{\special{dvitops: rotate #1}}
 \gdef\dvitopsTransform@x#1{\special{dvitops: transform #1}}
 \gdef\dvitopsColor@x#1#2{\special{dvitops: #1 color #2}}
}
\catcode`\^^M=\active
 \gdef\next{\catcode`\^^M=\active \let^^M=\space }}%
\xylet@\obeyDVIPSlines@=\next
\xydef@\dvitopsCurrpt@{\global\let\xyPScurrpt@@=\relax}%
\xydef@\dvitopsPS@{\dvitopsPStypes@ 
 \let\installxyps@@=\relax \installxyps@ }
\xydef@\dvitopsRotate@@{\dvitopsRotate@}
\xydef@\dvitopsRotate@{\dvitopsPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty
 \DN@{\xyinputorelse@{xyps-r}{\xydrivernoload@{ps-r}}%
 \installDVITOPSrotate@ }%
 \else\DN@{\xydriverfail@{rotations are}\UnloadRotate@\relax}\fi
 \next@ }
\xydef@\dvitopsRotScale@{%
 \def\xyrot@start{\dvitopsBegin@{rot}\dvitopsOrigin@{rot}}%
 \def\xyrot@end(##1){\dvitopsEnd@{rot}\dvitopsRotate@x{##1}}%
 \def\xyscale@start{\dvitopsBegin@{scal}\dvitopsOrigin@{scal}}%
 \def\xyscale@end(##1,##2){%
 \dvitopsEnd@{scal}\dvitopsTransform@x{##1 0 ##2 0}}%
 }
\xydef@\installDVITOPSrotate@{\installPSstyle@
 \let\xyRotate@@=\dvitopsRotate@
 \let\doSpecialRotate@@=\dvitopsSpecialRotate@
 \let\xyscale@@=\dvitopsScale@
 \dvitopsCurrpt@
 \dvitopsRotScale@ \xyPSshapes@true }
\xydef@\UnloadDVITOPSrotate@{\UnloadRotate@\relax}
 \xydef@\dvitopsRotate@#1{\xyPSsplitPS@
 {\dvitopsBegin@{rot}\dvitopsOrigin@{rot}}%
 {\dvitopsEnd@{rot}\dvitopsRotate@x{#1}}}%
 \xydef@\dvitopsScale@#1#2{\xyPSsplitPS@
 {\dvitopsBegin@{scal}\dvitopsOrigin@{scal}}%
 {\dvitopsEnd@{scal}\dvitopsTransform@x{#1 0 #2 0}}}
 \xydef@\dvitopsSpecialRotate@#1@@{\dvitopsRotate@{#1}}
\xydef@\dvitopsLine@@{\dvitopsLine@}
\xydef@\dvitopsLine@{\dvitopsPStypes@ 
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-l}{\xydrivernoload@{ps-l}}\installPSline@ }%
 \else\DN@{\xydriverfail@{line-widths are}\UnloadLine@\relax}\fi
 \next@ }
\xydef@\dvitopsFrames@@{\dvitopsFrames@}
\xydef@\dvitopsFrames@{\dvitopsPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-f}{\xydrivernoload@{ps-f}}\installPSframes@ }%
 \else\DN@{\xydriverfail@{frames are}\UnloadFrames@\relax}\fi
 \next@ }
\xydef@\dvitopsTiles@{\dvitopsPStypes@ 
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-t}{\xydrivernoload@{ps-t}}\installPSpatterns@ }%
 \else\DN@{\xydriverfail@{Patterns are}\UnloadPSpatterns@\relax}\fi
 \next@ }
\xydef@\dvitopsTPIC@@{\dvitopsTPIC@}
\xydef@\dvitopsTPIC@{\setupxyTPIC@}
\xyendinput


==> xyemtex.tex <==
%% xyemtex.tex from $Id: xyemtex.doc,v 3.3 1996/12/18 09:18:00 ross Exp $
%%
%% Xy-pic ``em-TeX'' back-end extension.
%% Copyright (c) 1995-1996 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1996 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{emtex}{em-TeX backend}{\stripRCS$Revision: 3.3 $}%
 {Ross Moore}{ross@mpce.mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xynew@{if}\ifEMspecials@
\xydef@\UseEMspecials{\EMspecials@true}
\xydef@\NoEMspecials{\EMspecials@false}
\xydef@\xyemtex@lineto{\xyEM@special{lineto}} 
\xydef@\xyemtex@moveto{\xyEM@special{moveto}} 
\xydef@\xyemtex@line#1{\xyEM@special{line #1}} 
\xydef@\xyemtex@point#1{\xyEM@special{point #1}} 
\xydef@\xyemtex@pen#1{\addtostyletoks@{\xyEM@special{linewidth #1}}}
{\catcode`:=12 \gdef\next#1{\special{em:#1}}}
\xylet@\xyEM@special=\next
{\catcode`:=12 \gdef\next#1{%
 \W@{EM:#1 (\the\X@p,\the\Y@p),(\the\X@c,\the\Y@c)}\special{em:#1}}}
\xylet@\xyEM@noisy=\next
\xydef@\NoisyEMTeX{\let\xyEM@special=\xyEM@noisy}
\xydef@\EMalternative@#1#2{%
\expandafter\global\expandafter\let\csname origxy#2@\endcsname=#1%
 \xdef#1{\noexpand\ifEMspecials@
 \noexpand\expandafter\expandafter\noexpand\csname xyemtex@#2@\endcsname
 \noexpand\else
 \noexpand\expandafter\expandafter\noexpand\csname origxy#2@\endcsname
 \noexpand\fi}}%
\xydef@\setupxyEMTeX@{\xywarning@{using em-TeX specials}%
 \EMalternative@{\solid@}{solid}%
 \EMalternative@{\splinesolid@}{splinesolid}%
 \let\setupxyEM@=\reloadxyEM@ 
 \activateEM@ }
\xydef@\xyunloadEM@{\xywarning@{EM specials turned off}%
 \xywithoption{line}{\xysetup@@\uninstallEMline@ }%
 \EMspecials@false
 \let\setupxyEM@=\reloadxyEM@ }
\xydef@\activateEM@{%
 \xywithoption{line}{\xysetup@@\installEMline@}%
 \EMspecials@true }
\xydef@\reloadxyEM@{\xywarning@{EM specials back on}\activateEM@ }
\xydef@\xyemtex@solid@{%
 \ifInvisible@ \let\next@=\no@@
 \else \DN@{\xyEMstraight@}\fi
 \next@ }
\xydef@\xyEMstraight@{\setupDirection@
 \edef\Creset@@{\cfromthec@ \pfromthep@ \DirectionfromtheDirection@}%
 \DN@##1##2{\def\checkoverlap@@{%
 \ifdim##1\X@p>##1\X@c \let\next@=\relax \fi
 \ifdim##2\Y@p>##2\Y@c \let\next@=\relax \fi}}%
 \edef\nextii@{{\sd@X}{\sd@Y}}\expandafter\next@\nextii@
 \noCshavep@@ \edef\Cshavep@@{\pfromthep@ \noexpand\resetDirection@}%
 \noCshavec@@ \edef\Cshavec@@{\cfromthec@ \noexpand\resetDirection@}%
 \ifHidden@\else
 \ifdim\Y@c>\Y@max \Y@max=\Y@c \fi \ifdim\Y@p>\Y@max \Y@max=\Y@p \fi
 \ifdim\Y@c<\Y@min \Y@min=\Y@c \fi \ifdim\Y@p<\Y@min \Y@min=\Y@p \fi
 \ifdim\X@c>\X@max \X@max=\X@c \fi \ifdim\X@p>\X@max \X@max=\X@p \fi
 \ifdim\X@c<\X@min \X@min=\X@c \fi \ifdim\X@p<\X@min \X@min=\X@p \fi \fi
 \ifInvisible@\let\next@=\relax \else
 \DN@{%
 \setboxz@h{\kern\X@p \raise\Y@p\hbox{\xyemtex@moveto}}%
 \ht\z@=\z@ \wd\z@=\z@ \dp\z@=\z@
 \setboxz@h{\boxz@ \kern\X@c \raise\Y@c\hbox{\xyemtex@lineto}}%
 \ht\z@=\z@ \wd\z@=\z@ \dp\z@=\z@ {\Drop@@}}%
 \fi 
 \checkoverlap@@
 \ifdim\d@X=\z@ \ifdim\d@Y=\z@ \DN@{\relax}\fi\fi \next@
 \def\Cslidep@@{\noCslidep@@}\def\Cslidec@@{\noCslidec@@}%
 \def\Calong@@{\noCalong@@}\Creset@@ }
\xydef@\xyemtex@splinesolid@{\setbox\splinebox@=\copy\voidb@x 
 \multiply\splinetol@\thr@@ 
 \gdef\splineextra@@{\xyemtex@moveto\gdef\splineextra@@{\xyemtex@lineto}}%
 \def\xycrvdrop@{ }\def\xycrvconn@{}\splineset@@ }
\xydef@\xyEMlinewidth@#1{\dimen@=#1\relax\edef\next@{\the\dimen@}}
\xydef@\installEMline@{%
 \let\xylinewidth@@=\xylinewidth@
 \let\xylineSpecial@@=\xyemtex@pen
 \let\transxyline@@=\xyEMlinewidth@ }
\xydef@\uninstallEMline@{\UnloadLine@\relax}%
\xydef@\UseEMlinewidth{\installEMline@}%
\xydef@\NoEMlinewidth{\uninstallEMline@}%
\xyendinput


==> xyframe.tex <==
%% xyframe.tex from $Id: xyframe.doc,v 3.7 1999/02/16 15:12:50 krisrose Exp $
%%
%% Xy-pic ``Frames and Brackets'' extension.
%% Copyright (c) 1991-1997 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1997 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{frame}{Frame and Bracket extension}{\stripRCS$Revision: 3.7 $}%
 {Kristoffer H.~Rose}{krisrose@brics.dk}%
 {BRICS/Computer Science, University of Aarhus, Ny Munkegade, building 540,
 DK--8000 Aarhus~C}
\xydef@\frm{\hbox{}\dimen@=\L@c \advance\dimen@\R@c \wdz@=\dimen@
 \ht\z@=\U@c \dp\z@=\D@c \dimen@=\U@c \advance\dimen@\D@c
 \ifdim\wdz@=\z@ \def\Leftness@{.5}\else \quotient@\Leftness@\L@c\wdz@ \fi
 \ifdim\dimen@=\z@ \def\Upness@{.5}\else \quotient@\Upness@\U@c\dimen@ \fi
 \expandafter\Edge@c\expandafter{\prevEdge@@}\let\frmradius@@=\z@
 \def\Drop@@{}%
 \def\Connect@@{\xy@@{\save@\cmerge@\Y@p\X@p\D@p\U@p\L@p\R@p\Drop@@}\restore}%
 \xyFN@\frm@i}
\xylet@\frmradius@@=\z@
\xydef@\frm@i{%
 \addLT@\ifx\next \addGT@{\addLT@\DN@##1}{\def\frmradius@@{##1}\xyFN@\frm@i}%
 \else \DN@##1##{\frm@{##1}}\fi \next@}
\xydef@\frm@#1#2{\DNii@{frm#1{#2}}%
 \expandafter\let\expandafter\next@\csname\codeof\nextii@\endcsname
 \ifx\next@\relax \DNii@{frm{#2}}%
 \expandafter\let\expandafter\next@\csname\codeof\nextii@\endcsname
 \ifx\next@\relax \let\next@=\frm@generic \fi\fi \next@}
\xydef@\frm@generic{\xyerror@{No generic frames yet!}{}}
\xydef@\frmDrop@#1{%
 \ifx\frmradius@@\z@ \addtoDrop@@{\let\frmradius@@=\z@ #1}%
 \else \expandafter\addtoDrop@@\expandafter{%
 \expandafter\def\expandafter\frmradius@@\expandafter{\frmradius@@}#1}\fi}
\xydef@\EdgefromtheEdge@{%
 \U@c=\the\U@c \D@c=\the\D@c \L@c=\the\L@c \R@c=\the\R@c
 \Edge@c={\expandafter\noexpand\the\Edge@c}}
\xydef@\prevEdgefromtheEdge@{%
 \U@c=\the\U@c \D@c=\the\D@c \L@c=\the\L@c \R@c=\the\R@c
 \noexpand\def\noexpand\prevEdge@@{\expandafter\noexpand\the\Edge@c}}
\xydef@\addtoDrop@@#1{%
 \expandafter\def\expandafter\Drop@@\expandafter{\Drop@@#1}}
\xydef@\addbeforeDrop@@#1{\DNii@{#1}%
 \expandafter\DN@\expandafter{\expandafter\nextii@\Drop@@}%
 \expandafter\expandafter\expandafter\def
 \expandafter\expandafter\expandafter\Drop@@
 \expandafter\expandafter\expandafter{\next@}}
\xydefcsname@{frm{}}{}
\xyletcsnamecsname@{frm[]{}}{frm{}}
\xyletcsnamecsname@{frm[o]{}}{frm{}}
\xydefcsname@{frm{.}}{\frmDrop@{\let\zerocorner=\framezerodot@@
 \let\framehfill=\frm@doth@@ \let\framevfill=\frm@dotv@@
 \framed@@{\frmradius@@}}}
\xyletcsnamecsname@{frm[]{.}}{frm{.}}
\xydef@\frm@doth@@{\setboxz@h{\kern5\B@\framezerodot@@\kern5\B@}\ht\z@=\B@
 \dp\z@=\B@\kern5\B@\xleaders\boxz@\hss\kern5\B@}
\xydef@\frm@dotv@@{\setboxz@h to2\B@{\hss\framezerodot@@\hss}\ht\z@=5\B@
 \dp\z@=5\B@\kern5\B@\xleaders\boxz@\vss\kern5\B@}
\xyletcsnamecsname@{frm{..}}{frm{.}}
\xylet@\framezerodot@@=\zerodot
\xydefcsname@{frm{-}}{\frmDrop@{\framed@\frmradius@@}}
\xyletcsnamecsname@{frm[]{-}}{frm{-}}
\xydef@\framed@{\let\zerocorner=\framezerodot@@
 \let\framehfill=\frm@solidh@@ \let\framevfill=\frm@solidv@@ \framed@@}
\xylet@\framesetthick@=\relax
\xydef@\frm@solidh@@{\framesetthick@\leaders\hrule height\B@ depth\B@\hfill}
\xydef@\frm@solidv@@{\framesetthick@\leaders\vrule width2\B@\vfill}
\xydefcsname@{frm{=}}{\frmDrop@{\framed@\frmradius@@
 {\advance\L@c-2\p@ \advance\R@c-2\p@ \advance\U@c-2\p@ \advance\D@c-2\p@
 \dimen@=\frmradius@@
 \ifdim\dimen@>2\p@ \advance\dimen@-2\p@ \else \dimen@=\z@\fi
 \framed@\dimen@}}}
\xyletcsnamecsname@{frm[]{=}}{frm{=}}
\xydef@\framesetthick@line{\B@=.5\xylinethick@}
\xydef@\frm@thickc@@{\hbox{\framesetthick@line
 \vrule height.5\B@ depth.5\B@ width\B@}}
\xywithoption{line}{%
 \let\framezerodot@@\frm@thickc@@ \let\framesetthick@=\framesetthick@line}
\xydef@\framed@@#1{\setboxz@h{\R@=#1\relax 
 \dimen@=\L@c \advance\dimen@\R@c \dimen@ii=\U@c \advance\dimen@ii\D@c
 \ifdim.5\dimen@<\R@ \R@=.5\dimen@ \fi
 \ifdim.5\dimen@ii<\R@ \R@=.5\dimen@ii \fi
 \A@=\X@c \advance\A@-\L@c \B@=\Y@c \advance\B@-\D@c
 \ifdim\R@<\p@\else \cirrestrict@@ \fi
 \dimen@=2\R@ \advance\dimen@-\L@c \advance\dimen@-\R@c
 \ifdim\dimen@>\z@ \advance\A@-.5\dimen@ \fi
 \dimen@=2\R@ \advance\dimen@-\U@c \advance\dimen@-\D@c
 \ifdim\dimen@>\z@ \advance\B@-.5\dimen@ \fi
 \kern\A@ \raise\B@\vbox to \dimen@ii{\framed@body@@}}%
 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \boxz@}
\xydef@\framed@body@{%
 \advance\dimen@ii.22\p@ \advance\dimen@-.2\p@ 
 \setboxz@h{\corn@@4\R@}\A@=-.5\wdz@ \B@=.5\xydashw@
 \dimen@=\L@c \advance\dimen@\R@c \advance\dimen@-.2\p@
 \setboxz@h to\dimen@{\kern\A@ \boxz@ \framehfill\corn@@3\R@\kern\A@}%
 \advance\dimen@ii-\dp\z@ \kern-\ht\z@ \nointerlineskip\boxz@
 \dimen@=\L@c \advance\dimen@\R@c \advance\dimen@-.2\p@
 \setboxz@h to\dimen@{\kern\A@\corn@@1\R@\framehfill\corn@@2\R@\kern\A@}%
 \advance\dimen@ii-\ht\z@
 \dimen@=\L@c \advance\dimen@\R@c \advance\dimen@.2\p@
 \nointerlineskip\hbox to\dimen@{%
 \setbox\z@=\vbox to\dimen@ii{\framevfill}\kern-.5\wdz@\copy\z@
 \hss \copy\z@\kern-.5\wdz@ }%
 \nointerlineskip\boxz@ \vss \kern\z@}
\xylet@\framed@body@@=\framed@body@
\xylet@\zerocorner=\framezerodot@@
\xydef@\solidcorner@#1#2{\hbox\bgroup \R@=#2\relax
 \ifdim\R@<\p@ \zerocorner
 \else \cirrestrict@@ \multiply\count@8
 \setboxz@h{\corn@x@@{#1}}\dimen@=\wdz@
 \ifcase#1\or \ht\z@=\z@ \kern\dimen@ \raise\dimen@\boxz@ 
 \or \ht\z@=\z@ \raise\dimen@\boxz@ \kern\dimen@
 \or \dp\z@=\z@ \lower\dimen@\boxz@ \kern\dimen@
 \or \dp\z@=\z@ \kern\dimen@ \lower\dimen@\boxz@ \fi
 \vrule height\dimen@ depth\dimen@ width\z@\fi
 \edef\tmp@{\egroup \U@c=\the\dimen@}\tmp@ \D@c=\U@c \L@c=\U@c \R@c=\U@c
 \Edge@c={\circleEdge}\ignorespaces}
\xydef@\corn@x@#1{\ifcase#1\or
 \circhar@@\z@ \circhar@@\@ne\or\circhar@@\tw@ \circhar@@3\or
 \circhar@@5\circhar@@4\or\circhar@@7\circhar@@6\fi}
\xylet@\corn@x@@=\corn@x@
\xydef@\corn@@{\DN@{\solidcorner@}%
 \ifx\framehfill\frm@doth@@ \DN@{\let\cirrestrict@@=\relax
 \let\corn@x@@=\dotcorner@@ \let\zerodot=\framezerodot@@
 \solidcorner@ }%
 \else\ifx\framehfill\frm@dashh@@ \DN@{\let\cirrestrict@@=\relax
 \let\corn@x@@=\dashcorner@@ \let\zerodot=\framezerodot@@
 \solidcorner@ }%
 \fi\fi \next@}
\xydef@\dotcorner@@#1{\zerocorner}
\xydef@\dashcorner@@#1{\zerocorner}
\xywithoption{curve}{%
 \let\dotcorner@@=\dotcorner@ \let\dashcorner@@=\dashcorner@}
\xydefcsname@{frm{--}}{%
 \frmDrop@{\let\zerocorner=\framezerodot@@ 
 \let\framehfill=\frm@dashh@@ \let\framevfill=\frm@dashv@@
 \framed@@\frmradius@@}}
\xyletcsnamecsname@{frm[]{--}}{frm{--}}
\xydef@\frm@dashh@@{\setboxz@h{\dashhfillchar}%
 \ht\z@=\B@ \dp\z@=\B@ \wdz@=2\xydashl@
 \copy\z@ \xleaders\copy\z@\hss \boxz@\kern-\xydashl@}
\xydef@\frm@dashv@@{\setboxz@h to2\B@{\hss\dashvfillchar\hss}\ht\z@=\z@
 \dp\z@=2\xydashl@ \nointerlineskip\copy\z@ \xleaders\copy\z@\vss
 \nointerlineskip\boxz@\kern-\xydashl@}%
\xydef@\dashhfillchar{{\rDirection@\xydashl@ \line@@}}
\xydef@\dashvfillchar{{\dDirection@\xydashl@ \line@@}}
\xydefcsname@{frm{o-}}{%
 \ifdim\frmradius@@<2\xydashl@\relax \dimen@=.8\xydashl@
 \expandafter\def\expandafter\frmradius@@\expandafter{\the\dimen@}\fi
 \frmDrop@{\let\zerocorner=\framezerodot@@ 
 \let\framehfill=\frm@rddashh@@ \let\framevfill=\frm@rddashv@@
 \framed@@\frmradius@@}}%
\xydef@\frm@rddashh@@{\setboxz@h{\kern\xydashl@\dashhfillchar}%
 \ht\z@=\B@ \dp\z@=\B@ \copy\z@ \xleaders\copy\z@\hss \boxz@ \kern\xydashl@}
\xydef@\frm@rddashv@@{\ifdim\dimen@ii<2\xydashl@\else
 \setbox\z@=\vbox to2\xydashl@{\hbox to2\B@{\hss\dashvfillchar\hss}\vss}%
 \kern\xydashl@ \copy\z@ \xleaders\copy\z@\vss
 {\ifdim\dimen@ii<2\xydashl@\else\aftergroup\boxz@\fi}\fi}
\xydefcsname@{frm{,}}{%
 \ifx\frmradius@@\z@ \shaded@{1.2\p@}\else \shaded@\frmradius@@ \fi}
\xydef@\shaded@#1{\frmDrop@{\R@=#1\relax
 {\advance\X@c\R@ \advance\Y@c-\D@c \U@c=\z@ \D@c=\R@ \blacked@}%
 {\advance\X@c\R@c \advance\Y@c-\R@ \L@c=\z@ \R@c=\R@ \blacked@}}}
\xydefcsname@{frm{-,}}{\addtoDrop@@{\drop\frm{-}\drop\frm{,}}}
\xydef@\blacked@{\setboxz@h{%
 \A@=\X@c \advance\A@-\L@c \dimen@=\L@c \advance\dimen@\R@c
 \B@=\Y@c \advance\B@-\D@c \dimen@ii=\Y@c \advance\dimen@ii\U@c
 \advance\A@-.5\xydashw@
 \kern\A@ \blacked@@ }%
 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \boxz@}
\xydef@\bblacked@{\setboxz@h{%
 \dimen@=\L@c \advance\dimen@\R@c \B@=-\D@c \dimen@ii=\U@c
 \kern-\L@c \blacked@@ \kern-\dimen@ \kern\L@c}%
 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \boxz@}
\xydef@\blacked@@{\vrule width\dimen@ depth-\B@ height\dimen@ii}
\xydefcsname@{frm{o}}{%
 \ifx\frmradius@@\z@
 \frmDrop@{\dimen@=.5\L@c \advance\dimen@.5\R@c
 \let\framehfill=\frm@solidh@@ \let\framevfill=\frm@solidv@@
 \circled@\dimen@}%
 \else
 \frmDrop@{\let\framehfill=\frm@solidh@@
 \let\framevfill=\frm@solidv@@ \circled@\frmradius@@}%
 \fi}
\xydefcsname@{frm{oo}}{%
 \ifx\frmradius@@\z@
 \frmDrop@{\dimen@=.5\L@c \advance\dimen@.5\R@c
 \let\framehfill=\frm@solidh@@ \let\framevfill=\frm@solidv@@
 {\circled@\dimen@}\advance\dimen@-2.1\p@ \circled@\dimen@}%
 \else
 \frmDrop@{\dimen@=\frmradius@@
 \let\framehfill=\frm@solidh@@ \let\framevfill=\frm@solidv@@
 {\circled@\dimen@}\advance\dimen@-2.1\p@ \circled@\dimen@}%
 \fi}
\xydef@\circled@#1{\setboxz@h\bgroup \R@=#1\relax 
 \setboxz@h{\vbox{\circled@x@@}}%
 \A@=\X@c \advance\A@-.5\wd\z@
 \B@=\Y@c \advance\B@-.5\ht\z@ \advance\B@.5\dp\z@ \advance\B@.2\p@
 \edef\tmp@{\egroup\dimen@=\the\wdz@}%
 \kern\A@ \raise\B@\boxz@
 \tmp@ \divide\dimen@4 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \boxz@}
\xydef@\circled@x@{\hbox{\corn@@4\R@ \corn@@3\R@}%
 \nointerlineskip\hbox{\corn@@1\R@ \corn@@2\R@}}
\xylet@\circled@x@@=\circled@x@
\xydefcsname@{frm{.o}}{%
 \ifx\frmradius@@\z@ \frmDrop@{\let\framehfill=\frm@doth@@ 
 \dimen@=.5\L@c \advance\dimen@.5\R@c \circled@\dimen@}%
 \else
 \frmDrop@{\let\framehfill=\frm@doth@@ \circled@\frmradius@@}%
 \fi}
\xydefcsname@{frm{-o}}{%
 \ifx\frmradius@@\z@ \frmDrop@{\let\framehfill=\frm@dashh@@
 \dimen@=.5\L@c \advance\dimen@.5\R@c \circled@\dimen@}%
 \else
 \frmDrop@{\let\framehfill=\frm@dashh@@ \circled@\frmradius@@}%
 \fi}
\xydefcsname@{frm{e}}{\ellipse@whichfrm@\ellipsesolidframed@}%
\xydefcsname@{frm{.e}}{\ellipse@whichfrm@\ellipsedotframed@}%
\xydefcsname@{frm{-e}}{\ellipse@whichfrm@\ellipsedashframed@}%
\xydefcsname@{frm{ee}}{\ellipse@whichdblfrm@\ellipsesolidframed@}%
\xydefcsname@{frm2{.e}}{\ellipse@whichdblfrm@\ellipsedotframed@}%
\xydefcsname@{frm2{-e}}{\ellipse@whichdblfrm@\ellipsedashframed@}%
\xyletcsnamecsname@{frm[o]{-}}{frm{e}}
\xyletcsnamecsname@{frm[o]{=}}{frm{ee}}
\xyletcsnamecsname@{frm[o]{.}}{frm{.e}}
\xyletcsnamecsname@{frm[o]{--}}{frm{-e}}
\xydef@\ellipse@whichfrm@#1{%
 \ifx\frmradius@@\z@
 \frmDrop@{#1\dimen@=.5\L@c \advance\dimen@.5\R@c
 \dimen@ii=.5\U@c \advance\dimen@ii.5\D@c
 \edef\next@{\noexpand\ellipsed@{\the\dimen@}{\the\dimen@ii}}\next@ }%
 \else
 \frmDrop@{#1\expandafter\ellipsed@i@\frmradius@@,,@@}%
 \fi}
\xydef@\ellipse@whichdblfrm@#1{%
 \ifx\frmradius@@\z@
 \frmDrop@{#1\dimen@=.5\L@c \advance\dimen@.5\R@c
 \dimen@ii=.5\U@c \advance\dimen@ii.5\D@c
 \edef\next@{\noexpand\ellipsed@e@{\the\dimen@}{\the\dimen@ii}}\next@ }%
 \else
 \frmDrop@{#1\expandafter\ellipsed@ei@\frmradius@@,,@@}%
 \fi}
\xydef@\ellipsed@i@#1,#2,#3@@{\DNii@{,}\DN@{#3}%
 \ifx\next@\nextii@
 \dimen@=#1\relax \dimen@ii=#2\relax
 \edef\next@{\noexpand\ellipsed@{\the\dimen@}{\the\dimen@ii}}%
 \else \ifx\next@\empty \DN@{#2}%
 \ifx\next@\empty \DN@{#1}%
 \dimen@=.5\L@c \advance\dimen@.5\R@c
 \dimen@ii=.5\U@c \advance\dimen@ii.5\D@c
 \edef\next@{\noexpand\ellipsed@{\the\dimen@}{\the\dimen@ii}}%
 \else \dimen@=#1\relax
 \edef\next@{\noexpand\ellipsed@{\the\dimen@}{\the\dimen@ii}}%
 \fi
 \else\xywarning@{ignoring extra tokens in elliptical frame: #3 }%
 \dimen@=#1\relax \dimen@ii=#2\relax 
 \edef\next@{\noexpand\ellipsed@{\the\dimen@}{\the\dimen@ii}}%
 \fi\fi \next@ }
\xydef@\ellipsed@ei@#1,#2,#3@@{\DNii@{,}\DN@{#3}%
 \ifx\next@\nextii@
 \dimen@=#1\relax \dimen@ii=#2\relax 
 \edef\next@{\noexpand\ellipsed@e@{\the\dimen@}{\the\dimen@ii}}%
 \else \ifx\next@\empty \DN@{#2}%
 \ifx\next@\empty \DN@{#1}%
 \dimen@=.5\L@c \advance\dimen@.5\R@c
 \dimen@ii=.5\U@c \advance\dimen@ii.5\D@c
 \edef\next@{\noexpand\ellipsed@e@{\the\dimen@}{\the\dimen@ii}}%
 \else 
 \dimen@=#1\relax 
 \edef\next@{\noexpand\ellipsed@e@{\the\dimen@}{\the\dimen@}}%
 \fi
 \else\xywarning@{ignoring extra tokens in elliptical frame: #3 }%
 \dimen@=#1\relax \dimen@ii=#2\relax 
 \edef\next@{\noexpand\ellipsed@e@{\the\dimen@}{\the\dimen@ii}}%
 \fi\fi \next@ }
\xydef@\ellipsed@e@#1#2{%
 \dimen@=#1\relax \dimen@ii=#2\relax 
 \edef\next@{\noexpand\ellipsed@{\the\dimen@}{\the\dimen@ii}}\next@ 
 \dimen@=#1\relax \dimen@ii=#2\relax 
 \ifdim\dimen@>2\p@ \advance\dimen@-2\p@ \else \dimen@=\z@\fi
 \ifdim\dimen@ii>2\p@ \advance\dimen@ii-2\p@ \else \dimen@ii=\z@\fi
 \edef\next@{\noexpand\ellipsed@{\the\dimen@}{\the\dimen@ii}}\next@ }%
\xydef@\ellipsed@#1#2{\setboxz@h\bgroup \relax
 \setboxz@h{\vbox{\ellipsed@x@@{#1}{#2}}}%
 \A@=\X@c \advance\A@-.5\wd\z@
 \B@=\Y@c \advance\B@-.5\ht\z@ \advance\B@.5\dp\z@ \advance\B@.2\p@
 \edef\tmp@{\egroup\dimen@=\the\wdz@}%
 \kern\A@ \raise\B@\boxz@
 \tmp@ \divide\dimen@4 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \boxz@}
\xydef@\ellipsed@i#1#2{{\R@c=#1\relax\L@c=\R@c
 \U@c=#2\relax\D@c=\U@c \ellipsed@{#1}{#2}}}
\xydef@\ellipsed@x@#1#2{\R@=#1\relax\advance\R@#2\relax
 \divide\R@\tw@ \circled@x@@ }
\xylet@\ellipsed@x@@=\ellipsed@x@
\xydef@\ellipsesolidframed@{%
 \let\framehfill=\frm@solidh@@ \let\framevfill=\frm@solidv@@}
\xydef@\ellipsedotframed@{%
 \let\framehfill=\frm@doth@@ \let\framevfill=\frm@dotv@@}
\xydef@\ellipsedashframed@{%
 \let\framehfill=\frm@dashh@@ \let\framevfill=\frm@dashv@@}
\xydefcsname@{frm{\{}}{\addtoDrop@@{\lbraced}}
\xydefcsname@{frm{\}}}{\addtoDrop@@{\rbraced}}
\xydefcsname@{frm{^\}}}{\addtoDrop@@{\ubraced}}
\xydefcsname@{frm{_\}}}{\addtoDrop@@{\dbraced}}
\xydef@\dbraced{\xy@@{\setboxz@h{%
 \A@=\X@c \advance\A@-\L@c \B@=\Y@c \advance\B@-\D@c
 \setboxz@h{$\m@th\bracelu$}\dimen@=2\wdz@ \advance\B@-.5\ht\z@
 \ifdim\R@c<\dimen@ \R@c=\dimen@ \fi
 \ifdim\L@c<\dimen@ \advance\A@-\dimen@ \advance\A@\L@c \L@c=\dimen@ \fi
 \advance\A@-.25pt
 \kern\A@\raise\B@\hbox{%
 \hbox to\L@c{$\m@th\bracelu\leaders\vrule\hfil\bracerd$}%
 \kern.5pt
 \hbox to\R@c{$\m@th\braceld\leaders\vrule\hfil\braceru$}}}%
 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \boxz@}}
\xydef@\ubraced{\xy@@{\setboxz@h{%
 \A@=\X@c \advance\A@-\L@c \B@=\Y@c \advance\B@\U@c
 \setboxz@h{$\m@th\bracelu$}\dimen@=2\wdz@
 \ifdim\R@c<\dimen@ \R@c=\dimen@ \fi
 \ifdim\L@c<\dimen@ \advance\A@-\dimen@ \advance\A@\L@c \L@c=\dimen@ \fi
 \advance\A@-.25pt
 \kern\A@\raise\B@\hbox{%
 \hbox to\L@c{$\m@th\braceld\leaders\vrule\hfil\braceru$}%
 \kern.5pt
 \hbox to\R@c{$\m@th\bracelu\leaders\vrule\hfil\bracerd$}}}%
 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \boxz@}}
{\catcode`\"=12
 \global\mathchardef\braceur="338
 \global\mathchardef\braceul="339
 \global\mathchardef\bracedr="33A
 \global\mathchardef\bracedl="33B
 \global\mathchardef\bracecl="33C
 \global\mathchardef\bracecr="33D
 \global\mathchardef\bracec="33E }
\xydef@\lbraced{\xy@@{\setboxz@h{%
 \A@=\X@c \advance\A@-\L@c \B@=\Y@c \advance\B@-\D@c
 \setboxz@h{$\m@th\bracecl$}\dimen@ii=\dp\z@ \advance\A@-.5\wdz@
 \setboxz@h{$\m@th\bracec$}\dimen@=\dp\z@
 \ifdim\U@c<.5\dimen@ \U@c=.5\dimen@ \fi
 \ifdim\D@c<.5\dimen@ \advance\B@-.5\dimen@ \advance\B@\D@c \D@c=.5\dimen@ \fi
 \advance\U@c.6\p@ \advance\D@c.6\p@ \advance\B@-.6\p@
 \kern\A@\raise\B@\vbox{\vbox to\U@c{%
 \nointerlineskip\hbox{$\m@th\braceur$}%
 \kern-.61\dimen@ \cleaders\copy\z@\vfil \kern-.4\dimen@
 \nointerlineskip\hbox{$\m@th\bracecl$}\kern-.5\dimen@ii}%
 \nointerlineskip\vbox to\D@c{\kern.5\dimen@ii
 \kern-.4\dimen@ \cleaders\copy\z@\vfil \kern-.61\dimen@
 \nointerlineskip\hbox{$\m@th\bracedr$}\kern\z@}}}%
 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \boxz@}}
\xydef@\rbraced{\xy@@{\setboxz@h{%
 \A@=\X@c \advance\A@\R@c \B@=\Y@c \advance\B@-\D@c
 \setboxz@h{$\m@th\bracecr$}\dimen@ii=\dp\z@ \advance\A@-.5\wdz@
 \setboxz@h{$\m@th\bracec$}\dimen@=\dp\z@
 \ifdim\U@c<.5\dimen@ \U@c=.5\dimen@ \fi
 \ifdim\D@c<.5\dimen@ \advance\B@-.5\dimen@ \advance\B@\D@c \D@c=.5\dimen@ \fi
 \advance\U@c.6\p@ \advance\D@c.6\p@ \advance\B@-.6\p@
 \kern\A@\raise\B@\vbox{\vbox to\U@c{%
 \nointerlineskip\hbox{$\m@th\braceul$}%
 \kern-.61\dimen@ \cleaders\copy\z@\vfil \kern-.4\dimen@
 \nointerlineskip\hbox{$\m@th\bracecr$}\kern-.5\dimen@ii}%
 \nointerlineskip\vbox to\D@c{\kern.5\dimen@ii
 \kern-.4\dimen@ \cleaders\copy\z@\vfil \kern-.61\dimen@
 \nointerlineskip\hbox{$\m@th\bracedl$}\kern\z@}}}%
 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \boxz@}}
\xydefcsname@{frm{(}}{\addtoDrop@@{\lparenthesized}}
\xydefcsname@{frm{)}}{\addtoDrop@@{\rparenthesized}}
\xydefcsname@{frm{^)}}{\addtoDrop@@{\uparenthesized}}
\xydefcsname@{frm{_)}}{\addtoDrop@@{\dparenthesized}}
\xydef@\dparenthesized{\xy@@{\setboxz@h{%
 \A@=\X@c \advance\A@-\L@c \B@=\Y@c \advance\B@-\D@c
 \setboxz@h{$\m@th\bracelu$}\dimen@=2\wdz@ \advance\B@-.5\ht\z@
 \ifdim\R@c<\dimen@ \R@c=\dimen@ \fi
 \ifdim\L@c<\dimen@ \advance\A@-\dimen@ \advance\A@\L@c \L@c=\dimen@ \fi
 \dimen@=\L@c \advance\dimen@\R@c
 \kern\A@\raise\B@\hbox to\dimen@{%
 $\m@th\bracelu\leaders\vrule\hfil\braceru$}}%
 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \boxz@}}
\xydef@\uparenthesized{\xy@@{\setboxz@h{%
 \A@=\X@c \advance\A@-\L@c \B@=\Y@c \advance\B@\U@c
 \setboxz@h{$\m@th\bracelu$}\dimen@=2\wdz@
 \ifdim\R@c<\dimen@ \R@c=\dimen@ \fi
 \ifdim\L@c<\dimen@ \advance\A@-\dimen@ \advance\A@\L@c \L@c=\dimen@ \fi
 \dimen@=\L@c \advance\dimen@\R@c
 \kern\A@\raise\B@\hbox to\dimen@{%
 $\m@th\braceld\leaders\vrule\hfil\bracerd$}}%
 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \boxz@}}
\xydef@\lparenthesized{\xy@@{\setboxz@h{%
 \A@=\X@c \advance\A@-\L@c \B@=\Y@c \advance\B@-\D@c
 \setboxz@h{$\m@th\bracecr$}\dimen@ii=\dp\z@ \advance\A@-.5\wdz@
 \setboxz@h{$\m@th\bracec$}\dimen@=\dp\z@
 \ifdim\U@c<.5\dimen@ \U@c=.5\dimen@ \fi
 \ifdim\D@c<.5\dimen@ \advance\B@-.5\dimen@ \advance\B@\D@c \D@c=.5\dimen@ \fi
 \advance\U@c.6\p@ \advance\D@c.6\p@ \advance\B@-.6\p@
 \dimen@ii\U@c \advance\dimen@ii\D@c
 \kern\A@\raise\B@\vbox to \dimen@ii{%
 \nointerlineskip\hbox{$\m@th\braceur$}%
 \kern-.61\dimen@ \cleaders\copy\z@\vfil \kern-.61\dimen@
 \nointerlineskip\hbox{$\m@th\bracedr$}\kern\z@}}%
 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \boxz@}}
\xydef@\rparenthesized{\xy@@{\setboxz@h{%
 \A@=\X@c \advance\A@\R@c \B@=\Y@c \advance\B@-\D@c
 \setboxz@h{$\m@th\bracecr$}\dimen@ii=\dp\z@ \advance\A@-.5\wdz@
 \setboxz@h{$\m@th\bracec$}\dimen@=\dp\z@
 \ifdim\U@c<.5\dimen@ \U@c=.5\dimen@ \fi
 \ifdim\D@c<.5\dimen@ \advance\B@-.5\dimen@ \advance\B@\D@c \D@c=.5\dimen@ \fi
 \advance\U@c.6\p@ \advance\D@c.6\p@ \advance\B@-.6\p@
 \dimen@ii\U@c \advance\dimen@ii\D@c
 \kern\A@\raise\B@\vbox to \dimen@ii{%
 \nointerlineskip\hbox{$\m@th\braceul$}%
 \kern-.61\dimen@ \cleaders\copy\z@\vfil \kern-.61\dimen@
 \nointerlineskip\hbox{$\m@th\bracedl$}\kern\z@}}%
 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \boxz@}}
\xydefcsname@{frm{*}}{%
 \expandafter\frmDrop@\expandafter{%
 \expandafter\def\expandafter\prevEdge@@\expandafter{\prevEdge@@}%
 \frame@fill@@\frmradius@@}}
\xydefcsname@{frm{**}}{%
 \expandafter\frmDrop@\expandafter{%
 \expandafter\def\expandafter\prevEdge@@\expandafter{\prevEdge@@}%
 \frame@emph@@\frmradius@@}}
\xydef@\frame@fill@#1{\filled@{#1}\empty}
\xydef@\frame@emph@#1{\framed@\frmradius@@}
\xylet@\frame@fill@@=\frame@fill@
\xylet@\frame@emph@@=\frame@emph@
\xydef@\filled@#1{\R@=#1\relax 
 \expandafter\DNii@\expandafter{\prevEdge@@}%
 \DN@{\rectangleEdge}\ifx\next@\prevEdge@@
 \ifdim\R@=\z@ \DN@{\filled@Rectangle@}%
 \else \DN@{\filled@Oval@}\fi
 \else \DN@{\circleEdge}\ifx\next@\prevEdge@@
 \ifdim\R@=\z@ \DN@{\filled@Ellipse@}%
 \else \DN@{\restR@max\filled@Circle@}\fi
 \else 
 \ifdim\R@=\z@ \DN@{\filled@Rectangle@}%
 \else \DN@{\filled@Circle@}\fi
 \fi\fi \next@}
\xydef@\restR@max{%
 \dimen@=\L@c\advance\dimen@\R@c
 \dimen@ii=\U@c \advance\dimen@ii\D@c
 \ifdim\dimen@ii>\dimen@ \dimen@=\dimen@ii\fi
 \ifdim\dimen@>\z@ \divide\dimen@\tw@
 \ifdim\R@>\dimen@\R@=\dimen@\fi\fi }
\xylet@\filledRectangle@@=\bblacked@
\xylet@\filledCircle@@=\bblacked@
\xylet@\filledEllipse@@=\bblacked@
\xylet@\filledOval@@=\bblacked@
\xydef@\filled@Region@#1#2{\setboxz@h\bgroup 
 \setboxz@h{\vbox{#1#2\empty}}%
 \A@=\X@c \advance\A@-.5\wd\z@
 \B@=\Y@c \advance\B@-.5\ht\z@ \advance\B@.5\dp\z@ 
 \edef\tmp@{\egroup\dimen@=\the\wdz@}%
 \kern\A@ \raise\B@\boxz@ \kern-\A@
 \tmp@ \divide\dimen@\tw@ \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \styledboxz@}
\xydef@\filled@Rectangle@{\filled@Region@\filledRectangle@@}
\xydef@\filled@Oval@{\filled@Region@\filledOval@@}
\xydef@\filled@Circle@{\filled@Region@\filledCircle@@}
\xydef@\filled@Ellipse@{\filled@Region@\filledEllipse@@}
\xydefcsname@{shape [F...]}#1{\xyFN@\Fshape@#1:@}
\xylet@\whichframe@@=\empty
\xylet@\whichoptions@@=\empty
\xydef@\Fshape@#1:{\def\whichframe@@{{#1}}%
 \DN@{{}}\ifx\whichframe@@\next@ \def\whichframe@@{{-}}\fi
 \expandafter\DN@\expandafter{\the\Edge@c}\DNii@{\circleEdge}\ifx\next@\nextii@
 \DN@##1{\def\whichframe@@{[o]##1}}%
 \expandafter\next@\expandafter{\whichframe@@}\fi
 \let\whichoptions@@=\empty \xyFN@\Fshape@i}
\xydef@\Fshape@i{%
 \ifx @\next \let\next@=\Fshape@x
 \else\addLT@\ifx\next \let\next@=\Fshape@iii
 \else \let\next@=\Fshape@ii \fi\fi \next@}
\xydef@\Fshape@ii#1:{%
 \expandafter\def\expandafter\whichoptions@@\expandafter{\whichoptions@@[#1]}%
 \xyFN@\Fshape@i}
\xydef@\Fshape@iii#1:{\DN@##1{\def\whichframe@@{#1##1}}%
 \expandafter\next@\expandafter{\whichframe@@}\xyFN@\Fshape@i}
\xydef@\Fshape@x @{%
 \edef\next@##1{\noexpand\addbeforeDrop@@{{\EdgefromtheEdge@##1}}}%
 \DNii@##1##2{\next@{\saveframestyles@{\setbox\z@=\object##2\frm##1%
 \xypre@Style@@\Drop@@\xypost@Style@@\restoreframestyles@}}}%
 \expandafter\expandafter\expandafter\nextii@
 \expandafter\expandafter\expandafter{%
 \expandafter\whichframe@@\expandafter}\expandafter{\whichoptions@@}}
\xydef@\saveframestyles@{%
 \edef\afterframe@preStyle@{\preXY@style@}%
 \edef\afterframe@postStyle@{\postXY@style@}}
\xydef@\restoreframestyles@{%
 \xdef\preXY@style@{\afterframe@preStyle@}\def\afterframe@preStyle@{}%
 \xdef\postXY@style@{\afterframe@postStyle@}\def\afterframe@postStyle@{}}
\xydef@\xycircleframe@x@{\L@=\R@ \xycircleframe@x@i}%
\xydef@\xyellipseframe@x@#1#2{\R@=#1\relax \L@=#2\relax \xycircleframe@x@i}
\xydef@\xycircleframe@x@i{%
 \ifx\framehfill\frm@solidh@@\def\circleSTYLE@{}%
 \else\ifx\framehfill\frm@doth@@
 \expandafter\def\expandafter\circleSTYLE@\expandafter{\addDOT@{}}%
 \else\ifx\framehfill\frm@dashh@@
 \expandafter\expandafter\expandafter\def\expandafter\expandafter
 \expandafter\circleSTYLE@\expandafter\expandafter\expandafter
 {\expandafter\addDASH@\addDASH@{}}%
 \fi\fi\fi \xycircleframe@x@x }
\xydef@\xycircleframe@x@x{\hbox{\vbox{\vskip\L@
 \hbox to2\R@{\hfill \buildcircle@ \hfill}\vskip\L@ }}}
\xydef@\UseCurveFrames@{%
 \let\circled@x@@=\xycircleframe@x@
 \let\ellipsed@x@@=\xyellipseframe@x@ }
\def\UseCurveFrames{\xywithoption{curve}{\UseCurveframes@}}%
\xydef@\UseFontFrames@{%
 \let\circled@x@@=\circled@x@
 \let\ellipsed@x@@=\ellipsed@x@ }
\xylet@\UseFontFrames=\UseFontFrames@
\xydef@\UnloadFrames@{%
 \let\framed@body@@=\framed@body@
 \let\circled@x@@=\circled@x@
 \let\ellipsed@x@@=\ellipsed@x@
 \let\frame@fill@@=\frame@fill@
 \let\frame@emph@@=\frame@emph@
 \let\filledRectangle@@=\bblacked@
 \let\filledCircle@@=\bblacked@
 \let\filledEllipse@@=\bblacked@
 \let\filledOval@@=\bblacked@
}
\xyaddunsupport{frame}\UnloadFrames@
\xyendinput


==> xygraph.tex <==
%% xygraph.tex from $Id: xygraph.doc,v 3.7 1999/02/16 15:12:50 krisrose Exp $
%%
%% Xy-pic ``Graph Combinator feature'' option.
%% Copyright (c) 1994-1997 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1997 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{graph}{Graph feature}{\stripRCS$Revision: 3.7 $}%
 {Kristoffer H.~Rose}{krisrose@brics.dk}%
 {BRICS/Computer Science, University of Aarhus, Ny Munkegade, building 540,
 DK--8000 Aarhus~C}
\xyrequire{arrow}\xycatcodes
\xydef@\xygraph#1{\relax\graph#1\endgraph}
\xydef@\graph{\if\inxy@ \DN@{\xy@@{\nter@{}}}%
 \else \DN@{\xy \xy@\xy{\nter@\endxy}}\fi \next@
 \xy@\xygraph{\senter@ \idfromc@{?NODE}\spushc@
 \expandafter\let\expandafter\next@\csname Q@graphbase\endcsname
 \ifx\next@\relax \setbase@\z@\z@{3pc}\z@
 \else \expandafter\next@ \fi}%
 \GRAPH[]}
\xydef@\endgraph{\ignorespaces}
\xydef@\GRAPH{\xyFN@\GRAPH@}
\xydef@\GRAPH@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\GRAPH@}%
 \else\ifx :\next \DN@:{\xy@:{}\expandafter\GRAPHar@\GRAPHeveryarrow@@}%
 \else\addDASH@\ifx\next
 \addDASH@\DN@{\xy@-{}\expandafter\GRAPHar@\GRAPHeveryline@@}%
 \else\ifx (\next
 \DN@({\xy@({\spushid@{?NODE}\idfromc@{?NODE}}\xyFN@\GRAPH@}%
 \else\ifx ,\next
 \DN@,{\xy@,{\cfromid@{?NODE}}\xyFN@\GRAPH@}%
 \else\ifx )\next
 \DN@){\xy@){\cfromid@{?NODE}%
 \tests@\z@{\idfroms@{?NODE}\z@ \spop@}{\xyerror@{) without (}{}}}%
 \xyFN@\GRAPH@}%
 \else\ifx \endgraph\next \DN@{\xy@@{\tests@\z@\spop@\sleave@\leave@}}%
 \else\ifx \end\next \DN@{\xy@@{\tests@\z@\spop@\sleave@\leave@}}%
 \else\ifx ~\next
 \DN@~{\xy@@{\enter@\cfromthec@}\afterNODE{\leave@ \xyFN@\GRAPH@}!}%
 \else \DN@{\afterNODE{\xyFN@\GRAPH@}}%
 \fi\fi\fi\fi\fi\fi\fi\fi\fi \next@}
\xylet@\GRAPHsaved@PATHafterPOS=\PATHafterPOS
\xylet@\GRAPHsaved@afterar@@=\afterar@@
\xydef@\GRAPHar@{%
 \let\PATHafterPOS=\afterNODE \let\afterar@@=\GRAPHafterar@ \ar}
\xydef@\GRAPHafterar@{%
 \let\PATHafterPOS=\GRAPHsaved@PATHafterPOS
 \let\afterar@@=\GRAPHsaved@afterar@@
 \xy@@{\cfromid@{}}\xyFN@\GRAPH@}
\xylet@\afterNODE@@=\empty
\xydef@\afterNODE#1{\xy@@{\enter@\pfromthep@}%
 \DN@##1{\def\afterNODE@@{\xy@@\leave@ \def\afterNODE@@{##1}#1}}%
 \expandafter\next@\expandafter{\afterNODE@@}%
 \xyFN@\NODE@}
\xylet@\theMOVE@@=\relax
\xydef@\NODE@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\NODE@}%
 \else\ifx [\next \DN@[##1]{\xy@{[##1]}{}%
 \def\theMOVE@@{[##1]}\xyFN@\MOVE@##1]}%
 \else\ifx "\next \DN@ "##1"{%
 \xy@{"##1"}{\cfromid@{##1}}\def\theMOVE@@{"##1"}\xyFN@\NODE@i}%
 \else\ifx ?\next \DN@ ?{%
 \xy@?{\cfromid@{?NODE}}\def\theMOVE@@{?}\xyFN@\NODE@i}%
 \else\ifx !\next \def\theMOVE@@{[]}\let\next@=\NODE@i
 \else \testAND@\iffalse
 \DN@##1{\xy@{}{\pfromc@ \advance\X@c\X@xbase \advance\Y@c\Y@xbase
 \czeroEdge@}\jumpMOVE@ \xyFN@\NODE@i}%
 \else\ifx \\\next
 \DN@\\{\xy@\\{\pfromc@ \advance\X@c\X@xbase \advance\Y@c\Y@xbase
 \R@c=\X@ybase \U@c=\Y@ybase \intersect@
 \advance\X@c-\X@ybase \advance\Y@c-\Y@ybase
 \czeroEdge@}\def\theMOVE@@{\\}\xyFN@\NODE@i}%
 \else \xyerror@{Illegal <node>: \string`\meaning\next\string' unexpected}{}%
 \fi\fi\fi\fi\fi\fi\fi \next@}
\xydef@\jumpMOVE@@{&}
\xydef@\jumpMOVE@{\let\theMOVE@@=\jumpMOVE@@}
\xydef@\MOVE@{\xy@@{\count@=\z@ \count@@=\z@}%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\MOVE@}%
 \else\ifcat A\noexpand\next \let\next@=\MOVE@letter
 \else \let\next@=\MOVE@x \fi\fi \next@}
\xydef@\MOVE@letter{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\MOVE@letter}%
 \else\ifx u\next \DN@ u{\xy@@{\advance\count@\@ne}\xyFN@\MOVE@letter}%
 \else\ifx d\next \DN@ d{\xy@@{\advance\count@\m@ne}\xyFN@\MOVE@letter}%
 \else\ifx l\next \DN@ l{\xy@@{\advance\count@@\m@ne}\xyFN@\MOVE@letter}%
 \else\ifx r\next \DN@ r{\xy@@{\advance\count@@\@ne}\xyFN@\MOVE@letter}%
 \else \let\next@=\MOVE@x \fi\fi\fi\fi\fi \next@}
\xydef@\MOVE@x{%
 \ifx ]\next \DN@ ]{\MOVE@hop \xyFN@\NODE@i}%
 \else\ifx (\next \DN@{\MOVE@hop \xyFN@\MOVE@place}%
 \else\ifx !\next \DN@{\MOVE@hop \xyFN@\MOVE@place}%
 \else\ifx /\next \DN@{\MOVE@hop \xyFN@\MOVE@place}%
 \else\addLT@\ifx\next \DN@{\MOVE@hop \xyFN@\MOVE@place}%
 \else\addGT@\ifx\next \DN@{\MOVE@hop \xyFN@\MOVE@place}%
 \else\addDASH@\ifx\next \addDASH@\DN@{\xyerror@{- not implemented yet}{}}%
 \else \xyerror@{illegal <move>: \codeof\theMOVE@@}{}\let\next@=\NODE@i
 \fi\fi\fi\fi\fi\fi\fi \next@}
\xydef@\MOVE@hop{\xy@@{\pfromc@ \czeroEdge@
 \edef\next@{\the\count@@,\the\count@ @}\expandafter\vfromcartesian@@\next@
 \advance\X@c-\X@origin \advance\Y@c-\Y@origin
 \advance\X@c\X@p \advance\Y@c\Y@p}}
\xydef@\MOVE@place{\xy@@\no@@ \afterPLACE{\xyFN@\MOVE@}}
\xydef@\NODE@i{\let\next@=\NODE@x
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\NODE@i}%
 \else\addEQ@\ifx \next
 \addEQ@\DN@"##1"{\xy@{="##1"}{\idfromc@{##1}}\xyFN@\NODE@i}%
 \else\ifx !\next \DN@!{\xyFN@\NODE@escape}%
 \else\ifx :\next 
 \else\addDASH@\ifx\next
 \else\ifx (\next
 \else\ifx ,\next
 \else\ifx )\next
 \else\ifx ~\next
 \else\ifx [\next
 \else\ifx "\next
 \else\ifx ?\next
 \else\ifx ^\next
 \else\ifx _\next
 \else\ifx |\next
 \else\addLQ@\ifx\next
 \else\addRQ@\ifx\next
 \else \testAND@ \iffalse
 \else\ifx \\\next
 \else\ifx \endgraph\next
 \else\ifx \end\next
 \else \let\next@=\NODE@it
 \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi \next@}
\xydef@\NODE@x{\xy@@{\idfromc@{}}\afterNODE@@}
\xydef@\NODE@it{\let\PATHlabelit@@=\NODEit@ \PATHit@}
{\xyuncatcodes \gdef\next{+}}
\xylet@\GRAPHnodemodifiers@@=\next
\xydef@\NODEit@#1{%
 \DN@{#1}\ifx\next@\empty
 \DN@{\expandafter\NODEit@i\expandafter{\GRAPHnodemodifiers@@}}%
 \else \DN@{\NODEit@i{#1}}\fi \next@}
\def\NODEit@i#1#2{\xy@{*#1{#2}}{\drop@{#1}{#2}}%
 \DN@{\addEQ@\ifx\next\else \xy@@{\idfromc@{#2}}\fi \NODE@i}%
 \xyFN@\next@}
\xydef@\NODE@escape{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\NODE@escape}%
 \else\ifcat A\noexpand\next \DN@##1{\rungraphescape@{##1}}%
 \else\ifcat !\noexpand\next \DN@##1{\rungraphescape@{##1}}%
 \else\ifx \bgroup\next \DN@##1{\xy@{!{##1}}{}\POS##1\relax \xyFN@\NODE@i}%
 \else\ifx ~\next \let\next@=\graphsetup@
 \else \DN@{\xyerror@{Unknown graph <escape>}{}\xyFN@\NODE@i}%
 \fi\fi\fi\fi\fi \next@}
\xydefcsname@{graph !M}#1#{\NODE@matrix{#1}}
\xydef@\NODE@matrix#1#2{\xyerror@{matrix feature not loaded}{}\xyFN@\GRAPH@}
\xydef@\NODE@matrix@#1#2{\xy@{!M#1{#2}}{}%
 \def\everyentry@{\GRAPHeveryentry}%
 \xymatrix#1{#2}%
 \let\everyentry@=\empty \insertmatrixingraph@ \xyFN@\NODE@i}
\xydef@\GRAPHeveryentry{\def\:{\ar}\def\="##1"{\xy@@{\idfromc@{##1}}}}
\xywithoption{matrix}{\let\NODE@matrix=\NODE@matrix@}
\xydef@\insertmatrixingraph@{%
 \xy@@{\enter@{\cfromthec@ \pfromthep@}%
 \expandafter\let\expandafter\next@\csname Q@1,1\endcsname
 \ifx\next@\relax\else
 \next@ \swap@
 \expandafter\let\expandafter\next@\csname Q@1,2\endcsname
 \ifx\next@\relax\else \next@ \setbase@\X@p\Y@p\X@c\Y@c
 \expandafter\let\expandafter\next@\csname Q@2,1\endcsname
 \ifx\next@\relax\else
 \next@ \setbase@@{-\X@c}{-\Y@c}\fi\fi\fi
 \leave@}}
\xydefcsname@{graph !P}#1#{\NODE@poly{#1}}
\xydef@\NODE@poly#1#2{\xyerror@{poly(gon) feature not loaded}{}\xyFN@\GRAPH@}
\xydef@\NODE@poly@#1#2{\xy@{!P#1{#2}}{}\xypoly@#1{#2}\xyFN@\NODE@i}
\xywithoption{poly}{\let\NODE@poly=\NODE@poly@}
\xydefcsname@{graph !E}#1#{\NODE@arc{#1}!}
\xydef@\NODE@arc#1#2{\xyerror@{(ellipse+)arc feature not loaded}{}%
 \xyFN@\GRAPH@}
\xydef@\NODE@arc@#1#2{\xy@{!E#1{#2}}{}\ellipse#1{#2}\xyFN@\NODE@i}
\xywithoption{arc}{\let\NODE@arc=\NODE@arc@}
\xylet@\GRAPHeveryarrow@@=\empty
{\xyuncatcodes \gdef\next{@{-}}}
\xylet@\GRAPHeveryline@@=\next
\xydef@\graphsetup@~{\xyFN@\graphsetup@i}
\xydef@\graphsetup@i{%
 \ifx :\next \DN@:##1{\def\GRAPHeveryarrow@@{##1}\xyFN@\NODE@i}%
 \else\addDASH@\ifx\next
 \addDASH@\DN@##1{\def\GRAPHeveryline@@{##1}\xyFN@\NODE@i}%
 \else\ifx *\next \DN@*##1{\def\GRAPHnodemodifiers@@{##1}\xyFN@\NODE@i}%
 \else\ifcat A\next \DN@##1##2{\newgraphescape{##1}{##2}\xyFN@\NODE@i}%
 \else \DN@{\xyerror@{illegal graph setup \codeof\next@}{}\xyFN@\NODE@i}%
 \fi\fi\fi\fi \next@}
\xydef@\newgraphescape#1{%
 \expandafter\let\expandafter\next\csname graph !#1\endcsname
 \ifx\next\relax\else \expandafter\let\csname G!#1\endcsname=\undefined
 \xywarning@{Redefining graph <escape> !#1}\fi
 \expandafter\gdef\csname graph !#1\endcsname{%
 \expandafter\let\expandafter\next\csname G!#1\endcsname
 \expandafter\xyFN@\expandafter\NODE@\next}%
 \DN@{\newgraphescape@{#1}}\xyFN@\next@}
\xydef@\newgraphescape@#1{%
 \ifx [\next
 \ifx\newcommand\undefined \xyerror@{[n] only with LaTeX}%
 \else
 \def\nextiv@{\expandafter\newcommand\expandafter{\csname G!#1\endcsname}}\fi
 \else \def\nextiv@{\expandafter\gdef\csname G!#1\endcsname}\fi \nextiv@}
\xydef@\rungraphescape@#1{%
 \expandafter\let\expandafter\next\csname graph !#1\endcsname
 \ifx\next\relax \xyerror@{Undefined graph <escape> !#1}\fi \next}
\xyendinput


==> xyidioms.tex <==
%% xyidioms.tex from $Id: xyidioms.doc,v 3.4 1997/05/18 01:14:25 krisrose Exp $
%%
%% Format-dependent idioms for Xy-pic.
%% Copyright (c) 1991-1997 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1997 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyidiomsloaded\empty \message{not reloaded}\endinput \fi
\let\xyidiomsloaded=\empty
\xywarnifdefined\A@ \dimendef\A@=4
\xywarnifdefined\B@ \dimendef\B@=6
\xywarnifdefined\R@ \dimendef\R@=8
\ifx\undefined\AveryUNLIKELYc@ntr@lSEQUENCE@@\else
\errmessage{Xy-pic Error: \string\undefined\space defined.}\fi
\ifx\undefined\literal@ \def\literal@#1{#1}\fi
\ifx\undefined\eat@ \def\eat@#1{}\fi
\xydef@\xyFN@{\futurelet\next}
\ifx\undefined\DN@ \def\DN@{\def\next@}\fi
\ifx\undefined\DNii@ \def\DNii@{\def\nextii@}\fi
\ifx\undefined\setboxz@h\def\setboxz@h{\setbox\z@\hbox}\fi
\ifx\undefined\wdz@ \def\wdz@{\wd\z@}\fi
\ifx\undefined\boxz@ \def\boxz@{\box\z@}\fi
\ifx\undefined\W@ \def\W@{\immediate\write16 }\fi
\ifx\undefined\space@ \def\space@.{\futurelet\space@\relax}\space@. \fi
\ifx\undefined\notempty \def\notempty#1{T\if @#1@F\else T\fi}\fi
\xydef@\xysetup@dummy#1{\xyuncatcodes#1}
\xywarnifdefined\xysetup@@
\ifx\AtEndDocument\undefined
 \expandafter\ifx\csname amsppt.sty\endcsname\relax
 \let\xysetup@@=\xysetup@dummy
 \else
 \def\xysetup@@#1{%
 \expandafter\def\expandafter\topmatter\expandafter{\topmatter
 #1\xyuncatcodes}}\fi
\else
 \def\xysetup@@#1{\AtBeginDocument{#1\xyuncatcodes}}
\fi
\ifx\xysetup@@\xysetup@dummy\else
 \xysetup@@{\let\xysetup@@=\xysetup@dummy \xyuncatcodes}\fi
\xywarnifdefined\xyclosedown@@
\ifx\AtEndDocument\undefined \let\xyclosedown@@=\eat@
\else \def\xyclosedown@@#1{\AtEndDocument{#1}}\fi
\xylet@\xy@begindvi=\literal@
\ifx\undefined\AtBeginDvi\else
 \AtBeginDocument{\let\xy@begindvi=\AtBeginDvi}
 \AtBeginDvi{\global\let\xy@begindvi=\literal@}\fi
\ifx\amstexloaded@\relax
\xylet@\toks@ii=\toks@@ \endinput \fi
\ifx\@tempcnta\undefined
\xynew@{count}\count@@
\xynew@{count}\count@@@
\else
\xylet@\count@@=\@tempcnta
\xylet@\count@@@=\@tempcntb
\fi
\ifx\undefined\toks@ii \toksdef\toks@ii=2 \fi
\endinput


==> xyimport.tex <==
%% xyimport.tex from $Id: xyimport.doc,v 3.6 1998/03/06 01:28:05 krisrose Exp $
%%
%% Xy-pic ``Import feature'' option.
%% Copyright (c) 1993-1997 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1997 Kristoffer H. Rose <krisrose@ens-lyon.fr>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{import}{Import graphics extension}{\stripRCS$Revision: 3.6 $}%
 {Ross Moore}{ross@mpce.mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xydef@\xyimport#1#{\xyimport@{#1}}
\xydef@\xyimport@#1#2{\xydelayimport@{#1}{#2}}
\xydef@\xydelayimport@#1#2{\xy@@ix@{#1{#2}}%
 \xy@@{\expandafter\xyextern@\the\toks9}}
\xydef@\xyextern@(#1,#2){\hbox\bgroup\R@c=#1\p@ \U@c=#2\p@\xyextern@i}
\xydef@\xyextern@i#1#{\DN@{#1}%
 \ifx\next@\empty \L@c=\z@ \D@c=\z@ \DN@{\xyextern@x}%
 \else \DN@{\xyextern@ii#1}\fi \next@ }
\xydef@\xyextern@ii(#1,#2){\L@c=#1\p@ \D@c=#2\p@ 
 \advance\R@c-\L@c \advance\U@c-\D@c \xyextern@x}
\xydef@\xyimportdefault@{3}
\xydef@\xyexportwarning@#1#2#3{\xywarning@{%
 #1 for import has zero #2; using \xyimportdefault@#3 default}}
\xydef@\xyextern@x#1{\toks@={\egroup\L@c=}\setboxz@h{#1}%
 \dimen@ii=\L@c \advance\dimen@ii\R@c \dimen@=\wdz@ 
 \ifdim\dimen@=\z@ \xyexportwarning@{graphic}{width}{cm}%
 \dimen@=\xyimportdefault@ cm\fi
 \ifdim\dimen@ii=\z@ \xyexportwarning@{coords}{width}{unit}%
 \dimen@ii=\xyimportdefault@\p@\fi
 \quotient@\next@\dimen@\dimen@ii \dimen@=\next@\p@
 \edef\tmp@{\expandafter\removePT@\the\L@c}\L@c=\tmp@\dimen@
 \expandafter\addtotoks@\expandafter{\the\L@c\relax\R@c=}%
 \edef\tmp@{\expandafter\removePT@\the\R@c}\R@c=\tmp@\dimen@
 \expandafter\addtotoks@\expandafter{\the\R@c\relax\setbase@\z@\z@}%
 \expandafter\addtotoks@\expandafter{\expandafter{\the\dimen@}\z@\D@c=}%
 \dimen@ii=\U@c \advance\dimen@ii\D@c \dimen@=\ht\z@\advance\dimen@\dp\z@
 \ifdim\dimen@=\z@ \xyexportwarning@{graphic}{height}{cm}%
 \dimen@=\xyimportdefault@ cm\fi
 \ifdim\dimen@ii=\z@ \xyexportwarning@{coords}{height}{unit}%
 \dimen@ii=\xyimportdefault@\p@\fi
 \quotient@\next@\dimen@\dimen@ii \dimen@=\next@\p@
 \edef\tmp@{\expandafter\removePT@\the\D@c}\D@c=\tmp@\dimen@
 \expandafter\addtotoks@\expandafter{\the\D@c\relax\U@c=}%
 \edef\tmp@{\expandafter\removePT@\the\U@c}\U@c=\tmp@\dimen@
 \expandafter\addtotoks@\expandafter{\the\U@c\relax\setbase@@\z@}%
 \expandafter\addtotoks@\expandafter{\expandafter{\the\dimen@}}%
 \setboxz@h{\kern-\L@c\lower\D@c\boxz@\kern\L@c}%
 \wd\z@=\z@ \ht\z@=\z@ \dp\z@=\z@ \boxz@ \the\toks@ \X@c=\z@ \Y@c=\z@
 \ifdim\X@min>-\L@c \X@min=-\L@c \fi \ifdim\X@max<\R@c \X@max=\R@c \fi
 \ifdim\Y@min>-\D@c \Y@min=-\D@c \fi \ifdim\Y@max<\U@c \Y@max=\U@c \fi
 \idfromc@{import}\POS }
\xyendinput


==> xyknot.tex <==
%% xyknot.tex from $Id: xyknot.doc,v 3.4 1997/05/18 01:13:24 ross Exp $
%%
%% Xy-pic ``Knots and Links'' feature.
%% Copyright (c) 1994-1996 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1996 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this macro package; if not, write to the Free Software Foundation,
%% Inc., 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{knot}{Knots and Links feature}{\stripRCS$Revision: 3.4 $}%
 {Ross Moore}{ross@mpce.mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\message{knots and links,}
\xyrequire{arrow}\xycatcodes 
\xydef@\xykparsecross@{%
 \def\xykSCALE@@{}\edef\xyknotPLACE{\xykmidPLACE@}%
 \let\xykparser@=\xykparsecross@@
 \def\xykdefaultbreak@{\let\xykbreak@=\xykforetemp@
 \def\xyknotPLACE{(.5)}\appendtoholder@}%
 \xyFN@\xykparsescale@ }
{\xyuncatcodes \catcode`@=11
\gdef\next{%
 \ifx\space@\next \expandafter\DN@\space{\xyFN@\xykparsecross@@}%
 \else\addLT@\ifx\next \addLT@\DN@{\xyprecross@}%
 \else\addGT@\ifx\next \addGT@\DN@{\xypostcross@}%
 \else\addEQ@\ifx\next \addEQ@\DN@{\xyFN@\xykparsetips@@}%
 \else\ifx|\next\DN@|{\xymidcross@}%
 \else\addAT@\ifx\next \addAT@\DN@(##1){%
 \xyadjustBREAK@i##1@@\xyFN@\xykparsecross@@}%
 \else\DN@{\afterknot@}%
 \fi\fi\fi\fi\fi\fi \next@ }}
\xylet@\xykparsecross@@=\next
\xydef@\xyprecross@{%
 \def\xykholder@{\xykprebreak@@}%
 \edef\xyknotPLACE{\xykprePLACE@}%
 \xyFN@\xykparsebreak@}
\xydef@\xypostcross@{%
 \def\xykholder@{\xykpostbreak@@}%
 \edef\xyknotPLACE{\xykpostPLACE@}%
 \xyFN@\xykparsebreak@}
\xydef@\xymidcross@{%
 \def\xykholder@{\xykmidbreak@@}%
 \edef\xyknotPLACE{\xykmidPLACE@}%
 \xyFN@\xykparsebreak@}
\xydef@\xykcross@#1{\xykcheckTIPS@
 \expandafter\toks@\expandafter{\expandafter#1\knotSTYLE}}
\xydef@\xykoverstring@{\addtotoks@{{}}\xykmidbreak@ \xyknottips@}
\xydef@\xykunderstring@{\xykprebreak@ \xykpostbreak@ \xyknottips@}
\xydef@\vcross{\begingroup\def\afterknot@{\xyvcross}%
 \def\xykprePLACE@{(.1)}\def\xykpostPLACE@{(.9)}%
 \def\xykmidPLACE@{(.9)}\def\xykpostbreak@@{|\knothole}%
 \xyFN@\xykparsecross@ }%
\xydef@\hcross{\begingroup\def\afterknot@{\xyhcross}%
 \def\xykprePLACE@{(.1)}\def\xykpostPLACE@{(.9)}%
 \def\xykmidPLACE@{(.9)}\def\xykpostbreak@@{|\knothole}%
 \xyFN@\xykparsecross@ }%
\xydef@\vcrossneg{\begingroup\def\afterknot@{\xyvcrossneg}%
 \def\xykprePLACE@{(.1)}\def\xykpostPLACE@{(.9)}%
 \def\xykmidPLACE@{(.9)}\def\xykpostbreak@@{|\knothole}%
 \xyFN@\xykparsecross@ }%
\xydef@\hcrossneg{\begingroup\def\afterknot@{\xyhcrossneg}%
 \def\xykprePLACE@{(.1)}\def\xykpostPLACE@{(.9)}%
 \def\xykmidPLACE@{(.9)}\def\xykpostbreak@@{|\knothole}%
 \xyFN@\xykparsecross@ }%
\xydef@\vuncross{\begingroup\def\afterknot@{\xyvuncross}%
 \def\xykprePLACE@{(.1)}\def\xykpostPLACE@{(.9)}%
 \def\xykmidPLACE@{(.9)}\def\xykpostbreak@@{}%
 \xyFN@\xykparsecross@ }%
\xydef@\huncross{\begingroup\def\afterknot@{\xyhuncross}%
 \def\xykprePLACE@{(.1)}\def\xykpostPLACE@{(.9)}%
 \def\xykmidPLACE@{(.9)}\def\xykpostbreak@@{}%
 \xyFN@\xykparsecross@ }%
\xydef@\xyvcross{\xykcross@\xykcrossv
 \xykoverstring@ \xykunderstring@ \xykhvobject@{+(0,-1)}}
\xydef@\xyhcross{\xykcross@\xykcrossh
 \xykoverstring@ \xykunderstring@ \xykhvobject@{+(1,0)}}
\xydef@\xyvcrossneg{\xykcross@\xykcrossv
 \xykunderstring@ \xykoverstring@ \xykhvobject@{+(0,-1)}}
\xydef@\xyhcrossneg{\xykcross@\xykcrossh
 \xykunderstring@ \xykoverstring@ \xykhvobject@{+(1,0)}}
\xydef@\xyvuncross{\xykcross@\xykuncrossv
 \xykoverstring@ \xykunderstring@ \xykhvobject@{+(0,-1)}}
\xydef@\xyhuncross{\xykcross@\xykuncrossh
 \xykoverstring@ \xykunderstring@ \xykhvobject@{+(1,0)}}
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8#9{\save,
 "^<",{\xykz_\ar #1@'{"_<"**{}?(.25)@+,?+(.375,0)@+,
 "_>";"^>"**{}?-(.375,0)@+,?(.25)@+}"_>"#3#4#5},
 "_<",{\xykz^\ar #2@'{"^<"**{}?(.25)@+,?+(.375,0)@+,
 "^>";"_>"**{}?-(.375,0)@+,?(.25)@+}"^>"#6#7#8}
 \restore\POS #9}}
\xylet@\xykcrossv=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8#9{\save,
 "_<",{\xykz_\ar #1@'{"_>"**{}?(.25)@+,?+(0,.375)@+,
 "^>";"^<"**{}?-(0,.375)@+,?(.25)@+}"^>"#3#4#5},
 "_>",{\xykz^\ar #2@'{"_<"**{}?(.25)@+,?+(0,.375)@+,
 "^<";"^>"**{}?-(0,.375)@+,?(.25)@+}"^<"#6#7#8}
 \restore\POS #9}}
\xylet@\xykcrossh=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8#9{\save,
 "^<",{\xykz^\ar #1@'{"_<"**{}?(.25)@+,?(.375)+(.375,0)@+,
 "^>";"_>"**{}?(.375)-(.375,0)@+,?(.25)@+}"^>"#3#4#5},
 "_<",{\xykz^\ar #2@'{"^<"**{}?(.25)@+,?(.375)+(.375,0)@+,
 "_>";"^>"**{}?(.375)-(.375,0)@+,?(.25)@+}"_>"#6#7#8}
 \restore\POS #9}}
\xylet@\xykuncrossv=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8#9{\save,
 "_<",{\xykz^\ar #1@'{"_>"**{}?(.25)@+,?(.375)+(0,.375)@+,
 "^<";"^>"**{}?(.375)-(0,.375)@+,?(.25)@+}"^<"#3#4#5},
 "_>",{\xykz^\ar #2@'{"_<"**{}?(.25)@+,?(.375)+(0,.375)@+,
 "^>";"^<"**{}?(.375)-(0,.375)@+,?(.25)@+}"^>"#6#7#8}
 \restore\POS #9}}
\xylet@\xykuncrossh=\next
\xydef@\vover{\begingroup\def\afterknot@{\xyvover}%
 \def\xykprePLACE@{(.2)}\def\xykpostPLACE@{(.9)}%
 \def\xykmidPLACE@{(.8)}\def\xykpostbreak@@{|(.725)\knothole}%
 \xyFN@\xykparsecross@ }%
\xydef@\hover{\begingroup\def\afterknot@{\xyhover}%
 \def\xykprePLACE@{(.2)}\def\xykpostPLACE@{(.9)}%
 \def\xykmidPLACE@{(.8)}\def\xykpostbreak@@{|(.725)\knothole}%
 \xyFN@\xykparsecross@ }%
\xydef@\vunder{\begingroup\def\afterknot@{\xyvunder}%
 \def\xykprePLACE@{(.1)}\def\xykpostPLACE@{(.8)}%
 \def\xykmidPLACE@{(.2)}\def\xykpostbreak@@{|(.275)\knothole}%
 \xyFN@\xykparsecross@ }%
\xydef@\hunder{\begingroup\def\afterknot@{\xyhunder}%
 \def\xykprePLACE@{(.1)}\def\xykpostPLACE@{(.8)}%
 \def\xykmidPLACE@{(.2)}\def\xykpostbreak@@{|(.275)\knothole}%
 \xyFN@\xykparsecross@ }%
\xydef@\vunover{\begingroup\def\afterknot@{\xyvunover}%
 \def\xykprePLACE@{(.1)}\def\xykpostPLACE@{(.9)}%
 \def\xykmidPLACE@{(.8)}\def\xykpostbreak@@{}%
 \xyFN@\xykparsecross@ }%
\xydef@\hunover{\begingroup\def\afterknot@{\xyhunover}%
 \def\xykprePLACE@{(.1)}\def\xykpostPLACE@{(.9)}%
 \def\xykmidPLACE@{(.8)}\def\xykpostbreak@@{}%
 \xyFN@\xykparsecross@ }%
\xydef@\xoverv{\begingroup\def\afterknot@{\xyxoverv}%
 \def\xykprePLACE@{(.15)}\def\xykpostPLACE@{(.85)}%
 \def\xykmidPLACE@{(.15)}\def\xykpostbreak@@{|\knothole}%
 \xyFN@\xykparsecross@ }%
\xydef@\xunderv{\begingroup\def\afterknot@{\xyxunderv}%
 \def\xykprePLACE@{(.15)}\def\xykpostPLACE@{(.85)}%
 \def\xykmidPLACE@{(.15)}\def\xykpostbreak@@{|\knothole}%
 \xyFN@\xykparsecross@ }%
\xydef@\xoverh{\begingroup\def\afterknot@{\xyxoverh}%
 \def\xykprePLACE@{(.15)}\def\xykpostPLACE@{(.85)}%
 \def\xykmidPLACE@{(.15)}\def\xykpostbreak@@{|\knothole}%
 \xyFN@\xykparsecross@ }%
\xydef@\xunderh{\begingroup\def\afterknot@{\xyxunderh}%
 \def\xykprePLACE@{(.15)}\def\xykpostPLACE@{(.85)}%
 \def\xykmidPLACE@{(.85)}\def\xykpostbreak@@{|\knothole}%
 \xyFN@\xykparsecross@ }%
\xydef@\xunover{\begingroup\def\afterknot@{\xyxunover}%
 \def\xykprePLACE@{(.15)}\def\xykpostPLACE@{(.85)}%
 \def\xykmidPLACE@{(.15)}\def\xykpostbreak@@{}%
 \xyFN@\xykparsecross@ }%
\xydef@\xunoverv{\begingroup\def\afterknot@{\xyxunoverv}%
 \def\xykprePLACE@{(.2)}\def\xykpostPLACE@{(.8)}%
 \def\xykmidPLACE@{(.2)}\def\xykpostbreak@@{}%
 \xyFN@\xykparsecross@ }%
\xydef@\xunoverh{\begingroup\def\afterknot@{\xyxunoverh}%
 \def\xykprePLACE@{(.2)}\def\xykpostPLACE@{(.8)}%
 \def\xykmidPLACE@{(.8)}\def\xykpostbreak@@{}%
 \xyFN@\xykparsecross@ }%
\xydef@\xyvover{\xykcross@\xykoverv
 \xykoverstring@ \xykunderstring@ \xykhvobject@{+(0,-1)}}
\xydef@\xyhover{\xykcross@\xykoverh
 \xykoverstring@ \xykunderstring@ \xykhvobject@{+(1,0)}}
\xydef@\xyvunder{\xykcross@\xykoverv
 \xykunderstring@ \xykoverstring@ \xykhvobject@{+(0,-1)}}
\xydef@\xyhunder{\xykcross@\xykoverh
 \xykunderstring@ \xykoverstring@ \xykhvobject@{+(1,0)}}
\xydef@\xyvunover{\xykcross@\xykunoverv
 \xykoverstring@ \xykunderstring@ \xykhvobject@{+(0,-1)}}
\xydef@\xyhunover{\xykcross@\xykunoverh
 \xykoverstring@ \xykunderstring@ \xykhvobject@{+(1,0)}}
\xydef@\xyxoverv{\xykcross@\xykxoverv
 \xykoverstring@ \xykunderstring@ \xykhvobject@{+(0,-1)}}
\xydef@\xyxunderv{\xykcross@\xykxoverv
 \xykunderstring@ \xykoverstring@ \xykhvobject@{+(0,-1)}}
\xydef@\xyxoverh{\xykcross@\xykxoverh
 \xykoverstring@ \xykunderstring@ \xykhvobject@{+(1,0)}}
\xydef@\xyxunderh{\xykcross@\xykxoverh
 \xykunderstring@ \xykoverstring@ \xykhvobject@{+(1,0)}}
\xydef@\xyxunover{\xykcross@\xykxoverv
 \xykoverstring@ \xykunderstring@ \xykhvobject@{+(1,0)}}
\xydef@\xyxunoverv{\xykcross@\xykxunoverv
 \xykoverstring@ \xykunderstring@ \xykhvobject@{+(0,-1)}}
\xydef@\xyxunoverh{\xykcross@\xykxunoverh
 \xykoverstring@ \xykunderstring@ \xykhvobject@{+(1,0)}}
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8#9{\save,
 "^<",{\xykz^\ar #1@'{"^>"**{}?(.25)@+,?(.625)+(0,-.125)@+,
 "_>";"^>"**{}?(.625)-(.125,0)@+,?(.25)@+}"_>"#3#4#5},
 "_<",{\xykz^\ar #2@'{"^<"**{}?(.25)@+,?(.625)+(.125,0)@+,
 "^>";"^<"**{}?(.625)-(0,.125)@+,?(.25)@+}"^>"#6#7#8},\restore\POS#9}}
\xylet@\xykoverv=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8#9{\save,
 "_<",{\xykz^\ar #1@'{"^<"**{}?(.25)@+,?(.625)+(.125,0)@+,
 "^>";"^<"**{}?(.625)-(0,.125)@+,?(.25)@+}"^>"#3#4#5},
 "_>",{\xykz^\ar #2@'{"_<"**{}?(.25)@+,?(.625)+(0,.125)@+,
 "^<";"_<"**{}?(.625)+(.125,0)@+,?(.25)@+}"^<"#6#7#8},\restore\POS#9}}
\xylet@\xykoverh=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8#9{\save,
 "^<",{\xykz^\ar #1@'{"^>"**{}?(.25)@+,?-(0,.175)@+,?(.75)@+}
 "^>"#3#4#5},
 "_<",{\xykz^\ar #2@'{"^<"**{}?(.25)@+,?+(.125,0)@+,
 "_>"**{}?+(0,.7)@+,"_>";"^>"**{}?-(.125,0)@+,?(.25)@+}
 "_>"#6#7#8},\restore\POS#9}}
\xylet@\xykunoverv=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8#9{\save,
 "_<",{\xykz^\ar #1@'{"^<"**{}?(.25)@+,?+(.175,0)@+,?(.75)@+}
 "^<"#3#4#5},
 "_>",{\xykz^\ar #2@'{"_<"**{}?(.25)@+,?+(0,.125)@+,
 "^>"**{}?-(.7,0)@+,"^>";"^<"**{}?-(0,.125)@+,?(.25)@+}
 "^>"#6#7#8},\restore\POS#9}}
\xylet@\xykunoverh=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8#9{\save,
 "^<";"^>"**{}?="^_","_<";"_>"**{}?;"^_",**{}?="^_",
 "^>",{\xykz^\ar #1@'{"^_"@+}"_<"#3#4#5},
 "^<",{\xykz_\ar #2@'{"^_"@+}"_>"#6#7#8},\restore\POS#9}}
\xylet@\xykxoverv=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8#9{\save,
 "^<";"_<"**{}?="^_","^>";"_>"**{}?;"^_",**{}?="^_",
 "^<",{\xykz_\ar #1@'{"^_"@+}"_>"#3#4#5},
 "_<",{\xykz_\ar #2@'{"^_"@+}"^>"#6#7#8},\restore\POS#9}}
\xylet@\xykxoverh=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8#9{\save,
 "^<";"^>"**{}?="^_","_<";"_>"**{}?;"^_",**{}?="^_",
 "^>",{\xykz^\ar #1@'{"^_"@+}"_>"#3#4#5},
 "^<",{\xykz^\ar #2@'{"^_"@+}"_<"#6#7#8},\restore\POS#9}}
\xylet@\xykxunoverv=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8#9{\save,
 "^<";"_<"**{}?="^_","^>";"_>"**{}?;"^_",**{}?="^_",
 "^<",{\xykz^\ar #1@'{"^_"@+}"^>"#3#4#5},
 "_<",{\xykz^\ar #2@'{"^_"@+}"_>"#6#7#8},
 \restore\POS#9}}
\xylet@\xykxunoverh=\next
\xydef@\vtwist{\begingroup\def\afterknot@{\xyvtwist}%
 \def\xykprePLACE@{(.1)}\def\xykpostPLACE@{(.9)}%
 \def\xykmidPLACE@{(.9)}\def\xykpostbreak@@{|\knothole}%
 \xyFN@\xykparsecross@ }%
\xydef@\htwist{\begingroup\def\afterknot@{\xyhtwist}%
 \def\xykprePLACE@{(.1)}\def\xykpostPLACE@{(.9)}%
 \def\xykmidPLACE@{(.9)}\def\xykpostbreak@@{|\knothole}%
 \xyFN@\xykparsecross@ }%
\xydef@\vtwistneg{\begingroup\def\afterknot@{\xyvtwistneg}%
 \def\xykprePLACE@{(.1)}\def\xykpostPLACE@{(.9)}%
 \def\xykmidPLACE@{(.9)}\def\xykpostbreak@@{|\knothole}%
 \xyFN@\xykparsecross@ }%
\xydef@\htwistneg{\begingroup\def\afterknot@{\xyhtwistneg}%
 \def\xykprePLACE@{(.1)}\def\xykpostPLACE@{(.9)}%
 \def\xykmidPLACE@{(.9)}\def\xykpostbreak@@{|\knothole}%
 \xyFN@\xykparsecross@ }%
\xydef@\vuntwist{\begingroup\def\afterknot@{\xyvuntwist}%
 \def\xykprePLACE@{(.15)}\def\xykpostPLACE@{(.85)}%
 \def\xykmidPLACE@{(.85)}\def\xykpostbreak@@{}%
 \xyFN@\xykparsecross@ }%
\xydef@\huntwist{\begingroup\def\afterknot@{\xyhuntwist}%
 \def\xykprePLACE@{(.15)}\def\xykpostPLACE@{(.85)}%
 \def\xykmidPLACE@{(.85)}\def\xykpostbreak@@{}%
 \xyFN@\xykparsecross@ }%
\xydef@\xyvtwist{\xykcross@\xyktwistv
 \xykoverstring@ \xykunderstring@ \xykhvobject@{+(0,-1)}}
\xydef@\xyvtwistneg{\xykcross@\xyktwistv
 \xykunderstring@ \xykoverstring@ \xykhvobject@{+(0,-1)}}
\xydef@\xyvuntwist{\xykcross@\xykuntwistv
 \xykoverstring@ \xykunderstring@ \xykhvobject@{+(0,-1)}}
\xydef@\xyhtwist{\xykcross@\xyktwisth
 \xykoverstring@ \xykunderstring@ \xykhvobject@{+(1,0)}}
\xydef@\xyhuntwist{\xykcross@\xykuntwisth
 \xykoverstring@ \xykunderstring@ \xykhvobject@{+(1,0)}}
\xydef@\xyhtwistneg{\xykcross@\xyktwisth
 \xykunderstring@ \xykoverstring@ \xykhvobject@{+(1,0)}}
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8#9{\save,
 "^>",{\xykz_\ar #1@'{"_>"**{}?(.25)@+,?-(.375,0)@+,
 "_<";"^<"**{}?+(.375,0)@+,?(.25)@+}"_<"#3#4#5},
 "^<",{\xykz^\ar #2@'{"_<"**{}?(.25)@+,?+(.375,0)@+,
 "_>";"^>"**{}?+(-.375,0)@+,?(.25)@+}"_>"#6#7#8}
 \restore\POS #9}}
\xylet@\xyktwistv=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8#9{\save,
 "^>",{\xykz^\ar #1@'{"_>"**{}?(.125)@+,?(.375)-(.25,0)@+,
 ?(.625)-(.25,0)@+,?(.875)@+}"_>"#3#4#5},
 "^<",{\xykz^\ar #2@'{"_<"**{}?(.125)@+,?(.375)+(.25,0)@+,
 ?(.625)+(.25,0)@+,?(.875)@+}"_<"#6#7#8}
 \restore\POS #9}}
\xylet@\xykuntwistv=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8#9{\save,
 "^<",{\xykz_\ar #1@'{"^>"**{}?(.25)@+,?+(0,-.375)@+,
 "_>";"_<"**{}?+(0,.375)@+,?(.25)@+}"_>"#3#4#5},
 "_<",{\xykz^\ar #2@'{"_>"**{}?(.25)@+,?+(0,.375)@+,
 "^>";"^<"**{}?-(0,.375)@+,?(.25)@+}"^>"#6#7#8}
 \restore\POS #9}}
\xylet@\xyktwisth=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8#9{\save,
 "^<",{\xykz^\ar #1@'{"^>",**{}?(.125)@+,?(.375)+(0,-.25)@+,
 ?(.625)+(0,-.25)@+,?(.875)@+}"^>"#3#4#5},
 "_<",{\xykz^\ar #2@'{"_>",**{}?(.125)@+,?(.375)+(0,.25)@+,
 ?(.625)+(0,.25)@+,?(.875)@+}"_>"#6#7#8},\restore\POS #9}}
\xylet@\xykuntwisth=\next
\xydef@\xykparsescale@{%
 \ifx\space@\next \expandafter\DN@\space{\xyFN@\xykparsescale@}%
 \else\addDASH@\ifx\next \addDASH@\DN@{\def\xykSCALE@@{-1}%
 \xyFN@\xykparser@}%
 \else\ifx[\next \DN@[##1]{\dimen@=##1\p@
 \ifdim\dimen@=\z@\xywarning@{\xykscaleerror@}%
 \else\edef\xykSCALE@@{\expandafter\removePT@\the\dimen@}\fi
 \xyFN@\xykparser@}%
 \else\ifx~\next \DN@~##1##2##3##4{%
 \def\xykSCALE@@{@{##1}{##2}{##3}{##4}}\xyFN@\xykparser@}%
 \else\DN@{\xyFN@\xykparser@}%
 \fi\fi\fi\fi \next@}
\xydef@\xykscaleerror@{Ignoring zero scale factor}
\xydef@\xykhobject@{\aftergroup\xykhadjust@
 \ifx\xykSCALE@@\empty\DN@{\xykkeepscale@}%
 \else \DN@{\xyksavescale@{}}%
 \fi \next@ }
\xydef@\xykvobject@{\aftergroup\xykvadjust@
 \ifx\xykSCALE@@\empty\DN@{\xykkeepscale@}%
 \else \DN@{\xyksavescale@{}}%
 \fi \next@ }
\xydef@\xykhvobject@{\aftergroup\xykhvadjust@
 \ifx\xykSCALE@@\empty\DN@{\xykkeepscale@}%
 \else \DN@{\xyksavescale@{}}%
 \fi \next@ }
\xydef@\xykhuobject@{\aftergroup\xykhuadjust@
 \ifx\xykSCALE@@\empty\DN@{\xykkeepscale@}%
 \else \DN@{\xyksavescale@{}}%
 \fi \next@ }
\xydef@\xyksavescale@#1#2{%
 \expandafter\ifx\the\Edge@c\zeroEdge\relax \def\xyksaveEdgec{}%
 \else
 \edef\xyksaveEdgec{\noexpand\Edge@c={\expandafter\noexpand\the\Edge@c}%
 \L@c=\the\L@c \R@c=\the\R@c \D@c=\the\D@c \U@c=\the\U@c}%
 \fi
 \edef\next@##1##2{\endgroup
 \def\noexpand\xyksaveEdgec{}%
 \def\noexpand\xykSCALE@@\noexpand{##1}%
 \def\noexpand\xykjoincontrol\noexpand{\xykjoincontrol}%
 \noexpand\toks@\noexpand{##2}%
 \noexpand\xy@@{\def\noexpand\xyksaveEdgec{}%
 \def\noexpand\xykSCALE@@{##1}%
 \def\noexpand\xykjoincontrol{\xykjoincontrol}}}%
 \expandafter\expandafter\expandafter\next@
 \expandafter\expandafter\expandafter{\expandafter\xykSCALE@@\expandafter}%
 \expandafter{\the\toks@}%
 \xykrescale@ #1\the\toks@\restore\POS#2}
\xydef@\xykkeepscale@{%
 \edef\next@##1{\endgroup \noexpand\toks@={##1}%
 \def\noexpand\xykjoincontrol{\xykjoincontrol}}%
 \expandafter\next@\expandafter{\the\toks@}%
 \def\xykSCALE@@{}\def\xyksaveEdgec{}%
 \xy@@{\def\xykSCALE@@{}\def\xyksaveEdgec{}}%
 \edef\next@{\def\noexpand\xykjoincontrol{\xykjoincontrol}}%
 \expandafter\xy@@\expandafter{\next@}%
 \xyknoflexscale@ \the\toks@}
\xydef@\xykrescale@{\expandafter\xykcheckscale@\xykSCALE@@ !}%
\xydef@\xykcheckscale@#1#2!{%
 \expandafter\DN@\expandafter{\codeof{#1}}%
 \expandafter\DNii@\expandafter{\codeof{@}}%
 \ifx\next@\nextii@\relax\DN@{\xykflexiscale@#2%
 \xy@@{\divide\X@xbase2\divide\X@ybase2\divide\Y@xbase2\divide\Y@ybase2%
 \def\xykSCALE@@{}}\def\xykSCALE@@{}%
 \expandafter\toks@\expandafter{\afterFLEX@}}%
 \else\DN@{\save \xykrescale@@}\fi \next@ }
\xydef@\xykflexiscale@{%
 \expandafter\def\expandafter\afterFLEX@\expandafter{\the\toks@}%
 \xykflexiscale@@ }
\xydef@\xykrescale@@{%
 \edef\next@{\X@xbase=\xykSCALE@@\X@xbase \X@ybase=\xykSCALE@@\X@ybase
 \Y@xbase=\xykSCALE@@\Y@xbase \Y@ybase=\xykSCALE@@\Y@ybase}%
 \expandafter\xy@@\expandafter{\next@}%
 \ifdim\xykSCALE@@\p@<\z@\relax \DN@{\xyknegflexscale@}%
 \else\DN@{\xyknoflexscale@}\fi \next@ }
{\xyuncatcodes \gdef\next#1#2#3#4{\save="@",
 #1,="^<",\POS"@",#2,="^>",\POS"@",#3,="_<",\POS"@",#4,="_>",
 (0,0);"^>"-"^<"+"_>"-"_<":"^<"-"_<"+"^>"-"_>"::}}
\xylet@\xykflexiscale@@=\next
{\xyuncatcodes \gdef\next{\save ="^<",
 +(1,0)="^>",-(1,1)="_<",+(1,0)="_>"\restore }}
\xylet@\xyknoflexscale@@=\next
\xylet@\xyknoflexscale@=\next
{\xyuncatcodes \gdef\next{\save ="_>",
 +(-1,1)="^<",+(1,0)="^>",-(1,1)="_<"\restore }}
\xylet@\xyknegflexscale@@=\next
\xylet@\xyknegflexscale@=\next
{\xyuncatcodes \gdef\next{\save ="_<",
 +(1,0)="_>",+(-1,1)="^<",+(1,0)="^>"\restore }}
\xylet@\xykhscale@@=\next
{\xyuncatcodes \gdef\next{\save ="^>",
 -(1,0)="^<",+(1,-1)="_>",-(1,0)="_<"\restore }}
\xylet@\xykvscale@@=\next
\xydef@\xykhadjust@{%
 \let\xyknoflexscale@=\xykhscale@@
 \let\xyknegflexscale@=\xyknegflexscale@@ }
\xydef@\xykvadjust@{%
 \let\xyknoflexscale@=\xyknoflexscale@@
 \let\xyknegflexscale@=\xykhscale@@ }
\xydef@\xykhvadjust@{%
 \let\xyknoflexscale@=\xyknoflexscale@@
 \let\xyknegflexscale@=\xyknegflexscale@@ }
\xydef@\xykhuadjust@{%
 \let\xyknoflexscale@=\xykhscale@@
 \let\xyknegflexscale@=\xykvscale@@ }
\xydef@\xykprebreak@{%
 \ifx\xykprebreak@@\empty\addtotoks@{{}}\else
 \expandafter\addtotoks@\expandafter{\expandafter{\xykprebreak@@}}\fi}
\xydef@\xykpostbreak@{%
 \ifx\xykpostbreak@@\empty\addtotoks@{{}}\else
 \expandafter\addtotoks@\expandafter{\expandafter{\xykpostbreak@@}}\fi}
\xydef@\xykmidbreak@{%
 \ifx\xykmidbreak@@\empty\addtotoks@{{}}\else
 \expandafter\addtotoks@\expandafter{\expandafter{\xykmidbreak@@}}\fi}
\xydef@\xykparsebreak@{%
 \ifx\space@\next \expandafter\DN@\space{\xyFN@\xykparsebreak@}%
 \else \addLT@\ifx\next 
 \expandafter\appendtoholder@\xykbacktemp@\next@
 \addLT@\DN@{\xyFN@\xykparser@}%
 \else \addGT@\ifx\next 
 \expandafter\appendtoholder@\xykforetemp@\next@
 \addGT@\DN@{\xyFN@\xykparser@}%
 \else \ifx|\next
 \expandafter\appendtoholer@\xyknulltemp@\next@
 \DN@|{\xyFN@\xykparser@}%
 \else \ifx\next \bgroup\DN@##1{\checkgroupbreak@##1@}%
 \else \ifx (\next\DN@(##1){\xyadjustknotPLACE@i##1@@%
 \xyFN@\xykparsebreak@}%
 \else \ifx\next \knothole@\DN@##1{\expandafter\appendtoholder@@
 \expandafter{\expandafter|\xyknotPLACE\knothole}\next@
 \xyFN@\xykparser@}%
 \else 
 \expandafter\xykdefaultbreak@\xykbreak@\next@
 \DN@{\xyFN@\xykparser@}%
 \fi\fi\fi\fi\fi\fi\fi \next@ }
{\xyuncatcodes \gdef\next{^>*\dir{>}}}
\xylet@\xykforetips@=\next
{\xyuncatcodes \gdef\next{^<*\dir{<}}}
\xylet@\xykbacktips@=\next
{\xyuncatcodes \gdef\next{*!/-1pt/=0\dir{>}}}
\xylet@\xykforetemp@=\next
{\xyuncatcodes \gdef\next{*!/1pt/=0\dir{<}}}
\xylet@\xykbacktemp@=\next
{\xyuncatcodes \gdef\next{*=<\xykholesize>[o]{}}}
\xylet@\xykholetemp@=\next
\xydef@\knothole@{\hbox to\xykholesize{%
 \dimen@=\xykholesize \divide\dimen@\tw@
 \hfill \vrule height\dimen@ depth\dimen@ width\z@ }}
\xylet@\knothole=\knothole@
\xylet@\khole=\knothole@
{\xyuncatcodes \gdef\next{*=<0pt>{}}}
\xylet@\xyknulltemp@=\next
\xylet@\xykbreak@=\xyknulltemp@
\xydef@\checkgroupbreak@#1#2@{%
 \ifx|#1\DN@{\appendtoholder@@#1#2\next@ \xyFN@\xykparser@}%
 \else \ifx_#1\DN@{\appendtoholder@@_#2\next@ \xyFN@\xykparser@}%
 \else \ifx^#1\DN@{\appendtoholder@@^#2\next@ \xyFN@\xykparser@}%
 \else 
 \def\next##1\next{\expandafter\DNii@\expandafter{\xyk@@##1}}%
 \expandafter\next\xyknotPLACE\next
 \ifx*#1%
 \expandafter\DN@\expandafter{%
 \expandafter\appendtoholder@@\nextii@#1#2\next@ \xyFN@\xykparser@}%
 \else
 \expandafter\DN@\expandafter{%
 \expandafter\appendtoholder@@\nextii@{#1#2}\next@ \xyFN@\xykparser@}%
 \fi\fi\fi\fi \next@ }
{\xyuncatcodes \gdef\next{%
 \expandafter{\expandafter^\xyknotPLACE##1}}}%
 \DN@{\xydef@\xykholder@@##1}\DNii@{\expandafter\toks@}%
 \expandafter\expandafter\expandafter\next@
 \expandafter\expandafter\expandafter{\expandafter\nextii@\next}
\xydef@\appendtoholder@#1\next@{\xykholder@@{#1}%
 \DN@##1{\expandafter\DN@\expandafter{\xykholder@##1}}%
 \expandafter\next@\expandafter{\the\toks@}\appendtoholder@@@ }
\xydef@\appendtoholder@@#1\next@{%
 \DN@##1\next@{\expandafter\DN@\expandafter{\xykholder@##1}}%
 \next@#1\next@ \appendtoholder@@@}%
\xydef@\appendtoholder@@@{%
 \expandafter\expandafter\expandafter\DN@
 \expandafter\expandafter\expandafter{\next@}%
 \DNii@{\expandafter\def\xykholder@}%
 \expandafter\nextii@\expandafter{\next@}}
{\xyuncatcodes \gdef\next{%
 \expandafter{\expandafter|\xyknotPLACE##1}}}%
\DN@{\xydef@\xykholer@@##1}\DNii@{\expandafter\toks@}%
 \expandafter\expandafter\expandafter\next@
 \expandafter\expandafter\expandafter{\expandafter\nextii@\next}
\xydef@\appendtoholer@#1\next@{\xykholer@@{#1}%
 \DN@##1{\expandafter\DN@\expandafter{\xykholder@##1}}%
 \expandafter\next@\expandafter{\the\toks@}\appendtoholder@@@ }
\xydef@\xykz#1{\let\xyk@@=#1\xy@@{\let\xyk@@=#1}}
{\xyuncatcodes \global\let\next=_}
\xylet@\xyk@@=\next
\xydef@\xyadjustknotPLACE@i{%
 \ifx\xyknotPLACE\empty\DN@{\dimen@=.5\p@}%
 \else\DN@{\expandafter\xygetknotPLACE@@\xyknotPLACE}%
 \fi \next@ \relax \let\xywhichknotPLACE@@=\xysetknotPLACE@@
 \xyFN@\xyadjustknotPLACE@}
\xydef@\xyadjustknotPLACE@{\expandafter\ifx\space@\next
 \expandafter\DN@\space{\xyFN@\xyadjustknotPLACE@}%
 \else\addDASH@\ifx\next\DN@{\xyadjustknotPLACE@@}%
 \else\addPLUS@\ifx\next\DN@{\xyadjustknotPLACE@@}%
 \else\addEQ@\ifx\next\addEQ@\DN@{\dimen@=\z@ \xyadjustknotPLACE@@}%
 \else \DN@{\dimen@=\z@ \xyadjustknotPLACE@@}%
 \fi\fi\fi\fi \next@}
\xydef@\xyadjustknotPLACE@@#1@@{\advance\dimen@#1\p@
 \expandafter\xysetknotPLACE@\expandafter{\the\dimen@}}
\xydef@\xysetknotPLACE@#1{%
 \expandafter\xywhichknotPLACE@@\expandafter{\removePT@#1}}
{\xyuncatcodes\gdef\next#1{\def\xyknotPLACE{(#1)}}}%
\xylet@\xysetknotPLACE@@=\next
{\xyuncatcodes \catcode`@=11
 \gdef\next(#1){\DN@\next@{#1}\ifx\next@\empty
 \dimen@=\z@\else\dimen@=#1\p@ \fi}}%
\xylet@\xygetknotPLACE@@=\next 
\xydef@\xyadjustJOIN@i{%
 \ifx\xykjoincontrol\empty\DN@{\dimen@=.75\p@}%
 \else\DN@{\expandafter\xygetknotPLACE@@\expandafter(\xykjoincontrol)}%
 \fi \next@ \relax \let\xywhichknotPLACE@@=\xysetjoincontrol@
 \xyFN@\xyadjustknotPLACE@}
\xydef@\xyadjustBREAK@i{%
 \ifx\xykpostbreak@@\empty\DN@{\dimen@=.5\p@}%
 \else\DN@{\expandafter\xygetpostBREAK@\xykpostbreak@@}%
 \fi \next@ \relax \let\xywhichknotPLACE@@=\xysetpostbreak@
 \xyFN@\xyadjustknotPLACE@}
\xydef@\xygetpostBREAK@|#1\knothole{\DN@{#1}%
 \ifx\next@\empty\dimen@=.5\p@\else \xygetknotPLACE@@#1\fi}
\xydef@\xysetpostbreak@#1{\def\xykpostbreak@@{|(#1)\knothole}}
\xydef@\xysetjoincontrol@#1{\edef\xykjoincontrol{#1}}
\xydef@\xykparsetips@{%
 \def\xyknotTIPS@@{}\def\xyknotPLACE{}%
 \let\xykparser@=\xykparsetips@@
 \xyFN@\xykparser@ }
\xydef@\xykparsetips@@{%
 \ifx\space@\next \expandafter\DN@\space{\xyFN@\xykparsetips@@}%
 \else\addLT@\ifx\next
 \ifx\xyknotTIPS@@\empty \def\xyknotTIPS@@{TF}%
 \else\DN@{FF}\ifx\next@\xyknotTIPS@@ \def\xyknotTIPS@@{TF}%
 \else\DN@{FT}\ifx\next@\xyknotTIPS@@ \def\xyknotTIPS@@{TT}%
 \fi\fi\fi
 \addLT@\DN@{\xyFN@\xykparser@}%
 \else\addGT@\ifx\next
 \ifx\xyknotTIPS@@\empty \def\xyknotTIPS@@{FT}%
 \else\DN@{FF}\ifx\next@\xyknotTIPS@@ \def\xyknotTIPS@@{FT}%
 \else\DN@{TF}\ifx\next@\xyknotTIPS@@ \def\xyknotTIPS@@{TT}%
 \fi\fi\fi
 \addGT@\DN@{\xyFN@\xykparser@}%
 \else\addEQ@\ifx\next \def\xyknotTIPS@@{TT}%
 \addEQ@\DN@{\xyFN@\xykparser@}%
 \else \ifx!\next \def\xyknotTIPS@@{FF}\DN@!{\xyFN@\xykparser@}%
 \else\DN@{\xyFN@\xykparser@}%
 \fi\fi\fi\fi\fi \next@ }
\xydef@\xykcheckTIPS@{%
 \ifx\xyknotTIPS@@\empty \edef\xyknotTIPS@@{\xyknotTIPS@}\fi
 \DN@{FF}\ifx\next@\xyknotTIPS@@\def\tmp@{}%
 \else\DN@{FT}\ifx\next@\xyknotTIPS@@
 \expandafter\def\expandafter\tmp@\expandafter{\xykforetips@}%
 \else\DN@{TF}\ifx\next@\xyknotTIPS@@
 \expandafter\def\expandafter\tmp@\expandafter{\xykbacktips@}%
 \else 
 \DN@##1\next@{\DN@{\xykforetips@##1}}%
 \expandafter\next@\xykbacktips@\next@
 \DNii@{\expandafter\def\expandafter\tmp@\expandafter}%
 \expandafter\nextii@\expandafter{\next@}%
 \fi\fi\fi \def\xyknotTIPS@@{}}
\xydef@\xyknottips@{%
 \ifx\tmp@\empty\addtotoks@{{}}\else
 \expandafter\addtotoks@\expandafter{\expandafter{\tmp@}}\fi}
\xydef@\xykparsejoin@{%
 \def\xykSCALE@@{}%
 \edef\xyknotPLACE{\xykmidPLACE@}%
 \let\xykparser@=\xykparsejoin@@
 \def\xykdefaultbreak@{\let\xykbreak@=\xykforetemp@
 \def\xyknotPLACE{(.5)}\appendtoholder@}%
 \xyFN@\xykparsescale@ }
{\xyuncatcodes \catcode`@=11
\gdef\next{%
 \ifx\space@\next \expandafter\DN@\space{\xyFN@\xykparsejoin@@}%
 \else\addLT@\ifx\next \let\xykbreak@=\xykbacktemp@
 \def\xykdefaultbreak@{\def\xyknotPLACE{(.5)}%
 \appendtoholder@}\addLT@\DN@{\xyprecross@}%
 \else\addGT@\ifx\next \let\xykbreak@=\xykforetemp@
 \def\xykdefaultbreak@{\def\xyknotPLACE{(.5)}%
 \appendtoholder@}\addGT@\DN@{\xypostcross@}%
 \else\ifx|\next \let\xykbreak@=\xyknulltemp@
 \def\xykdefaultbreak@{\def\xyknotPLACE{(.5)}%
 \appendtoholer@}\DN@|{\xymidcross@}%
 \else\addEQ@\ifx\next \addEQ@\DN@{\xyFN@\xykparsetips@@}%
 \else\addAT@\ifx\next \addAT@\DN@(##1){%
 \xyadjustJOIN@i##1@@\xyFN@\xykparsejoin@@}%
 \else\DN@{\afterknot@}%
 \fi\fi\fi\fi\fi\fi \next@ }}
\xylet@\xykparsejoin@@=\next
\xydef@\xykjoincontrol@@{.75}%
\xydef@\xyk@joincontrol@#1{\DN@{#1}%
 \ifx\next@\empty\edef\xykjoincontrol@@{.75}%
 \else\dimen@=#1\p@
 \edef\xykjoincontrol@@{\expandafter\removePT@\the\dimen@}\fi}
\xylet@\xykjoincontrol\empty
\xydef@\xykjoincontrol@(#1){\DN@{#1}%
 \ifx\next@\empty\edef\xykjoincontrol{\xykjoincontrol@@}%
 \else\dimen@=#1\p@
 \edef\xykjoincontrol{\expandafter\removePT@\the\dimen@}%
 \fi \xyFN@\xykparsejoin@@ }
\xydef@\xykjoincontrol@i#1{\DN@{#1}%
 \ifx\next@\empty\edef\xykjoincontrol{\xykjoincontrol@@}%
 \else\dimen@=#1\p@
 \edef\xykjoincontrol{\expandafter\removePT@\the\dimen@}\fi}
\xydef@\xykjoin@#1{%
 \expandafter\toks@\expandafter{\expandafter#1\knotSTYLE}}
\xydef@\xyksetjoin@{\xykcheckTIPS@ 
 \xykprebreak@ \xykmidbreak@ \xykpostbreak@ \xyknottips@ }
\xydef@\hcap{\begingroup\def\afterknot@{\xyhcap}%
 \def\xykprePLACE@{(.385)}\def\xykpostPLACE@{(.615)}%
 \def\xykmidPLACE@{(.5)}\edef\xykjoincontrol{.25}%
 \xyFN@\xykparsejoin@ }%
\xydef@\vcap{\begingroup\def\afterknot@{\xyvcap}%
 \def\xykprePLACE@{(.385)}\def\xykpostPLACE@{(.615)}%
 \def\xykmidPLACE@{(.5)}\edef\xykjoincontrol{.25}%
 \xyFN@\xykparsejoin@ }%
\xydef@\xcapv{\begingroup\def\afterknot@{\xyxcapv}%
 \def\xykprePLACE@{(.2)}\def\xykpostPLACE@{(.8)}%
 \def\xykmidPLACE@{(.5)}\edef\xykjoincontrol{.5}%
 \xyFN@\xykparsejoin@ }%
\xydef@\xcaph{\begingroup\def\afterknot@{\xyxcaph}%
 \def\xykprePLACE@{(.2)}\def\xykpostPLACE@{(.8)}%
 \def\xykmidPLACE@{(.5)}\edef\xykjoincontrol{.5}%
 \xyFN@\xykparsejoin@ }%
\xydef@\xyvcap{\xykjoin@\xykcapv \xyksetjoin@ \xykhobject@{}}
\xydef@\xyhcap{\xykjoin@\xykcaph \xyksetjoin@ \xykvobject@{}}
\xydef@\xyxcapv{\xykjoin@\xykxcapv \xyksetjoin@ \xykvobject@{+(0,-1)}}
\xydef@\xyxcaph{\xykjoin@\xykxcaph \xyksetjoin@ \xykhobject@{+(1,0)}}
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7{\save,
 "_>",{\xyksaveEdgec},{\xykz_\ar #1@'{"^>"**{}?(\xykjoincontrol)@+
 ,?-(.25,0)@+,"_<";"^<"**{}?+(.25,0)@+,?(\xykjoincontrol)@+}
 "_<"#3#4#5#6},\restore \POS#7}}
\xylet@\xykcapv=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7{\save,
 "_<",{\xyksaveEdgec},{\xykz_\ar #1@'{"_>"**{}?(\xykjoincontrol)@+,
 ?+(0,.25)@+,"^<";"^>"**{}?-(0,.25)@+,?(\xykjoincontrol)@+}
 "^<"#3#4#5#6}
 \restore \POS#7}}
\xylet@\xykcaph=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7{\save,
 "^>";"_>"**{}?="^_","^<";"_<"**{}?;"^_",**{}?(\xykjoincontrol)="^_",
 "_<",{\xyksaveEdgec},{\xykz_\ar #1@'{"^_"@+}
 "^<"#3#4#5#6},\restore \POS#7}}
\xylet@\xykxcapv=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7{\save,
 "^<";"^>"**{}?="^_","_<";"_>"**{}?;"^_",**{}?(\xykjoincontrol)="^_",
 "_>",{\xyksaveEdgec},{\xykz_\ar #1@'{"^_"@+}
 "_<"#3#4#5#6},\restore \POS#7}}
\xylet@\xykxcaph=\next
\xydef@\hloop{\begingroup\def\afterknot@{\xyhloop}%
 \def\xykprePLACE@{(.07)}\def\xykpostPLACE@{(.93)}%
 \def\xykmidPLACE@{(.5)}\edef\xykjoincontrol{.75}%
 \xyFN@\xykparsejoin@ }%
\xydef@\vloop{\begingroup\def\afterknot@{\xyvloop}%
 \def\xykprePLACE@{(.07)}\def\xykpostPLACE@{(.93)}%
 \def\xykmidPLACE@{(.5)}\edef\xykjoincontrol{.75}%
 \xyFN@\xykparsejoin@ }%
\xydef@\xyvloop{\xykjoin@\xykloopv \xyksetjoin@ \xykhobject@{}}
\xydef@\xyhloop{\xykjoin@\xyklooph \xyksetjoin@ \xykvobject@{}}
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7{\save,
 "_>",{\xykz_\ar #1@'{"^>"**{}?(\xykjoincontrol)@+,?(1.25)-(.25,0)@+,
 "_<";"^<"**{}?(1.25)+(.25,0)@+,?(\xykjoincontrol)@+}"_<"#3#4#5#6}
 \restore \POS#7}}
\xylet@\xykloopv=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7{\save,
 "_<",{\xykz_\ar #1@'{"_>"**{}?(\xykjoincontrol)@+,?(1.25)+(0,.25)@+,
 "^<";"^>"**{}?(1.25)+(0,-.25)@+,?(\xykjoincontrol)@+}"^<"#3#4#5#6}
 \restore \POS#7}}
\xylet@\xyklooph=\next
\xydef@\zbendh{\begingroup\def\afterknot@{\xyzbendh}%
 \def\xykprePLACE@{(.25)}\def\xykpostPLACE@{(.75)}%
 \def\xykmidPLACE@{(.5)}\edef\xykjoincontrol{\xykjoincontrol@@}%
 \xyFN@\xykparsejoin@ }%
\xydef@\sbendv{\begingroup\def\afterknot@{\xysbendv}%
 \def\xykprePLACE@{(.25)}\def\xykpostPLACE@{(.75)}%
 \def\xykmidPLACE@{(.5)}\edef\xykjoincontrol{\xykjoincontrol@@}%
 \xyFN@\xykparsejoin@ }%
\xydef@\sbendh{\begingroup\def\afterknot@{\xysbendh}%
 \def\xykprePLACE@{(.25)}\def\xykpostPLACE@{(.75)}%
 \def\xykmidPLACE@{(.5)}\edef\xykjoincontrol{\xykjoincontrol@@}%
 \xyFN@\xykparsejoin@ }%
\xydef@\zbendv{\begingroup\def\afterknot@{\xyzbendv}%
 \def\xykprePLACE@{(.25)}\def\xykpostPLACE@{(.75)}%
 \def\xykmidPLACE@{(.5)}\edef\xykjoincontrol{\xykjoincontrol@@}%
 \xyFN@\xykparsejoin@ }%
\xydef@\xbendr{\begingroup\def\afterknot@{\xyxbendr}%
 \def\xykprePLACE@{(.15)}\def\xykpostPLACE@{(.75)}%
 \def\xykmidPLACE@{(.5)}\edef\xykjoincontrol{.5}%
 \xyFN@\xykparsejoin@ }%
\xydef@\xbendl{\begingroup\def\afterknot@{\xyxbendl}%
 \def\xykprePLACE@{(.15)}\def\xykpostPLACE@{(.75)}%
 \def\xykmidPLACE@{(.5)}\edef\xykjoincontrol{.5}%
 \xyFN@\xykparsejoin@ }%
\xydef@\xbendu{\begingroup\def\afterknot@{\xyxbendu}%
 \def\xykprePLACE@{(.15)}\def\xykpostPLACE@{(.75)}%
 \def\xykmidPLACE@{(.5)}\edef\xykjoincontrol{.5}%
 \xyFN@\xykparsejoin@ }%
\xydef@\xbendd{\begingroup\def\afterknot@{\xyxbendd}%
 \def\xykprePLACE@{(.15)}\def\xykpostPLACE@{(.75)}%
 \def\xykmidPLACE@{(.5)}\edef\xykjoincontrol{.5}%
 \xyFN@\xykparsejoin@ }%
\xydef@\xyzbendh{\xykjoin@\xykzbendh \xyksetjoin@ \xykhvobject@{+(1,-1)}}
\xydef@\xysbendv{\xykjoin@\xyksbendv \xyksetjoin@ \xykhvobject@{+(1,-1)}}
\xydef@\xysbendh{\xykjoin@\xyksbendh \xyksetjoin@ \xykhuobject@{+(1,1)}}
\xydef@\xyzbendv{\xykjoin@\xykzbendv \xyksetjoin@ \xykhuobject@{+(1,1)}}
\xydef@\xyxbendr{\xykjoin@\xykxbendr \xyksetjoin@ \xykhvobject@{+(1,-1)}}
\xydef@\xyxbendl{\xykjoin@\xykxbendl \xyksetjoin@ \xykhvobject@{+(0,-1)}}
\xydef@\xyxbendu{\xykjoin@\xykxbendu \xyksetjoin@ \xykhvobject@{+(1,0)}}
\xydef@\xyxbendd{\xykjoin@\xykxbendd \xyksetjoin@ \xykhvobject@{+(1,-1)}}
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7{\save,
 "^<",{\xyksaveEdgec},
 {\xykz^\ar #1@'{"^>"**{}?(\xykjoincontrol)@+,
 "_>";"_<"**{}?(\xykjoincontrol)@+}"_>"#3#4#5#6}%
 \restore \POS#7}}
\xylet@\xykzbendh=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7{\save,
 "^<",{\xyksaveEdgec},
 {\xykz_\ar #1@'{"_<"**{}?(\xykjoincontrol)@+,
 "_>";"^>"**{}?(\xykjoincontrol)@+}"_>"#3#4#5#6}%
 \restore \POS#7}}
\xylet@\xyksbendv=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7{\save,
 "_<",{\xyksaveEdgec},
 {\xykz_\ar #1@'{"_>"**{}?(\xykjoincontrol)@+,
 "^>";"^<"**{}?(\xykjoincontrol)@+}"^>"#3#4#5#6}%
 \restore \POS#7}}
\xylet@\xyksbendh=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7{\save,
 "_<",{\xyksaveEdgec},
 {\xykz^\ar #1@'{"^<"**{}?(\xykjoincontrol)@+,
 "^>";"_>"**{}?(\xykjoincontrol)@+}"^>"#3#4#5#6}%
 \restore \POS#7}}
\xylet@\xykzbendv=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7{\save,
 "^<"-(0,.5),{\xyksaveEdgec},
 {\xykz_\ar #1@'{"_<";"_>"**{}?(\xykjoincontrol)@+,}"_>"#3#4#5#6}%
 \restore \POS#7}}
\xylet@\xykxbendr=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7{\save,
 "^>"-(0,.5),{\xyksaveEdgec},
 {\xykz^\ar #1@'{"_>";"_<"**{}?(\xykjoincontrol)@+,}"_<"#3#4#5#6}%
 \restore \POS#7}}
\xylet@\xykxbendl=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7{\save,
 "_<"+(.5,0),{\xyksaveEdgec},
 {\xykz_\ar #1@'{"_>";"^>"**{}?(\xykjoincontrol)@+,}"^>"#3#4#5#6}%
 \restore \POS#7}}
\xylet@\xykxbendu=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7{\save,
 "^<"+(.5,0),{\xyksaveEdgec},
 {\xykz^\ar #1@'{"^>";"_>"**{}?(\xykjoincontrol)@+,}"_>"#3#4#5#6}%
 \restore \POS#7}}
\xylet@\xykxbendd=\next
{\xyuncatcodes \gdef\next{{@{-}}{@{-}}}}
\xylet@\knotSTYLE=\next 
{\xyuncatcodes \gdef\next#1{\def\knotSTYLE{{@{#1}}{@{#1}}}}}
\xylet@\knotstyle=\next 
{\xyuncatcodes \gdef\next#1#2{\def\knotSTYLE{{@{#1}}{@{#2}}}}}
\xylet@\knotstyles=\next 
{\xyuncatcodes \gdef\next#1{\def\knotSTYLE{#1}}}
\xylet@\KNOTstyle=\next 
\xydef@\knotholesize@#1{\def\xykholesize{#1}}
\xydef@\xykholesize{5pt}
\xylet@\knotholesize=\knotholesize@
\xylet@\holesize=\knotholesize@
\xydef@\knottips#1{\def\xyknotTIPS@{#1}}
\xydef@\xyknotTIPS@{FF}
\xydef@\xyknotTIPS@@{}
\xydef@\xykSCALE@@{}
\xydef@\xykprebreak@@{}%
\xydef@\xykpostbreak@@{}%
\xydef@\xykmidbreak@@{}%
\xydef@\xykprePLACE@{(.25)}%
\xydef@\xykpostPLACE@{(.75)}%
\xydef@\xykmidPLACE@{}%
\xylet@\xykPLACE@=\xykmidPLACE@
{\gdef\next#1#2#3#4{%
 \save(0,0);"#2"-"#1"+"#4"-"#3":(.5,0):
 "#3"-"#1"+"#4"-"#2"::(0,.5)::}}
\xylet@\xykflexbase@=\next
\xylet@\xykflexbase=\xykflexbase@
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8{\xykflexbase{#1}{#2}{#3}{#4}%
 "#1",{\ar @{#5}@'{"#1"+(0,.125)@++(.1875,.125)@+,
 "#4"-(.1875,.25)@++(.1875,.125)@+}"#4" #6},
 "#2",{\ar @{#5}@'{"#2"+(0,.125)@++(-.1875,.125)@+,
 "#3"+(.1875,-.25)@++(-.1875,.125)@+}"#3" #7}%
\restore \POS#8}}
\xylet@\Xtwist=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8{\xykflexbase{#1}{#2}{#3}{#4}%
 "#1",{\ar @{#5}@'{"#1"+(0,.0625)@++(.1875,.0625)@+,
 "#3"+(.1875,-.125)@++(-.1875,.0625)@+}"#3" #6},
 "#2",{\ar @{#5}@'{"#2"+(0,.0625)@++(-.1875,.0625)@+,
 "#4"-(.1875,.125)@++(.1875,.0625)@+}"#4" #7}%
\restore \POS#8}}
\xylet@\Xuntwist=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8#9{\xykflexbase{#1}{#2}{#3}{#4}%
 "#1",{\ar @{#5}@'{"#1"+(.1875,.0625)@++(.1875,.1875)@+,
 "#4"+(-#9,-.125)@+}"#4" #6},
 "#2",{\ar @{#5}@'{"#2"+(-.1875,.0625)@++(-.1875,.1875)@+,
 "#3"+(#9,-.125)@+}"#3" #7}%
\restore \POS#8}}
\xylet@\Xover=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8#9{\xykflexbase{#1}{#2}{#3}{#4}%
 "#1",{\ar @{#5}@'{"#1"+(.1875,.0625)@++(.1875,.1875)@+,
 "#2"+(-.1875,.0625)@+}"#2" #6},
 "#3",{\ar @{#5}@'{"#3"+(#9,-.125)@+,"#3"+(.25,-.25)@+,
 "#4"+(-#9,-.125)@+}"#4" #7}%
\restore \POS#8}}
\xylet@\Xunover=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7{\xykflexbase{#1}{#2}{#3}{#4}%
 "#1",{\ar @{#5}@'{"#1"+(0,.125)@++(.125,.25)@+,
 "#4"+(-.125,.375)@++(.125,-.25)@+}"#4" #6},
\restore \POS#7}}
\xylet@\Xcap=\next
{\xyuncatcodes \catcode`@=11
 \gdef\next#1#2#3#4#5#6#7#8#9{\dimen@=#1\p@
 \ifdim\dimen@=\z@ \DN@{\Xunover{#2}{#3}{#4}{#5}{#8}{#6}{#7}{"#5"}}%
 \else\ifdim\dimen@>\z@
 \DNii@{#6}\ifx\nextii@\empty
 \DN@{\Xover{#2}{#3}{#4}{#5}{#8}{|(.45)\knothole}{#7}{"#5"}}%
 \else \DN@{\Xover{#2}{#3}{#4}{#5}{#8}{#6}{#7}{"#5"}}\fi
 \else
 \DNii@{#7}\ifx\nextii@\empty
 \DN@{\Xover{#2}{#3}{#4}{#5}{#8}{#6}{|(.45)\knothole}{"#5"}}%
 \else\DN@{\Xover{#2}{#3}{#4}{#5}{#8}{#6}{#7}{"#5"}}\fi
 \fi\fi 
 \def\tmp@{{#9}}\ifx\tmp@\empty\def\tmp@{{0}}\else\dimen@=#9\p@\fi
 \expandafter\next@\tmp@ }}
\xylet@\XXover=\next
{\xyuncatcodes \catcode`@=11
 \gdef\next#1#2#3#4#5#6#7#8{\dimen@=#1\p@
 \ifdim\dimen@=\z@ \DN@{\Xuntwist{#2}{#4}{#3}{#5}{#8}{#6}{#7}{"#5"}}%
 \else\ifdim\dimen@>\z@
 \DNii@{#6}\ifx\nextii@\empty
 \DN@{\Xtwist{#2}{#4}{#3}{#5}{#8}{|(.45)\knothole}{#7}{"#5"}}%
 \else \DN@{\Xtwist{#2}{#4}{#3}{#5}{#8}{#6}{#7}{"#5"}}\fi
 \else
 \DNii@{#7}\ifx\nextii@\empty
 \DN@{\Xtwist{#2}{#4}{#3}{#5}{#8}{#6}{|(.45)\knothole}{"#5"}}%
 \else\DN@{\Xtwist{#2}{#4}{#3}{#5}{#8}{#6}{#7}{"#5"}}\fi
 \fi\fi \next@ }}
\xylet@\XXtwist=\next
{\xyuncatcodes \catcode`@=11
 \gdef\next#1#2#3#4{\dimen@=#1\p@
 \ifdim\dimen@=\z@ \DN@{\xykuncrossv{#4}{#2}{#3}{+(0,-1)}}%
 \else\ifdim\dimen@>\z@
 \DNii@{#2}\ifx\nextii@\empty
 \DN@{\xyktwistv{#4}{|\knothole}{#3}{+(1,0)}}%
 \else \DN@{\xyktwistv{#4}{#2}{#3}{+(1,0)}}\fi
 \else
 \DNii@{#3}\ifx\nextii@\empty
 \DN@{\xyktwistv{#4}{#2}{|\knothole}{+(0,-1)}}%
 \else\DN@{\xyktwistv{#4}{#2}{#3}{+(0,-1)}}\fi
 \fi\fi \next@ }}
\xylet@\Vcross=\next
{\xyuncatcodes \catcode`@=11
 \gdef\next#1#2#3#4{\dimen@=#1\p@
 \ifdim\dimen@=\z@ \DN@{\xykuncrossh{#4}{#2}{#3}{+(0,-1)}}%
 \else\ifdim\dimen@<\z@
 \DNii@{#2}\ifx\nextii@\empty
 \DN@{\xyktwisth{#4}{|\knothole}{#3}{+(1,0)}}%
 \else \DN@{\xyktwisth{#4}{#2}{#3}{+(1,0)}}\fi
 \else
 \DNii@{#3}\ifx\nextii@\empty
 \DN@{\xyktwisth{#4}{}{|\knothole}{+(1,0)}}%
 \else\DN@{\xyktwisth{#4}{#2}{#3}{+(1,0)}}\fi
 \fi\fi \next@ }}
\xylet@\Hcross=\next
{\xyuncatcodes \catcode`@=11
 \gdef\next#1#2#3{\dimen@=#1\p@ \save
 \ifdim\dimen@<\z@
 \DN@{\POS="@",p="@@",(0,0);(-1,0):(0,-1)::"@@";"@",}%
 \else\DN@{}\fi
 \next@ \xykcaph{#3}{#2}\restore }}
\xylet@\Hcap=\next
{\xyuncatcodes \catcode`@=11
 \gdef\next#1#2#3{\dimen@=#1\p@ \save
 \ifdim\dimen@<\z@
 \DN@{\POS="@",p="@@",(0,0);(0,-1)::"@@";"@",}%
 \else\DN@{}\fi
 \next@ \xykcapv{#3}{#2}\restore }}
\xylet@\Vcap=\next
\xyendinput


==> xyline.tex <==
%% xyline.tex from $Id: xyline.doc,v 3.6 1998/03/06 01:28:05 krisrose Exp $
%%
%% Xy-pic ``Line Width'' extension.
%% Copyright (c) 1993-1996 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1996 Kristoffer H. Rose <krisrose@ens-lyon.fr>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{line}{Line styles extension}{\stripRCS$Revision: 3.6 $}%
 {Ross Moore}{ross@mpce.mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xydefcsname@{*stylechar@|@}#1{\xyFN@\xywidthchar@#1@@}%
\xydefcsname@{style [thinner]}{\xyshape@thinner@}
\xydefcsname@{style [thicker]}{\xyshape@thicker@}
\xynew@{dimen}\xylinethick@ \xylinethick@=\xydashw@
\xydef@\xyshape@thicker@{\xylinewidth@i{\multiply\xylinethick@\tw@}}
\xydef@\xyshape@thinner@{\xylinewidth@i{\divide\xylinethick@\tw@}}
\xydef@\xylinewidth@i#1{\edef\xyprevwidth@@{\the\xylinethick@}%
 #1\edef\next@{\xylinethick@=\the\xylinethick@}%
 \edef\next@ii{\noexpand\addtotoks@{%
 \noexpand\xylinewidth@@{\next@}{\xyprevwidth@@}}}%
 \next@ii }
\xydef@\xywidthchar@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\xywidthchar@}%
 \else\ifx @\next \DN@ @@{\checkXyStyle@}%
 \else\ifx (\next \DN@ (##1)##2@@{%
 \xylinewidth@i{\xylinethick@=##1\xydashw@}}%
 \else\addLT@\ifx \next \addGT@{\addLT@\DN@ ##1}##2@@{%
 \xylinewidth@i{\xylinethick@=##1\relax}}%
 \else\ifx *\next \DN@ *@@{\recoverXyStyle@}%
 \else\addEQ@\ifx \next \addEQ@\DN@##1@@{\checkXyStyle@
 \addtotoks@{\xynamestyle@{##1}}}%
 \else\ifx C\next \DN@ C##1@@{\xysetlinecap@{##1}@}%
 \else\ifx J\next \DN@ J##1@@{\xysetlinejoin@{##1}@}%
 \else\ifx M\next \DN@ M(##1)@@{\xymiterlimit@{##1}@}%
 \else \DN@##1@@{\xylinewidth@i{\xylinethick@=##1\relax}}%
 \fi\fi\fi\fi\fi\fi\fi\fi\fi \next@}
\xydef@\xylinecap@{2}
\xydef@\xylinejoin@{2}
\xydef@\xylinemiter@{10}
\xydefcsname@{style [bevel]}{\xyshape@bevel@}
\xydefcsname@{style [roundjoin]}{\xyshape@rdjoin@}
\xydefcsname@{style [miter]}{\xyshape@miter@}
\xydefcsname@{style [butt]}{\xyshape@butt@}
\xydefcsname@{style [roundcap]}{\xyshape@rdcap@}
\xydefcsname@{style [projcap]}{\xyshape@projcap@}
\xydef@\xyshape@butt@{\xysetlinecap@@0}
\xydef@\xyshape@rdcap@{\xysetlinecap@@1}
\xydef@\xyshape@projcap@{\xysetlinecap@@2}
\xydef@\xyshape@miter@{\xysetlinejoin@@0}
\xydef@\xyshape@rdjoin@{\xysetlinejoin@@1}
\xydef@\xyshape@bevel@{\xysetlinejoin@@2}
\xydef@\xysetlinecap@#1@{\DN@ii{#1}\count@=#1\relax
 \expandafter\DN@\expandafter{\the\count@}%
 \ifx\next@\next@ii\else
 \xywarning@{ignoring extra tokens in line-cap: \next@}\fi
 \expandafter\xysetlinecap@@\expandafter{\next@}}
\xydef@\xysetlinejoin@#1@{\DN@ii{#1}\count@=#1\relax
 \expandafter\DN@\expandafter{\the\count@}%
 \ifx\next@\next@ii\else
 \xywarning@{ignoring extra tokens in line-join: \next@}\fi
 \expandafter\xysetlinejoin@@\expandafter{\next@}}
\xydef@\xysetmiterlimit@#1@{\DN@ii{#1}\dimen@=#1\p@\relax
 \edef\next@{\expandafter\removePT@\the\dimen@}%
 \ifx\next@\next@ii\else
 \xywarning@{ignoring extra tokens in miter-limit: \next@}\fi
 \expandafter\xysetmiterlimit@@\expandafter{\next@}}
\xydef@\xysetlinecap@@#1{\xy@linecap@i{\def\xylinecap@{#1}}}
\xydef@\xysetlinejoin@@#1{\xy@linejoin@i{\def\xylinejoin@{#1}}}
\xydef@\xysetmiterlimit@@#1{%
 \xy@linemiter@i{\def\xylinemiter@{#1}}}
\xydef@\xy@linecap@i#1{#1\addtotoks@{\xy@linecap@@{#1}}}
\xydef@\xy@linejoin@i#1{#1\addtotoks@{\xy@linejoin@{#1}}}
\xydef@\xy@linemiter@i#1{#1\addtotoks@{\xy@linemiter@{#1}}}
\xydef@\xy@linecap@#1{\checkXyStyle@ \edef\xyprevcap@@{\xylinecap@}%
 #1\let\prexylinecap@=\prexylinecap@@ \let\postxylinecap@=\postxylinecap@@
 \applyLIFOstyle@\prexylinecap@{\xylinecap@}%
 \postxylinecap@{\xyprevcap@@}}
\xydef@\prexylinecap@@{\let\prexylinecap@=\eat@ 
 \let\postxylinecap@=\postxylinecap@@ \outputxylinecap@ }
\xydef@\postxylinecap@@{\let\postxylinecap@=\eat@ 
 \let\prexylinecap@=\prexylinecap@@ \resetxylinecap@@ }
\xylet@\prexylinecap@=\prexylinecap@@
\xylet@\postxylinecap@=\postxylinecap@@
\xydef@\outputxylinecap@#1{\xycapSpecial@@{#1}}
\xydef@\resetxylinecap@#1{\resetxylinecap@i{#1}\outputxylinecap@{#1}}
\xydef@\resetxylinecap@i#1{\def\xylinecap@{#1}}
\xylet@\resetxylinecap@@=\resetxylinecap@
\xylet@\xycapSpecial@@=\eat@
\xydef@\xy@linejoin@#1{\checkXyStyle@
 \edef\xyprevjoin@@{\xylinejoin@}#1%
 \let\prexylinejoin@=\prexylinejoin@@
 \let\postxylinejoin@=\postxylinejoin@@
 \applyLIFOstyle@\prexylinejoin@{\xylinejoin@}%
 \postxylinecap@{\xyprevjoin@@}}
\xydef@\prexylinejoin@@{\let\prexylinejoin@=\eat@ 
 \let\postxylinejoin@=\postxylinejoin@@ \outputxylinejoin@ }
\xydef@\postxylinejoin@@{\let\postxylinejoin@=\eat@ 
 \let\prexylinejoin@=\prexylinejoin@@ \resetxylinejoin@@ }
\xylet@\prexylinejoin@=\prexylinejoin@@
\xylet@\postxylinejoin@=\postxylinejoin@@
\xydef@\outputxylinejoin@#1{\xyjoinSpecial@@{#1}}
\xydef@\resetxylinejoin@#1{\resetxylinejoin@i{#1}\outputxylinejoin@{#1}}
\xydef@\resetxylinejoin@i#1{\def\xylinejoin@{#1}}
\xylet@\resetxylinejoin@@=\resetxylinejoin@
\xylet@\xyjoinSpecial@@=\eat@
\xydef@\xy@linemiter@#1{\checkXyStyle@
 \edef\xyprevmiter@@{\xylinemiter@}#1%
 \let\prexylinemiter@=\prexylinemiter@@
 \let\postxylinemiter@=\postxylinemiter@@
 \applyLIFOstyle@\prexylinemiter@{\xylinemiter@}%
 \postxylinecap@{\xyprevmiter@@}}
\xydef@\prexylinemiter@@{\let\prexylinemiter@=\eat@ 
 \let\postxylinemiter@=\postxylinemiter@@ \outputxylinemiter@ }
\xydef@\postxylinemiter@@{\let\postxylinemiter@=\eat@ 
 \let\prexylinemiter@=\prexylinemiter@@ \resetxylinemiter@@ }
\xylet@\prexylinemiter@=\prexylinemiter@@
\xylet@\postxylinemiter@=\postxylinemiter@@
\xydef@\outputxylinemiter@#1{\xymiterSpecial@@{#1}}
\xydef@\resetxylinemiter@#1{\resetxylinemiter@i{#1}\outputxylinemiter@{#1}}
\xydef@\resetxylinemiter@i#1{\def\xylinemiter@{#1}}
\xylet@\resetxylinemiter@@=\resetxylinemiter@
\xylet@\xymiterSpecial@@=\eat@
\xydef@\xypolyline#1{\xypolyline@{#1}}
\xydef@\xypolyline@#1{\hbox\bgroup
 \enter@{\pfromthep@ \basefromthebase@ \cfromthec@}%
 \def\xyps@list{}\edef\smapp@@{\s@bot}%
 \smapxy@i{\enter@{\pfromthep@ \basefromthebase@ }%
 \edef\xyps@list{\expandafter\removePT@\the\X@c\space
 \expandafter\removePT@\the\Y@c\space \xyps@list}\leave@}%
 \leave@ \xy@polystyle@@{#1}\xydopoly@style\egroup
 \def\Drop@@{\styledboxz@}\def\Connect@@{\styledboxz@}}%
\xylet@\xypolyline@Special=\eat@
\xylet@\xypolyfill@Special=\eat@
\xylet@\xypolyeofill@Special=\eat@
\xylet@\xypolydot@Special=\eat@
\xylet@\xypolydash@Special=\eat@
\xydef@\UnloadpolySpecials@{%
 \let\xypolyline@Special=\eat@
 \let\xypolyfill@Special=\eat@
 \let\xypolyeofill@Special=\eat@
 \let\xypolydot@Special=\eat@
 \let\xypolydash@Special=\eat@
}
\xydef@\xy@polystyle@#1{%
 \let\poly@style@@=\xypolyline@Special
 \DNii@{#1}\ifx\nextii@\empty 
 \else\DN@{*}\ifx\next@\nextii@ \let\poly@style@@=\xypolyfill@Special
 \else\DN@{?}\ifx\next@\nextii@ \let\poly@style@@=\xypolyeofill@Special
 \else\expandafter\DN@\expandafter{\addDOT@{}}\ifx\next@\nextii@
 \let\poly@style@@=\xypolydot@Special
 \else\expandafter\DN@\expandafter{\addDASH@{}}\ifx\next@\nextii@
 \let\poly@style@@=\xypolydash@Special
 \else\DN@{{*}}\ifx\next@\nextii@ \def\poly@style@@{\xypolystraight@{*}}%
 \else \def\poly@style@@{\xypolystraight@{#1}}%
 \fi\fi\fi\fi\fi\fi }
\xydef@\xydopoly@style{\expandafter\poly@style@@\expandafter{\xyps@list}}
\xydef@\xynopolystyle@#1#2{\xyundefinedLine@{polyline}{{#1}}@@}
\xydef@\xypolynospec@#1{\DNii@{#1}%
 \ifx\nextii@\empty\def\poly@style@@{\xypolystraight@{-}}%
 \else\DN@{.}\ifx\next@\nextii@ \def\poly@style@@{\xypolystraight@{.}}%
 \else\DN@{-}\ifx\next@\nextii@ \def\poly@style@@{\xypolystraight@{--}}%
 \else\DN@{*}\ifx\next@\nextii@ \def\poly@style@@{\xypolystraight@{.}}%
 \else\DN@{?}\ifx\next@\nextii@ \def\poly@style@@{\xypolystraight@{.}}%
 \else\DN@{{*}}\ifx\next@\nextii@ \def\poly@style@@{\xypolystraight@{*}}%
 \else \def\poly@style@@{\xypolystraight@{#1}}%
 \fi\fi\fi\fi\fi\fi }
\xydef@\xypolystraight@#1#2{%
 \enter@{\pfromthep@ \basefromthebase@ \cfromthec@}%
 \edef\smapp@@{\s@bot}\csname S@0\endcsname\czeroEdge@\pfromc@\def\smapp@@{0}%
 \smapxy@i{\czeroEdge@\enter@{\pfromthec@}{\connect@\dir{#1}}\leave@}\leave@ }
\xylet@\xy@polystyle@@=\xypolynospec@
\xydef@\UninstallPolylines@{%
 \UnloadpolySpecials@
 \let\xy@polystyle@@=\xypolynospec@ }
\UninstallPolylines@
\xydef@\xyundefinedLine@#1#2@@{%
 \xywarning@{The #1 #2 effect is not implemented with the current driver.}}%
\xydef@\xynolinewidth@#1#2{%
 \xyundefinedLine@{linewidth}{\the\xylinethick@}@@}%
\xydef@\xynolinecap@#1{\xyundefinedLine@{linecap}{\xylinecap@}@@}%
\xydef@\xynolinejoin@#1{\xyundefinedLine@{linejoin}{\xylinejoin@}@@}%
\xydef@\xynolinemiter@#1{\xyundefinedLine@{miterlimit}{\xylinemiter@}@@}%
\xylet@\xylinewidth@@=\xynolinewidth@
\xylet@\xy@linecap@@=\xynolinecap@
\xylet@\xy@linejoin@@=\xynolinejoin@
\xylet@\xy@linemiter@@=\xynolinemiter@
\xydef@\UnloadLine@#1{%
 \ifx#1\relax\else\xyunload@{line width extension}\fi
 \let\resetxyline@@=\resetxyline@
 \let\resetxylinecap@@=\resetxylinecap@
 \let\resetxylinejoin@@=\resetxylinejoin@
 \let\resetxylinemiter@@=\resetxylinemiter@
 \let\transxyline@@=\DN@
 \let\xylineSpecial@@=\eat@
 \let\xycapSpecial@@=\eat@
 \let\xyjoinSpecial@@=\eat@
 \let\xymiterSpecial@@=\eat@
 \let\xylinewidth@@=\xynolinewidth@
 \let\xy@linecap@@=\xynolinecap@
 \let\xy@linejoin@@=\xynolinejoin@
 \let\xy@linemiter@@=\xynolinemiter@
 \UninstallPolylines@ }
\xyaddunsupport{line}{\UnloadLine@\relax}
\xydef@\xylinewidth@#1#2{\checkXyStyle@
 #1\let\prexyline@=\prexyline@@ \let\postxyline@=\postxyline@@
 \applyLIFOstyle@\prexyline@{\the\xylinethick@}\postxyline@{#2}}
\xydef@\prexyline@@{\let\prexyline@=\eat@ 
 \let\postxyline@=\postxyline@@ \outputxyline@ }
\xydef@\postxyline@@{\let\postxyline@=\eat@ 
 \let\prexyline@=\prexyline@@ \resetxyline@@ }
\xylet@\prexyline@=\prexyline@@
\xylet@\postxyline@=\postxyline@@
\xydef@\resetxyline@#1{\resetxyline@i{#1}\outputxyline@{#1}}
\xydef@\resetxyline@i#1{\xylinethick@=#1\relax}
\xydef@\outputxyline@#1{\transxyline@@{#1}%
 \expandafter\xylineSpecial@@\expandafter{\next@}}
\xylet@\resetxyline@@=\resetxyline@
\xydef@\transxyline@#1{\edef\next@{\removePT@#1}}
\xylet@\transxyline@@=\DN@
\xylet@\xylineSpecial@@=\eat@
\xyendinput


==> xymatrix.tex <==
%% xymatrix.tex from $Id: xymatrix.doc,v 3.4 1997/05/18 01:14:25 krisrose Exp $
%%
%% Xy-pic ``Matrix'' feature.
%% Copyright (c) 1991-1997 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1997 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{matrix}{Matrix feature}{\stripRCS$Revision: 3.4 $}%
 {Kristoffer H.~Rose}{krisrose@brics.dk}%
 {BRICS/Computer Science, University of Aarhus, Ny Munkegade, building 540,
 DK--8000 Aarhus~C}
\xynew@{count}\Row
\xynew@{count}\Col
\xydef@\maxrow@{0}
\xydef@\maxcol@{0}
\xydef@\maxcolrow@{0}
\xynew@{toks}\queue@
\xynew@{toks}\queue@@
\xynew@{count}\qcount@
\xynew@{count}\qcount@@
\xydef@\clearq@{%
 \global\queue@={}\global\qcount@=\@ne
 \global\queue@@={}\global\qcount@@=\z@}
\xydef@\addq@#1{\global\advance\matrixsize@\@ne
 \ifnum\qcount@@<\qcount@ \let\addq@@=\addq@i
 \else \let\addq@@=\addq@ii \fi
 \expandafter\addq@@\the\queue@@\addq@@{#1}}
\xylet@\addq@@=\relax
\xydef@\addq@i#1\addq@@#2{%
 \global\advance\qcount@@\@ne \global\queue@@={#1#2}}
\xydef@\addq@ii#1\addq@@#2{%
 \global\advance\qcount@\@ne \global\qcount@@=\z@ 
 \global\queue@=\expandafter{\the\queue@#1#2}\global\queue@@={}}
\xydef@\finishq@{\expandafter\addq@ii\the\queue@@\addq@@{}}
\xynew@{count}\matrixsize@
\xynew@{if}\ifnoisymatrices@ \noisymatrices@true
\xydef@\SilentMatrices{\noisymatrices@false}
\xydef@\NoisyMatrices{\noisymatrices@true}
\xydef@\xymatrixnocompile{\global\matrixsize@=\z@
 \ifnoisymatrices@\message{<xymatrix}\fi
 \if\inxy@
 \DN@{\nter@{}\xy@\xymatrix{\enter@{%
 \def\noexpand\xy@minX@@{\xy@minX@@}\def\noexpand\xy@maxX@@{\xy@maxX@@}%
 \def\noexpand\xy@minY@@{\xy@minY@@}\def\noexpand\xy@maxY@@{\xy@maxY@@}%
 \edef\noexpand\xymatrixprefix@@{\codeof\xymatrixprefix@@}}}}%
 \else \DN@{\xy \nter@\endxy \xy@\xymatrix{\nter@{}}}\fi \next@
 \xy@@{\save@ \edef\matrixorigin@{\X@c=\the\X@c \Y@c=\the\Y@c}%
 \edef\xy@minX@@{\the\X@c}\edef\xy@maxX@@{\the\X@c}%
 \edef\xy@minY@@{\the\Y@c}\edef\xy@maxY@@{\the\Y@c}}%
 \xdef\maxrow@{0}\xdef\maxcol@{0}\xdef\maxcolrow@{0}%
 \mkHWdefaults@ \xymatrix@prefix""}
\xylet@\xymatrix=\xymatrixnocompile
\xydef@\xymatrixprefix@@{}
\xydef@\xymatrix@prefix"#1"{\DN@{#1}\edef\xymatrixprefix@@{\codeof\next@}%
 \DNii@##1{\xy@{"#1"}{\edef\xymatrixprefix@@{##1}}}%
 \expandafter\nextii@\expandafter{\xymatrixprefix@@}%
 \xyFN@\xymatrix@setup}
\xydef@\xymatrix@setup{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\xymatrix@setup}%
 \else\ifx \bgroup\next \let\next@=\xymatrix@ii
 \else\addAT@\ifx\next \addAT@\DN@{\xy@{@}{}\xyFN@\xymatrix@at}%
 \else\ifx "\next \let\next@=\xymatrix@prefix
 \else \DN@{\xyerror@{\string\xymatrix<setup>{<rows>} expected}{}}%
 \fi\fi\fi\fi \next@}
\xydef@\xymatrix@ii#1{%
 \xymatrix@pretypeset{#1}%
 \ifnum\maxcol@=\z@ \mkWcol@ \mkWmax@ \mkHrow@ \mkHmax@
 \xdef\maxcol@{\the\Col}\xdef\maxcolrow@{\the\Row}\fi
 \ifnoisymatrices@\message{\maxcol@ x\maxrow@}\fi
 \xymatrix@measureit@@ \the\queue@ \global\queue@={}%
 \xymatrix@typeset{#1}\restore\xymatrix@insert
 \xy@@\leave@ \leave@
 \ifnoisymatrices@\message{\the\matrixsize@>}\fi \ignorespaces}
\xydef@\xymatrixcompile#1#{\xymatrixcompile@{#1}}
\xydef@\xymatrixcompile@#1#2{\xycompile{\xymatrixnocompile#1{#2}}}
\xydef@\CompileMatrices{\let\xymatrix=\xymatrixcompile}
\xydef@\NoCompileMatrices{\let\xymatrix=\xymatrixnocompile}
\xydef@\xy@cossign@@{+}
\xydef@\xy@sinsign@@{+}
\xydef@\xy@cosabs@@{1}
\xydef@\xy@sinabs@@{0}
\xydef@\xy@tanabs@@{0}
\xydef@\xy@cotabs@@{100}
\xydef@\xymatrix@rotation{%
 \xy@@{%
 \edef\xy@cossign@@{\ifdim\cosDirection\p@<\z@-\else+\fi}%
 \edef\xy@sinsign@@{\ifdim\sinDirection\p@<\z@-\else+\fi}%
 \edef\xy@cosabs@@{%
 \if\xy@cossign@@\cosDirection\else\xy@cossign@@\cosDirection\fi}%
 \edef\xy@sinabs@@{%
 \if\xy@sinsign@@\sinDirection\else\xy@sinsign@@\sinDirection\fi}%
 \dimen@=\xy@cosabs@@\p@ \dimen@ii=\xy@sinabs@@\p@
 \ifdim\dimen@ii<.01\p@ \def\xy@cotabs@@{100}%
 \else \quotient@\xy@cotabs@@\dimen@\dimen@ii \fi
 \dimen@=\xy@cosabs@@\p@ \dimen@ii=\xy@sinabs@@\p@
 \ifdim\dimen@<.01\p@ \def\xy@tanabs@@{100}%
 \else \quotient@\xy@tanabs@@\dimen@ii\dimen@ \fi}}
\xylet@\xymatrixsavedCOORD@=\relax
\xydef@\xymatrix@pretypeset#1{%
 \global\Row=\z@ \xdef\maxcol@{0}\clearq@
 \setbox8=\vtop{%
 \ifx\xymatrixsavedCOORD@\relax \let\xymatrixsavedCOORD@=\COORD@ \fi
 \let\COORD@=\xymatrixCOORD@
 \everycr{}\let\\=\cr \tabskip=\z@ \offinterlineskip
 \halign{\prentry@ ##!@&&\xyFN@\prentry@@##!@\cr#1\crcr}%
 \prentry@@@}%
 \xdef\maxrow@{\the\Row}%
 \finishq@}
\xydef@\prentry@{\relax
 \ifnum\Row>\z@
 \ifnum\maxcol@<\Col\xdef\maxcol@{\the\Col}\xdef\maxcolrow@{\the\Row}\fi
 \expandafter\xdef\csname maxcol@\the\Row\endcsname{\the\Col}\fi
 \global\advance\Row\@ne \global\Col=\z@ \xyFN@\prentry@@}
\xylet@\lastprentry@@=\relax
\xydef@\xyeatall@{\let\xy@=\xyeat@ \change@oxy@\xyeat@ \let\xy@@ix@=\eat@}
\xydef@\prentry@@{\global\advance\Col\@ne
 \let\next@=\prentry@@norm
 \ifoldxymatrix@\else \ifx *\next \DN@*{\xyFN@\prentry@@star}\fi \fi
 \next@}
\xydef@\prentry@@star{\ifx *\next \DN@*{\xyFN@\prentry@@star@ii}%
 \else \DN@##1##{\prentry@@star@i{##1}}\fi \next@}
\xydef@\prentry@@star@i#1#2#3!@{\gdef\lastprentry@@{*#1{#2}#3}%
 \setbox\lastobjectbox@=\object#1{#2}%
 \prentry@@x}
\xydef@\prentry@@star@ii{%
 \ifx [\next
 \DN@[##1]{\DN@####1{\def\entrymodifiers@{[##1]####1}}%
 \expandafter\next@\expandafter{\entrymodifiers@}\prentry@@norm}%
 \else
 \DN@##1{\DN@####1{\def\entrymodifiers@{##1####1}}%
 \expandafter\next@\expandafter{\entrymodifiers@}\prentry@@norm}%
 \fi \next@}
\xydef@\prentry@@norm#1!@{\gdef\lastprentry@@{#1}%
 \DN@{\setbox\lastobjectbox@=\object}%
 \expandafter\next@\entrymodifiers@{\xyeatall@ \everyentry@ #1}%
 \prentry@@x}
\xydef@\prentry@@x{%
 \edef\next@{{\noexpand\pre@emit{\the\Row}{\Upness@}{\the\Col}{\Leftness@}%
 {\the\L@c}{\the\R@c}{\the\D@c}{\the\U@c}{\expandafter\noexpand\the\Edge@c}}}%
 \expandafter\addq@\next@ \box\lastobjectbox@}
\xynew@{if}\ifoldxymatrix@ \oldxymatrix@false
\xydef@\prentry@@@{\relax \let\next@=\prentry@@@i
 \ifoldxymatrix@ \ifnum\Col=\@ne \ifx\lastprentry@@\empty
 \global\advance\Row\m@ne \let\next@=\relax \fi\fi\fi
 \global\let\lastprentry@@=\relax \next@}
\xydef@\prentry@@@i{%
 \ifnum\maxcol@<\Col \xdef\maxcol@{\the\Col}\xdef\maxcolrow@{\the\Row}\fi
 \expandafter\xdef\csname maxcol@\the\Row\endcsname{\the\Col}}
\xydef@\xy@minX@@{\z@}
\xydef@\xy@maxX@@{\z@}
\xydef@\xy@minY@@{\z@}
\xydef@\xy@maxY@@{\z@}
\xydef@\pre@emit#1#2#3#4#5#6#7#8#9{%
 \global\Row=#1\global\Col=#3\relax
 \ifnum#3=\@ne
 \ifnum#1=\@ne \xy@@{\matrixorigin@}%
 \else \count@@=#1\advance\count@@\m@ne
 \edef\next@{\noexpand\xy@@{\noexpand\cfromid@
 {\xymatrixprefix@@\the\count@@,1}}}\next@
 \pre@emit@ \W@maxout\Hrow@c@@\W@maxin\Hrow@in\xy@tanabs@@
 \X@c\xy@sinsign@@\xy@sinabs@@\xymatrixrowsep@
 \pre@emit@ \Hrow@c@@\W@maxout\Hrow@in\W@maxin\xy@cotabs@@
 \Y@c{-\xy@cossign@@}\xy@cosabs@@\xymatrixrowsep@
 \fi
 \else \count@@=#3\advance\count@@\m@ne
 \pre@emit@ \Wcol@c@@\H@maxout\Wcol@in\H@maxin\xy@cotabs@@
 \X@c\xy@cossign@@\xy@cosabs@@\xymatrixcolsep@
 \pre@emit@ \H@maxout\Wcol@c@@\H@maxin\Wcol@in\xy@tanabs@@
 \Y@c\xy@sinsign@@\xy@sinabs@@\xymatrixcolsep@
 \fi
 \DN@##1{\xy@@{\L@c=#5\R@c=#6\D@c=#7\U@c=#8\Edge@c={#9}\idfromc@{##1#1,#3}}}%
 \expandafter\next@\expandafter{\xymatrixprefix@@}%
 \xy@@{%
 \dimen@=\X@c \advance\dimen@-\L@c
 \ifdim\dimen@<\xy@minX@@ \edef\xy@minX@@{\the\dimen@}\fi
 \dimen@=\X@c \advance\dimen@+\R@c
 \ifdim\dimen@>\xy@maxX@@ \edef\xy@maxX@@{\the\dimen@}\fi
 \dimen@=\Y@c \advance\dimen@-\D@c
 \ifdim\dimen@<\xy@minY@@ \edef\xy@minY@@{\the\dimen@}\fi
 \dimen@=\Y@c \advance\dimen@+\U@c
 \ifdim\dimen@>\xy@maxY@@ \edef\xy@maxY@@{\the\dimen@}\fi}}
\xydef@\pre@emit@#1#2#3#4{#1\A@ #2\B@ #3\R@ #4\dimen@
 \edef\next@{{\the\A@}{\the\B@}{\the\R@}{\the\dimen@}}%
 \expandafter\pre@emit@i\next@}
\xydef@\pre@emit@i#1#2#3#4#5{\xy@@{%
 \dimen@=#2\R@=#5\dimen@ \dimen@=#1\relax \ifdim\R@>\dimen@ \R@=\dimen@ \fi
 \dimen@=#4\B@=#5\dimen@ \dimen@=#3\relax \ifdim\B@>\dimen@ \B@=\dimen@ \fi
 \advance\R@\B@}%
 \pre@emit@ii}
\xydef@\pre@emit@ii#1#2#3#4{\xy@@{%
 \dimen@=#4\dimen@=#3\dimen@ \advance\R@\dimen@ \advance#1#2\R@}}
\xydef@\Wcol@in#1{#1=\csname Wcol@\the\Col\endcsname #1=.5#1}
\xydef@\Wcol@out#1{#1=\csname Wcol@\the\Col\endcsname #1=.5#1}
\xydef@\Wcol@c@@#1{#1=\csname Wcol@\the\count@@\endcsname #1=.5#1}
\xydef@\W@maxin#1{#1=\W@max #1=.5#1}
\xydef@\W@maxout#1{#1=\W@max #1=.5#1}
\xydef@\Hrow@in#1{#1=\csname Hrow@\the\Row\endcsname #1=.5#1}
\xydef@\Hrow@out#1{#1=\csname Hrow@\the\Row\endcsname #1=.5#1}
\xydef@\Hrow@c@@#1{#1=\csname Hrow@\the\count@@\endcsname #1=.5#1}
\xydef@\H@maxin#1{#1=\H@max #1=.5#1}
\xydef@\H@maxout#1{#1=\H@max #1=.5#1}
\xydef@\H@max{\z@}
\xydef@\W@max{\z@}
\xydef@\HW@max{\z@}
\xydef@\mkHrow@{}
\xydef@\mkWcol@{}
\xydef@\mkHmax@{}
\xydef@\mkWmax@{}
\xydef@\mkHWmax@{}
\xydef@\mkHWdefaults@{\let\xymatrix@measureit@@=\xymatrix@measureit
 \let\mkHrow@=\Hrow@R \let\mkWcol@=\Wcol@C
 \def\mkHmax@{\ifdim\dimen@>\H@max\relax \xdef\H@max{\the\dimen@}\fi}%
 \def\mkWmax@{\ifdim\dimen@>\W@max\relax \xdef\W@max{\the\dimen@}\fi}%
 \let\mkHWmax@=\HWmax@max}
\xydef@\Hrow@R{\expandafter\xdef\csname Hrow@\the\Row\endcsname{\the\dimen@}}
\xydef@\Wcol@C{\expandafter\xdef\csname Wcol@\the\Col\endcsname{\the\dimen@}}
\xydef@\Hrow@max{\expandafter\gdef\csname Hrow@\the\Row\endcsname{\H@max}}
\xydef@\Wcol@max{\expandafter\gdef\csname Wcol@\the\Col\endcsname{\W@max}}
\xydef@\Hrow@HWmax{\expandafter\gdef\csname Hrow@\the\Row\endcsname{\HW@max}}
\xydef@\Wcol@HWmax{\expandafter\gdef\csname Wcol@\the\Col\endcsname{\HW@max}}
\xydef@\HWmax@max{%
 \ifdim\H@max>\W@max\global\let\HW@max=\H@max\else\global\let\HW@max=\W@max\fi}
\xydef@\HWmax@set#1{\gdef\HW@max{#1}%
 \global\let\H@max=\HW@max \global\let\W@max=\HW@max}
\xydef@\xymatrix@measureit{%
 \xdef\H@max{\z@}\xdef\W@max{\z@}%
 \setbox6=\vbox{\unvbox8 \global\Row=\maxrow@
 \loop@ \dimen@ii=\lastskip\unskip \ifnum\z@<\Row
 \setbox4=\lastbox \dimen@=\dp4 \advance\dimen@\ht4 \mkHrow@ \mkHmax@
 \ifnum\Row=\maxcolrow@
 \setbox2=\hbox{\unhbox4
 \global\Col=\maxcol@
 \loop@ \dimen@ii=\lastskip\unskip \ifnum\z@<\Col
 \setbox\z@=\lastbox \dimen@=\wdz@ \mkWcol@ \mkWmax@
 \global\advance\Col\m@ne
 \repeat@}\fi
 \global\advance\Row\m@ne
 \repeat@}%
 \mkHWmax@}
\xylet@\xymatrix@measureit@@=\relax
\xydef@\xymatrix@typeset#1{%
 \clearq@
 \hbox{\vtop{\xyqall@
 \xy@@{\ifx\xymatrixsavedCOORD@\relax
 \enter@{\noexpand\let\noexpand\COORD@\noexpand\xymatrixsavedCOORD@}%
 \let\xymatrixsavedCOORD@=\COORD@ \let\COORD@=\xymatrixCOORD@
 \else \enter@{}\fi}%
 \ifx\xymatrixsavedCOORD@\relax \let\xymatrixsavedCOORD@=\COORD@ \fi
 \let\COORD@=\xymatrixCOORD@
 \kern\z@ \global\Row=\z@
 \everycr{}\let\\=\cr \tabskip=\z@ \offinterlineskip
 \halign{\entry@##!@&&\entry@@##!@\cr#1\crcr}%
 \xy@@{\leave@}}}%
 \finishq@ \expandafter\xy@@\expandafter{\the\queue@}\global\queue@={}}
\xydef@\entry@{\relax \global\advance\Row\@ne \global\Col=\z@ \entry@@}
\xydef@\entry@@{\global\advance\Col\@ne
 \DN@##1,##2,##3@{\xy@{ENTRY "##3##1,##2"}{\Row=##1 \Col=##2\relax
 \cfromid@{##3##1,##2}\pfromc@}}%
 \edef\nextii@{\the\Row,\the\Col,\xymatrixprefix@@ @}%
 \expandafter\next@\nextii@
 \xyFN@\entry@@i}
\xydef@\entry@@i{\let\next@=\entry@@norm
 \ifoldxymatrix@\else \ifx *\next \DN@*{\xyFN@\entry@@star}\fi \fi
 \next@}
\xydef@\entry@@star{\ifx *\next \DN@*{\xyFN@\entry@@star@ii}%
 \else \DN@##1##{\entry@@star@i{##1}}\fi \next@}
\xydef@\entry@@star@i#1#2#3!@{%
 \xy@@ix@{{#1}{#2}}\xy@@{\expandafter\dropentry@\the\toks9}%
 \setboxz@h{\xyqall@
 \ifx\xymatrixsavedCOORD@\relax \let\xymatrixsavedCOORD@=\COORD@ \fi
 \let\COORD@=\xymatrixCOORD@ \everyentry@ #3}%
 \setbox\z@=\copy\voidb@x}
\xydef@\entry@@star@ii{%
 \ifx [\next
 \DN@[##1]{\DN@####1{\def\entrymodifiers@{[##1]####1}}%
 \expandafter\next@\expandafter{\entrymodifiers@}\entry@@norm}%
 \else
 \DN@##1{\DN@####1{\def\entrymodifiers@{##1####1}}%
 \expandafter\next@\expandafter{\entrymodifiers@}\entry@@norm}%
 \fi \next@}
\xydef@\entry@@norm#1!@{%
 \DN@##1{\expandafter\xy@@ix@
 \expandafter{\expandafter{\entrymodifiers@}{##1}}}%
 \expandafter\next@\expandafter{\everyentry@#1}%
 \xy@@{\expandafter\dropentry@\the\toks9}%
 \setbox\z@=\expandafter\object\entrymodifiers@{\xyqall@
 \ifx\xymatrixsavedCOORD@\relax \let\xymatrixsavedCOORD@=\COORD@ \fi
 \let\COORD@=\xymatrixCOORD@ \everyentry@ #1}%
 \setbox\z@=\copy\voidb@x}
\xydef@\dropentry@#1#2{\drop@{#1}{\xyeatall@
 \ifx\xymatrixsavedCOORD@\relax \let\xymatrixsavedCOORD@=\COORD@ \fi
 \let\COORD@=\xymatrixCOORD@ #2}}
\xydef@\xyqall@{%
 \ifxysaving@ \let\xy@=\xyqs@ \let\xy@@ix@=\xysave@@toksix@
 \else \let\xy@=\xyq@ \let\xy@@ix@=\xyq@@toksix@ \fi
 \change@oxy@\xy@}
\xydef@\xyq@#1#2{\addq@{#2}}
\xydef@\xyq@@toksix@{\begingroup
 \xyuncatcodes \afterassignment\xyq@@toksix@i \global\toks9=}
\xydef@\xyq@@toksix@i{%
 \DN@##1{\endgroup \xy@@{\global\toks9={##1}}}%
 \expandafter\next@\expandafter{\the\toks9}}
\xydef@\xyqs@{\global\advance\matrixsize@\@ne \xysave@}
\xydef@\xymatrix@insert{%
 \xy@@{\edef\nextii@{{\xy@minX@@}{\xy@maxX@@}{\xy@minY@@}{\xy@maxY@@}}%
 \expandafter\xymatrix@insert@\nextii@}}
\xydef@\xymatrix@insert@#1#2#3#4{\matrixorigin@
 \L@c=+\X@c \advance\L@c-#1\relax
 \R@c=-\X@c \advance\R@c+#2\relax
 \D@c=+\Y@c \advance\D@c-#3\relax
 \U@c=-\Y@c \advance\U@c+#4\relax
 \Edge@c={\rectangleEdge}}
\xylet@\thematrixCOORD@@=\relax
\xylet@\thematrixprefix@@=\relax
\xydef@\xymatrixCOORD@{%
 \ifx [\next
 \DN@[##1]{\xy@{[##1]}{\def\thematrixCOORD@@{[##1]}}%
 \xyFN@\xymatrixCOORD@i##1]}%
 \else \let\next@=\xymatrixsavedCOORD@ \fi \next@}
\xydef@\xymatrixCOORD@i{\count@=\Row \count@@=\Col
 \let\thematrixprefix@@=\xymatrixprefix@@
 \ifcat A\noexpand\next
 \DN@##1{\expandafter\notrelaxorelse@\csname xymatrixCOORD@i@##1\endcsname
 \xymatrixCOORD@other}%
 \else\ifx ]\next \DN@]{\xymatrixCOORD@x}%
 \else\ifx "\next \DN@"##1"{\DN@{##1}\edef\thematrixprefix@@{\codeof\next@}%
 \xyFN@\xymatrixCOORD@ii}%
 \else \let\next@=\xymatrixCOORD@other \fi\fi\fi \next@}
\xydef@\xymatrixCOORD@i@u{\advance\count@ \m@ne\xyFN@\xymatrixCOORD@ii}
\xydef@\xymatrixCOORD@i@d{\advance\count@ \@ne \xyFN@\xymatrixCOORD@ii}
\xydef@\xymatrixCOORD@i@l{\advance\count@@\m@ne\xyFN@\xymatrixCOORD@ii}
\xydef@\xymatrixCOORD@i@r{\advance\count@@\@ne \xyFN@\xymatrixCOORD@ii}
\xydef@\xymatrixCOORD@ii{%
 \ifcat A\noexpand\next
 \DN@##1{\expandafter\notrelaxorelse@\csname xymatrixCOORD@i@##1\endcsname
 \xymatrixCOORD@error}%
 \else\ifx ]\next \DN@]{\xymatrixCOORD@x}%
 \else \let\next@=\xymatrixCOORD@xx \fi\fi \next@}
\xydef@\xymatrixCOORD@error#1{\DN@{#1}%
 \xyerror@{illegal <coord> (\codeof\next@): illegal [...] target form}{}%
 \xyFN@\xymatrixCOORD@ii}
\xydef@\xymatrixCOORD@other#1,#2]{%
 \advance\count@#1\advance\count@@#2\xymatrixCOORD@x}
\xydef@\xymatrixCOORD@x{%
 \DN@##1{\xy@@{%
 \expandafter\let\expandafter\next@\csname Q@##1\endcsname
 \ifx\next@\relax \xyerror@RC{##1}\else \next@ \fi}%
 \afterCOORD@}%
 \edef\nextii@{{\thematrixprefix@@\the\count@,\the\count@@}}%
 \expandafter\next@\nextii@}
\xydef@\xymatrixCOORD@xx{%
 \DN@##1{\xy@@{%
 \expandafter\let\expandafter\next@\csname Q@##1\endcsname
 \ifx\next@\relax \xyerror@RC{##1}\else \next@\no@@ \fi}%
 \afterPLACE\xymatrixCOORD@after}%
 \edef\nextii@{{\thematrixprefix@@\the\count@,\the\count@@}}%
 \expandafter\next@\nextii@}
\xydef@\xymatrixCOORD@after{%
 \ifx ]\next \DN@]{\afterCOORD@}%
 \else \let\next@=\xymatrixCOORD@error \fi \next@}
\xydef@\xyerror@RC#1{\xyerror@{in entry \string"\the\Row,\the\Col\string":
 No \codeof\thematrixCOORD@@\space(is \string"#1\string") from here}{}}
\xylet@\xymatrix@addop@@=\relax
\xydef@\xymatrix@at{\def\xymatrix@addop@@{\xymatrix@R\xymatrix@C}%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\xymatrix@at}%
 \else\ifx !\next \DN@!{\xyFN@\xymatrix@fix}%
 \else\addPLUS@\ifx \next \let\next@=\xymatrix@addop
 \else\addDASH@\ifx \next \let\next@=\xymatrix@addop
 \else\addEQ@\ifx \next \let\next@=\xymatrix@addop
 \else\ifx 1\next \DN@1{\def\everyentry@{\vphantom(}%
 \let\objectmargin@=\p@ \xyFN@\xymatrix@setup}%
 \else\ifx R\next \def\xymatrix@addop@@{\xymatrix@R}\DN@ R{\xymatrix@addop}%
 \else\ifx C\next \def\xymatrix@addop@@{\xymatrix@C}\DN@ C{\xymatrix@addop}%
 \else\ifx M\next \def\xymatrix@addop@@{\xymatrix@M}\DN@ M{\xymatrix@addop}%
 \else\ifx L\next \def\xymatrix@addop@@{\xymatrix@L}\DN@ L{\xymatrix@addop}%
 \else\ifx H\next \def\xymatrix@addop@@{\xymatrix@H}\DN@ H{\xymatrix@addop}%
 \else\ifx W\next \def\xymatrix@addop@@{\xymatrix@W}\DN@ W{\xymatrix@addop}%
 \else\ifx *\next \DN@*{\xyFN@\xymatrix@mods}%
 \else \DN@{\afterDIRECTIONorEMPTY
 {\xymatrix@rotation \xyFN@\xymatrix@setup}{%
 \xyerror@{<addop> or <direction> or one of RCMLHW*! expected}{}%
 \xyFN@\xymatrix@setup}}%
 \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi \next@}
\xydef@\xymatrix@fix{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\xymatrix@fix}%
 \else\ifx R\next \let\mkHrow@=\Hrow@max \DN@ R{\xyFN@\xymatrix@fix@}%
 \else\ifx C\next \let\mkWcol@=\Wcol@max \DN@ C{\xyFN@\xymatrix@fix@}%
 \else \let\mkHrow@=\Hrow@HWmax \let\mkWcol@=\Wcol@HWmax
 \let\next@=\xymatrix@fix@
 \fi\fi\fi \next@}
\xydef@\xymatrix@fix@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\xymatrix@fix@}%
 \else\ifx 0\next \def\mkHWmax@{\HWmax@set\z@}\DN@ 0{\xyFN@\xymatrix@setup}%
 \else\addEQ@\ifx\next \addEQ@\DN@{\afterassignment\xymatrix@fix@x\dimen@ii=}%
 \else \let\mkHWmax@=\HWmax@max \let\next@=\xymatrix@setup \fi\fi\fi \next@}
\xydef@\xymatrix@fix@x{%
 \edef\mkHWmax@{\noexpand\HWmax@set{\the\dimen@ii}}\xyFN@\xymatrix@setup}
\xydef@\xymatrix@addop{\afterADDOP{\xyFN@\xymatrix@addop@}}
\xydef@\xymatrix@addop@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\xymatrix@addop@}%
 \else\ifx R\next \DN@ R{\xy@{R}{}\dimen@ii=\xymatrixrowsep@\xymatrix@addop@x}%
 \else\ifx C\next \DN@ C{\xy@{C}{}\dimen@ii=\xymatrixcolsep@\xymatrix@addop@x}%
 \else \DN@{\afterassignment\xymatrix@addop@x\dimen@ii=}\fi\fi\fi \next@}
\xydef@\xymatrix@addop@x{\expandafter\xy@\expandafter{\the\dimen@ii}{}%
 \xymatrix@addop@@ \xyFN@\xymatrix@setup}
\xydef@\xymatrix@R{\Addop@@\xymatrixrowsep@\dimen@ii}
\xydef@\xymatrix@C{\Addop@@\xymatrixcolsep@\dimen@ii}
\xydef@\xymatrix@M{\Addop@@\objectmargin@\dimen@ii}
\xydef@\xymatrix@L{\Addop@@\labelmargin@\dimen@ii}
\xydef@\xymatrix@H{\Addop@@\objectheight@\dimen@ii}
\xydef@\xymatrix@W{\Addop@@\objectwidth@\dimen@ii}
\xydef@\xymatrixrowsep@{2pc}
\xydef@\xymatrixcolsep@{2pc}
\xydef@\xymatrixrowsep{\afterADDOP{\Addop@@\xymatrixrowsep@}}
\xydef@\xymatrixcolsep{\afterADDOP{\Addop@@\xymatrixcolsep@}}
\xydef@\xymatrix@mods{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\xymatrix@mods}%
 \else\ifx [\next
 \DN@ [##1]{\xy@{[##1]}{}\DN@####1{\def\entrymodifiers@{[##1]####1}}%
 \expandafter\next@\expandafter{\entrymodifiers@}\xyFN@\xymatrix@setup}%
 \else\addPLUS@\ifx \next \DN@##1{\DNii@{##1}\xyFN@\xymatrix@change}%
 \else\addDASH@\ifx \next \DN@##1{\DNii@{##1}\xyFN@\xymatrix@change}%
 \else\addEQ@\ifx \next \DN@##1{\DNii@{##1}\xymatrix@set}%
 \else \let\next@=\xymatrix@mods@error \fi\fi\fi\fi\fi \next@}
\xydef@\xymatrix@set{%
 \begingroup \plainxy@
 \afterVECTORorEMPTY\xymatrix@mods@x\xymatrix@mods@error}
\xydef@\xymatrix@change{%
 \addEQ@\ifx\next \DN@##1{\expandafter\DNii@\expandafter{\nextii@##1}%
 \expandafter\xy@\expandafter{\nextii@}{}\begingroup \plainxy@
 \afterVECTORorEMPTY\xymatrix@mods@x\xymatrix@mods@xx}%
 \else \DN@{\expandafter\xy@\expandafter{\nextii@}{}\begingroup \plainxy@
 \afterVECTORorEMPTY\xymatrix@mods@x\xymatrix@mods@xx}\fi
 \next@}
\xydef@\xymatrix@mods@x{\expandafter\xy@\expandafter{\nextii@}{}%
 \def\next@##1##2##3{\def\nextii@####1{##1##2####1##3}}%
 \addGT@{\addLT@{\expandafter\next@\expandafter{\nextii@}}}%
 \DN@##1{\gdef\tmp@@@{{##1}}}%
 \edef\nextiii@{{\the\X@c,\the\Y@c}}%
 \expandafter\expandafter\expandafter\next@
 \expandafter\expandafter\expandafter{\expandafter\nextii@\nextiii@}%
 \endgroup
 \DN@##1{\xy@{##1}{}\DN@####1{\def\entrymodifiers@{##1####1}}%
 \expandafter\next@\expandafter{\entrymodifiers@}\xyFN@\xymatrix@setup}%
 \expandafter\next@\tmp@@@}
\xydef@\xymatrix@mods@xx{\expandafter\xy@\expandafter{\nextii@}{}%
 \expandafter\gdef\expandafter\tmp@@@\expandafter{\expandafter{\nextii@}}%
 \endgroup
 \DN@##1{\xy@{##1}{}\DN@####1{\def\entrymodifiers@{##1####1}}%
 \expandafter\next@\expandafter{\entrymodifiers@}\xyFN@\xymatrix@setup}%
 \expandafter\next@\tmp@@@}
\xydef@\xymatrix@mods@error{\endgroup
 \xyerror@{Impossible @*<addop><size> <setup>.}{}\xyFN@\xymatrix@setup}
\xywarnifdefined\entrymodifiers
\expandafter\def\addEQ@\entrymodifiers#1{\def\entrymodifiers@{#1}\ignorespaces}
\xydef@\entrymodifiers@{\entrybox}
\xydef@\entrybox#1{\hbox{\setbox\z@=\objectbox{#1}%
 \L@p=\wdz@ \D@p=\ht\z@ \advance\D@p\dp\z@
 \dimen@=\objectwidth@ \advance\dimen@-\L@p
 \ifdim\dimen@>\z@ \advance\L@p\dimen@ \R@p=.5\dimen@ \else \R@p=\z@ \fi
 \dimen@=\objectheight@ \advance\dimen@-\D@p
 \ifdim\dimen@>\z@ \advance\D@p\dimen@ \fi
 \dimen@=\objectmargin@ \advance\L@p2\dimen@ \advance\D@p2\dimen@ 
 \U@p=-.5\ht\z@ \advance\U@p.5\dp\z@ \advance\R@p\objectmargin@
 \setboxz@h{\kern\R@p \raise\U@p\boxz@}%
 \wdz@=\L@p \ht\z@=.5\D@p \dp\z@=.5\D@p \boxz@}}
\xywarnifdefined\everyentry
\expandafter\def\addEQ@\everyentry#1{\def\everyentry@{#1}\ignorespaces}
\xylet@\everyentry@=\empty
\xyendinput


==> xymovie.tex <==
%% xymovie.tex from $Id: xymovie.doc,v 3.5 1997/05/28 13:05:01 krisrose Exp $
%%
%% Xy-pic ``Movie Storyboard extension'' option.
%% Copyright (c) 1996-1997 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1997 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{movie}{Movie Storyboard extension}{\stripRCS$Revision: 3.5 $}%
 {Kristoffer H.~Rose}{krisrose@brics.dk}%
 {BRICS/Computer Science, University of Aarhus, Ny Munkegade, building 540,
 DK--8000 Aarhus~C}
\xynew@{dimen}\m@height
\xynew@{dimen}\m@width
\xydef@\extractparameterm@#1#2#3{%
 \DN@##1,#1=##2,##3@{\csname m@#1\endcsname=##2\relax}%
 \next@,#2,#3,@}
\xydef@\MovieSetup#1{%
 \extractparameterm@{height}{#1}{height=2in}%
 \extractparameterm@{width}{#1}{width=2in}%
}
\xydef@\theScene{0}
\xydef@\theF{0}
\xydef@\theFr{1}
\xydef@\F#1{#1(0)}
\xydef@\Fr#1{#1(1)}
\xynew@{if}\iflastframe@
\xynew@{count}\m@scene
\xydef@\scene{\advance\m@scene\@ne
 \DN@{\ifx*\next \lastframe@true \DN@*{\xyFN@\scene@}%
 \else \let\next@=\scene@ \fi \next@}%
 \xyFN@\next@}
\xydef@\scene@{%
 \ifx[\next \DN@[##1]{\scene@i}\else \let\next@=\scene@i \fi \next@}
\long\def\scene@i#1{{%
 \def\caption##1{\gdef\m@caption{Scene \the\m@scene. ##1}}%
 \edef\theScene{\the\m@scene}%
 \def\theF{0}\def\theFr{1}%
 \def\F##1{##1(0)}\def\Fr##1{##1(1)}%
 \scene@frame{#1}%
 \iflastframe@
 \def\caption##1{}%
 \gdef\m@caption{The End.}%
 \def\theF{1}\def\theFr{0}%
 \def\F##1{##1(1)}\def\Fr##1{##1(0)}%
 \scene@frame{#1}%
 \fi
 }\ignorespaces}
\def\scene@frame#1{\vbox{\null
 \dimen@=\m@width \advance\dimen@2\xydashw@
 \hrule width\dimen@
 \hbox to\dimen@{\vrule width\xydashw@ \hss
 \vbox to\m@height{\hsize=\m@width \null\vfil{#1}\vfil\null}%
 \hss \vrule width\xydashw@}%
 \hrule width\dimen@
 \setbox0=\hbox{%
 \setbox0=\hbox to\m@width{\hss\strut \m@caption\hss}%
 \dimen0=\dp0 \ht0=0pt \dp0=0pt \raise\dimen0\box0}%
 \ht0=0pt \dp0=0pt \box0\relax
 \null}}
\xyendinput


==> xynecula.tex <==
%% xynecula.tex from $Id$
%%
%% Xy-pic ``Necula extensions'' option.
%% Copyright (c) 1998 George C. Necula <necula@cs.cmu.edu>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1998 Kristoffer H. Rose <krisrose@ens-lyon.fr>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{necula}{Necula's extensions}{\stripRCS$Revision: 0.0 $}%
 {George C. Necula}{necula@cs.cmu.edu}%
 {School of Computer Science,
 Carnegie Mellon University,
 5000 Forbes Avenue,
 Pittsburgh, PA 15213-3891, USA}
\def\expandbeforenext@#1{%
 \DN@ e|##1|{\edef\tmp@{##1}\expandafter\xyFN@\expandafter#1\tmp@}%
}
\xylet@\xy@oldOBJECT@=\OBJECT@
\xydef@\xy@newOBJECT@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\xy@newOBJECT@}%
 \else\ifx e\next
 \expandbeforenext@\OBJECT@
 \else
 \DN@{\xy@oldOBJECT@}\fi\fi
 \next@}%
\let\OBJECT@=\xy@newOBJECT@
\xylet@\xy@oldCOORD@=\COORD@
\xydef@\xy@newCOORD@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\xy@newCOORD@}%
 \else\ifx e\next
 \expandbeforenext@\COORD@
 \else
 \DN@{\xy@oldCOORD@}\fi\fi
 \next@}%
\let\COORD@=\xy@newCOORD@
\xydefcsname@{*stylechar@P@}#1{\Pshape@#1@}
\xynew@{count}\c@poly@count \c@poly@count=\z@
\xydef@\Pshape@:#1@{%
 \addtotoks@{%
 \def\poly@list{@}%
 \poly@parse #1,\relax,%Sets the poly@list
 \def\poly@cache{}%
 \edef\poly@id{\the\c@poly@count}%
 \global\advance\c@poly@count\@ne
 \poly@setEdge
 \edef\poly@saveLcshape{\the\L@c}%
 \polygonEdge@Outer% Set U,R,D,L
 \poly@setEdge
 \dimen@=\poly@saveLcshape\advance\dimen@-\L@c
 \advance\R@p -\dimen@
}}
\xydef@\poly@setEdge{\expandafter\poly@setEdge@\poly@list\poly@id}
\xydef@\poly@setEdge@#1@#2{\Edge@c={\polygonEdge#1@#2@}%
 \expandafter\xdef\csname poly@cache#2%
 \endcsname{\poly@cache}}
\xydefcsname@{frm[P]{-}}{\expandafter\draw@polyframe\the\Edge@c{-}}
\xydefcsname@{frm[P]{.}}{\expandafter\draw@polyframe\the\Edge@c{.}}
\xydefcsname@{frm[P]{=}}{\expandafter\draw@polyframe\the\Edge@c{=}}
\xydef@\draw@polyframe\polygonEdge#1@#2@#3{%
 \def\poly@dir{#3}%
 \def\poly@list{#1@}%
 \def\poly@id{#2}%
 \edef\poly@cache{\csname poly@cache\poly@id\endcsname}%
 \draw@polygon}
\xydef@\poly@empty{}
\xydef@\poly@map#1#2,#3;#4@{%
 #1{#2}{#3}%
 \def\tmp@{#4}%
 \ifx \poly@empty\tmp@ \else
 \poly@map@next#1#4@%
 \fi
}
\xydef@\poly@map@stop#1@{}
\xydef@\poly@mapExpand#1#2{%
 \edef\tmp@{\noexpand\poly@map\noexpand #1#2}%
 \tmp@}
\xydef@\poly@parse #1,{%
 \ifx #1\relax
 \poly@close
 \let\next@=\relax
 \else
 \save@
 \POS #1%
 \edef\tmp@{{\the\X@c}{\the\Y@c}}%
 \expandafter\poly@append\tmp@
 \restore
 \let\next@=\poly@parse
 \fi
 \next@
}
\xydef@\poly@append#1#2{\expandafter\poly@append@\poly@list{#1,#2;}}
\xydef@\poly@append@#1@#2{\global\def\poly@list{#1#2@}}
\xydef@\poly@close{\expandafter\poly@close@\poly@list}
\xydef@\poly@close@#1,#2;#3@{\poly@append{#1}{#2}}
\xydef@\draw@polygon{%
 \save@
 \X@origin=\X@c \Y@origin=\Y@c
 \poly@setp
 \U@c=\z@\R@c=\z@\D@c=\z@\L@c=\z@\U@p=\z@\R@p=\z@\D@p=\z@\L@p=\z@
 \Edge@c={\zeroEdge}\Edge@p={\zeroEdge}%
 \let\poly@map@next=\poly@map
 \poly@mapExpand\poly@drawseg\poly@rest
 \restore
}
\xydef@\poly@setp{\expandafter\poly@setp@\poly@list}
\xydef@\poly@setp@#1,#2;#3@{%
 \X@p=#1\advance\X@p\X@origin \Y@p=#2\advance\Y@p\Y@origin%
 \global\def\poly@rest{#3@}}
\xydef@\poly@drawseg#1#2{%
 \dimen@=#1\X@c=\the\dimen@\advance\X@c \X@origin
 \dimen@=#2\Y@c=\the\dimen@\advance\Y@c \Y@origin
 \expandafter\connect@\expandafter\dir\poly@dir%
 \X@p=\X@c\Y@p=\Y@c}
\xydef@\polygonEdge#1@#2@#3{%
 \def\poly@list{#1@}%
 \def\poly@id{#2}%
 \edef\poly@cache{\csname poly@cache\poly@id\endcsname}%
 \ifcase#3\relax
 \DN@{\polygonEdge@Inters
 }%
 \or \DN@{\polygonEdge@Under}%
 \or \DN@{\polygonEdge@Dist}%
 \or \DN@{\rectangleProp@}%
 \or \DN@{\polygonEdge@Inner}%
 \or \DN@{\polygonEdge@Outer}%
 \else \DN@{}\fi
 \next@}
\newif\ifpoly@badinters
\xydef@\polygonEdge@Inters{%
 \ifx\poly@cache\poly@empty
 \poly@intersdoit
 \else
 \expandafter\poly@intersprobecache\poly@cache @%
 \fi
}
\xydef@\poly@cachehit#1#2{%
 \X@c=#1\Y@c=#2}
\xydef@\poly@cachehitdisable#1#2{\poly@intersdoit}
\xydef@\poly@intersprobecache#1,#2,#3,#4,#5@{%
 \dimen@=#1\advance\dimen@-\d@X
 \ifdim\zz@\dimen@
 \dimen@=#2\advance\dimen@-\d@Y
 \ifdim\zz@\dimen@
 \poly@cachehit{#3}{#4}
 \else
 \poly@intersdoit
 \fi
 \else
 \poly@intersdoit
 \fi
}
\xydef@\poly@intersdoit{%
 \edef\polyoldA@{\the\A@}\edef\polyoldB@{\the\B@}%
 \def\poly@intersneg{}\def\poly@interspos{}%
 \save@
 \poly@setorigin
 \def\zeroDivide@{\poly@badinterstrue}%
 \let\poly@map@next=\poly@map
 \poly@mapExpand\poly@interseg\poly@rest
 \ifx\poly@intersneg\poly@empty
 \poly@badinterstrue
 \else
 \ifx\poly@interspos\poly@empty
 \poly@badinterstrue
 \else
 \poly@badintersfalse
 \fi
 \fi
 \restore
 \A@=\polyoldA@\B@=\polyoldB@
 \ifpoly@badinters \else
 \edef\tmp@{\poly@interspos,\poly@intersneg @}%
 \expandafter\poly@intersfinish\tmp@
 \fi
}
\xydef@\poly@intersfinish#1,#2,#3@{%
 \X@c=#1\Y@c=#2\relax
 \xdef\poly@cache{\the\d@X,\the\d@Y,#1,#2,#3}%
 \poly@setEdge
}
\xydef@\poly@setorigin{\expandafter\poly@setorigin@\poly@list}
\xydef@\poly@setorigin@#1,#2;#3@{%
 \X@origin=#1\advance\X@origin\X@c \Y@origin=#2\advance\Y@origin\Y@c%
 \global\def\poly@rest{#3@}}
\xydef@\poly@interseg#1#2{%
 \dimen@=#1\advance\dimen@\X@c \edef\poly@saveXcinters{\the\dimen@}%
 \dimen@=#2\advance\dimen@\Y@c \edef\poly@saveYcinters{\the\dimen@}%
 \save@
 \poly@badintersfalse
 \R@c=\poly@saveXcinters \advance\R@c -\X@origin
 \U@c=\poly@saveYcinters \advance\U@c -\Y@origin
 \intersect@
 \A@=\X@c \B@=\Y@c
 \restore
 \ifpoly@badinters
 \else
\poly@isonseg\X@origin\Y@origin\A@\B@\poly@saveXcinters\poly@saveYcinters
 \ifpoly@badinters
 \else
 \poly@isonray\X@c\Y@c\A@\B@\X@p\Y@p
 \ifpoly@badinters
 \edef\poly@intersneg{\the\A@,\the\B@}%
 \else
 \edef\poly@interspos{\the\A@,\the\B@}%
 \fi
 \fi
 \fi
 \X@origin=\poly@saveXcinters\Y@origin=\poly@saveYcinters
}
\xydef@\polygonEdge@Dist{\xyerror@{Dist is not yet implemented for polygons}}
\newif\ifpoly@closedrange
\xydef@\poly@isinrange#1#2#3{%
 \ifpoly@badinters \else
 \dimen@=#1\dimen@i=#2\dimen@ii=#3\relax
 \advance\dimen@ii -\dimen@ \advance\dimen@i -\dimen@
 \ifdim\dimen@ii<0pt\relax
 \ifdim\dimen@i>100\almostz@
 \poly@badinterstrue
 \fi
 \dimen@i=-\dimen@i \dimen@ii=-\dimen@ii
 \else
 \ifdim\dimen@i<-100\almostz@\relax
 \poly@badinterstrue
 \fi
 \fi
 \ifpoly@closedrange
 \advance\dimen@ii 100\almostz@
 \ifdim\dimen@i>\dimen@ii
 \poly@badinterstrue
 \fi
 \fi
 \fi}
\xydef@\poly@isonseg#1#2#3#4#5#6{%
 \poly@closedrangetrue
 \poly@isinrange{#1}{#3}{#5}%
 \poly@isinrange{#2}{#4}{#6}%
}
\xydef@\poly@isonray#1#2#3#4#5#6{%
 \poly@closedrangefalse
 \poly@isinrange{#1}{#3}{#5}%
 \poly@isinrange{#2}{#4}{#6}%
}
\xydef@\polygonEdge@Under{%
 \edef\polysaveA@under{\the\A@}\edef\polysaveB@under{\the\B@}%
 \edef\poly@saveXcUnder{\the\X@c}\edef\poly@saveYcUnder{\the\Y@c}%
 \polygonEdge@Inters
 \ifpoly@badinters% p is very close to c
 \Inside@true
 \else
 \A@=\X@c\B@=\Y@c
 \X@c=\poly@saveXcUnder\Y@c=\poly@saveYcUnder
 \poly@isonseg\X@c\Y@c\X@p\Y@p\A@\B@
 \ifpoly@badinters \Inside@false \else \Inside@true\fi
 \A@=\polysaveA@under\B@=\poly@saveB@under
 \fi
}
\xydef@\polygonEdge@Inner{%
 \enter@{\basefromthebase@ \pfromthep@ \DirectionfromtheDirection@}%
 \L@c=\X@c \D@c=\Y@c
 \polygonEdge@Inters
 \ifpoly@badinters
 \czeroEdge@
 \else
 \expandafter\poly@getinterspoints\poly@cache @%
 \ifdim\X@c>\R@c
 \L@c=\R@c \R@c=\X@c
 \else
 \L@c=\X@c
 \fi
 \X@c=0.5\L@c \advance\X@c 0.5\R@c \advance\R@c -\X@c \L@c=\R@c
 \ifdim\Y@c>\U@c
 \D@c=\U@c \U@c=\Y@c
 \else
 \D@c=\Y@c
 \fi
 \Y@c=0.5\D@c \advance\Y@c 0.5\U@c \advance\U@c -\Y@c \D@c=\U@c
 \Edge@c={\rectangleEdge}%
 \fi
 \leave@
}
\xydef@\poly@getinterspoints#1,#2,#3,#4,#5,#6@{%
 \R@c=#3\U@c=#4\X@c=#5\Y@c=#6}
\xydef@\polygonEdge@Outer{%
 \enter@{\basefromthebase@ \pfromthep@ \DirectionfromtheDirection@}%
 \czeroEdge@
 \let\poly@map@next=\poly@map
 \poly@mapExpand\poly@findextent\poly@list
 \Edge@c={\rectangleEdge}%
 \leave@
}
\xydef@\poly@findextent#1#2{%
 \dimen@=#1\dimen@=\the\dimen@% it fails if I remove the second assign
 \ifdim\dimen@>\R@c \R@c=\dimen@ \fi
 \ifdim -\dimen@>\L@c \L@c=-\dimen@ \fi
 \dimen@=#2\dimen@=\the\dimen@% it fails if I remove the second assign
 \ifdim\dimen@>\U@c \U@c=\dimen@ \fi
 \ifdim -\dimen@>\D@c \D@c=-\dimen@ \fi
}
\xydef@\Fshape@#1:{\def\whichframe@@{{#1}}\let\whichoptions@@=\empty
 \DN@{{}}\ifx\whichframe@@\next@ \def\whichframe@@{{-}}\fi
 \expandafter\xyFN@\expandafter\Fshape@whichframe\the\Edge@c}
\xydef@\Fshape@whichframe{%
 \ifx\next\circleEdge
 \edef\whichframe@@{[o]\whichframe@@}%
 \DN@##1{\xyFN@\Fshape@i}%
 \else
 \ifx\next\polygonEdge
 \edef\whichframe@@{[P]\whichframe@@}%
 \DN@\polygonEdge##1@##2@{\xyFN@\Fshape@i}%
 \else
 \DN@##1{\xyFN@\Fshape@i}%
 \fi\fi
 \next@
}
\xyendinput


==> xyoztex.tex <==
%% xyoztex.tex from $Id: xyoztex.doc,v 3.3 1996/12/18 09:26:26 ross Exp $
%%
%% Xy-pic ``OzTeX'' driver interface option.
%% Copyright (c) 1995-1996 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1996 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{oztex}{OzTeX driver}{\stripRCS$Revision: 3.3 $}%
 {Ross Moore}{ross@mpce.mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xydef@\OzTeX@@#1{\dvimessage@{OzTeX}{#1}}
\newdriver{%
 \xyaddsupport{color}\oztexColor@@
 \xyaddsupport{crayon}\oztexCrayon@@
 \xyaddsupport{ps}\oztexPS@@
 \xyaddsupport{rotate}\oztexRotate@@
 \xyaddsupport{line}\oztexLine@@
 \xyaddsupport{frame}\oztexFrames@@
 \xyaddsupport{tile}\oztexTiles@@
 \xyaddsupport{cmtip}\relax
}
\xydef@\oztexColor@@{\OzTeXColours@}
\xydef@\OzTeXColours@{\OzTeXPStypes@
 \let\xylocalColor@=\xyNoColor@@ \def\xycolor@{\xycolor@@}%
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-c}{\xydrivernoload@{ps-c}}%
 \installPScolor@ }\else\DN@{}\fi \next@
 \ifx\xycrayolaloaded\empty \DN@{\xystandardcolors@\OzTeXCrayon@@{}}%
 \else\let\next@=\xystandardcolors@\fi \next@
 \let\xycolorwarning@=\relax 
 \let\oztexColor@@=\relax
 \let\UnloadColor@@=\NoOzTeXColor@
}
\xydef@\NoOzTeXColor@{%
 \let\xylocalColor@=\xyNoColor@@
 \let\xycolor@=\xyNoColor@
 \let\xycolorwarning@=\xycolorwarning@@
 \let\oztexColor@@=\OzTeXColours@
 \let\UnloadColor@@=\UnloadColor@
 }
\xydef@\OzTeXCrayon@@{\installCrayolaColors@}
\xydef@\oztexPS@@{\oztexPS@}
\xydef@\oztexPSunload@{\UnloadPS@
 \def\xyPSdictname{}\UsePSdict@@false
 \let\installxyps@@=\relax
 \let\UnloadPS@@=\UnloadPS@
 \xyPSshapes@true 
 \let\oztexPS@@=\oztexPS@ }
\xydef@\OzTeXSpecial@#1{\special{empty.ps {#1}xy}}
\xydef@\OzTeXMacro@#1{\special{empty.ps {#1}xy}}
\xydef@\OzTeXDict@#1{\special{empty.ps @bxy{#1}stopped pop @exy}}
\xydef@\OzTeXinclude@#1{\special{#1}}
\xydef@\OzTeXraw@#1{\special{empty.ps @bxy #1 @exy}}%
\xydef@\OzTeXPStypes@{%
 \xyinputorelse@{xyps-ps}{\xydrivernoload@{ps-ps}}%
 \ifx\PSspecial@@\OzTeXSpecial@\else
 \let\PSspecial@@=\OzTeXSpecial@
 \let\PSmacro@@=\OzTeXMacro@
 \let\PSdict@@=\OzTeXDict@
 \let\PSraw@@=\OzTeXraw@
 \let\PSinclude@@=\OzTeXinclude@
 \let\xyPSobeylines@@=\obeyOzTeXlines@
 \let\PSspecialdict@@=\OzTeXDict@
 \OzTeX@@{PostScript}%
 \fi
 \OzTeXCurrpt@ }
{\catcode`\^^M=\active
 \gdef\next{\catcode`\^^M=\active \let^^M=\space \obeyspaces}}
\xylet@\obeyOzTeXlines@=\next
\xydef@\OzTeXCurrpt@{\let\xyPScurrpt@@=\OzTeXCurrpt@@}%
\xydef@\OzTeXCurrpt@@{\PSraw@@{xyp}}
\xydef@\oztexPS@{\OzTeXPStypes@ 
 \let\oztexPS@@=\relax
 \let\UnloadPS@@=\oztexPSunload@
 \let\installxyps@@=\@OzTeX@PS@
 \installxyps@ }
\xydef@\@OzTeX@PS@{\UsePSdict@@true
 \let\includePSmessage@=\xyOzTeXheader 
 \ifx\undefined\xyPSdictname\def\xyPSdictname{global.ps}\fi}
\xydef@\xyOzTeXheader#1#2#3{\UsePSdict@@true}
\xydef@\oztexLine@@{\oztexLine@}
\xydef@\oztexLine@{\OzTeXPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-l}{\xydrivernoload@{ps-l}}\installPSline@ }%
 \else\DN@{\xydriverfail@{line-styles are}\UnloadLine@\relax}\fi
 \next@ }
\xydef@\oztexFrames@@{\OzTeXFrames@}
\xydef@\OzTeXFrames@{\OzTeXPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-f}{\xydrivernoload@{ps-f}}\installPSframes@ }%
 \else\DN@{\xydriverfail@{frames are}\UnloadPSFrames@\relax}\fi
 \next@ }
\xydef@\oztexTiles@@{\OzTeXTiles@}
\xydef@\OzTeXTiles@{\OzTeXPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-t}{\xydrivernoload@{ps-t}}\installPSpatterns@
 \xystandardpatterns@ }%
 \else\DN@{\xydriverfail@{Patterns are}\UnloadPSpatterns@\relax}\fi
 \next@ }
\xydef@\oztexRotate@@{\OzTeXRotate@}
\xydef@\OzTeXRotate@{\OzTeXPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-r}{\xydrivernoload@{ps-r}}%
 \OzTeXRotScale@ \installPSrotscale@ \xyPSshapes@false }%
 \else\DN@{\xydriverfail@{rotations are}\UnloadRotate@\relax}\fi
 \next@ }
\xydef@\OzTeXRotScale@{%
 \def\xyrot@start(##1){%
 {xyp xyt ##1\space xyr}{OzXy begin gsave}}%
 \def\xyscale@start(##1,##2){%
 {xyp xyt ##1\space##2\space xys}{OzXy begin gsave}}%
 \def\xyrot@end{grestore end}\def\xyscale@end{grestore end}}
\let\OzTeXRotScale@=\xyRotScale@@
\xyendinput


==> xypic.tex <==
%% xypic.tex from $Id: xypic.doc,v 3.3 1996/12/19 03:31:56 krisrose Exp $
%%
%% Xy-pic v2 compatibility loading.
%% Copyright (c) 1993-1996 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1996 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\input xyv2
\endinput


==> xypoly.tex <==
%% xypoly.tex from $Id: xypoly.doc,v 3.7 1999/02/16 15:12:50 krisrose Exp $
%%
%% Xy-pic ``Polygon'' feature.
%% Copyright (c) 1994-1997 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1997 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this macro package; if not, write to the Free Software Foundation,
%% Inc., 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{poly}{Polygon feature}{\stripRCS$Revision: 3.7 $}%
 {Ross Moore}{ross@mpce.mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xyrequire{arrow}\xycatcodes
\message{polygons,}
\xynew@{count}\xypolynode@\xypolynode@=\m@ne
\xydef@\xypolynode{\the\xypolynode@}
\xydef@\xypolyNUMSIDES@{}
\xydef@\xypolynum{\xypolyNUMSIDES@}
\xydef@\xypolygon{\xypoly@}%
\xydef@\xypoly@{%
 \if\inxy@ 
 \if\inxypoly@
 \edef\next@{\noexpand\xy@@{\noexpand\nter@{\xypolynode@=\the\xypolynode@
 \noexpand\def\noexpand\xypolyNUMSIDES@{\xypolyNUMSIDES@}}}}%
 \else
 \DN@{\xy@@{\def\inxypoly@{TT}%
 \nter@{\def\inxypoly@{TF}\xypolynode@=\m@ne}}}%
 \fi
 \else
 \if\inxypoly@
 \edef\next@{\noexpand\xy 
 \noexpand\xy@@{\noexpand\nter@{\xypolyside=\the\xypolyside
 \noexpand\def\noexpand\xypolyNUMSIDES@{\xypolyNUMSIDES@}\endxy}}}%
 \else
 \DN@{\xy \xy@@{\def\inxypoly@{TT}%
 \nter@{\def\inxypoly@{TF}\xypolynode@=\m@ne \endxy}}}%
 \fi
 \fi
 \next@ \count@=\z@ \xyFN@\xypoly@n}
\xydef@\inxypoly@{TF}%
\xydef@\xypoly@x{\xy@@{\leave@\leave@}}
\xydef@\xypoly@n{%
 \DN@##1{\multiply\count@10\relax \advance\count@##1\relax \xyFN@\xypoly@n}%
 \ifx \space@\next
 \ifnum\count@>\z@ \expandafter\DN@\space@{\xyFN@\xypoly@i}%
 \else \expandafter\DN@\space@{\xyFN@\xypoly@n}\fi
 \else\ifx 0\next \else\ifx 1\next \else\ifx 2\next \else\ifx 3\next
 \else\ifx 4\next \else\ifx 5\next \else\ifx 6\next \else\ifx 7\next
 \else\ifx 8\next \else\ifx 9\next
 \else \let\next@=\xypoly@i \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi \next@}
\xydef@\xypoly@i{\edef\xypolyNUMSIDES@{\the\count@}\xyFN@\xygetpolyprefix@}
\xydef@\xypolyPREFIX@{}%
\xydef@\xypolyPREFIX@@{}%
\xydef@\xypolyname{\xypolyPREFIX@}%
\xydef@\xygetpolyprefix@{%
 \ifx\next"\DN@"##1"{\def\xypolyPREFIX@@{##1}\expandafter
 \edef\csname\xypolyPREFIX@@ NUMSIDES\endcsname{\xypolyNUMSIDES@}%
 \xypolyprefix@@ }%
 \else 
 \ifnum\xypolynode@<\z@\def\xypolyPREFIX@@{}%
 \else
 \edef\xypolyPREFIX@@{\xypolyPREFIX@\the\xypolynode@,}%
 \fi \DN@{\xypolyprefix@@}%
 \fi \next@ }
\xydef@\xypolyprefix@@{%
 \expandafter\toks@\expandafter{\addEQ@\POS"}%
 \expandafter\addtotoks@\expandafter{\xypolyPREFIX@@0"\relax}%
 \the\toks@ 
 \ifnum\xypolynode@<\z@
 \expandafter\def\expandafter\xypolyPREFIX@\expandafter{\xypolyPREFIX@@}%
 \xy@@{\enter@{\xypolynode@=\the\xypolynode@
 \noexpand\def\noexpand\xypolyPREFIX@{\xypolyPREFIX@}}\xypolynode@=\z@ }%
 \else
 \xy@@{\enter@{\xypolynode@=\the\xypolynode@
 \noexpand\def\noexpand\xypolyPREFIX@{\xypolyPREFIX@}}\xypolynode@=\z@ }%
 \expandafter\def\expandafter\xypolyPREFIX@\expandafter{\xypolyPREFIX@@}%
 \fi
 \xypoly@@i }
\xydef@\xypoly@@i#1#{\begingroup
 \DN@{#1}\ifx\next@\empty\else
 \xywarning@{discarding unused tokens: #1}\fi \xypoly@@ }
\xydef@\xypoly@@#1{\xypolydefaults@
 \DN@{#1}\ifx\next@\empty\DN@{\xypoly@@@}%
 \else \DN@{\xyFN@\xypolyparams@#1~!}\fi \next@}
\xydef@\xypolydefaults@{\def\xypolySCALE@{}%
 \def\xypolySPOKES@{{}}\def\xypostSPOKES@{}\let\xypreSPOKES@\relax
 \def\xypolySIDES@{{-}}\def\xypostSIDES@{}\let\xypreSIDES@\relax
 \def\xypolyVERTEX@{}\def\xypolyALIGN@{}}
{\xyuncatcodes \gdef\next{*=0}}
\xylet@\xypolynullvertex@=\next
{\xyuncatcodes \gdef\next{*[o]}}
\xylet@\xypolyvertex@=\next
{\xyuncatcodes \gdef\next{*+[o]}}
\xylet@\xypolywidevertex@=\next
\xydef@\xypolyparams@{%
 \ifx\space@\next \expandafter\DN@\space{\xyFN@\xypolyparams@}%
 \else\ifx\next~\DN@~{\xyFN@\xypolywhich@}%
 \else\ifx\next\bgroup\DN@##1~!{%
 \ifx\empty\xypolyVERTEX@\expandafter
 \def\expandafter\xypolyVERTEX@\expandafter{\xypolyvertex@{##1}}%
 \else\xypolyVERTEXerror@{##1}\fi \xypoly@@@}%
 \else\DN@##1~!{\DN@{##1}\ifx\next@\empty\else
 \ifx\empty\xypolyVERTEX@\def\xypolyVERTEX@{*##1}%
 \expandafter\checkpolytok@\expandafter\xypolyVERTEX@
 \expandafter{\xypolynullvertex@}##1@@!\relax
 \else\xypolyVERTEXerror@{##1}\fi\fi \xypoly@@@}%
 \fi\fi\fi \next@ }
\xydef@\xypolyVERTEXerror@#1{\xywarning@{%
 vertex already specified, discarding unused tokens:#1}}
\xydef@\xypolywhich@{%
 \ifx\next!\DN@!{\xypoly@@@}%
 \else \addLT@\ifx\next \addLT@\DN@{\xyFN@\xypoly@SPOKES@}%
 \else \addGT@\ifx\next \addGT@\DN@{\xyFN@\xypoly@SIDES@}%
 \else \addEQ@\ifx\next \addEQ@\DN@##1{%
 \def\xypolyALIGN@{##1}\xyFN@\xypolyparams@ }%
 \else \ifx :\next \DN@:##1{%
 \def\xypolySCALE@{##1}\xyFN@\xypolyparams@ }%
 \else\ifx\next*\DN@*##1{\expandafter
 \def\expandafter\xypolyVERTEX@\expandafter{\xypolywidevertex@{##1}}%
 \xyFN@\xypolyparams@}%
 \fi\fi\fi\fi\fi\fi \next@ }
\xydef@\xypoly@SPOKES@{%
 \addLT@\ifx\next \addLT@\DN@##1{%
 \def\xypreSPOKES@{##1}\def\xypolySPOKES@{}\xyFN@\xypolyparams@ }%
 \else \addGT@\ifx\next \addGT@\DN@##1{%
 \def\xypostSPOKES@{##1}\xyFN@\xypolyparams@ }%
 \else \ifx\next\bgroup \DN@##1{%
 \def\xypolySPOKES@{##1}\let\xypreSPOKES@\relax
 \checkpolytok@\xypolySPOKES@{}##1@@!{\xyFN@\xypolyparams@}}%
 \else \DN@##1{%
 \let\xypreSPOKES@\relax \def\xypolySPOKES@{{##1}}\xyFN@\xypolyparams@}%
 \fi\fi\fi \next@ }
\xydef@\xypoly@SIDES@{%
 \addLT@\ifx\next \addLT@\DN@##1{%
 \def\xypreSIDES@{##1}\def\xypolySIDES@{}\xyFN@\xypolyparams@ }%
 \else \addGT@\ifx\next \addGT@\DN@ ##1{%
 \def\xypostSIDES@{##1}\xyFN@\xypolyparams@ }%
 \else \ifx\next\bgroup \DN@##1{%
 \def\xypolySIDES@{##1}\let\xypreSIDES@\relax
 \checkpolytok@\xypolySIDES@{}##1@@!{\xyFN@\xypolyparams@}}%
 \else \DN@##1{%
 \let\xypreSIDES@\relax \def\xypolySIDES@{{##1}}\xyFN@\xypolyparams@}%
 \fi\fi\fi \next@ }
\xydef@\checkpolytok@#1#2#3#4@!#5{\DNii@{#1}\DN@{#4}%
 \ifx\next@\empty\expandafter\def\nextii@{{}}%
 \else\ifx#4@\expandafter\def\nextii@{#2{#3}}\fi\fi #5}
\xydef@\xytrigerror@#1#2{\string#1 only works from 0 to 12}
\xydef@\cosPIon#1{\ifcase#1 1\or-1\or0\or.5\or\halfroottwo\or
 .809017\or\halfrootthree\or.900969\or.92388\or.939693\or.951057\or
 .959493\or.965926\else1\xytrigerror@\cosPIon{#1}\fi}
\xydef@\sinPIon#1{\ifcase#1 0\or0\or1\or\halfrootthree\or\halfroottwo\or
 .587785\or.5\or.433884\or.382683\or.34202\or.309017\or
 .281733\or.258819\else0\xytrigerror@\sinPIon{#1}\fi}
\xydef@\cosTwoPIon#1{\ifcase#1 1\or1\or-1\or-\cosPIon3\or\cosPIon2\or
 \sinPIon{10}\or\cosPIon3\or.62349\or\cosPIon4\or
 .766044\or\cosPIon5\or.841254\or\cosPIon6%
 \else1\xytrigerror@\cosTwoPIon{#1}\fi}
\xydef@\sinTwoPIon#1{\ifcase#1 0\or0\or0\or-\sinPIon3\or\sinPIon2\or
 \cosPIon{10}\or\sinPIon3\or.781831\or\sinPIon4\or
 .642788\or\sinPIon5\or.540641\or\sinPIon6%
 \else0\xytrigerror@\sinTwoPIon{#1}\fi}
\xydef@\cosThreePIon#1{\ifcase#1 1\or-1\or0\or-1\or-\cosPIon4\or
 -\cosPIon5\or\cosPIon2\or.222521\or\sinPIon8\or\cosPIon3\or
 \sinTwoPIon5\or.654861\or\cosPIon4%
 \else1\xytrigerror@\cosThreePIon{#1}\fi}
\xydef@\sinThreePIon#1{\ifcase#1 0\or0\or1\or0\or\sinPIon4\or
 \sinTwoPIon5\or\sinPIon2\or.974928\or\cosPIon8\or\sinPIon3\or
 \cosTwoPIon5\or.75575\or\sinPIon4%
 \else0\xytrigerror@\sinThreePIon{#1}\fi}
\xydef@\cosFourPIon#1{\ifcase#1 1\or1\or1\or-\cosPIon3\or-1\or-\cosPIon5\or
 \cosTwoPIon3\or-\cosThreePIon7\or0\or.173648\or\cosTwoPIon5\or
 .415415\or\cosPIon3%
 \else1\xytrigerror@\cosFourPIon{#1}\fi}
\xydef@\sinFourPIon#1{\ifcase#1 0\or0\or0\or-\sinPIon3\or0\or\sinPIon5\or
 \sinTwoPIon3\or\sinThreePIon7\or1\or.984808\or\sinTwoPIon5\or
 .909632\or\sinPIon3%
 \else0\xytrigerror@\sinFourPIon{#1}\fi}
\xydef@\cosFivePIon#1{\ifcase#1 1\or-1\or0\or\cosPIon3\or-\cosPIon4\or
 -1\or-\cosPIon6\or-\cosTwoPIon7\or-\cosThreePIon8\or-\cosFourPIon9\or
 0\or.142315\or\sinPIon{12}%
 \else1\xytrigerror@\cosFivePIon{#1}\fi}
\xydef@\sinFivePIon#1{\ifcase#1 0\or0\or1\or-\sinPIon3\or-\sinPIon4\or
 0\or\sinPIon6\or\sinTwoPIon7\or\sinThreePIon8\or\sinFourPIon9\or1\or
 .989821\or\cosPIon{12}%
 \else0\xytrigerror@\sinFivePIon{#1}\fi}
\xydef@\xypoly@@@{\count@=\xypolyNUMSIDES@\relax
 \ifx\xypolyALIGN@\empty
 \ifnum\count@<\thr@@\relax\DN@{\xypolytoosmall@{\the\count@}}%
 \else \advance\count@-\thr@@
 \ifcase\count@ \DN@{\xyPolygon@@@\xytriangle@@}%
 \or \DN@{\xyPolygon@@@\xysquare@@}%
 \or \DN@{\xyPolygon@@@\xypentagon@@}%
 \or \DN@{\xyPolygon@@@\xyhexagon@@}%
 \or \DN@{\xyPolygon@@@\xyheptagon@@}%
 \or \DN@{\xyPolygon@@@\xyoctagon@@}%
 \or \DN@{\xyPolygon@@@\xynonagon@@}%
 \or \DN@{\xyPolygon@@@\xydecagon@@}%
 \or \DN@{\xyPolygon@@@\xyundecagon@@}%
 \or \DN@{\xyPolygon@@@\xydodecagon@@}%
 \else \DN@{\xylargePolygon@{0}{\xypolyNUMSIDES@}}%
 \fi\fi
 \else 
 \DN@{\xylargePolygon@{\xypolyALIGN@}{\xypolyNUMSIDES@}}%
 \fi \next@ \xypoly@@@x}
\xydef@\xypoly@@@x{\restore\xypoly@x}
\xydef@\xypolytoosmall@#1{\xyerror@{#1 sides is too few for a polygon}}
\xydef@\xyPolygon@@@#1{%
 \toks@={\def\xypolyNUMSIDES@}%
 \expandafter\addtotoks@\expandafter{\expandafter{\xypolyNUMSIDES@}\save}%
 \ifx\empty\xypolySCALE@ \addtotoks@{\POS"}%
 \else \addtotoks@{\POS;0;}%
 \expandafter\addtotoks@\expandafter{\xypolySCALE@\relax\POS"}%
 \fi
 \expandafter\addtotoks@\expandafter{\xypolyPREFIX@0"\relax}%
 \ifx\xypreSPOKES@\relax
 \addtotoks@{#1{;}}%
 \expandafter\addtotoks@\expandafter{\expandafter{\xypolyVERTEX@}}%
 \expandafter\addtotoks@\expandafter{\expandafter{\xypolyPREFIX@}}%
 \DN@##1\next@{\def\tmp@{**\dir##1}}%
 \expandafter\next@\expandafter{\xypolySPOKES@}\next@
 \expandafter\addtotoks@\expandafter{\expandafter{\tmp@}}%
 \else
 \expandafter\DN@\expandafter{\expandafter\ar\xypreSPOKES@}%
 \addtotoks@{#1}%
 \expandafter\addtotoks@\expandafter{\expandafter{\next@}}%
 \expandafter\addtotoks@\expandafter{\expandafter{\xypolyVERTEX@}}%
 \expandafter\addtotoks@\expandafter{\expandafter{\xypolyPREFIX@}{}}%
 \fi
 \expandafter\addtotoks@\expandafter{\expandafter{\xypostSPOKES@}}%
 \ifx\xypreSIDES@\relax
 \addtotoks@{{;}}%
 \DN@##1\next@{\def\tmp@{**\dir##1}}%
 \expandafter\next@\expandafter{\xypolySIDES@}\next@
 \expandafter\addtotoks@\expandafter{\expandafter{\tmp@}}%
 \else
 \expandafter\DN@\expandafter{\expandafter\ar\xypreSIDES@}%
 \expandafter\addtotoks@\expandafter{\expandafter{\next@}{}}%
 \fi
 \expandafter\addtotoks@\expandafter{\expandafter{\xypostSIDES@}}%
 \ifx\xypolyALIGN@\empty
 \ifnum\xypolyNUMSIDES@>12\addtotoks@{{0}}\fi
 \else
 \expandafter\addtotoks@\expandafter{\expandafter{\xypolyALIGN@}}%
 \fi
 \expandafter\DN@\expandafter{\expandafter\endgroup\the\toks@ }%
 \next@}
\xydef@\xytriangle@@#1#2#3#4#5#6#7#8{%
 \xy@@{\xypolynode@=\@ne}%
 \POS#1"#30"+(0,1)#2="#31"#4#5\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#30"#1"#30"+(-\cosPIon6, -.5)#2="#32"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#31"#6"#32"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(\cosPIon6,-.5)#2="#33"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#32"#6"#33"#7#8\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#33"#6"#31"#7#8\relax }
\xydef@\xysquare@@#1#2#3#4#5#6#7#8{%
 \xy@@{\xypolynode@=\@ne}%
 \POS#1"#30"+(\halfroottwo,\halfroottwo)#2="#31"#4#5\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#30"#1"#30"+(-\halfroottwo,\halfroottwo)#2="#32"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#31"#6"#32"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\halfroottwo,\halfroottwo)#2="#33"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#32"#6"#33"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(-\halfroottwo,\halfroottwo)#2="#34"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#33"#6"#34"#7#8\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#34"#6"#31"#7#8\relax }
\xydef@\xypentagon@@#1#2#3#4#5#6#7#8{%
 \xy@@{\xypolynode@=\@ne}%
 \POS#1"#30"+(\cosPIon{10},\sinPIon{10})#2="#31"#4#5\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#30"#1"#30"+(0,1)#2="#32"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#31"#6"#32"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(-\cosPIon{10},\sinPIon{10})#2="#33"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#32"#6"#33"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\sinPIon5,\cosPIon5)#2="#34"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#33"#6"#34"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(\sinPIon5,-\cosPIon5)#2="#35"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#34"#6"#35"#7#8\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#35"#6"#31"#7#8\relax }
\xydef@\xyhexagon@@#1#2#3#4#5#6#7#8{%
 \xy@@{\xypolynode@=\@ne}%
 \POS#1"#30"+(1,0)#2="#31"#4#5\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#30"#1"#30"+(.5,\halfrootthree)#2="#32"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#31"#6"#32"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(-.5,\halfrootthree)#2="#33"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#32"#6"#33"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(1,0)#2="#34"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#33"#6"#34"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(.5,\halfrootthree)#2="#35"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#34"#6"#35"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(-.5,\halfrootthree)#2="#36"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#35"#6"#36"#7#8\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#36"#6"#31"#7#8\relax }
\xydef@\xyheptagon@@#1#2#3#4#5#6#7#8{%
 \xy@@{\xypolynode@=\@ne}%
 \POS#1"#30"+(\sinTwoPIon7,\cosTwoPIon7)#2="#31"#4#5\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#30"#1"#30"+(0,1)#2="#32"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#31"#6"#32"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(-\sinTwoPIon7,\cosTwoPIon7)#2="#33"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#32"#6"#33"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\sinThreePIon7,\cosThreePIon7)#2="#34"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#33"#6"#34"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\sinPIon7,\cosPIon7)#2="#35"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#34"#6"#35"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(\sinPIon7,-\cosPIon7)#2="#36"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#35"#6"#36"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(\sinThreePIon7,-\cosThreePIon7)#2="#37"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#36"#6"#37"#7#8\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#37"#6"#31"#7#8\relax }
\xydef@\xyoctagon@@#1#2#3#4#5#6#7#8{%
 \xy@@{\xypolynode@=\@ne}%
 \POS#1"#30"+(\cosPIon8,\sinPIon8)#2="#31"#4#5\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#30"#1"#30"+(\sinPIon8,\cosPIon8)#2="#32"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#31"#6"#32"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\sinPIon8,-\cosPIon8)#2="#33"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#32"#6"#33"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\cosPIon8,-\sinPIon8)#2="#34"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#33"#6"#34"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\cosPIon8,\sinPIon8)#2="#35"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#34"#6"#35"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\sinPIon8,\cosPIon8)#2="#36"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#35"#6"#36"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(\sinPIon8,-\cosPIon8)#2="#37"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#36"#6"#37"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(\cosPIon8,-\sinPIon8)#2="#38"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#37"#6"#38"#7#8\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#38"#6"#31"#7#8\relax }
\xydef@\xynonagon@@#1#2#3#4#5#6#7#8{%
 \xy@@{\xypolynode@=\@ne}%
 \POS#1"#30"+(\sinFourPIon9,\cosFourPIon9)#2="#31"#4#5\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#30"#1"#30"+(\sinTwoPIon9,\cosTwoPIon9)#2="#32"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#31"#6"#32"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(0,1)#2="#33"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#32"#6"#33"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(-\sinTwoPIon9,\cosTwoPIon9)#2="#34"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#33"#6"#34"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(-\sinFourPIon9,\cosFourPIon9)#2="#35"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#34"#6"#35"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\cosPIon6,\sinPIon6)#2="#36"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#35"#6"#36"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\sinPIon9,\cosPIon9)#2="#37"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#36"#6"#37"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(\sinPIon9,-\cosPIon9)#2="#38"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#37"#6"#38"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(\cosPIon6,-\sinPIon6)#2="#39"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#38"#6"#39"#7#8\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#39"#6"#31"#7#8\relax }
\xydef@\xydecagon@@#1#2#3#4#5#6#7#8{%
 \xy@@{\xypolynode@=\@ne}%
 \POS#1"#30"+(1,0)#2="#31"#4#5\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#30"#1"#30"+(\cosPIon5,\sinPIon5)#2="#32"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#31"#6"#32"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(\sinPIon{10},\cosPIon{10})#2="#33"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#32"#6"#33"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\sinPIon{10},-\cosPIon{10})#2="#34"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#33"#6"#34"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\cosPIon5,-\sinPIon5)#2="#35"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#34"#6"#35"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(1,0)#2="#36"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#35"#6"#36"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\cosPIon5,\sinPIon5)#2="#37"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#36"#6"#37"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\sinPIon{10},\cosPIon{10})#2="#38"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#37"#6"#38"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(\sinPIon{10},-\cosPIon{10})#2="#39"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#38"#6"#39"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(\cosPIon5,-\sinPIon5)#2="#310"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#39"#6"#310"#7#8\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#310"#6"#31"#7#8\relax }
\xydef@\xyundecagon@@#1#2#3#4#5#6#7#8{%
 \xy@@{\xypolynode@=\@ne}%
 \POS#1"#30"+(\sinFourPIon{11},\cosFourPIon{11})#2="#31"#4#5\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#30"#1"#30"+(\sinTwoPIon{11},\cosTwoPIon{11})#2="#32"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#31"#6"#32"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(0,1)#2="#33"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#32"#6"#33"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(-\sinTwoPIon{11},\cosTwoPIon{11})#2="#34"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#33"#6"#34"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(-\sinFourPIon{11},\cosFourPIon{11})#2="#35"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#34"#6"#35"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\sinFivePIon{11},\cosFivePIon{11})#2="#36"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#35"#6"#36"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\sinThreePIon{11},\cosThreePIon{11})#2="#37"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#36"#6"#37"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\sinPIon{11},\cosPIon{11})#2="#38"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#37"#6"#38"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(\sinPIon{11},-\cosPIon{11})#2="#39"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#38"#6"#39"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(\sinThreePIon{11},-\cosThreePIon{11})#2="#310"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#39"#6"#310"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(\sinFivePIon{11},-\cosFivePIon{11})#2="#311"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#310"#6"#311"#7#8\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#311"#6"#31"#7#8\relax }
\xydef@\xydodecagon@@#1#2#3#4#5#6#7#8{%
 \xy@@{\xypolynode@=\@ne}%
 \POS#1"#30"+(\cosPIon{12},\sinPIon{12})#2="#31"#4#5\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#30"#1"#30"+(\halfroottwo,\halfroottwo)#2="#32"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#31"#6"#32"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(\sinPIon{12},\cosPIon{12})#2="#33"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#32"#6"#33"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\sinPIon{12},-\cosPIon{12})#2="#34"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#33"#6"#34"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\halfroottwo,-\halfroottwo)#2="#35"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#34"#6"#35"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\cosPIon{12},-\sinPIon{12})#2="#36"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#35"#6"#36"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\cosPIon{12},\sinPIon{12})#2="#37"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#36"#6"#37"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\halfroottwo,\halfroottwo)#2="#38"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#37"#6"#38"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\sinPIon{12},\cosPIon{12})#2="#39"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#38"#6"#39"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(\sinPIon{12},-\cosPIon{12})#2="#310"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#39"#6"#310"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(\halfroottwo,-\halfroottwo)#2="#311"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#310"#6"#311"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(\cosPIon{12},-\sinPIon{12})#2="#312"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#311"#6"#312"#7#8\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#312"#6"#31"#7#8\relax }
\xydef@\xylargePolygon@#1#2{%
 \dimen@=#1\p@
 \xyPolygon@@@\xypolygon@@}
\xydef@\xypolyrepeat@{\fi}
\xydef@\xypolybody@{}
\xydef@\xypolyiterate@{\xypolybody@\expandafter\xypolyiterate@\else\fi}
\xydef@\xypolyloop@#1\xypolyrepeat@{\def\xypolybody@{#1}\xypolyiterate@}
\xydef@\xypolygon@@#1#2#3#4#5#6#7#8#9{\save
 \vfromcartesianangle@{#9}\edef\next@{\the\X@c,\the\Y@c\addGT@\empty}%
 \xy@@{\xypolynode@=\@ne}%
 \toks@={\POS#1"#30"+}%
 \expandafter\expandafter\expandafter\addtotoks@\expandafter
 \expandafter\expandafter{\addLT@\empty}%
 \expandafter\addtotoks@\expandafter{\next@#2="#31"#4#5\relax}%
 \xy@@\dontleave@ \the\toks@
 \xypolyloop@
 \dimen@=360\p@ \count@@=\xypolyNUMSIDES@\relax \advance\dimen@ .5\count@@
 \divide\dimen@ \xypolyNUMSIDES@ \relax 
 \multiply\dimen@\xypolynode@ \relax \advance\dimen@ #9\p@ 
 \edef\tmp@{%
 \noexpand\vfromcartesianangle@{\expandafter\removePT@\the\dimen@}}%
 \tmp@ \edef\next@{\the\X@c,\the\Y@c\addGT@\empty}%
 \xy@@{\advance\xypolynode@\@ne}\count@=\xypolynode@
 \toks@={\POS"#30"#1"#30"+}\edef\nextii@{\the\count@}%
 \expandafter\expandafter\expandafter\addtotoks@\expandafter
 \expandafter\expandafter{\addLT@\space}%
 \expandafter\addtotoks@\expandafter{\next@#2="#3}%
 \expandafter\addtotoks@\expandafter{\nextii@"#4#5\relax}%
 \the\toks@ 
 \count@=\xypolynode@ \xy@@{\advance\xypolynode@\m@ne}%
 \toks@={\POS"#3}\expandafter\addtotoks@\expandafter{\the\xypolynode@"#6"#3}%
 \expandafter\addtotoks@\expandafter{\the\count@"#7#8\relax}%
 \the\toks@
 \xy@@{\advance\xypolynode@\@ne}\count@=\xypolyNUMSIDES@ \relax
 \ifnum\xypolynode@<\count@ \relax \xypolyrepeat@
 \toks@={\POS"#3}%
 \expandafter\addtotoks@\expandafter{\xypolyNUMSIDES@"#6"#31"#7#8\relax}%
 \the\toks@ \restore }
\xyendinput


==> xyps-c.tex <==
%% xyps-c.tex from $Id: xyps-c.doc,v 3.7 1999/02/16 15:12:50 krisrose Exp $
%%
%% Xy-pic ``Colour extension'' PostScript backend support.
%% Copyright (c) 1993-1996 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1996 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\expandafter\ifx\csname xyps-cloaded\endcsname\empty
 \message{not reloaded}\endinput \fi
\expandafter\let\csname xyps-cloaded\endcsname=\empty \xycatcodes
\expandafter\ifx \csname xyps-sloaded\endcsname\empty\else
 \xyinputorelse@{xyps-s}{\xyerror@{Could not load xyps-s}{}}%
 \xycatcodes\fi
\xydef@\UsePScolor{\installPScolor@}
\xydef@\NoPScolor{\UnloadColor@}
\xydef@\installPScolor@{\installPSstyle@
 \let\xymath@=\xyPSmath@ \let\xynomath@=\xyPSnomath@
 \let\checkxyPScolor@=\checkxyPScolor@@
 \let\xycolor@@=\xyPScolor@@
 \xystandardcolors@ 
 \xyuncatcodes }
\xydef@\xyPSmath@{\hbox\bgroup\dimen@=.55ex \checkxyPScolor@ \xyinside@}
\xydef@\xyPSnomath@{\hbox\bgroup\dimen@=\z@ \checkxyPScolor@ \xyinside@}
\xydef@\checkxyPScolor@@{\xycolor@raw@@{}\let\checkxyPScolor@=\relax}
\xylet@\checkxyPScolor@=\relax
\xydef@\xyPSnewcolor@#1#2#3#4#5{%
 \expandafter\DN@\expandafter{\csname shape [#1]\endcsname}%
 \DNii@{\relax}\ifx\next@\nextii@\newxycolor{#1}{}\relax\fi
 \DNii@{#4}\ifx\nextii@\empty
 \expandafter\DNii@\expandafter{\csname xyPSshape@#1@\endcsname}%
 \expandafter\def\nextii@{\xyPScolor@{#2 #3}}\else
 \expandafter\DNii@\expandafter{\csname xyPSshape@#1@\endcsname}%
 \expandafter\def\nextii@{\xyPScolor@{#4}}\fi
 \ifx\nextii@\empty\expandafter\def\next@{\xyPSnotimplemented@@`#1'@@}%
 \else
 \edef\tmp@{\noexpand\let\expandafter\noexpand\next@
 \expandafter\noexpand\nextii@}\expandafter\tmp@\fi }
\xydef@\xyPScolor@{\ifPSspecials@\expandafter\xyPScolor@@
 \else\expandafter\eat@\fi}
\xydef@\xyPScolor@@#1{\bgroup \checkXyStyle@ 
 \def\preStyle@@{\expandafter\addtostyletoks@\expandafter{\xyPSpre@}}%
 \def\postStyle@@{\expandafter\addtostyletoks@\expandafter{\xyPSpost@}}%
 \let\modPSboxz@=\modXYstyle@ \xyPS@color@@{#1}%
 \toks@={\egroup\let\xy@style@=\relax \def\Drop@@}%
 \expandafter\addtotoks@\expandafter{\expandafter{\Drop@@}\def\Connect@@}%
 \expandafter\addtotoks@\expandafter{\expandafter{\Connect@@}}%
 \the\toks@ }
\xydef@\xyPS@color@@#1{\xyPSsplitPS@{{#1}cc}{}}
\xydef@\xycolor@raw@@#1{\PSraw@@{xyc}}
\endinput


==> xyps-col.tex <==
%% xyps-col.tex from $Id: xyps-col.doc,v 3.7 1999/02/16 15:12:50 krisrose Exp $
%%
%% Xy-pic ``Crayola colour names'' PostScript colour support.
%% Copyright (c) 1995-1996 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1996 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyrequire{color}\xycatcodes
\newxycolor@{GreenYellow}{0.15 0 0.69 0}{cmyk}{}{}%
\newxycolor@{Yellow}{0 0 1. 0}{cmyk}{}{}%
\newxycolor@{Goldenrod}{0 0.10 0.84 0}{cmyk}{}{}%
\newxycolor@{Dandelion}{0 0.29 0.84 0}{cmyk}{}{}%
\newxycolor@{Apricot}{0 0.32 0.52 0}{cmyk}{}{}%
\newxycolor@{Peach}{0 0.50 0.70 0}{cmyk}{}{}%
\newxycolor@{Melon}{0 0.46 0.50 0}{cmyk}{}{}%
\newxycolor@{YellowOrange}{0 0.42 1. 0}{cmyk}{}{}%
\newxycolor@{Orange}{0 0.61. 0.87 0}{cmyk}{}{}%
\newxycolor@{BurntOrange}{0 0.51 1. 0}{cmyk}{}{}%
\newxycolor@{Bittersweet}{0 0.75 1. 0.24}{cmyk}{}{}%
\newxycolor@{RedOrange}{0 0.77 0.87 0}{cmyk}{}{}%
\newxycolor@{Mahogany}{0 0.85 0.87 0.35}{cmyk}{}{}%
\newxycolor@{Maroon}{0 0.87 0.68 0.32}{cmyk}{}{}%
\newxycolor@{BrickRed}{0 0.89 0.94 0.28}{cmyk}{}{}%
\newxycolor@{Red}{0 1. 1. 0}{cmyk}{}{}%
\newxycolor@{OrangeRed}{0 1. 0.50 0}{cmyk}{}{}%
\newxycolor@{RubineRed}{0 1. 0.13 0}{cmyk}{}{}%
\newxycolor@{WildStrawberry}{0 0.96 0.39 0}{cmyk}{}{}%
\newxycolor@{Salmon}{0 0.53 0.38 0}{cmyk}{}{}%
\newxycolor@{CarnationPink}{0 0.63 0 0}{cmyk}{}{}%
\newxycolor@{Magenta}{0 1. 0 0}{cmyk}{}{}%
\newxycolor@{VioletRed}{0 0.81 0 0}{cmyk}{}{}%
\newxycolor@{Rhodamine}{0 0.82 0 0}{cmyk}{}{}%
\newxycolor@{Mulberry}{0.34 0.90 0 0.02}{cmyk}{}{}%
\newxycolor@{RedViolet}{0.07 0.90 0 0.34}{cmyk}{}{}%
\newxycolor@{Fuchsia}{0.47 0.91 0 0.08}{cmyk}{}{}%
\newxycolor@{Lavender}{0 0.48 0 0}{cmyk}{}{}%
\newxycolor@{Thistle}{0.12 0.59 0 0}{cmyk}{}{}%
\newxycolor@{Orchid}{0.32 0.64 0 0}{cmyk}{}{}%
\newxycolor@{DarkOrchid}{0.40 0.80 0.20 0}{cmyk}{}{}%
\newxycolor@{Purple}{0.45 0.86 0 0}{cmyk}{}{}%
\newxycolor@{Plum}{0.50 1. 0 0}{cmyk}{}{}%
\newxycolor@{Violet}{0.79 0.88 0 0}{cmyk}{}{}%
\newxycolor@{RoyalPurple}{0.75 0.90 0 0}{cmyk}{}{}%
\newxycolor@{BlueViolet}{0.86 0.91 0 0.04}{cmyk}{}{}%
\newxycolor@{Periwinkle}{0.57 0.55 0 0}{cmyk}{}{}%
\newxycolor@{CadetBlue}{0.62 0.57 0.23 0}{cmyk}{}{}%
\newxycolor@{CornflowerBlue}{0.65 0.13 0 0}{cmyk}{}{}%
\newxycolor@{MidnightBlue}{0.98 0.13 0 0.43}{cmyk}{}{}%
\newxycolor@{NavyBlue}{0.94 0.54 0 0}{cmyk}{}{}%
\newxycolor@{RoyalBlue}{1. 0.50 0 0}{cmyk}{}{}%
\newxycolor@{Blue}{1. 1. 0 0}{cmyk}{}{}%
\newxycolor@{Cerulean}{0.94 0.11 0 0}{cmyk}{}{}%
\newxycolor@{Cyan}{1. 0 0 0}{cmyk}{}{}%
\newxycolor@{ProcessBlue}{0.96 0 0 0}{cmyk}{}{}%
\newxycolor@{SkyBlue}{0.62 0 0.12 0}{cmyk}{}{}%
\newxycolor@{Turquoise}{0.85 0 0.20 0}{cmyk}{}{}%
\newxycolor@{TealBlue}{0.86 0 0.34 0.02}{cmyk}{}{}%
\newxycolor@{Aquamarine}{0.82 0 0.30 0}{cmyk}{}{}%
\newxycolor@{BlueGreen}{0.85 0 0.33 0}{cmyk}{}{}%
\newxycolor@{Emerald}{1. 0 0.50 0}{cmyk}{}{}%
\newxycolor@{JungleGreen}{0.99 0 0.52 0}{cmyk}{}{}%
\newxycolor@{SeaGreen}{0.69 0 0.50 0}{cmyk}{}{}%
\newxycolor@{Green}{1. 0 1. 0}{cmyk}{}{}%
\newxycolor@{ForestGreen}{0.91 0 0.88 0.12}{cmyk}{}{}%
\newxycolor@{PineGreen}{0.92 0 0.59 0.25}{cmyk}{}{}%
\newxycolor@{LimeGreen}{0.50 0 1. 0}{cmyk}{}{}%
\newxycolor@{YellowGreen}{0.44 0 0.74 0}{cmyk}{}{}%
\newxycolor@{SpringGreen}{0.26 0 0.76 0}{cmyk}{}{}%
\newxycolor@{OliveGreen}{0.64 0 0.95 0.40}{cmyk}{}{}%
\newxycolor@{RawSienna}{0 0.72 1. 0.45}{cmyk}{}{}%
\newxycolor@{Sepia}{0 0.83 1. 0.70}{cmyk}{}{}%
\newxycolor@{Brown}{0 0.81 1. 0.60}{cmyk}{}{}%
\newxycolor@{Tan}{0.14 0.42 0.56 0}{cmyk}{}{}%
\newxycolor@{Gray}{0 0 0 0.50}{cmyk}{}{}%
\newxycolor@{Black}{0 0 0 1.}{cmyk}{}{}%
\newxycolor@{White}{0 0 0 0}{cmyk}{}{}%
\endinput


==> xyps-f.tex <==
%% xyps-f.tex from $Id: xyps-f.doc,v 3.7 1999/02/16 15:12:50 krisrose Exp $
%%
%% Xy-pic ``Frame extension'' PostScript backend support.
%% Copyright (c) 1995-1997 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1997 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\expandafter\ifx\csname xyps-floaded\endcsname\empty
 \message{not reloaded}\endinput \fi
\expandafter\let\csname xyps-floaded\endcsname=\empty \xycatcodes
\xydef@\installPSframes@{%
 \let\framed@body@@=\xyPSframed@body@
 \let\circled@x@@=\xyPScircled@x@
 \let\ellipsed@x@@=\xyPSellipsed@x@
 \installPSfills@
 \xyuncatcodes}
\xydef@\UsePSframes{\installPSframes@}
\xydef@\NoPSframes{\UnloadFrames@}
\xydef@\xyPSframed@body@{\DN@{\framed@body@}%
 \ifx\framehfill\frm@solidh@@
 \DN@{\xyPSframed@oval@\xyPSoval@Special}%
 \else\ifdim\R@=\z@\else
 \ifx\framehfill\frm@dashh@@
 \DN@{\xyPSframed@oval@\xyPSdashoval@Special}%
 \else\ifx\framehfill\frm@doth@@
 \DN@{\xyPSframed@oval@\xyPSdotoval@Special}%
 \fi\fi
 \fi\fi \next@ }
\xydef@\xyPSframed@oval@#1{\vglue\U@c
 \hbox{\hglue\L@c\xypsoval@#1\hglue\R@c}\vglue\D@c}
\xydef@\xyPScircled@x@{\DN@{\xyPScircled@x@@\xyPScirc@Special}%
 \ifx\framehfill\frm@doth@@
 \DN@{\xyPScircled@x@@\xyPSdotcirc@Special}%
 \else\ifx\framehfill\frm@dashh@@
 \DN@{\xyPScircled@x@@\xyPSdashcirc@Special}%
 \fi\fi \next@ }
\xydef@\xyPScircled@x@@#1{\vglue2\R@
 \hbox{\hglue2\R@\xypscircle@#1\hglue2\R@}%
 \vglue2\R@}
\xydef@\xyPSellipsed@x@#1#2{%
 \DN@{\xyPSellipsed@x@@\xyPScirc@Special}%
 \ifx\framehfill\frm@doth@@
 \DN@{\xyPSellipsed@x@@\xyPSdotcirc@Special}%
 \else\ifx\framehfill\frm@dashh@@
 \DN@{\xyPSellipsed@x@@\xyPSdashcirc@Special}%
 \fi\fi \next@{#1}{#2}}
\xydef@\xyPSellipsed@x@@#1#2#3{\vglue #3\vglue #3\relax
 \hbox{\L@c = #2\relax \R@c=\L@c \D@c = #3\relax \U@c=\D@c 
 \hglue#2\hglue#2\relax\xypsellipse@#1\hglue#2\hglue#2\relax}%
 \vglue #3\vglue #3\relax}
\xydef@\xyPSdashhfill@{{\SemiDirectionChar=95 \Direction=3072 \xyPSdash@}}
\xydef@\xyPSdashvfill@{{\SemiDirection=31 \Direction=1023 \xyPSdash@}}
\xydef@\xypsoval@#1{%
 \dimen@=\L@c \advance\dimen@\R@c
 \dimen@ii=\U@c \advance\dimen@ii\D@c 
 \ifdim\dimen@ii<\dimen@ \relax \dimen@=\dimen@ii\fi \divide\dimen@\tw@
 \ifdim\R@>\dimen@ \relax \R@=\dimen@ \fi
 \D@c=-\D@c \L@c=-\L@c 
 \edef\tmp@{\expandafter\removePT@\the\R@
 \space\expandafter\removePT@\the\R@c 
 \space\expandafter\removePT@\the\D@c 
 \space\expandafter\removePT@\the\L@c 
 \space\expandafter\removePT@\the\U@c }%
 \expandafter#1\expandafter{\tmp@}}
\xydef@\xypscircle@#1{\dimen@=\R@
 \edef\tmp@{\expandafter\removePT@\the\dimen@}%
 \expandafter#1\expandafter{\tmp@}}
\xydef@\xypsellipse@#1{\edef\tmp@{%
 \expandafter\removePT@\the\U@c \space
 \expandafter\removePT@\the\D@c \space
 \expandafter\removePT@\the\L@c \space
 \expandafter\removePT@\the\R@c }%
 \expandafter#1\expandafter{\tmp@}}
\xydef@\xyPSoval@Special#1{\PSmacro@{#1 ov}}
\xydef@\xyPScirc@Special#1{\PSmacro@{#1 ox}}
\xydef@\xyPSdotcirc@Special#1{\PSmacro@{#1 ot}}
\xydef@\xyPSdashcirc@Special#1{\PSmacro@{#1 od}}
\xydef@\xyPSdotoval@Special#1{\PSmacro@{#1 vt}}
\xydef@\xyPSdashoval@Special#1{\PSmacro@{#1 vd}}
\xydef@\xyPSfilledRegion#1#2{\setboxz@h{\lower\D@c\vbox{%
 \vglue\U@c\hbox{#1#2\empty\hglue\L@c\hglue\R@c}\vglue\D@c}}%
 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \boxz@}
\xydef@\filledRectangle@PS{%
 \xyPSfilledRegion{\xypsoval@\xyPSfilloval@Special}}
\xydef@\filledCircle@PS#1{{\R@c=\R@ \L@c=\R@ \U@c=\R@ \D@c=\R@
 \xyPSfilledRegion{\xypscircle@\xyPSfillcirc@Special}#1}}
\xydef@\filledEllipse@PS{%
 \xyPSfilledRegion{\xypsellipse@\xyPSfillellipse@Special}}
\xydef@\filledOval@PS{%
 \xyPSfilledRegion{\xypsoval@\xyPSfilloval@Special}}
\xydef@\frame@emph@PS#1{\filled@{#1}\relax}
\xydef@\installPSfills@{%
 \let\frame@emph@@=\frame@emph@PS
 \let\filledRectangle@@=\filledRectangle@PS
 \let\filledOval@@=\filledOval@PS
 \let\filledCircle@@=\filledCircle@PS
 \let\filledEllipse@@=\filledEllipse@PS
}
\xydef@\xyPSfilloval@Special#1#2{%
 \ifx#2\relax\PSmacro@{#1 sfo}%
 \else\PSmacro@{#1 fo}\fi}
\xydef@\xyPSfillcirc@Special#1#2{%
 \ifx#2\relax\PSmacro@{#1 sfc}%
 \else\PSmacro@{#1 fc}\fi}
\xydef@\xyPSfillellipse@Special#1#2{%
 \ifx#2\relax\PSmacro@{#1 sfe}%
 \else\PSmacro@{#1 fe}\fi}
\endinput


==> xyps-l.tex <==
%% xyps-l.tex from $Id: xyps-l.doc,v 3.7 1999/02/16 15:12:50 krisrose Exp $
%%
%% Xy-pic ``Line extension'' PostScript backend support.
%% Copyright (c) 1993-1997 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1997 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\expandafter\ifx\csname xyps-lloaded\endcsname\empty
 \message{not reloaded}\endinput \fi
\expandafter\let\csname xyps-lloaded\endcsname=\empty \xycatcodes
\expandafter\ifx\csname xyps-sloaded\endcsname\empty\else
 \xyinputorelse@{xyps-s}{\xyerror@{Could not load xyps-s}{}}%
 \xycatcodes\fi
\xydef@\installPSline@{\installPSstyle@
 \installPSlinestyles@ \installPSpolylines@ }
\xydef@\UsePSlines{\installPSline@}
\xydef@\NoPSlines{\UnloadLine@\relax}
\xydef@\xyPSlineSpecial@#1{\addtostyletoks@{ #1 lw}}
\xydef@\xyPScapSpecial@#1{\addtostyletoks@{ #1 lc}}
\xydef@\xyPSjoinSpecial@#1{\addtostyletoks@{ #1 lj}}
\xydef@\xyPSmiterSpecial@#1{\addtostyletoks@{ #1 ml}}
\xydef@\installPSlinestyles@{%
 \let\xylinewidth@@=\xylinewidth@
 \let\transxyline@@=\transxyline@
 \let\xylineSpecial@@=\xyPSlineSpecial@
 \let\resetxyline@@=\resetxyline@i
 \let\xy@linecap@@=\xy@linecap@
 \let\xycapSpecial@@=\xyPScapSpecial@
 \let\resetxylinecap@@=\resetxylinecap@i
 \let\xy@linejoin@@=\xy@linejoin@
 \let\xyjoinSpecial@@=\xyPSjoinSpecial@
 \let\resetxylinejoin@@=\resetxylinejoin@i
 \let\xy@linemiter@@=\xy@linemiter@
 \let\xymiterSpecial@@=\xyPSmiterSpecial@
 \let\resetxylinemiter@@=\resetxylinemiter@i
}
\xydef@\xypolylinePS@Special#1{\PSmacro@{#1 pl}}
\xydef@\xypolydotPS@Special#1{\PSmacro@{#1 pt}}
\xydef@\xypolydashPS@Special#1{\PSmacro@{#1 pd}}
\xydef@\xypolyfillPS@Special#1{\PSmacro@{#1 pf}}
\xydef@\xypolyeofillPS@Special#1{\PSmacro@{#1 pe}}
\xydef@\installPSpolylines@{%
 \let\xypolyline@Special=\xypolylinePS@Special
 \let\xypolydot@Special=\xypolydotPS@Special
 \let\xypolydash@Special=\xypolydashPS@Special
 \let\xypolyfill@Special=\xypolyfillPS@Special
 \let\xypolyeofill@Special=\xypolyeofillPS@Special
 \let\xy@polystyle@@=\xy@polystyle@ }
\endinput


==> xyps-pro.tex <==
%% xyps-pro.tex from $Id: xyps-pro.doc,v 3.7 1999/02/16 15:12:50 krisrose Exp $
%%
%% Xy-pic ``PostScript Prolog'' for PostScript support.
%% Copyright (c) 1993-1996 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1996 Kristoffer H. Rose <krisrose@ens-lyon.fr>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
\begingroup \xycatcodes%
 \count@=\xydashl@\relax \count@@=\xydashw@\relax%
 \let\firstPS@@=\relax%
 \xyPSobeylines@@%
\PSspecialdict@@{%
/XYdict where not{250 dict /XYdict exch def 
 /xy{mark exch XYdict begin countdictstack /xylevel exch def
 xyopen xycolor mark xypatt xypattern stopped xyclose end
 cleartomark}def /xyg{gsave xy}def 
 /xyf{currentfont exch xy grestore setfont}def
 /xycc{{xychgcol}xy}def /xyc{XYdict begin xycolstore end}def
 /xyx{/xyYpos exch def /xyXpos exch def}def 
 /xyp{currentpoint xyx}def
 /xyd{setupDirection XYdirection 2 mul}def 
 /xyct{currentpoint xyt 2 copy 6 2 roll}def
 /xyt{xyXpos xyYpos 2 copy translate}def /xyr{neg rotate xynt}def
 /xyrs{neg rotate 3 -1 roll sub neg 3 1 roll sub exch moveto xynt}def
 /xynt{neg exch neg exch translate}def /xys{scale xynt}def
 /xyss{scale 3 -1 roll sub neg 3 1 roll sub exch moveto xynt}def
 /xyi{0 0 transform grestore gsave itransform}def
 }if}%
\tmp@false\def\do#1{\DN@{#1}\ifx\next@\nextii@\tmp@true\fi}%
\DNii@{17oztex}\xydriversselected@@\iftmp@\PSspecialdict@@{%
 /@boxy{prespecialVM restore grestore}def
 /@eoxy{gsave /prespecialVM save def}def
 }%
\else \DNii@{oztex}\xydriversselected@@\iftmp@\PSspecialdict@@{%
 /@oxy{prespecialVM restore grestore}def
 /@oxy{gsave /prespecialVM save def}def
 }\fi\fi% 
\PSdict@@{/XYdict where pop begin XYdict begin}%
\PSdict@@{%
 /xyopen{currentdict /XYddict known{XYddict null eq{}
 {XYddict begin xyopen}ifelse}if}def
 /xyclose{countdictstack -1 xylevel 1 add{pop end}for}def
 /xychgcol{/xycolor exch def}def /xysetcol{xypush xychgcol}def 
}%
\PSdict@@{%
 /xypush{16 dict /XYddict exch def XYddict begin}def
 /undef where
 {pop /xypop{countdictstack xylevel eq{}{end}ifelse
 currentdict /XYddict undef}def}
 {/xypop{countdictstack xylevel eq{}{end}ifelse
 /XYddict null def}def}ifelse
 /pu /xypush load def /pp /xypop load def}%
\PSdict@@{%
 /xypspt{72 72.27 div dup scale}bind def /pscorrect{.85 mul}bind def 
 /gstartxy{gsave xypspt xywidth xycap xyjoin xymiter newpath 0 0 moveto}def 
 /xypath{gstartxy rmoveto counttomark 2 idiv -1 1{pop lineto}for}def 
 /xystroke{stroke grestore}bind def 
 /xyfill{closepath fill grestore}bind def
 /xystfil{closepath gsave fill grestore 0 setgray 
 0 setlinewidth xystroke}bind def
 /xyeofill{closepath eofill grestore}bind def
}%
\PSdict@@{%
 /xypolyline{xypath xystroke}def /xypolyfill{xypath xyfill}def
 /xydotsep{/@ currentlinewidth 2 mul def}def
 /xypolydot{xypath xydotsep [xydt @] 0 setdash xystroke}def
 /xypolydash{xypath xydotsep [@ @] 0 setdash xystroke}def
 /xypolyeofill{xypath xyeofill}def /pe /xypolyeofill load def 
 /pl /xypolyline load def /pf /xypolyfill load def 
 /pt /xypolydot load def /pd /xypolydash load def }%
\PSdict@@{%
 /arc4pop{arcto 4{pop}repeat}bind def 
 /xyoval{gstartxy oval closepath xystroke}def
 /xycircle{gstartxy circle xystroke}def
 /circle{dup 0 moveto 0 0 3 -1 roll 0 360 arc}def
 /oval{newpath 2 copy exch 5 index add 2 div exch 3 copy 10 3 roll 
 moveto 1 index dup 5 1 roll 3 index 7 index arc4pop
 dup dup 4 1 roll 4 index exch 6 index arc4pop
 1 index dup 8 1 roll 4 index 4 index arc4pop
 arc4pop closepath}def
 /xyellipse{gstartxy counttomark 1 gt{squarify pop pop 1}if
 circle xystroke}def
 /ov /xyoval load def /ox /xyellipse load def }%
\PSdict@@{%
 /dotit{dup currentlinewidth 6 mul div round div
 /@ exch def [xydt @] 0 setdash}def
 /elldash{dup 4 -1 roll 10 exch div dashit}def
 /ovdash{dup 10 dashit}def
 /dashit{div round 2 mul div /@ exch def [@ @] 0 setdash}def
 /dotcirc{gstartxy cirlen dotit circle xystroke}def
 /dashcirc{gstartxy cirlen dashit circle xystroke}def
 /dotoval{gstartxy 5 copy ovlen dotit oval xystroke}def
 /dashoval{gstartxy 5 copy ovlen ovdash oval xystroke}def
 /cirlen{dup 6.283185 mul}bind def
 /ovlen{3 -1 roll sub 3 1 roll sub add exch 1.716815 mul sub}def
 /dotellipse{gstartxy counttomark 1 gt{squarify pop pop 1}if
 cirlen dotit circle closepath xystroke}def
 /dashellipse{gstartxy counttomark 1 gt{squarify add 2 div 1}
 {1 exch 1 exch}ifelse cirlen elldash circle xystroke}def
 /ot /dotellipse load def /od /dashellipse load def 
 /vt /dotoval load def /vd /dashoval load def }%
\PSdict@@{%
 /filloval{gstartxy oval xyfill}def
 /stfiloval{gstartxy oval xystfil}def
 /fillcircle{gstartxy circle xyfill}def 
 /stfilcircle{gstartxy circle xystfil}def 
 /fillellipse{gstartxy squarify pop pop 1 circle xyfill}def
 /stfilellipse{gstartxy squarify pop pop 1 circle xystfil}def
 /squarify{4 copy sub 2 div 3 1 roll sub 2 div translate
 add 2 div 3 1 roll add 2 div 2 copy scale
 2 copy add 2 div currentlinewidth exch div setlinewidth
 newpath}def
 /fe /fillellipse load def /sfe /stfilellipse load def 
 /fo /filloval load def /sfo /stfiloval load def
 /fc /fillcircle load def /sfc /stfilcircle load def }%
\PSdict@@{%
 /xywidth{.4 pscorrect setlinewidth}bind def
 /xydash{[] 0 setdash}bind def /xycap{1 setlinecap}bind def
 /xyjoin{1 setlinejoin}bind def /xymiter{10 setmiterlimit}bind def
}%
\PSdict@@{%
 /cc{dup exec xychgcol}def
 /lw{dup setlinewidth /@l exch def
 /xywidth{@l setlinewidth}bind def}def
 /lc{dup setlinecap /@c exch def
 /xycap{@c setlinecap}bind def}def
 /lj{dup setlinejoin /@j exch def
 /xyjoin{@j setlinejoin}bind def}def
 /ml{dup setmitrelimit /@m exch def
 /xymiter{@m setmitrelimit}bind def}def
}%
\PSdict@@{%
 /setupDirection{dup -2048 lt{3072 add neg 1024 exch}
 {dup 0 lt{1024 add neg -1024}{dup 2048 lt{1024 sub -1024 exch}
 {3072 sub 1024}ifelse}ifelse}ifelse atan 
 dup 180 gt{360 sub}if dup /XYdirection exch def rotate}def
 }%
\PSdict@@{%
 userdict begin 
 /gray{setgray}bind def /gray@{setgray}bind def
 /rgb{setrgbcolor}bind def /rgb@{setrgbcolor}bind def
 /hsb{sethsbcolor}bind def /hsb@{sethsbcolor}bind def
 /setcmykcolor where{pop}{/setcmykcolor{dup 3 1 roll dup 5 1 roll
 exch sub 1 add 5 1 roll exch sub 1 add 4 1 roll 
 exch sub 1 add 3 1 roll setrgbcolor}bind def}ifelse
 /cmyk{setcmykcolor}bind def /cmyk@{setcmykcolor}bind def
 /sethalftone where{/sethalftone load /tone exch def}if
 /xycolarray 3 array def /xycolstore{currentrgbcolor 2 -1 0
 {exch xycolarray 3 1 roll put}for}def xycolstore
 /xycolor{0 1 2{xycolarray exch get}for setrgbcolor}def
 /xypatt{}def /xypattern{cleartomark}bind def
 end}%
\PSdict@@{end end}%
\endgroup%
\endinput


==> xyps-ps.tex <==
%% xyps-ps.tex from $Id: xyps-ps.doc,v 3.7 1999/02/16 15:12:50 krisrose Exp $
%%
%% Xy-pic ``PS-PS'' PostScript support.
%% Copyright (c) 1993-1997 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1997 Kristoffer H. Rose <krisrose@ens-lyon.fr>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\expandafter\ifx\csname xyps-psloaded\endcsname\empty
 \message{not reloaded}\endinput \fi
\expandafter\let\csname xyps-psloaded\endcsname=\empty \xycatcodes
\xylet@\PSmacro@@=\eat@
\xylet@\PSdict@@=\eat@
\xylet@\PSspecial@@=\eat@
\xylet@\PSread@@=\eat@
\xylet@\PSinclude@@=\eat@
\xylet@\PSraw@@=\eat@
\xylet@\xyPSobeylines@@=\relax
\xylet@\PSspecialdict@@=\eat@
\xydef@\UnloadPSps@{%
 \let\PSmacro@@=\eat@
 \let\PSdict@@=\eat@
 \let\PSspecial@@=\eat@
 \let\PSread@@=\eat@
 \let\PSinclude@@=\eat@
 \let\PSraw@@=\eat@
 \let\xyPSobeylines@@=\relax
 \let\PSspecialdict@@=\eat@
}
\xydef@\UnloadPS@{\UnloadPSps@
 \expandafter\ifx\csname xypsloaded\endcsname\unknown\PSspecials@false
 \else\expandafter\NoPSspecials\fi}
\xylet@\UnloadPS@@=\UnloadPS@
\ifx\undefined\dvitype@\xydef@\dvitype@{null}\fi
\xylet@\xyrealshipout@=\shipout
\xydef@\xyPSshipout@{\setbox9=\copy\voidb@x
 \afterassignment\xyPSshipout@i\setbox9=}
\xydef@\xyPSshipout@i{\ifvoid9 \expandafter\aftergroup\fi\xyPSshipout@ii}
\xydef@\xyPSshipout@ii{\xyrealshipout@\vbox{\XYpredict@@\box9}}
\xydef@\@PSshipout{\global\let\shipout=\xyPSshipout@ }
\xydef@\xyPSshipout@PSii{%
 \ifUsePSdict@@\let\XYshipdict@=\includeXYPSdict@@
 \else\def\XYshipdict@{\XYpredict@@\XYdict@@}\fi
 \xyrealshipout@\vbox{\XYshipdict@\box9}}
\xydef@\firstPS@{%
 \global\let\firstPS@@=\relax \global\let\firstPS@=\relax}
\xylet@\firstPS@@=\firstPS@
\ifx\undefined\dumpPSdict@@ \xylet@\dumpPSdict@@=\relax \fi
\xydef@\installxyps@{%
 \xyinputorelse@{xyps-ps}{\xydrivernoload@{ps-ps}}\xycatcodes
 \installxyps@@ \installxyps@x }
\xylet@\installxyps@@=\relax
\xylet@\setupxyPS@@=\relax
\xywithoption{ps}{\let\setupxyPS@@=\setupxyPS@}
\xydef@\installxyps@x{\dumpPSdict@@ 
 \ifx\xyrealshipout@\undefined \let\xyrealshipout@=\shipout\fi
 \ifx \shipout \xyrealshipout@ 
 \ifUsePSdict@@ \DN@{\includePSmessage@\includeXYPSdict@\message{>}}%
 \else \DN@{\XYdict@\endXYdict@}\fi
 \else \DN@{\let\xyPSshipout@ii=\xyPSshipout@PSii \@PSshipout}\fi
 \let\firstPS@=\relax \next@
 \let\XYpredict@=\relax
 \setupxyPS@@ }
\let\realinstallxyps@x=\installxyps@x
\ifx\undefined\AfterBeginDocument
 \def\installxyps@x{\xysetup@@{\realinstallxyps@x}}%
\else
 \def\installxyps@x{\AfterBeginDocument{\realinstallxyps@x}}%
\fi
\xydef@\xydefaultdriver@{dvips}
\xydef@\xyPSdriver#1{\def\xydefaultdriver@{#1}}
\xydef@\installxyps@orig{\DN@{}%
 \ifx\xydriversselected@@\empty
 \DN@{\expandafter\defaultinstallps@\expandafter{\xydefaultdriver@}}%
 \else \def\do##1{%
 \expandafter\ifx\csname##1@xy@ps\endcsname\relax
 \DN@{\defaultinstallps@{##1}}}%
 \xydriversselected@@ 
 \else \DN@##1{}\fi\fi \next@ }
\xydef@\defaultinstallps@#1#2{%
 \xywarning@{no driver specified, using #1 }%
 \xyrequire{#1}\csname #1@xy@ps\endcsname{}}
\xydef@\null@xy@ps{\installxyps@}
\xydefcsname@{shape [!...]}#1{%
 \expandafter\ifx\csname xyps-sloaded\endcsname\empty \DN@{\xyPSescapestyle@{#1}@@}%
 \else\ifxyPSshapes@\DN@{\xyPSshapechar@{#1}@@}%
 \else \DN@{\xyPScharwarning@}\fi\fi \next@ }
\xydefcsname@{shape [psxy]}{\ifxyPSshapes@\DN@{\xyPSpsxy@}%
 \else \DN@{\xyPScharwarning@}\fi \next@ }
\xydef@\xyPSpsxy@{%
 \setboxz@h{\dimen@=\L@p \advance\dimen@-\R@p 
 \dimen@ii=-\U@p \raise\dimen@ii\hbox to\z@{%
 \kern\dimen@\xyPScurrpt@\kern-\dimen@}\boxz@}}%
\xydef@\xyPScurrpt@{\ifxyPSshapes@\expandafter\xyPScurrpt@@\fi}
\xydef@\xyPScurrpt@@@{\PSspecial@@{xyi}\PSraw@@{userdict begin xyx end}}
\ifx\undefined\xyPScurrpt@@ \xylet@\xyPScurrpt@@=\xyPScurrpt@@@ \fi
\xywarnifdefined\xyPSshapechar@
\xywarnifdefined\xyPSsplitshape@
{\xyuncatcodes \catcode`@=11
 \gdef\xyPSshapechar@#1@@{\xyPSsplitshape@#1<><>@@}%
 \gdef\xyPSsplitshape@#1<>#2<>#3@@{\xyPSsplitPS@{#1}{#2}}}
\xydef@\xyPSrawA@#1{\expandafter\xyPSrawAA@ #1{}}%
\xydef@\xyPSrawAA@#1#2{\PSraw@@{{pu #1}xyg #2}%
 \PSmessage{{pu #1}xyg #2}}%
\xydef@\xyPSrawZ@#1{\PSraw@@{{#1 pp}xyf}\PSmessage{{#1 pp}xyf}}%
\xydef@\modPSboxz@{%
 \expandafter\DN@\expandafter{\xyPSpre@{}}\ifx\next@\empty\else
 \setboxz@h{\expandafter\xyPSrawA@\expandafter{\xyPSpre@{}}\boxz@
 \expandafter\xyPSrawZ@\expandafter{\xyPSpost@}}\DN@{}\fi}%
\xydef@\modPSdrop@{%
 \expandafter\DNii@\expandafter{%
 \expandafter\xyPSrawA@\expandafter{\xyPSpre@{}}}%
 \DN@##1{\expandafter\def\expandafter\tmp@\expandafter{\nextii@ ##1}}%
 \expandafter\next@\expandafter{\Drop@@}%
 \expandafter\DNii@\expandafter{%
 \expandafter\xyPSrawZ@\expandafter{\xyPSpost@}}%
 \DN@##1{\expandafter\def\expandafter\Drop@@\expandafter{\tmp@ ##1}}%
 \expandafter\next@\expandafter{\nextii@}}%
\xydef@\modPSconnect@{%
 \expandafter\DNii@\expandafter{%
 \expandafter\xyPSrawA@\expandafter{\xyPSpre@{}}}%
 \DN@##1{\expandafter\def\expandafter\tmp@\expandafter{\nextii@ ##1}}%
 \expandafter\next@\expandafter{\Connect@@}%
 \expandafter\DNii@\expandafter{%
 \expandafter\xyPSrawZ@\expandafter{\xyPSpost@}}%
 \DN@##1{\expandafter\def\expandafter\Connect@@\expandafter{\tmp@ ##1}}%
 \expandafter\next@\expandafter{\nextii@}}%
\xydef@\xyPSpre@{{}{}}
\xydef@\xyPSpost@{}
\xydef@\PSmessage@#1{\W@{PS: #1, direction=\the\Direction}}
\xydef@\PSignore@#1{}%
\xydef@\showPSmessages{\let\PSmessage=\PSmessage@}
\xydef@\hidePSmessages{\let\PSmessage=\PSignore@}
\xylet@\PStracing=\showPSmessages
\hidePSmessages
\xydef@\PSmacro@#1{\PSmacro@@{#1}\PSmessage{#1}}
\xydef@\includeXYPSdict@@{%
 \expandafter\PSinclude@@\expandafter{\xyPSdictname}}
\xydef@\includeXYPSdict@r{\message{PS: includeXYPSdict}\includeXYPSdict@@
 \let\includeXYPSdict@=\relax}
\xylet@\includeXYPSdict@\includeXYPSdict@r
\xydef@\endXYdict@{}
\xydef@\includePSmessage@@{\message{<xyps: including \xyPSdictname}}
\xylet@\includePSmessage@=\includePSmessage@@ 
\xydef@\xyPSdictknown@{%
 \immediate\closein\xyread@
 \xywarning@{File \xyPSdictname\space already exists}
 \message{ Do you wish to overwrite it \string? y/n }%
 \read16 to \next
 \DNii@{\xywarning@{You did not type Y or N -- try again please}%
 \xyPSdictknown@}%
 \DN@{Y }\ifx\next@\next \DNii@{\writePSdict@@}%
 \else\DN@{y }\ifx\next@\next \DNii@{\writePSdict@@}%
 \else\DN@{n }\ifx\next@\next \DNii@{\cancelPSdict@}%
 \else\DN@{N }\ifx\next@\next \DNii@{\cancelPSdict@}%
 \fi\fi\fi\fi \nextii@ }
\xydef@\cancelPSdict@{%
 \xywarning@{cancelling dump of PostScript dictionary}}
\xydef@\noDictmessage@{%
 \xywarning@{\dvitype@\space does not support the use of a header file}}
\DN@{\csname newif\endcsname\ifUsePSdict@@\DN@{}}
 \ifx\undefined\UsePSdict@@true\else\DN@{}\fi \next@
\ifx\undefined\xyPSdefaultdict
 \xydef@\xyPSdefaultdict{%
 \DN@##1.##2.##3@{\gdef\xyPSdictname{xy##1##2dict.pro}}%
 \expandafter\next@\xyversion.@}%
\fi
\ifx\undefined\UsePSheader@
 \xydef@\UsePSheader@#1{%
 \DN@{#1}\ifx\next@\empty
 \else \gdef\xyPSdictname{#1}\fi
 \ifx\xyPSdictname\undefined\xyPSdefaultdict\fi
 \gdef\xyHeaderMessage@{%
 It includes a reference to the PostScript file \xyPSdictname.^^J}%
 \UsePSdict@@true}%
 \let\UsePSheader=\UsePSheader@
\fi
\xywarnifdefined\xyPS@@
\xywarnifdefined\xyPS@@@
{\catcode`|=14 \catcode`\%=12 \catcode`\<=1 \catcode`\>=2 |
 \gdef\xyPS@@<%%>\gdef\xyPS@@@<%!>}
\xydef@\writePSdict@@{\message{PS: writePSdict@@}\writePSdict@ 
 \def\writePSdict@@{\message{write PS relaxed}}}
{\catcode`|=14 \catcode`\%=12 
 \gdef\writePSdict@{{\begingroup|
 \immediate\openout\xywrite@=\xyPSdictname \relax
 \message{<xyps: dumping \xyPSdictname}|
 \def\PSdict@@@##1{\immediate\write\xywrite@{##1}}|
 \let\xyPSobeylines@@=\obeyoutlines@
 \let\firstPS@@=\relax
 \let\endXYdict@=\relax
 \PSdict@@@{\xyPS@@@ PS-Adobe-3.0 Resource-procset}|
 \PSdict@@@{\xyPS@@ Title: \xyPSdictname}|
 \PSdict@@@{\xyPS@@ Version: 3.7}|
 \PSdict@@@{\xyPS@@ Creator: Xy-ps backend to Xy-pic}|
 \PSdict@@@{\xyPS@@ DocumentSuppliedProcSets: XYdict}|
 \ifx\dvitype@\undefined
 \PSdict@@@{\xyPS@@ For: use with Xy-pic}\else
 \PSdict@@@{\xyPS@@ For: \dvitype@ use of Xy-pic}\fi
 \PSdict@@@{\xyPS@@ BeginResource: procset XYdict}|
 \def\PSspecialdict@@##1{\PSdict@@@{##1^^J}}|
 \let\PSdict@@=\PSdict@@@ \let\xy@begindvi=\literal@|
 \UsePSdict@@false\XYpredict@@|
 \XYdict@@|
 \PSdict@@@{\xyPS@@ EndResource}|
 \immediate\closeout\xywrite@
 \message{>}|
 \endgroup}}}
\xywarnifdefined\obeyoutlines@
{\catcode`\^^M=\active%
 \gdef\obeyoutlines@{\catcode`\^^M=\active \def^^M{^^J}%
 \newlinechar=`\^^J\obeyspaces}}
\xydef@\XYpredict@@{\ifUsePSdict@@\DN@{}\else
 \DN@{\xy@begindvi{\xyinputorelse@{xyps-pro}%
 {\xyerror@{Could not load xyps-pro}{}}\xyuncatcodes}}%
 \next@
 \DN@{\xy@begindvi{\xyinputorelse@{xypspatt}%
 {\xyerror@{Could not load xypspatt}{}}\xyuncatcodes}}\fi
 \next@ }
\xydef@\XYpredict@r{\XYpredict@@ \let\XYpredict@=\relax \installxyps@}
\xylet@\XYpredict@\XYpredict@r
\xydef@\XYdict@{\XYdict@@\def\XYdict@{\message{PS relaxed}}}%
\xydef@\XYdict@@{\DN@{\xyinputorelse@{xypsdict}%
 {\xyerror@{Could not load xypsdict}{}}\xyuncatcodes}%
 \expandafter\xy@begindvi\expandafter{\next@}}
\xydef@\forceload@XYdict{%
 \let\includeXYPSdict@=\includeXYPSdict@r
 \let\XYpredict@=\XYpredict@r
 \let\XYdict@=\XYdict@@ \expandafter\installxyps@ }
\xynew@{if}\ifxyPSshapes@ \xyPSshapes@true 
\xydef@\xyPScharwarning@@{\xyPScharmessage@
 \gdef\xyPScharwarning@@{\xyPScharmessage@
 \xywarning@{...no further PostScript warnings will be given}%
 \global\let\xyPScharwarning@@=\relax }}
\xydef@\xyPScharmessage@{\xywarning@{%
 the current <driver> does not fully support PostScript effects}}%
\xydef@\newxyshape#1#2#3{%
 \DN@{#3}\ifx\next@\empty
 \xydefcsname@{shape [#1]}{\csname xyshape@#1@\endcsname}%
 \else \expandafter\def\csname shape [#1]\endcsname{%
 \csname xyshape@#1@\endcsname}\fi
 \DN@{#2}\ifx\next@\empty
 \expandafter\def\csname xyshape@#1@\endcsname{%
 \xyundefinedEffect@{#1}{}@@}%
 \else \expandafter\def\csname xyshape@#1@\endcsname{#2}\fi }
\xydef@\xyundefinedEffect@#1#2@@{%
 \xywarning@{The #1 #2 effect is not implemented with the current driver}}%
\xydef@\newxyPSshape#1#2{%
 \expandafter\DN@\expandafter{\csname shape [#1]\endcsname}%
 \DNii@{\relax}\ifx\next@\nextii@ \newxyshape{#1}{}\relax\fi
 \expandafter\DNii@\expandafter{\csname xyPSshape@#1@\endcsname}%
 \expandafter\def\nextii@{#2}%
 \ifx\nextii@\empty\expandafter\def\next@{\xyPSnotimplemented@@`#1'@@}%
 \else
 \edef\tmp@{\noexpand\let\expandafter\noexpand\next@
 \expandafter\noexpand\nextii@}%
 \expandafter\tmp@\fi }
\xydef@\xyPSnotimplemented@@#1@@{%
 \xywarning@{This PostScript effect is not implemented yet}}%
\xydef@\xyPSnotfinished@@{%
 \xywarning@{This effect is not reliable yet; box sizes may be wrong}}%
\endinput


==> xyps-r.tex <==
%% xyps-r.tex from $Id: xyps-r.doc,v 3.7 1999/02/16 15:12:50 krisrose Exp $
%%
%% Xy-pic ``PostScript Rotations and Scaling''.
%% Copyright (c) 1993-1996 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1996 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\expandafter\ifx\csname xyps-rloaded\endcsname\empty
 \message{not reloaded}\endinput \fi
\expandafter\let\csname xyps-rloaded\endcsname=\empty \xycatcodes
\expandafter\ifx\csname xyps-sloaded\endcsname\empty\else
 \xyinputorelse@{xyps-s}{\xyerror@{Could not load xyps-s}{}}%
 \xycatcodes\fi
\xydef@\installPSrotscale@{\installPSstyle@
 \let\xyRotate@@=\xyPSrotate@@
 \let\doSpecialRotate@@=\doPSspecialRotate@@
 \let\xyscale@@=\xyPSscale@@
 \xyPSshapes@true
 \xyuncatcodes }
\xydef@\UsePSrotate{\installPSrotscale@}
\xydef@\NoPSrotate{\UnloadRotate@\relax}
\xydef@\xyPSpretransform@{\xyPSrawA@{\preXYtransform@@}}
\xydef@\xyPSposttransform@{\xyPSrawZ@{\postXYtransform@@}}
\let\preXYtransform@=\xyPSpretransform@
\let\postXYtransform@=\xyPSposttransform@
\xydef@\xyPSrotSplit@{%
 \expandafter\def\expandafter\preShape@@\expandafter{\xyPSpre@}%
 \expandafter\def\expandafter\postShape@@\expandafter{\xyPSpost@}}
\xydef@\xyPSscale@@#1#2{%
 \xyPSsplitPS@{\xyscale@start(#1,#2)}{\xyscale@end}%
 \xyPSrotSplit@\xyPSpsxy@ }
\xydef@\xyPSrotate@@#1{%
 \xyPSsplitPS@{\xyrot@start(#1 xyd)}{\xyrot@end}%
 \xyPSrotSplit@\xyPSpsxy@ }
\xydef@\xyPSspecialRotate@#1{%
 \xyPSsplitPS@{\xyrot@start(#1)}{\xyrot@end}\xyPSrotSplit@\xyPSpsxy@ }
\xydef@\doPSspecialRotate@@#1@@{\xyPSspecialRotate@{#1}}
\xydef@\xyRotScale@@{%
 \def\xyrot@start(##1){{xyt ##1\space xyr}}%
 \def\xyscale@start(##1,##2){{xyt ##1\space##2\space xys}}%
 \def\xyrot@end{}\def\xyscale@end{}}
\endinput


==> xyps-s.tex <==
%% xyps-s.tex from $Id: xyps-s.doc,v 3.7 1999/02/16 15:12:50 krisrose Exp $
%%
%% Xy-pic ``Style extension'' PostScript support.
%% Copyright (c) 1995-1996 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1996 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\expandafter\ifx\csname xyps-sloaded\endcsname\empty
 \message{not reloaded}\endinput \fi
\expandafter\let\csname xyps-sloaded\endcsname=\empty \xycatcodes
\xydef@\xykillstyles@@{\Unloadstyle@}%
\xywarnifdefined\xyPSescapestyle@
\xywarnifdefined\xyPSsplitescape@
{\xyuncatcodes \catcode`@=11
 \gdef\xyPSescapestyle@#1@@{\xyPSsplitescape@#1<><>@@}%
 \gdef\xyPSsplitescape@#1<>#2<>#3@@{\xyescape@@{#1}{#2}}}
\xydef@\xyPSsplitPS@#1#2{%
 \def\xyPSpre@{#1}\def\xyPSpost@{#2}\modPSboxz@ }
\xydef@\xyescape@@#1#2{\checkXyStyle@ 
 \applyFIFOstyle@\prexyescape@{#1}\postxyescape@{#2}}
\xydef@\prexyescape@{\xyescapeSpecial@}
\xydef@\postxyescape@{\xyescapeSpecial@}
\xylet@\xyescapeSpecial@=\eat@
\let\xyescapeSpecial@=\addtostyletoks@
\xydef@\installPSstyle@{%
 \def\preXYstyle@@{\xyPSpre@}%
 \let\xydoprestyles@=\xyPSrawstyleA@
 \let\xydopoststyles@=\xyPSrawZ@
 \let\xykillstyles@=\xykillstyles@@
 }
\xydef@\xyPSrawstyleA@#1{\xyPSrawA@{{#1}{}}}
\endinput


==> xyps-t.tex <==
%% xyps-t.tex from $Id: xyps-t.doc,v 3.7 1999/02/16 15:12:50 krisrose Exp $
%%
%% Xy-pic ``Pattern and Tile extension'' PostScript support.
%% Copyright (c) 1993-1997 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1997 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\expandafter\ifx\csname xyps-tloaded\endcsname\empty
 \message{not reloaded}\endinput \fi
\expandafter\let\csname xyps-tloaded\endcsname=\empty \xycatcodes
\expandafter\ifx\csname xyps-sloaded\endcsname\empty\else
 \xyinputorelse@{xyps-s}{\xyerror@{Could not load xyps-s}{}}%
 \xycatcodes\fi
\xydef@\installPSpatterns@{\installPSstyle@
 \let\xypattern@=\xyPSpattern@@
 \let\xypatternwarning@=\relax
 \xystandardpatterns@
 \xyuncatcodes }
\xylet@\UnloadPSpatterns@=\Unloadpattern@
\xydef@\UsePStiles{\installPSpatterns@}
\xydef@\NoPStiles{\UnloadPSpatterns@\relax}
\xydef@\xyPSnewpattern@#1#2#3#4#5{%
 \expandafter\DN@\expandafter{\csname shape [#1]\endcsname}%
 \DNii@{\relax}\ifx\next@\nextii@\newxypattern{#1}{}\relax\fi
 \DNii@{#4}\ifx\nextii@\empty
 \expandafter\DNii@\expandafter{\csname xyPSshape@#1@\endcsname}%
 \expandafter\def\nextii@{\xyPSpattern@{#2 #3}}\else
 \expandafter\DNii@\expandafter{\csname xyPSshape@#1@\endcsname}%
 \expandafter\def\nextii@{\xyPSpattern@{#4}}\fi
 \ifx\nextii@\empty\expandafter\def\next@{\xyPSnotimplemented@@`#1'@@}%
 \else
 \edef\tmp@{\noexpand\let\expandafter\noexpand\next@
 \expandafter\noexpand\nextii@}\expandafter\tmp@\fi }
\xydef@\xyPSpattern@{\ifPSspecials@\expandafter\xyPSpattern@@
 \else\expandafter\eat@\fi}%
\xydef@\xyPSpattern@@#1{\bgroup \checkXyStyle@ 
 \def\preStyle@@{\expandafter\addtostyletoks@\expandafter{\xyPSpre@}}%
 \def\postStyle@@{\expandafter\addtostyletoks@\expandafter{\xyPSpost@}}%
 \let\modPSboxz@=\modXYstyle@ \xyPS@pattern@@{#1}%
 \toks@={\egroup\let\xy@style@=\relax \def\Drop@@}%
 \expandafter\addtotoks@\expandafter{\expandafter{\Drop@@}\def\Connect@@}%
 \expandafter\addtotoks@\expandafter{\expandafter{\Connect@@}}%
 \the\toks@ }
\xydef@\xyPS@pattern@@#1{\xyPSsplitPS@{{#1}sp}{}}
\endinput


==> xyps.tex <==
%% xyps.tex from $Id: xyps.doc,v 3.7 1999/02/16 15:12:50 krisrose Exp $
%%
%% Xy-pic ``PostScript backend''.
%% Copyright (c) 1993-1997 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1997 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{ps}{PostScript backend}{\stripRCS$Revision: 3.7 $}%
 {Ross Moore}{ross@mpce.mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xydef@\UsePSspecials{\DNii@{{[4]}}\xyFN@\UsePSspecials@i}
\xydef@\UsePSspecials@i{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\UsePSspecials@i}%
 \else\ifx [\next \DN@[##1]{\DNii@{{[##1]}}\xyFN@\UsePSspecials@i}%
 \else\ifcat 5\noexpand\next \DN@##1{\DNii@{{[##1]}}\xyFN@\UsePSspecials@i}%
 \else\ifx\bgroup\next \DN@{\expandafter\UsePS@specials\nextii@}%
 \else \DN@{\UsePS@specials{[4]}}%
 \fi\fi\fi\fi \next@ }
\xydef@\UsePS@specials#1#2{%
 \ifx\empty\whichPSspecials@
 \DN@{#2}\ifx\next@\empty
 \else
 \expandafter\let\expandafter\next\csname#2@\endcsname
 \ifx\next\relax \DN@{\UsePSspecials@{#2}{}}%
 \else \DN@{\UsePSspecials@{#2}{#1}}\fi
 \fi
 \else
 \DN@{#2}\ifx\next@\empty \DN@{\PSspecials@true}%
 \else
 \DN@{#2}%
 \edef\nextii@{\expandafter\string\whichPSspecials@}%
 \ifx\next@\nextii@\DN@{\PSspecials@true}%
 \else
 \ifx\firstPS@@\relax
 \DN@{\xyerror@{Only one PS <driver> allowed: \dvitype@ already loaded}{}}%
 \else
 \expandafter\let\expandafter\next\csname#2@\endcsname
 \ifx\next\relax
 \DN@{\xyerror@{PostScript specials for `#2' not supported}{}}%
 \else 
 \xywarning@{Changing PS <driver> to #2 }%
 \DN@{\UsePSspecials@{#2}{#1}}%
 \fi
 \fi
 \fi
 \fi
 \fi \next@}
\xydef@\UseDVIPSspecials{\UsePSspecials@\dvips@}
\xydef@\UseTexturesPSspecials{\UsePSspecials@\Textures@}
\xydef@\UseTexturesSpecials{\UsePSspecials@\Textures@}
\xydef@\UsePostScriptSpecials{\UsePSspecials@\dvips@}
\xydef@\UseOzTeXspecials{\UsePSspecials@\OzTeX@}
\xydef@\UseDVITOPSspecials{\UsePSspecials@\dvitops@}
\message{drivers,}
\xydef@\loadPSdriver@#1#2{\xyinputorelse@{xy#1}%
 {\xyrequire{#2}\expandafter\ifx\csname xy#2loaded\else
 {\xyerror@{Unable to load xy#1.tex for #2 driver}{}}\fi}}
\xydef@\dvips@{\loadPSdriver@{ps-dvi}{dvips}}
\xydef@\Textures@{\loadPSdriver@{ps-txt}{Textures}}
\xydef@\OzTeX@{\loadPSdriver@{ps-oz}{OzTeX}}
\xydef@\dvitops@{\loadPSdriver@{ps-dto}{dvitops}}
\xydef@\dvipsone@{\loadPSdriver@{ps-one}{dvipsone}}
\global\newif\ifPSspecials@ 
\xydef@\UsePSspecials@#1{\def\whichPSspecials@{#1}%
 \DN@{\Textures@}\ifx\next@\whichPSspecials@
 \DN@##1{\xyrequire{textures}%
 \def\whichPSspecials@{textures}\xyps@options}%
 \else\DN@{\dvips@}\ifx\next@\whichPSspecials@
 \DN@##1{\xyrequire{dvips}%
 \def\whichPSspecials@{dvips}\xyps@options}%
 \else\DN@{\OzTeX@}\ifx\next@\whichPSspecials@
 \DN@##1{\xyrequire{oztex}%
 \def\whichPSspecials@{oztex}\xyps@options}%
 \else\DN@{\dvitops@}\ifx\next@\whichPSspecials@
 \DN@##1{\xyrequire{dvitops}%
 \def\whichPSspecials@{dvitops}\xyps@options}%
 \else
 \DN@##1{\xyrequire{ps}\xyrequire{#1}\xyps@options}%
 \fi\fi\fi\fi \next@ }
\xydef@\xyps@options{%
 \xyrequire{ps}\xyrequire{line}\xyrequire{color}\xyrequire{crayon}%
 \xyrequire{rotate}\xyrequire{tile}\xyrequire{frame}\xyuncatcodes }
\xydef@\whichPSspecials@{}
\xydef@\NoPSspecials{\xyPSwarning@{off}%
 \PSspecials@false\aftergroup\resetPS@}
\xydef@\resetPS@{\ifPSspecials@\xyPSwarning@{back on}\fi}
\xydef@\UsePSspecials@x{\PSspecials@true\resetPS@}
\xydef@\xyPSwarning@#1{\xywarning@{PostScript switched #1}}
\xyaddunsupport{ps}{\csname UnloadPS@@\endcsname}
\xydef@\PSspecials@{%
 \ifx\next[\DN@[##1]{\setxyPSlevel@{##1}\xyFN@\PSspecials@}%
 \else\DN@{\whichPSspecials@\PSspecials@@}%
 \fi \next@ }%
\xydef@\PSspecials@@{%
 \ifx\und@fined\PSmessage\hidePSmessages\fi \setupxyPS@}
\xydef@\setupxyPSlevelO@{\relax}
\xydef@\setxyPSlevel@#1{\ifcase#1%
 \gdef\setupxyPS@{\setupxyPSlevelO@}%
 \or\gdef\setupxyPS@{\setupxyPSlevelA@}%
 \or\gdef\setupxyPS@{\setupxyPSlevelB@}%
 \or\gdef\setupxyPS@{\setupxyPSlevelC@}%
 \or\gdef\setupxyPS@{\setupxyPSlevelD@}%
 \else\gdef\setupxyPS@{\setupxyPSlevelD@}\fi }
\xywarnifdefined\setupxyPS@ 
 \gdef\setupxyPS@{\setupxyPSlevelD@ \gdef\setupxyPS@{\PSspecials@true}}
\xydef@\PSincrease@#1{%
 \xywarning@{The PS level may only increase: #1 is already active}}
\DN@{\csname newif\endcsname\ifUsePSdict@@\DN@{}}
 \ifx\undefined\UsePSdict@@true\else\DN@{}\fi \next@
\ifx\undefined\xyPSdefaultdict
 \xydef@\xyPSdefaultdict{%
 \DN@##1.##2.##3@{\gdef\xyPSdictname{xy##1##2dict.pro}}%
 \expandafter\next@\xyversion.@}%
\fi
\ifx\undefined\UsePSheader@
 \xydef@\UsePSheader@#1{%
 \DN@{#1}\ifx\next@\empty
 \else \gdef\xyPSdictname{#1}\fi
 \ifx\xyPSdictname\undefined\xyPSdefaultdict\fi
 \gdef\xyHeaderMessage@{%
 It includes a reference to the PostScript file \xyPSdictname.^^J}%
 \UsePSdict@@true}%
 \let\UsePSheader=\UsePSheader@
\fi
\xydef@\dumpPSdict#1{\DN@{#1}\ifx\next@\empty
 \ifx\undefined\xyPSdictname\xyPSdefaultdict\fi
 \else\gdef\xyPSdictname{#1}\fi
 \def\dumpPSdict@@{\writePSdict@@}%
 \ifx\xydriversselected@@\empty\DN@{\xysetup@@\null@xy@ps}%
 \else \DN@{\installxyps@x}\fi \next@}
\message{hooks,}
\gdef\xyPSalternative@#1#2{%
\expandafter\global\expandafter\let\csname origxy#2@\endcsname=#1%
 \xdef#1{\noexpand\ifPSspecials@
 \noexpand\expandafter\expandafter\noexpand\csname xyPS#2@\endcsname
 \noexpand\else
 \noexpand\expandafter\expandafter\noexpand\csname origxy#2@\endcsname
 \noexpand\fi}}%
\xydef@\setupxyPSlevelA@{\xyPStips@%
 \xyPSalternative@{\Tip@@}{Tip}%
 \xyPSalternative@{\Ttip@@}{Ttip}%
 \xyPSalternative@{\Tip@@eu}{Tip@eu}%
 \xyPSalternative@{\Ttip@@eu}{Ttip@eu}%
 \xyPSalternative@{\hook@@}{hook}%
 \xyPSalternative@{\ahook@@}{ahook}%
 \xyPSalternative@{\bhook@@}{bhook}%
 \xyPSalternative@{\aturn@@}{aturn}%
 \xyPSalternative@{\bturn@@}{bturn}%
 \xyPSalternative@{\squiggle@@}{squiggle}%
 \xyPSalternative@{\stopper@@}{stopper}%
 \xyPSalternative@{\line@@}{dash}%
 \xyPSalternative@{\circhar@@}{circhar@}%
 \gdef\setupxyPSlevelA@{\PSincrease@{1}}%
 \global\let\UsePSspecials=\UsePSspecials@x \PSspecials@true}
\xydef@\setupxyPSlevelB@{%
 \let\xyPSfont@=\empty \let\xyPSsemifont@=\empty
 \xyPSalternative@{\cirrestrict@@}{cirrest}%
 \gdef\setupxyPSlevelB@{\PSincrease@{2}}%
 \setupxyPSlevelA@ }
\xydef@\setupxyPSlevelC@{%
 \xyPSalternative@{\cirbuild@}{cirbuild}%
 \xyPSalternative@{\CIRfull@}{CIRfull}%
 \xyPSalternative@{\solid@}{solid}%
 \xyPSalternative@{\point@}{point}%
 \xywithoption{curve}{%
 \xyPSalternative@{\splinesolid@}{splinesolid}}%
 \gdef\setupxyPSlevelC@{\PSincrease@{3}}%
 \setupxyPSlevelB@ }%
\xydef@\setupxyPSlevelD@{%
 \xyPSalternative@{\dash@}{dashed}%
 \xywithoption{curve}{%
 \xyPSalternative@{\splinedashed@}{splinedashed}%
 \xyPSalternative@{\splinedotted@}{splinedotted}}%
 \gdef\setupxyPSlevelD@{}%
 \setupxyPSlevelC@ }
\xydef@\xyPSchar@#1{%
 \PSmacro@{\the\Direction\space \xyPSfont@ #1}}
\xydef@\xyPSsemichar@#1{%
 \PSmacro@{\the\Direction\space \xyPSsemifont@ #1}}
\xydef@\xyPSfont@{f }%
\xydef@\xyPSsemifont@{fs }%
\xydef@\xyPStip@{\xyPSchar@{t}}%
\xydef@\xyPSTip@{\xyPSchar@{/XT tt}}%
\xydef@\xyPSTtip@{\setboxz@h\bgroup 
 \reverseDirection@\line@ \wdz@=\z@ \ht\z@=\z@ \dp\z@=\z@ 
 \kern-\L@c \boxz@ \kern\L@c \xyPSchar@{/Xt tT}}%
\xydef@\xyPSTip@eu@{\xyPSchar@{/ET tt}}%
\xydef@\xyPSTtip@eu@{\setboxz@h\bgroup 
 \reverseDirection@\line@ \wdz@=\z@ \ht\z@=\z@ \dp\z@=\z@ 
 \kern-\L@c \boxz@ \kern\L@c \xyPSchar@{/ET tT}}%
\xydef@\xyPScm@\tip@x{\xyFN@\xyPScm@@}%
\xydef@\xyPScm@@{%
 \ifx\next\tip@@ \DN@\tip@@{\tip@x\xyPScmtip@}%
 \else\ifx\next\atip@@ \DN@\atip@@{\tip@x\xyPScmatip@}%
 \else\ifx\next\btip@@ \DN@\btip@@{\tip@x\xyPScmbtip@}%
 \else\DN@{}%
 \fi\fi\fi \next@}%
\xydef@\xyPScmtip@{\xyPSchar@{ct}}%
\xydef@\xyPScmatip@{\xyPSchar@{ca}}%
\xydef@\xyPScmbtip@{\xyPSchar@{cb}}%
\xydef@\xyPStips@{%
 \xyPSalternative@{\atip@@}{atip}%
 \xyPSalternative@{\btip@@}{btip}%
 \xyPSalternative@{\tip@@}{abtip}%
}%
\xydef@\xyPSatip@{\xyPSwhichatip@ 
 \expandafter\xyPSchar@\expandafter{\xyPSfont@@}}%
\xydef@\xyPSbtip@{\xyPSwhichbtip@
 \expandafter\xyPSchar@\expandafter{\xyPSfont@@}}%
\xydef@\xyPSabtip@{\xyPSwhichabtip@
 \expandafter\xyPSchar@\expandafter{\xyPSfont@@}}%
\xydef@\xyPSwhichatip@{\ifx\xyatipfont\xy@@atfont
 \expandafter\xyPSatip@i \else\def\xyPSfont@@{10 /xy A}\fi }%
\xydef@\xyPSwhichbtip@{\ifx\xybtipfont\xy@@btfont
 \expandafter\xyPSbtip@i \else\def\xyPSfont@@{10 /xy B}\fi }%
\xydef@\xyPSwhichabtip@{\ifx\xyatipfont\xy@@atfont
 \expandafter\xyPSabtip@i \else\def\xyPSfont@@{10 /xy AB}\fi }%
\xydef@\xyPSatip@i{%
 \edef\xyPSfont@@{\tipsize@@\space/\tipfamily@@\space A}} 
\xydef@\xyPSbtip@i{%
 \edef\xyPSfont@@{\tipsize@@\space/\tipfamily@@\space B}} 
\xydef@\xyPSabtip@i{%
 \edef\xyPSfont@@{\tipsize@@\space/\tipfamily@@\space AB}} 
\xydef@\xyPSTtips@{%
 \let\Ttip@xy=\Ttip@
 \let\Ttip@cm=\Ttip@
 \let\Ttip@eu=\Ttip@ }
\xydef@\xyPShook@{\xyPSchar@{h}}%
\xydef@\xyPSahook@{\xyPSchar@{ha}}%
\xydef@\xyPSbhook@{\xyPSchar@{hb}}%
\xydef@\xyPSaturn@{\xyPSchar@{ta}}%
\xydef@\xyPSbturn@{\xyPSchar@{tb}}%
\xydef@\xyPSsquiggle@{\xyPSchar@{g}}%
\xydef@\xyPSstopper@{\xyPSchar@{st}}%
\xydef@\xyPSfliptrue@{\DN@{\xyPSsemichar@{T d}}}
\xydef@\xyPSdash@{%
 \DN@{\xyPSsemichar@{F d}}%
 \ifnum\SemiDirectionChar=31
 \ifdim\d@Y<\z@ 
 \ifdim\d@X<\z@ \ifx\xyPSsemifont@\empty\xyPSfliptrue@\fi\fi
 \else
 \ifdim\z@>\d@X 
 \ifx\xyPSsemifont@\empty\else\xyPSfliptrue@\fi
 \else\xyPSfliptrue@\fi
 \fi\fi
 \next@ \setboxz@h{\origxydash@}\kern\wdz@ 
 \setbox\z@=\box\voidb@x }
\xydef@\xyPScirchar@#1{\count@=#1\edef\tmp@{\the\count@}%
 \ifcase#1%
 \xyPScirchar@@@{-180}{-135}{\tmp@}\dimen@=\partroottwo\R@
 \or\xyPScirchar@@@{-135}{-90}{\tmp@}\dimen@=\halfroottwo\R@
 \or\xyPScirchar@@@{-90}{-45}{\tmp@}\dimen@=\halfroottwo\R@
 \or\xyPScirchar@@@{-45}0{\tmp@}\dimen@=\partroottwo\R@
 \or\xyPScirchar@@@0{45}{\tmp@}\dimen@=\partroottwo\R@
 \or\xyPScirchar@@@{45}{90}{\tmp@}\dimen@=\halfroottwo\R@
 \or\xyPScirchar@@@{90}{135}{\tmp@}\dimen@=\halfroottwo\R@
 \or\xyPScirchar@@@{135}{180}{\tmp@}\dimen@=\partroottwo\R@
 \fi}
\xydef@\xyPScirrest@{\relax}%
\xydef@\xyPScirchar@@#1{\relax\count@=#1\edef\tmp@{\the\count@}%
 \expandafter\xyPScirchar@@@\ifcase#1%
 {-180}{-135}{\tmp@}\kern\partroottwo\R@
 \or{-135}{-90}{\tmp@}\kern\halfroottwo\R@
 \or{-90}{-45}{\tmp@}\kern\halfroottwo\R@
 \or{-45}0{\tmp@}\kern\partroottwo\R@
 \or 0{45}{\tmp@}\kern\partroottwo\R@
 \or{45}{90}{\tmp@}\kern\halfroottwo\R@
 \or{90}{135}{\tmp@}\kern\halfroottwo\R@
 \or{135}{180}{\tmp@}\kern\partroottwo\R@
 \fi}
\xydef@\xyPScirchar@@@#1#2#3{\edef\tmp@{#1\space#2\space
 \expandafter\removePT@\the\R@\space #3\space c}%
 \PSmacro@{\tmp@}}
\xydef@\xyPScirc@#1#2{\edef\tmp@{\expandafter\removePT@\the\R@}%
 \PSmacro@{\tmp@\space #1 #2 o}}
\xydef@\xyPSCIRfull@{\setboxz@h{\kern\R@\xyPScirc@0{360}\kern\R@}%
 \wd\z@=\z@ \ht\z@=\R@ \dp\z@=\R@ \boxz@}%
\xydef@\xyPScirbuild@{{%
 \count@=\CIRlo@@ \count@@=\CIRhi@@ 
 \multiply\count@ by45 \advance\count@-180 \relax
 \multiply\count@@ by45 \advance\count@@-180 \relax
 \def\tmp@{}%
 \ifx\CIRtest@@\CIRtest@inside 
 \ifnum\count@@>\count@
 \edef\tmp@{\noexpand\xyPScirc@{\the\count@}{\the\count@@}}\fi
 \else\ifx\CIRtest@@\CIRtest@outside
 \ifnum\count@>-180 \advance\count@ by360 \relax
 \edef\tmp@{\noexpand\xyPScirc@{\the\count@@}{\the\count@}}%
 \else
 \ifnum\count@@<180 \relax
 \edef\tmp@{\noexpand\xyPScirc@{\the\count@@}{180}}%
 \fi\fi
 \fi\fi
 \kern\R@\tmp@\kern\R@}}
\xydef@\xyPSstraight@#1{\setupDirection@
 \edef\Creset@@{\cfromthec@ \pfromthep@ \DirectionfromtheDirection@}%
 \DN@##1##2{\def\checkoverlap@@{%
 \ifdim##1\X@p>##1\X@c \let\next@=\relax \fi
 \ifdim##2\Y@p>##2\Y@c \let\next@=\relax \fi}}%
 \edef\nextii@{{\sd@X}{\sd@Y}}\expandafter\next@\nextii@
 \noCshavep@@
 \edef\Cshavep@@{\pfromthep@ \noexpand\resetDirection@}%
 \noCshavec@@
 \edef\Cshavec@@{\cfromthec@ \noexpand\resetDirection@}%
 \ifHidden@\else
 \ifdim\Y@c>\Y@max \Y@max=\Y@c \fi \ifdim\Y@p>\Y@max \Y@max=\Y@p \fi
 \ifdim\Y@c<\Y@min \Y@min=\Y@c \fi \ifdim\Y@p<\Y@min \Y@min=\Y@p \fi
 \ifdim\X@c>\X@max \X@max=\X@c \fi \ifdim\X@p>\X@max \X@max=\X@p \fi
 \ifdim\X@c<\X@min \X@min=\X@c \fi \ifdim\X@p<\X@min \X@min=\X@p \fi \fi
 \ifInvisible@\let\next@=\relax \else
 \DN@{\setboxz@h{\kern\X@c \raise\Y@c\hbox{#1}}%
 \ht\z@=\z@ \wd\z@=\z@ \dp\z@=\z@ {\xykillstyles@\Drop@@}}%
 \fi 
 \checkoverlap@@
 \ifdim\d@X=\z@ \ifdim\d@Y=\z@ \DN@{\relax}\fi\fi \next@
 \def\Cslidep@@{\noCslidep@@}\def\Cslidec@@{\noCslidec@@}%
 \def\Calong@@{\noCalong@@}\Creset@@ }
\xylet@\xykillstyles@=\relax
\xydef@\xyPSsolid@{\straight@\xyPSsolidSpread@}%
\xydef@\xyPSsolidSpread@{\xyPSspread@{solid}{l}@@}%
\xydef@\xyPSdottedSpread@{\xyPSspread@{dotted}{dt}@@}%
\xydef@\xyPSdashed@{\line@ \def\Connect@@{\straight@\xyPSdashedSpread@}}
\xydef@\xyPSdashedSpread@{\xyPSspread@{dashed}{dd}@@}%
\xydef@\xyPSspread@#1#2@@#3\repeat@{\edef\tmp@{%
 \expandafter\removePT@\the\d@X\space\expandafter\removePT@\the\d@Y}%
 \setboxz@h{\kern\X@c \raise\Y@c\hbox{%
 \PSmessage{#1 line:}\PSmacro@{\tmp@\space #2}}}%
 \ht\z@=\z@ \wd\z@=\z@ \dp\z@=\z@ \boxz@}
\xydef@\xyPSpoint@{\xyPSzerodot@\egroup
 \Invisible@false \Hidden@false \def\Leftness@{.5}\def\U@pness@{.5}\ctipEdge@
 \def\Drop@@{\styledboxz@}\def\Connect@@{\straight@\xyPSdottedSpread@}}
\xydef@\xyPSzerodot@{\PSmessage{dot:}\PSmacro@{p}}
\xydef@\xyPScubic@#1{\readsplineparams@
 \PSmessage{CUBIC:}%
 \DN@{#1}\ifx\next@\empty\PSmacro@{mark \cubicinfo@\space bz}%
 \else\PSmacro@{mark \cubicinfo@\space b#1}\fi}
\xydef@\xyPSsquine@#1{\readsplineparams@
 \PSmessage{SQUINE:}%
 \DN@{#1}\ifx\next@\empty\PSmacro@{mark \squineinfo@\space q#1}%
 \else\PSmacro@{mark \squineinfo@\space q#1}\fi}
\xydef@\xyPSsplinesolid@{\ifx\splineinfo@\squineinfo@
 \expandafter\xyPSsquine@\else\expandafter\xyPScubic@\fi{}}
\xydef@\xyPSsplinedashed@{\ifx\splineinfo@\squineinfo@
 \expandafter\xyPSsquine@\else\expandafter\xyPScubic@\fi{d}}
\xydef@\xyPSsplinedotted@{\ifx\splineinfo@\squineinfo@
 \expandafter\xyPSsquine@\else\expandafter\xyPScubic@\fi{t}}
\xyendinput


==> xypsdict.tex <==
%% xypsdict.tex from $Id: xypsdict.doc,v 3.7 1999/02/16 15:12:50 krisrose Exp $
%%
%% Xy-pic ``PostScript backend prolog''.
%% Copyright (c) 1995-1997 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1997 Kristoffer H. Rose <krisrose@ens-lyon.fr>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
\begingroup \xycatcodes%
 \count@=\xydashl@\relax \count@@=\xydashw@\relax%
 \XYpredict@\relax \xycatcodes \xyPSobeylines@@%
\PSdict@@{/XYdict where pop begin XYdict begin}%
\PSdict@@{%
 /xysize 10 def /T true def /F false def
 /dimendiv{65536 div}bind def 
 /xysegl \number\count@\space dimendiv def 
 /xyopp{1 -1 scale}bind def 
 /xynormwidth{\number\count@@\space dimendiv pscorrect}bind def
 /xywidth{xynormwidth setlinewidth}bind def 
}%
\PSdict@@{%
 /xyfont{4096 add 64 div round 64 mul 4096 sub}def /xydt 0.01 def
 /xysdfont{4096 add 32 div round 32 mul 4096 sub}def 
 /xydots{xywidth 1 setlinecap [xydt 2] 0 setdash}bind def 
 /f /xyfont load def /fs /xysdfont load def}%
\PSdict@@{%
 /xyCheckDir{dup 8 div 3 mul 3 -1 roll sub neg exch div 360 mul 
 dup dup XYdirection sub 180 div round 180 mul XYdirection add 
 dup 3 -1 roll sub abs 10 gt not{exch}if pop}def 
}%
\ifdim\xydashw@=0pt\xydashw@=.4pt\fi\count@@=\xydashw@\relax%
\PSdict@@{%
 /xyrulth{\number\count@@\space dimendiv pscorrect setlinewidth 
 0 setlinecap}bind def
}%
\PSdict@@{%
 /gsavexy{gsave xypspt XYdirection rotate xywidth newpath 0 0 moveto}def 
 /gchksavexy{gsave xypspt setupDirection xywidth newpath 0 0 moveto}def 
}%
\PSdict@@{%
 /xyswap{XYdirection 180 add /XYdirection exch def}def 
 /xyline{gstartxy setupDirection rlineto xystroke}def 
}%
\PSdict@@{%
 /dash{exch gchksavexy xysegl XYdirection dup 
 -90 lt{pop neg}{90 gt{neg}if}ifelse exch{neg}if
 0 rlineto xystroke}def 
 /stopper{gstartxy setupDirection 0 xysegl 2 div rmoveto 
 0 xysegl neg rlineto xystroke }def 
 /d /dash load def /st /stopper load def}%
\PSdict@@{%
 /solid{gstartxy xydash neg exch neg exch rlineto xystroke}def 
 /dashed{gstartxy 2 copy dup mul exch dup mul add sqrt dup 
 xysegl add xysegl 2 mul div round 2 mul 1 sub div [ exch dup ] 0 setdash 
 neg exch neg exch rlineto xystroke}def
 /l /solid load def /dd /dashed load def}%
\PSdict@@{%
 /dot{gstartxy 2 setlinecap [xydt 2] 0 setdash 
 1 0 rlineto xystroke}def 
 /dotted{gstartxy 2 copy dup mul exch dup mul add sqrt dup 
 2 div round 1 add div 2 setlinecap [xydt 3 -1 roll] 0 setdash 
 neg exch neg exch rlineto 0 0 rlineto xystroke}def
 /p /dot load def /dt /dotted load def}%
\PSdict@@{%
 /cubic{gstartxy docubic} def 
 /docubic{chkvalid 
 {chkcubedge 8 -2 roll moveto curveto xystroke pop}
 {cleartomark grestore}ifelse}def 
 /chkcubedge{2 copy 1.0 eq{0.0 eq{pop pop}{cubicedge}ifelse}
 {pop cubicedge}ifelse}def
 /bz /cubic load def}%
\PSdict@@{%
 /dotcubic{gstartxy 1 setlinecap [xydt 2] 0 setdash docubic}def 
 /dashcubic{gstartxy [5 5] 0 setdash docubic}def 
 /bt /dotcubic load def /bd /dashcubic load def}%
\PSdict@@{%
 /squine{gstartxy dosquine}def 
 /dosquine{chkvalid 
 {chksquedge 2 copy moveto xysq2cub curveto xystroke pop}
 {cleartomark grestore}ifelse}def
 /q /squine load def}%
\PSdict@@{%
 /chkvalid{2 copy lt{dup 1 gt{false}{true}ifelse}{false}ifelse}def 
}%
\PSdict@@{%
 /chksquedge{2 copy 1.0 eq{0.0 eq{pop pop}{squineedge}ifelse}
 {pop squineedge}ifelse}def 
 /xysq2cub{xysq2cubit 6 1 roll xysq2cubit 6 1 roll 3 index 3 index 
 xysq2cubit 6 1 roll xysq2cubit 6 1 roll pop pop}def 
 /xysq2cubit{2 index 2 mul add 3 div}def 
}%
\PSdict@@{%
 /dotsquine{gstartxy 1 setlinecap [xydt 2] 0 setdash dosquine}def 
 /dashsquine{gstartxy [5 5] 0 setdash dosquine}def 
 /qt /dotsquine load def /qd /dashsquine load def}%
\PSdict@@{%
/xy4mul{8 copy 
 5 -1 roll mul 5 1 roll 6 -1 roll mul 6 1 roll 
 3 -1 roll mul exch 4 -1 roll mul 3 1 roll 
 add 3 1 roll add exch 10 2 roll 
 7 -1 roll mul 7 1 roll 4 -1 roll mul 5 1 roll 
 4 -1 roll mul 4 1 roll mul add 3 1 roll add 
 exch 3 -1 roll }def 
}%
\PSdict@@{%
 /xy44mul{4 copy 16 4 roll exch 3 1 roll 4 copy 12 4 roll
 xy4mul 12 4 roll xy4mul 12 -4 roll 4 copy 16 4 roll
 8 4 roll xy4mul 12 4 roll xy4mul}def
}%
\PSdict@@{%
 /cubicedge{10 2 roll exch 8 1 roll 3 -1 roll dup dup 9 2 roll
 5 -1 roll dup dup 9 1 roll 8 3 roll
 4 1 roll dup dup 5 3 roll dup dup 5 1 roll 3 -1 roll
 18 -2 roll 2 copy 1 sub neg 4 1 roll 1 sub neg exch 4 1 roll
 xy444mul
 pop pop pop 13 1 roll pop pop pop 9 1 roll 10 1 roll
 pop 8 1 roll 7 1 roll 8 1 roll pop 5 1 roll 3 1 roll}def
}%
\PSdict@@{%
 /xy444mul{4 copy 24 4 roll 12 -4 roll 16 4 roll 4 copy 16 4 roll
 xy44mul 20 8 roll xy44mul
 12 -4 roll 4 -1 roll 7 1 roll exch 4 1 roll exch 6 -1 roll exch
 4 2 roll 16 8 roll 8 4 roll
 4 -1 roll 7 1 roll exch 4 1 roll exch 6 -1 roll exch 4 2 roll
 8 4 roll 16 4 roll 8 4 roll 20 -4 roll exch 3 1 roll
 4 copy 20 4 roll 4 copy 16 4 roll 4 copy 12 4 roll
 xy4mul 28 4 roll xy4mul 20 4 roll xy4mul 12 4 roll xy4mul}def
}%
\PSdict@@{%
 /squineedge{8 2 roll
 exch 5 1 roll 3 -1 roll dup 6 2 roll 1 index exch
 10 -2 roll 2 copy 1 sub neg 4 1 roll 1 sub neg exch 4 1 roll
 xy44mul 4 1 roll pop 5 1 roll 6 1 roll 3 -1 roll pop}def
}%
\PSdict@@{%
 /xyshort{2 copy abs exch abs add xysegl .5 mul lt
 {pop pop grestore}{rlineto xystroke}ifelse}def
}%
\PSdict@@{%
 /tipwidth{xywidth xynormwidth dup currentlinewidth exch div 
 sqrt dup dup scale mul setlinewidth 1 setlinecap}def
}%
\PSdict@@{%
 /halftip{tipwidth xysize 10 div 0 0 moveto
 -.25 0 3 -1 roll -2.5 mul 0 xysize 2 div neg
 dup .62 mul 2 div neg curveto}bind def
}%
\PSdict@@{/atip{gchksavexy halftip xystroke}def
 /btip{gchksavexy xyopp halftip xystroke}def
 /tip{gchksavexy gsave halftip stroke grestore
 xyopp halftip xystroke}def
 /t /tip load def /a /atip load def /b /btip load def}%
\PSdict@@{/cmatip{gchksavexy halfcmtip xystroke}def 
 /cmbtip{gchksavexy xyopp halfcmtip xystroke}def
 /cmtip{gchksavexy gsave halfcmtip stroke grestore
 xyopp halfcmtip xystroke}def
 /halfcmtip{tipwidth 0 0 moveto
 -.1333 0 .25 neg dup .125 3 -1 roll .25 curveto}bind def
 /ct /cmtip load def /ca /cmatip load def /cb /cmbtip load def}%
\PSdict@@{%
 /xyfscale{/xyfsize exch def}def /xyfsize{10}def
 /eu{-0.0551 0.0643 -0.0976 0.1386 -0.125 0.2188}def
 /cm{-0.105 0.0437 -0.1804 0.1380 -0.2 0.25}def
 /XY{-0.1753 0.0181 -0.3452 0.0708 -0.5 0.155}def
 /tipstart{3 -1 roll gchksavexy exch xyfscale tipwidth dup XYdict exch 
 known{dup /xy eq{pop /XY}if}{pop /XY}ifelse XYdict exch get}def
 /tipend{halfxytip xystroke}def 
 /halfxytip{1 1 6{pop xyfsize mul 6 1 roll}for 0 0 moveto curveto}def
 /A{tipstart D}def /B{tipstart C}def /C{xyopp D}def /D{exec tipend}def
 /AB{tipstart dup gsave exec halfxytip stroke grestore C}def
}%
\PSdict@@{%
 /Tip{exch gchksavexy /xyfsize{10}def tipwidth gsave 
 dup XYdict exch known{dup /xy eq{pop /XT}if}{pop /XT}ifelse
 XYdict exch get dup
 halfTip stroke grestore xyopp halfTip xystroke}def
 /XT{360 32 div neg}def /Xt{-1 .31 mul 1 atan}def
 /ET{360 64 div 5 mul neg}def /Et{-1 .31 mul 1 atan}def
 /halfTip{exec rotate XY halfxytip}def /halfTtip{halfTip}def
 /Ttip{exch gchksavexy /xyfsize{10}def tipwidth gsave 
 dup XYdict exch known{dup /xy eq{pop /Xt}if}{pop /Xt}ifelse
 XYdict exch get dup
 halfTtip stroke grestore xyopp halfTtip xystroke}def
 /tt /Tip load def /tT /Ttip load def}%
\PSdict@@{/halfturn{xysegl 2 div dup dup neg exch rmoveto
 0 exch dup exch -180 -90 arc}bind def
 /aturn{gchksavexy halfturn xystroke}def
 /bturn{gchksavexy xyopp halfturn xystroke}def
 /ta /aturn load def /tb /bturn load def}%
\dimen@=\xybsqll@\relax\count@=\dimen@%
\PSdict@@{%
 /xysqll \the\count@\space dimendiv def 
 /squigl{gchksavexy xysqll dup neg 0 rmoveto
 2 div dup dup neg dup 3 -1 roll
 2 sqrt mul dup 5 1 roll
 135 45 arcn dup 3 -1 roll -135 -45 arc
 xystroke}def
 /g /squigl load def}%
\PSdict@@{/fullhook{0 xysegl 2 div dup -90 90 arcn}bind def
 /halfhook{xysegl 2 div dup 0 exch 180 90 arcn}bind def
}%
\PSdict@@{/ahook{gchksavexy fullhook xystroke}def
 /bhook{gchksavexy xyopp fullhook xystroke}def
 /hook{gchksavexy gsave halfhook stroke grestore
 xyopp halfhook xystroke}def
 /h /hook load def /ha /ahook load def /hb /bhook load def}%
\PSdict@@{%
 /xyqcirc{dup dup neg exch translate newpath 
 dup neg 0 exch moveto 0 0 3 -1 roll -90 0 arc}bind def
}%
\PSdict@@{%
 /circ{gstartxy 
 3 copy pop 2 copy cos mul 3 1 roll sin mul
 rmoveto 0 0 5 2 roll arc xystroke}bind def
 /o /circ load def}%
\PSdict@@{%
 /circhar{gsave dup 3 gt{7 sub neg}if dup
 3 eq{pop dup 2 sqrt -2 div mul}{dup 1 eq{pop dup 2 sqrt 2 div mul}
 {0 eq{dup}{0}ifelse}ifelse}ifelse 
 0 translate 3 1 roll circ grestore}bind def
 /c /circhar load def}%
\PSdict@@{end end}%
\endgroup%
\endinput


==> xypspatt.tex <==
%% xypspatt.tex from $Id: xypspatt.doc,v 3.7 1999/02/16 15:12:50 krisrose Exp $
%%
%% Xy-pic ``PostScript pattern prolog''.
%% Copyright (c) 1995-1998 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1998 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\begingroup \xycatcodes \xyPSobeylines@@%
\PSdict@@{/XYdict where pop begin XYdict begin}%
\PSdict@@{/:patt
{XYddict begin 
14 dict begin
/BGnd exch def
/FGnd exch def
/PaintData exch def
/PatternType 1 def
/PaintType 1 def
/BBox[0 0 1 1]def
/TilingType 1 def
/XStep 1 def
/YStep 1 def
/PatternMtx[24 0 0 24 0 0]def
/PaintProc BGnd null ne
 {{begin BGnd aload pop setrgbcolor 0 0 1 1 rF
 FGnd aload pop setrgbcolor
 24 24 true PatternMtx PaintData imagemask end}}
 {{begin FGnd aload pop setrgbcolor
 24 24 true PatternMtx PaintData imagemask end}}
 ifelse def
 currentdict PatternMtx end
 gsave patangle xyland{180 add}if
 rotate macfreq patfreq div dup neg exch scale matrix currentmatrix 
 grestore gsave setmatrix /DeviceRGB setcolorspace makepattern grestore
 end}def}%
\PSdict@@{%
/rF{gsave
 newpath 4 2 roll moveto 1 index 0 rlineto 0 exch rlineto neg 0 rlineto
 fill grestore}bind def }%
\PSdict@@{%
 /setpatscreen{/pattstring exch store patfreq
 patangle xyport not{90 add}if
 {1 add 4 mul cvi pattstring exch get exch 1 add 4 mul cvi 7 sub 
 bitshift 1 and}setscreen}bind def 
 /setcolpattern{setpatscreen 64 div 1 exch sub currentrgbcolor
 1 1 3{pop 1 exch sub 3 index mul 1 exch sub 3 1 roll}for
 setrgbcolor pop}def
 /setgraypattern{setpatscreen 64 div setgray}def
 /macfreq 9.375 def /patangle 0 def /patfreq 12.5 def}%
\PSdict@@{/checkland{%
 /normland where{pop normland not}{false}ifelse
 /xyland exch def
 /por where{pop por}{/isls where{pop isls not /xyland true def}
 {/land where{pop land not}{true}
 ifelse}ifelse}ifelse /xyport exch def}def }%
\PSdict@@{%
 /setpatfreq{/patfreq exch def}def
 /setpatangle{/patangle exch def}def
 /setbackcolor{/backcolor exch def}def
 /setforecolor{/forecolor exch def}def
 [1 1 1] setbackcolor xycolarray setforecolor
 /bg /setbackcolor load def /fg /setforecolor load def 
 /pa /setpatangle load def /pq /setpatfreq load def }%
\PSdict@@{%
 /xypattern{checkland counttomark dup 0 eq{pop}
 {dup 1 eq{pop setpatscreen}
 {dup 2 eq{pop setcolpattern}
 {dup 3 eq{pop 
 /setcolorspace where {
 /.setcolorspace where{pop pop pop setcolpattern}
 {/.buildpattern where {pop
 forecolor backcolor :patt setpattern
 }{pop pop setcolpattern}ifelse}ifelse}
 {pop setcolpattern}ifelse}
 {5 eq{/setcolorspace where{
 /.setcolorspace where{pop pop pop pop pop setcolpattern}
 {/.buildpattern where {pop
 :patt setpattern
 }{pop pop pop pop setcolpattern}ifelse}ifelse}
 {pop pop pop setcolpattern}ifelse
 }{}ifelse}ifelse}ifelse}ifelse}ifelse cleartomark }def 
 /xysetpattern{/xypatt exch def}def
 /sp /xysetpattern load def }%
\PSdict@@{end end}%
\endgroup%
\endinput


==> xyrecat.tex <==
%% xyrecat.tex from $Id: xyrecat.doc,v 3.3 1996/12/19 03:31:56 krisrose Exp $
%%
%% Xy-pic ``Reset Category Codes'' utility.
%% Copyright (c) 1994-1996 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1996 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\xyuncatcodes
\xyrecat @ 64 \catcode 64 11
\xymakeADD@\addHASH@ # 35
\xymakeADD@\addDOLL@ $ 36
\xymakeADD@\addAND@ & 38
\xymakeADD@\addRQ@ ' 39
\xymakeADD@\addPLUS@ + 43
\xymakeADD@\addDASH@ - 45
\xymakeADD@\addDOT@ . 46
\xymakeADD@\addLT@ < 60
\xymakeADD@\addEQ@ = 61
\xymakeADD@\addGT@ > 62
\xymakeADD@\addLQ@ ` 96
\endinput


==> xyrotate.tex <==
%% xyrotate.tex from $Id: xyrotate.doc,v 3.3 1996/12/18 09:40:16 ross Exp $
%%
%% Xy-pic ``Rotate and Scale extension'' option.
%% Copyright (c) 1993-1996 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1996 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{rotate}{Rotate and Scale extension}{\stripRCS$Revision: 3.3 $}%
 {Ross Moore}{ross@mpce.mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xydef@\xyundefinedRotate@#1#2@@{%
 \xywarning@{The #1 #2 effect is not implemented with the current driver.}}%
\xydef@\NoResizing{\xyNoResizing@}
\xydef@\UseResizing{\xyUseResizing@}
\xydef@\xyNoResizing@{%
 \global\let\origxyrescale@=\xyrescale@
 \global\let\origxyrotSizeMod@=\xyrotateSizeMod@
 \global\let\xyNoResizing@=\xyNoResizing@@
 \global\let\xyUseResizing@=\xyUseResizing@@
 \xyNoResizing@@ }
\xydef@\xyNoResizing@@{%
 \global\let\xyrescale@=\xyignorescale@
 \global\let\xyrotateSizeMod@=\xyignoreSizeMod@
 }
\xylet@\xyUseResizing@=\relax
\xydef@\xyUseResizing@@{%
 \global\let\xyrescale@=\origxyrescale@
 \global\let\xyrotateSizeMod@=\origxyrotSizeMod@
 }
\xydefcsname@{shape [@...]}#1{\xyrotatechar@#1@@}%
\xydefcsname@{shape [<...]}#1{\xyshearchar@{#1}@@}%
\xydefcsname@{shape [*...]}#1{\xyscalechar@{#1}@@}%
\xydefcsname@{shape [left]}{\xyshape@left@}
\xydefcsname@{shape [right]}{\xyshape@right@}
\xydefcsname@{shape [flip]}{\xyshape@flip@}
\xydefcsname@{shape [halfsize]}{\xyshape@halfsize@}
\xydefcsname@{shape [dblsize]}{\xyshape@dblsize@}
\xydefcsname@{shape [vflip]}{\xyshape@vflip@}
\xydefcsname@{shape [hflip]}{\xyshape@hflip@}
\xydef@\preXYtransform@{}
\xydef@\postXYtransform@{}
\xywarnifdefined\preXYtransform@@
\xywarnifdefined\postXYtransform@@
 \gdef\preXYtransform@@{}
 \gdef\postXYtransform@@{}
\xydef@\xy@transform@{}
\xydef@\preShape@@{}
\xydef@\postShape@@{}
\xydef@\modXYtransform@{%
 \ifx\xy@transform@\empty
 \transformDrop@\transformConnect@\resetTransform@\fi
 \DN@##1{\expandafter\def\expandafter\tmp@\expandafter{##1}}%
 \expandafter\next@\expandafter{\preShape@@}%
 \DN@##1{\expandafter\gdef\expandafter\preXYtransform@@\expandafter{%
 \tmp@ ##1}}\expandafter\next@\expandafter{\preXYtransform@@}%
 \DN@##1{\expandafter\def\expandafter\tmp@\expandafter{##1}}%
 \expandafter\next@\expandafter{\postShape@@}%
 \DN@##1{\expandafter\gdef\expandafter\postXYtransform@@\expandafter{%
 \postXYtransform@@ ##1}}\expandafter\next@\expandafter{\tmp@}}%
\xydef@\transformDrop@{\let\xy@transform@=\relax
 \expandafter\def\expandafter\Drop@@\expandafter{%
 \expandafter\preXYtransform@\Drop@@\postXYtransform@}}
\xydef@\transformConnect@{\let\xy@transform@=\relax
 \expandafter\def\expandafter\Connect@@\expandafter{%
 \expandafter\preXYtransform@\Connect@@\postXYtransform@}}
\xydef@\resetTransform@{\gdef\preXYtransform@@{}\gdef\postXYtransform@@{}}
\xydef@\xynametransform@#1{%
 \DN@{\expandafter\gdef\expandafter#1\expandafter{\the\toks@}}\next@ }
\xydef@\xyscalechar@#1@@{\xyscalechars@#1,#1,@@}
\xydef@\xyscalechars@#1,#2,#3@@{%
 \DN@{\xyrescale@(#1,#2)}%
 \dimen@=#1\p@
 \ifdim\dimen@>\z@ \else \ifdim\dimen@<\z@ \else
 \DN@{\xywarning@{invalid scaling factors #1, #2}}%
 \fi\fi \dimen@=#2\p@
 \ifdim\dimen@>\z@ \else \ifdim\dimen@<\z@ \else
 \DN@{\xywarning@{invalid scaling factors #1, #2 }}%
 \fi\fi \next@ }
\xydef@\xyrescale@(#1,#2){%
 \setboxz@h{\xyscale@@{#1}{#2}%
 \dimen@=\ifx-#1\R@c\advance\dimen@-\R@c \dimen@=-\dimen@
 \else#1\L@c \advance\dimen@-\L@c\fi
 \kern\dimen@\boxz@\kern-\dimen@}%
 \R@c=\if-#1\L@c\else#1\R@c\fi
 \L@c=\if-#1\R@c\else#1\L@c\fi
 \U@c=\if-#2\D@c\else#2\U@c\fi
 \D@c=\if-#2\U@c\else#2\D@c\fi }
\xydef@\xyignorescale@(#1,#2){\xywarning@{Ignoring rescale: #1,#2}%
 \setboxz@h{\xyscale@@{#1}{#2}\boxz@}}%
\xydef@\xyshape@halfsize@{\xyrescale@(.5,.5)}
\xydef@\xyshape@dblsize@{\xyrescale@(2,2)}
\xydef@\xyshape@flip@{\xyrescale@(-1,-1)}
\xydef@\xyshape@vflip@{\xyrescale@(1,-1)}
\xydef@\xyshape@hflip@{\xyrescale@(-1,1)}
\xydef@\xyrotatechar@{\bgroup
 \afterDIRECTIONorEMPTY{\xyrotateSizeMod@}{\xyFN@\xySpecialRotate@i}}
\xydef@\xySpecialRotate@i{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\xySpecialRotate@i}%
 \else\ifx @\next \let\next@=\xyrotateSizeMod@
 \else\addEQ@\ifx \next
 \addEQ@\DN@##1@@{%
 \expandafter\xynametransform@\csname shape [##1]\endcsname\egroup}%
 \else\ifx !\next \DN@!{\egroup\getSpecialRotate@}%
 \else\ifx *\next \DN@*@@{\egroup\transformDrop@}%
 \else \DN@{\xySpecialRotate@@}%
 \fi\fi\fi\fi\fi \next@ }
\xydef@\getSpecialRotate@{\doSpecialRotate@@}
\xydef@\xyRotate@#1{\xyundefinedRotate@{rotate}{#1}@@}
\xydef@\xySpecialRotate@#1@@{\xyundefinedRotate@{rotate}{#1}@@\egroup}
\xydef@\doSpecialRotate@#1@@{\xyundefinedRotate@{special rotate}{#1}@@}
\xydef@\xyscale@#1#2{\xyundefinedRotate@{scale}{#1,#2}@@}
\xydef@\UnloadRotate@#1{%
 \ifx#1\relax\else\xyunload@{rotation extension}\fi
 \let\xyRotate@@=\xyRotate@
 \let\xySpecialRotate@@=\xySpecialRotate@
 \let\doSpecialRotate@@=\doSpecialRotate@
 \let\xyscale@@=\xyscale@ }
\UnloadRotate@\relax
\xyaddunsupport{rotate}{\UnloadRotate@\relax}
\xydef@\xyrotateSizeMod@ @@{%
 \L@p=\L@c \R@p=\R@c \U@p=\U@c \D@p=\D@c 
 \ifdim\cosDirection\p@>\z@ 
 \R@c=\cosDirection\R@p \L@c=\cosDirection\L@p
 \U@c=\cosDirection\U@p \D@c=\cosDirection\D@p 
 \else
 \R@c=\cosDirection\L@p \L@c=\cosDirection\R@p
 \U@c=\cosDirection\D@p \D@c=\cosDirection\U@p 
 \fi
 \advance\L@c \if-\sinDirection\D@p\else\sinDirection\U@p\fi
 \advance\R@c \if-\sinDirection\U@p\else\sinDirection\D@p\fi
 \advance\U@c \if-\sinDirection\L@p\else\sinDirection\R@p\fi
 \advance\D@c \if-\sinDirection\R@p\else\sinDirection\L@p\fi
 \dimen@ii=\L@c \advance\dimen@ii-\L@p
 \edef\tmp@{\egroup \L@c=\the\L@c \R@c=\the\R@c \U@c=\the\U@c \D@c=\the\D@c
 \dimen@ii=\the\dimen@ii \noexpand\setboxz@h\bgroup
 \noexpand\xyRotate@@{\the\Direction}}\tmp@
 \xydropRotated@ }
\xydef@\xydropRotated@@{%
 \kern\dimen@ii \boxz@ \kern-\dimen@ii \modXYtransform@ \egroup }
\xylet@\xydropRotated@=\xydropRotated@@
\xydef@\xyignoreSizeMod@ @@{\xywarning@{Ignoring rotation}}
\xydef@\xyshape@left@{\xyrotatechar@ v(0,1)@@}
\xydef@\xyshape@right@{\xyrotatechar@ v(0,-1)@@}
\xydef@\xyshearchar@{\xyundefinedRotate@{shearing}}
\xyendinput


==> xysmart.tex <==
%% xysmart.tex from $Id$
%%
%% Xy-pic ``Smart Path feature'' option.
%% Copyright (c) 1998 George C. Necula <necula@cs.cmu.edu>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1998 Kristoffer H. Rose <krisrose@ens-lyon.fr>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{smartpath}{Smart Path option}{\stripRCS$Revision: 0.0 $}%
 {George C. Necula}{necula@cs.cmu.edu}%
 {School of Computer Science,
 Carnegie Mellon University,
 5000 Forbes Avenue,
 Pittsburgh, PA 15213-3891, USA}
\xyrequire{arrow}\xycatcodes
\let\origPATHturn@=\PATHturn@
\def\PATHturn@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\PATHturn@}%
 \else\ifx s\next
 \let\origPATHturn@i=\PATHturn@i\let\PATHturn@i=\PATHsmartturn@i
 \let\origPATHturn@cir=\PATHturn@cir\let\PATHturn@cir=\PATHsmartturn@cir
 \DN@ s{\xyFN@\origPATHturn@}%
 \else
 \DN@{\origPATHturn@}%
 \fi\fi
 \next@}
\xydef@\PATHsmartturn@cir{%
 \edef\next@{{\CIRin@@}{\expandafter\noexpand\CIRorient@@}{\CIRout@@}}%
 \expandafter\PATHturn@i\next@}
\xydef@\PATHsmartturn@i#1#2#3{%
 \DN@##1{%
 \def\PATHinit@@{%
 \xy@@{%
 \def\sm@CIRin{#1}\def\sm@CIRout{#3}%
 \ifx\sm@CIRout\empty
 \let\sm@CIRout=\sm@CIRin
 \let\sm@CIRin=\PATHlastout@@
 \fi
 ##1\relax}%
 \xy@@{\enter@{\basefromthebase@}}%
 \xy@@{\sm@conn}%
 \xy@@{\X@p=\X@c \Y@p=\Y@c \czeroEdge@% Save the start of the segment
 \count@=\sm@CIRout\count@=\the\count@% Move forward a dash to
 \dimen@=\xydashl@ \ABfromdiag@ \advance\X@c\A@ \advance\Y@c\B@
 \edef\PATHpostpos@@{\X@c=\the\X@c \Y@c=\the\Y@c \noexpand\czeroEdge@
 \noexpand\PATHomitslide@@true}}%
 \xy@@{\leave@
 \edef\PATHlastout@@{\sm@CIRout}%
 \count@=\sm@CIRout \dimen@=\xydashl@ \Directionfromdiag@}}}%
 \expandafter\next@\expandafter{\the\toks@}\toks@={}%
 \let\PATHextra@@=\empty
 \def\PATHpost@@{\xy@@\PATHpostpos@@}%
 \let\PATHlabelsextra@@=\relax
 \let\PATHturn@i=\origPATHturn@i
 \let\PATHturn@cir=\origPATHturn@cir
 \xyFN@\PATHturn@ii}
\xydef@\sm@nil{}
\xydef@\sm@nnil{\sm@nil}
\xydef@\sm@maxcost{1000mm}%
\xydef@\sm@conn{
 \enter@{\cfromthec@ \DirectionfromtheDirection@}\cfromp@% Adjust p
 \count@=\sm@CIRin\count@=\the\count@
 \dimen@=\xydashl@ \ABfromdiag@ \advance\X@p\A@\advance\Y@p\B@
 \setupDirection@ \the\Edge@c\z@ \czeroEdge@
 \pfromc@
 \reverseDirection@
 \count@=\sm@CIRin\count@=\the\count@
 \dimen@=\xydashl@ \ABfromdiag@
 \edef\tmp@{\noexpand\dir\artail@@}\expandafter\sm@drop@\tmp@
 \X@c=\X@p\advance\X@c\A@ \Y@c=\Y@p\advance\Y@c\B@ \czeroEdge@
 \sm@stri
 \X@p=\X@c \Y@p=\Y@c
 \leave@
 \enter@{\pfromthep@ \DirectionfromtheDirection@}\pfromc@% Adjust c
 \count@=\sm@CIRout\count@=\the\count@
 \dimen@=\xydashl@ \ABfromdiag@ \advance\X@p-\A@\advance\Y@p-\B@
 \setupDirection@ \the\Edge@c\z@
 \advance\X@c-\A@\advance\Y@c-\B@% Leave room for a dash to terminate the seg
 \czeroEdge@
 \def\PATHlabelsnext@@{}%
 \leave@
 \R@=\turnradius@
 \cirrestrict@@%Adjust the radius to fit the circles
 \let\sm@circles=\sm@nil
 \edef\sm@bestcost{\sm@maxcost}%
 \sm@trycircles 1%Try counter clockwise first
 \sm@trycircles{-1}%
 \ifdim\sm@bestcost<\sm@maxcost
 \cfromp@
 \expandafter\sm@conndraw\sm@bestconn
 \else
 \xyerror@{Cannot draw the smart connector}{}%
 \fi
}
\xydef@\sm@trycircles#1{%
 \ifnum #1>0% Compute the opposite orientation
 \def\sm@CIRorienti{-1}%
 \else
 \def\sm@CIRorienti{1}%
 \fi
 \edef\tmp@{{{\sm@CIRin}{#1}{\sm@CIRout}}}%
 \expandafter\sm@trycirclelist\expandafter{\tmp@\sm@nil}%
 \count@@=\sm@CIRin\count@@=\the\count@@\count@=\count@@
 \sm@roundcount@{#1}%
 \edef\sm@savecount@{\the\count@}%
 \ifnum\the\count@=\the\count@@ \else
 \edef\tmp@{{{\sm@CIRin}{#1}{\the\count@}}%
 {{\the\count@}{\sm@CIRorienti}{\sm@CIRout}}}%
 \expandafter\sm@trycirclelist\expandafter{\tmp@\sm@nil}%
 \fi
 \count@=\sm@savecount@\count@=\the\count@
 \sm@advancecount@ 2{#1}\edef\sm@savecount@{\the\count@}%
 \edef\tmp@{{{\sm@CIRin}{#1}{\the\count@}}%
 {{\the\count@}{\sm@CIRorienti}{\sm@CIRout}}}%
 \expandafter\sm@trycirclelist\expandafter{\tmp@\sm@nil}%
 \count@=\sm@savecount@\count@=\the\count@
 \sm@advancecount@ 2{#1}\edef\sm@savecount@{\the\count@}%
 \edef\tmp@{{{\sm@CIRin}{#1}{\the\count@}}%
 {{\the\count@}{\sm@CIRorienti}{\sm@CIRout}}}%
 \expandafter\sm@trycirclelist\expandafter{\tmp@\sm@nil}%
 \count@=\sm@savecount@\count@=\the\count@
 \sm@advancecount@ 2{#1}\edef\sm@savecount@{\the\count@}%
 \edef\tmp@{{{\sm@CIRin}{#1}{\the\count@}}%
 {{\the\count@}{\sm@CIRorienti}{\sm@CIRout}}}%
 \expandafter\sm@trycirclelist\expandafter{\tmp@\sm@nil}%
}
\xydef@\sm@advancecount@#1#2{%
 \ifnum #2>0
 \edef\tmp@{#1}%
 \else
 \edef\tmp@{-#1}%
 \fi
 \advance\count@\tmp@\count@=\the\count@
 \ifnum\the\count@<0 \advance\count@ 8\fi
 \ifnum\the\count@>7 \advance\count@ -8\fi
 \count@=\the\count@
}
\xydef@\sm@roundcount@#1{%
 \ifcase\the\count@
 \advance\count@ #1\or
 \or \advance\count@ #1\or
 \or \advance\count@ #1\or
 \or \advance\count@ #1\fi
 \count@=\the\count@
 \ifnum\the\count@<0 \advance\count@ 8\fi
 \ifnum\the\count@>7 \advance\count@ -7\fi
 \count@=\the\count@
}
\newif\ifsm@firstseg
\newif\ifsm@acceptable
\xydef@\sm@trycirclelist#1{%
 \R@p=\z@\U@p=\R@p% Clear the deltas
 \def\sm@exthp{0}\def\sm@exthm{0}%
 \def\sm@extvp{0}\def\sm@extvm{0}%
 \def\sm@dxp{0pt}\def\sm@dxm{0pt}%
 \def\sm@dyp{0pt}\def\sm@dym{0pt}%
 \def\sm@segs{}%
 \sm@firstsegtrue
 \def\sm@connlen{0pt}%
 \let\sm@tryclcont=\sm@trycirclelist@i
 \sm@trycirclelist@i #1%Strip {} to expose the list elements
 \count@@=\sm@CIRout\count@@=\the\count@\count@=\the\count@
 \sm@roundcount@{1}%
 \ifnum\count@=\count@@
 \edef\sm@segs{\sm@segs{{\the\count@}{1}{\the\count@}}}%
 \fi
 \A@=\X@p\advance\A@\R@p\advance\A@ -\X@c\A@=-\A@
 \B@=\Y@p\advance\B@\U@p\advance\B@ -\Y@c\B@=-\B@
 \sm@acceptabletrue
 \ifdim\A@>0pt
 \ifnum\sm@exthp>0 \dimen@=\A@ \divide\dimen@\sm@exthp
 \edef\sm@dxp{\the\dimen@}%
 \else \sm@acceptablefalse\fi\fi
 \ifdim\A@<0pt
 \ifnum\sm@exthm>0 \dimen@=\A@ \divide\dimen@\sm@exthm
 \edef\sm@dxm{\the\dimen@}%
 \else \sm@acceptablefalse\fi
 \A@=-\A@%Make it positive
 \fi
 \ifdim\B@>0pt
 \ifnum\sm@extvp>0 \dimen@=\B@ \divide\dimen@\sm@extvp
 \edef\sm@dyp{\the\dimen@}%
 \else \sm@acceptablefalse\fi\fi
 \ifdim\B@<0pt
 \ifnum\sm@extvm>0 \dimen@=\B@ \divide\dimen@\sm@extvm
 \edef\sm@dym{\the\dimen@}%
 \else \sm@acceptablefalse\fi
 \B@=-\B@
 \fi
 \ifsm@acceptable
 \dimen@=\sm@connlen\advance\dimen@\A@\advance\dimen@\B@
 \ifdim\dimen@<\sm@bestcost
 \edef\sm@bestcost{\the\dimen@}%
 \edef\sm@bestconn{{\sm@dxp}{\sm@dxm}{\sm@dyp}{\sm@dym}{\sm@segs}}%
 \fi
 \fi
}
\xydef@\sm@showext#1{%
 \W@{#1\space hp=\sm@exthp,hm=\sm@exthm,vp=\sm@extvp
 ,vm=\sm@extvm,len=\sm@connlen}}
\xydef@\sm@trycirclelist@i#1{%
 \def\@tmp{#1}%
 \ifx \@tmp\sm@nnil \let\sm@tryclcont=\relax\else
 \expandafter\sm@tryclcar\@tmp \fi
 \sm@tryclcont}
\xydef@\sm@tryclcar#1#2#3{%
 \dimen@=\ifnum #2<0 -\fi\R@
 \count@=#1\count@=\the\count@ \ABfromdiag@
 \advance\R@p -\B@ \advance\U@p \A@
 \count@=#3\count@=\the\count@ \ABfromdiag@
 \advance\R@p \B@ \advance\U@p -\A@
 \sm@computeext{#1}{#2}{#3}%
}
\xydef@\sm@computeext#1#2#3{%
 \ifsm@firstseg
 \sm@accumext#1%
 \sm@firstsegfalse
 \fi
 \count@@=#1\count@@=\the\count@@\count@=\count@@
 \dimen@=\sm@connlen
 \sm@roundcount@{#2}%
 \ifnum \count@=\count@@
 \sm@advancecount@ 1{#2}%
 \advance\dimen@ 0.7854\R@% It was incremented with 1/8 circle
 \ifnum \count@=#3% Check if done
 \else
 \sm@advancecount@ 1{#2}%
 \advance\dimen@ 0.7854\R@% It was incremented with 1/8 circle
 \fi
 \else
 \advance\dimen@ 0.7854\R@% It was incremented with 1/8 circle
 \fi
 \edef\sm@connlen{\the\dimen@}%
 \sm@accumext{\the\count@}%
 \edef\sm@segs{\sm@segs{{#1}{#2}{\the\count@}}}%
 \ifnum\the\count@=#3 \else
 \edef\tmp@{{\the\count@}{#2}{#3}}%
 \expandafter\sm@computeext\tmp@
 \fi
}
\xydef@\sm@accumext#1{%
 \ifcase #1%
 \or \count@@=\sm@extvm\advance\count@@ by1%
 \edef\sm@extvm{\the\count@@}%
 \or\or \count@@=\sm@exthp\advance\count@@ by1%
 \edef\sm@exthp{\the\count@@}%
 \or\or \count@@=\sm@extvp\advance\count@@ by1%
 \edef\sm@extvp{\the\count@@}%
 \or\or \count@@=\sm@exthm\advance\count@@ by1%
 \edef\sm@exthm{\the\count@@}%
 \fi
}
\xydef@\sm@conndraw#1#2#3#4#5{%
 \def\sm@contlist{\sm@drawseglist}%
 \edef\sm@dxp{#1}%
 \edef\sm@dxm{#2}%
 \edef\sm@dyp{#3}%
 \edef\sm@dym{#4}%
 \sm@drawseglist #5\sm@nil}
\xydef@\sm@drawseglist#1{%
 \ifx #1\sm@nil \def\sm@contlist{}\else
 \sm@drawseg #1\fi
 \sm@contlist}
\xydef@\sm@drawseg#1#2#3{%
 \def\CIRin@@{#1}\def\CIRout@@{#3}%
 \sm@straight%See if a straight line is needed here. Insert it and
 \ifnum\CIRin@@=\CIRout@@ \else
 \count@=\CIRin@@
 \dimen@=\ifnum #2<0 -\fi\R@
 \ABfromdiag@
 \advance\X@c -\B@ \advance\Y@c \A@
 \ifnum #2>0 \def\CIRorient@@{\CIRacw@}%
 \else \def\CIRorient@@{\CIRcw@}\fi
 \drop@\literal@{\hbox\bgroup\cir@i}%
 \dimen@=\ifnum #2<0 -\fi\R@
 \count@=\CIRout@@\count@=\count@%Wierd. If I remove this last assignm
 \ABfromdiag@
 \advance\X@c\B@ \advance\Y@c-\A@
 \fi
}
\xydef@\sm@straight{%
 \U@c=\z@\D@c=\U@c\L@c=\U@c\R@c=\U@c
 \pfromc@
 \ifcase \CIRin@@ \or% 1 is V-
 \A@=\sm@dym\advance \Y@c\A@
 \or\or
 \A@=\sm@dxp\advance \X@c\A@
 \or\or
 \A@=\sm@dyp\advance \Y@c\A@
 \or\or
 \A@=\sm@dxm\advance \X@c\A@ \fi
 \ifdim\X@c=\X@p\ifdim\Y@c=\Y@p\else \sm@stri \fi\else \sm@stri \fi
}
\xydef@\sm@stri{%
 \edef\tmp@{\expandafter\noexpand\arstemprefix@@\arstem@@}%
 \expandafter\sm@connect@\tmp@}
\xydef@\sm@connect@#1#{%
 \DN@##1{\connect@{#1}{##1}}\next@}
\xydef@\sm@drop@#1#{%
 \DN@##1{\drop@{#1}{##1}}\next@}
\xydef@\smconn#1#2#3{%
 \edef\sm@CIRin{#1}\edef\sm@CIRout{#2}%
 \R@=#3\R@=\the\R@
 \sm@conn}
\xyendinput


==> xytextures.tex <==
%% xytextures.tex from $Id: xytextures.doc,v 3.3 1996/12/18 09:41:45 ross Exp $
%%
%% Xy-pic ``Textures'' driver interface option.
%% Copyright (c) 1995-1996 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1996 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{textures}{Textures driver}{\stripRCS$Revision: 3.3 $}%
 {Ross Moore}{ross@mpce.mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xydef@\Textures@@#1{\dvimessage@{Textures}{#1}}
\newdriver{%
 \xyaddsupport{color}\texturesColor@@
 \xyaddsupport{crayon}\texturesCrayon@@
 \xyaddsupport{ps}\texturesPS@@
 \xyaddsupport{rotate}\texturesRotate@@
 \xyaddsupport{line}\texturesLine@@
 \xyaddsupport{frame}\texturesFrames@@
 \xyaddsupport{tile}\texturesTiles@@
 \xyaddsupport{cmtip}\relax
}
\xydef@\TexturesColor@push#1{\special{color push}\special{color #1}}
\xydef@\TexturesColours@{\texturesPStypes@
 \let\xylocalColor@=\xystackcolor@
 \let\xycolor@push=\TexturesColor@push
 \def\xycolor@{\xycolor@@}%
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-c}{\xydrivernoload@{ps-c}}%
 \installPScolor@ }\else\DN@{}\fi \next@
 \ifx\xycolor@@\xyNoColor@ \let\xycolor@@=\xycolor@raw@@\fi
 \ifx\xycrayolaloaded\empty \DN@{\xystandardcolors@\texturesCrayon@@{}}%
 \else\let\next@=\xystandardcolors@ \fi \next@ 
 \let\xycolorwarning@=\relax \Textures@@{color}%
 \let\texturesColor@@=\relax
 \let\UnloadColor@@=\NoTexturesColor@
 }
\xydef@\texturesColor@@{\TexturesColours@}
\xydef@\NoTexturesColor@{%
 \let\xylocalColor@=\xyNoColor@@
 \let\xycolor@=\xyNoColor@
 \let\xycolorwarning@=\xycolorwarning@@
 \let\texturesColor@@=\TexturesColours@
 \let\UnloadColor@@=\UnloadColor@
 }
\xydef@\texturesCrayon@@{\texturesColor@@\texturesCrayon@}
\xydef@\texturesCrayon@{\installCrayolaColors@}%
\xydef@\texturesPS@@{\texturesPS@}
\xydef@\texturesPSunload@{\UnloadPS@
 \let\UnloadPS@@=\UnloadPS@
 \let\texturesPS@@=\texturesPS@ }
\xydef@\texturesPStypes@{%
 \xyinputorelse@{xyps-ps}{\xydrivernoload@{ps-ps}}%
 \ifx\PSspecial@@\TexturesSpecial@\else
 \let\PSspecial@@=\TexturesSpecial@
 \let\PSmacro@@=\TexturesMacro@
 \let\PSdict@@=\TexturesDict@
 \let\PSraw@@=\TexturesRaw@
 \let\PSinclude@@=\TexturesInclude@
 \let\PSspecialdict@@=\TexturesSpecialDict@
 \let\xyPSobeylines@@=\obeyTextureslines@
 \Textures@@{PostScript}%
 \fi \texturesCurrpt@ \XYpredict@ }
\xydef@\TexturesSpecial@#1{\firstPS@@\special{postscript #1}}
\xydef@\TexturesMacro@#1{\special{postscript {#1}xy}}
\xydef@\TexturesDict@#1{\special{prePostScript #1}}
\xydef@\TexturesSpecialDict@#1{\special{prePostScript #1}}
\xydef@\TexturesInclude@#1{\firstPS@@\special{prePostScriptfile #1}}
\xydef@\TexturesRaw@#1{\firstPS@@\special{rawpostscript #1}}%
{\catcode`\^^M=\active%
 \gdef\next{\catcode`\^^M=\active \let^^M=\par%
 \let\PSspecial@@=\TexturesDict@ \obeyspaces}}
\xylet@\obeyTextureslines@=\next
\xydef@\texturesCurrpt@{\let\xyPScurrpt@@=\texturesCurrpt@@}%
\xydef@\texturesCurrpt@@{\PSspecial@@{xyi}\PSraw@@{userdict begin xyx end}}
\xydef@\texturesPS@{\texturesPStypes@
 \let\texturesPS@@=\relax
 \let\UnloadPS@@=\texturesPSunload@ 
 \let\installxyps@@=\relax \installxyps@ }
\xydef@\texturesRotate@@{\texturesRotate@}
\xydef@\texturesRotate@{\texturesPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-r}{\xydrivernoload@{ps-r}}%
 \xyRotScale@@ \installPSrotscale@ }%
 \else\DN@{\xydriverfail@{rotations are}\UnloadRotate@\relax}\fi
 \next@}
\xydef@\texturesLine@@{\texturesLine@}
\xydef@\texturesLine@{\texturesPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-l}{\xydrivernoload@{ps-l}}%
 \installPSline@ }%
 \else\DN@{\xydriverfail@{line-widths are}\UnloadLine@\relax}\fi
 \next@ }
\xydef@\texturesFrames@@{\texturesFrames@}
\xydef@\texturesFrames@{\texturesPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-f}{\xydrivernoload@{ps-f}}%
 \installPSframes@ }%
 \else\DN@{\xydriverfail@{frames are}\UnloadPSFrames@\relax}\fi
 \next@ }
\xydef@\texturesTiles@@{\texturesTiles@}
\xydef@\texturesTiles@{\texturesPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-t}{\xydrivernoload@{ps-t}}%
 \installPSpatterns@ \xystandardpatterns@}%
 \else\DN@{\xydriverfail@{Patterns are}\UnloadPSpatterns@\relax}\fi
 \next@ }
\xyendinput


==> xytile.tex <==
%% xytile.tex from $Id: xytile.doc,v 3.4 1997/05/18 01:13:24 ross Exp $
%%
%% Xy-pic ``Pattern and Tile extension'' option.
%% Copyright (c) 1993-1997 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1997 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{tile}{Pattern and Tile extension}{\stripRCS$Revision: 3.4 $}%
 {Ross Moore}{ross@mpce.mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xydef@\xypatternwarning@@{\xypatternmessage@
 \gdef\xypatternwarning@{\xypatternmessage@
 \xywarning@{...no further pattern warnings will be given.}%
 \global\let\xypatternwarning@=\relax }}
\xylet@\xypatternwarning@=\xypatternwarning@@
\xydef@\xypatternmessage@{%
 \xywarning@{Current driver does not support patterns.}}%
\xydef@\newxypattern{\begingroup\xycatcodes\newxypattern@i}
\xydef@\newxypattern@i#1#2{\edef\next@{\endgroup
 \noexpand\newxyPattern{#1}{}{#2}{}}\next@}
\xydef@\newxyPattern#1#2#3#4{\newxypattern@{#1}{#2}{#3}{#4}{}}
\xydef@\newxypattern@#1#2#3#4#5{%
 \expandafter\let\expandafter\next@\csname shape [#1]\endcsname
 \ifx\next@\relax
 \DN@{#4}\ifx\next@\empty
 \DN@{#2}\ifx\next@\empty
 \DN@{\newxystyle{#1}{\xylocalpattern@{}{#3}\xypattern@{#3}}}%
 \else
 \DN@{\newxystyle{#1}{\xylocalpattern@{#2}{#3}\xypattern@{#2 #3}}}%
 \fi
 \else\DN@{#2#3}\ifx\next@\empty
 \DN@{\newxystyle{#1}{\xylocalpattern@{#4}{}\xypattern@{#4}}}%
 \else
 \DN@{\newxystyle{#1}{\xylocalpattern@{#2}{#3}\xypattern@{#4}}}%
 \fi\fi 
 \else \def\tmp@{\relax}\DNii@{#5}%
 \ifx\nextii@\tmp@
 \DN@{#4}\ifx\next@\empty
 \DN@{#2}\ifx\next@\empty
 \DN@{\newxystyle{#1}{\xylocalpattern@{}{#3}\xypattern@{#3}}}%
 \else
 \DN@{\newxystyle{#1}{\xylocalpattern@{#2}{#3}\xypattern@{#2 #3}}}%
 \fi
 \else
 \DN@{#2#3}\ifx\next@\empty
 \DN@{\newxystyle{#1}{\xylocalpattern@{#4}{}\xypattern@{#4}}}%
 \else
 \DN@{\newxystyle{#1}{\xylocalpattern@{#2}{#3}\xypattern@{#4}}}%
 \fi\fi 
 \else\DN@{}\fi\fi \next@\relax }
\xydef@\xyNopattern@#1{}
\xylet@\xypattern@@=\xyNopattern@
\xydef@\xyNopattern@@#1#2{\xypatternwarning@}
\xylet@\xypattern@=\xypattern@@
\xylet@\xylocalpattern@=\xyNopattern@@
\xydef@\Unloadpattern@{%
 \let\xylocalpattern@=\xyNopattern@@
 \let\xypattern@=\xyNopattern@
 \let\xypatternwarning@=\xypatternwarning@@ }
\Unloadpattern@
\xydef@\xystandardpatterns@{}%
\xynew@{read}{\xypatread@}
\xydef@\defaultpattfile@{}
\xydef@\xygetfilepatterns@#1{\DN@{#1}%
 \ifx\next@\empty
 \ifx\defaultpattfile@\empty \xywarning@{No pattern file specified.}%
 \else \DN@{\expandafter\openpattfile@\expandafter{\defaultpattfile@}}\fi
 \else \DN@{\openpattfile@{#1}}\fi \next@ }
\xydef@\openpattfile@#1{\openin\xypatread@=#1.xyp
 \ifeof\xypatread@\xywarning@{No patterns in file: #1.xyp}%
 \closein\xypatread@
 \else \expandafter \xyreadpatfile@ \fi }%
\xydef@\UsePatternFile#1{\def\defaultpattfile@{#1}}
\xydef@\LoadAllPatterns{\let\parsepattern@=\parsepattern@@
 \xygetfilepatterns@ }
\xydef@\LoadPattern#1{\let\parsepattern@=\filepattern@@
 \def\pattname@{#1}\xygetfilepatterns@}
\xydef@\AliasPattern#1#2{\let\parsepattern@=\aliaspattern@@
 \def\aliasname@{#1}\def\pattname@{#2}\xygetfilepatterns@}
\xydef@\xyreadpatfile@{%
 \loop@ \bgroup\xycatcodes
 \global\read\xypatread@ to\xypatline@
 \ifeof\xypatread@ \aftergroup\endpatread@
 \else\aftergroup\morepatread@\fi \edef\next@{%
 \egroup\noexpand\getxypattern@{\xypatline@!!!}\relax}\next@
 \repeat@ }
\xydef@\endpatread@{\closein\xypatread@\iffalse}
\xydef@\morepatread@{\iftrue}
\xydef@\getxypattern@#1{\def\next{#1}\getxypattern@@}
\xydef@\getxypattern@@{\DN@{!!!}\ifx\next\next@\DN@{}%
 \else\DN@{\expandafter\parsepattern@\next}\fi \next@ }
\xydef@\parsepattern@@#1 #2!#3\relax{\newxypattern{#1}{#2}}
\xydef@\filepattern@@#1 #2!#3\relax{\DN@{#1}%
 \ifx\next@\pattname@
 \DN@{\expandafter\foundpattern@\expandafter{\pattname@}{#2}}%
 \else\DN@{}\fi \next@ }
\xydef@\foundpattern@#1#2{\newxypattern{#1}{#2}\endpatread@\fi
 \expandafter\eat@}
\xydef@\aliaspattern@@#1 #2!#3\relax{\DN@{#1}%
 \ifx\next@\pattname@
 \DN@{\expandafter\foundpattern@\expandafter{\aliasname@}{#2}}%
 \else\DN@{}\fi \next@ }
\DN@{\xyaddunsupport{tile}\Unloadpattern@}%
\ifx\xyeverywithoption@tile@\undefined
\else\ifx\xyeverywithoption@tile@\empty
\else
 \DN@{\xysetup@@{\xywithoption{tile}{\xyeverywithoption@tile@\xydriversloaded@@}}}%
\fi\fi \next@
\xyendinput


==> xytips.tex <==
%% xytips.tex from $Id: xytips.doc,v 3.3 1996/12/19 04:12:13 krisrose Exp $
%%
%% Xy-pic ``More Tips'' extension.
%% Copyright (c) 1992-1996 Kristoffer H. Rose <kris@diku.dk>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% Copyright (c) 1991-1996 Kristoffer H. Rose <kris@diku.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{tips}{More Tips extension}{\stripRCS$Revision: 3.3 $}%
 {Kristoffer H.~Rose}{kris@diku.dk}%
 {BRICS/Computer Science, University of Aarhus, Ny Munkegade, building 540,
 DK--8000 Aarhus~C}
\xylet@\tip@xy=\tip@
\xylet@\atip@xy=\atip@
\xylet@\btip@xy=\btip@
\xylet@\Tip@xy=\Tip@
\xylet@\Ttip@xy=\Ttip@
\xylet@\tipjot@xy=\tipjot@
\xyfont@\xy@@atfont=xycmat10
\xyfont@\xy@@btfont=xycmbt10
\xydef@\tipfamily@@{cm}
\xydef@\tipsize@@{10}
\xydef@\SelectTips#1#2{%
 \DN@{#1}\ifx\next@\empty\else \def\tipfamily@@{#1}\fi
 \DN@{#2}\ifx\next@\empty\else \def\tipsize@@{#2}\fi
 \csname tipfamily \tipfamily@@\endcsname \ignorespaces}
\xydefcsname@{tipfamily cm}{\loadtipfonts@
 \let\tip@=\tip@cm \let\atip@=\atip@cm \let\btip@=\btip@cm
 \let\Tip@=\Tip@xy \let\Ttip@=\Ttip@xy \def\tipjot@{.2em}}
\xydef@\loadtipfonts@{\edef\next##1##2{##1=xy\tipfamily@@##2\tipsize@@}%
 \next{\font\xy@@atfont}{at}
 \next{\font\xy@@btfont}{bt}
}
\xydef@\tip@cm{\activatetips@ \tip@x\tip@@}
\xydef@\atip@cm{\activatetips@ \tip@x\atip@@}
\xydef@\btip@cm{\activatetips@ \tip@x\btip@@}
\xydef@\activatetips@{\let\xyatipfont=\xy@@atfont \let\xybtipfont=\xy@@btfont}
\xydefcsname@{tipfamily eu}{\loadtipfonts@
 \let\tip@=\tip@cm \let\atip@=\atip@cm \let\btip@=\btip@cm
 \let\Tip@=\Tip@eu \let\Ttip@=\Ttip@eu \def\tipjot@{.15em}}
\xydef@\Tip@eu{\kern1.5pt \vrule height1.5pt depth1.5pt width\z@
 \Tip@@eu \kern1.5pt \egroup
 \U@c=1.5pt \D@c=1.5pt \L@c=1.5pt \R@c=1.5pt \Edge@c={\circleEdge}%
 \Invisible@false \Hidden@false \def\Leftness@{.5}\def\Upness@{.5}%
 \def\Drop@@{\styledboxz@}\def\Connect@@{\straight@{\dottedSpread@\jot}}}
\xydef@\Tip@@eu{\count@=\DirectionChar
 \advance\count@-10 \ifnum\count@<\z@ \advance\count@128 \fi
 \xyatipfont\char\count@
 \advance\count@ 20 \ifnum127<\count@ \advance\count@-128 \fi
 \xybtipfont\char\count@}
\xydef@\Ttip@eu{\kern2.4pt \vrule height2.4pt depth2.4pt width\z@
 \Ttip@@eu \kern2.4pt \egroup
 \U@c=2.4pt \D@c=2.4pt \L@c=2.4pt \R@c=2.4pt \Edge@c={\circleEdge}%
 \Invisible@false \Hidden@false
 \def\Leftness@{.5}\def\Upness@{.5}%
 \def\Drop@@{\styledboxz@}\def\Connect@@{\straight@{\dottedSpread@\jot}}}
\xydef@\Ttip@@eu{%
 \setboxz@h\bgroup\reverseDirection@\line@ \wdz@=\z@ \ht\z@=\z@ \dp\z@=\z@
 \kern-\L@c \boxz@ \kern\L@c \Tip@@eu}
\xydef@\UseTips{\csname tipfamily \tipfamily@@\endcsname}
\xydef@\NoTips{\let\tip@=\tip@xy \let\atip@=\atip@xy \let\btip@=\btip@xy
 \let\Tip@=\Tip@xy \let\Ttip@=\Ttip@xy \let\tipjot@=\tipjot@xy}
\xyendinput


==> xytp-f.tex <==
%% xytp-f.tex from $Id: xytp-f.doc,v 3.3 1996/12/18 09:49:07 ross Exp $
%%
%% Xy-pic ``Frame extension'' TPIC backend support.
%% Copyright (c) 1995-1996 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1996 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xytpfloaded\empty \message{not reloaded}\endinput \fi
\let\xytpfloaded=\empty \xycatcodes
\xydef@\installTPICframes@{%
 \let\framed@body@@=\xyTPICframed@body@
 \let\circled@x@@=\xyTPICcircled@x@
 \let\ellipsed@x@@=\xyTPICellipsed@x@
 \installTPICfills@
 \xyuncatcodes}
\xydef@\UseTPICframes{\installTPICframes@}
\xydef@\NoTPICframes{\UnloadFrames@}
\xydef@\xyTPICframed@body@{\DN@{\framed@body@}%
 \ifdim\R@=\z@ 
 \ifx\framehfill\frm@solidh@@
 \DN@{\xyTPICframed@rect@i\xytpic@solid@@}%
 \else\ifx\framehfill\frm@dashh@@
 \DN@{\xyTPICframed@rect@i\xytpic@dashed@@}%
 \else\ifx\framehfill\frm@doth@@
 \DN@{\xyTPICframed@rect@i\xytpic@dotted@@}%
 \fi\fi\fi\fi \next@ }
\xydef@\xyTPICframed@rect@i#1{\vglue\U@c
 \hbox{\hglue\L@c\xyTPICrect@{#1}\hglue\R@c}\vglue\D@c}
\xydef@\xyTPICcircled@x@{\DN@{\xyTPICcircled@xx{}}%
 \ifx\framehfill\frm@doth@@ \DN@{\xyTPICdotcirc@}%
 \else\ifx\framehfill\frm@dashh@@\DN@{\xyTPICdashcirc@}%
 \fi\fi \next@ }
\xydef@\xyTPICcircled@xx#1{\vglue2\R@
 \hbox{\hglue2\R@\xyTPICfullcircle@#1\hglue2\R@}\vglue2\R@}
\xydef@\xyTPICdotcirc@{\let\zerodot=\framezerodot@@ 
 \L@=\R@ \circled@x@@ }
\xydef@\xyTPICdashcirc@{\L@=\R@ \circled@x@@ }
\xydef@\xyTPICdotellip@{\ellipsed@x@@ }
\xydef@\xyTPICdashellip@{\ellipsed@x@@ }
\xydef@\xyTPICellipsed@x@#1#2{\DN@{\xyTPICellipsed@xx{}}%
 \ifx\framehfill\frm@doth@@\DN@{\xyTPICdotellip@}%
 \else\ifx\framehfill\frm@dashh@@\DN@{\xyTPICdashellip@}%
 \fi\fi \next@{#1}{#2}}
\xydef@\xyTPICellipsed@xx#1#2#3{\vglue #3\vglue #3\relax
 \hbox{\L@c = #2\relax \R@c=\L@c \D@c = #3\relax \U@c=\D@c 
 \hglue#2\hglue#2\relax \R@=#2\relax \L@=#3\relax
 \xyTPICfullcircle@#1\hglue#2\hglue#2\relax}%
 \vglue #3\vglue #3\relax}
\xydef@\xyTPICrect@#1{\DNii@{\relax}\DN@{#1}\toks@={}%
 \ifx\next@\nextii@ \xytpic@pn0\relax\xytpic@bk
 \def\xytpic@style@@{\xytpic@fp}%
 \else\DNii@{\empty}%
 \ifx\next@\nextii@\def\xytpic@style@@{\xytpic@ip}\xytpic@bk
 \else\ifx\next@\empty\def\xytpic@style@@{\xytpic@ip}\xytpic@bk
 \else#1\fi\fi\fi 
 \xytpic@pt\R@c 
 \expandafter\addtotoks@\expandafter{\expandafter{\the\count@}}%
 \xytpic@pt\D@c 
 \expandafter\addtotoks@\expandafter{\expandafter{\the\count@}}%
 \xytpic@pt{\L@c}%
 \expandafter\addtotoks@\expandafter{\expandafter{\the\count@}}%
 \xytpic@pt{\U@c}%
 \expandafter\addtotoks@\expandafter{\expandafter{\the\count@}}%
 \expandafter\xyTPICrect@x\the\toks@
 \DNii@{\relax}\DN@{#1}\ifx\next@\nextii@
 \def\xytpic@style@@{\xytpic@fp}\expandafter\xyTPICrect@x\the\toks@\fi }
\xydef@\xyTPICrect@x#1#2#3#4{\xyTPIC@special{pa -#3 -#4}%
 \xyTPIC@special{pa -#3 #2}\xyTPIC@special{pa #1 #2}%
 \xyTPIC@special{pa #1 -#4}\xyTPIC@special{pa -#3 -#4}%
 \xytpic@style@@ }
\xydef@\xyTPICoval@#1{\DN@{#1}\DNii@{\relax}%
 \ifx\next@\nextii@ \DN@{\xyTPICfilledoval@\relax}%
 \else\DNii@{\empty}\ifx\next@\nextii@ \DN@{\xyTPICfilledoval@\empty}%
 \else\DN@{\xyTPICoval@i{#1}}\fi\fi \next@ }
\xylet@\xyTPICoval@i=\eat@
\xydef@\xyTPICfilledoval@#1{%
 {\advance\L@c-\R@ \advance\R@c-\R@ \xyTPICrect@{\empty}}%
 {\advance\U@c-\R@ \advance\D@c-\R@ \xyTPICrect@{\empty}}%
 \L@=\R@ \bgroup 
 \dimen@=-\U@c \advance\dimen@\R@ \xytpic@pt\dimen@ 
 \edef\tmp@{\the\count@}%
 \dimen@=-\L@c \advance\dimen@\R@ \xytpic@pt\dimen@
 \edef\tmp@{\noexpand\toks@={{\the\count@}{\tmp@}}}%
 \setTPICcircstyle@ \xyTPICcircle@{\tmp@}\egroup
 \bgroup 
 \dimen@=-\U@c \advance\dimen@\R@ \xytpic@pt\dimen@ 
 \edef\tmp@{\the\count@}%
 \dimen@=\R@c \advance\dimen@-\R@ \xytpic@pt\dimen@
 \edef\tmp@{\noexpand\toks@={{\the\count@}{\tmp@}}}%
 \setTPICcircstyle@ \xyTPICcircle@{\tmp@}\egroup
 \bgroup 
 \dimen@=\D@c \advance\dimen@-\R@ \xytpic@pt\dimen@ 
 \edef\tmp@{\the\count@}%
 \dimen@=-\L@c \advance\dimen@\R@ \xytpic@pt\dimen@
 \edef\tmp@{\noexpand\toks@={{\the\count@}{\tmp@}}}%
 \setTPICcircstyle@ \xyTPICcircle@{\tmp@}\egroup
 \bgroup 
 \dimen@=\D@c \advance\dimen@-\R@ \xytpic@pt\dimen@ 
 \edef\tmp@{\the\count@}%
 \dimen@=\R@c \advance\dimen@-\R@ \xytpic@pt\dimen@
 \edef\tmp@{\noexpand\toks@={{\the\count@}{\tmp@}}}%
 \setTPICcircstyle@ \xyTPICcircle@{\tmp@}\egroup
 \DN@{#1}\DNii@{\relax}\ifx\next@\nextii@
 \def\tmp@{{\xytpic@pn0\def\xytpic@style@@{\xytpic@fp}}}%
 \DN@{\expandafter\xyTPICoval@i\tmp@}%
 \else\DN@{}\fi \next@ }
\xydef@\setTPICcircstyle@{%
 \def\xytpic@circstyle@@{\xytpic@ia}\xytpic@bk}
\xydef@\xyTPICcircle@#1{\DNii@{\relax}%
 \DN@{#1}\toks@={00}\ifx\next@\nextii@ 
 \xytpic@pn0\relax\xytpic@bk \def\xytpic@circstyle@@{\xytpic@ar}%
 \else\DNii@{\empty}%
 \ifx\next@\nextii@ \setTPICcircstyle@
 \else\ifx\next@\empty \setTPICcircstyle@
 \else#1\fi\fi\fi 
 \xytpic@pt\R@ 
 \expandafter\addtotoks@\expandafter{\expandafter{\the\count@}}%
 \xytpic@pt\L@ 
 \expandafter\addtotoks@\expandafter{\expandafter{\the\count@}}%
 \expandafter\xytpic@circstyle@@\the\toks@ 0\twoPi@}
\xydef@\xyTPICellipse@{%
 \X@p=\R@c \advance\X@p-\L@c \divide\X@p\tw@ \R@=\R@c \advance\R@-\X@p
 \Y@p=\D@c \advance\Y@p-\U@c \divide\Y@p\tw@ \L@=\D@c \advance\L@-\Y@p
 \xyTPICcircle@}
\xydef@\xyTPICrect@Special#1#2#3#4{\TPICmacro@@{#1 fp}}
\xydef@\xyTPICdotrect@Special#1{\TPICmacro@@{#1 fp}}
\xydef@\xyTPICdashrect@Special#1{\TPICmacro@@{#1 fp}}
\xydef@\xyTPICcirc@Special#1{\TPICmacro@@{#1 ar}}
\xydef@\xyTPICdotcirc@Special#1{\TPICmacro@@{#1 ar}}
\xydef@\xyTPICdashcirc@Special#1{\TPICmacro@@{#1 ar}}
\xydef@\xyTPICfilledRegion#1#2{\vglue\U@c
 \hbox{\hglue\L@c#1#2\empty\hglue\R@c}\vglue\D@c}
\xydef@\filledRectangle@TPIC@@{%
 \ifdim\R@=\z@ \DN@{\xyTPICfilledRegion\xyTPICrect@}%
 \else \DN@{\xyTPICfilledRegion\xyTPICoval@}%
 \fi \next@ }
\xydef@\filledCircle@TPIC@@#1{{\R@c=\R@ \L@c=\R@ \U@c=\R@ \D@c=\R@
 \xyTPICfilledRegion\xyTPICcircle@#1{}}}
\xydef@\filledEllipse@TPIC@@{\xyTPICfilledRegion\xyTPICellipse@}
\xydef@\filledOval@TPIC@@{\xyTPICfilledRegion\xyTPICoval@}
\xydef@\installTPICfills@{%
 \let\filledRectangle@@=\filledRectangle@TPIC@@
 \let\filledOval@@=\filledOval@TPIC@@
 \let\filledCircle@@=\filledCircle@TPIC@@
 \let\filledEllipse@@=\filledEllipse@TPIC@@
}
\xydef@\xyTPICfillrect@Special#1#2{%
 \ifx#2\relax\TPICmacro@@{#1 fp}%
 \else\TPICmacro@@{#1 ip}\fi}
\xydef@\xyTPICfilloval@Special#1#2{%
 \ifx#2\relax\TPICmacro@@{#1 fp}%
 \else\TPICmacro@@{#1 ip}\fi}
\xydef@\xyTPICfillcirc@Special#1#2{%
 \ifx#2\relax\TPICmacro@@{#1 ar}%
 \else\TPICmacro@@{#1 ai}\fi}
\xydef@\xyTPICfillellipse@Special#1#2{%
 \ifx#2\relax\TPICmacro@@{#1 ar}%
 \else\TPICmacro@@{#1 ai}\fi}
\endinput


==> xytpic.tex <==
%% xytpic.tex from $Id: xytpic.doc,v 3.3 1996/12/18 09:50:38 ross Exp $
%%
%% Xy-pic ``tpic'' TPIC backend, for lines, curves and fills.
%% Copyright (c) 1995-1996 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1996 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{tpic}{TPIC backend}{\stripRCS$Revision: 3.3 $}%
 {Ross Moore}{ross@mpce.mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xynew@{if}\ifTPICspecials@
\xydef@\UseTPICspecials{\TPICspecials@true}
\xydef@\NoTPICspecials{\TPICspecials@false}
\xynew@{count}\xytpic@cnt
\xydef@\xytpic@max{300}
\xydef@\maxTPICpoints#1{\count@=#1 \relax
 \ifnum\count@>\tw@ \edef\xytpic@max{\the\count@}%
 \else\expandafter\xyTPICmaxwarning@\expandafter{\the\count@}\fi}
\xydef@\xyTPICmaxwarning@#1{max points must be at least 2, #1 invalid}
\xydef@\xytpic@style@@{\xytpic@fp}
\xydef@\xytpic@reset@{\gdef\xytpic@style@@{\xytpic@fp}%
 \global\xytpic@cnt=\z@ }
\xydef@\xytpic@set@#1{\xdef\xytpic@style@@{\noexpand#1}}
\xydef@\xytpic@pn#1{\xyTPIC@special{pn #1}}
\xydef@\xytpic@pa#1#2{\global\advance\xytpic@cnt\@ne\relax
 \ifnum\xytpic@cnt=\xytpic@max\relax \xyTPIC@special{pa #1 #2}%
 \kern-\X@c\raise-\Y@c\hbox{\xytpic@style@@}\kern\X@c
 \global\xytpic@cnt=\@ne \relax\fi \xyTPIC@special{pa #1 #2}}
\xydef@\xytpic@fp{\xyTPIC@special{fp}}
\xydef@\xytpic@ip{\xyTPIC@special{ip}}
\xydef@\xytpic@da#1{\xyTPIC@special{da #1}}
\xydef@\xytpic@dt#1{\xyTPIC@special{dt #1}}
\xydef@\xytpic@sp#1{\xyTPIC@special{sp #1}}
\xydef@\xytpic@ar#1#2#3#4#5#6{\xyTPIC@special{ar #1 #2 #3 #4 #5 #6}}
\xydef@\xytpic@ia#1#2#3#4#5#6{\xyTPIC@special{ia #1 #2 #3 #4 #5 #6}}
\xydef@\xytpic@sh#1{\xyTPIC@special{sh #1}}
\xydef@\xytpic@wh{\xyTPIC@special{sh 0}}
\xydef@\xytpic@bk{\xyTPIC@special{sh 1}}
\xydef@\xyTPIC@special#1{\special{#1}}
\xydef@\xyTPIC@noisy#1{\W@{TPIC: #1}\special{#1}}
\xydef@\NoisyTPIC{\let\xyTPIC@special=\xyTPIC@noisy}
\xydef@\xyTPICsplit@#1#2{\setboxz@h{#1\boxz@#2}}%
\xydef@\xytpic@pt#1{\dimen@=#1\divide\dimen@ by72
 \multiply\dimen@ by 1000 \advance\dimen@.5\p@
 \count@=\dimen@ \divide\count@\p@ }
\xydef@\xytpic@in#1{\dimen@=#1\divide\dimen@ by72
 \edef\next@{\expandafter\removePT@\the\dimen@}}%
\xydef@\xytpic@dot@@{\xytpic@pa00}
\xydef@\xytpic@width@{\xytpic@pt{\xylinethick@}%
 \expandafter\xytpic@pn\expandafter{\the\count@}}
\xydef@\xytpic@line{%
 \xytpic@dot@@ \xytpic@pt{-\d@X}\count@@=\count@
 \xytpic@pt\d@Y \edef\next@{{\the\count@@}{\the\count@}}%
 \expandafter\xytpic@pa\next@ \xytpic@style@@ \xytpic@reset@ }
\xydef@\xytpic@solid@@{\xytpic@set@\xytpic@fp}
\xydef@\xytpic@dashed@@{\xytpic@in\xydashl@ \xytpic@dad}
\xydef@\xytpic@dotted@@{\dimen@=.5\xydashl@ \xytpic@in\dimen@ \xytpic@dtd}
\xydef@\xytpic@dad{\expandafter\xytpic@set@\expandafter{%
 \expandafter\xytpic@da\expandafter{\next@}}}
\xydef@\xytpic@dtd{\expandafter\xytpic@set@\expandafter{%
 \expandafter\xytpic@dt\expandafter{\next@}}}
\xydef@\xytpic@polysolid@{\xytpic@set@\xytpic@fp}
\xydef@\xytpic@polydashed@#1{\count@=#1 \xytpic@dad}
\xydef@\xytpic@polydotted@#1{\count@=#1 \xytpic@dtd}
\xydef@\xytpic@postpoly@{\xytpic@style@@ \xytpic@reset@}
\xydef@\TPICalternative@#1#2{%
\expandafter\global\expandafter\let\csname origxy#2@\endcsname=#1%
 \xdef#1{\noexpand\ifTPICspecials@
 \noexpand\expandafter\expandafter\noexpand\csname xytpic@#2@\endcsname
 \noexpand\else
 \noexpand\expandafter\expandafter\noexpand\csname origxy#2@\endcsname
 \noexpand\fi}}%
\xydef@\setupxyTPIC@{\xywarning@{using TPIC specials}%
 \TPICalternative@{\solid@}{solid}%
 \TPICalternative@{\dash@}{dashed}%
 \TPICalternative@{\point@}{point}%
 \TPICalternative@{\circhar@@}{circhar}%
 \TPICalternative@{\splinesolid@}{splinesolid}%
 \xywithoption{frame}{\xyinputorelse@{xytp-f}{}\xyuncatcodes}%
 \let\setupxyTPIC@=\reloadxyTPIC@ 
 \activateTPIC@ }
\xydef@\xyunloadTPIC@{\xywarning@{TPIC specials turned off}%
 \xywithoption{curve}{\xysetup@@\uninstallTPICcurves@ }%
 \xywithoption{line}{\xysetup@@\uninstallTPICline@ }%
 \xywithoption{frame}{\xysetup@@\uninstallTPICframes@ }%
 \TPICspecials@false
 \let\setupxyTPIC@=\reloadxyTPIC@ }
\xydef@\activateTPIC@{%
 \xywithoption{line}{\xysetup@@\installTPICline@}%
 \xywithoption{curve}{\xysetup@@\installTPICcurves@}%
 \xywithoption{frame}{\xysetup@@\installTPICframes@}%
 \TPICspecials@true }
\xydef@\reloadxyTPIC@{\xywarning@{TPIC specials back on}\activateTPIC@ }
\xydef@\xytpic@solid@{%
 \ifInvisible@ \let\next@=\no@@
 \else \DN@{\xyTPICstraight@{\xytpic@solid@@ \xytpic@line}}\fi
 \next@ }
\xydef@\xytpic@dashed@{\line@
 \def\Connect@@{\xyTPICstraight@{\xytpic@dashed@@ \xytpic@line}}}
\xydef@\xytpic@point@{\xytpic@dot@@\xytpic@fp\egroup
 \Invisible@false \Hidden@false \def\Leftness@{.5}\def\Upness@{.5}\ctipEdge@
 \def\Drop@@{\styledboxz@}%
 \def\Connect@@{\xyTPICstraight@{\xytpic@dotted@@ \xytpic@line}}}
\xydef@\xyTPICstraight@#1{\setupDirection@
 \edef\Creset@@{\cfromthec@ \pfromthep@ \DirectionfromtheDirection@}%
 \DN@##1##2{\def\checkoverlap@@{%
 \ifdim##1\X@p>##1\X@c \let\next@=\relax \fi
 \ifdim##2\Y@p>##2\Y@c \let\next@=\relax \fi}}%
 \edef\nextii@{{\sd@X}{\sd@Y}}\expandafter\next@\nextii@
 \noCshavep@@ \edef\Cshavep@@{\pfromthep@ \noexpand\resetDirection@}%
 \noCshavec@@ \edef\Cshavec@@{\cfromthec@ \noexpand\resetDirection@}%
 \ifHidden@\else
 \ifdim\Y@c>\Y@max \Y@max=\Y@c \fi \ifdim\Y@p>\Y@max \Y@max=\Y@p \fi
 \ifdim\Y@c<\Y@min \Y@min=\Y@c \fi \ifdim\Y@p<\Y@min \Y@min=\Y@p \fi
 \ifdim\X@c>\X@max \X@max=\X@c \fi \ifdim\X@p>\X@max \X@max=\X@p \fi
 \ifdim\X@c<\X@min \X@min=\X@c \fi \ifdim\X@p<\X@min \X@min=\X@p \fi \fi
 \ifInvisible@\let\next@=\relax \else
 \DN@{\setboxz@h{\kern\X@c \raise\Y@c\hbox{#1}}%
 \ht\z@=\z@ \wd\z@=\z@ \dp\z@=\z@ {\Drop@@}}%
 \fi 
 \checkoverlap@@
 \ifdim\d@X=\z@ \ifdim\d@Y=\z@ \DN@{\relax}\fi\fi \next@
 \def\Cslidep@@{\noCslidep@@}\def\Cslidec@@{\noCslidec@@}%
 \def\Calong@@{\noCalong@@}\Creset@@ }
\xydef@\xytpic@splinesolid@{\xyTPICspline@\xytpic@fp }
\xydef@\xytpic@splinedashed@{\xytpic@in\xydashl@\expandafter\xyTPICspline@
 \expandafter{\expandafter\xytpic@da\expandafter{\next@}}}
\xydef@\xytpic@splinedotted@{\xytpic@in{.5\xydashl@}\expandafter\xyTPICspline@
 \expandafter{\expandafter\xytpic@dt\expandafter{\next@}}}
\xydef@\xyTPICspline@#1{\setbox\splinebox@=\copy\voidb@x
 \SloppyCurves
 \global\xytpic@cnt=\@ne \xytpic@set@{#1}%
 \def\splineextra@@{\xyTPICspline@dot}%
 \def\xycrvdrop@{ }\def\xycrvconn@{}\splineset@@ \xytpic@style@@}
\xydef@\xyTPICspline@dot{\xytpic@pt{\X@c}\count@@=\count@
 \xytpic@pt{-\Y@c}\edef\next@{{\the\count@@}{\the\count@}}%
 \expandafter\xytpic@pa\next@ }
\xydef@\xyTPIClinewidth@#1{\xytpic@pt{#1}\edef\next@{\the\count@}}
\xydef@\installTPICline@{%
 \let\xylinewidth@@=\xylinewidth@
 \let\xylineSpecial@@=\xytpic@pn
 \let\transxyline@@=\xyTPIClinewidth@ }
\xydef@\uninstallTPICline@{\UnloadLine@}%
\xydef@\xydoTPICcircle@#1{\DN@{#1}%
 \ifx\next@\empty\DN@{\xyTPICfullcircle@}%
 \else\expandafter\DNii@\expandafter{\addDASH@{}}%
 \ifx\next@\nextii@\DN@{\L@=\R@ \xyTPICfullcircle@}%
 \else\DN@{\dosolidcircle@{#1}}\fi\fi \next@ }
\xydef@\xyTPICfullcircle@{\xyTPICpartcircle@{00}0\twoPi@}%
\xydef@\xyTPICpartcircle@#1#2#3{%
 \xytpic@pt{\R@}\expandafter\DNii@\expandafter{\the\count@}%
 \xytpic@pt{\L@}\edef\next@{#1{\nextii@}{\the\count@}{#2}{#3}}%
 \expandafter\xytpic@ar\next@ }
\xydef@\qartPi@{0.7853981}
\xydef@\tartPi@{2.3561944}
\xydef@\xytpic@circhar@#1{\xytpic@width@\ifcase#1%
 \xytpic@pt{\R@}\edef\next@{{{\the\count@}0}}%
 \expandafter\xyTPICcirchar@i\next@{\tartPi@}{\fullPi@}\kern\partroottwo\R@
 \or
 \xytpic@pt{\halfroottwo\R@}\edef\next@{{{\the\count@}0}}%
 \expandafter\xyTPICcirchar@i\next@{\halfPi@}{\tartPi@}\kern\halfroottwo\R@
 \or
 \xytpic@pt{\z@}\edef\next@{{{\the\count@}0}}%
 \expandafter\xyTPICcirchar@i\next@{\qartPi@}{\halfPi@}\kern\halfroottwo\R@
 \or
 \xytpic@pt{-\halfroottwo\R@}\edef\next@{{{\the\count@}0}}%
 \expandafter\xyTPICcirchar@i\next@0{\qartPi@}\kern\partroottwo\R@
 \or
 \xytpic@pt{-\halfroottwo\R@}\edef\next@{{{\the\count@}0}}%
 \expandafter\xyTPICcirchar@i\next@{-\qartPi@}0\kern\partroottwo\R@
 \or
 \xytpic@pt{\z@}\edef\next@{{{\the\count@}0}}%
 \expandafter\xyTPICcirchar@i\next@{-\halfPi@}{-\qartPi@}\kern\halfroottwo\R@
 \or
 \xytpic@pt{\halfroottwo\R@}\edef\next@{{{\the\count@}0}}%
 \expandafter\xyTPICcirchar@i\next@{-\tartPi@}{-\halfPi@}\kern\halfroottwo\R@
 \or
 \xytpic@pt{\R@}\edef\next@{{{\the\count@}0}}%
 \expandafter\xyTPICcirchar@i\next@{-\fullPi@}{-\tartPi@}\kern\partroottwo\R@
 \fi}
\xydef@\xyTPICcirchar@i#1#2#3{\L@=\R@ \xyTPICpartcircle@{#1}{#2}{#3}}
\xydef@\xyTPIC@spline@ii@{\DN@{\xy@spline@ii}%
 \ifx\splineSTYLE@\empty\DN@{\xyTPICqspline@{0}}%
 \else\expandafter\DNii@\expandafter{\addDASH@{}}%
 \ifx\splineSTYLE@\nextii@\DN@{\xyTPICqspline@{0}}%
 \else\expandafter\DNii@\expandafter{\addDOT@{}}%
 \ifx\splineSTYLE@\nextii@\DN@{\xyTPICqspline@{-.5}}%
 \else\expandafter\expandafter\expandafter\DNii@\expandafter\expandafter
 \expandafter{\expandafter\addDASH@\addDASH@{}}%
 \ifx\splineSTYLE@\nextii@\DN@{\xyTPICqspline@{}}%
 \fi\fi\fi\fi
 \next@ }%
\xydef@\xyTPIC@accumulate{\xytpic@pt\X@c \count@@=\count@ 
 \xytpic@pt{-\Y@c}\edef\next@{{\the\count@@}{\the\count@}}%
 \expandafter\xytpic@pa\next@ }
\xydef@\xyTPICqspline@#1{\xytpic@width@
 \xytpic@in{#1\xydashl@}\expandafter\gdef\expandafter\xytpic@style@@
 \expandafter{\expandafter\xytpic@sp\expandafter{\next@}}%
 \save@ \cfromp@ \xyTPIC@accumulate
 \edef\smapp@@{\s@bot}\smapxy@i{\xyTPIC@accumulate}%
 \leave@ \xyTPIC@accumulate \xytpic@style@@ \xytpic@reset@
 \enter@{}\xy@spline@x }
\xydef@\installTPICcurves@{%
 \let\dosolidcircle@@=\xydoTPICcircle@
 \let\xy@spline@ii@@=\xyTPIC@spline@ii@
 }
\xydef@\uninstallTPICcurves@{%
 \let\dosolidcircle@@=\dosolidcircle@
 \let\xy@spline@ii@@=\xy@spline@ii }
 \xywithoption{frame}{\xyinputorelse@{xytp-f}{}}
\xydef@\uninstallTPICframes@{\UnloadFrames@}
\xyendinput


==> xyv2.tex <==
%% xyv2.tex from $Id: xyv2.doc,v 3.4 1997/05/18 01:14:25 krisrose Exp $
%%
%% Xy-pic ``Version 2 compatibility'' feature.
%% Copyright (c) 1993-1995 Kristoffer H. Rose <kris@diku.dk>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1995 Kristoffer H. Rose <kris@diku.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{v2}{Version 2 Compatibility}{\stripRCS$Revision: 3.4 $}%
 {Kristoffer H.~Rose}{krisrose@brics.dk}%
 {BRICS/Computer Science, University of Aarhus, Ny Munkegade, building 540,
 DK--8000 Aarhus~C}
\xylet@\XY=\Xy
\ifx\redefine\undefined \let\redefine=\def \fi
\ifx\define\undefined \let\define=\xydef@ \fi
\ifx\dsize\undefined \let\dsize=\displaystyle \fi
\ifx\tsize\undefined \let\dsize=\textstyle \fi
\ifx\ssize\undefined \let\ssize=\scriptstyle \fi
\ifx\sssize\undefined \let\sssize=\scriptscriptstyle \fi
\ifx\text\undefined
 \def\text{\relax\textC}%
 \xydef@\textC#1{\relax
 \ifmmode\mathchoice
 {\hbox{\the\textfont0\relax#1}}%
 {\hbox{\the\textfont0\relax#1}}%
 {\hbox{\the\scriptfont0\relax#1}}%
 {\hbox{\the\scriptscriptfont0\relax#1}}%
 \else{\relax#1}\fi}
\fi
\xydef@\Text{\relax\xyFN@\Text@}
\xydef@\TextC{\relax\textC}%
\xydef@\Text@{%
 \addLT@\ifx\next \addGT@{\addLT@\DN@##1}{\A@=##1\Text@i}%
 \else \DN@{\A@=\maxdimen \Text@i}\fi \next@}
\xydef@\Text@i#1{%
 \ifmmode \mathchoice
 {\expandafter\Text@ii\the\textfont0{#1}}%
 {\expandafter\Text@ii\the\textfont0{#1}}%
 {\expandafter\Text@ii\the\scriptfont0{#1}}%
 {\expandafter\Text@ii\the\scriptscriptfont0{#1}}%
 \else
 \leavevmode \expandafter\Text@ii\the\textfont0{#1}%
 \fi\ignorespaces}
\xydef@\Text@ii{\hbox\bgroup \txt@i}
\xylet@\cL=\L@c
\xylet@\cR=\R@c
\xylet@\cD=\D@c
\xylet@\cH=\U@c
\xylet@\Xc=\X@c
\xylet@\Yc=\Y@c
\xylet@\Uc=\U@c
\xylet@\Dc=\D@c
\xylet@\Lc=\L@c
\xylet@\Rc=\R@c
\xylet@\Xp=\X@p
\xylet@\Yp=\Y@p
\xylet@\Up=\U@p
\xylet@\Dp=\D@p
\xylet@\Lp=\L@p
\xylet@\Rp=\R@p
\xylet@\dX=\d@X
\xylet@\dY=\d@Y
\xylet@\Xorigin=\X@origin
\xylet@\Yorigin=\Y@origin
\xylet@\Xxbase =\X@xbase 
\xylet@\Yxbase =\Y@xbase 
\xylet@\Xybase =\X@ybase 
\xylet@\Yybase =\Y@ybase 
\xylet@\Xmin=\X@min
\xylet@\Ymin=\Y@min
\xylet@\Xmax=\X@max
\xylet@\Ymax=\Y@max
\xydef@\go{\aftergo{}}
\xydef@\aftergo#1{\xy@\aftergo{\enter@\pfromthec@}\afterPOS{\xy@@\leave@#1}}
\xydef@\merge{\POS.p\relax}
\xydef@\swap{\xy@\swap\swap@}
\xydef@\Drop{\expandafter\drop\entrymodifiers@}
\xydef@\none{\xy@\none{}\ignorespaces}
\xydef@\solid{\connect h\dir{-}}
\xydef@\Solid{\connect h\dir2{-}}
\xydef@\Ssolid{\connect h\dir3{-}}
\xydef@\dashed{\connect h\dir{--}}
\xydef@\Dashed{\connect h\dir2{--}}
\xydef@\Ddashed{\connect h\dir3{--}}
\xydef@\dotted{\connect h\dir{.}}
\xydef@\Dotted{\connect h\dir2{.}}
\xydef@\Ddotted{\connect h\dir3{.}}
\xydef@\dottedwith#1{\connect h{#1}}
\xydef@\notip{\dir{}}
\xydef@\stop{\dir{|}}
\xydef@\astop{\dir^{|}}
\xydef@\bstop{\dir_{|}}
\xydef@\tip{\dir{>}}
\xydef@\atip{\dir^{>}}
\xydef@\btip{\dir_{>}}
\xydef@\Tip{\dir2{>}}
\xywarnifdefined\aTip
\xywarnifdefined\bTip
{\xyuncatcodes
 \gdef\aTip{\object=<5pt>:(32,-1)\dir^{>}}
 \gdef\bTip{\object=<5pt>:(32,+1)\dir_{>}}}
\xydef@\Ttip{\dir3{>}}
\xydef@\ahook{\dir^{(}}
\xydef@\bhook{\dir_{(}}
\xydef@\aturn{\dir^{'}}
\xydef@\bturn{\dir_{'}}
\xydef@\rotate{\hbox\bgroup
 \DN@{\ifx (\next
 \DN@(####1){\rotate@ii{####1}}%
 \else \DN@{\rotate@i}\fi\next@}\xyFN@\next@}
\xydef@\rotate@i#1{\reverseDirection@ #1\OBJECT@x}
\xydef@\rotate@ii#1#2{\dimen@=#1\p@
 \ifdim \dimen@=-\p@ \aboveDirection@\xydashl@
 \else\ifdim\dimen@= \p@ \belowDirection@\xydashl@
 \else\ifdim\dimen@<-1.5\p@ \advance\dimen@-2\p@
 \edef\next@{\expandafter\removePT@\the\dimen@}\vDirection@(-1,\next@){1pc}%
 \else\ifdim\dimen@<-.5\p@ \vDirection@(#1,-1){1pc}%
 \else\ifdim\dimen@< .5\p@ \vDirection@( 1,#1){1pc}%
 \else\ifdim\dimen@<1.5\p@ \vDirection@(#1, 1){1pc}%
 \else \dimen@=-\dimen@ \advance\dimen@2\p@
 \edef\next@{\expandafter\removePT@\the\dimen@}\vDirection@(-1,\next@){1pc}%
 \fi\fi\fi\fi\fi\fi
 #2\OBJECT@x}
\xydef@\squash#1{%
 \ifmmode\setboxz@h{\m@th${\mathstrut}#1{\mathstrut}$}\else\setboxz@h{#1}\fi
 \setboxz@h{\kern-.5\wdz@ \dimen@=.5\ht\z@ \advance\dimen@-.5\dp\z@
 \lower\dimen@\boxz@}%
 \wdz@=\z@ \ht\z@=\z@ \dp\z@=\z@ \boxz@}
\xydef@\grow{%
 \DN@{\ifx <\next \DN@<####1>{\dimen@=####1\grow@\empty}%
 \else \DN@{\dimen@=2\p@ \grow@\empty}\fi\next@}\xyFN@\next@}
\xydef@\grow@#1#{\grow@@{#1}}
\xydef@\grow@@#1#2{\relax
 \ifmmode \setboxz@h{\kern\dimen@ \m@th$#2$\kern\dimen@}%
 \else \setboxz@h{\kern\dimen@ {#2}\kern\dimen@}\fi
 \dimen@ii=\ht\z@ \advance\dimen@ii\dimen@ \ht\z@=\dimen@ii
 \dimen@ii=\dp\z@ \advance\dimen@ii\dimen@ \dp\z@=\dimen@ii \boxz@}
\xydef@\squarify{\addEQ@{\addPLUS@\object}}
\xydef@\qc{\corn@@}
\xyrequire{frame}\xycatcodes
\xydef@\framed{\relax\convertframed{-}}
\xydef@\Framed{\relax\convertframed{=}}
\xydef@\circled{\relax\convertframed{o}}
\xydef@\Circled{\relax\convertframed{oo}}
\xydef@\convertframed#1{\DNii@##1@{\drop\frm##1{#1}}\xyFN@\convertframed@i}
\xydef@\convertframed@i{%
 \addLT@\ifx \next
 \addGT@{\addLT@\DN@##1}{\addGT@{\addLT@{\nextii@}##1}@}%
 \else \DN@{\nextii@ @}\fi \next@}
\xydef@\dotframed{\relax\drop\frm{.}}
\xydef@\dashframed{\relax\drop\frm{--}}
\xydef@\rounddashframed{\relax\drop\frm{o-}}
\xydef@\filled{\DN@{%
 \addLT@\ifx \next
 \addGT@{\addLT@\DN@####1}{\xy@@{\frame@fill@@{####1}}}%
 \else \DN@{\xy@@{\frame@fill@@\z@}}%
 \fi\next@}\xyFN@\next@}
\xydef@\Filled{\DN@{%
 \addLT@\ifx \next
 \addGT@{\addLT@\DN@####1}{\xy@@{\frame@emph@@{####1}}}%
 \else \DN@{\xy@@{\frame@emph@@\z@}}%
 \fi\next@}\xyFN@\next@}
\xyrequire{matrix}\xycatcodes
\xydef@\diagram#1\enddiagram{\relax\diagram@\diagram@@{#1}}
\xydef@\diagram@{\relax
 \ifmmode \DN@##1##2{\vcenter{\oldxymatrix@true \xy##1{\xymatrix{##2}}\endxy}}%
 \else\DN@##1##2{{\oldxymatrix@true \xy/u.8ex/##1{\xymatrix{##2}}\endxy}}%
 \fi \next@}
\xydef@\LaTeXdiagrams{\def\diagram{\ltxdiagram@\diagram@@}%
 \def\diagramnocompile{\ltxdiagram@\literal@}%
 \def\diagramcompileto##1{\ltxdiagram@{\NoCompileMatrices\xycompileto{##1}}}}
\xydef@\ltxdiagram@#1#2\end#3{\relax
 \DN@{#3}\DNii@{diagram}\ifx\next@\nextii@\diagram@{#1}{#2}\end{diagram}%
 \else\xyerr@{Put \string{\string} around \string\begin...\string\end\space
 within diagrams}\fi}
\xylet@\diagram@@=\literal@
\xydef@\NoisyDiagrams{}
\xydef@\spreaddiagramrows#1{\addPLUS@\xymatrixrowsep{#1}}
\xydef@\spreaddiagramcolumns#1{\addPLUS@\xymatrixcolsep{#1}}
\xyrequire{arrow}\xycatcodes
\xylet@\arrow=\ar
{\xyuncatcodes
 \gdef\morPHISM#1#2#3{\PATH~={\oldconnect{#1}}~<{|<*{#3}}~>{|>*{#2}}}}
\xydef@\morphism{\relax\morPHISM}
\xylet@\connect@iii=\connect
\xydef@\oldconnect#1{%
 \let\PATHlabelabove@@=\PATHlabelabove@
 \let\PATHlabelbelow@@=\PATHlabelbelow@
 \let\connect=\preconnect#1\let\connect=\connect@iii}
\xydef@\definemorphism#1#2#3#4{%
 \xydefcsname@{x#1}{\morphism{#2}{#3}{#4}}%
 \xydefcsname@{u#1}{\morphism{#2}{#3}{#4}[u]}%
 \xydefcsname@{d#1}{\morphism{#2}{#3}{#4}[d]}%
 \xydefcsname@{l#1}{\morphism{#2}{#3}{#4}[l]}%
 \xydefcsname@{r#1}{\morphism{#2}{#3}{#4}[r]}%
 \xydefcsname@{uu#1}{\morphism{#2}{#3}{#4}[uu]}%
 \xydefcsname@{dd#1}{\morphism{#2}{#3}{#4}[dd]}%
 \xydefcsname@{ll#1}{\morphism{#2}{#3}{#4}[ll]}%
 \xydefcsname@{rr#1}{\morphism{#2}{#3}{#4}[rr]}%
 \xydefcsname@{ur#1}{\morphism{#2}{#3}{#4}[ur]}%
 \xydefcsname@{ul#1}{\morphism{#2}{#3}{#4}[ul]}%
 \xydefcsname@{dr#1}{\morphism{#2}{#3}{#4}[dr]}%
 \xydefcsname@{dl#1}{\morphism{#2}{#3}{#4}[dl]}%
 \xydefcsname@{uul#1}{\morphism{#2}{#3}{#4}[uul]}%
 \xydefcsname@{uur#1}{\morphism{#2}{#3}{#4}[uur]}%
 \xydefcsname@{ull#1}{\morphism{#2}{#3}{#4}[ull]}%
 \xydefcsname@{urr#1}{\morphism{#2}{#3}{#4}[urr]}%
 \xydefcsname@{ddl#1}{\morphism{#2}{#3}{#4}[ddl]}%
 \xydefcsname@{ddr#1}{\morphism{#2}{#3}{#4}[ddr]}%
 \xydefcsname@{dll#1}{\morphism{#2}{#3}{#4}[dll]}%
 \xydefcsname@{drr#1}{\morphism{#2}{#3}{#4}[drr]}%
 \xydefcsname@{uull#1}{\morphism{#2}{#3}{#4}[uull]}%
 \xydefcsname@{uurr#1}{\morphism{#2}{#3}{#4}[uurr]}%
 \xydefcsname@{ddll#1}{\morphism{#2}{#3}{#4}[ddll]}%
 \xydefcsname@{ddrr#1}{\morphism{#2}{#3}{#4}[ddrr]}}
\definemorphism{to}\solid\tip\notip
\definemorphism{line}\solid\notip\notip
\definemorphism{dashed}\dashed\notip\notip
\definemorphism{dotted}\dotted\notip\notip
\definemorphism{double}\Solid\notip\notip
\xywarnifdefined\xyviitoi
\xywarnifdefined\xyviitoii
\xydef@\XXtoY@#1#2#3#4#5{\save;[#3]\relax
 \xy@@{%
 \dimen@=\turnradius@ \ifdim#1<#2\relax \dimen@ii=#2\else\dimen@ii=#1\fi
 \advance\dimen@\ifdim\dimen@>\dimen@ii +\dimen@\else +\dimen@ii\fi
 \edef\xyviitoi{\the\dimen@}\leave@}%
 \xto ~{[#3]} `#4[#3]#5/#4\xyviitoi/ `[#3]}
\xydef@\toXY@#1#2#3#4#5{\xy@@{\idfromc@{@}%
 \dimen@=\turnradius@ \dimen@ii=#1\relax
 \advance\dimen@\ifdim\dimen@>\dimen@ii +\dimen@\else +\dimen@ii\fi
 \edef\xyviitoi{\the\dimen@}%
 \dimen@=\turnradius@ \dimen@ii=#2\relax
 \advance\dimen@\ifdim\dimen@>\dimen@ii +\dimen@\else +\dimen@ii\fi
 \edef\xyviitoii{\the\dimen@}}%
 \morphism\solid{\object #4:(-1,0)\dir{>}}\notip
 ~{`"@" "@"} `#3"@"#5/#3\xyviitoi/#5/#4\p@/ `"@"#5/#4\xyviitoii/}
\xyuncatcodes \catcode64=11
\xydef@\lltod{\XXtoY@\D@c\D@p{ll}{d}+}
\xydef@\lltou{\XXtoY@\U@c\U@p{ll}{u}+}
\xydef@\rrtod{\XXtoY@\D@c\D@p{rr}{d}+}
\xydef@\rrtou{\XXtoY@\U@c\U@p{rr}{u}+}
\xydef@\ddtol{\XXtoY@\L@c\L@p{dd}{l}+}
\xydef@\ddtor{\XXtoY@\R@c\R@p{dd}{r}+}
\xydef@\uutol{\XXtoY@\L@c\L@p{uu}{l}+}
\xydef@\uutor{\XXtoY@\R@c\R@p{uu}{r}+}
\xydef@\told{\toXY@\L@c\D@c{l}{d}+}
\xydef@\tolu{\toXY@\L@c\U@c{l}{u}+}
\xydef@\tord{\toXY@\R@c\D@c{r}{d}+}
\xydef@\toru{\toXY@\R@c\U@c{r}{u}+}
\xydef@\todl{\toXY@\D@c\L@c{d}{l}+}
\xydef@\todr{\toXY@\D@c\R@c{d}{r}+}
\xydef@\toul{\toXY@\U@c\L@c{u}{l}+}
\xydef@\tour{\toXY@\U@c\R@c{u}{r}+}
\xycatcodes
\xydef@\TurnRadius{\addEQ@\turnradius}
\xydef@\diagramcompileto#1#2\enddiagram{\relax
 \diagram@{\NoCompileMatrices\xycompileto{#1}}{#2}}
\xydef@\diagramnocompile#1\enddiagram{\relax\diagram@\literal@{#1}}
\xydef@\CompileAllDiagrams#1{\CompilePrefix{#1}\CompileMatrices}
\xydef@\NoCompileAllDiagrams{\NoCompileMatrices}
\xydef@\ReCompileAllDiagrams{\CompileMatrices}
\xyendinput


==> xyweb.tex <==
%% xyweb.tex from $Id: xyweb.doc,v 3.3 1996/12/18 09:52:11 ross Exp $
%%
%% Xy-pic ``Lattice and web'' feature.
%% Copyright (c) 1994-1996 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1996 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{web}{Lattice and web feature}{\stripRCS$Revision: 3.3 $}%
 {Ross Moore}{ross@mpce.mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\message{lattices,}
\xynew@{count}\lattice@A
\xynew@{count}\lattice@B
\xydef@\latticeA{\lattice@A}
\xydef@\latticeB{\lattice@B}
\xydef@\xylattice#1#2#3#4{\xy@{LATTICE}{\xylattice@{#1}{#2}{#3}{#4}}}%
\xydef@\xylattice@#1#2#3#4{%
 \lattice@A=#1\relax
 \loop \bgroup\lattice@B=#3\relax
 \innerlatticeloop@{#4}%
 \edef\tmp@{\egroup
 \X@min=\the\X@min \X@max=\the\X@max
 \Y@min=\the\Y@min \Y@max=\the\Y@max 
 }\tmp@ \ifnum\lattice@A<#2\relax \advance\lattice@A\@ne
 \repeat }
\xydef@\innerlatticeloop@#1{%
 \loop \enter@{\cfromthec@}\enter@{\cplusthec@}%
 \vfromcartesian@@ \the\lattice@A,\the\lattice@B @%
 \edef\latticeX{\expandafter\removePT@\the\X@c}%
 \edef\latticeY{\expandafter\removePT@\the\Y@c}%
 \leave@ \latticebody \leave@
 \ifnum\lattice@B<#1\relax \advance\lattice@B\@ne
 \repeat }
\xydef@\croplattice#1#2#3#4#5#6#7#8{\xy@{LATTICE}%
 {\xycroplattice@{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}}}%
\xydef@\xycroplattice@#1#2#3#4#5#6#7#8{%
 \enter@{\X@min=\the\X@min \X@max=\the\X@max 
 \Y@min=\the\Y@min \Y@max=\the\Y@max}%
 \enter@{\cfromthec@}\enter@{\cplusthec@}%
 \vfromcartesian@@ #5,0 @\leave@ \X@min=\X@c \leave@
 \enter@{\cfromthec@}\enter@{\cplusthec@}%
 \vfromcartesian@@ #6,0 @\leave@ \X@max=\X@c \leave@
 \enter@{\cfromthec@}\enter@{\cplusthec@}%
 \vfromcartesian@@ 0,#7 @\leave@ \Y@min=\Y@c \leave@
 \enter@{\cfromthec@}\enter@{\cplusthec@}%
 \vfromcartesian@@ 0,#8 @\leave@ \Y@max=\Y@c \leave@
 \lattice@A=#1\relax
 \loop
 \bgroup\lattice@B=#3\relax
 \enter@{\cfromthec@}\innercroplatticeloop@{#4}\leave@
 \egroup
 \ifnum\lattice@A<#2\relax \advance\lattice@A\@ne
 \repeat \mergecropextents@ }
\xydef@\innercroplatticeloop@#1{%
 \loop 
 \enter@{\cfromthec@}\enter@{\cplusthec@}%
 \vfromcartesian@@ \the\lattice@A,\the\lattice@B @%
 \edef\latticeX{\expandafter\removePT@\the\X@c}%
 \edef\latticeY{\expandafter\removePT@\the\Y@c}%
 \leave@ \DN@{\latticebody}%
 \ifdim\X@c<\X@min\DN@{}%
 \else\ifdim\X@c>\X@max\DN@{}%
 \else\ifdim\Y@c<\Y@min\DN@{}%
 \else\ifdim\Y@c>\Y@max\DN@{}%
 \fi\fi\fi\fi \next@ \leave@
 \ifnum\lattice@B<#1\relax \advance\lattice@B\@ne
 \repeat }
\xydef@\mergecropextents@{%
 \edef\tmp@{%
 \noexpand\ifdim\X@min>\the\X@min \X@min=\the\X@min\noexpand\fi
 \noexpand\ifdim\X@max<\the\X@max \X@max=\the\X@max\noexpand\fi
 \noexpand\ifdim\Y@min>\the\Y@min \Y@min=\the\Y@min\noexpand\fi
 \noexpand\ifdim\Y@max<\the\Y@max \Y@max=\the\Y@max\noexpand\fi}%
 \leave@ \tmp@ }
\xydef@\deflatticebody@{\def\latticebody{\drop{\bullet}}}
\xydef@\defaultlatticebody{\deflatticebody@}
\deflatticebody@
\xyendinput


==> xyxdvi.tex <==
%% xyxdvi.tex from $Id: xyxdvi.doc,v 3.3 1996/12/18 09:53:22 ross Exp $
%%
%% Xy-pic ``xdvi-driver'' option.
%% Copyright (c) 1995-1996 Ross Moore <ross@mpce.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1996 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, write to the Free Software Foundation, Inc.,
%% 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{xdvi}{XDVI driver}{\stripRCS$Revision: 3.3 $}%
 {Ross Moore}{ross@mpce.mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xydef@\xdvi@@#1{\dvimessage@{xdvi}{#1}}
\newdriver{%
 \xyaddsupport{color}\xdviColor@@
 \xyaddsupport{crayon}\xdviCrayola@@
 \xyaddsupport{ps}\xdviPS@@
 \xyaddsupport{rotate}\xdviRotate@@
 \xyaddsupport{line}\xdviLine@@
 \xyaddsupport{frame}\xdviFrames@@
 \xyaddsupport{tile}\xdviTiles@@
 \xyaddsupport{tpic}\xdviTPIC@ 
}
\xydef@\xdvi@Color@{\xdviPStypes@ 
 \let\xylocalColor@=\xyNoColor@@
 \def\xycolor@{\xycolor@@}\let\xycolorwarning@=\relax
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-c}{\xydrivernoload@{ps-c}}\installPScolor@ }%
 \else\DN@{}\fi \next@ 
 \ifx\xycolor@@\xyNoColor@ \let\xycolor@@=\xycolor@raw@@\fi
 \ifx\xycrayolaloaded\empty \DN@{\xystandardcolors@\xdviCrayola@{}}%
 \else \DN@{\xystandardcolors@}\fi \next@
 \let\xdviColor@@=\relax
 \let\UnloadColor@@=\NoXDVIcolor@
 }%
\xydef@\xdviColor@@{\xdvi@Color@}
\xydef@\NoXDVIcolor@{%
 \def\xycolor@{\xycolor@@}%
 \let\xycolor@@=\xyNoColor@
 \let\xylocalColor@=\xyNoColor@@
 \let\xycolorwarning@=\xycolorwarning@@
 \let\xdviColor@@=\xdvi@Color@
 \let\UnloadColor@@=\UnloadColor@
 }
\xydef@\NoXDVIcolordvi@{\xywarning@{%
 Neither colordvi.tex nor colordvi.sty could be found.}%
 \xyBEcolorcheck@}%
\xydef@\xdviCrayola@@{\xdviColor@@\xdviCrayola@}
\xydef@\xdviCrayola@{%
 \let\prevxycolor@=\newxycolor@
 \def\newxyXDVIcolor@##1##2##3{\prevxycolor@{##1}{}{##1}}%
 \let\newxycolor@=\newxyXDVIcolor@
 \installCrayolaColors@
 \let\newxycolor@=\prevxycolor@ }%
\xydef@\xdviPS@@{\xdviPS@}
\xydef@\xdviPS@unload{\UnloadPS@
 \let\UnloadPS@@=\UnloadPS@
 \let\xdviPS@@=\xdviPS@ }
\xydef@\xdviPStypes@{%
 \xyinputorelse@{xyps-ps}{\xydrivernoload@{ps-ps}}%
 \ifx\PSspecial@@\xdviSpecial@\else
 \let\PSspecial@@=\xdviSpecial@
 \let\PSmacro@@=\xdviMacro@
 \let\PSdict@@=\xdviDict@
 \let\PSspecialdict@@=\xdviDict@
 \let\PSraw@@=\xdviRaw@
 \let\PSinclude@@=\xdviInclude@
 \let\xyPSobeylines@@=\obeyXDVIlines@
 \let\xyPScurrpt@@=\xdviCurrpt@@
 \xdvi@@{PostScript}%
 \fi \XYpredict@ }
\xywarnifdefined\xdviSpecial@
\xywarnifdefined\xdviMacro@
\xywarnifdefined\xdviDict@
\xywarnifdefined\xdviInclude@
\xywarnifdefined\xdviRaw@
{\catcode`\"=11 \catcode`\!=11 \catcode`\:=11
 \gdef\xdviSpecial@#1{\special{ps:: SDict begin #1 end}}
 \gdef\xdviMacro@#1{\firstPS@@\special{" {#1}xy}}
 \gdef\xdviDict@#1{\special{! #1}}
 \gdef\xdviInclude@#1{\special{header=#1}}
 \gdef\xdviRaw@#1{\special{ps: SDict begin #1 end}}
\catcode`\^^M=\active
 \gdef\next{\catcode`\^^M=\active \let^^M=\space }}%
\xylet@\obeyXDVIlines@=\next
\xydef@\xdviCurrpt@{\let\xyPScurrpt@@=\xdviCurrpt@@}%
\xydef@\xdviCurrpt@@{\PSraw@@{xyp}}
\xydef@\xdviPS@{\xdviPStypes@ 
 \let\xdviPS@@=\PSspecials@true
 \let\UnloadPS@@=\xdviPS@unload 
 \let\installxyps@@=\relax \installxyps@ }
\xydef@\xdviRotate@@{\xdviRotate@}
\xydef@\xdviRotate@{\xdviPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-r}{\xydrivernoload@{ps-r}}%
 \xdviCurrpt@ \xdviRotScale@ \installPSrotscale@ }%
 \else\DN@{\xydriverfail@{rotations are}UnloadRotate@\relax}\fi
 \next@ }
\xydef@\xdviRotScale@{%
 \def\xyrot@start(##1){{xyct ##1\space xyrs }}%
 \def\xyrot@end{}%
 \def\xyscale@start(##1,##2){{xyct ##1\space##2\space xyss }}%
 \def\xyscale@end{}}
\xydef@\xdviLine@@{\xdviLine@}
\xydef@\xdviLine@{\xdviPStypes@ 
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-l}{\xydrivernoload@{ps-l}}\installPSline@ }%
 \else\DN@{\xydriverfail@{line-widths are}\UnloadLine@\relax}\fi
 \next@ }
\xydef@\xdviFrames@@{\xdviFrames@}
\xydef@\xdviFrames@{\xdviPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-f}{\xydrivernoload@{ps-f}}\installPSframes@ }%
 \else\DN@{\xydriverfail@{frames are}\UnloadFrames@\relax}\fi
 \next@ }
\xydef@\xdviTiles@@{\xdviTiles@}
\xydef@\xdviTiles@{\xdviPStypes@ 
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-t}{\xydrivernoload@{ps-t}}\installPSpatterns@ }%
 \else\DN@{\xydriverfail@{Patterns are}\UnloadPSpatterns@\relax}\fi
 \next@ }
\xydef@\xdviTPIC@@{\xdviTPIC@}
\xydef@\xdviTPIC@{\setupxyTPIC@}
\xyendinput

